Lazily Adapted Constant Kinky Inference for Nonparametric Regression and Model-Reference Adaptive Control

Techniques known as Nonlinear Set Membership prediction, Lipschitz Interpolation or Kinky Inference are approaches to machine learning that utilise presupposed Lipschitz properties to compute inferences over unobserved function values. Provided a bound on the true best Lipschitz constant of the target function is known a priori they offer convergence guarantees as well as bounds around the predictions. Considering a more general setting that builds on Hoelder continuity relative to pseudo-metrics, we propose an online method for estimating the Hoelder constant online from function value observations that possibly are corrupted by bounded observational errors. Utilising this to compute adaptive parameters within a kinky inference rule gives rise to a nonparametric machine learning method, for which we establish strong universal approximation guarantees. That is, we show that our prediction rule can learn any continuous function in the limit of increasingly dense data to within a worst-case error bound that depends on the level of observational uncertainty. We apply our method in the context of nonparametric model-reference adaptive control (MRAC). Across a range of simulated aircraft roll-dynamics and performance metrics our approach outperforms recently proposed alternatives that were based on Gaussian processes and RBF-neural networks. For discrete-time systems, we provide guarantees on the tracking success of our learning-based controllers both for the batch and the online learning setting.

==> content2/Ch_dealing_with_noise.tex <==
\section{Dealing with noise}



\begin{figure}
        \centering
				  \subfigure[$L(0) = L(1)= 5$;$\obserrbnd = 0.5$; $\hestthresh =1$]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/figs/LACKInoise_e_alpha_trueLinit_7tex.pdf}
    \label{fig:LACKInoise1}
  } 	
	 \subfigure[$L(0) =0.01, L(1) = 2.8 $;$\obserrbnd = 0$; $\hestthresh =0$.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/figs/LACKInoise_noe_noalpha_smallLinit_7tex.pdf}
    \label{fig:LACKInoise2}
  } 	
  %
  %\hspace{2cm}
	  \subfigure[$L(0) =0.01, L(1) = 1.76 $;$\obserrbnd = 0.5$; $\hestthresh =1$.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/figs/LACKInoise_e_alpha_smallLinit_7tex.pdf}
    \label{fig:LACKInoise3}
  } 
  				  \subfigure[$L(0) = L(2)= 5$;$\obserrbnd = 0.5$; $\hestthresh =1$.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/figs/LACKInoise_e_alpha_trueLinit_77tex.pdf}
    \label{fig:LACKInoise4}
  } 	
	 \subfigure[$L(0) =0.01, L(2) = 14.9 $;$\obserrbnd= 0$; $\hestthresh =0$.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/figs/LACKInoise_noe_noalpha_smallLinit_77tex.pdf}
    \label{fig:LACKInoise5}
  } 	
  %
  %\hspace{2cm}
	  \subfigure[$L(0) =0.01; L(2)= 3.18$;$\obserrbnd = 0.5$; $\hestthresh =1$.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/figs/LACKInoise_e_alpha_smallLinit_77tex.pdf}
    \label{fig:LACKInoise6}
  } 	
   \caption{LACKI inference on the basis of two noisy data sets 
   $\data_1,\data_2$ with varying parameter settings. Target (blue curve) was $f:x \mapsto 5 \sqrt{\abs x}$ and observational model (magenta curve) $\tilde f: x \mapsto f(x) + \phi_x$ where $\phi_x$ is a uniformly distributed disturbance with $\phi_x \stackrel{i.i.d.}{\sim} \mathcal U(-0.5,0.5),\forall x$. 
  %
   \textbf{1st column:} Initial constant L(0) = 5; assumed obs. error bound $\obserrbnd= 0.5$; $\hestthresh = 2 \obserrbnd=1$. 
   %
   \textbf{2nd column:} Initial constant L(0) = 0.01; assumed obs. error bound $\obserrbnd = 0$; $\hestthresh = 2 \obserrbnd =0$.
   %
   \textbf{3rd column:} Initial constant L(0) = 0.01; assumed obs. error bound $\obserrbnd = 0.5$; $\hestthresh = 2 \obserrbnd =1$.
   %
   \textbf{Top row:} Data set $\data_1$ of size 7. 
   \textbf{Bottom row:} Data set $\data_2$ of size 77.
   In all cases the exponent parameter was set to $\hexp = 0.5$.}
			\label{fig:LACKInoise}
\end{figure}	

\subsection{Uncertain inputs}
So far, we have considered output uncertainty but not input uncertainty. That is, we have assumed that the function values $f(s_i)$ at the sample inputs are uncertain but that query inputs $x$ as well as sample 
inputs $s_i$ are known exactly. However, in many applications this assumption typically is not met. For example, in Sec. \ref{sec:hfeandcontrol}, we will employ KI for learning and controlling dynamic systems.
Here the target functions are state-dependent vector fields and the state measurements often are corrupted by noise (e.g. due to sensor noise or delays) which can affect both training data and query inputs. In the latter case, the controller might query the KI method to predict 
a function value $f(x)$ based on the assumption of the plant being in state $x$ while the plant may in fact be in a different state $x+\delta_x$. We would like to guarantee that our inference over the actual function value still is within the predicted bounds provided the input estimation error $\delta_x$ is known or known to be bounded. 
Fortunately, the H\"older property of the target can help to address the problem of quantifying the prediction error due to input uncertainty. For instance, consider $\metric(x,x') = \norm{x-x'}$. By H\"older continuity, the error of the prediction of the $j$th output component of the target function $f$ is bounded by $\abs{f_j(x+\delta_x) - f_j(x)} \leq \norm{\delta_x}^p$. 

Firstly, assume the training inputs $s_i$ were certain but the query inputs $x$ during prediction are uncertain.
Therefore, assuming we know an upper bound $\errinp(x)$ on the input uncertainty, i.e. 
$\norm{\delta_x}^p\leq \errinp(x), \forall x$, we can add this term to the uncertainty estimate $\prederr(x)$ as per Eq. \ref{eq:KIprederr}.
%This means that the additional uncertainty only affects the prediction of this particular query point. 

Secondly, consider the case were both the sample inputs $s_i$ and the query inputs $x$ are uncertain with the uncertainty being quantified by the function $\errinp(\cdot)$. In this case, the uncertainty of the sample inputs
 affects the posterior hypothesis (i.e. the enclosure) over $f$ and hence, the inferences over function values at all inputs. 
By the same argument as for the case of query noise, we accommodate for this fact leveraging the H\"older property. Instead of adjusting just the prediction uncertainty, we simply add $ \errinp(\cdot)$ to the error function $\varepsilon(\cdot)$ (that we have previously used to model observational 
error of the function values). That is, the observational uncertainty model has absorbed the input uncertainty.  Predictions with uncertain query points can then be done as per Def. \ref{def:KIL} (but with $ \errinp(\cdot)+ \varepsilon(\cdot)$ in place of $\varepsilon(\cdot) )$.

==> content2/Ch_kinkyinf/HoelderNLipcontfacts.tex <==
\section{H\"older and Lipschitz continuity for inference}%\label{sec:HoeldNLipfacts}
\label{sec:Hoelder_brief}
%\subsubsection{Introduction}

 
H\"older continuous functions are uniformly continuous functions that may exhibit infinitely many points of non-differentiability and yet are sufficiently regular to facilitate. That is, they have properties that make it possible to make assertions of global properties on the basis of a finite function sample. 

H\"older continuity is a generalisation of Lipschitz continuity.  Lipschitz properties are widely used in applied mathematics to establish error bounds and, among many other, finds application in optimisation \cite{Shubert:72,direct:93} and quadrature \cite{Baran2008,curbera1998,dereich2006} and is a key property to establish convergence properties of approximation rules in (stochastic) differential equations \cite{kloedenandplaten1992,Gardiner2009}. 

Throughout this thesis, we take advantage on a priori knowledge about H\"older continuity to perform inference.
For instance, in Ch. \ref{ch:contcoll}, we leverage this regularity property to infer the absence of negative function values of a criterion function in the context of collision detection. In Ch. \ref{ch:kinkyinf}, H\"older continuity restricts the posterior hypothesis space of our kinky inference learning method and facilitates learning. 

 Upon submission of this work, we have become aware of related work published in mathematical and operations research journals \cite{Cooper2006,Cooper1995,Zabinsky2003}. For instance, Zabinsky et. al. \cite{Zabinsky2003} consider the problem of estimating a one-dimensional Lipschitz function (with respect to the canonical norm-induced metric). Similar to the analysis we employ to establish our guarantees, they use a pair of bounding functions and make predictions by taking the average of these functions. While we have developed our kinky inference rule independently, it can be seen as a generalisation of their approach. Our method provides extensions to H\"older continuous multi-output functions over general, multi-dimensional (pseudo-) metric spaces, can cope with with erroneous observations and inputs, can fold in additional knowledge about boundedness, learn parameters from data and provide different guarantees such as (uniform) convergence of the prediction uncertainty. 
As part of the analysis of our method (see Ch. \ref{ch:kinkyinf} and Ch. \ref{ch:KIderivations}), we construct bounding functions we refer \textit{ceiling} and \textit{floor} functions. The construction of similar functions is a recurring theme that, in the standard Lipschitz context, can be found in global optimisation \cite{Shubert:72} and quadrature \cite{Baran2008} as well as in the analysis of linear splines for function estimation \cite{Cooper1995}. Cooper \cite{Cooper2006,Cooper1995} utilises such upper and lower bound functions in a multi-dimensional setting to derive probabilistic PAC-type error bounds \cite{Valiant1984} for a linear interpolation rule. He assumes the data is sampled uniformly at random on a hypercube domain. This precludes the application of his results to much of our control applications where the data normally is collected along continuous trajectories visited by a controlled plant. Our inference rule is different from his and our guarantees do not rely on distributional assumptions. Indeed, to fit many contexts of relevance, we have  However, in future work, we would be interested in how far some of Cooper's statistical analysis techniques could be harnessed to translate our own guarantees to stochastic settings.

None of the aforementioned works seems to consider interval-bounded input uncertainty and observational errors, folds in additional knowledge such as boundedness or considers inference over multi-output functions as we do.
Finally, we are not aware of any work that employs these methods in the context of learning in dynamical systems, control or collision avoidance as we do. 

At the bottom line, while it seems that the general idea that is at the heart of our kinky inference framework is not new, our approach offers several novel extensions and generalisations that are important for our 
control and coordination applications. Most importantly for the aims of this thesis, the merger with control will yields a variety of new adaptive controllers with guarantees of boundedness we also believe to be novel.

The remainder of this section is structured as follows. Firstly, we will go over basic definitions and engage in some preliminary derivations that will be of importance throughout the thesis.
Afterwards we will briefly talk about utilising H\"older properties for conservative inference over extrema -- that is, for bounded optimisation. While we do not claim novelty on any of the results we provide proofs for in this section, we had not found them in the literature and hence, had to derive them on our own.
%In particular, we will look into the inference problems of bounded optimisation and quadrature. That is, based on the knowledge of a sample of a H\"older continuous function we will derive upper and lower bounds on its maximum, minimum and definite Riemann integral. In addition we will touch upon adaptive algorithms that can utilise knowledge of the function's H\"older properties to guide exploration. That is, since the regularity of the function allows us to provide interval bounds on the uncertainty of the function, the magnitude of the uncertainty can be a guide to identify regions that are to be sampled next in order to maximise the shrinkage of the provided error bounds. 
%\jcom{The latter is more the 1-dim case, which I may or may not include}\\

\subsubsection{Basic facts and derivations}
Before proceeding, we will establish basic properties of H\"older continuity. 

\begin{defn} 
Let $(\inspace ,\metric_\inspace ), (\outspace , \metric_\outspace )$ be two metric spaces and 
$I \subset \inspace$ be an open set. A function $f: \inspace \to \outspace $ is called (L-p-) \emph{H\"older} 
continuous on $I \subset \inspace$ if there exists a \emph{(H\"older) coefficient} $L[I] \geq 0$ and \emph{(H\"older) 
exponent} $p\geq 0$ such that 
\[\forall x,x' \in I : \metric_\outspace \bigl(f(x),f(x')\bigr) \leq L[I] \, \bigl( \metric_\inspace (x,x') \bigr)^p. \]
We denote the space of all L-p- H\"older functions by $\hoelset L \metric p$.
 \end{defn}
H\"older functions are known to be uniformly continuous. 
A special case of importance is the class of $L$-\textit{Lipschitz} functions. These are H\"older continuous 
functions with exponent $p=1$. In this context, coefficient $L$ is referred to as\textit{ Lipschitz constant} or \textit{Lipschitz number}.

\begin{ex}[Square root function]\label{ex:sqrtfctHoelder}
As an example of a Hoelder function that is not Lipschitz we can consider $x \mapsto \sqrt x$ on domain $I = [0+\epsilon,c]$ where 
$c >\epsilon \geq 0 $. For $\epsilon >0 $ the function is Lipschitz with $L[I] = \sup_{x \in I} \frac{1} {2 \sqrt{x}}$. We can see that the 
coefficient grows infinitely large as $\epsilon \to 0$. By contrast, the function is H\"older continuous 
with H\"older coefficient $L[I]=1$ and exponent $p=\frac 1 2 $ for any bounded $I \subset \Real$.
We can see this as follows: Let $\epsilon =0,$ $x,y \in I$ and, without loss of generality,  $y \geq x$. Let $\xi := \sqrt{x}, \gamma := \sqrt{y}$ and thus, $\gamma \geq \xi$. We have:
$\xi \leq \gamma $ $\Leftrightarrow 2 \xi^2 \leq 2\xi\gamma$ $\Leftrightarrow \gamma^2 - 2 \xi\gamma + \xi^2  \leq \gamma^2 - \xi^2$ $\Leftrightarrow (\gamma-\xi)^2  \leq \gamma^2-\xi^2$ $\Leftrightarrow \abs{\gamma-\xi}^2  \leq \abs{\gamma^2-\xi^2}$
 $\Leftrightarrow \abs{\gamma-\xi}  \leq \sqrt{\abs{\gamma^2-\xi^2}}$  $\Leftrightarrow \abs{\sqrt{x}-\sqrt{y}}  \leq \abs{y-x}^{\frac{1}{2}}$. Since, $x,y$ were chosen arbitrarily, we have shown H\"older continuity as desired.
\end{ex}
 
Most commonly, one considers H\"older continuity for the special case of the standard metric induced by a norm, i.e.  $\metric(x,x') = \norm{x-x'}$.
For a function $f: \inspace \to \outspace$, the H\"older condition becomes:
 \[\forall x,x' \in I : \norm{f(x)-f(x')}_\outspace \leq L[I] \, \norm{x-x'}_\inspace^p. \]

Similarly, we can consider H\"older continuity for each output component: 

\begin{defn} \label{def:outputwisehoelder}
Let $\outspace \subseteq \Real^m $ and $\inspace$ be a space endowed with a metric (or indeed a semi-metric) $\metric_\inspace$. Then, the function $f: \inspace \to \outspace$ is output-component-wise H\"older continuous with exponent $p$ and constant $L \in \Real^m_{\geq 0}$ if $f \in \hoelset L {\metric_\inspace} p$ where
\[\hoelset L {\metric_\inspace} p:= \bigl\{ \phi: \inspace \to \outspace \,\ | \, \forall j \in \{1,...,m \}, \forall x,x' \in \inspace: \abs{\phi_j(x) - \phi_j(x')} \leq L_j \metric_\inspace(x,x') \bigr\}\] 
is the set of all functions whose component functions are H\"older continuous with respect to input space metric $\metric_\inspace$ and an output space metric that is induced by the canonical norm $\metric_{\outspace} (x,x')= \abs{x-x'}$.  
\end{defn}
%
%
%
%\subsection{Hoelder continuity of the maps  $x \mapsto  L \, \metric(x,s)^p$ for $p \in (0,1], s\in I, L \geq 0$}
%
 %
%We endeavor to show that $x \mapsto L \norm{ x -s}^p$ is Hoelder continuous with coefficient $L$ and exponent $p$. This will become important since these functions will serve as essential building blocks of our conservative Hoelder function estimates. 
%
%To this end, we will show that $(x,y) \mapsto \norm{x-y}^p$, for $p \in (0,1] $, is a metric.  This can be utilized to show that
%$x \mapsto \norm{ x -s}^p$ is a Hoelder continuous function.
%
%To establish the metric property, we note that any positive definite function that is subadditive gives rise to a canonical metric. Formally :
%
%
%To prove $(x,y) \mapsto \norm{x-y}^p$ is a metric, we need to establish a few facts. 
%Firstly, we remind ourselves of the following well-known fact:
%\begin{lem} \label{lem:pd_n_concave_subadditive}
 %A nonnegative, concave function $g:\Real_{\geq 0} \to \Real$ with $g(0) = 0$ is subadditive. 
 %That is, $\forall x,y \in \Real_{\geq 0}: g(x+y) \leq g(x) + g(y)$. 
 %
 %\begin{proof}
%If $x = y = 0$ then subadditivity trivally holds:  $0=g(x+y) \leq g(x) + g(y) = 0$.
%So, let $x, y \in \Real_+$ such that $x >0 \vee y >0$.
%We have, $g( x +y) = \frac{x}{x+y} g(x+y) + \frac{y}{x+y} g(x+y) \leq g(\frac{x}{x+y} (x+y) ) +  g(\frac{y}{x+y}(x+y)) = g(x) + g(y)$.
%Taking into account that $\frac{x}{x+y}, \frac{x}{x+y} \in [0,1]$, the last inequality can be seen as follows:
%
 %Since $g$ is concave we have 
%$\forall p \in [0,1], x \in \Real: g(p x) =  g(px + (1-p) 0) \geq p g(x) + (1-p) g(0) \geq p g(x)  $. The last inequality follows from $g(0) \geq 0$.
%\end{proof}
%\end{lem}
%
%\begin{lem} \label{lem:x2p_pdNsubadd}
 %Let $h: \begin{cases} \Real_{\geq 0} \to \Real_{\geq 0},\\ \, x \mapsto x^p\end{cases}$, for $p \in (0,1] $. $h$ is positive definite and subadditive. 
 %That is, (i) $h(0) = 0 $ and  $h(x) > 0, \forall x \neq 0$ and (ii) $\forall x,y \in \Real_{\geq 0}: h(x+y) \leq h(x) + h(y)  $.
 %Moreover, $h$ is concave. If $p \in (0,1)$, h is strictly concave. 
 %
%\begin{proof}
%\textit{Pos. def. :} $h(0) = 0$.  Also $\lim_{x \to 0_+} h(x) =0$. Since $\nabla h (x) = p h^{p-1}(x) >0 $ for $x >0$, $h$ is strictly monotonically increasing on $\Real_+$. Hence, $h(x) > 0, \forall x >0$. 
%
%\textit{Concavity:} If $p =1$, $h$ is linear and hence, concave. If $p \in (0,1)$, $\nabla^2 h(x) = p (p-1) h(x)^{p-2} > 0$ regardless of $x$.
%
%\textit{Subadditivity:} Follows directly with Lem. \ref{lem:pd_n_concave_subadditive} on the basis of established positive definiteness and concavity.
  %
%\end{proof}
%\end{lem}
%
%
%
%\begin{lem}\label{lem:hoeldererror_metric}
%Let $p \in (0,1]$.
%With definitions as in Thm. \ref{thm:subaddmetric1}, we assume that set $G$ is endowed with a quasi- metric $d$. Function
%$\metric: \begin{cases} \inspace \times \inspace \to \Real_{\geq 0} \\ (x,y) \mapsto \Bigl(d(x,y)\Bigr)^p \end{cases}$ is a quasi-metric on $G$.
%If $d$ is a metric then so is $\metric$.
%\begin{proof}
 %By Lem. \ref{lem:x2p_pdNsubadd}, $x\mapsto x^p$ is pos. def. and subadditive. Therefore, positive definiteness and the triangle inequality of $d$ readily extend to $\metric$ as follows: 
%
%\textit{Pos. def.:}
%Let $x=0$. $\metric(x,x) = d(x,x)^p = 0^p = 0$. If $x \neq 0$ then $k :=d(x,x) \neq 0$. Hence   $\metric(x,x) = d(x,x)^p = k^p \neq 0$.
%
%\textit{Triangle inequality:}
%Choose arbitrary $x,y,z \in \inspace $. We have $\metric(x,z) = d(x,z)^p \leq (d(x,y) + d(y,z) \bigr)^p \leq d(x,y)^p + d(y,z)^p = \metric(x,y) + \metric(y,z)$. Here, the first inequality followed from the triangle inequality of quasi-metric $d$ and the second from subadditivity properties established in Lem. \ref{lem:x2p_pdNsubadd}.
%
%\textit{Symmetry:} If $d$ is a metric it is symmetric. Hence, $\metric(x,y) = d(x,y)^p = d(y,x)^p = \metric(y,x), \forall x,y \in \inspace $ in which case $\metric$ also is symmetric.
%\end{proof}
%\end{lem}
%
%Before proceeding we establish a slight generalization of the well-known \textit{reverse triangle inequality}:
%
%\begin{lem}[Reverse Triangle Inequality] \label{thm:revtriangle}
%Let  $\inspace$ be a set and $\metric : \inspace^2 \to \Real$ a symmetric function that fulfills the triangle inequality. 
%That is,  $\forall x,y,z \in \inspace: \metric (x,y) = \metric(y,x) \wedge \metric(x,z) \leq \metric(x,y) + \metric(y,z)$.
%
%Then \[\forall x,y,z \in \inspace: \abs{\metric(x,y) - \metric(z,y)} \leq \metric(x,z).\]
%\begin{proof}
%
%For contradiction, assume 
%$\abs{\metric(x,y) - \metric(z,y)}>\metric(x,z)$ for some $x,y,z \in \inspace$.
%This is implies  
%$
%(i)\,\,\, \metric(x,y) - \metric(z,y)>\metric(x,z) 
%\, \, $  or  $
  %\,\,  (ii) \,\,\,\, \metric(z,y)-\metric(x,y) >\metric(x,z)$.
%Both inequalities contradict the triangle inequality:
%$(i) \Leftrightarrow \metric(x,y)  >\metric(x,z) \metric(z,y) $ and 
%$(ii) \Leftrightarrow  \metric(z,y) > \metric(x,z) + \metric(x,y) =  \metric(z,x) + \metric(x,y)$.
%
%\end{proof}
%\end{lem}
%
%
%\begin{thm}
%Let $\metric$ be a metric on set $G$. For arbitrary $s \in \inspace $ we define $\phi_s: \inspace \to \Real $ as $\phi_s: x \mapsto \metric (x,s) $.
%$\phi_s $ is Lipschitz with respect to metric $\metric$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq \metric (x,y). \]
%\begin{proof}
%$\abs{\phi_s(x) - \phi_s(y)} = \abs{\metric(x,s) - \metric(y,s)} \stackrel{Thm. \ref{thm:revtriangle}} {\leq} \metric(x,y), \forall x,y,s \in \inspace $.
%\end{proof}
%\end{thm}
%Finally, combining this theorem with Lem. \ref{lem:hoeldererror_metric} immediately establishes that mappings of the form $\metric(\cdot,s)^p$ and hence, of the form
%$\norm{\cdot -s}^p$ are Hoelder continuous with exponent $p$ ($\in (0,1]$):
%
%\begin{thm}
%Let $\metric$ be a metric on set $G$ and let $p \in (0,1], L \geq 0$. For arbitrary $s \in \inspace $ we define $\phi_s:\begin{cases}  \inspace \to \Real \\ x \mapsto L \, \bigl(\metric (x,s) \bigr)^p\end{cases}$.
%$\phi_s $ is Hoelder with exponent $p$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq L \, \metric (x,y)^p. \]
%In particular, for any norm $\norm \cdot$ on $G$ and $s \in \inspace $, mapping $x \mapsto L \norm{x-s}^p$ is Hoelder with constant $L$ and exponent $p$.
%\begin{proof}
%By Lem. \ref{lem:hoeldererror_metric}, $\metric(\cdot,\cdot)$ is a metric on $G$. Hence, Lem. \ref{thm:revtriangle} is applicable yielding:
%$\abs{\phi_s(x) - \phi_s(y)} = L \, \abs{\metric(x,s)^p - \metric(y,s)^p} \stackrel{Lem. \ref{thm:revtriangle} } {\leq} \metric(x,y)^p, \forall x,y,s \in \inspace$. The last sentence concerning the norms follows from the fact that a mapping $(x,y) \mapsto \norm{x-y}$ defines a metric.
%\end{proof}
%\end{thm}
%
%
%
 %At first glance, the result may seem intuitive. However, it should be noted that, for $p >1$, $x \mapsto \norm{x -s}^p$ no longer is Hoelder with exponent $p$. This is consistent with the well-known fact that Hoelder functions with exponent $>1$ are constant functions.
%
%We conclude this section by the following theorem stating that any concatenation of Hoelder continuous functions is Hoelder continuous:
%
%\begin{thm} \label{thm:concathoelder}
%Let $(\statespace, \metric)$ be a metric space and $f,g : \statespace \to \statespace$ be two Hoelder continuous mappings with Hoelder constants $L_f, L_g$ and Hoelder exponents $p_f,p_g$, respectively.
%Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also Hoelder continuous with Hoelder constant $L_h:= L_f L_g^{p_f}$ and exponent $p_h:=p_g \, p_f$.
%That is, 
%\[\forall \state,\state' \in \statespace: \metric\bigl(h(\state),h(\state')\bigr) \leq L_h \bigl(\metric(\state,\state')\bigr)^{p_h}.\]
%\begin{proof}
%%\begin{align}
%$\metric\bigl(f \circ g(\state),f\circ g(\state')\bigr) \leq L_f  \Bigl(\metric(g(\state),g(\state'))\Bigr)^{p_f}$
%$\leq L_f  \Bigl(L_g \metric(\state,\state')^{p_g}\Bigr)^{p_f}$ $= L_f L_g^{p_f}   \Bigl(\metric(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using Hoelder continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
%
%\end{proof}
%\end{thm} 
%In conjunction with Hoelder properties of the square root function established in Ex. \ref{ex:sqrtfctHoelder}, Thm. 
%\ref{thm:concathoelder} immediately yields the following result:
%\begin{cor}
%If $f: \statespace \to \statespace $ is Hoelder continuous with constant $L_f$ and exponent $p_f$ then $\sqrt{f}$ also is Hoelder, having  Hoelder constant $\sqrt{L_f}$ and exponent $p_f$.
%\end{cor}


\begin{thm} \label{thm:hoelderconcat}
Let $(\statespace, \d)$ be a metric space and $f,g : \statespace \to \statespace$ be two H\"older continuous mappings with H\"older constants $L(f), L(g)$ and H\"older exponents $p_f,p_g$, respectively.
Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also H\"older continuous with H\"older constant $L(h):= L(f) L(g)^{p_f}$ and exponent $p_h:=p_g \, p_f$.
That is, 
\[\forall \state,\state' \in \statespace: \d\bigl(h(\state),h(\state')\bigr) \leq L(h) \, \bigl(\d(\state,\state')\bigr)^{p_h}.\]
\begin{proof}
%\begin{align}
$\d\bigl(f \circ g(\state),f\circ g(\state')\bigr)$ $\leq L(f)\,  \Bigl(\d(g(\state),g(\state'))\Bigr)^{p_f}$
$\leq L(f)\,  \Bigl(L(g)\, \d(\state,\state')^{p_g}\Bigr)^{p_f}$ 

$= L(f)\, L(g)\,^{p_f}   \Bigl(\d(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using H\"older continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
\end{proof}
\end{thm} 


%A special case of Hoelder continuity is Lipschitz continuity. A Lipschitz continuous function is Hoelder continuous with exponent 1.
%If the metric space is $(\Real,(x,y) \mapsto \abs{x-y})$, $f$ is Lipschitz with constant $L(f)$ if $\forall t,t': \abs{f(t)-f(t')} \leq L(f) \, \abs{t-t'}$. 

Several numerical methods, such as Lipschitz optimisation \cite{Shubert:72}, rely on the knowledge of a Lipschitz constant. In the more general case of H\"older continuous functions this will correspond to the need of knowing a H\"older constant and exponent. To avoid having to derive these for each new function from first principles, we establish the following collection of facts that allows us determine bounds on H\"older constants of combinations of functions with known H\"older parameters.
While we provide proofs for a restatement in the H\"older continuous setting, a number of the following statements have also been proven in \cite{Weaver1999} in the context of Lipschitz algebras.



%\begin{lem}[Lipschitz arithmetic] \label{lem:Liparithmetic}
%Let, $I,J \subset \Real_+$. Let $f : \Real \to \Real$ be Lipschitz on $I$ with Lipschitz number $L_I (f)$ 
%and $g :\Real \to \Real$ be Lipschitz on $J$ with Lipschitz number $L_J (g)$.
%We have:
%
%
%
%
%\begin{enumerate}
	%\item Mapping $t \mapsto |f(t)|$ is Lipschitz on $I$ with constant $L_I(f)$.
	%\item If $g$ is Lipschitz on all of $J=f(I)$ the concatenation $g \circ f: t \mapsto g(f(t))$ is Lipschitz on $I$ with Lipschitz constant 
	      %$L_I(g \circ f) \leq$ $L_J (g) \, L_I(f)$.
	%\item Let $r \in \Real$. $r \, f: x \mapsto r \, f(x)$ is Lipschitz on $I$ having a Lipschitz constant $L_I (r \,f) = |r| \, L_I(f)$.
	%\item $f+g: t \mapsto f(t) + g(t)$ has Lipschitz number at most $L_I(f) + L_J(g)$.
	%\item Let $m_f = \sup_{t\in \indset } f(t)$ and $m_g = \sup_{t\in \indset } g(t)$. Product function $f\cdot g: x \mapsto f(x) \, g(x)$ has a Lipschitz number on $I$ which is at most $(m_f \, L_J(g)+ m_g \, L_I(f))$.
	%\item Let $h(t) = \max\{f(t), g(t) \}, \forall t \in \indset  \cap J$. We have $L_{I \cap J}(h) = \max\{L_I(f),L_J(g)\}$.
	%\item Let $b := \inf_{t \in \indset }| f(t)| > 0$ and let 
	%$\phi(t) = \frac{1}{f(t)}, \forall t \in \indset $.  
	      %Then $L_I(\phi) \leq b^{-2} \, L_I(f)$ on $I$.  
	%\item $f$ cont. differentiable on I $\Rightarrow$ $L_I(f) = \sup_{t \in \indset } |\dot f(t)|. $ 
	 %\item Let $c \in \Real$, $f( t) = c, \forall t \in \indset $. Then $L_I(f) =0$.  
	%\item $L_I(f^2) \leq 2 \, s(f)\, L_I(f)$.
	%\item $f$ cont. differentiable $\Rightarrow \forall q \in \mathbb Q : L_I(f^q) = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $.
%\end{enumerate}
%\begin{proof}
%
%\textbf{1)}  We show $|f|$ has the same Lipschitz number as $f$. Let $t,t' \in \indset $ arbitrary. 
%We enter a case differentiation:
%
%\textit{1st case: $f(t), f(t') \geq 0$}. 
%
%Hence, $\bigl| |f(t)| - |f(t')| \bigr| = \bigl| f(t) - f(t') \bigr|  \stackrel{f \, Lipschitz}{\leq} L_I(f) |t-t'|$.\\
%
%\textit{2nd case: $f(t) \geq 0, f(t') \leq 0$.} 
%
%Note, $|y| = - y$, iff $y \leq 0$. Hence,  $\bigl| |f(t)| - |f(t')| \bigr| \leq \bigl| |f(t)| + |f(t')| \bigr| $
%$= \bigl| |f(t)| - f(t') \bigr|  =  \bigl| f(t) - f(t') \bigr| \leq L_I(f) \, |t-t'|$.\\
%
%\textit{3rd case: $f(t) \leq 0, f(t') \geq 0$.} Completely analogous to the second case.\\
%
%\textit{4th case: $f(t), f(t') \leq 0$}. 
%
%$\bigl| |f(t)| - |f(t')| \bigr| = \bigl| f(t') - f(t) \bigr|= \bigl| f(t) - f(t') \bigr|  \stackrel{f \, Lipschitz}{\leq} L_I(f) |t-t'|$.\\
%
%The remaining points are proven in \cite{Weaver1999}.
%\textbf{2)}  For arbitrary $t,t' \in \indset $ we have:
%
%$\bigl| g(f(t)) - g(f(t'))| \bigr| \leq L_J(g) \, |f(t) - f(t') | \leq L_J(g) \, L_I(f)\, |t-t'|$ 
%where the two inequalities are due to the Lipschitz properties of $g$ and $f$, respectively.\\
%
%\textbf{3)}  For arbitrary $t,t' \in \indset , r \in \Real$ we have:
%
%$\bigl| r \, f(t) - r \, f(t')| \bigr| = |r|\, |f(t) - f(t')| \leq |r| \,L_I(f)\,  |t-t'|$.\\ 
%
%\textbf{4)}  For arbitrary $t,t' \in \indset , r \in \Real$ we have:
%
%$\bigl| g(t) + f(t) - (g(t') + f(t'))| \bigr| = \bigl| g(t)  - g(t') + f(t)- f(t')| \bigr|$ 
%$\leq \bigl| g(t)  - g(t')\bigr|  + \bigl| f(t)- f(t')| \bigr|$ $\leq (L_J(g)+L_I(f))\,  |t-t'|$.\\
%
%\textbf{5)}  Let  $t,t' \in \indset $, $d := f(t) - f(t')$.
%
%$\bigl| g(t) f(t) - g(t')  f(t') \bigr| = \bigl| g(t) (f(t') +d) - g(t') f(t') \bigr|$ 
%$= \bigl|\bigl( g(t) - g(t') \bigl)  f(t')+ g(t)  d \bigr|  $
%$\leq \bigl| g(t) - g(t') \bigr|  |f(t')|   + \bigl|g(t)\bigr| \,  |d|  $
%$\leq L_I(g) |t-t'|  |f(t')|   + \bigl|g(t)\bigr| \,  L_I(f) |t-t'|  $
%$\leq L_I(g) |t-t'|  \sup_{t' \in \indset } \{|f(t')|\}   + \sup_{t \in \indset }\{\bigl|g(t)\bigr|\} \,  L_I(f) |t-t'|  $
%$= \Bigl(L_I(g)  \sup_{t' \in \indset } \{|f(t')|\}   + \sup_{t \in \indset }\{\bigl|g(t)\bigr|\} \,  L_I(f)\Bigl) |t-t'|  $.\\
%
%\textbf{6)}  Proof in "` Nick Weaver, Lipschitz algebras"'.
%
%\textbf{7)}  Let  $t,t' \in \indset $.
%$\bigl| \frac{1}{f(t)} - \frac{1}{f(t')} \bigr|$ 
%$=\bigl| \frac{f(t')}{f(t') f(t)} -\frac{f(t)}{f(t') f(t)} \bigr|$ 
%$= \frac{\bigl|f(t')-f(t) \bigr|}{\bigl|f(t')\bigr| \bigr| f(t)\bigr|}$ 
%$\leq \frac{L_I(f) |t-t'|}{\inf_{t \in \indset } |f(t)|}$.\\
%
%\textbf{8)} Define $\ell := \sup_{t \in \indset } | \dot f(t) | = L_I(f)$. In two steps, we show that $\ell$ is the smallest Lipschitz constant.
%
%Firstly, we show that it is a Lipschitz constant: Let $t,t' \in \indset , t < t'$. Due to the mean value theorem $\exists \xi \in [t,t'] \subset I: \frac{|f(t) - f(t')|}{|t-t'|} = | \dot f (\xi) | \leq \ell$. 
%Secondly, we show that $\ell$ is the smallest Lipschitz constant: Let $\bar \ell$ be another Lipschitz constant such that $\bar \ell \leq \ell$. Since $I$ is compact and $\dot f$ is continuous there is some $\xi \in \indset $ such that $\dot f(\xi) = \ell$. Pick any sequence $(t_k)_{k=1}^\infty$ such that $t_k \stackrel{k \to \infty}{\longrightarrow} \xi$.
%$\forall k: t_k \in \indset $ and $\bar \ell$ is a Lipschitz constant on $I$. Hence, $ \bar \ell \geq \frac{|f(t_k) - f(\xi)|}{|t_k-\xi|}\stackrel{k \to \infty}{\longrightarrow} | \dot f(\xi)| = \ell$. Thus, $\bar \ell = \ell$.\\
  %
%
%
%\textbf{9)} Immediate consequence of 8).\\
%
%\textbf{10)} $L(f^2) = L(f \, f) \leq s(f) L(f) + L(f) s(f)$ where the last inequality follows from property 5).
%
%\textbf{11)} $L(f^q) \stackrel{8)}{=} \sup_{\tau \in \indset } |\dif{}{t} f^q(\tau)| = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $. 
%
%\end{proof}
%\end{lem} 


\begin{lem}[H\"older arithmetic] \label{lem:Hoeldarithmetic}
Let, $I,J \subset \inspace$ where $\inspace$ is a metric space endowed with metric $\metric$. Let $f : \inspace \to \Real$ be H\"older on $I$ with constant number $L_I (f)$ 
and $g :\inspace \to \Real$ be H\"older on $J$ with constant $L_J (g)$. Assume both functions have the same H\"older exponent $p \in (0,1]$. That is, $\forall x, x' \in \inspace: \abs{f(x)-f(x')} \leq L(f) \metric(x,x')^p$ and  $\forall x, x' \in \inspace: \abs{g(x)-g(x')} \leq L(g)  \metric(x,x')^p$.
We have:

\begin{enumerate}
	\item Mapping $x \mapsto |f(x)|$ is H\"older on $I$ with constant $L_I(f)$ and exponent $p_f$.
	\item If $g$ is H\"older on all of $J=f(I)$ the concatenation $g \circ f: t \mapsto g(f(t))$ is H\"older on $I$ with constant 
	      $L_I(g \circ f) \leq$ $L_J (g) \, L_I^p(f)$ and exponent $p^2$.
	\item Let $r \in \Real$. $r \, f: x \mapsto r \, f(x)$ is H\"older on $I$ having a constant $L_I (r \,f) = |r| \, L_I(f)$.
	\item $f+g: x \mapsto f(x) + g(x)$ has H\"older constant at most $L_I(f) + L_J(g)$.
	\item Let $m_f = \sup_{x\in \inspace } f(x)$ and $m_g = \sup_{x \in \inspace } g(x)$. Product function $f\cdot g: x \mapsto f(x) \, g(x)$ has H\"older exponent $p$ and a H\"older constant on $I$ which is at most $(m_f \, L_J(g)+ m_g \, L_I(f))$.
	%\item Let $\tilde h(x) = \min\{f(x),g(x) \}$, $h(x) = \max\{f(x), g(x) \}, \forall x \in \inspace  \cap J$. We have $L_{I \cap J}(h) \leq \max\{L_I(f),L_J(g)\}$ and $L_{I \cap J}(\tilde h) \leq \max\{L_I(f),L_J(g)\}$.	
	\item For some countable index set $\indsett$, let the sequence of functions $f_i$ be H\"older with exponent $p$ and constant $L(f_i)$ each. Furthermore, let $H(x) =\sup_{i \in \indsett} f_i(x) $ and $h(x) := \inf_{i \in \indsett} f_i(x)$ be finite for all $x$. Then $H,h$ are also H\"older with exponent $p$ and have a H\"older constant which is at most $\sup_{i \in \indsett} L(f_i)$.
	\item Let $b := \inf_{x \in \inspace }| f(x)| > 0$ and let 
	$\phi(x) = \frac{1}{f(x)}, \forall x \in \inspace$ be well-defined.  
	      Then $L_I(\phi) \leq b^{-2} \, L_I(f)$.  
	\item Let $p=1$ (that is we consider the Lipschitz case), let $I$ be convex and $\metric(x,x') = \norm{x-x'}$. $f$ cont. differentiable on I $\Rightarrow$ $L_I(f) \leq \sup_{x \in I } \norm{\nabla f(x)}. $ 
	For one-dimensional input space, $\inspace = \Real$, $L_I(f) = \sup_{x \in I } \abs{\nabla f(x)}$ is the smallest Lipschitz number. 
	 \item Let $c \in \Real$, $f( t) = c, \forall x \in I $. Then $f$ is H\"older continuous with constant $L_I(f) =0$ and for any coefficient $p_f \in \Real$.  
	\item $L_I(f^2) \leq 2 \, L_I(f)\, \sup_{t \in I} f\,$.
	\item With conditions as in 8), and input space dimension one, we have $\forall q \in \mathbb Q : L_I(f^q) = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $.
\end{enumerate}
\begin{proof}

\textbf{1)}  We show $|f|$ has the same constant and exponent as $f$. Let $X,X' \in \inspace $ arbitrary. 
We enter a case differentiation:

\textit{1st case: $f(x), f(x') \geq 0$}. 

Hence, $\bigl| \abs{f(x)}- \abs{f(x')} \bigr| = \bigl| f(x) - f(x') \bigr|  \stackrel{f \,Hoelder}{\leq} L_I(f) \metric(x,x')^{p}$.\\

\textit{2nd case: $f(x) \geq 0, f(x') \leq 0$.} 

Note, $|y| = - y$, iff $y \leq 0$. Hence,  $\bigl| |f(x)| - |f(x')| \bigr| \leq \bigl| |f(x)| + |f(x')| \bigr| $
$= \bigl| |f(x)| - f(x') \bigr|  =  \bigl| f(x) - f(x') \bigr| \leq L_I(f) \, \metric(x,x')^{p}$.\\

\textit{3rd case: $f(x) \leq 0, f(x') \geq 0$.} Completely analogous to the second case.\\

\textit{4th case: $f(x), f(x') \leq 0$}. 

$\bigl| |f(x)| - |f(x')| \bigr| = \bigl| f(x') - f(x) \bigr|= \bigl| f(x) - f(x') \bigr|  \stackrel{f \, Hoelder}{\leq} L_I(f) \metric(x,x')^{p}$.\\

The remaining points are also proven in \cite{Weaver1999} in the context of Lipschitz functions.

\textbf{2)} Special case of Thm. \ref{thm:hoelderconcat}.
% For arbitrary $t,t' \in \indset $ we have:
%
%$\bigl| g(f(t)) - g(f(t'))| \bigr| \leq L_J(g) \, |f(t) - f(t') | \leq L_J(g) \, L_I(f)\, |t-t'|$ 
%where the two inequalities are due to the Lipschitz properties of $g$ and $f$, respectively.\\

\textbf{3)}  For arbitrary $x,x' \in \inspace , r \in \Real$ we have:

$\bigl| r \, f(x) - r \, f(x')| \bigr| = |r|\, |f(x) - f(x')| \leq |r| \,L_I(f)\,  \metric(x,x')^{p}$.\\ 

\textbf{4)}  For arbitrary $x,x' \in \inspace , r \in \Real$ we have:

$\bigl| g(x) + f(x) - (g(x') + f(x'))| \bigr| = \bigl| g(x)  - g(x') + f(x)- f(x')| \bigr|$ 
$\leq \bigl| g(x)  - g(x')\bigr|  + \bigl| f(x)- f(x')| \bigr|$ $\leq (L_J(g)+L_I(f))\,  \metric(x,x')^{p}$.\\

\textbf{5)}  Let  $x,x' \in \inspace $, $d := f(t) - f(t')$.

$\bigl| g(x) f(x) - g(x')  f(x') \bigr| = \bigl| g(x) (f(x') +d) - g(x') f(x') \bigr|$ 
$= \bigl|\bigl( g(x) - g(x') \bigl)  f(x')+ g(x)  d \bigr|  $

$\leq \bigl| g(x) - g(x') \bigr|  |f(x')|   + \bigl|g(x)\bigr| \,  |d|  $
$\leq L_I(g) \metric(x,x')^p  |f(x')|   + \bigl|g(x)\bigr| \,  L_I(f) \metric(x,x')^p  $

$\leq L_I(g) \metric(x,x')^p  \sup_{x' \in \inspace } \{|f(x')|\}   + \sup_{x \in \inspace }\{\bigl|g(x)\bigr|\} \,  L_I(f) \metric(x,x')^p  $

$= \Bigl(L_I(g)  \sup_{x' \in \inspace } \{|f(x')|\}   + \sup_{x \in \inspace }\{\bigl|g(x)\bigr|\} \,  L_I(f)\Bigl) \metric(x,x')^p  $.\\

\textbf{6)}  The proof of Proposition 1.5.5 in \cite{Weaver1999} proves our statement if one replaces their 
metric $\rho$ by $\metric^p$.

\textbf{7)}  Let  $x,x' \in \inspace $.
$\bigl| \frac{1}{f(x)} - \frac{1}{f(x')} \bigr|$ 
$=\bigl| \frac{f(x')}{f(x') f(x)} -\frac{f(x)}{f(x') f(x)} \bigr|$ 
$= \frac{\bigl|f(x')-f(x) \bigr|}{\bigl|f(x')\bigr| \bigr| f(x)\bigr|}$ 
$\leq \frac{L_I(f) \metric(x,x')^p}{\inf_{x \in \inspace } |f(x)|^2}$.\\

\textbf{8)} Let $p=1$ and $\metric(x,x') = \norm{x-x'}$ be the standard norm. Define $\ell := \sup_{x \in I } \norm{ \nabla f(x) } = L_I(f)$. 
Firstly, we show that it is a Lipschitz constant: Let $x,x' \in I $ and 
$\overline{xx'} := \{tx + (1-t) x' \, | \, t \in [0,1]\}$. 
%$\overline{xx'} := \{y | \exists t \in [0,1] : y = tx + (1-t) x'\}$. 
Owing to convexity of I, $\overline{xx'} \subset I$. Due to the mean value theorem $\exists \xi \in \overline{xx'} \subset I: |f(x) - f(x')|=  T_\xi (x-x')$. where $T_\xi (x) = \SP{\nabla f(\xi)}{ x}$ is a linear OP. Assuming the derivative of $f$ is bounded, $T_\xi$ is a bounded OP and we have $\abs{T_\xi (x-x') } \leq \matnorm{T_\xi} \norm{x-x'}$ where 
$\matnorm{T_\xi} = \sup_{\norm{x} = 1} \SP{\nabla f(\xi)}{x} \leq \norm{\nabla f(\xi)}$. In conjunction,
$|f(x) - f(x')| \leq \norm{\nabla f(\xi)} \norm{x-x'}$. 

Secondly, we show that $\ell$ is the smallest Lipschitz constant in the one-dimensional case: Let $\bar \ell$ be another Lipschitz constant on $I$ such that $\bar \ell \leq \ell$. Of course, here $\norm{\cdot} = \abs{\cdot}$. Since $I$ is compact and $\norm{\nabla f(\cdot) }$ is continuous, there is some $\xi \in I$ such that $\norm{\nabla f(\xi)} = \sup_{x \in I} \norm{\nabla f(\xi)} = \ell$. Pick any sequence $(y_k)_{k=1}^\infty$ contained in $I$ such that $y_k \stackrel{k \to \infty}{\longrightarrow} \xi$ and $y_k \neq \xi$.
$\forall k: y_k \in I $ and $\bar \ell$ is a Lipschitz constant on $I$. Hence, $ \bar \ell \geq \frac{|f(y_k) - f(\xi)|}{\norm{y_k-\xi}}\stackrel{k \to \infty}{\longrightarrow} \norm{ \nabla f(\xi)} = \ell$. Thus, $\bar \ell = \ell$.

\textbf{9)} Trivial. 

\textbf{10)} Special case of property 5).

\textbf{11)} $L(f^q) \stackrel{8)}{=} \sup_{\tau \in \indset } |\dif{}{t} f^q(\tau)| = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $. 

\end{proof}
\end{lem} 

As a simple illustration, assume we desire to establish that $f(t) = \max\{ 1- 3 \sin(t), \exp\bigl(- \sin(t) \bigr)\}$ is Lipschitz and to find a Lipschitz number on $\Real$. Application of 8. shows that $t \mapsto \sin(t)$ and $t \mapsto \exp(- t)$ have a Lipschitz number of $1$. Application, of 2., 9. 1. and 6. then show that $L(f) =3$ is a Lipschitz number of $f$.


An example that will be of relevance to our collision avoidance applications in Ch. \ref{ch:contcoll} is the following:
\begin{ex} \label{ex:hoelderOUstd}
Consider the function $h(t) = f \circ g(t)$ where $f(\cdot) = \sqrt \cdot$ is the square root function and $g(t) = \frac{B^2}{2 K} (1- \fexp{-2Kt}) $, $K >0$. $g$ is the non-stationary factor of the variance trajectory of an Ornstein-Uhlenbeck process (cf. Sec. \ref{sec:OUprocess}). We show that $h$ is H\"older and has constant $L(h)= \sqrt{2K}$ and H\"older exponent $p_h = \frac 1 2$. This can be easily done by applying Lem. \ref{lem:Hoeldarithmetic}.8 to show that $L(g)$ is Lipschitz with constant $L(g) = B^2 $ and then combining the H\"older constant and exponent derived in Ex. \ref{ex:sqrtfctHoelder} with Thm. \ref{thm:hoelderconcat} to yield the H\"older exponent $p_h = p_g p_f = \frac 1 2$ and constant $L(h) = 1 \sqrt{L(g)}  = \abs B$.  
\end{ex}



==> content2/Ch_kinkyinf/KIMPCcollavoid.tex <==
\begin{figure*}[ht!]
        \centering
				  \subfigure[Open-loop plan.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt1_plan1}
    \label{fig:akt1fig1}
  } 	 
					  \subfigure[Planned trajectory.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt1_plan1traj}
    \label{fig:akt1fig2}
  } 	  
					  \subfigure[Actual trajectory.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt1_exec1traj}
    \label{fig:akt1fig3}
  } 	 
%
   \caption{\textit{Exp1.} The leftmost plot shows the plans of agent 1 (blue) and agent 2 (green). The boxes depict the safety tube bounding the error whereas the circles indicate the physical expansion of the circular agents. Their start positions are $S1 = (-5,0)^\top$ and $S2 = (5,0)^\top$ while their goal locations are $G1 = (-1,0)^\top$ and $G2 = (1,0)^\top$, respectively. With the agents having a radius of $r=0.5$ and not assuming any disturbances, the planner computes control actions that are projected to allow the agents to come to rest at their goal locations (see Fig. \ref{fig:akt1fig2} and Fig \ref{fig:akt1fig2}). However, when the plans are executed in the real system, the unforeseen drift $f$ causes the trajectories to collide when the plans are executed (Fig. \ref{fig:akt1fig3}).  }
		\label{fig:KIcollavoidopenloopakt1}
\end{figure*}	
%
\section{Application to collision avoidance of learning agents with uncertain drift}
\label{sec:KIcollavoiddiscretetime}
%\textbf{Overview.} 

Due to its mathematical properties, optimal multi-agent planning with collision avoidance is a hard coordination problem \cite{lavallebook:2006}. In the context of model-predictive control (MPC) \cite{Jmacmpcbook2002}, it is typically modelled as a finite-time horizon problem and stated as a \textit{mixed integer linear programme (MILP)} (e.g. \cite{schouwenaars2001mixed,Kuwata2005,Kuwata2006,LyonsACC2012,Lyons2011}). In robust predictive control, it is assumed that the agents are governed by control-affine dynamics up to some error whose norm is bounded \cite{Kuwata2005,Kuwata2006}. This gives rise to a \textit{tube} of conceivable trajectories around an error-free \textit{nominal} trajectory whose expansion (i.e. tube radius) reflects the maximum error norm. Collision avoidance can be enforced by adding constraints to the statement of the optimisation problem that ensure that the tubes cannot overlap.

In this section, we connect this planning approach to our kinky inference method. Here, the error is due to epistemic uncertainty over the governing dynamics. 
In particular, we will assume that the drift of the system is uncertain. The drift then is (partially) inferred from observations employing kinky inference. Folding in information about the drift afforded by the partially identified model, the agents are controlled with a variation of the optimisation-based open-loop MPC approach considered in \cite{LyonsACC2012,Lyons2011}. Taking the uncertainty estimates around the KI predictions into account, collision avoidance is ensured by constraints on the tube distances around the uncertain trajectories. In contrast to \cite{LyonsACC2012,Lyons2011} the size of the tubes is chiefly determined by the uncertainty quantification provided by the kinky inference rule. Assuming the prior assumptions are true and the drift is contained in $\mathcal K_{prior}$ (cf. Sec. \ref{sec:KI_core}), Thm. \ref{thm:KIdesiderata} asserts that the resulting controls will be conservative. That is, as long as we ensure the tubes do not intersect, the actual trajectories are guaranteed not to intersect. In addition, the theorem guarantees that the conservatism will shrink as additional data about the drift will become available. 

Below, we will provide illustrations of the application of these results to the multi-agent collision avoidance problem. The simulations behave as predicted by our theory. 
There are numerous works in the control literature that give guarantees on control success in a robust setting as well as a vast number of works on multi-agent 
coordination and collision avoidance (e.g. \cite{schouwenaars2001mixed,Kuwata2005,Kuwata2006,Ong2010,LyonsACC2012,calliessARMS2011:LNAI}). Nonetheless, we believe this to be the first work that can provide guarantees on the belief of collision avoidance that is due to bounds of learning algorithms that have identified an uncertain dynamic system.

\subsection{Conservative predictive control for collision avoidance of kinky inference learners}


Suppose we have $A$ agents with index set $\agset, \abs{\agset}=A$. Each agent $\agi \in \agset$ has plant dynamics 
\begin{equation}
	x^\agi[{k+1}] = A x^\agi[k] + B u^\agi[k] + f(x^\agi[k])
\end{equation}
with matrices as defined in the double-integrator UAV model considered in \cite{LyonsACC2012}. 
Here, $x^\agi[k]$ denotes the state of agent $\agi$ at discrete time $k \in \{1,...,T\}$ and $u^\agi[k]$ is the pertaining control action chosen by the agent.
%That is, we chose 
%\begin{footnotesize}
%\begin{align}
		%A = \left(\begin{array}[h]{cccc}
				%1 & 0&\tinc&0\\
				%0 & 1&0&\tinc\\
				%0 & 0&1&0\\
				%0 & 0&0&1
		%\end{array}\right), \, & 
			%B = \left(\begin{array}[h]{cc}
				%0& 0\\
				%0 & 0\\
				%\tinc & 0\\
				%0 & \tinc
		%\end{array}\right)
%\end{align}
%\end{footnotesize}
%
%where $\tinc = 0.2$ was a predefined time increment representing the temporal discretisation resolution of the discrete-time approximation of the dynamics.


 
\begin{figure*}
        \centering
				  \subfigure[Open-loop plan.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt2_plan1}
    \label{fig:akt2fig1}
  } 	 
					  \subfigure[Planned trajectory.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt2_plan1traj}
    \label{fig:akt2fig2}
  } 	  
					  \subfigure[Actual trajectory.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt2_exec1traj}
    \label{fig:akt2fig3}
  } 	 
	%
   \caption{Exp2. Taking into account the conservative uncertainty bounds of the kinky inference predictions, the decisions (control actions) are conservative and hence, collisions are avoided during plan execution (Fig. \ref{fig:akt2fig3}) according to plan (Fig. \ref{fig:akt2fig1} and Fig. \ref{fig:akt2fig2}). Due to the poorly trained predictor the uncertainty is large and the plans are so conservative the goals are never reached. }
	\label{fig:KIcollavoidopenloopakt2}
\end{figure*}	 


As before, $f$ is an (uncertain or unknown) drift, $x^\agi[k] \in \statespace \subset \Real^4$ denotes the state at time step $k$ and $u^\agi[k]$ is the pertaining control input to be determined by the planner. In our collision avoidance scenario interactions between agents take place on a map of locations $\iaspace = [-10,10]^2 \subset \Real^2$. We assume the first two components of the state are locations and the final two are the pertaining velocities.
A collision is the event where the plant locations of two agents get too close to each other, which is to be avoided. Formally, a collision is considered to occur if $\exists k \in \nat, \agi, \agii \in \agset: \norm{\isv^\agi[k] - \isv^\agii[k]} \leq \Lambda$ where $\Lambda \in \Real_+$ is the agents' physical radius and $s^\agi = (x_1^\agi,x_2^\agi)^\top \in \iaspace$ is agent $\agi$'s interaction-space positions, i.e. its location in the environment given by a (bounded) set of attainable locations $\iaspace$.
 
\textbf{Exp. 1.}
In predictive control, a correct model can be crucial for control success \cite{Jmacmpcbook2002}. This holds true especially in open-loop control where no feedback is provided to reduce the effects of model uncertainty. As an illustration, consider the plots of Fig. \ref{fig:KIcollavoidopenloopakt1}. Here, two agents were tasked to move from their start locations to their respective goal locations. Assuming our linear double-integrator model in the absence of a nonlinear drift ($f \equiv 0$), they plan 
to generate control sequences $( u^\agi[k])_{k=1,...,T}$ offline (by solving aforementioned optimisation problem similar to \cite{Lyons2011}) so that the resulting trajectories are anticipated to lead the agents' plants to settle at their respective goal locations $G1 = (-1,0)^\top$ and $G2 = (1,0)^\top$ in a cost-optimal manner. 

We then simulated the trajectories resulting from executing the planned control sequences. However, deviating from the control-affine model utilised during planning, we set the drift function to the non-zero function $f(x) := f^\agi(x) := \tinc \bigl(0,0, - \sin(0.5\, x_1), - \sin(0.5 \, x_2) \bigr)$ for all agents $\agi \in \agset =\{1,2\}$.  In the context of mobile robot control, the drift function might simulate gravitational terms due to an a priori uncertain hilly terrain that has a valley around the origin. (That is, the gravitational forces are proportional to the slope of the terrain. So, with this choice of drift forces pushing towards the origin in a neighbourhood of the origin, this corresponds to a valley being located at the origin.) 

Since the influence of the drift $f$ was unaccounted for during planning, the actual trajectories (Fig. \ref{fig:akt1fig3}), resulting from executing the plans, markedly deviated from the anticipated ones (Fig. \ref{fig:akt1fig2}), yielding a collision around time step $k = 12$ (refer to Fig. \ref{fig:akt1fig3}).  

 

\begin{figure*}
        \centering
				  \subfigure[Open-loop plan.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt3_plan1}
    \label{fig:akt3fig1}
  } 	 
					  \subfigure[Planned trajectory.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt3_plan1traj}
    \label{fig:akt3fig2}
  } 	  
					  \subfigure[Actual trajectory after plan execution.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.5cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt3_exec1traj}
    \label{fig:akt3fig3}
  } 	 
%
   \caption{\textit{Exp3.} The simulation is restarted, but with a KI given 100 randomised, noisy observations of the drift resulting in reduced uncertainty bounds (compare the box size in Fig. \ref{fig:akt3fig1} against those in Fig. \ref{fig:akt2fig1}). This reduces the conservatism of the plans markedly (Fig. \ref{fig:akt3fig1} and Fig. \ref{fig:akt3fig2}). With the adaptive element being well trained to compensate for the drift, the executed trajectories match the planned trajectories closely. The reduced conservatism allows the trajectories to arrive close to their goals. }
	%to be reached, before the growing uncertainty bounds cause the green agent to slowly withdraw.   }
		\label{fig:KIcollavoidopenloopakt3}
\end{figure*}	 
%
\textbf{Exp. 2.} 
To compensate for this, we employed a kinky inference learner to infer the drift based on a noisy sample. The latter could be obtained via observing state differences $\d x[k] = x[k+1] - x[k]$ and then solving for $f(x[k]) = \d x[k
] - A x[k] + B u[k]$. Assuming the state is observable up to error $\varepsilon_x$ this allows us to generate a data set of the form $\data_n = \bigl\{ x[k_i], f(x[k_i]), \varepsilon\bigr \vert i=1, \ldots, N_n\}$ where $\varepsilon$ captures the effects of input and output noise as discussed above.


We initialised the KI learner with one training point for the drift value at each agent's start location in interaction space $\iaspace = [-10,10]^2$, perturbed by some noise of $\varepsilon = 0.01$. That is, with notation of Sec. \ref{sec:KI_core}, we generated
 a data set $\data_1 = \{ (S1, f(S1), 0.01), (S2, f(S2), 0.01)  \}$. The parameters were chosen to $L=1,p=1,\ubf = \infty, \lbf = -\infty$. Appealing to arguments of maximal derivatives (cf. \cite{Weaver1999}), it is easy to see that the drift $f$ is Lipschitz with constant $L=\frac 1 2$. Therefore, $f \in \mathcal K_{prior}$ as required by Thm. \ref{thm:KIdesiderata} to establish conservatism of the uncertainty bounds. 
(Note, in practice, the constant $L$ could also be estimated from the data \cite{anonymous,Wood1996}.) Folding in knowledge that the drift was only dependent on interaction space inputs, the KI learner determined a maximum error of $\maxerr = \sup_{\isv \in \iaspace} \norm{\prederr_1(\isv)}_{\infty } = 1.27$. The resulting (coarse) prediction model $\predf_1(\cdot)$ is depicted in Fig. \ref{fig:KIcollavoidopenlooppredmodels1} for various query points on a subset of the interaction space $\iaspace$.
 

In lieu to feedback linearisation and MRAC control approaches \cite{chowdharyacc2013} discussed above, we chose a control $u^\agi[k]:= (- \nu^\agi_{ad} + \bar u^\agi[k]  ) $ with $\nu^\agi_{ad} =  \predf(x)$ defined by the kinky inference prediction rule as per Def. \ref{def:KIL}. Here, $\bar u^\agi$ denotes a pseudo control yet to be defined. In contrast, to MRAC \cite{chowdharyacc2013} we did not ascribe a fixed feedback policy to the pseudo-control. Instead, we intended to determine the pseudo control trajectory with MILP-based open-loop planning analogously to the procedure in Exp.1.

Applying the control yielded the closed-loop dynamics,
\begin{equation}
	x^\agi[{k+1}] = A x^\agi[k] + B \bar u^\agi[k] + F(x^\agi[k])
\end{equation}
 where $F(x) = f(x) - \predf(x) $ denotes an uncertain increment determining the deviation of the actual trajectory $x^\agi [\cdot]$ from the nominal trajectory 
given by the \textit{nominal dynamics}
\begin{equation}
	\bar x^\agi[{k+1}] = A \bar x^\agi[k] + B \bar u^\agi[k].
\end{equation}
%
Note, in contrast to the work in stochastic collision avoidance \cite{LyonsACC2012} we have based our planner on, the discrepancy is not modelled in a stochastic manner, but is assumed to be due to rest uncertainty of the kinky inference rule. 
Since the latter provides an error estimate around its predictions, we can utilise these uncertainty quantifications to bound the discrepancy between nominal and actual dynamics.
Since we aim to do planning on the basis of the nominal model, we need to determine how much extra space to leave between the agents to enforce collision avoidance in the presence of error $e^\agi[k] = x^\agi[k] - \bar x^\agi[k]$. 
In other words, how large do we have to choose the tube radius around the nominal trajectory?

In pursuit of an answer, we once again consider the error dynamics:
\begin{equation}
	e^\agi[{k+1}] = A e^\agi[k] + F(x^\agi[k]). 
\end{equation}
%where $F_k = F(x[k])$.


%Going through analogous steps as in Sec. \ref{sec:KIMRACstabbounds} (with $A$ in place of $M$), we see that 
%
%$e^\agi[k]= A^k \, \vc e^\agi[0] +  \sum_{i=0}^{k-1} A^{k-1-i} \, \vc F(x^\agi[i])	$ and hence, 
%%\begin{equation}
	%$\norm{\vc e^\agi[k]} \leq \matnorm{A^{k}} \, \norm{\vc e^\agi[0]} +  \maxerr_k	 \sum_{i=0}^{k-1}  \matnorm{A^{k-1-i}}$
%%\end{equation}
%where $\maxerr_k	= \max_{i=1,...,k-1} \norm{F(x^\agi[i])}$. Since $F$ is nonlinear, we would rather allow our control decisions to be conservative than having to incorporate the nonlinear term $F(x)$ in the  constraints of our optimisation problem. 
%%(Note, that for certain input norms, the KI rule generates piece-wise linear prediction uncertainty functions. In future work, we would like to investigate using this property to convert constraints on $F$ into linear constraints. We hope to be able to do so employing techniques akin to LP conversion techniques found in piece-wise linear optimisation \cite{boyd:2004}. )
%
%%\begin{figure}
        %%\centering
				  %%\subfigure[S.]{
    %%%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %%\includegraphics[width = 5cm]
								%%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%%{content/Ch_kinkyinf/figs/akt1_dist}
    %%\label{fig:KIcollavoidopenlooppredmodels1}
  %%} 	 
				  %%\subfigure[Initial prediction.]{
    %%%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %%\includegraphics[width = 5cm]
								%%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%%{content/Ch_kinkyinf/figs/akt1_dist}
    %%\label{fig:KIcollavoidopenlooppredmodels1}
  %%} 	 
				  %%\subfigure[Initial prediction.]{
    %%%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %%\includegraphics[width = 5cm]
								%%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%%{content/Ch_kinkyinf/figs/akt1_dist}
    %%\label{fig:KIcollavoidopenlooppredmodels1}
  %%} 	 
	%%\label{fig:stagesoccostmashfe}
   %%\caption{Distance of the actual trajectories.}
%%\end{figure}	 
%
%Therefore, we replace $\maxerr_k$ by the more conservative constant 
%%
%%\begin{equation}
	%$\maxerr := \sup_{s \in \iaspace} \norm{F(s)} \leq c \sup_{s \in \iaspace} \norm{\prederr(s)}_\infty.$
%%\end{equation}
%%
%Here, $c$ is a norm conversion constant that ensures
%
 %$\norm{\cdot } \leq c \norm{\cdot}_\infty$. For instance, if $\norm{\cdot}$ denotes the Euclidean norm, then $c = \sqrt 2$ (e.g. \cite{koenigsberger:2000}).
%
%
%This allows us to obtain the state-independent bound 


%Define $\maxerr_k	= \max_{i=1,...,k-1} \norm{F(x^\agi[i])}$ and 
Let $\maxerr := \sup_{s \in \iaspace} \norm{F(s)} \leq c \sup_{s \in \iaspace} \norm{\prederr(s)}_\infty.$
%\end{equation}
%
Here, $c$ is a norm conversion constant that ensures
 $\norm{\cdot } \leq c \norm{\cdot}_\infty$. For instance, if $\norm{\cdot}$ denotes the Euclidean norm, then $c = \sqrt 2$ (e.g. \cite{koenigsberger:2000}).

Leveraging sub-multiplicativity and sub-additivity of vector and matrix norms, an inductive argument shows 
%
\begin{eqnarray} \label{eq:tuberadKIMPCcollavoid}
	\norm{\vc e^\agi[k]} \leq \matnorm{A^{k}} \, \norm{\vc e^\agi[0]} +  \maxerr	 \sum_{i=0}^{k-1} \matnorm{A^{k-1-i}} =: r^\agi[k].
\end{eqnarray}

%
%This bound $r^\agi_k$ is more conservative than if we had based it upon $\maxerr_k$ instead of on $\maxerr$. Nonetheless, it has the advantage of being state-independent and hence, can be pre-computed for all time steps within a given planning horizon.

In the absence of a nonlinear dependence on the state, open-loop planning could be conducted based on mixed-integer linear programming, analogously to the approach described in \cite{Lyons2011}. The difference between the approaches is that in our simulations, the radii $r^\agi[k]$ of the tube were computed as per Eq. \ref{eq:tuberadKIMPCcollavoid}. In particular, they were based on the uncertainty due to the KI predictions quantified by $\prederr$ rather than on the basis of probabilistic tail radii. To enforce collision avoidance, we then introduced tube constraints of the form $\gamma^{\agi,\agii}[k] > 0, \forall k \forall \agi,\agii \in \agset$ with 
$\gamma^{\agi,\agii}(k) = \norm{\bar \isv^\agi[k] - \bar \isv^\agii[k] }_\infty - \Lambda - r^\agi[k] - r^\agii[k] $ where the tube radii $r^\agi[k], r^\agii[k]$ were defined as in Eq. \ref{eq:tuberadKIMPCcollavoid} and rule out the possibility of any collisions between agents $\agi$ and $\agii$.

The results of the planning process with these conservative constraints are depicted in Fig. \ref{fig:KIcollavoidopenloopakt2}.


This time, the planner had successfully taken into account the uncertainty, resulting in successful collision avoidance. However, due to the fact that the drift model had been scarcely identified, the resulting large uncertainty estimates, in conjunction with the conservatism of the decision making process due to our bounds, caused the planner to conceive control actions that resulted in trajectories that kept a rather larger safety distance between the agents. While this did prevent collisions, the goal locations could not be reached (Fig. \ref{fig:akt2fig3}).


 
\textbf{Exp. 3.}
Since all uncertainty is due to epistemic uncertainty of the inductive inference rule over the deterministic drift field, we expect the conservatism to reduce with increasing learning experience. To test this, we updated the data set from $\data_1$ to $\data_2$ the latter of which now contained 100 samples of the drift drawn uniformly at random from the interaction space. 
The results are shown in Fig. \ref{fig:KIcollavoidopenloopakt3}.
As expected, the reduced uncertainty bound ($\maxerr = 0.31$) yielded less conservative plans (see Fig. \ref{fig:akt3fig1}). Furthermore, the actual trajectories observed from plan execution (Fig. \ref{fig:akt3fig3})  closely matched the planned trajectories (Fig. \ref{fig:akt3fig2}). This probably was a result of the improved identification result (see Fig. \ref{fig:KIcollavoidopenlooppredmodels}) afforded by the larger data set. Note, the reduced uncertainty allowed the trajectories to closely approach their goal positions (Fig. \ref{fig:akt3fig3}). Since we had tied the agents' cost to the distances to their goal state, this translates to reduced social stage cost. 

In conclusion, our simulations have demonstrated that the uncertainty quantifications of our kinky inference method can be successfully employed to facilitate conservative decision making in the context of multi-agent collision avoidance such that guarantees on collision avoidance can be given (whose veracity rests on the prior assumption $f \in \mathcal K_{prior}$). As expected, the simulations have illustrated the positive effect increased certainty (via learning) has on the conservatism of the decision-making process and hence, on the social cost (measuring distances to the goals) of the resulting trajectories (see Fig. \ref{fig:KIsoccost}).  
\begin{figure} 
        \centering
				  \subfigure[Initial prediction $\predf_1$.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt2learneddrift}
    \label{fig:KIcollavoidopenlooppredmodels1}
  } 	 
					  \subfigure[Improved prediction $\predf_2$.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/akt3learneddrift}
    \label{fig:KIcollavoidopenlooppredmodels2}
  } 	
							  \subfigure[Social cost after each experiment.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3.1cm 9.5cm 4.5cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/soccost}
    \label{fig:KIsoccost}
  } 
	%
   \caption{Belief over drift models based on $\data_1$ and $\data_2 \supset \data_1$ with $\abs{\data_1} = 2, \abs{\data_2} = 100$. Here, the top figures show the predictions of $\predf_{n,3}(s)$ and the bottom plots depict the predictions of $\predf_{n,4}(s)$ for $n =1$ and $n=2$, respectively. The ground-truth drift model was $f(x) = \bigl(0,0, - \sin(0.5 \, x_1), - \sin( 0.5 \, x_2) \bigr)^\top$. Rightmost plot: Social cost after each experiment. Note how the reduced uncertainty translated to reduced social cost of the last experiment (bar plot 3) vs the cost in the second (bar plot 2). While the first experiment (bar plot 1) also accumulated low social cost, a collision occurred.}
	\label{fig:KIcollavoidopenlooppredmodels}
\end{figure}	 

==> content2/Ch_kinkyinf/KIMRAC_wingrock.tex <==
\section{LACKI and model reference adaptive control for online learning and aircraft tracking control in the presence of wing rock dynamics }
\label{sec:KIMRAC}
As pointed out in \cite{chowdharyacc2013}, modern fighter aircraft designs are susceptible to lightly damped oscillations in roll known as ``wing rock''. Commonly occurring during landing \cite{Saad2000}, removing wing rock from the dynamics is crucial for precision control of such aircraft.
Precision tracking control in the presence of wing rock is a nonlinear problem of practical importance and has served as a test bed for a number nonlinear adaptive control methods \cite{Chowdhary2013,Monahemi1996,chowdharyacc2013}.

We replicate the experiments of the recent work of Chowdhary et. al. \cite{Chowdhary2013,ChowdharyCDC2013}.\footnote{We are grateful to the authors for kindly providing the code.}
Here the authors have compared their Gaussian process based approach, called \textit{GP-MRAC}, to the more established adaptive model-reference control approach based on RBF networks \cite{Sanner1992,Kim1998}, referred to as \textit{RBFN-MRAC}. Replacing the Gaussian process learner by our kinky inference learner, we readily obtain an analogous approach which we will refer to as \emph{kinky inference model reference adaptive control} (\textit{LACKI-MRAC}). As an additional baseline, we also examine the performance of a simple linear controller.

While with the exact same parameters settings of the experiments in \cite{Chowdhary2013}, performance of our LACKI-MRAC method comes second to GP-MRAC, we also evaluate the performance of all controllers over a range of 555 random parameter settings and initial conditions. As we will see, across this range of problem instances and parameter settings, LACKI-MRAC markedly outperforms all other methods.

\subsection{Model reference adaptive control}
Before proceeding with the wing rock application we will commence with (i) outlining model reference adaptive control (MRAC) \cite{astroemadaptivectrlbook2013} as considered in \cite{Chowdhary2013} and (ii) describe the deployment of the LACKI learning algorithm to this framework to yield our LACKI-MRAC adaptive controller. 
We will now rehearse the description of MRAC for second-order systems following \cite{Chowdhary2013}:

Assume $m \in \nat$ to be the dimensionality of a configuration of the system in question and define $d = 2m$ to be the dimensionality of the pertaining state space $\statespace$.

Let $x = [x_1;x_2] \in \statespace$ denote the state of the plant to be controlled.
Given the control-affine system 
 %
\begin{align}
\dot x_1 = x_2, \hspace{1cm}  \dot x_2 = a(x) + b(x) \, u(x) \label{eq:secorddynctrlaff}
\end{align}
%
it is desired to find a control law $u(x)$ such that the closed-loop dynamics exhibit a desired reference behaviour:
%
\begin{align}
\dot \xi_1 = \xi_2, \hspace{1cm}   \dot \xi_2 = f_{r}(\xi,r)
\end{align}
where $r$ is a reference command $f_r$ some desired response and $t \mapsto \xi (t)$ is the reference trajectory.

If a priori $a$ and $b$ are believed to coincide with $\hat a_0, \hat b_0$ respectively, the inversion control 
$u = \hat b_0^{-1} (- \hat a_0 +u')$ is applied. This reduces the closed-loop dynamics to 
$\dot x_1 = x_2, \dot x_2 = u' + \tilde a(x,u) $
where $\tilde a(x,u)$ captures the modelling error of the dynamics: 
\begin{equation}
	\tilde a (x,u ) = a(x) - \hat a_0(x) + \bigl(b(x) - \hat b_0(x)\bigr) u.
\end{equation}
 For $m = \frac d 2$, let $I_m \in \Real^{m \times m}$ denote the $m \times m$- identity matrix.  If $b$ was perfectly known, then $b - \hat b_0^{-1} = 0$ and the model error can be written as $\tilde a (x)= a(x) - \hat a_0(x)$. In particular, $\tilde a$ has lost its dependence on the control input. 



In this situation \cite{Chowdhary2013,ChowdharyCDC2013} propose to set 
the pseudo control as follows: $u'(x) :=  \nu_{r} + \nu_{pd} - \nu_{ad}$ where $\nu_{r} = f_{r}(\xi,r)$is a feed-forward reference term,  $\nu_{ad}$ is a yet to be defined output of a learning module \emph{adaptive element} and $\nu_{pd} = (K_1 \, K_2) e$ is a feedback error term designed to decrease the \textit{tracking error} $e(t) = \xi(t) - x(t)$ by defining $K_1,K_2 \in \Real^{m \times m}$ as in described in what is to follow.

Inserting these components, we see that the resulting \textit{error dynamics} are:
%
%
\begin{equation}\label{eq:errordynmrac}
	\dot e = \dot \xi - [x_2; \nu_r + \nu_{pd}+ \tilde a(x) ] = M e + B \bigl(\nu_{ad}(x) -  \tilde a(x)\bigr)
\end{equation}
%
%
where $M = \left(\begin{array}[h]{cc}
			O_m &  \, I_{m}\\
			-K_1 & -K_2 
					\end{array}\right)$ and $B = \left(\begin{array}[h]{c}
			O_m \\ I_m
					\end{array}\right)$.
If the feedback gain matrices $K_1,K_2$ parametrising $\nu_{pd}$ are chosen such that $M$ is stable then the error dynamics converge to zero as desired if the learning error $E_\lambda$ vanishes: $E_\lambda (x(t)) = \norm{\nu_{ad}(x(t)) - \tilde a(x(t))} \stackrel{t \to \infty} {\longrightarrow} 0$. 

It is assumed that the adaptive element is the output of a learning algorithm that is tasked to learn $\tilde a$ online. This is done by continuously feeding it training examples of the form $\bigl(x(t_i), \tilde a(x(t_i)) + \varepsilon_i\bigr)$ where $\varepsilon_i$ is observational noise.  

Intuitively, assuming the learning algorithm is suitable to learn target $\tilde a$ (i.e. $\tilde a$ is close to some element in the hypothesis space \cite{mitchellbook:97} of the learner) and that the controller manages to keep the visited state space bounded, the learning error (as a function of time $t$) should vanish.

Substituting different learning algorithms yields different adaptive controllers. \textit{RBFN-MRAC} \cite{Kim1998} utilises radial basis function neural networks for this purpose whereas \textit{GP-MRAC} 
employs Gaussian process learning \cite{GPbook:2006} to learn $\tilde a$ \cite{Chowdhary2013,ChowdharyCDC2013}. 

In what is to follow, we utilise our LACKI learning method as the adaptive element. Following the nomenclature of the previous methods we name the resulting adaptive controller \textit{LACKI-MRAC}.

\subsection{The wing rock control problem}
The wing rock dynamics control problem considers an aircraft in flight. Denoting $x_1$ to be the roll attitude (angle of the aircraft wings) and $x_2$ the roll rate (measured in angles per second), the controller can set the aileron control input $u$ to influence the state $x := [x_1;x_2]$.

Based on \cite{Monahemi1996}, Chowdhary et. al. \cite{Chowdhary2013,ChowdharyCDC2013} consider a second-order control-affine model of the wing rock dynamics as per  Eq. \ref{eq:secorddynctrlaff} 
where $b =3$ is a known constant and 
$a(x) = W_0^* + W_1^* x_1 + W_2^* x_2 + W_3^* \abs{x_1} x_2 + W_4^* \abs{x_2} x_2 + W^*_5 x_2^3$ is an priori unknown nonlinear drift. 



Note, the drift is non-smooth but, employing Lem. \ref{lem:Hoeldarithmetic}, it would be easy to derive a Lipschitz constant on any bounded subset of state space if the parameters $W := (W_0^*,\ldots, W_5^*)$ were known.

To control the system, we employ LACKI-MRAC as the adaptive element $\nu_{ad}$. Our simulations were computed on the basis of a first-order Euler approximation of the continuous-time dynamics
with a time increment step size of $\tinc = 0.1 [sec.]$

Our kinky inference learner was initialised with $L(0) =\underline L =p= 1$. The parameters $L(n)$ were  updated online following our lazy update method as per Eq. \ref{eq:lazyconstupdaterule_batch_main} with $\hestthresh = 0$. 

Since the point of learning-based and adaptive control is to be able to adapt to various settings, we test the controllers across a range of randomised problem settings, initial conditions and parameter settings.
We created 555 randomised test runs of the wingrock tracking problems and tested each algorithm on each one of them. The initial state $x(t_0)$ was drawn uniformly at random from $[0,7] \times [0,7]$, the initial kernel length scales were drawn uniformly at random from $[0.05,2]$, and used both for RBF-MRAC and GP-MRAC. The H\"older constant $L$ for the LACKI-MRAC was initialised at random from the same interval but allowed to be adapted as part of the online learning process. The parameter weights $W$ of the system dynamics specified above were multiplied by a constant drawn uniformly at random from the interval $[0,2]$. To allow for better predictive performance of GP-MRAC we doubled the maximal budget to 200 training examples. 
The feedback gains were chosen to be one, $K_1=K_2=1$. 

In addition to the three adaptive controllers we also tested the performance of a simple $PD$- controller with just these feedback gains (i.e. we executed x-MRAC with adaptive element $\nu_{ad}=0$). This served as a baseline comparison to highlight the benefits of the adaptive element over simple feedback control.

The performance of all controllers across these randomised trials is depicted in Fig. \ref{fig:wingrockresultsbp}. Each data point of each boxplot represent a performance measurement for one particular trial.


\begin{figure}
        \centering
				%  \subfigure[Results over 555 randomised examples.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
   \includegraphics[width = 8cm, clip, trim = 1.5cm 8cm 1cm 7cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wingrockbp}
   % \label{fig:wingrockresultsbp}
  %} 
   \caption{Performance of the different online controllers over a range of 555 trials with randomised parameter settings and initial conditions. 1: RBF-MRAC, 2: GP-MRAC, 3: LACKI-MRAC, 4: linear controller.  LACKI-MRAC outperforms all other methods with respect to all performance measures, except for prediction runtime (where the parametric learner RBF-MRAC performs best).} 
       \label{fig:wingrockresultsbp}
\end{figure}	  

 






	For each method, the figures show the boxplots of the following recorded quantities: 
	\begin{itemize}
		\item log-XERR: cummulative angular position error (log-deg), i.e. $\log(\int_{t_0}^{t_f} \norm{\xi_1(t) - x_1 (t)} \dt )$.
		\item log-XDOTERR:  cummulative roll rate error (log-deg/sec.), i.e. $\log(\int_{t_0}^{t_f} \norm{\xi_2(t) - x_2 (t)} \dt )$.
		\item log-PREDERR: log-prediction error. \\ That is,  $\log(\int_{t_0}^{t_f} \norm{\nu_{ad}(x(t)) - \tilde a(x(t))} \dt )$.
		\item log-CMD: cummulative control magnitude (log-scale), i.e. $\log(\int_{t_0}^{t_f} \norm{u(t)} \dt )$.
		\item log-max. RT(predictions): the log of the maximal runtime (within time span $[t_0,t_f]$) each method took to generate a prediction $\nu_{ad}$ within the time span.
		\item log-max. RT (learning): the log of the maximal runtime (within time span $[t_0,t_f]$) it took each method to incorporate a new training example of the drift $\tilde a$.
	\end{itemize}
	
	
	
%	\begin{wrapfigure}{r}{0.5\textwidth}
%  \begin{center}
%    \includegraphics[width=0.48\textwidth,clip, trim = 1.5cm 8cm 1cm 7cm]{content/Ch_kinkyinf/figs/wingrockbp}
%      \end{center}
%   \caption{Performance of the different online controllers over a range of 555 trials with randomised parameter settings and initial conditions. 1: RBF-MRAC, 2: GP-MRAC, 3: LACKI-MRAC, 4: linear controller.  LACKI-MRAC outperforms all other methods with respect to all performance measures, except for prediction runtime (where the parametric learner RBF-MRAC performs best).} 
%   	       \label{fig:wingrockresultsbp}
%\end{wrapfigure}	
	
	
	As can be seen from Fig. \ref{fig:wingrockresultsbp}, all three adaptive methods outperformed the simple $PD$- controller in terms of tracking error. 
	
	In terms of prediction runtime, the RBF-MRAC outperformed both GP-MRAC and LACKI-MRAC. This is hardly surprising. After all, RBF-MRAC is a parametric method with constant prediction time. By contrast, both non-parametric methods will have prediction times growing with the number of training examples.
That is, it would be the case if GP-MRAC were given an infinite training size budget. Indeed one might argue whether GP-MRAC, if operated with a finite budget, actually is a parametric approximation where the parameter consists of the hyper-parameters along with the fixed-size training data matrix $X$. When comparing the (maximum) prediction and learning runtimes one should also bear in mind that GP-MRAC predicted with up to 200 examples in the training data set. By contrast, LACKI-MRAC undiscerningly had incorporated all 10001 training points by the end of each trial.

Across the remaining metrics, LACKI-MRAC markedly outperformed all other methods.

Note, we have also attempted to test all methods across a greater range of problem settings, including larger initial states, more varied hyper-parameter settings, lower feedback gains and more varied choices of dynamics coefficients $W$. However, this resulted in GP-MRAC to often run into conditioning problems. This is a common issue in GP learning due to the necessity of matrix inversion or Cholesky decompositions of the covariance matrix. Similar behaviour ensued when setting the training size budget to large values. All these changes often resulted in long learning runtimes, spiky control outputs and thus, poor overall performance. Similarly, code execution of our RBF-MRAC implementation was frequently interrupted with error messages when the state was initialised to positions outside of the rectangle $[0,7] \times [0,7]$.

We have not investigated the root cause of these issues in greater detail yet. However, it might be worth exploring whether the great robustness of kinky inference might be an additional selling point that sets it apart from other recent adaptive control methods. Such robustness is of course important in control settings such as flight control where failure or erratic behaviour of the adaptive element may result in critical incidents. 
%
An example where GP-MRAC failed to track the reference occurred when repeating our first experiment  with the following modifications: The initial state was chosen to be $x(t_0) = (-90,40)^\top$ corresponding to a rapidly rotating aircraft. Furthermore, the wing rock coefficients $W$ were multiplied by a factor of $5$, amplifying the non-linearities of the drift field. 

When initialised with the length scale parameter of 0.3, the GP ran into conditioning problems and caused the output of the adaptive element in GP-MRAC to produce spikes of very large magnitude and to further destabilise the system. We tried the problem with various kernel length scale settings ranging from $0.3$ to $20$. Increasing the length scale parameter to length scale of at least 1 seemed to fix the conditioning problem. Nonetheless, the GP-MRAC still did not manage to learn and stabilise the system in any of these settings. A record of GP-MRAC's performance in this example (for length scale of 1) is depicted in  Fig. \ref{fig:gpfail} (top row). As the plots show, the GP starts with relatively high tracking and prediction error from which it cannot recover. At about 26 seconds into the simulation the state rapidly diverges.

 
\begin{figure*}
        \centering
				  \subfigure[Position (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail1}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Tracking error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail2}
   % \label{fig:wingrockresultsbp}
  } 
							  \subfigure[Log - prediction error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[scale =.34]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_gpprederr}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Position (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail1_hfe}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Tracking error (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail2_hfe}
   % \label{fig:wingrockresultsbp}
  } 
%
					  \subfigure[Log - prediction error (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[scale =.34]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_hfeprederr}
   % \label{fig:wingrockresultsbp}
  } 
						  %\subfigure[State path (LACKI-MRAC).]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm, clip, trim = 2cm 9cm 1cm 7cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/gpfail_statepathHfe}
   %% \label{fig:wingrockresultsbp}
  %} 	
	%
   \caption{Example where GP-MRAC fails. By contrast, LACKI-MRAC manages to adapt and direct the system back to the desired trajectory.}
	\label{fig:gpfail}
\end{figure*}	 
%

For comparison, we also tried LACKI-MRAC on the same problem. Starting with initial $L(0) =\underline L =1$ as before. Starting out with a relatively large tracking and prediction error, LACKI-MRAC nonetheless managed to recover and successfully track the system (see  Fig. \ref{fig:gpfail}, bottom row). The state path and learned drift model obtained by LACKI-MRAC are depicted in Fig. \ref{fig:gpfail2}.

\begin{figure}
        \centering
				  \subfigure[State path (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 6cm, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_statepathHfe}
   % \label{fig:wingrockresultsbp}
  } 	\hspace{.5cm}
	  \subfigure[Learned drift model (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 6cm, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_hfelearnedmodel}
   % \label{fig:wingrockresultsbp}
  } 	
	%
   \caption{Depicted are the state path and the drift model learned online by LACKI-MRAC.}
	\label{fig:gpfail2}
\end{figure}	 

==> content2/Ch_kinkyinf/KIMRAC_wingrock_old.tex <==
\subsection{Kinky inference and model reference adaptive control for online learning and tracking control in the presence of wing rock dynamics }
\label{sec:KIMRAC}
As pointed out in \cite{chowdharyacc2013}, modern fighter aircraft designs are susceptible to lightly damped oscillations in roll known as ``wing rock''. Commonly occurring during landing \cite{Saad2000}, removing wing rock from the dynamics is crucial for precision control of such aircraft.
Precision tracking control in the presence of wing rock is a nonlinear problem of practical importance and has served as a test bed for a number nonlinear adaptive control methods \cite{Chowdhary2013,Monahemi1996,chowdharyacc2013}.

For comparison, we replicate the experiments of the recent work of Chowdhary et. al. \cite{Chowdhary2013,ChowdharyCDC2013}.\footnote{We are grateful to the authors for kindly providing the code.}
Here the authors have compared their Gaussian process based approach, called \textit{GP-MRAC}, to the more established adaptive model-reference control approach based on RBF networks \cite{Sanner1992,Kim1998}, referred to as \textit{RBFN-MRAC}. Replacing the Gaussian process learner by our kinky inference learner, we readily obtain an analogous approach which we will refer to as \textit{LACKI-MRAC}. As an additional baseline, we also examine the performance of a simple P-controller.

While with the exact same parameters settings of the experiments in \cite{Chowdhary2013}, performance of our LACKI-MRAC method comes second to GP-MRAC, we also evaluate the performance of all controllers over a range of 555 random parameter settings and initial conditions. As we will see, across this range of problem instances and parameter settings,LACKI-MRAC markedly outperforms all other methods.

\subsubsection{Model reference adaptive control}
Before proceeding with the wing rock application we will commence with (i) outlining model reference adaptive control (MRAC) \cite{astroemadaptivectrlbook2013} as considered in \cite{Chowdhary2013} and (ii) describe the deployment of kinky inference to this framework. 
We will now rehearse the description of MRAC for second-order systems following \cite{Chowdhary2013}. 

Assume $m \in \nat$ to be the dimensionality of a configuration of the system in question and define $d = 2m$ to be the dimensionality of the pertaining state space $\statespace$.

Let $x = [x_1;x_2] \in \statespace$ denote the state of the plant to be controlled.
Given the control-affine system 
 
\begin{align}
\dot x_1 &= x_2 \\
\dot x_2 &= a(x) + b(x) \, u(x) \label{eq:secorddynctrlaff}
\end{align}

it is desired to find a control law $u(x)$ such that the closed-loop dynamics exhibit a desired reference behaviour:

\begin{align}
\dot \xi_1 &= \xi_2 \\
\dot \xi_2 &= f_{r}(\xi,r)
\end{align}
where $r$ is a reference command, $f_r$ some desired response and $t \mapsto \xi (t)$ is the reference trajectory.

If a priori $a$ and $b$ are believed to coincide with $\hat a_0, \hat b_0$ respectively, the inversion control 
$u = \hat b_0^{-1} (- \hat a_0 +u')$ is applied. This reduces the closed-loop dynamics to 
$\dot x_1 = x_2, \dot x_2 = u' + \tilde a(x,u) $
where $\tilde a(x,u)$ captures the modelling error of the dynamics: 
\begin{equation}
	\tilde a (x,u ) = a(x) - \hat a_0(x) + \bigl(b(x) - \hat b_0(x)\bigr) u.
\end{equation}
 Let $I_d \in \Real^{d \times d}$ denote the identity matrix.  If $b$ is perfectly known, then $b - \hat b_0^{-1} = 0$ and the model error can be written as $\tilde a (x)= a(x) - \hat a_0(x)$. In particular, $\tilde a$ has lost its dependence on the control input. 



In this situation \cite{Chowdhary2013,ChowdharyCDC2013} propose to set 
the pseudo control as follows: $u'(x) :=  \nu_{r} + \nu_{pd} - \nu_{ad}$ where $\nu_{r} = f_{r}(\xi,r)$ is a feed-forward reference term,  $\nu_{ad}$ is a yet to be defined output of a learning module \emph{adaptive element} and $\nu_{pd} = [K_1 K_2] e$ is a feedback error term designed to decrease the \textit{tracking error} $e(t) = \xi(t) - x(t)$ by defining $K_1,K_2 \in \Real^{m \times m}$ as described in what is to follow.

Inserting these components, we see that the resulting \textit{error dynamics} are:


\begin{equation}\label{eq:errordynmrac}
	\dot e = \dot \xi - [x_2; \nu_r + \nu_{pd}+ \tilde a(x) ] = M e + B \bigl(\nu_{ad}(x) -  \tilde a(x)\bigr)
\end{equation}


where $M = \left(\begin{array}[h]{cc}
			O_m &  \, I_{m}\\
			-K_1 & -K_2 
					\end{array}\right)$ and $B = \left(\begin{array}[h]{c}
			O_m \\ I_m
					\end{array}\right)$.
If the feedback gain matrices $K_1,K_2$ parametrising $\nu_{pd}$ are chosen such that $M$ is stable then the error dynamics converge to zero as desired, provided the learning error $E_\lambda$ vanishes: $E_\lambda (x(t)) = \norm{\nu_{ad}(x(t)) -  a(x(t))} \stackrel{t \to \infty} {\longrightarrow} 0$. 

It is assumed that the adaptive element is the output of a learning algorithm that is tasked to learn $\tilde a$ online. This is done by continuously feeding it training examples of the form $\bigl(x(t_i), \tilde a(x(t_i)) + \varepsilon_i\bigr)$ where $\varepsilon_i$ is observational noise.  

Intuitively, assuming the learning algorithm is suitable to learn target $\tilde a$ (i.e. $\tilde a$ is close to some element in the hypothesis space \cite{mitchellbook:97} of the learner) and that the controller manages to keep the visited state space bounded, the learning error (as a function of time $t$) should vanish.

Substituting different learning algorithms yields different adaptive controllers. \textit{RBFN-MRAC} \cite{Kim1998} utilises radial basis function neural networks for this purpose whereas \textit{GP-MRAC} 
employs Gaussian process learning \cite{GPbook:2006} to learn $\tilde a$ \cite{Chowdhary2013,ChowdharyCDC2013}. 

%\jcom{possibly the following paragraph will go into a related work section:}
%Note, this setting of GP-MRAC is a special case of the SP-SIIC approach we introduced in Ch. \ref{ch:SPSIIC}. Here $\hat a_0$ is the prior mean function of the s.p. we place over the drift. Our exposition in Sec. \ref{ch:SPSIIC} is more general in that it allows for uncertain $b$ that is learned from data, considers under-actuated systems and makes no distributional restrictions. As an additional feature, GP-MRAC assumes that the data sets can be updated continuously. While of course this is not tractable the authors maintain a data corpus of a fixed size by a range of methods including simple FIFO queues as well as sparsification methods \cite{Kingravi2014,Csato2002}. In contrast, we utilise learning criteria to only include informative data points. In addition, we employ hyper-parameter optimisation which we show to be highly beneficial. While hyper-parameter training cannot be done at high frequency, it would be possible to run it in the background on a separate CPU (in parallel to the CPU on which the controller runs). 

In what is to follow, we utilise our LACKI method as the adaptive element. Following the nomenclature of the previous methods we name the resulting adaptive controller \textit{LACKI-MRAC}.

\subsubsection{The wing rock control problem}
The wing rock dynamics control problem considers an aircraft in flight. Denoting $x_1$ to be the roll attitude (angle of the aircraft wings) and $x_2$ the roll rate (measured in angles per second), the controller can set the aileron control input $u$ to influence the state $x := [x_1;x_2]$.

Based on \cite{Monahemi1996}, Chowdhary et. al. \cite{Chowdhary2013,ChowdharyCDC2013} consider the following model of the wing rock dynamics: 

\begin{align}
\dot x_1 &= x_2 \\
\dot x_2 &= a(x) + b \, u 
\end{align}
where $b =3$ is a known constant and 
$a(x) = W_0^* + W_1^* x_1 + W_2^* x_2 + W_3^* \abs{x_1} x_2 + W_4^* \abs{x_2} x_2 + W^*_5 x_2^3$ is an priori unknown nonlinear drift. 



Note, the drift is non-smooth but, employing Lem. \ref{lem:Hoeldarithmetic}, it would be easy to derive a Lipschitz constant on any bounded subset of state space if the parameters $W := (W_0^*,\ldots, W_5^*)$ were known.

To control the system we employ LACKI as the adaptive element $\nu_{ad}$.
In the absence of the knowledge of a Lipschitz constant, we start with a guess of $\underline L=1$ (which will turn out to be too low) and update it following the procedure described in Sec. \ref{sec:lacki}.

In a first instance, we replicated the experiments conducted in \cite{Chowdhary2013,chowdharyacc2013} with the exact same parameter settings. That is, we chose $W_0^* = 0.8, W_1^* = 0.2314, W_2^* = 0.6918, W_3^* = -0.6245, W_4^* = 0.0095, W_5^* = 0.0214$. 



The simulation initialised with start state $x = (3,6)^\top$ and simulated forward with a first-order Euler approximation with time increment $\tinc = 0.005 [s]$ over a time interval $\indsett = [t_0,t_f]$ with $t_0 = 0[s]$ and $t_f = 50[s]$. Training examples and control signal were continuously updated every $\Delta_u= \Delta_o = \tinc [s]$. The RBF and GP learning algorithms were initialised with fixed length scales of 0.3 units. The GP was given a training example budget of a maximum of 100 training data points to condition the posterior model on. Our kinky inference learner was initialised with $L =p= 1$ and updated online following the lazy update method described in Sec. \ref{sec:lazylipconstupdate}.

The test runs also exemplify the working of the lazy update rule.
The initial guess $\underline L=1$ was too low. However, our lazy update rule successfully picked up on this and had ended up increasing constant to $L=2.6014$ by the end of the online learning process.



%
%
\begin{figure*}
        \centering
				  \subfigure[Tracking error (RBF-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[ width=.3\textwidth, clip, trim = 2.5cm 8cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr2RBF}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Tracking error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 2.5cm 8cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr2GP}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Tracking error (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 2.5cm 8cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr2}
   % \label{fig:wingrockresultsbp}
  }
   \caption{Tracking error comparison of first example.}
	 \label{fig:wrtrackerrorsex1}
\end{figure*}	   

The results are plotted in Fig. \ref{fig:wrtrackerrorsex1}. 
We can see that in terms of tracking error of the reference our LACKI-MRAC outperformed RBF-MRAC and was a close runner-up to GP-MRAC which had the lowest tracking errors.  

%
To obtain an impression of the learning performance of the three learning algorithms we also recorded the prediction error histories for this example problem. The results are depicted in Fig. \ref{fig:wrprederrorsex1}. We can see that our kinky inference method and the GP method both succeeded in predicting the drift quite accurately while the RBFN method was somewhat lagging behind.
This is consistent with the observations made in \cite{Chowdhary2013,ChowdharyCDC2013}. The authors explain the relatively poor performance of the radial basis function network method by the fact that the reference trajectory on occasion led outside the region of state space where the centres of the basis function were placed in advance. By contrast, due to the non-parametric nature of the GP, GP-MRAC does not suffer from such a priori limitations. In fact, it can be seen as an RBF method that flexibly places basis functions around all observed data points \cite{GPbook:2006}. We would add that, as a non-parametric method, LACKI-MRAC shares this kind of flexibility, which might explain the fairly similar performance. 

However, being an online method, the authors of GP-MRAC explicitly avoided hyperparameter training via optimising the marginal log-likelihood. The latter is commonly done in GP learning \cite{GPbook:2006} to avoid the impact of an unadjusted prior but is often a computational bottle neck. Therefore, avoiding such hyperparameter optimisation greatly enhances learning and prediction speed in an online setting. However, we would expect the performance of the prediction to be dependent upon the hyperparameter settings. As we have noted above, the Lipschitz constant depends on the part of state space visited at runtime. Similarly, we might expect length scale changes depending on the part of state space the trajectory is in. Unfortunately, \cite{Chowdhary2013,ChowdharyCDC2013,chowdharyacc2013} provide no discussion of the length scale parameter setting and also called the choice of the maximum training corpus size ``arbitrary''. 

Since the point of learning-based and adaptive control is to be able to adapt to various settings, we test the controllers across a range of randomised problem settings, initial conditions and parameter settings.

We created 555 randomised test runs of the wingrock tracking problems and tested each algorithm on each one of them. The initial state $x(t_0)$ was drawn uniformly at random from $[0,7] \times [0,7]$, the initial kernel length scales were drawn uniformly at random from $[0.05,2]$, and used both for RBF-MRAC and GP-MRAC. The initial H\"older constant $\underline L$ for LACKI-MRAC was initialised at random from the same interval but was allowed to be adapted as part of the online learning process. Furthermore, we chose $\hestthresh =0$. The parameter weights $W$ of the system dynamics specified above were multiplied by a constant drawn uniformly at random from the interval $[0,2]$. To allow for better predictive performance of GP-MRAC we doubled the maximal budget to 200 training examples. 
The feedback gains were chosen to be $K_1=K_2=1$. 

In addition to the three adaptive controllers we also tested the performance of a simple $P$ controller with just these feedback gains (i.e. we executed x-MRAC with adaptive element $\nu_{ad}=0$). This served as a baseline comparison to highlight the benefits of the adaptive element over simple feedback control.

The performance of all controllers across these randomised trials is depicted in Fig. \ref{fig:wingrockresultsbp}. Each data point of each boxplot represent a performance measurement for one particular trial.

\begin{figure*}
        \centering
				  \subfigure[Prediction v.s. ground truth  (RBF-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .3\textwidth, clip, trim = 3cm 9cm 3cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr4RBF}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Prediction v.s. ground truth  (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 3cm 9cm 3cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr4GP}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Prediction v.s. ground truth  (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 3cm 9cm 3cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr4}
   % \label{fig:wingrockresultsbp}
  } 
   \caption{Prediction vs ground truth comparisons for the first example. Both nonparametric methods accurately predict the true drift and clearly outperform the RBFN learner.}
	\label{fig:wrprederrorsex1}
\end{figure*}	   


\begin{figure}
        \centering
				  \subfigure[Results over 555 randomised examples.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .5\textwidth, clip, trim = 1.5cm 8cm 1cm 7cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wingrockbp}
   % \label{fig:wingrockresultsbp}
  } 
   \caption{Performance of the different online controllers over a range of 555 trials with randomised parameter settings and initial conditions. 1: RBF-MRAC, 2: GP-MRAC, 3:LACKI-MRAC, 4: P-Controller. LACKI-MRAC outperforms all other methods with respect to all performance measures, except for prediction runtime (where the parametric learner RBF-MRAC performs best).} 
       \label{fig:wingrockresultsbp}
\end{figure}	   
  
	
	For each method, the figures show the boxplots of the following recorded quantities: 
	\begin{itemize}
		\item \textit{log-XERR}: cummulative angular position error (log-deg), i.e. $\log(\int_{t_0}^{t_f} \norm{\xi_1(t) - x_1 (t)} \dt )$.
		\item \textit{log-XDOTERR}:  cummulative roll rate error (log-deg/sec.), i.e. $\log(\int_{t_0}^{t_f} \norm{\xi_2(t) - x_2 (t)} \dt )$.
		\item \textit{log-PREDERR}: log-prediction error, i.e. 
		
		$\log(\int_{t_0}^{t_f} \norm{\nu_{ad}(x(t)) - \tilde a(x(t))} \dt )$.
		\item \textit{log-CMD}: cummulative control magnitude (log-scale), i.e. $\log(\int_{t_0}^{t_f} \norm{u(t)} \dt )$.
		\item \textit{log-max. RT (predictions)}: the log of the maximal runtime (within time span $[t_0,t_f]$) each method took to generate a prediction $\nu_{ad}$ within the time span.
		\item \textit{log-max. RT (learning)}: the log of the maximal runtime (within time span $[t_0,t_f]$) it took each method to incorporate a new training example of the drift $\tilde a$.
	\end{itemize}
	
	As can be seen from Fig. \ref{fig:wingrockresultsbp}, all three adaptive methods outperformed the simple $P$ controller in terms of tracking error. 
	
	In terms of prediction runtime, the RBF-MRAC outperformed both GP-MRAC and LACKI-MRAC. This is hardly surprising. After all, RBF-MRAC is a parametric method with constant prediction time. By contrast, both non-parametric methods will have prediction times growing with the number of training examples.
That is, it would be the case if GP-MRAC were given an infinite training size budget. Indeed one might argue whether GP-MRAC, if operated with a finite budget, actually is a parametric approximation where the parameter consists of the hyperparameters along with the fixed-size training data matrix. When comparing the (maximum) prediction and learning runtimes one should also bear in mind that GP-MRAC predicted with up to 200 examples in the training data set. By contrast, LACKI-MRAC undiscerningly had incorporated all 10001 training points by the end of each trial.

Across the remaining metrics, LACKI-MRAC markedly outperformed all other methods.

Note, we have also attempted to test all methods across a greater range of problem settings, including larger initial states, more varied hyper-parameter settings, lower feedback gains and more varied choices of dynamics coefficients $W$. However, this resulted in GP-MRAC to often run into conditioning problems. This is a common issue in GP learning due to the necessity of matrix inversion or Cholesky decompositions of the covariance matrix. Similar behaviour ensued when setting the training size budget to large values. All these changes often resulted in long learning runtimes, spiky control outputs and thus, poor overall performance. Similarly, code execution of our RBF-MRAC implementation was frequently interrupted with error messages when the state was initialised to positions outside of the rectangle $[0,7] \times [0,7]$.

We have not investigated the root cause of these issues in greater detail yet. However, it might be worth exploring whether the great robustness of kinky inference might be an additional selling point that sets it apart from other recent adaptive control methods. Such robustness is of course important in control settings such as flight control where failure or erratic behaviour of the adaptive element may result in critical incidents. 

An example where GP-MRAC failed to track the reference occurred when repeating our first experiment  with the following modifications: The initial state was chosen to be $x(t_0) = (-90,40)^\top$ corresponding to a rapidly rotating aircraft. Furthermore, the wing rock coefficients $W$ were multiplied by a factor of $5$, amplifying the non-linearities of the drift field. 

When initialised with a length scale parameter of 0.3, the GP ran into conditioning problems and caused the output of the adaptive element in GP-MRAC to produce spikes of very large magnitude and thus, further destabilised the system. We tried the problem with various kernel length scale settings ranging from $0.3$ to $20$. Increasing the length scale parameter to length scale of at least 1 seemed to fix the conditioning problem. Nonetheless, GP-MRAC still did not manage to learn and stabilise the system in any of these settings. A record of GP-MRAC's performance in this example (for length scale of 1) is depicted in Fig.  \ref{fig:gpfailGPWR1} -  \ref{fig:gpfailGPWR3}. As the plots show, GP-MRAC starts with relatively high tracking and prediction error from which it could not recover. At about 26 seconds into the simulation the state rapidly diverged.

 
\begin{figure*}
        \centering
				  \subfigure[Position (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 4cm 9cm 4cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail1}
   \label{fig:gpfailGPWR1}
  } 
					  \subfigure[Tracking error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 4cm 9cm 4cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail2}
   \label{fig:gpfailGPWR2}
  } 
							  \subfigure[Log - prediction error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[scale =.35]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_gpprederr}
    \label{fig:gpfailGPWR3}
  } 
					  \subfigure[Position (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 3.5cm 9cm 4cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail1_hfe}
    \label{fig:gpfailKIWR1}
  } 
					  \subfigure[Tracking error (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 3.5cm 9cm 4cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail2_hfe}
    \label{fig:gpfailKIWR2}
  } 
%
					  \subfigure[Log - prediction error (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[scale =.35,clip, trim = 0cm 0cm 0cm .1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_hfeprederr}
    \label{fig:gpfailKIWR3}
  } 
						  %\subfigure[State path (KI-MRAC).]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm, clip, trim = 2cm 9cm 1cm 7cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/gpfail_statepathHfe}
   %% \label{fig:wingrockresultsbp}
  %} 	
	%
   \caption{Example where GP-MRAC fails. By contrast,LACKI-MRAC manages to adapt and direct the system back to the desired trajectory.}
	\label{fig:gpfail}
\end{figure*}	 


For comparison, we also tried LACKI-MRAC on the same problem, starting with initial $L=1$ as before. Starting out with a relatively large tracking and prediction error, LACKI-MRAC nonetheless managed to recover and successfully track the system (see  Fig.  \ref{fig:gpfailKIWR1} -  \ref{fig:gpfailKIWR3}). The state path and learned drift model obtained by LACKI-MRAC are depicted in Fig. \ref{fig:gpfail2}.
%
\begin{figure*}
        \centering
				  \subfigure[State path (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .4\textwidth, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_statepathHfe}
   % \label{fig:wingrockresultsbp}
  } 	
	  \subfigure[Learned drift model (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .4\textwidth, clip, trim = 4.3cm 9cm 4cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_hfelearnedmodel}
   % \label{fig:wingrockresultsbp}
  } 	
	%
   \caption{Depicted are the state path and the drift model learned online byLACKI-MRAC.}
	\label{fig:gpfail2}
\end{figure*}	 

==> content2/Ch_kinkyinf/KISIICKIIML.tex <==
\section{Outlook on additional learning-based control methods}
In the following we will briefly discuss applications of KI to the system identification and inversion control (KI-SIIC), followed by an application to inversion dynamics model learning and control (IMLC)  \cite{Tuongmodellearningsurvey2011}. While providing rigorous examinations and comparisons was beyond the time limit and scope of this work, we have included the latter application to highlight our method's applicability in control that is based on black-box learning \cite{Ljungperspectives:2010}.

\subsection{Kinky inference for system identification and inversion control (KI-SIIC)}
In this section, we will apply kinky inference to our SIIC approach of Ch. \ref{ch:SPSIIC}. Let $q$ be a generalised coordinate (a configuration) and $x = [q; \dot q]$ be the state.  
Given the second-order control-affine dynamics $\ddot q = a(x) + b(x) u$, we infer both $a$ and $b$ with a separate KI learner. The online learning process other-wise proceeds just as described in Ch. \ref{ch:SPSIIC}. Note, in the case of random field learning, we placed a log-normal prior over the components of $b$ to learn it. The motivation was to encode the knowledge that $b$ was positive and bounded away from zero. Fortunately, in our KI framework, we can encode knowledge of boundedness quite explicitly by setting the lower bound function $\lbf$ to zero. As before, we set the pseudo-control to linear feedback with gain weights $w_1=w_2=2$. This weight is large enough to drive the linearised dynamics to the goal, but sufficiently weak to ensure that learning success was important to achieve stabilisation.

As an illustration that our SIIC framework also works well with the KI learner in place of the random fields, we have repeated a double pendulum simulation. The results of the learning process are depicted in Fig. \ref{fig:hfesiic}. In this simulation, we have repeated the stabilisation task of moving the pendulum to the goal state $\xi =[\pi;\pi;0;0]$. Firstly, we recorded the state and control trajectories for an episode of ten seconds of online learning. The resulting squared control error evolution (measuring the squared distances of the state variables to the goal state $\xi$ at each time step) is depicted in Fig. \ref{fig:hfesiic21}. During online learning, we allowed the controller to update the training examples to be updated every $\Delta_\lambda = 0.3$ seconds and set the observational uncertainty level to $\varepsilon \equiv 0.01$. In the initial round, the controller was unsuccessful to stabilise the double pendulum. Next, we repeated online learning for another nine episodes. Then, we restarted the trained controller with learning switched off. This time, the controller was more successful in achieving the task, without further learning, although having some remaining error that seemed to become worse again towards the end of the recorded time span (see Fig. \ref{fig:hfesiic22}). As expected, this remaining error was removed when we restarted the simulation on the bases of additional learning experience (refer to  Fig. \ref{fig:hfesiic23}). The control signal generated by KI-SIIC in the last run is depicted in Fig. \ref{fig:hfesiic4}. 
Unsurprisingly, the control signal generated by kinky inference can indeed be ``kinky'', i.e. non-smooth. This in contrast to RF-SIIC which produced smooth control signals once learning was switched off. We attribute this behaviour to the kinks in the predictions of the kinky inference rule. However, in applications where this ought to be a problem, we expect to be able to alleviate this issue by replacing the vanilla KI rule by the smoothed version introduced in Sec. \ref{sec:SKI}.



%
 %\begin{figure}
        %\centering
			%\subfigure[State evolution (1st round).]{\label{fig:hfesiic1}
    %\includegraphics[width = 3.9cm]{content/Ch_kinkyinf/figs/hfesiic1}
  %}
%%
	%\subfigure[Control evolution (1st round).]{\label{fig:hfesiic2}
   %\includegraphics[width = 4cm, clip, trim = 0cm 0cm 0cm 0cm]
%{content/Ch_kinkyinf/figs/hfesiic2}
  %} 
	%\subfigure[State evolution (after learning).]{\label{fig:hfesiic3} 
    %\includegraphics[width = 3.9cm]{content/Ch_kinkyinf/figs/hfesiic3}
  %}
	%%
 	%\subfigure[Control evolution  (after learning).]{\label{fig:hfesiic4} 
    %\includegraphics[width = 4cm, clip, trim = 0cm 0cm 0cm 0cm]{content/Ch_kinkyinf/figs/hfesiic4}
  %}
%
        %\caption{Fig. \ref{fig:hfesiic1}: State trajectory of the first online learning round. The blue and green lines are the configurations $q_1,q_2$ (angles in radians), respectively. The red and cyan lines are the pertaining velocities. Fig. \ref{fig:hfesiic2}: The control signal. As in Ch. \ref{ch:SPSIIC}, clearly visible are the drops to zero injected to take measurements about $a$ without the influence of $b$. Fig. \ref{fig:hfesiic3} and Fig. \ref{fig:hfesiic3} show the state and control trajectories in the 20th run with learning switched off. This run was preceded by $10$ episodes of online learning lasting ten seconds each. As can be seen from the plots, no additional learning was necessary to successfully stabilise the pendulum.}
%\label{fig:hfesiic}
%\end{figure}	 

\begin{figure}
        \centering
			\subfigure[Error evolution (1st trial).]{\label{fig:hfesiic21}
    \includegraphics[width = 3.9cm]{content/Ch_kinkyinf/figs/HfeSIIC_sqrddist2ep}
  }
%
	\subfigure[Error evolution (10 trials).]{\label{fig:hfesiic22} 
    \includegraphics[width = 3.9cm]{content/Ch_kinkyinf/figs/HfeSIIC_sqrddist10ep}
  }
	%
 	\subfigure[Error evolution  (20 trials).]{\label{fig:hfesiic23} 
    \includegraphics[width = 4cm, clip, trim = 0cm 0cm 0cm 0cm]{content/Ch_kinkyinf/figs/HfeSIIC_sqrddist20ep}
  }
	 	\subfigure[Control evolution  (after learning).]{\label{fig:hfesiic4} 
    \includegraphics[width = 4cm, clip, trim = 0cm 0cm 0cm 0cm]{content/Ch_kinkyinf/figs/hfesiic4}
  }


        \caption{Fig. \ref{fig:hfesiic21}- Fig. \ref{fig:hfesiic21}: Depicted are the squared distances to the goal as a function of time steps. The abscissa marks the time steps the squared distances were recorded. The step size was 0.01 seconds. The blue and green lines are the squared distances to the goal (i.e. errors) of the configurations $q_1,q_2$ (angles in radians), respectively. The red and cyan lines are the pertaining squared velocity errors. Fig. \ref{fig:hfesiic21} shows the squared errors during the first episode of online learning. Fig. \ref{fig:hfesiic22} shows the squared error evolution during control (with online learning switched off) on the basis of learning experience gathered over the course of 10 preceding learning episodes of 10 seconds each. Fig. \ref{fig:hfesiic23} depicts this error evolution on the basis of 20 preceding episodes. Not surprisingly, the controller becomes better at controlling the plant with increased learning experience. The last plot depicts the control evolution (as a function of time in seconds) of the last episode (with learning switched off).
}
\label{fig:hfesiic}
\end{figure}	



\subsection{Kinky inference in inverse dynamics model learning (KI-IML)}
So far, we have considered the learning of \textit{forward} dynamic models of the form $\dot x = \psi(x,u)$ which we identified and then feedback linearised.  An alternative that has become popular in robotics is \textit{inverse (dynamics) model learning (IML)}.
The inverse dynamics model is the mapping $\psi^{-} : \statespace \times \statespace \to \ctrlspace,$
$ (x,\dxref) \mapsto u$ where $\dxref$ is a desired reference state derivative. In a configuration space formulation this translates to a mapping $ (q,\dot q,\ddot q) \mapsto u$ which can be learned by observing data of the form $\data =\{ \bigl((q_i,\dot q_i, \ddot q_i), u_i) \bigr)| i=1,...,N\}$. While having the disadvantage of having to learn over a markedly higher dimensional space, the advantage is that being a black-box model, the IML approach has a great degree of flexibility. Also, because it does not linearise the dynamics, it might be able to benefit from the intrinsic properties of the dynamics rather than cancelling them.


Learning inverse dynamic models with standard Gaussian process regression has been considered in \cite{GPbook:2006,Chai2008}. Analogous approaches have considered the application of nonparametric learning methods to learning inverse kinematics models \cite{souza2001} or inverse operational space models \cite{Petersoperational2006}.
To speed up computation of the IML problem, 
Tuong et. al. \cite{TuongSeegerPeters2009} propose to combine the predictions of many GPs (each having small data sets that contain localised information) to make local predictions at different parts of state space. 
A similar idea, but with linear prediction models, had been proposed in LWPR \cite{lwpr2000,Schaal2002}.
In their paper, Tuong et. al. \cite{TuongSeegerPeters2009} compare a variety of learning methods against standard Gaussian process regression (GPR) for learning inverse dynamic models of real robots. Their data suggests that GPR requires high computational cost for learning and prediction but outperforms other methods such as LWPR \cite{lwpr2000} and LGP \cite{TuongSeegerPeters2009} in terms of prediction accuracy and tracking performance. 
Therefore, we use the standard method of GPR as a baseline method. We will refer to the resulting controller as \textit{GP-IMLC} and compare it to a controller that substitutes the GP by our kinky inference learner. This new controller will be referred to as \textit{kinky inference inverse model learning (KI-IML)}.

Note, in order to speed up computation, we could just as easily apply the localisation methods proposed in \cite{TuongSeegerPeters2009} to the KI-IML approach. This may also have the advantage that a variety of localised KI-IML models would benefit from local estimates of the H\"older constant.
For now however, we restrict ourselves to the standard method. To test the viability of kinky inference for inverse dynamics model learning and control, we repeated our double-pendulum experiment from the previous subsection. This time, we replaced the KI-SSIC controller by KI-IML. 

Note, without further modifications,  KI-IML per se does not lend itself to online learning. To see this, consider a situation where at time $t$, the system is in a state $x(t) = [q(t);\dot q(t)]$ where the KI rule is very uncertain about the reference acceleration $\ddot q_{ref}$. Furthermore, if the present acceleration $\ddot q$ is very distinct from the desired one $\ddot q_{ref}$ (as measured by metric $\metric_\inspace$) then incorporation of a new sample point $\Bigl( \bigl(q(t), \dot q(t), \ddot q(t)\bigr),u\bigl(q(t), \dot q(t), \ddot q(t)\bigr)\Bigr) $ provides little information about the control $u\bigl((q(t), \dot q(t), \ddot q_{ref} \bigr)  \bigr)$ for the reference acceleration $\ddot q_{ref}$. This may mean that the controller may fail to reach the goal. As a solution, it might be conceivable to feed the controller a reference trajectory that smoothly connects the true reference with the current state and acceleration. However, we will not consider this any further. Instead, we will confine our exposition to offline learning.




To this end, we generate an offline sample set $\data$ containing tuples of the form $\Bigl( \bigl(q, \dot q, \ddot q\bigr), u \Bigr) $. The sample inputs $\bigl(q, \dot q, \ddot q\bigr)$ were drawn uniformly at random from the hyperrectangle $[-10,10]^4 \times [-50,50]$. That is, the state training example inputs were allowed to assume values between $-10$ and $10$ while we drew  accelerations from the larger interval [-50,50]. The H\"older constant was adapted to the random sample utilising the lazy update rule outlined in Sec. \ref{sec:lazylipconstupdate}. On the basis of the accordingly adapted KI rule, the pertaining control was determined by inverting the ground-truth dynamics with these inputs (and adding a bit of noise of magnitude up to 0.01). 

We tested the control performance of KI-IML in our double-pendulum test-bed. Here, KI-IML made inference  about the correct control on the basis of the sample $\data$. As a reference acceleration, we chose $\ddot q_{ref} = w(\xi_1 - q) + w (\xi_2 -\dot q)$ where $\xi_1 $ was the goal angle setpoint and $\xi_2$ the goal angular velocity. This choice means that in the limit of dense data, a perfectly trained KI-IML controller would control the system such that the closed-loop dynamics would mimic a double-integrator controlled by a P-controller with setpoint $\xi$.


\begin{figure}
        \centering
			\subfigure[Double-pendulum controlled by KI-IMLC.]{\label{fig:IML0}
    \includegraphics[width = 6.5cm]{content/Ch_kinkyinf/figs/HfeIML_animatehist2}
  }
				\subfigure[Error evolutions (1st try).]{\label{fig:IML1}
    \includegraphics[width = 4.5cm]{content/Ch_kinkyinf/figs/distIMLvSIICpend2}
  }
%
	\subfigure[Error evolutions (2nd try).]{\label{fig:IML2} 
    \includegraphics[width = 4.5cm]{content/Ch_kinkyinf/figs/distIMLvSIICpend2_allhyperparoptbadGPIML}
  }				

%
	%\subfigure[Error evolutions (2nd try).]{\label{fig:IML2} 
    %\includegraphics[width = 3.9cm]{content/Ch_kinkyinf/figs/distIMLvSIICpend2_allhyperparoptbadGPIML}
  %}
	%
 	%\subfigure[Error evolution  (20 trials).]{\label{fig:hfesiic23} 
    %\includegraphics[width = 4cm, clip, trim = 0cm 0cm 0cm 0cm]{content/Ch_kinkyinf/figs/HfeSIIC_sqrddist20ep}
  %}
	 	%\subfigure[Control evolution  (after learning).]{\label{fig:hfesiic4} 
    %\includegraphics[width = 4cm, clip, trim = 0cm 0cm 0cm 0cm]{content/Ch_kinkyinf/figs/hfesiic4}
  %}


        \caption{Fig. \ref{fig:IML1}: Example of KI-IML being successful at driving a learned double-pendulum to goal state $\xi = [\pi;\pi/2;0;0]$. Fig. \ref{fig:IML1}: Depicted is a comparison of the error evolutions, i.e. the distances to the goal as a function of time (seconds), of the control task solved by different methods. All methods managed to stabilise the system well on the basis of the randomly generated data set. Fig. \ref{fig:IML2} exposes a recurring issue we encountered with GP-IML. Depending on the randomly generated data set, GP-IMLC sometimes failed. We attribute this to the outcome of hyperparameter optimisation.
}
\label{fig:IML1}
\end{figure}	




As a first illustration, consider Fig. \ref{fig:IML0}. On the basis of a random data set of size 20, and with reference parameter $w =20$, we tasked KI-IMLC to control the double-pendulum to reach the goal state $\xi=[\pi;\pi/2,0;0]$. In this situation, KI-IMLC had no difficulty. As a first comparison, we redid the experiment with the different the different algorithms GP-IMLC, RF-SIIC (from Ch: \ref{ch:SPSIIC}), KI-IMLC and KI-SIIC. For the purposes of the comparison, the SIIC methods were trained offline on the same randomly generated data set as the other methods. As in previous experiments, the initial state was $x_0=[0;0;-1;-1]$ and the goal state was chosen to be $\xi=[\pi;\pi/2,0;0]$. The random field methods, were allowed to perform hyperparameter optimisation.
In the first run (Fig. \ref{fig:IML0}), all methods accomplished the task with little rest error.
However, repeating experiments like this several times, we frequently encountered GP-IMLC struggling on a variety of instances. Inspecting the trained hyperparameters gives us reason to conjecture that this might be due to the fact that the optimisation hyperparameter optimisation procedure failed to produce good results and got stuck in a local minimum of the marginal posterior log-likelihood. Note, we did not register this problem with any of the other methods. One explanation might be the fact that, owing to the increased dimensionality of the input space in the IMLC setup, GP-IMLC had to optimise over a higher-dimensional space than RF-SIIC. As a note of caution though, is that in the present setup, both methods are not entirely comparable on a level playing field. This is results from the fact that in the current setup, GP-IMLC generated the control by imitating a feedback controller via pure learning. By contrast, the feedback pseudo-control employed in the SIIC method may be able the compensate for some learning error (provided the model over $b(x)$, as defined above, is not profoundly off). 

While time did not permit this, in future work, we would like to make a more extensive comparison on higher-dimensional robotic tracking tasks. Here, we would endow the methods with forward references (instead of eror feedback). We anticipate that this will increase comparability and shed light on the respective inherent benefits and drawbacks more clearly. 

%
%%Simulations}
%In the related work that has applied GP-IML to robotic tracking (e.g. \cite{tuongACC2008}) the authors trained the models with large numbers of data points (around 1000) and on exactly  
%
%Note that the random generation of the offline data set gives the learners a harder task than in the related literature on GP-IML tracking in robotics \cite{tuongACC2008,TuongSeegerPeters2009}. In lieu to imitation learning, in these works, the authors trained their models with large data sets that contained records from the robot performing the desired tasks. This means that the data sets contained exactly the right kind of information. Similarly, in the online learning scenarios considered in Ch. \ref{ch:SPSIIC} and in the previous subsection, the data sets could be kept sparse since the controller automatically decided whenever a data point promised to be informative. 
%
%By contrast, the random selection of data points in the simulations of this section means that the majority of examples will bear little information about the situations that are encountered during online control.
%This means we will require much larger data sets to guarantee comparable density in those parts of state (and acceleration) space that matter.



==> content2/Ch_kinkyinf/KI_core.tex <==




\subsection{Kinky Inference}
\label{sec:KI_core}
In this section, we will introduce the class of learning rules we refer to as \emph{Kinky Inference}. They encompass a host of other methods such as Lipschitz Interpolation and Nonlinear Set Interpolation.  The approach also fits into the more general framework of inference over group mappings considered in Sec. \ref{sec:group_learners}. 
%
%We will then establish some theoretical guarantees for certain parameter settings, in particular of the sequence of Lipschitz parameters $L(n)$. In subsequent parts of this section we will then consider a method for adapting these parameters to the data yielding a rule we will refer to as \emph{Lazily Adapted Constant Kinky Inference (LACKI)}. The section culminates in establishing universal approximation guarantees for our LACKI rule.

The rules possess a parameter $L(n)$ that needs to be specified by any KI algorithm. In this paper, we are most concerned with studying LACKI, a KI rule algorithm where $L(n)$ coincides with a noise-robust and multi-variate generalisation of Strongin's estimate \cite{Strongin1973} of a H\"older constant computed from the data set $\data_n$ available at time step $n$. 

%We will consider the special case $\inspace = \Real^d, \outspace \subseteq \Real^m$ with pseudo-metric $\metric_\inspace$ on the input space and output-space metric defined by $\metric_\outspace(x,x') := \norm{x-x'}_\infty , \forall x,x' \in \inspace$. 

%\subsubsection{Conservative learning and inference in a nutshell}
%
%The general approach we will consider is as follows. We desire to learn a function $f$ based prior knowledge of the form that $f \in \mathcal K_{prior}$ and some (noisy) function sample $\data$. 
%The task of conservative inference over functions (i.e. learning) then is the step of forming a posterior belief of the form $f \in \mathcal K_{post}= \mathcal K_{prior} \cap \mathcal K(\data)$. Here,
%$\mathcal K (\data)$ is the set of all functions that could have generated the observed data. 
%The conservatism lies in the fact that we have not ruled out any candidate functions that are consistent with our information. 
%To perform inference over a function value at input $x$ in a conservative manner, we merely infer that $f \in \prederrbox(x) =[\boden(x), \decke(x)]$ 
%where \textit{floor function} $\boden(x) =\inf_{\phi \in \mathcal K_{post}} \phi(x)$ and  \textit{ceiling function } $\decke(x) = \sup_{\phi \in \mathcal K_{post}} \phi(x)$ delimit the values that any function in the posterior class $\mathcal K_{post}$ could give rise to. If a point prediction of a function value is required, we could choose any function value between the values given by the floor and ceiling which also give rise to the bounds on the point prediction. 
%Of course, the type of inference we get from this general procedure depends on the chosen prior class $\mathcal K_{prior}$ and the specifics of the data. We will develop \textit{kinky inference} which is a method for considering prior classes of multi-output functions over metric input spaces that are optionally constrained by boundedness and by knowledge of H\"older regularity as well as knowledge on uncertainty bounds on the observations and function inputs. For this class of inference mechanisms we prove conservatism and convergence guarantees to the learning target. What is more, we will consider classes where the imposed regularity assumptions are uncertain or adapted lazily to adjust for overly restrictive prior assumptions that do not fit the observations.
%
%
%
%This capability of imposing boundedness assumptions, accommodating for noise and being able to adjust the regularity assumptions will prove of great importance in the 
%control applications of our method.
%
%\subsection{The framework of conservative inference -- definitions, setting and desiderata }
%\label{sec:prob_def}

%As a basic example, consider the ordinary differential equation $\frac{\d x}{\d t} = (\xi - x)$ where $\xi: I \subset \Real \to \Real $ is an absolutely continuous function superimposed by a countable number of steps. Suppose, the ODE describes the trajectory $x: I \to \Real$ of a controlled particle in one-dimensional state space. Based on $N$ time-state observations $D_N=(t_1,x_1 ),..., (t_N,x_N )$ we desire to estimate the total distance travelled $S$ in time interval $I$, $S = \int_I x(t) \d t$. Solving


%%\textbf{Setting.}
%Let $(\inspace, \metric_\inspace)$, $(\outspace ,\metric_\outspace)$ be two metric spaces and $f: \inspace \to \outspace$ be a function. Spaces $\inspace, \outspace$ will be referred to as \textit{input space} and \textit{output space}, respectively.
%Assume, we have access to a \textit{sample set} $\data_n:= \{\bigl( s_i, \tilde f_i, \obserr(s_i) \bigr) \vert i=1,\ldots, N_n \} $ containing $N_n \in \nat$ sample vectors $\tilde f_i \in \outspace$ of function $f$ at sample input $s_i \in \inspace$. To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the \textit{grid} of sample inputs contained in $\data_n$.
%
%
%The sampled function values are allowed to have interval-bounded \textit{observational error} given by $\obserr : \inspace \to \Real^m_{\geq 0}$. That is, all we know is that $f(s_i) \in \obserrhyprec_i := [\underline f_1(s_i), \overline f_1(s_i) ] \times \ldots \times [\underline f_d(s_i), \overline f_d(s_i) ]$ where $\underline f_j(s_i) := \tilde f_{i,j} - \obserr_j(s_i)$, $\overline f(s_i) := \tilde f_{i,j} + \obserr_j(s_i)$ and $\tilde f_{i,j}$ denotes the $j$th component of vector $\tilde f_{i}$.
%
%The interpretation of these errors depends on the given application. For instance, in the context of system identification, the sample might be based on noisy measurements of velocities. The noise may be due to sensor noise or may represent numerical approximation errors. As we will see below, $\obserr$ may also quantify \textit{input} uncertainty (that is when predicting $f(x)$, $x$ is uncertain). This is an important case to consider, especially in the context of control applications where the ground truth might represent a vector field or an observer model.
%
%
%It is our aim to learn function $f$ in the sense that, folding in knowledge about $\data_n$, we infer \textit{predictions} $\predf(x)$ of $f(x)$ at unobserved \textit{query inputs} $x \notin G_n$. Being the target of learning, we will refer to $f$ as the \emph{target} or \emph{ground-truth} function. 
%
%In addition to the predictions themselves, we are also interested in \textit{conservative bounds} on the error of the inferred predictions. Depending on the hypothesis space under consideration these bounds can be of a probabilistic or deterministic nature. In this chapter, for the time being, we are interested in the latter.
%
%That is, we desire to provide a computable \textit{prediction uncertainty} function $\prederr: \inspace \to \outspace$ such that we can guarantee that for any query $x$, our prediction $\predf(x)$ is within the cube of error given by $\prederr(x)$ as follows 
%
%
%Being interested in conservative worst-case guarantees, we are mostly interested 
%
%
%
%In order to be able to deduce the error bounds around the predictions $\predf$, it is important to impose a priori restrictions on the class of possible targets (the hypothesis space). 

%\textbf{Definitions.}
%
\textbf{Setting.}  Let $\inspace$, $\outspace$ be two spaces endowed with (pseudo-) metrics $\metric_{\inspace}: \inspace^2 \to \Real_{\geq 0}, \metric_\outspace:\outspace^2 \to \Real_{\geq 0}$, respectively. Spaces $\inspace, \outspace$ will be referred to as \textit{input space} and \textit{output space}, respectively. 
It will be convenient to restrict our attention to input and output spaces that are additive abelian groups and which are \emph{translation-invariant} with respect to their (pseudo) metrics. That is, for the input space $\inspace$, we assume $ \metric_\inspace(x+x',x''+x') = \metric(x,x''),\forall x,x',x'' \in \inspace$. 

For simplicity, throughout the remainder of this work, we will assume the output space is the canonical Hilbert space $\outspace = \Real^m$ $(m \in \nat)$ endowed with the $\metric_{\outspace}(y,y') = \norm{y-y'}_\infty, \forall y,y' \in \outspace$. 

Let $f: \inspace \to \outspace$ be a \emph{target} or \emph{ground-truth} function we desire to learn. For our purposes, learning means regression. That is, we utilise the data to construct a computable function that allows us predict values of the target function at any given input.

%\footnote{Extensions to more general output spaces seem very possible, albeit, instead of learning a function, we would then learn a discrepancy from a nominal reference in output space. We will leave this to future work.}
%In contrast, we do not impose restrictions on the input space (pseudo-) metric. 
%While our simulations will consider the deterministic case, it would be entirely possible to consider input spaces that are index sets of stochastic processes endowed with suitable norm metrics. Since the output metric is defined via a norm, we will often drop the subscript of the input metric. That is we may on occasion write $\metric$ instead of $\metric_\inspace$.





Assume that, at time step $n$, we have access to a \textit{sample} or \textit{data set} $\data_n:= \{\bigl( s_i, \tilde f_i \bigr) \, \vert \, i=1,\ldots, N_n \} $ containing $N_n \in \nat$ (possibly erroneous) sample vectors $\tilde f_i \in \outspace$ of \emph{target function} $f$ at sample input $s_i \in \inspace$. 
The sampled function values are allowed to have interval-bounded \textit{observational error} or \emph{noise} given by a bound $\obserr : \inspace \to \Real^m_{\geq 0}$. That is, all we know is that $f(s_i) \in \obserrhyprec_i := [\underline f_1(s_i), \overline f_1(s_i) ] \times \ldots \times [\underline f_d(s_i), \overline f_d(s_i) ]$ where $\underline f_j(s_i) := \tilde f_{i,j} - \obserr_j(s_i)$, $\overline f(s_i) := \tilde f_{i,j} + \obserr_j(s_i)$ and $\tilde f_{i,j}$ denotes the $j$th component of vector $\tilde f_{i}$. 
The interpretation of these errors depends on the given application and this ``noise'' may be deterministic or stochastic. For instance, in the context of system identification, the sample might be based on noisy measurements of velocities and it may be due to sensor noise or may capture numerical approximation error. 

Furthermore, $\obserr$ may also accommodate \textit{input} uncertainty (that is when predicting $f(x)$, $x$ is uncertain) (for details refer to \cite{calliess2014_thesis}). In the course of our theoretical considerations below the error will also serve to absorb the discrepancy between a H\"older and a non-H\"older function.
%
%This is an important case to consider, especially in the context of control applications where the ground truth might represent a vector field or an observer model. Finally, the observational error can also model error around the computation of the metric. This might be of interest if the metric has to be approximated numerically or estimated with statistical methods that provide confidence intervals (in the latter case our predictions also only hold within pertaining confidence bounds). 

\textbf{Learning.}
It is our aim to learn target function $f$ in the sense that, combining prior knowledge about $f$ with the observed data $\data_n$, we infer \textit{predictions} $\predfn(x)$ of $f(x)$ at unobserved \textit{query inputs} $x \notin G_n$. Here, $G_n =\{s_i | i =1\ldots,N_n\}$ refers to the (not necessarily regular) \emph{grid} of sample inputs. In our context, the evaluation of $\predf_n$ is what we refer to as \textit{(inductive) inference}. 
%
%For a discussion of the competing definitions of non-deductive inference in a philosophical context, the reader is referred to \cite{Flach2000}. 
%
The entire function $\predfn$ that is learned to facilitate predictions is referred to as the \textit{predictor}. 

A typical \textit{desideratum} of a good predictor is that it is efficiently \textit{computable} and \textit{converges to the target} (up to the observational error given by $\obserr$) in the limit of increasingly dense data sets.
%Typically,
%the predictor lies in the space that coincides with (or is at least dense in) the a priori hypothesis space $\mathcal K_{prior}$ of conceivable target functions. In this case the predictor can be referred to as a \textit{candidate function} or \textit{hypothesis} \cite{mitchellbook:97}.

%In addition to the predictions themselves, we are also interested in \textit{uncertainty bounds} on the error of the inferred predictions. 
%%Depending on the hypothesis space under consideration, these bounds can be of a probabilistic or deterministic nature. In this chapter, we  restrict ourselves to the latter.
%
%That is, we desire to provide a computable \textit{prediction uncertainty function} $\prederr: \inspace \to \outspace$ such that we \textit{believe} that for any query $x \in \inspace$, the ground truth value $f(x)$ lies somewhere within the \textit{uncertainty hyperrectangle }
%\begin{equation}
%	\prederrbox_n(x) := \Bigl\{ y \in \outspace \, | \, \forall j \in \{1,...,\dim{\outspace}\} : y_j \in \prederrbox_{n,j}(x)\Bigr\}
%\end{equation} around the prediction $\predfn (x)$ where 
%\begin{equation}\label{eq:prederrint}
%	\prederrbox_{n,j}(x) : = [ \predfnj(x) - \prederrnj(x), \predfnj(x) + \prederrnj(x)] 
%\end{equation}
%is referred to as the $j$th \textit{prediction uncertainty} interval.
%Here, $\predfnj(x)$, $\prederrnj(x)$ denote the $j$th components of vectors $\predfn(x), \prederrn(x)$, respectively.

 %As a word of caution, we remark that using the last statement as a definition still seems very broad. 

%\textbf{Desiderata.}
In our context, we will understand a \textit{machine learning algorithm} to implement a computable function that maps a data set $\data_n $ to a 
 $\predf_n$ (and possibly an uncertainty estimate function $\prederr_n$). 

%The resulting learning or inference rule is called \textit{conservative} if the uncertainty quantifications never underestimate the error. That is, based on the an a priori assumption $f \in \mathcal K_{prior}$, we can guarantee $f(x) \in \prederrbox_n(x), \forall x$, regardless of the observed data set $\data_n$.

In this work we will expand on the basis of the following class of predictors to perform learning as inference over unobserved function values:

\begin{defn}[Kinky Inference (KI) rule ] \label{def:KIL}
Let  $\Real_\infty := \Real \cup\{- \infty, \infty\}$ and $\inspace$ be some space endowed with a pseudo-metric $\metric_\inspace$. Let $\lbf,\ubf: \inspace \to \outspace \subseteq \Real_\infty^m$ denote \textit{lower- and upper bound functions}, that can be specified in advance and assume $\lbf(x) \leq \ubf(x), \forall x \in I \subset \inspace$ component-wise. 
Furthermore, let $\obserrpar$ denote a parameter that specifies a deterministic belief about the true observational error bound $\obserr$.
Given sample set $\data_n$, we define the predictive functions $\predfn: \inspace \to \outspace, \prederrn: \inspace \to \Real^m_{\geq 0}$ to perform inference over function values.
For $j=1,\ldots,m$, their $j$th output components are given by:
%Furthermore, define
% $\coeff1,\coeff2 \in \Real_{\geq0}$ such that $\coeff1+\coeff2 =1$ (unless explicitly stated otherwise, we assume $\coeff1=\coeff2 =\frac 1 2)$.
	\begin{align*}
   \predfnj(x) :=& \frac{1}{2} \min\{ \ubf_j(x), \decke_{n,j}(x;L(n)\bigr)\} \\
    &+ \frac{1}{2} \max\{ \lbf_j(x), \boden_{n,j}(x;L(n)\bigr) \},\\
	\prederrnj(x) :=& \frac{1}{2} \min\{ \ubf_j(x), \decke_{n,j}\bigl(x;L(n)\bigr)\} \\
	&- \frac{1}{2} \max\{ \lbf_j, \boden_{n,j}\bigl(x;L(n)\bigr) \}.
	\end{align*}
	Here, $\decke_n\bigl(\cdot;L(n)\bigr), \boden_n\bigl(\cdot;L(n)\bigr): \inspace \to \Real^m$ are called ceiling and floor functions, respectively. Their $j$th component functions are given by
	\[\decke_{n,j}\bigl(x; L(n)\bigr) := \min_{i=1,\ldots,N_n}   \tilde f_{i,j} + L_j(n) \metric^\hexp(x,s_i) + \obserrpar_j(x)\] and 
	\[\boden_{n,j}\bigl(x; L(n)\bigr) := \max_{i=1,\ldots,N_n}   \tilde f_{i,j} - L_j(n) \metric^\hexp(x,s_i) - \obserrpar_j(x),\] respectively.
  Here $\hexp \in \Real, L(n) \in \Real^m, \forall n \in \nat_0$ and functions $\lbf,\ubf,\obserrpar:  \inspace \to \Real_\infty^m$ are parameters that have to be specified in advance. To disable restrictions of boundedness, it is allowed to specify the upper and lower bound functions to constants $\infty$ or $-\infty$, respectively.	
	Function $\predfn$ is the predictor that is to be utilised for predicting/inferring function values at unseen inputs. Function $\prederrn(x)$ is meant to quantify the uncertainty of prediction $\predfn(x)$. 
	%Note, if the data set is fixed (i.e. $n$ does not change), we may sometimes drop the subscript $n$ and write $\predf$ instead of $\predf_n$.
\end{defn}

To provide an intuition, consider the following special case where we have access to a noise-free sample $\data_n$ and suppose 
the target $f$ is a real-valued $L^*-p$ H\"older continuous function. Observing the noise-free sample point $(s_i,f_i)$ constrains the set of function values $f(x)$ to the set $\mathbb S_i(x) =\{ \phi \in \outspace | \metric_\outspace(\phi, f_i) \leq L^* \metric_\inspace(s_i,x) \}$. Considering a set of sample points $\data_n$, target value $f(x)$ is constrained to lie in the intersection $\mathbb S(x)=\cap_{i=1}^{N_n} \mathbb S_i(x)$. It is easy to see that the floor and ceiling functions are tight lower and upper bounds of $\mathbb S(x)$ with $\mathbb S(x) := \{ \phi \in \outspace | \boden_n(x; L^*) \leq \phi \leq \decke_n(x;L^*)\}$. In other words, setting parameter $L(n)$ to the best H\"older constant $L^*$ and bounds $\lbf =-\infty,\ubf=+\infty$ yields a predictor $\predfn(x)$ that for every query $x$ chooses the mid-point of the set $\mathbb S(x)$ of those function values that can possibly be assumed by a H\"older continuous function that interpolates the observed sample. Prediction error $\prederrn(x)$ simply is the radius of the set.

For the case of $p=1$, this approach is known as \emph{Lipschitz interpolation} \cite{Beliakov2006,Zabinsky2003}. Since a set is utilised for interpolation, the approach is also known as \emph{Nonlinear Set Interpolation} \cite{Milanese2004}. Specification of $\ubf,\lbf$ allows us to incorporate additional knowledge and constrain our set $\mathbb S(x)$ further. 
For instance, when estimating densities we might incorporate the knowledge of dealing with nonnegative functions. In this case, it makes sense to set $\lbf$ to a constant value of zero yielding $\mathbb S(x) = \{\phi | \phi \geq 0 \} \cap_{i=1}^{N_n} \mathbb S_i(x) $.

%\begin{figure*}
        %\centering
				  %\subfigure[Initial prediction $\predf_1$.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/akt2learneddrift}
    %\label{fig:KIcollavoidopenlooppredmodels1}
  %} 	 
					  %\subfigure[Improved prediction $\predf_2$.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/akt3learneddrift}
    %\label{fig:KIcollavoidopenlooppredmodels2}
  %} 	
							  %\subfigure[Social cost after each experiment.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm, clip, trim = 3.1cm 9.5cm 4.5cm 9cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/soccost}
    %\label{fig:KIsoccost}
  %} 
	%\label{fig:KIcollavoidopenlooppredmodels}
   %\caption{Belief over drift models based on $\data_1$ and $\data_2 \supset \data_1$ with $\abs{\data_1} = 2, \abs{\data_2} = 100$. Here, the top figures show the predictions of $\predf_{n,3}(s)$ and the bottom plots depict the predictions of $\predf_{n,4}(s)$ for $n =1$ and $n=2$, respectively. The ground-truth drift model was $f(x) = \bigl(0,0, - \sin(0.5 \, x_1), - \sin( 0.5 \, x_2) \bigr)^\top$. Rightmost plot: Social cost after each experiment. Note how the reduced uncertainty translated to reduced social cost of the last experiment (bar plot 3) vs the cost in the second (bar plot 2). While the first experiment (bar plot 1) also accumulated low social cost, a collision occurred.}
%\end{figure*}	 
%
%\begin{figure}
%        \centering
%				  \subfigure[KI prediction with two examples.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.1cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/ex1hfe1.pdf}
%    \label{fig:hfe1}
%  } 	
%	 \subfigure[Refined prediction.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.1cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/ex1hfe2.pdf}
%    \label{fig:hfe2}
%  } 	%\hspace{2cm}
%	  \subfigure[Using a periodic pseudo-metric.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.1cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/ex1hfeperiodic.pdf}
%    \label{fig:hfe3}
%  } 	
%   \caption{Examples of different target functions and full kinky inference predictions. \textbf{Fig. \ref{fig:hfe1} and  Fig. \ref{fig:hfe2}} show kinky inference performed for two and ten noisy sample inputs of target function $x\mapsto \sqrt{\abs{\sin(x)}}$ with observational noise level $\varepsilon =0.3$. The floor function folds in knowledge of the non-negativity of the target function ($\lbf = 0$). The predictions were made based on the assumption of $p=\frac 1 2$ and $L = 1$ and employed the standard metric $\metric_\inspace(x,x') = \abs{x-x'}$. 
%	As can be seen from the plots, the function is well interpolated between sample points with small perturbations. Furthermore, the target is within the bounds predicted by the ceiling and floor functions.
%		\textbf{Fig. \ref{fig:hfe3}} depicts a prediction folding in knowledge about the periodicity of the target function by choosing a pseudo-metric $\metric_\inspace = \Bigl|\sin(\pi \abs{x-x'}\Bigr|$. The prediction performs well even in unexplored parts of input space taking advantage of the periodicity of the target. This time, there was no observational error and the target function was $x \mapsto \abs{\sin(\pi x)} +1$.   }
%			\label{fig:exHfe1}
%\end{figure}	  

%
%\begin{figure}
%        \centering
%							  %\subfigure[Wingrock dynamics.]{
%    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    %\includegraphics[width = 5.5cm]
%								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								%{content/Ch_kinkyinf/figs/hfewingrock_dyn_groundtruth}
%    %\label{fig:KIvs2NN}
%  %} 	
%				  \subfigure[Wingrock dynamics.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 5.5cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/hfewingrock_dyn_groundtruth}
%    \label{fig:hfe5}
%  } 	
%	 \subfigure[Inferred model.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 5.5cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/hfewingrock_dyn_learned}
%    \label{fig:hfe4}
%  } 	%\hspace{2cm}
%	 
%%
%   \caption{Example of a prediction of the KI rule on two-dimensional input space. \textit{Left plot:} the target function being a patch of the wingrock dynamics we will study in Sec. \ref{sec:KIMRAC}. \textit{Right plot:} the predictions inferred on the basis of 100 sample points using metric $\metric_\inspace(x,x') = \norm{x-x'}_\infty$ and $p=1, L=2.5$.}
%		\label{fig:exHfe2}
%\end{figure}	 

%Note the inference rule is nonparametric in that, that its complexity grows with the sample size. However, as any inference method one has to a priori specify prior knowledge, some of which is encoded in hyper-parmeters. In the KI rule, these parameters include the choice of pseudo-metric (or its parameters), parameter $\hexp$, the sequence of constants $\seq{L(n)}{n \in \nat}$ as well as the presupposed level of observational error $\obserr$.

%To develop a first feel for this kinky inference rule, we plotted some examples of target functions and pertaining predictions in Fig. \ref{fig:exHfe1}. %and Fig. \ref{fig:exHfe2}.
%Firstly, we can see that the predictions involve kinks. This is due to the minimisations and maximisations that occur in the computation of the ceiling and floor functions which introduce kinks into the prediction signal. This property provided the motivation behind the term ``kinky inference'' \cite{calliess2014_thesis}.

When choosing $L(n)$ to coincide with the best H\"older constant, one can give strong guarantees of convergence to the target as on the tightness of the prediction bounds  \cite{calliess2014_thesis}. 
Unfortunately, this requires us to know at least an upper bound of $L^*$ and therefore, several authours have proposed different approaches of how to estimate the constant from the data (e.g. \cite{Strongin1973,Wood1996}). However, it appears to be largely unknown how to do so in the presence of bounded observational noise $\obserr >0$ in a principled manner. Furthermore, when we replace $L(n)$ by the empirical estimates, nothing seems to be known about the convergence properties of the resulting kinky inference rule that is based on these estimates.  

In the remainder of the paper, we shall address this gap. Firstly, we propose a choice a lazy estimator for to be utilised in place of $L(n)$ that can be set to be robust to noise (i.e. does not grow unbounded). We then prove universal approximation properties of the LACKI rule before examining its performance in a control application.

%\textbf{Properties.}
%%
%%For now, we assume we are given constant $$
%Given H\"older constant $L^* \in \Real^m_+$ and exponent $p \in [0,1]$ we define  $\hoelset {L^*} {\metric_\inspace} p =\{ f: \inspace \to \outspace \subset \Real^m \, |  \forall j \in \{1,\ldots,m\} \forall x,x' \in \inspace: \abs{f_j(x) - f_j(x')}  \leq \, L_j^* \metric^p_{\inspace}(x,x') \}$ to be the class of $L_j^*-p$- H\"older continuous functions with respect to (pseudo-) metric $\metric_\inspace$. Furthermore, let $\bfset :=\{\phi : \inspace \to \outspace \, | \, \forall x \in \inspace, j \in\{1,...,m\}: \lbf_j(x) \leq \phi_j(x) \leq \ubf_j(x)\} $
%denote the set of all functions bounded component-wise between functions $\lbf,\ubf: \inspace \to \Real_\infty^m$.
%
%The next theorem tells us that for targets contained in the intersection of these two function classes, our kinky inference rule as per Def. \ref{def:KIL} is monotonically convergent (in the limit of dense sample grids) and provides conservative yet optimally tight uncertainty bounds, provided that parameters are set appropriately.
%
%\begin{thm} \label{thm:KIdesiderata}
%
%Let the target $f: \inspace \to \outspace$ be contained in the class   
%%\begin{equation}
%	$\mathcal K_{prior}= \bigl\{ f : \inspace \to \outspace \subseteq \Real^m |  f \in \hoelset L {\metric_{\inspace}} \rho \cap \bfset \bigr\}$. Furthermore assume the parameters of the KI rule as per as per Def. \ref{def:KIL} are chosen to be 
%	$L(n) := L^*$  ($n \in \nat_0$).
%%\end{equation}
%Then the inference rule exhibits the following properties:
%\begin{enumerate}
%	\item \textit{Conservatism:} $\forall x \in \inspace: f(x) \in \prederrbox_n(x)$.
%	\item \textit{Monotonicity:} Additional data cannot increase the uncertainty. 
%	%
%	That is, $\data_n \subseteq \data_{n+1} $ implies 
%		$\prederrbox_n(x) \supseteq \prederrbox_{n+1}(x)$ or equivalently, $\prederr_n(x) \geq \prederr_{n+1}(x), \forall x \in \inspace$ (where the inequality holds for each component).
%	%\item \textbf{Convergence} to the target: Let the set of sample inputs $G_n$ in $D_n$ converge to a dense subset of domain $I \subset \inspace$ and for each input $x \in I$ let the sample error function $\obserr: I \to \Real_{\geq 0}$ be bounded by $m_x \geq 0$ in some neighbourhood of $x$. Then, we have 
%%\begin{itemize}
%%\item (a) The uncertainty converges point-wise: $\forall x \in I: 0 \leq \lim_{n \to \infty} \prederrn(x) \leq m_x$.
%%In particular, the enclosure converges to the target $f(x)$ at inputs $x$ where $m_x=0$.  
%		%
%		%\item (b) If convergence of $G_n$ is uniform and the target observations are error-free, i.e. $m_x = 0, \forall x \in I$, then the enclosure converges to the target $f$ uniformly.
%%\end{itemize}	
%	\item \textit{Convergence}: If $(G_n )_{n \in \nat }$ is a sample grid sequence of inputs converging to a dense subset of $I \subset \inspace$ (as $n \to \infty$) then  $\prederrn(x) \stackrel{n \to \infty}{\longrightarrow} \obserr(x), \forall x \in I$. If convergence of the grid to the dense subset is uniform and the observational error is zero everywhere ($\obserr(x) = 0, \,\forall x$) then the convergence  $\prederrn \stackrel{n \to \infty}{\longrightarrow} 0$ is uniform on $I$. 
%	   \item \textit{Minimality}: There is no conservative uncertainty bound that is tighter than $\prederr_n$.
%%If an enclosure $\mathcal E^b_a$  satisfies \emph{Desideratum 2} then it is a superset of our enclosure $\einschluss$, i.e. $b \geq \decke_n, a \leq \boden_n$, $\einschluss \subseteq \mathcal E^b_a$.    
%\end{enumerate}
%%\begin{enumerate}
%%\item  
%
%%\item If in addition, for some $d \in \nat$, $\inspace \subseteq \Real^d$ and $\metric_{\inspace}(x,x') = \norm{x-x'}$ for some norm that is equivalent to the Euclidean norm then the inference mechanism is also optimal (as per Desideratum 4 in Def. \ref{def:KIdesiderata}). That is, there is no other conservative inference mechanism with tighter uncertainty bound function $\prederrn$. 
%%\end{enumerate}
%\end{thm}
%\begin{proof}
%The proof is contained in \cite{calliess2014_thesis}.
%\end{proof}
%
%%We have assumed that the H\"older exponent $p \in(0,1)$ is a free parameter. It is well known that The following Lemmata tell us that our inference rule is typically conservative and appropriate if we choose $p$ as the assumed H\"older exponent, as long as it does not exceed the (largest) H\"older exponent of the target function.
%
%
%
%
%\textbf{Computational effort.} 
%We can see from Def. \ref{def:KIL} that the kinky inference method can be classified as a supervised nonparametric learning method with prediction effort growing linearly with the data set size $\abs{\data_n} = N_n$. If the computational effort for computing the metric for a given input is in the class $\mathcal O(\delta)$ and the computational effort for computing the bounding functions $\lbf$ and $\ubf$ is in $\mathcal O(\beta)$ then the computational effort for computing the prediction functions is generally in $\mathcal O\bigl(m (N_n \delta+\beta) \bigr)$. On the other hand, batch learning simply requires storing the $N_n$ data points, which generally can be done in the order of $\mathcal O\bigl((m+d) N_n \bigr)$ where $d$ denotes the input space dimensionality. In incremental learning, the computation required to add a new data point requires a computation in $\mathcal O(m+d)$.
%
%For the special case of $d=m=1$, with $p=1$, no error $\obserr = 0$, metric $\metric_\inspace(x,x') = \abs{x-x'}$ and bounds $\lbf=-\infty, \ubf =\infty$, our inference rule reduces to the interpolation rule considered in \cite{Zabinsky2003}. Here, the prediction only depends on the two most adjacent data points. Finding those can be accomplished by binary search in $\mathcal O(\log N_n)$, provided the inputs are stored in an ordered list.



%For example, in case the simple metric $\metric_\inspace(x,x') = \norm{x-x'}$ is utilised and the bounding functions are constant we have $\mathcal O(\delta) = \mathcal O(d)$ and $\mathcal O(\beta) = \mathcal O(1)$, yielding a total computational effort of $\mathcal O(d \, N_n)$ for performing inference. Finally, as we have derived in Sec. \ref{sec:onedimlipfloorceil}, the effort reduces to logarithmic asymptotic complexity $\mathcal O(\log N_n)$ in the one-dimensional case where the metric $\metric(x,x') = \abs{x-x'} $ is used and if $p=1$ (cf. Rem. \ref{rem:lipencl1d4KI}). This can make a significant difference in terms of computational speed of the inference in the presence of large data sets.

%
%\begin{defn}[Desiderata] \label{def:KIdesiderata} With definitions as above, we desire a machine learning algorithm to implement a mapping $\data_n \mapsto (\predfn,\prederrn)$ such that, for all data sets $\data_n$, the resulting inductive inference satisfies the following \textbf{desiderata}:
%\begin{enumerate}
	%\item \textit{Conservatism:} We can guarantee $\forall x \in \inspace \, \forall \phi \in \mathcal K_{prior} \cap \mathcal K(\data_n): \phi(x) \in \prederrbox_n(x)$. In particular, the ground-truth $f$ is always contained in the posterior set and its function values always are contained in the corresponding uncertainty hyperrectangles.
	%\item \textit{Monotonicity:} Additional data cannot increase the uncertainty. 
	%
	%That is, $\data_n \subseteq \data_{n+1} $ implies 
		%$\prederrbox_n(x) \supseteq \prederrbox_{n+1}(x)$ or equivalently, $\prederr_n(x) \geq \prederr_{n+1}(x), \forall x \in \inspace$ (where the inequality holds for each component).
	%%\item \textbf{Convergence} to the target: Let the set of sample inputs $G_n$ in $D_n$ converge to a dense subset of domain $I \subset \inspace$ and for each input $x \in I$ let the sample error function $\obserr: I \to \Real_{\geq 0}$ be bounded by $m_x \geq 0$ in some neighbourhood of $x$. Then, we have 
%%\begin{itemize}
%%\item (a) The uncertainty converges point-wise: $\forall x \in I: 0 \leq \lim_{n \to \infty} \prederrn(x) \leq m_x$.
%%In particular, the enclosure converges to the target $f(x)$ at inputs $x$ where $m_x=0$.  
		%%
		%%\item (b) If convergence of $G_n$ is uniform and the target observations are error-free, i.e. $m_x = 0, \forall x \in I$, then the enclosure converges to the target $f$ uniformly.
%%\end{itemize}	
	%\item \textit{Convergence}: If $(G_n )_{n \in \nat }$ is a sample grid sequence of inputs converging to a dense subset of $\inspace$ (as $n \to \infty$) then  $\prederrn(x) \stackrel{n \to \infty}{\longrightarrow} \obserr(x), \forall x \in \inspace$. If convergence of the grid to the dense subset is uniform (cf. Def. \ref{def:uniform_setconvergence}) and the observational error is zero everywhere ($\obserr(x) = 0, \,\forall x$) then the convergence  $\prederrn \stackrel{n \to \infty}{\longrightarrow} 0$ is uniform. 
	   %\item \textit{Minimality (optimality)}: There is no conservative uncertainty bound that is tighter than $\prederr_n$. That is, if for some hyperrectangle $H$, $x \in \inspace$ we have $H \subsetneq \prederrbox_n(x)$ then we have: $\exists x \in \inspace, \phi \in \mathcal K_{prior} \cap \mathcal K(\data_n) : \phi(x) \notin H$. In particular, it might be possible that the function value of the ground-truth function at $x$ is not contained in $H$.
%%If an enclosure $\mathcal E^b_a$  satisfies \emph{Desideratum 2} then it is a superset of our enclosure $\einschluss$, i.e. $b \geq \decke_n, a \leq \boden_n$, $\einschluss \subseteq \mathcal E^b_a$.    
%\end{enumerate}
%\end{defn}
%
%\begin{rem}
%Note the statement of uniform convergence in the absence of observational error is interesting from a machine learning theoretic point of view. It tells us that if we can construct  a grid sequence $(G_n)_{n \in \nat}$ that uniformly converges to a dense set of the domain $\inspace$ then the worst-case approximation error  $\sup_{x \in \inspace} \norm{ \predfn(x) - f(x) }_{\infty} $ vanishes as $n \to \infty$.
%This can also be of interest in quadrature: if we construct a closed-form expression of the integral of the functions $\decke_n: x \mapsto \predfn(x) + \prederrn(x), \boden_n: x \mapsto \predfn(x) - \prederrn(x)$ then due to uniform convergence, $\int_\inspace f(x) \d x= \int_{\inspace} \lim_{n \to \infty} \decke_n(x) \d x = \lim_{n \to \infty} \int_{\inspace}  \decke_n(x) \d x $ assuming the integrals exists.
%Past work, not included in the thesis, has utilised this result for conservative quadrature of H\"older continuous functions. 
%\end{rem}
%
%%Note, Desiderta 1-3 combined imply that in the absence of observational errors ($\obserr \equiv 0$), the prediction $\predfn$ converges monotonically to the target when data sets become increasingly dense.
%
%\subsection{The kinky inference and nonparametric machine learning mechanism}
%Having specified general desirable properties on conservative inference we will now define an inference rule which satisfies these desiderata under certain conditions.
%This inference rule, which we will call \textit{kinky inference} is defined as follows:
%%We are now in a position to define our kinky inference rule:
%
%\begin{defn}[Kinky inference rule (KIR)] \label{def:KIL}
%Let  $\Real_\infty := \Real \cup\{- \infty, \infty\}$ and $\inspace$ be some space endowed with a pseudo-metric $\metric_\inspace$. Let $\lbf,\ubf: \inspace \to \outspace \subseteq \Real_\infty^m$ denote \textit{lower- and upper bound functions}, that can be specified in advance and assume $\lbf(x) \leq \ubf(x), \forall x \in I \subset \inspace$ component-wise. 
%Given sample set $\data_n$, we define the predictive functions $\predfn: \inspace \to \outspace, \prederrn: \inspace \to \Real^m_{\geq 0}$ to perform inference over function values.
%For $j=1,\ldots,m$, their $j$th output components are given by:
%%Furthermore, define
%% $\coeff1,\coeff2 \in \Real_{\geq0}$ such that $\coeff1+\coeff2 =1$ (unless explicitly stated otherwise, we assume $\coeff1=\coeff2 =\frac 1 2)$.
	%\begin{align}
   %\predfnj(x) &:= \frac{1}{2} \min\{ \ubf_j(x), \decke_{n,j}(x)\} + \frac{1}{2} \max\{ \lbf_j, \boden_{n,j}(x) \} \label{eq:KIpred}\\  
	%\prederrnj(x) &:= \frac{1}{2} \bigl(\min\{ \ubf_j(x), \decke_{n,j}(x)\} - \max\{ \lbf_j, \boden_{n,j}(x) \} \bigr)   \label{eq:KIprederr}
	%\end{align}
	%Here, $\decke_n, \boden_n: \inspace \to \Real^m$ are called ceiling and floor functions, respectively. Their $j$th component functions are given by
	%$\decke_{n,j}(x) := \min_{i=1,\ldots,N_n}   \tilde f_{i,j} + L_j \metric^p(x,s_i) + \obserr_j(x)$ and 
	%$\boden_{n,j}(x) := \max_{i=1,\ldots,N_n}   \tilde f_{i,j} - L_j \metric^p(x,s_i) - \obserr_j(x)$, respectively.
  %Here $p \in \Real, L \in \Real^m$ and functions $\lbf,\ubf,\obserr$ are parameters that have to be specified in advance. To disable restrictions of boundedness, it is allowed to specify the upper and lower bound functions to constant $\infty$ or $-\infty$, respectively.	
	%Function $\predfn$ is the predictor that is to be utilised for predicting/inferring function values at unseen inputs. Function $\prederrn(x)$ quantifies the uncertainty of prediction $\predfn(x)$. 
	%%Note, if the data set is fixed (i.e. $n$ does not change), we may sometimes drop the subscript $n$ and write $\predf$ instead of $\predf_n$.
%\end{defn}
%
%%
%%\begin{defn}[Kinky inference rule (KIR)] \label{def:KIL}
%%Define $\lbf,\ubf: \inspace \to \Real \cup\{- \infty, \infty\}$ to be the \textit{lower- and upper bound function}, and assume $\lbf(x) \leq \ubf(x), \forall x \in I \subset \inspace$. 
%%Given sample set $D_n$ we define the following predictive functions to perform inductive inference:
%%%Furthermore, define
%%% $\coeff1,\coeff2 \in \Real_{\geq0}$ such that $\coeff1+\coeff2 =1$ (unless explicitly stated otherwise, we assume $\coeff1=\coeff2 =\frac 1 2)$.
	%%\begin{align}
   %%\predf_n(x) &:= \frac{1}{2} \min\{ \ubf(x), \decke_n(x)\} + \frac{1}{2} \max\{ \lbf, \boden_n(x) \} \\  
	%%\prederr_n(x) &:= \frac{1}{2} \bigl(\min\{ \ubf(x), \decke_n(x)\} - \max\{ \lbf, \boden_n(x) \} \bigr) \label{eq:KIprederr}\\  
	%%\end{align}
	%%where $\decke_n(x) := \min_{i=1,\ldots,N_n}  \tilde f_i + L \metric(x,s_i)+\obserr(x)$
	%%is called the ceiling 
	%%and $\boden_n(x) := \max_{i=1,\ldots,N_n}   \tilde f_i - L \metric(x,s_i) - \obserr(x)$
	%%is called the floor function.
	%%Function $\predf$ is the predictor that is to be utilised for predicting/inferring function values at unseen inputs. Function $\prederr_n(x)$ quantifies the uncertainty of prediction $\predf_n(x)$. Note, if the data set is fixed (i.e. $n$ does not change), we will drop the subscript $n$ and write $\predf$ instead of $\predf_n$.
%%\end{defn}
 %
%
%\begin{figure}
        %\centering
				  %\subfigure[KI prediction with two examples.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/ex1Hfe1}
    %\label{fig:hfe1}
  %} 	
	 %\subfigure[Refined prediction.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/ex1Hfe2}
    %\label{fig:hfe2}
  %} 	%\hspace{2cm}
	  %\subfigure[Using a periodic pseudo-metric.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/ex1hfeperiodic}
    %\label{fig:hfe3}
  %} 	
	%\label{fig:exHfe1}
   %\caption{Examples of different target functions and kinky inference predictions. \textbf{Fig. \ref{fig:hfe1} and  Fig. \ref{fig:hfe2}} show kinky inference performed for two and ten noisy sample inputs of target function $x\mapsto \sqrt{\abs{\sin(x)}}$ with observational noise level $\obserr =0.3$. The floor function folds in knowledge of the non-negativity of the target function ($\lbf = 0$). The predictions were made based on the assumption of $p=\frac 1 2$ and $L = 1$ and employed the standard metric $\metric(x,x') = \abs{x-x'}$. 
	%As can be seen from the plots, the function is well interpolated between sample points with small perturbations. Furthermore, the target is within the bounds predicted by the ceiling and floor functions.
		%\textbf{Fig. \ref{fig:hfe3}} depicts a prediction folding in knowledge about the periodicity of the target function by choosing a pseudo-metric $\metric = \Bigl|\sin(\pi \abs{x-x'}\Bigr|$. The prediction performs well even in unexplored parts of input space taking advantage of the periodicity of the target. This time, there was no observational error and the target function was $x \mapsto \abs{\sin(\pi x)} +1$.   }
%\end{figure}	  
%
%
%\begin{figure}
        %\centering
				  %\subfigure[Wingrock dynamics.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5.5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/hfewingrock_dyn_groundtruth}
    %\label{fig:hfe5}
  %} 	
	 %\subfigure[Inferred model.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5.5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/hfewingrock_dyn_learned}
    %\label{fig:hfe4}
  %} 	%\hspace{2cm}
	 %
	%\label{fig:exHfe2}
   %\caption{Example of a prediction on two-dimensional input space. \textit{Left plot:} the target function being a patch of the wingrock dynamics we will study in Sec. \ref{sec:KIMRAC}. \textit{Right plot:} the predictions inferred on the basis of 100 sample points using metric $\metric(x,x') = \norm{x-x'}_\infty$ and $p=1, L=2.5$.}
%\end{figure}	 
%
%To develop a first feel for the kinky inference rule, we have plotted some examples of ground-truth functions and pertaining predictions in Fig. \ref{fig:exHfe1} and Fig. \ref{fig:exHfe2}. Firstly, we can see that the predictions involve kinks. This is due to the minimisations and maximisations that occur in the computation of the ceiling and floor functions which introduce breakpoints into the prediction signal. This property provided the motivation behind the term ``kinky inference''.
%
%Secondly, we note that in all the examples, the conservative bounds were accurate. That is, the target remained contained in them. An example where we see how the bounds shrink to the ground-truth (up to the observational error tube) will be given in Sec. \ref{sec:agentexploration}, where we consider an agent that utilises kinky inference to learn a drift vector field it is immersed in. Also, note from Fig. \ref{fig:hfe3} how the choice of distance metric $\metric$ can affect the predictions. In this example, a metric was chosen that took into account a priori knowledge about periodicity of the target function. This allowed predictions to be accurate even in unexplored parts of the input space. 
%
%%\jcom{probably move remark below where the experiments are and we can show a periodic kernel.}
%\begin{rem}[Remarks on the relationship to kernels and distance metric learning]
%Unless altered by $\ubf,\lbf$, the kinky inference predictor assigns similar function values to inputs that are similar (i.e. close) with respect to the chosen input metric. Therefore, the choice of metric is important. Metrics are measures of dissimilarity and therefore, are closely related to similarity measures such as kernels.
%%For instance, we have seen that  $\metric(x,y) := \normtop{x-y}$ defines a proper metric and (uniform) convergence with respect to this metric is equivalent to (uniform) convergence with respect to metric $ D: (x,y) \mapsto \norm{x-y}$ (see Sec. \ref{sec:unifconvhoeldermetricequivmetricunifconv}). 
%In much of the recent machine learning literature, kernel functions are utilised to perform inference.
%Note, a kernel function is a measure of similarity often based on quantities inversely related to metrics (which are dissimilarity measures). In order to gain inspiration about metrics or pseudo-metrics suitable for an application at hand, we can draw on the parts of the kernel learning literature that is concerned with the tailoring of kernels to specific applications  (for a recent overview of \textit{kernel engineering}, including periodic ones, refer to\cite{duvenaud2014}). 
%As we have seen in the example depicted in Fig. \ref{fig:hfe3}, we might consider folding in knowledge of periodicity of the underlying function class. However, as a future direction, one might consider exploring to harness more sophisticated automated kernel construction techniques (e.g. \cite{argyriou2005,Kloft2010,duvenaud2014}) and distance metric learning methods (see \cite{Kulis2012}) that have been developed throughout the machine learning community in recent years.
%\end{rem}
%
%
%
%
%\subsection{Theoretical guarantees}
%
%The examples depicted in the plots of Fig. Fig. \ref{fig:exHfe1} and Fig. \ref{fig:exHfe2} seem to be consistent with what we would expect from an inference mechanism that is conservative and monotonically convergent and hence, might satisfy the desiderata we stated in Def. \ref{def:KIdesiderata}.
%We will now give conditions under which we can guarantee the desiderata to be fulfilled. 
%
%Of course, the validity of our guarantees depends on the a priori hypothesis space $\mathcal K_{prior}$. Inspection of the prediction rules reveals that the minimisation and maximisations eliminate all those function values that do not adhere to boundedness conditions (imposed by $\lbf,\ubf$) and conditions on H\"older continuity up to a margin of error given by $\obserr$. 
%
%That this is exactly the right class for which our desiderata hold is asserted by the following theorem:
%
%\begin{thm} \label{thm:KIdesiderata}
%Assuming all (a priori) possible targets $f: \inspace \to \outspace$ are given by the class   
%\begin{equation}
	%\mathcal K_{prior}= \bigl\{ f : \inspace \to \outspace \subseteq \Real^m |  f \in \hoelset L {\metric_{\inspace}} p \cap \bfset \bigr\}
%\end{equation}
%where $\hoelset L {\metric_\inspace} p =\{ f: \inspace \to \outspace \subset \Real^m \, |  \forall j \in \{1,\ldots,m\} \forall x,x' \in \inspace: \abs{f_j(x) - f_j(x')}  \leq \, L_j \metric^p_{\inspace}(x,x') \}$ denotes the class of $L-p$- H\"older continuous functions with respect to metric $\metric_\inspace$ and $\bfset :=\{\phi : \inspace \to \outspace \, | \, \forall x \in \inspace, j \in\{1,...,m\}: \lbf_j(x) \leq \phi_j(x) \leq \ubf_j(x)\} $
%is the set of all functions bounded component-wise between functions $\lbf,\ubf: \Real^d \to \Real \cup \{- \infty, \infty\}$, where we will always define $\Real_\infty := \Real \cup\{- \infty, \infty\}$. 
%
%Then we have:
%%\begin{enumerate}
%%\item  
%The inference rule as per Def. \ref{def:KIL} is conservative, monotonically convergent (in the limit of dense sample grids) and optimal in the sense of Def. \ref{def:KIdesiderata}. That is, it satisfies Desiderata 1-4 as per Def. \ref{def:KIdesiderata}. 
%%\item If in addition, for some $d \in \nat$, $\inspace \subseteq \Real^d$ and $\metric_{\inspace}(x,x') = \norm{x-x'}$ for some norm that is equivalent to the Euclidean norm then the inference mechanism is also optimal (as per Desideratum 4 in Def. \ref{def:KIdesiderata}). That is, there is no other conservative inference mechanism with tighter uncertainty bound function $\prederrn$. 
%%\end{enumerate}
%\end{thm}
%\begin{proof}
%The statement is derived in the appendix, Sec. \ref{sec:proofKIdesiderata}.
%\end{proof}
%
%%\jcom{Requirements on the regularity of the bound functions or error ? Can metric be a pseudo-metric?}
%
   %%
%%%=================
%%
%%Let  $\Real_\infty := \Real \cup\{- \infty, \infty\}$.
%%In this work, we are primarily interested in functions restricted to be H\"older continuous and bounded component-wise by some known bounding functions $\lbf,\ubf: \inspace \to \Real^m_\infty$. That is, we know the target is contained in 
%%the a priori hypothesis space 
%%\begin{equation}
	%%\mathcal K_{prior}= \bigl\{ f : \inspace \to \Real |  f \in \hoelset L \metric p \cap \bfset \bigr\}
%%\end{equation}
%%where $\hoelset L \metric p =\{ f: \inspace \to \outspace \subset \Real^m \, |  \norm{}  \leq \, \}$ denotes the class of $L-p$- H\"older continuous functions with respect to metric $\metric$ and $\bfset :=\{\phi : \inspace \to \outspace \, | \, \forall x \in \inspace, j \in\{1,...,m\}: \lbf_j(x) \leq \phi_j(x) \leq \ubf_j(x)\} $
%%is the set of all functions bounded component-wise between functions $\lbf,\ubf: \Real^d \to \Real \cup \{- \infty, \infty\}$, where we will always define $\Real_\infty := \Real \cup\{- \infty, \infty\}$. 
%%
%%For ease of notation, we will follow the convention of dropping the subscripts from inequalities and interpret an inequality component-wise. Similarly, if we omit the argument from an inequality, the inequality is understood to hold point-wise. For example, we interpret write $\lbf \leq \phi$ in place of  $\lbf_j(x) \leq \phi_j(x), \forall j,x$. 
%
%%
%%%=======================
%%
%%
%%
%%From the perspective of topological inference, the estimator is a data inference method for function estimation:
%%$B(\cdot) = M_{dinf}(\mathcal K_{prior}, \cdot, \gamma ) $ (for some sufficiently large $\gamma$) mapping sample data into a hypothesis interval of possible functions. 
%%Here,  our a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L_J$ such that the underlying target $f \in \mathcal F$ is $L_J-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L_J \norm{x-x'}\}$. 
%%Note, we will not explicitly compute the prior knowledge set. Instead will will fold in the Lipschitz continuity to define an optimal estimator output defining an enclosure that coincides with $\mathcal K_{post} \subset \mathcal K_{prior}$ and hence, with $T (\mathcal K_{post} \cup \mathcal K_{prior})$. Therefore, the resulting inference mechanism will be optimal. 
%%
%%Note, how our desiderata are equivalent to the corresponding notions of the inference mechanism that is to be designed.
%
%
%%Our method will 
%%
%%We 
%%
%%In this section, we consider hypotheses spaces comprising H\"older continuous functions. This is a very general class of uniformly continuous functions that can exhibit infinitely many non-differentiable points.
%%
%%
 %%In addition to a learned hypothesis, our approach also provides error bounds around each prediction that are conservative and tight. That is, the bounds contain exactly those function within the assumed H\"older class that could have generated the sample. 
%%
%%The rest of the section is structured as follows: First we 
%%
%%
%%
%%Our conservative function estimation procedure constructed upper and lower bound functions that are sample-consistent. The enclosure encompasses all possible candidate functions with an assumed H\"older property that could have generated the sample. Therefore, any H\"older function within the enclosure is a valid hypothesis that could have generated the data and hence, a suitable generalisation model for non-deductive inference. 
%%
%%
%%We assume the dimensionality of the target's input domain $I$ is $d \geq 1$. Remember, we defined the set of function samples as $D_n= \{\bigl( s_i, \tilde f_i, \obserr(s_i) \bigr) \vert i=1,\ldots, N_n \} $. 
%%Let $f$ denote the \textit{ground-truth} or \textit{target function} generating the data. $\tilde f_i$ is a noisy function value such that we know $f(s_i) \in [\tilde f_i - \obserr(s_i) , \tilde f_i + \obserr(s_i)], \, (i=1,\ldots, N_n)$. To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the grid of sample inputs contained in $D_n$.  
%%
%%A robust learning rule is a computable mapping $\mathcal R : D_n \mapsto (\predf, \prederr) $.
%%Here $\predf$ is a predictor allowing to make inductive inference and $\prederr(x)$ quantifies the uncertainty or error around the prediction $\predf(x)$.
%%
 %%
%%Let $\metric: \inspace^2 \to \Real$ be a metric. We propose the following nonparametric inference rule:
%
%\subsubsection{Computational effort}
%We can see from Def. \ref{def:KIL} that the kinky inference method can be classified as a supervised nonparametric learning method. That is, the computational effort for predicting grows with the data set size $N_n$. If the computational effort for computing the metric for a given input is in the class $\mathcal O(\delta)$ and the computational effort for computing the bounding functions $\lbf$ and $\ubf$ is in $\mathcal O(\beta)$ then the computational effort for computing the prediction functions is in  $\mathcal O(N_n \delta+\beta)$. 
%For example, in case the simple metric $\metric_\inspace(x,x') = \norm{x-x'}$ is utilised and the bounding functions are constant we have $\mathcal O(\delta) = \mathcal O(d)$ and $\mathcal O(\beta) = \mathcal O(1)$, yielding a total computational effort of $\mathcal O(d \, N_n)$ for performing inference. Finally, as we have derived in Sec. \ref{sec:onedimlipfloorceil}, the effort reduces to logarithmic asymptotic complexity $\mathcal O(\log N_n)$ in the one-dimensional case where the metric $\metric(x,x') = \abs{x-x'} $ is used and if $p=1$ (cf. Rem. \ref{rem:lipencl1d4KI}). This can make a significant difference in terms of computational speed of the inference in the presence of large data sets.
%%
%%
%%
%%\subsection{Uncertain inputs}
%%So far, we have considered output uncertainty but not input uncertainty. That is, we have assumed that the function values $f(s_i)$ at the sample inputs are uncertain but that query inputs $x$ as well as sample 
%%inputs $s_i$ are known exactly. However, in many applications this assumption typically is not met. For example, in Sec. \ref{sec:hfeandcontrol}, we will employ KI for learning and controlling dynamic systems.
%%Here the target functions are state-dependent vector fields. Here, the state measurements often are corrupted by noise (e.g. due to sensor noise or delays) which can affect both training data and query inputs. In the latter case, the controller might query the KI method to predict 
%%a function value $f(x)$ based on the assumption of the plant being in state $x$ while the plant may in fact be in a different state $x+\delta_x$. We would like to guarantee that our inference over the actual function value still is within the predicted bounds provided the input estimation error $\delta_x$ is known or known to be bounded. 
%%Fortunately, the H\"older property of the target can help to address the problem of quantifying the prediction error due to input uncertainty. For instance, consider $\metric(x,x') = \norm{x-x'}$. By H\"older continuity, the error of the prediction of the $j$th output component of the target function $f$ is bounded by $\abs{f_j(x+\delta_x) - f_j(x)} \leq \norm{\delta_x}^p$. 
%%
%%Firstly, assume the training inputs $s_i$ were certain but the query inputs $x$ during prediction are uncertain.
%%Therefore, assuming we know an upper bound $\errinp(x)$ on the input uncertainty, i.e. 
%%$\norm{\delta_x}^p\leq \errinp(x), \forall x$, we can add this term to the uncertainty estimate $\prederr(x)$ as per Eq. \ref{eq:KIprederr}.
%%%This means that the additional uncertainty only affects the prediction of this particular query point. 
%%
%%Secondly, consider the case were both the sample inputs $s_i$ and the query inputs $x$ are uncertain with the uncertainty being quantified by the function $\errinp(\cdot)$. In this case, the uncertainty of the sample inputs
 %%affects the posterior hypothesis (i.e. the enclosure) over $f$ and hence, the inferences over function values at all inputs. 
%%By the same argument as for the case of query noise, we accommodate for this fact leveraging the H\"older property. Instead of adjusting just the prediction uncertainty, we simply add $ \errinp(\cdot)$ to the error function $\obserr(\cdot)$ (that we have previously used to model observational 
%%error of the function values). That is, the observational uncertainty model has absorbed the input uncertainty.  Predictions with uncertain query points can then be done as per Def. \ref{def:KIL} (but with $ \errinp(\cdot)+ \obserr(\cdot)$ in place of $\obserr(\cdot) )$.
%%
%%
%%\subsection{A smoothed inference rule} \label{sec:SKI}
%%The inferred predictor of kinky inference as per Eq. \ref{eq:KIpred} contains kinks. In certain applications, this can be disadvantageous. For instance, below we will feed the predictor into a control signal. However, in applications such as robotics, smooth controllers are typically preferred over non-smooth ones since the latter give rise to increase wear and tear of the actuators. With this in mind we will consider a modification of the predictor which filters the prediction output through a smoothing filter as known from computer vision \cite{forsyth2002,Baessmann2004}. The idea is to convolve the predictor with a function that implements a low-pass filter and abates high frequencies thereby smoothing out rough transitions in the signal. 
%%For now, we will restrict the exposition to one-dimensional input and output spaces. However, extensions to multiple output dimensions result from following our steps through for each component function. Extensions to multi-dimensional input spaces follow by taking advantage of the corresponding filters developed for multi-dimensional signal processing (see e.g \cite{young1995,Prorakis2006}). 
%%As an example, for some $n \in \nat, w_i \geq 0 \, (i=1,...,n)$ and (typically small) step size $\sigma \in \Real \geq 0$, consider the modified prediction rule (\textit{smoothed kinky inference (SKI) rule} ):
%%%
%%\begin{equation}
%%f_n^* = \frac{1}{\sum_{i=-q}^q w_i} 
%%\sum_{i=-q}^q w_i \predfn (x+i \sigma) .
%%\end{equation}
%%%
%%Either $w_0 = 2$ and $w_{-1}=w_2 =1$ or $w_{-2} = w_2 = 7, w_{-1}=w_1 = 26, w_0 = 41$  are common choices for discrete approximations of a Gaussian filter \cite{Baessmann2004}. 
%%
%%A comparison of the predictions made by the {smoothed kinky inference rule (SKI) } against the prediction function of the standard kinky inference rule is depicted in Fig. \ref{fig:exSKI1}. As can be seen from the plot, in the SKI prediction the kinks have been smoothed out while all the predictions still are contained within the prediction bounds given by the floor and ceiling functions.
%%
%%\begin{figure}
        %%\centering
				  %%%\subfigure[KI on a sine curve.]{
    %%%%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %%%\includegraphics[width = 5cm]
								%%%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%%%{content/Ch_kinkyinf/figs/sinKI1}
    %%%\label{fig:KI1}
  %%%} 	
	 %%\subfigure[KI on a sine curve.]{
    %%%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %%\includegraphics[width = 5cm]
								%%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%%{content/Ch_kinkyinf/figs/sinKI3}
    %%\label{fig:KI2}
  %%} 	%\hspace{2cm}
	  %%%\subfigure[SKI on a sine curve.]{
    %%%%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %%%\includegraphics[width = 5cm]
								%%%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%%%{content/Ch_kinkyinf/figs/sinSKI1}
    %%%\label{fig:SKI1}
		%%%} 	
	  %%\subfigure[SKI on a sine curve.]{
    %%%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %%\includegraphics[width = 5cm]
								%%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%%{content/Ch_kinkyinf/figs/sinSKI3}
    %%\label{fig:SKI2}
  %%} 	
	%%\label{fig:exSKI1}
   %%\caption{Comparison of the kinky inference rule (left) versus the smoothed kinky inference rule (right) when predicting a sine curve. Note the smoothed out kinks of the SKI rule due to the application of the smoothing filter. Here we chose $\sigma =0.1$. }
%%\end{figure}	  
%%
%%The question arises how the smoothing might affect the theoretical properties. Firstly, we note that due to Lem. \ref{lem:Hoeldarithmetic}, the H\"older exponent and constant remain unchanged. For the constant, we apply point 4 and 9 of the lemma to see that $L(f_n^*) = \frac{1}{\sum_{i=-q}^q w_i} 
%%\sum_{i=-q}^q w_i L(\predfn (x+i \sigma)) = L(\predf_n) \frac{1}{\sum_{i=-q}^q w_i}  \sum_{i=-q}^q w_i = L(\predfn)$.
%%
%%Secondly, the question arises what the maximal discrepancy between $\predfn$ and $f_n^*$ is. This question is of importance to make sure that the prediction still is within the bounds given by the ceiling and floor functions. To this end, assume $\predfn$ is H\"older with constant $L$ and exponent $p$. For simplicity assume we utilise Gaussian smoothing for the SKI rule with $n=1$, $w_{-1} = w_1 =1, w_0 =2$. The deviation of this resulting smoothed predictor $f_n^* $ from the kinky inference predictor $\predfn$ can be bounded as follows
%%\begin{align}
%%\abs{\predfn(x) - f_n^*(x)} &= \abs{\predfn(x) - \frac 1 {w_{-1}+w_0+w_1} (w_{-1} \predfn(x-\sigma) + w_0 \predfn(x)+ w_1 \predfn(x+\sigma)} \\
%%&= \frac 1 4 \abs{ 2 \predfn(x) -   \predfn(x-\sigma) - \predfn(x+\sigma)} \\
%%&\leq  \frac 1 4 \abs{  \predfn(x) -   \predfn(x-\sigma)} + \frac 1 4 \abs{ \predfn(x) - \predfn(x+\sigma)}\\
%%&\leq  \frac L 4  \metric^p(x,x-\sigma) + \frac L 4 \metric^p(x,x+\sigma).
%%\end{align}
%%If the metric is induced by a norm $\norm{\cdot}$ the last expression simplifies to $\frac L 2 \norm{\sigma}^p$.
%%In order to ensure that uncertainty bound takes this error into account, we can add this error to the uncertainty quantification $\prederrn$. This guarantees that the ground truth is contained within the error bounds around predictions $f_n^*$. Furthermore, since the bound is valid for all inputs $x \in \inspace$, the convergence guarantees established for kinky inference also hold for the smoothed version up to supremum norm error of at most $\sup_{x \in \inspace} \frac L 4  \metric^p(x,x-\sigma) + \frac L 4 \metric^p(x,x+\sigma)$ (which in the norm-based metric case equals $\frac L 2 \norm{\sigma}^p$).
%%
%%%\subsection{Discussion}
%%%As we observed, our posterior knowledge coincides with the set of sample-consistent functions. Therefore, an exhaustive enclosure is a superset of $\mathcal K_{prior} \cap \mathcal K_{post}$. 
%%%Remembering our discussion of topological inference, we realize that all we need to do to solve Task 1 (as specified in Sec. \ref{sec:problemdef_task1}), is to define our data inference mechanism $M_{\text{dinf}}$ to output the optimal enclosure. A prescription for computing the bounds of this enclosure was given in the definitions above. From these, we see that $M_{dinf}$computes in $\mathcal O(N_n d)$. That is, its computational effort (translating to the necessary inference investment $\gamma_{\text{dinf}})$ is linear in the number of samples and dimensionality of the problem. If we deal with maximum-norms, norm computation can be done with computation that is logarithmic in $d$, reducing the overall evaluation effort to $\mathcal O(N_n \log d)$.   

==> content2/Ch_kinkyinf/KI_metricparopt.tex <==
\section{Parameter optimisation}
In order to infer function values, the KI rules had to be given a number of parameters that were assumed to be specified a priori. These parameter include the chosen H\"older number sequences $L(n)$ as well as the distance metric $\metric_\inspace$.

However, these design parameters determine much of the predictive performance of the resulting inferences. For example, in Fig. \ref{fig:exHfe1} above, we have illustrated how knowing a periodic target function's frequency allows one to predict well even in parts of input space where no sample inputs exist. 
In the given example we considered target function $f(x)= \abs{\sin(\pi \param x)} +1$ having a frequency $\param =1$. Here, the choice of pseudo-metric $\metric_\inspace(x,x';\hat \param) = \abs{\sin(\pi \hat \param \abs{x-x'})} $ with $\hat \param= \param$ proved appropriate for predicting with the right periodicity.

Obviously, if one presupposes a false frequency $\hat \param \neq \param$ then the prediction performance can suffer dramatically. For instance, consider the plot 

\begin{figure}
        \centering
				  \subfigure[KI prediction with two examples.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/ex1hfe1.pdf}
    \label{fig:metricparopt1}
  } 	
	 \subfigure[Refined prediction.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/ex1hfe2.pdf}
    \label{fig:metricparopt2}
  } 	%\hspace{2cm}
	  \subfigure[Using a periodic pseudo-metric.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/ex1hfeperiodic.pdf}
    \label{fig:metricparopt3}
  } 	
   \caption{Lalala }
			\label{fig:metricparopt}
\end{figure}	 

....

In the absence of accurate knowledge of the suitable parameter $\param$ of the pseudo-metric, it would be helpful to estimate it from the data. To this end we will modify standard ideas from 
machine learning. In particular, we will optimise the parameter based on the model assumption that the data was drawn independently from a Laplacian distribution with the mode coinciding with the posterior prediction. That is, a function value $f_s \in \Real$ at input $x \in I$ is assumed to have density $p(f_x| x,\data,\param) = \frac{1}{2\lambda}\exp(-\frac{\abs{f_x - \predfn(x;\param)}}{\lambda})$ for some parameter $\lambda$.
Given some set of \emph{objective function evaluation data} $\data = \bigl\{ ( s_i, f(s_i) ) | \, i=1,\dots, N \bigr\}$ we will determine the estimate by maximising the conditional likelihood  
$p\bigl(f(s_1),\ldots,f(s_N)  | s_1,...,s_N,\data \bigr) = \frac{1}{2\lambda}\exp \Bigl(-\prod_{i=1}^N\frac{\abs{f(s_i) - \predfn(s_i;\param)}}{\lambda} \Bigr) $.
This can be done be minimising the negative log-likelihood. Since multiplication with positive factors does not change the minimiser, we thus obtain the parameter estimate $\hat \param$ as  
\begin{equation}
\hat \param = \argmin_\param -\frac{\lambda}{N}\log p\bigl(f(s_1),\ldots,f(s_N)  | s_1,...,s_N,\data_n \bigr) = \argmin_\param \sum_{i=1}^N\frac{\abs{f(s_i) - \predfn(s_i;\param)}}{N}.
\end{equation}

The H\"older function of the objective function is just less than or equal to the maximum H\"older constant of the functions $\varphi_1,...,\varphi_N$ where 
 $\varphi_i (\param) = \predfn(s_i;\param)$.
 
 The determination of the H\"older constant thus depends on the definition of the parameter within the definition of the predictor. 
 
\subsection{$\param = p$}
By Eq. \ref{eq:hru582jsokbbbn},
\begin{align}
\predfn(x) &= \frac 1 2 \bigl( \tilde f_j + L \metric^p(s_j,x)   \bigr) + \frac 1 2 \bigl( \tilde  f_k - L \metric^p(s_k,x) \bigr)
\end{align}
for some $k,j \in \{1,...,N\}$ being the indices of the sample inputs minimising and maximising the ceiling and floor functions, respectively.

 Hence, by application of Lem. \ref{lem:Hoeldarithmetic}.8) we can examine the absolute values of the derivatives (in $p$), showing that  $L(\varphi_i) \leq\sup_{p \in (0,1)} (\abs{ \frac 1 2  \log(\metric(s_k,s_i) ) \, \metric^p(s_k,s_i)  }+ \abs{\frac 1 2 \log(\metric(s_j,s_i) ) \,  \metric^p(s_j,s_i)})$. 
 
\subsection{Learning a good Lipschitz constant and observational error bound.}
 
 The choice of H\"older constant can greatly influence predictive performance. Chosen conservatively large, it will exactly interpolate all data points. However, in the presence of noise this might cause poorer predictive performance on a test set. 
Generally, the presence of noise introduces large (and in theory, unbounded) derivatives. Therefore, any empirical estimates of H\"older constant can grow unbounded in the presence of noise. Consequently, the resulting predictor will behave akin to a nearest neighbour regression approach and hence, overfit to the noise. An example of this is depicted in Fig. \ref{fig:LACKInoise0}
\begin{figure}
        \centering
        			  \subfigure[Prediction with empirical estimate of $L(n)$.]{        \includegraphics[width = 4.1cm]
								{content/figs/LACKInoise.pdf}
    \label{fig:LACKInoise00}
  }  
			  \subfigure[Prediction with $L(n)$ minimising test error.]{
        \includegraphics[width = 4.1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/figs/Loptnoise.pdf}
    \label{fig:LACKInoise01}
  }    
  %
  \caption{Comparison of predictions based on noise sample with parameter $L(n)$ chosen in two different manners. Left: $L(n)$ chosen to coincide with the empirical estimate of the Lipschitz constant computed based on the entire sample (light blue and green dots). We can see that the resulting prediction (black curve) overfits to the noisy signal (magenta curve) resulting in a poor alignment with the target (blue curve). Right: $L(n)$ chosen to minimise empirical prediction error on test set (light blue dots). We can see that the resulting prediction smoothes out the noise and is a much better fit to the target.}
			\label{fig:LACKInoise0}
\end{figure}	


Instead relying on empirical estimates, we will therefore follow a different approach. That is, we will determine the $L(n)$ based on their predicted performance assessed based on the available data. As we will see this approach will often result in automated smoothing and avoid .


Therefore, we choose to estimate the H\"older constant parameter $\param = L(n)$ on based on the predictive performance of the predictor $\predfn(\cdot;\param)$ on the evaluation data.
Once this is done, we then estimate the noise levels by setting them just large enough so that they can account for the discrepancy between the predictor and all the available data.
 
 \subsection{Learning the periodicity of the data.}
 
 
 
 \subsection{Automated Relevance determination (ARD) }
 Assume $p=1$.
 
 \subsubsection{One-norm}
 Let $\param =  (\param_1,\ldots,\param_d) \geq 0$ and define a weighted metric as per $\metric(x,x';\param) = \sum_{i=1}^d \param_i \abs{x_i-x_i'} = \abs{x-x'}^\top \param$. The weight $\param_i$ quantifies the degree to which the $i$th input component should contribute to the prediction. Large weights suggest a strong degree of importance: i.e. small deviations of a query $x_i$ from the closest example $s_{j,i}$ in the $i$th component will result in large uncertainty of the prediction. Conversely, if $\param_i=0$ effectively disables any influence of the $i$th input dimension in the prediction process.
 
Owing to this interpretation and in keeping with analogous definitions in the kernel literature, inferring $\param$ from the data will be referred to as \emph{automated relevance determination (ARD)}. 

Our chosen metric is differentiable with respect to parameter $\param$. Therefore, we can appeal to Lem. \ref{lem:Hoeldarithmetic}.8) to show that as a function of $\param$ a Lipschitz number of $\param \mapsto \metric(s_i,s_j;\param)$ is bounded from above by 
$\norm{s_i-s_j} _1$. By definition of the predictor we have \begin{align}
\predfn(x;\param) &= \frac 1 2 \bigl( \tilde f_j + L(n) \metric^p(s_j,x;\param)   \bigr) + \frac 1 2 \bigl( \tilde  f_k - L(n) \metric^p(s_k,x;\param) \bigr)
\end{align}
for some $k,j \in\{1,\ldots,N_n\}$.

Once again appealing to Lem. \ref{lem:Hoeldarithmetic}.8), we see that 
$L(\varphi_i) \leq \frac {L(n)} 2 \sup_{i,j} \norm{s_i-s_j} _1+ \frac {L(n)} 2 \sup_{i,j} \norm{s_i-s_j} _1 = {L(n)} \max_{i,j=1,...,N_n} \norm{s_i-s_j} _1$.

 \subsubsection{Maximum-norm}
 Let $\param =  (\param_1,\ldots,\param_d) \geq 0$ and define a weighted metric as per $\metric(x,x';\param) = \max_{i=1,\ldots,d} \param_i \abs{x_i-x_i'}$. The weight $\param_i$ quantifies the degree to which the $i$th input component should contribute to the prediction. Large weights suggest a strong degree of importance: i.e. small deviations of a query $x_i$ from the closest example $s_{j,i}$ in the $i$th component will result in large uncertainty of the prediction. Conversely, if $\param_i=0$ effectively disables any influence of the $i$th input dimension in the prediction process.
 
Owing to this interpretation and in keeping with analogous definitions in the kernel literature, inferring $\param$ from the data will be referred to as \emph{automated relevance determination (ARD)}. 

We can appeal to Lem. \ref{lem:Hoeldarithmetic} to show that as a function of $\param$ a Lipschitz number of $\param \mapsto \metric(s_i,s_j;\param)$ is bounded from above by 
$\norm{s_i-s_j}_\infty$. By definition of the predictor we have \begin{align}
\predfn(x;\param) &= \frac 1 2 \bigl( \tilde f_j + L(n) \metric^p(s_j,x;\param)   \bigr) + \frac 1 2 \bigl( \tilde  f_k - L(n) \metric^p(s_k,x;\param) \bigr)
\end{align}
for some $k,j \in\{1,\ldots,N_n\}$.

Once again appealing to Lem. \ref{lem:Hoeldarithmetic}.8), we see that 
$L(\varphi_i) \leq \frac {L(n)} 2 \sup_{i,j} \norm{s_i-s_j} _\infty+ \frac {L(n)} 2 \sup_{i,j} \norm{s_i-s_j}_\infty = {L(n)} \max_{i,j=1,...,N_n} \norm{s_i-s_j}_\infty$.

\subsubsection{Example -- Pendulum dynamics}
As a first example, we consider learning the dynamics of a friction-less pendulum based on a sample. Denoting the angle of a pendulum by $q$,  its dynamics are given by the ordinary differential equation $\ddot q = f(x)$ where [m;b;l;g] 
$x = [q;\dot q]$ is called the state and 
$f(x) = - 9.81 \sin(x_1)$. Here, we learn the dynamics by learning the function $f$ based on a sample of triplets of angles, velocities and accelerations. We can see that this target function only depends on the first component of its input, namely the angle. So, if we incorporate this in our KI method by choosing the metric $\metric(x,x';\param) = \max\{\param_1 \abs{x_1-x_1'},\param_2\abs{x_2-x_2'}$ with $\param =[1; 0]$ we should expect superior predictive power over using the standard maximum norm (where $\param =[1; 1]$). 
Therefore, we expect ARD method to automatically uncover this advantageous parameter. As an 
example affirming this intuition, refer to Fig. \ref{fig:LACKIARD_1pend}.
The example of Fig. \ref{fig:LACKIARD_1pend_target} - Fig. \ref{fig:LACKIARD_1pend_pred1} illustrate how the ARD method can uncover the fact that the target function only depends on one of the input components and how this can affect the predictive performance. Since the success of ARD depends on the composition of the data sets we, assessed its potency across a range of 1000 different randomised training data sets $\data_1,\ldots,\data_{1000}$.  We recorded the average prediction errors $\sum_{i=1}^M \frac{\abs{f(s_i) - \predf_j(s_i) }}{M}$ of each of the resulting predictors $\predf_j$ $(j=1,\ldots,1000)$ on a test set of size $M=1000$. The resulting box plots are depicted in Fig. \ref{fig:LACKIARD_1pend_bp}. 
The plots show that on the vast majority of trials, the ARD approach succeeded in uncovering the fact that only the first input component impacts target function and to take advantage in terms of improved prediction accuracy.  




\begin{figure}
        \centering
        				  \subfigure[Target function.]{
    \includegraphics[width = 6.2cm,trim = 19mm 15mm 19mm 19mm, clip]
								{content/figs/ARD1pend_target.pdf}
    \label{fig:LACKIARD_1pend_target}
  } 	
  				  \subfigure[Prediction without ARD.]{
    \includegraphics[width = 6.2cm,trim = 19mm 15mm 19mm 19mm, clip]
								{content/figs/ARD1pend_pred0.pdf}
    \label{fig:LACKIARD_1pend_pred0}
  } 
    				  \subfigure[Prediction with ARD.]{
    \includegraphics[width = 6.2cm,trim = 19mm 15mm 19mm 19mm, clip]
								{content/figs/ARD1pend_pred1.pdf}
    \label{fig:LACKIARD_1pend_pred1}
  } 
      				  \subfigure[Comparison over 1000 rnd trials.]{
    \includegraphics[width = 5.5cm]
								{content/figs/ARD1pend_bp.pdf}
    \label{fig:LACKIARD_1pend_bp}
  } 
%				  \subfigure[Target function.]{
%    \includegraphics[width = 6.2cm,trim = 1mm 1mm 1mm 1mm, clip]
%								{content/figs/ARD1pend_target_2000.pdf}
%    \label{fig:LACKIARD_1pend_target}
%  } 	
%  				  \subfigure[Prediction without ARD.]{
%    \includegraphics[width = 6.2cm,trim = 1mm 1mm 1mm 1mm, clip]
%								{content/figs/ARD1pend_pred0_2000.pdf}
%    \label{fig:LACKIARD_1pend_pred0}
%  } 
%    				  \subfigure[Prediction with ARD.]{
%    \includegraphics[width = 6.2cm,trim = 1mm 1mm 1mm 1mm, clip]
%								{content/figs/ARD1pend_pred1_2000.pdf}
%    \label{fig:LACKIARD_1pend_pred1}
%  } 
%      				  \subfigure[Comparison over 1000 rnd trials.]{
%    \includegraphics[width = 5.5cm]
%								{content/figs/ARD1pend_bp_2000.pdf}
%    \label{fig:LACKIARD_1pend_bp}
%  } 
   \caption{LACKI with automated relevance determination.  Fig. \ref{fig:LACKIARD_1pend_target} depicts the target on a test set of M=1000 sample points (plotted in blue). Fig. \ref{fig:LACKIARD_1pend_pred0} depicts the prediction of LACKI based on the maximum-norm metric and a sample $\data$ containing 14 data points (cyan) of triples of angles, angular velocities and accelerations. Fig. \ref{fig:LACKIARD_1pend_pred1} depicts the corresponding prediction $\predf$ but where the ARD-metric was employed whose parameters were automatically determined as the maximiser of predictiveness. To this end, the available data was partitioned into objective function evaluation (plotted in magenta) and conditioning data (plotted in green) as described above. In the depicted example the parameters were determined to be $\param_1 = 0.99$ and $\param_2 = 0.02$ accurately reflecting the dominance of the importance of the angle over the velocity to predict accelerations.
Fig. \ref{fig:LACKIARD_1pend_bp} depicts prediction errors and determined parameters across a range of 1000 randomised trials. 
The first and second boxplots pertain to the average prediction errors of LACKI without and with ARD, respectively.} The last two box plots depict the recorded automatically determined parameter components $\param_1$ and $\param_2$. 			\label{fig:LACKIARD_1pend}
\end{figure}	






==> content2/Ch_kinkyinf/KI_stability_discrtime.tex <==
\section{Stability guarantees in discrete-time systems}
\label{sec:KIMRACstabbounds}

In the previous section, we gave an illustration LACKI-MRAC -- a combination of a feedback-linearising controller with our KI learning method. The results are encouraging -- our adaptive control law managed to learn a dynamic system online and to track a reference in the presence of wingrock dynamics where other state of the art methods failed. 

To simulate the dynamics we relied on a first-order Euler approximation resulting in a discrete-time dynamical system.

In this section, we study the convergence of LACKI-MRAC in such discrete-time systems.
In these we will consider both the offline and the online learning setting. In the former, the LACKI-learner receives a sample set once and builds a controller that remains unaltered during execution time.
For this case, we will provide robustness bounds on the control success (as quantified by a bound on the norm of the error dynamics) as a function of the remaining uncertainty of the trained LACKI model. 

In the online learning setting, which we considered in the wing-rock control simulations, the LACKI-learner gets updated with the most recent observation after each time step. Provided the initial uncertainty is bounded on the given state space, we will be able to guarantee that LACKI-MRAC leads to a closed-loop system that is globally asymptotically stable.

\subsection{Tracking error bounds for the offline learning setting} 
In the offline learning setting, the predictor sequence $\seq{\predfn}{n \in \nat}$ of adaptive elements is based on only one fixed data set $\data_0$ at time $0$ which is not updated subsequently.
That is $\data_n = \data_0, \forall n \in \nat$.

Given some data set $\data_n =\data_0$ at time $n$ and the resulting predictor $\predfn(\cdot)$, the model error is given by $F_n(\cdot) := f(\cdot) - \predfn(\cdot)$. Since we assume constant data, the error does not change either. That is, we have $F_n \equiv F_0 \equiv: F, \forall n$.
 
In our analysis, we consider discrete-time dynamical systems. For example the dynamics might be first-order Euler approximations of the control-affine dynamics of Sec. \ref{sec:KIMRAC}.
Consequently, the error dynamics as per Eq. \ref{eq:errordynmrac} translate to the recurrence relation:
\begin{equation}\label{eq:errordynmrac_nIMRACdiscrete}
	e_{n+1}  = M e_n + \tinc F_n(x_n)
\end{equation}
where $\tinc \in \Real_+$ is a positive time increment and  $n$ is the time step index. Furthermore,
%
\begin{equation}
	F_n(x_n) = f(x_n) - \predfn(x_n) = B \bigl(\nu_{ad}(x_n) -  \tilde a(x_n)\bigr) 
\end{equation}
is an uncertain increment due to the model error of the learner (cf. Eq. \ref{eq:errordynmrac}), 						$B = \left(\begin{array}[h]{c}
				O_m \\ \tinc I_m
						\end{array}\right)$ and 

\begin{equation}
	M = \left(\begin{array}[h]{cc}
				I_m &  \, \tinc I_{m}\\
				-\tinc K_1 & I_m- \tinc K_2 
						\end{array}\right) 
\end{equation}
					is the (error state) transition matrix. 	
Here, $m = \frac d 2$ is half the dimensionality of the state space, $I_m$ denotes the $m \times m$ identity matrix and $K_1,K_2$ are gain matrices that can be freely chosen by the designer of the linear pseudo controller.		
%This is completely consistent with the uncertain recurrence considered in Eq. \ref{eq:dynextstatediscrete1}, with the exception, that the uncertainty of increment $F_n$ is not probabilistic. Instead it is an uncertain quantity reflecting the prediction error of the trained KI learner. Assuming its assumptions are met, Thm. \ref{thm:KIdesiderata} tells us that $F_n$ is interval-bounded. Employing the same type of argument as in Lem. \ref{lem:origprocdiscrfacts} we see that the solution of the recurrence is given by:
By induction, it is easy to show that the recurrence can be converted into the closed-form expression:
\begin{align*}
	\vc e_n &= M \vc e_{n-1} + \tinc \vc F(x_{n+1})  \\ 
	&= \dots= M^k \, \vc e_0 + \tinc \sum_{i=0}^{n-1} M^{n-1-i} \, \vc F(x_i)	.	
\end{align*}	
For vector norm $\norm{\cdot}$, let $\matnorm{\cdot}$ denote a matrix norm such that $\norm{Mv} \leq \matnorm{M} \norm{v}$ for all suitable matrices $M$ and vectors $v$.
We desire to bound the  norm of the error. To this end, we leverage that the norms are sub-additive and sub-multiplicative to deduce: 
\begin{align*}
	\norm{\vc e_n} &\leq   \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \sum_{i=0}^{n-1}  \matnorm{M^{n-1-i}} \, \norm{\vc F(x_i)}		\\
	&\leq \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \maxerrn_n	 \sum_{i=0}^{n-1}  \matnorm{M^{n-1-i}} =: \varrho[n]
\end{align*}
where  $\maxerrn_n$ is chosen such that we can guarantee that $\maxerrn_n	\geq \max_{i=1,...,n-1} \norm{F(x_i)}$.
For instance, we could choose $\maxerrn_n := \sup_{s \in \iaspace_n} \norm{F(s)} $
	where $\iaspace_n = \bigcup_{t< k} \{x \in \iaspace | \norm{x - \xi[t]} \leq \varrho[t] \}$ is the union of the possible states around the reference trajectory $\xi[\cdot]$ at previous time steps.
\begin{remark}	[Bounded error innovations] 
We assume there exists a maximum model error norm $\maxerrn$, i.e. $\forall i: \norm{F_i(x_i)} \leq \maxerrn$ for some bound $\maxerrn \in \Real$.
This is a realistic assumption in any physically plausible systems where the drift forces $a(x)$ are inevitably bounded. Since also, for any finite data, our KI learner has a bounded prediction function, the discrepancy given by $F$ is bounded as well. 
\label{rem:bnd_err_innovations}
\end{remark}

Given the boundedness of $F$ we have: \vspace{-1em}
\begin{equation}
	\norm{\vc e_n} \leq   \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \maxerrn \sum_{i=0}^{n-1}  \matnorm{M^{n-1-i}}.
\end{equation}

The right-hand side is convergent provided the gains $K_1, K_2$ are chosen such that $M$ is stable, i.e. $\specrad(M) <1$, and provided $\maxerrn_n$ is is bounded (see e.g. \cite{calliess2014_thesis}). 

Whether or not $M$ is stable, in low dimensions, the sums can be computed offline and in advance. This is of great benefit if 
 the controller that is building on the error bounds is utilising optimisation-based control with a finite time-horizon.   

To obtain a (conservative) closed-form bound on the error norms \cite{calliess2014_thesis}
contains a derivation and discussion of the following result:

\begin{thm}\label{thm:normboundsboundeddisturbmainbody}
Let $(F_n)_{k \in \nat_0}$ be a norm-bounded sequence of vectors with $\maxerrn_n :=\max_{i \in \{0,\ldots,n-1\}} \norm{F_i(x_i)} \leq \maxerrn \in \Real$. 
For error sequence $(e_n)_{n \in \nat_0}$ defined by the linear recurrence 
	$e_{n+1}  = M e_n + \tinc F_n(x_n) \,\,\,\, (k \in \nat_0)$, we can define the following bounds:
	
	\begin{enumerate}
	\item $\norm{\vc e_n} \leq \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \maxerrn_{n} \sum_{i=0}^{n-1}  \matnorm{M^{i}}$. If $\specrad(M) <1$ and $\exists \maxerrn$ $:\maxerrn\geq \maxerrn_{n-1} \geq 0, \forall n$, the right-hand side converges as $n \to \infty$.
	\item Let $k_0 \in \nat, k_0 >1$ such that $\matnorm{M^n} <1, \forall n \geq k_0$, let $\varphi := \matnorm{M^{k_0}} <1$ and let $\delta_n := \floor{n/k_0}$. If $r:=\specrad(M) < 1$, for $n > k_0$,  we also have:
	\begin{align*} \norm{\vc e_n} &\leq c \, \varphi^{\delta_n} \, \norm{\vc e_0} + \tinc \maxerrn_{n} \Bigl(\sum_{j=0}^{n_0-1} \matnorm{M^j} + c \, k_0 \frac{\varphi-\varphi^{ \floor{\frac{n}{k_0}}+1 }}{1-\varphi} \Bigr)\\
	& \stackrel{n \to \infty}{\longrightarrow} C \leq \tinc \maxerrn \sum_{j=0}^{n_0-1} \matnorm{M^j} 
	+ \frac{\tinc \maxerrn\,  c\, k_0 \,\varphi}{1-\varphi} 
	\end{align*} 
	for some constants $C,c \in \Real$.
	Here, possible choices for $c \in \Real$ are: 
	
(i) $c= \max\{\matnorm{M^i} | i=1,\ldots,k_0-1 \}$ 

or (ii) $c = \frac{1}{(d-1)!} \Bigl(\frac{1 - d}{\log r}\Bigr)^{d-1}	\matnorm{M}^{d-1}\, \, \, r^{\frac{1 - d}{\log r}-d+1}  $.
%
Since $\matnorm{M} \neq 1$, one can also choose (iii) $c:= \matnorm{M}^{n_0}$. %In this case, $\matnorm{M^k} \leq  \, \matnorm{M}^{n_0}^{(k \text{ div } k_0) +1} $.

\item If $\matnorm{M} \neq 1$, we have: \newline
$\norm{\vc e_n} \leq \matnorm{M}^{n} \, \norm{\vc e_0} + \tinc \maxerrn_{n}   \frac{1-\matnorm{M}^n}{1-\matnorm{M}}. $
	\end{enumerate}
%\begin{proof}
%The theorem is proven in \cite{calliess2014_thesis}.
%
%\end{proof}	
\end{thm}


\subsection{Global asymptotic stability of KI-MRAC in the online learning setting}
In this subsection, we lift the assumption that the available sample is static. Instead we assume that at time step $k+1$ we get to see an additional sample of the uncertain drift at the state visited in the previous time step $k$. 
That is, the predictor $\predf_{n+1}(\cdot)$ is based on $\data_{n+1} = \data_n \cup \{ \bigl(\state_n, f(\state_n) \bigr)\}, \forall n $.
Therefore, we also need to index the innovations vector field by time. That is, $F_n := f - \predfn$ denotes the prediction error function (or innovation) due to the data available at time $n \in \nat$. 
As pointed out in Rem. \ref{rem:bnd_err_innovations}, the error innovations $F_n$ are assumed to be bounded for all finite sample sets $\data_n$. 

Above, we have seen that any continuous function can be approximated by some H\"older continuous LACKI predictor up to an arbitrarily small error. 
For convenience, we will establish the following definition:

\begin{defn}
We say that a continuous function $f$ is $L^*-p$-H\"older \emph{up to} error $\bar E_h \in \Real$ on domain $\inspace$ iff there is an $L^*-p$-H\"older function $\phi \in \hoelset {L^*} { } p$ and a function $\psi$ such that $\forall x: f(x) = \phi(x)+\psi(x), \, \sup_{x \in \inspace} \metric_\outspace\bigl(0,\psi(x)\bigr) \leq \bar E_h$.
\end{defn}


%\begin{lem} Assume the target $f$ is bounded on sub-domain $I \subseteq \inspace$ and that the data increases between time steps, i.e. $\data_n \subseteq \data_{n+1}, \forall n \in \nat_0$. Then we have:
%\[\forall x \in I \subset \inspace : \norm{F_n (x)}_\infty \geq \norm{F_{n+1}(x)}_\infty.\]
%\jcom{true? perhaps not needed anyway..}
%\end{lem}
 
%Above theorems consider the case where the data becomes dense in the domain and we are interested in the worst-case prediction error. Relevant to our online-learning and control setting below is the situation where we are only interested in the error on a specific trajectory of inputs. If the prediction error on such a trajectory vanishes then we will be able to establish stability of the trajectory.
%In preparation of these considerations, we will establish the following facts:

%
%\begin{lem}
%Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs that is bounded, i.e. where 
%$\metric_\inspace(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
%Define $G_n = \{ x_i | i \in \nat, i < n\}$.
%
%Then we have \[ \dist(G_n,x_n) = \min\{\metric_\inspace(g,x_n) | \, g \in G_n\} \stackrel{n \to \infty}{\longrightarrow} 0.\]
%\begin{proof}
%The intuition of the following proof is that if the distances were not to converge there would be an infinite number of disjoint balls around the input points that summed up to infinite volume. This however, would be a contradiction to the presupposed boundedness of the sequence.
%We formalise this intuition as follows:
%For contradiction assume there is an $\epsilon >0$ such that for all $n \in \nat$ there exists an $N_n \geq n $ such that 
%\begin{equation}
%\dist(x_{N_n}, G_{N_n}) > \epsilon.
%\end{equation} 
%Hence, by definition of $G_{N_n} =\{ x_i | i < N_n\} $,
%\eqn{eq:i34kjjk3}{\forall i < N_n : \metric_\inspace(x_{N_n},x_i) > \epsilon.}
%
%Let $C_n := \bigcup_{i < n} \ball{\frac \epsilon 2}{x_i} $ be the union of all $\frac \epsilon 2$-balls around each point in $G_n$ and define $\bar I = \bigcup_{n \in \nat} C_n$.
%By definition, each $x_n$ is contained in $\bar I$.
%Since sequence $(x_n)_{n \in \nat}$ is bounded, $\bar I $ has a finite volume relative to some positive, shift-invariant measure $\mu$. I.e. $\mu(\bar I) < \infty$. Furthermore, $\mu(C_n) \leq \sum_{i <n} \mu(B_i) \leq \mu(\bar I)< \infty$ where $B_i := \ball{\frac \epsilon 2}{x_i}$. Since $M:=\mu(B_1) = \mu(B_n)\forall n \in \nat$ we have $\mu(C_n) \leq (n-1) M$.
%Define $m:= \ceil{\frac{\mu(\bar I)}{M}}$.
%Now, choose $n > m+1$. For $i=1,...,n$ $\exists N_i \geq i \forall j \leq N_i: \metric_\inspace(x_{N_i},x_j) > \epsilon$.  Define a permutation $\pi$ such that $\pi(N_1) \leq \ldots \leq \pi(N_n)$. Hence, we have $\metric_\inspace(x_{\pi(N_i)},x_{\pi(N_j)}) > \epsilon , \forall i,j =1,...,n, i < j$. Thus, $B_{\pi(N_i)} \cap B_{\pi(N_j)} = \emptyset , \forall i,j =1,...,n, i \neq j$. Hence, $\mu(\bar I) \geq \mu(C_{\pi(N_n)+1}) = \mu(C_{\pi(N_1)}) + \sum_{i=1}^n \mu(B_{\pi(N_i)}) = \mu(C_{\pi(N_1)}) +  n M > \mu(C_{\pi(N_1)}) + (m+1) M >\mu(C_{\pi(N_1)}) + \mu(\bar I)$ by definition of $m= \ceil{\frac{\mu(\bar I)}{M}}$. But since $\mu(C_{\pi(N_1)}) \geq 0$, we conclude the false statement $\mu(\bar I) > \mu(\bar I)$.
%\end{proof}
%\label{lem:bndseq_entails_distgridvanish}
%\end{lem} 
%
%
%\begin{lem}
%As before, let the observational noise level be bounded by $\obserr$ and assume the output- space pseudo-metric to be translation-invariant.
%Let target $f$ be $L^*-p$-H\"older up to error $E$. That is, there is an $L^*-p$-H\"older function $\psi$ and a function $\phi$ such that $\forall x: f(x) = \phi(x)+\psi(x), \, \metric_\outspace\bigl(0,\psi(x)\bigr) \leq E $.
%
%Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs that is bounded, i.e. where 
%$\metric_\inspace(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
%Furthermore, assume $\data_{n+1} = \data_n \cup \{ \bigl(x_n, \tilde f(x_n)\bigr) \}$ and thus, $G_n = \{ x_i | i \in \nat, i < n\}$.
%Then the prediction error on the sequence vanishes, i.e. \[\metric_\outspace\bigl(\predfn(x_n),f(x_n) \bigr) \stackrel{n \to \infty}{\longrightarrow} \metric_\outspace(0,\obserr) + 2E.\]
%\begin{proof}
%We have established that $\predfn$ is $L(n)-p$- H\"older with $L(n) \leq \bar L$ for some $\bar L \in \Real_{\geq 0}$.
%
%Since sequence $(x_n)$ is bounded, Lem. \ref{lem:bndseq_entails_distgridvanish} is applicable. 
%Let $\xi_n := \argmin_{g \in G_n} \metric_\inspace(x_n,g)$ denote the nearest neighbour of $x_n$ in $G_n = \{x_1,...,x_{n-1}\}$.
%Hence, $\forall n \in \nat: \metric_\inspace (x_n,\xi_n) \to 0$ as $n \to \infty$.
%
%We have:
%$\metric_\outspace\bigl(\predfn(x_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) ,  f(\xi_n)  \bigr) + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \stackrel{(i)}{=}\metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) +\metric_\outspace\bigl(0 , \obserr\bigr) + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) +\metric_\outspace\bigl(0 , \obserr\bigr) + \metric_\outspace\bigl(\phi(\xi_n) , \phi(x_n)\bigr) + 2E \stackrel{(ii)}{\leq} 2 \max\{\bar L, L^* \} \metric_\inspace(x,\xi_n^x )^p + \metric_\outspace(0,\obserr) + 2E \longrightarrow \metric_\outspace(0,\obserr) + 2E$.
%where steps denoted by (i) follow from Lem. \ref{lem:bilinaddtransinvgroup} and (ii) follows from the assumed H\"older properties.
%\end{proof}
%\label{lem:vanisishingseqprederr_groups}
%\end{lem} 
 
 
\begin{lem} For some constant $L^*$ let the target $f$ be $L^*-p$-H\"older continuous up to level $\bar E_h$. 
%Furthermore, 
%assume that the observational error is zero, i.e. $\obserrbnd =0$.

If $F_n(x_n) = f(x_n) - \predfn(x_n)$ is bounded for all $ n \in \nat_0$ then we have 
\[\forall k \in \nat_0: \norm{F_n(\state_{n+k})}_\infty \stackrel{n \to \infty}{\longrightarrow} [0, \frac \hestthresh 2 +  \obserrbnd +2\bar E_h]. \] 


\begin{proof}
If sequence $\seq{F_n(x_n)}{n\in \nat} $ is bounded then by Thm. \ref{thm:normboundsboundeddisturbmainbody}, sequence \seq{x_n}{n\in \nat} is bounded. 
Furthermore,
by Lem. \ref{lem:LACKIsampleconsistency}, we know that our predictors $\predfn(\cdot)$ are sample-consistent up to $\frac \lambda 2$ and hence, $\norm{ F_n(x)}_\infty \leq \frac \hestthresh 2 +  \obserrbnd=: E_s ,\forall x \in \data_n=\{x_1,...,x_{n-1}\}$.

The rest follows directly from Lem. \ref{lem:vanisishingseqprederr_groups} assuming $\metric_\outspace (f,f') = \norm{f-f'}_\infty$.
\end{proof}
\label{lem:innovnorm_convergence}
\end{lem}


\begin{remark}
In particular, in case the target is H\"older continuous $(\bar E_h =0)$ and there is no observational error ($\obserrbnd =0$), parameterising our LACKI rule with $\hestthresh =0$ yields vanishing innovations, i.e. 
\[\forall k \in \nat_0: \norm{F_n(\state_{n+k})}_\infty \stackrel{n \to \infty}{\longrightarrow} 0. \]
\end{remark}

The next theorem gives a stability guarantee for the tracking error of our LACKI-MRAC controller:

\begin{thm}[Tracking error convergence]
Assume the preconditions and definitions of Lem. \ref{lem:innovnorm_convergence} hold.
If the initial error innovation function is bounded, i.e. if $\exists b \in \Real \forall x: \norm{F_0(x)} \leq b $, and, if $M$ is a stable matrix, i.e. if $\specrad(M) <1$, then the tracking error converges to the interval $[0,\frac \hestthresh 2 +  \obserrbnd + 2 \bar E_h]$. That is,
\[\norm{e_n} \stackrel{n \to \infty}{\longrightarrow} [0,\frac \hestthresh 2 +  \obserrbnd + 2 \bar E_h]. \]

\end{thm}
\begin{proof}
We show 
\begin{equation}
\forall \epsilon > 0 \exists N \in \nat \forall n\geq N: \norm{e_n} \leq \epsilon.
\end{equation}
Referring to (i) in Thm. \ref{thm:normboundsboundeddisturbmainbody} we see that for all $k \in \nat$ we have: 
\begin{equation}
\norm{\vc e_{n+k}} \leq \matnorm{M^{k}} \, \norm{\vc e_n} + \sigma \, \tinc \, Q_{n:n+k} 
\label{eq:errdyn320894}
\end{equation}
where $\sigma$ is some nonnegative number and $Q_{n:n+k}:=\max\{\norm{F_n(x_n)},\ldots,\norm{F_{k+n-1}(x_{k+n-1})} \}$.


Let $\epsilon >0$. By Lem. \ref{lem:innovnorm_convergence}, the sequence $\seq{\norm{F_n(x_n)}_\infty}{n \in \nat}$ converges to the interval $[0, \frac \hestthresh 2 +  \obserrbnd +2\bar E_h]$. Hence, we can infer the following two statements:


(I) There exists an index $n_0 \in \nat$ such that for all $k$: $Q_{n_0:n_0+k} \leq \frac{\epsilon}{2 \Delta \sigma}+\frac \hestthresh 2 +  \obserrbnd +2\bar E_h$.

On the other hand,
by Thm. \ref{thm:normboundsboundeddisturbmainbody}, boundedness of $F_0$ entails boundedness of the error dynamics. Thus, $\exists b \in \Real \forall n: \norm{e_n} \leq \beta$.
Knowing that the error dynamics are bounded by some $\beta \geq 0$ we see that $\matnorm{M^{k}} \, \norm{\vc e_n} \leq \matnorm{M^{k}} \beta \stackrel{k \to \infty}{\longrightarrow} 0$. Here, the convergence to zero follows from the assumption that $M$ is a stable matrix. Hence,
we have:

(II) For any $n$ we can choose $k_0(n) \in \nat$ such that for all $k \geq k_0(n): \matnorm{M^{k}} \, \norm{\vc e_n} \leq \frac\epsilon 2 $.
%
Combining (I) and (II) with Eq. \ref{eq:errdyn320894} allows us to conclude that for any $n \geq N:= n_0 +k_0(n_0)$  we have 
\begin{equation*}
\norm{\vc e_{n}} \leq \frac \epsilon 2 + \sigma \, \tinc \,\frac{\epsilon}{2 \Delta \sigma} +\frac \hestthresh 2 +  \obserrbnd +2\bar E_h= \epsilon +\frac \hestthresh 2 +  \obserrbnd +2\bar E_h. 
\label{eq:errdyn3208942}
\end{equation*}
Hence, we have shown that $\forall \epsilon >0 \exists N \geq 0 \forall n\geq 0: \norm{\vc e_{n}} \leq \epsilon +\frac \hestthresh 2 +  \obserrbnd +2\bar E_h$ which is the desired convergence result.

\end{proof}
Note, since the error converges to a bounded set the state will converge to the target trajectory. So, if the target trajectory is bounded, the continuity of the control law (as a function of state) implies that the control is bounded as well.

%
%
\begin{cor}
In the special case of error-free observations of a H\"older continuous target function, choosing a parameter $\hestthresh =0$ implies:
\[\norm{e_n} \stackrel{n \to \infty}{\longrightarrow} 0. \]
That is, the error dynamics are globally asymptotically stable with equilibrium point 0.
Furthermore, the control action sequence $\seq{u(x_n)}{n \in \nat}$ converges, provided the target trajectory $\seq{\xi_n}{n \in \nat}$ does and $\inspace$ is a Hilbert space.
\end{cor}

\begin{proof} The stability statement is an immediate consequence of the preceding theorem. 
Remember the control action at time $n$ is of the form $u_n := u(x_n) = -\predfn(x_n) - A x_n $ for some Matrix $A$. We show that $(u_n)$ is a Cauchy sequence, provided that the target sequence $\xi_n$ is. Due to the Hilbert space assumption this implies the desired convergence result.

So, let $\epsilon >0$. Since $(e_n),(\xi_n)$ converge the state sequence $(x_n)$ converges and all three are Cauchy sequence. Hence, there is $N$ such that for all $n,m >N$: $\norm{e_n-e_m}< \frac{\epsilon} {2 \matnorm{K}}$ and $\norm{x_n-x_m}< \frac{\epsilon} {2\bar L}$. 
Hence, by definition of the control law and H\"older continuity of the predictors with constant $\bar L$, for all $m,n >N:$ $\norm{u_n-u_m} \leq \matnorm{K} \norm{e_n -e_m} + \norm{\predfn(x_n) - \predf_m(x_m) } \leq \frac{\epsilon}{2} + \bar L \norm{x_n -x_m} \leq \epsilon $.

\end{proof}




==> content2/Ch_kinkyinf/KI_theory_derivations.tex <==

\chapter{Supplementary derivations for kinky inference}
\label{ch:KIderivations}
%\section{H\"older continuity and metric property of the exponentiated map \jcom{Check -- don't think this subsection needed anymore.. (?)} }
%
 %
%We endeavour to show that $x \mapsto L \norm{ x -s}^p$ is Hoelder continuous with coefficient $L$ and exponent $p$. This will become important since these functions will serve as essential building blocks of our conservative Hoelder function estimates. 
%
%To this end, we will show that $(x,y) \mapsto \norm{x-y}^p$, for $p \in (0,1] $, is a metric.  This can be utilized to show that
%$x \mapsto \norm{ x -s}^p$ is a Hoelder continuous function.
%
%To establish the metric property, we note that any positive definite function that is subadditive gives rise to a canonical metric. Formally :
%
%
%To prove $(x,y) \mapsto \norm{x-y}^p$ is a metric, we need to establish a few facts. 
%Firstly, we remind ourselves of the following well-known fact:
%\begin{lem} \label{lem:pd_n_concave_subadditive}
 %A nonnegative, concave function $g:\Real_{\geq 0} \to \Real$ with $g(0) = 0$ is subadditive. 
 %That is, $\forall x,y \in \Real_{\geq 0}: g(x+y) \leq g(x) + g(y)$. 
 %
 %\begin{proof}
%If $x = y = 0$ then subadditivity trivally holds:  $0=g(x+y) \leq g(x) + g(y) = 0$.
%So, let $x, y \in \Real_+$ such that $x >0 \vee y >0$.
%We have, $g( x +y) = \frac{x}{x+y} g(x+y) + \frac{y}{x+y} g(x+y) \leq g(\frac{x}{x+y} (x+y) ) +  g(\frac{y}{x+y}(x+y)) = g(x) + g(y)$.
%Taking into account that $\frac{x}{x+y}, \frac{x}{x+y} \in [0,1]$, the last inequality can be seen as follows:
%
 %Since $g$ is concave we have 
%$\forall p \in [0,1], x \in \Real: g(p x) =  g(px + (1-p) 0) \geq p g(x) + (1-p) g(0) \geq p g(x)  $. The last inequality follows from $g(0) \geq 0$.
%\end{proof}
%\end{lem}
%
%\begin{lem} \label{lem:x2p_pdNsubadd}
 %Let $h: \begin{cases} \Real_{\geq 0} \to \Real_{\geq 0},\\ \, x \mapsto x^p\end{cases}$, for $p \in (0,1] $. $h$ is positive definite and subadditive. 
 %That is, (i) $h(0) = 0 $ and  $h(x) > 0, \forall x \neq 0$ and (ii) $\forall x,y \in \Real_{\geq 0}: h(x+y) \leq h(x) + h(y)  $.
 %Moreover, $h$ is concave. If $p \in (0,1)$, h is strictly concave. 
 %
%\begin{proof}
%\textit{Pos. def. :} $h(0) = 0$.  Also $\lim_{x \to 0_+} h(x) =0$. Since $\nabla h (x) = p h^{p-1}(x) >0 $ for $x >0$, $h$ is strictly monotonically increasing on $\Real_+$. Hence, $h(x) > 0, \forall x >0$. 
%
%\textit{Concavity:} If $p =1$, $h$ is linear and hence, concave. If $p \in (0,1)$, $\nabla^2 h(x) = p (p-1) h(x)^{p-2} > 0$ regardless of $x$.
%
%\textit{Subadditivity:} Follows directly with Lem. \ref{lem:pd_n_concave_subadditive} on the basis of established positive definiteness and concavity.
  %
%\end{proof}
%\end{lem}
%
%
%
%\begin{lem}\label{lem:hoeldererror_metric}
%Let $p \in (0,1]$.
%With definitions as in Thm. \ref{thm:subaddmetric1}, we assume that set $G$ is endowed with a quasi- metric $d$. Function
%$\metric: \begin{cases} \inspace \times \inspace \to \Real_{\geq 0} \\ (x,y) \mapsto \Bigl(d(x,y)\Bigr)^p \end{cases}$ is a quasi-metric on $G$.
%If $d$ is a metric then so is $\metric$.
%\begin{proof}
 %By Lem. \ref{lem:x2p_pdNsubadd}, $x\mapsto x^p$ is pos. def. and subadditive. Therefore, positive definiteness and the triangle inequality of $d$ readily extend to $\metric$ as follows: 
%
%\textit{Pos. def.:}
%Let $x=0$. $\metric(x,x) = d(x,x)^p = 0^p = 0$. If $x \neq 0$ then $k :=d(x,x) \neq 0$. Hence   $\metric(x,x) = d(x,x)^p = k^p \neq 0$.
%
%\textit{Triangle inequality:}
%Choose arbitrary $x,y,z \in \inspace $. We have $\metric(x,z) = d(x,z)^p \leq (d(x,y) + d(y,z) \bigr)^p \leq d(x,y)^p + d(y,z)^p = \metric(x,y) + \metric(y,z)$. Here, the first inequality followed from the triangle inequality of quasi-metric $d$ and the second from subadditivity properties established in Lem. \ref{lem:x2p_pdNsubadd}.
%
%\textit{Symmetry:} If $d$ is a metric it is symmetric. Hence, $\metric(x,y) = d(x,y)^p = d(y,x)^p = \metric(y,x), \forall x,y \in \inspace $ in which case $\metric$ also is symmetric.
%\end{proof}
%\end{lem}
%
%Before proceeding we establish a slight generalization of the well-known \textit{reverse triangle inequality}:
%
%\begin{lem}[Reverse Triangle Inequality] \label{thm:revtriangle}
%Let  $\inspace$ be a set and $\metric : \inspace^2 \to \Real$ a symmetric function that fulfills the triangle inequality. 
%That is,  $\forall x,y,z \in \inspace: \metric (x,y) = \metric(y,x) \wedge \metric(x,z) \leq \metric(x,y) + \metric(y,z)$.
%
%Then \[\forall x,y,z \in \inspace: \abs{\metric(x,y) - \metric(z,y)} \leq \metric(x,z).\]
%\begin{proof}
%
%For contradiction, assume 
%$\abs{\metric(x,y) - \metric(z,y)}>\metric(x,z)$ for some $x,y,z \in \inspace$.
%This is implies  
%$
%(i)\,\,\, \metric(x,y) - \metric(z,y)>\metric(x,z) 
%\, \, $  or  $
  %\,\,  (ii) \,\,\,\, \metric(z,y)-\metric(x,y) >\metric(x,z)$.
%Both inequalities contradict the triangle inequality:
%$(i) \Leftrightarrow \metric(x,y)  >\metric(x,z) \metric(z,y) $ and 
%$(ii) \Leftrightarrow  \metric(z,y) > \metric(x,z) + \metric(x,y) =  \metric(z,x) + \metric(x,y)$.
%
%\end{proof}
%\end{lem}
%
%
%\begin{thm}
%Let $\metric$ be a metric on set $G$. For arbitrary $s \in \inspace $ we define $\phi_s: \inspace \to \Real $ as $\phi_s: x \mapsto \metric (x,s) $.
%$\phi_s $ is Lipschitz with respect to metric $\metric$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq \metric (x,y). \]
%\begin{proof}
%$\abs{\phi_s(x) - \phi_s(y)} = \abs{\metric(x,s) - \metric(y,s)} \stackrel{Thm. \ref{thm:revtriangle}} {\leq} \metric(x,y), \forall x,y,s \in \inspace $.
%\end{proof}
%\end{thm}
%Finally, combining this theorem with Lem. \ref{lem:hoeldererror_metric} immediately establishes that mappings of the form $\metric(\cdot,s)^p$ and hence, of the form
%$\norm{\cdot -s}^p$ are Hoelder continuous with exponent $p$ ($\in (0,1]$):
%
%\begin{thm}
%Let $\metric$ be a metric on set $G$ and let $p \in (0,1], L \geq 0$. For arbitrary $s \in \inspace $ we define $\phi_s:\begin{cases}  \inspace \to \Real \\ x \mapsto L \, \bigl(\metric (x,s) \bigr)^p\end{cases}$.
%$\phi_s $ is Hoelder with exponent $p$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq L \, \metric (x,y)^p. \]
%In particular, for any norm $\norm \cdot$ on $G$ and $s \in \inspace $, mapping $x \mapsto L \norm{x-s}^p$ is Hoelder with constant $L$ and exponent $p$.
%\begin{proof}
%By Lem. \ref{lem:hoeldererror_metric}, $\metric(\cdot,\cdot)$ is a metric on $G$. Hence, Lem. \ref{thm:revtriangle} is applicable yielding:
%$\abs{\phi_s(x) - \phi_s(y)} = L \, \abs{\metric(x,s)^p - \metric(y,s)^p} \stackrel{Lem. \ref{thm:revtriangle} } {\leq} \metric(x,y)^p, \forall x,y,s \in \inspace$. The last sentence concerning the norms follows from the fact that a mapping $(x,y) \mapsto \norm{x-y}$ defines a metric.
%\end{proof}
%\end{thm}
%
%
%
 %At first glance, the result may seem intuitive. However, it should be noted that, for $p >1$, $x \mapsto \norm{x -s}^p$ no longer is Hoelder with exponent $p$. This is consistent with the well-known fact that Hoelder functions with exponent $>1$ are constant functions.
%
%We conclude this section by the following theorem stating that any concatenation of Hoelder continuous functions is Hoelder continuous:
%
%\begin{thm} \label{thm:concathoelder}
%Let $(\statespace, \metric)$ be a metric space and $f,g : \statespace \to \statespace$ be two Hoelder continuous mappings with Hoelder constants $L_f, L_g$ and Hoelder exponents $p_f,p_g$, respectively.
%Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also Hoelder continuous with Hoelder constant $L_h:= L_f L_g^{p_f}$ and exponent $p_h:=p_g \, p_f$.
%That is, 
%\[\forall \state,\state' \in \statespace: \metric\bigl(h(\state),h(\state')\bigr) \leq L_h \bigl(\metric(\state,\state')\bigr)^{p_h}.\]
%\begin{proof}
%%\begin{align}
%$\metric\bigl(f \circ g(\state),f\circ g(\state')\bigr) \leq L_f  \Bigl(\metric(g(\state),g(\state'))\Bigr)^{p_f}$
%$\leq L_f  \Bigl(L_g \metric(\state,\state')^{p_g}\Bigr)^{p_f}$ $= L_f L_g^{p_f}   \Bigl(\metric(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using Hoelder continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
%
%\end{proof}
%\end{thm} 
%In conjunction with Hoelder properties of the square root function established in Ex. \ref{ex:sqrtfctHoelder}, Thm. 
%\ref{thm:concathoelder} immediately yields the following result:
%\begin{cor}
%If $f: \statespace \to \statespace $ is Hoelder continuous with constant $L_f$ and exponent $p_f$ then $\sqrt{f}$ also is Hoelder, having  Hoelder constant $\sqrt{L_f}$ and exponent $p_f$.
%\end{cor}

\section{Convergence properties }
We will construct function estimates that converge to the ground truth in the limit of large sample sets, provided the samples fulfil certain convergence properties themselves. To establish this in a rigorous manner, we need to review a few core convergence concepts. 
\begin{defn}[Uniform convergence of function sequences] Let $(\inspace, \metric_\inspace), (\outspace,\metric_\outspace)$ be two metric spaces.
For $n \in \nat$, let $f_n : I \to \Real$. $f_n \stackrel{n \to \infty}{\longrightarrow} f$ \emph{uniformly} (with respect to $\metric_\outspace$) if
\[  \forall \epsilon >0  \exists N_0 \in \nat \forall n\geq N_0 \forall x \in I: \metric_\outspace(f_n(x), f(x)) < \epsilon. \] 
\end{defn}

The key distinction between both variants of convergence is that in point-wise convergence, the convergence rate can depend on $x$. By contrast, in uniform convergence the rate is independent of function input $x$.


For our purpose the following definition of a dense set suffices:
\begin{defn}[Dense] Let $(\mathcal X,\metric)$ be a metric space.  
A set $D \subset \mathcal X$ is ($\metric$-) dense in a set $I \subset \mathcal X$ if every  $\metric-$ open subset of $I$ contains at least one point of $D$. That is:
$\forall x \in I, \epsilon > 0 \exists \xi \in D: \metric(\xi,x) < \epsilon$.     
\end{defn}


\begin{defn}[Uniform convergence of sequences of sets]\label{def:uniform_setconvergence}
Let $\bigl(\mathcal X,\metric\bigr)$ be a metric space.  
A sequence of sets $(Q_n)_{n \in \nat}$, $Q_n \subset \mathcal X$, $\abs{Q_n} < \infty$ converges to set $Q \subset \mathcal X$ \textit{uniformly} if we have:
\[\forall \epsilon > 0 \exists N_0 \in \nat \forall n \geq N_0 \forall q \in Q \exists q_n \in Q_n : \metric(q_n,q) \leq \epsilon. \]

If the sequence consists of finite sets, we can rewrite the condition as 
\[\forall \epsilon > 0 \exists N_0 \in \nat \forall n \geq N_0 \forall q \in Q : \min_{q_n \in Q_n} \metric(q_n,q) \leq \epsilon. \]

\end{defn}

In analogy to the intuition of uniform convergence of function sequences, uniform convergence of sets means that the rate of convergence does not depend on the location within the set.


In preparation for the derivations below, it will be useful to establish that uniform convergence to a dense subset of set $I$ implies uniform convergence to $I$ itself. Formally we express this as follows:

\begin{lem}
\label{lem:unifdenseset1}
Let $Q$ be a dense subset of $I$ and let $Q_n$ be a sequence of sets uniformly converging to $Q$ in the limit of $n \to \infty$. We have \[\forall e > 0 \exists N_0 \forall n \geq N_0 \forall x \in I \exists s \in Q_n: \metric(x,s) \leq e. \]


\begin{proof}
Let $e>0$, $N_0 \in \nat$ such that for all $n \geq N_0$ we have $\forall q \in Q \exists s_n(q) \in Q_n: \metric(s_n(q),q) \leq \frac{e}{2}$. 
Now, choose any $x \in I, n \geq N_0$. Since $Q$ is dense in $I$ we can choose $q \in Q$ such that $\metric(q,x) \leq \frac{e}{2}$. 
Hence, utilising the triangle inequality, we conclude $\metric(x,s_n(q)) \leq \metric(x,q) +\metric(q,s_n(q)) \leq \frac{e}{2} + \frac{e}{2} = e$.
\end{proof}
\end{lem}
An alternative statement of the lemma is that, under the lemma's premise, we have 

\[\forall e > 0 \exists N_0 \forall n \geq N_0 \forall x \in I : \inf_{s \in Q_n} \metric(x,s) \leq e. \]


\begin{defn} [``Eventually dense partition '']
For each $n \in \nat$ let $\mathcal P_n :=\{P_{n,1},...P_{n,n}\}$ be a partition of $I$ into subsets, each being a connected set and having the property that $P_{n,i}$ contains exactly one sample input $s_i$. Furthermore, let $r_{n,i} = \sup_{x,x' \in P_{n,i}} \frac{1}{2} \norm{x-x'}$ be $ P_{n,i}$'s ``radius'' w.r.t norm $\norm{\cdot}$. 
We call $(\mathcal P_n)_{n \in \nat}$ an \emph{eventually dense} partition sequence if the sequence $(r^*_n)$ of maximum radii, $r^*_n : = \max \{ r_{n,i} \}$, converges to zero as $n \to \infty$.

A sequence of inputs $(G_n)_{n \in \nat}$ will be called ``eventually dense'' if it is impossible to define a partition sequence separating the points in $G_n$ for each $n$ such that $G_n$ is not eventually dense.
\end{defn}
It should be clear that a sample grid that converges to a dense subset in $I$ is eventually dense (and vice versa).


%\jcom{dont think I need the next 2 results statements anymore:}
It will become useful to remind ourselves of the standard fact that monotone sequences converge if they are bounded:
\begin{thm}[Monotone convergence theorem]
Let $(a_n)_{n \in \nat}$ be a monotone sequence of real numbers. That is, $a_n \geq a_{n+1}, \forall n \in \nat$ or $a_n \leq a_{n+1}, \forall n \in \nat$. The sequence converges to a finite real number if and only if the sequence is bounded. In particular, if the sequence is monotonically increasing then $\lim_{n \to \infty} a_n = \sup a_n$. If it is decreasing, we have $\lim_{n \to \infty} a_n = \inf a_n$.
\end{thm}
This theorem can be directly applied to prove the following result:
\begin{cor}
\label{cor:monseqfctsencl}
Let $(\phi_n)_{n \in \nat}$, $\phi_n : I \to \Real$ be a point-wise monotonically increasing sequence of functions and, let $(\gamma_n)_{n \in \nat}$, $\gamma_n : I \to \Real$ be a point-wise monotonously decreasing sequence of functions. That is, $\forall x \in I \forall n \in \nat: \phi_n(x) \leq \phi_{n+1}(x) \wedge \gamma_n(x) \geq \gamma_{n+1}(x) $. Furthermore, we assume $\forall x \in I \forall n \in \nat: \phi_n(x) \leq \gamma_{n}(x)$. 

Then, both sequences are point-wise convergent with point-wise limits 
$\lim_{n \to \infty} \phi_n (x) = \sup_{n \in \nat} \phi_n \leq \inf_{n \in \nat} = \lim_{n \to \infty} \gamma_n (x) $.
\end{cor}
The corollary will be needed below when we establish convergence of our function estimate bounds.

\subsection{Convergence with respect to the exponentiated metric}
\label{sec:unifconvhoeldermetricequivmetricunifconv}
The purpose of the next two results is to show that it does not matter whether one establishes a convergence property with respect to a metric $\metric$ or whether one does so with respect to $\metric^p$.
\begin{lem}\label{lem:hoeldermetricconv}
Let $p \in (0,1]$, $\mathcal X$ be a metric space and $(x_n)_{n \in \nat}$ be a sequence in $\mathcal X$ converging to $x \in \mathcal X$ with respect to metric $\metric$ iff the sequence converges to $x$ with respect to $\metric^p$.

\begin{proof}
$\Rightarrow:$
Define the sequence $d_n :=  \metric(x_n,x) $.
Convergence with respect to $\metric$ means that $d_n \to 0$ as $n \to \infty$. Since $d_n \geq$ mapping $ \psi: \mathfrak x \mapsto \mathfrak x^p$ is well-defined for sequence inputs $d_n$. Furthermore, $\psi$ is a continuous function and thus, 
$\lim_{n \to \infty} \metric^p(x_n,x) = \lim_{n \to \infty} \psi(d_n) =  \psi( \lim_{n \to \infty} d_n) = \psi (0)  =0$.
Hence, $x_n$ converges to $x$ with respect to $\metric^p$ as well.
$\Leftarrow:$ Completely analogous.

\end{proof}  
\end{lem}

\begin{lem}\label{lem:hoeldermetricconv}
Let $p \in  (0,1]$, $\mathcal F$ be a metric space of functions. Sequence of functions $(f_n)_{n \in \nat}$ converges uniformly to $f$ with respect to metric $\metric$ iff the sequence also converges uniformly to $f$ with respect to $\metric^p$.


\begin{proof} $\Rightarrow:$
Since $f_n \to f$ uniformly, we have 
$\forall e >0 \exists N_e \geq 0 \forall n \geq N_e, x \in I : \metric(f_n , f) < e$. We show that also $\forall e >0 \exists N_e \geq 0 \forall n \geq N_e, x \in I : \metric(f_n , f)^p < e$.
Mapping $\psi: x \mapsto x^p$ invectively maps positive numbers onto the set of positive real numbers. Hence, $\metric(f_n, f) < e \Leftrightarrow \metric(f_n , f)^p < e^p$.
Let $e >0$ and $ \varepsilon := \sqrt[p]{e}$. Due to uniform convergence, we can choose $ N_\varepsilon$ such that $\forall x \in I, n \geq N_\varepsilon: \metric(f_n , f) <\varepsilon$ which is equivalent to stating $\forall x \in I, n \geq N_\varepsilon: \metric(f_n , f)^p <\varepsilon^p = e$. $\Leftarrow:$ Completely analogous.
\end{proof}  
\end{lem}




\section{Theoretical guarantees of the enclosure}

%\jcom{Talks about Lipschitz instead of Hoelder .. needs to be fixed}
%We assume the dimensionality of the target's input domain $I \subseteq \inspace$ is $d \geq 1$. 
 Remember, we defined the set of samples as $D_n= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N_n \} $. To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the grid of sample inputs contained in $D_n$.
Our exposition of this subsection focusses on the case of one-dimensional output space. That is, $\outspace = \Real$ and we assume to be the target function $f$ to be a mapping $f: I \subseteq \inspace \to \Real$.


In this subsection, we assume $\metric_\inspace$ to be any suitable metric on the target function domain and  $\metricp(x,x') := \metric_\inspace^p(x,x')$. We have seen that (uniform) convergence with respect to $\metricp$ is equivalent to (uniform) convergence with respect to metric $\metric$ (see Sec. \ref{sec:unifconvhoeldermetricequivmetricunifconv}). Also note, that Lipschitz continuity with respect to $\metricp$ is H\"older continuity with respect to metric $\metric_\inspace$. %Therefore, we may use the terms Lipschitz continuity and H\"older continuity interchangeably if it is clear which metrics the terms refer to.
Furthermore, remember we are primarily interested in functions restricted to be H\"older with respect to $\metric$ and bounded by functions $\lbf,\ubf$. That is, we know the target is contained in $\mathcal K_{prior} = \lipset L \metricp  \cap \bfset$ where $\lipset L \metric$ denotes the $L$- Lipschitz functions with respect to  $\metricp$ and $\bfset :=\{\phi : \inspace \to \Real \, | \, \forall x \in \inspace : \lbf(x) \leq \phi(x) \leq \ubf(x)\} $. 

As a final note, at no point will we utilise the definiteness property of the metric. Therefore, our definitions and results extend from metrics to the more general class of semi-metrics.

%We will now define a data inference mechanism $M_{dinf}$ that maps the sample $D_n$ into a subset 
%
%\subsubsection{A priori knowledge} We assume, our  a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L[J]$ such that the underlying target $f \in \mathcal F$ is $L[J]-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L[J] \norm{x-x'}\}$.

%\subsubsection{Computing a posteriori knowledge}

\begin{defn}[Sample-consistent functions]
A function $\kappa: I \to \Real$ is called \textit{consistent with sample} $D_n$ (shorthand: \emph{sample-consistent}) if \[ \forall i \in \{1,\ldots,N_n\}: \kappa(s_i) \in [\tilde f_i - \varepsilon(s_i), \tilde f_i + \varepsilon(s_i)  ] =[\underline f(s_i),\overline f(s_i) ].\] The set of all sample-consistent functions on $I$ will be denoted by $\mathcal K(D_n)$.
\end{defn}
Informally speaking, $\mathcal K(D_n)$ contains all functions that could have created the sample set. Conversely, sample $D_n$ rules out all functions that are not sample-consistent as candidates for being the target. 

%In the lingo of our consideration on topological inference, $\mathcal K(D_n)$ embodies part of our posterior knowledge: $\mathcal K_{\text{post}} = \mathcal K(D_n)$. 





\begin{defn}[Enclosure]
Let $\decke,\boden: I \to \Real$ be two functions, such that $\decke
\geq \boden$ pointwise on $I$. We define their enclosure on $I$ as
the compact interval $\mathcal E^\decke_\boden (I)$ of all functions
between them. That is, \[\mathcal E^\decke_\boden (I) := \{\phi: I
\to \Real \vert \forall t \in I: \decke(t) \geq \phi(t) \geq
\boden(t) \}.\]
\end{defn}
For ease of notation we omit the domain argument whenever we refer
to $I$. That is, we write  $\mathcal E^\decke_\boden :=\mathcal
E^\decke_\boden (I)$.


An \emph{enclosure} is sample-consistent if it is contained in the set $\mathcal K(D_n)$ of sample-consistent functions. 

Based on the sample, we desire to find two
\emph{enclosing functions} $\decke_n: I \to \Real$, $\mathfrak
\boden_n: I \to \Real$ bounding the target from above and below that
are as tight as possible and converge to the target in the limit of
infinite, sample set size $N$. 
More formally, we would ideally like it to satisfy the following desiderata:

\begin{defn}[Desiderata] \label{defn:desiderata}
 Based on an observed, erroneous data set $D_n$, we desire to define enclosing functions $\decke_n, \boden_n$ that give rise to an enclosure $\einschluss$ with the following properties:

\begin{enumerate} 

    \item \textbf{Sample-Consistency}: The enclosure is sample-consistent, i.e. $\einschluss \subseteq \mathcal K(D_n)$.
		%The enclosing functions are sample-consistent, i.e. $\decke_n,\boden_n \in \mathcal K(D_n)$.
    
     \item \textbf{Exhaustiveness (conservatism)}: Every $\phi, \lbf \leq \phi \leq \ubf$ coinciding with target $f$ on with grid $G_n$ and
having at most constant $L[J]$ on every subset $J \subset I$ is also contained in the enclosure: $\forall \phi: I \to \Real, \phi \in \mathcal K_{prior} \cap \mathcal K(D_n): \phi \in \einschluss $. That is, $\mathcal K_{prior} \cap \mathcal K(D_n) \subseteq \einschluss$.
    In particular, the target is always contained in the enclosure: $f \in \einschluss$.

\item \textbf{Monotonicity:} Additional data does not increase uncertainy. That is,
if $G_n \subseteq G_{n+1} $, we have $\mathcal E^{\decke_{n+1}}_{\boden_{n+1}} \subseteq \einschluss, \forall n \in \nat$.
		   
\item \textbf{Convergence} to the target: Let the set of sample inputs $G_n$ in $D_n$ converge to a dense subset of domain $I$ and for each input $x \in I$ let the sample error function $\varepsilon: I \to \Real_{\geq 0}$ be bounded by $m_x \geq 0$ in some neighbourhood of $x$. Then, we have 
\begin{itemize}
\item (a) The sequence of enclosures converges point-wise. In particular, 

$\forall x \in I: 0 \leq \lim_{n \to \infty} \decke_n (x) -\boden_n(x) \leq 2 m_x$.
In particular, the enclosure converges to the target $f(x)$ at inputs $x$ where $m_x=0$.  
		
		\item (b) If convergence of $G_n$ is uniform and the target observations are error-free, i.e. $m_x = 0, \forall x \in I$, then the enclosure converges to the target $f$ uniformly.
\end{itemize}	
   \item \textbf{Minimality (optimality)}: 
If an enclosure $\mathcal E^b_a$  satisfies \emph{Desideratum 2} then it is a superset of our enclosure $\einschluss$, i.e. $b \geq \decke_n, a \leq \boden_n$, $\einschluss \subseteq \mathcal E^b_a$.    

\end{enumerate}

\end{defn}
 
Next, we will derive enclosing functions that give rise to such an enclosure.

\begin{defn}[Sample point ceiling and floor functions]
\label{def:sampleceilandfloormultidim}
Remember, $\overline f(s_i) = \tilde f_i + \varepsilon(s_i)$ and $\underline f(s_i) = \tilde f_i - \varepsilon(s_i)$.  For the $i$th sample ($i \in \{1,\ldots,N_n\}$, $L \geq 0$, $x \in I$, we define  
\begin{enumerate}
	\item The $i$th \emph{sample point ceiling} function: \[\decke_n^i (x; L) :x \mapsto  \overline f (s_i) +  \,L \, \metricp(x, s_i), \]
	\item and the $i$th \emph{sample point floor} function: \[\boden_n^i (x; L) :x \mapsto  \underline f (s_i) -  \,L \, \metricp(x, s_i) .\] 
\end{enumerate}
%Here $n_i$ is a norm-dependent constant ensuring that both functions are $L$-Lipschitz with repect to $\norm{\cdot}$. 
If constant $L$ is clear from the context, its explicit mention shall be omitted.
\end{defn}
%Note, for the maximum-norm $\norm{\cdot}_\infty$ it is easy to see that  $n_i =1$ renders both functions $L$-Lipschitz. For the 1-norm, one can either utilize Lipschitz arithmetic to show that for $n_i=1$ the functions would be $d L$-Lipschitz or, one can leverage the well-known inequality~\cite{koenigsberger:2000}   $\norm{\cdot}_1 \leq d \norm{\cdot}_\infty$ to determine $n_i := \frac{1}{d}$.

We show that these functions give rise to enclosures that satisfy the first three Desiderata of Def. \ref{defn:desiderata}:
\begin{lem} 
\label{lem:samplefloorceiling}
Let  $i \in \{1,...,N_n\}$.
Enclosure $\mathcal E^{\decke_n^i}_{\boden_n^i}$ is (i) consistent with the $i$th sample and (ii) conservative. 
More specifically: 

(i)  \[\forall i \in \{1,...,N_n\}, \phi \in \mathcal E^{\decke_n^i}_{\boden_n^i}:  \phi(s_i) \in [\underline f(s_i), \overline f(s_i)].\]

(ii) If target $f: I \to \Real$ is $L$-Lipschitz on $J \subset I$ with respect to $\metricp$ then the corresponding sample ceilings are upper bounds and the sample floor functions are lower bounds. That is, for $i =1,\ldots, N$, $\forall x \in J$ we have \[\decke_n^i (x; L) \geq f(x)  \geq  \boden_n^i (x; L).\]

\begin{proof}
(i) Follows directly from the definitions.
(ii) We show the first inequality, $\decke_n^i (x; L) \geq f(x)$. (The proof of the second inequality,  $f(x)  \geq  \boden_n^i (x; L)$, is completely analogous.) 

Due to the H\"older property, we have 
$\forall x,x' \in J: \abs{f(x) - f(x')} \leq L \metricp(x,x').$
In particular, 
$\forall x \in J: f(x) - f(s_i) \leq\abs{f(x) - f(s_i)} \leq L \, \metricp(x, s_i).$
Hence, 
$\forall x \in J: f(x)  \leq f(s_i) + L \, \metricp(x, s_i)$ 
$\leq \tilde f(s_i) +\varepsilon(s_i) + L \, \metricp(x, s_i) = \decke_n^i (x; L)$.

%Since $\decke_n^i (x; L)  = \tilde f_i + \varepsilon(s_i) + L_i \metricp(x, s_i)$, this entails $\decke_n^i (x; L) \geq f(x)$ for all $\varepsilon(s_i) \geq 0$. Therefore, it suffices to focus on the case for $\varepsilon(s_i) =0$.
 %So, let $\varepsilon(s_i) =0$. 

%&\leq f(c_i) + \ell_i \normtop{x-c_i}_{\infty}:= \decke^i_n(x)
%\end{align}
%where $\ell_i = \sqrt d L_i$ is a Lipschitz constant for the max-norm.
%The last inequality is due to the well-known relationship 
%$\normtop{x}_\infty \leq \normtop{x}_2 \leq \sqrt{d} \, \normtop{x}_\infty $.



\end{proof}
\end{lem}



\begin{defn}[H\"older enclosure] \label{def:optenclosingfcts} On  $J \subset I$, define the \emph{optimal ceiling} as
\[\decke^*_n (x; L) : x \mapsto  \min_{i=1,\ldots,N_n} \decke^i_n(x;L)\]
and the \emph{optimal floor function} as
 \[\boden^*_n (x; L) :x \mapsto   \max_{i=1,\ldots,N_n} \boden^i_n(x; L).\]
The enclosure $\einschluss$ with enclosing function choices $\decke_n := \decke_n^*$ and $\boden_n := \boden_n^*$ will be called ``H\"older enclosure'' and be denoted by $\opteinschluss$.
If constant $L$ is fixed and clear from the context we may omit its explicit mention from the syntax.
\end{defn}
%An example for a Lipschitz enclosure is depicted in Fig. \ref{figlipencl_nonoise_neo}.
%\begin{figure*}
%%
	%\centering
		%\includegraphics[scale = .4]{content/content_hoelderquad2/figs/enclosure.pdf}
	%\caption{Example of an enclosure (for metric $\metricp: (x,y) \mapsto \norm{x-y}$) for a given sample of function values on one-dimensional domain $I = [0,2.5]$. The Lipschitz constant was one, uniformly over the entire domain. The samples were noise-free.}
	%\label{figlipencl_nonoise_neo}
%\end{figure*}

Before we can prove that the optimal functions are indeed optimal, we need to undergo some derivative preparations.

\begin{lem} \label{lem:optenclcontainstarget}
The H\"older enclosure always contains the target. That is, $\decke^*_n(x) \geq f(x) \geq \boden^*_n(x), \forall x \in I, n \in \nat$.
\begin{proof}
This is a direct consequence of Lem. \ref{lem:samplefloorceiling}.
\end{proof}
\end{lem}


\begin{thm} \label{thm:enclmain}
Choosing $\decke_n := \min\{ \decke_n^*, \ubf\}$ and $\boden_n := \max\{\boden_n^*,\lbf\}$ yields an enclosure $\einschluss$ that satisfies Desiderata 1-5 specified in Def. \ref{defn:desiderata}.
\begin{proof}
We bear in mind that $\einschluss = \bfset \cap \opteinschluss$.

\textit{1) Consistency}. By definition of $\decke_n^*$ and $\boden_n^*$ in conjunction with Lem. \ref{lem:samplefloorceiling}.(i) we see that $\opteinschluss = \cap_i \mathcal E_{\boden_n^i}^{\decke_n^i} \subseteq \mathcal K(D_n)$. Desideratum 1 follows from $\einschluss = \bfset \cap \opteinschluss \subseteq \opteinschluss$.\\

\textit{2) Conservatism}. By definition of $\decke_n^*$ and $\boden_n^*$ in conjunction with Lem. \ref{lem:samplefloorceiling}.(ii) we have $\mathcal K(D_n) \cap \lipset L \metricp \subseteq \opteinschluss $. Hence, $\mathcal K_{prior} \cap \mathcal K(D_n) =  \bfset \cap \lipset L \metricp \cap \mathcal K(D_n) \subseteq \opteinschluss \cap \bfset = \einschluss$ proving
Desideratum 2.

\textit{3) Monotonicity.} 

This follows directly from the way the ceiling and floor functions are defined. Considering the ceiling:
We have $\decke_n (x) = \min\{\ubf,\min_{i =1,...,N_n} \decke^i_{n}(x) \} $. W.l.o.g., for $i=1,\ldots,N_n$, let $\decke_n^i = \decke_{n+1}^{i}$. 

Then 
$\decke_{n+1} (x) = \min\{\ubf(x),\min\Bigl\{ \min_{i =1,...,N_n} \decke^i_{n}(x), \min_{i= N_n +1,\ldots,N_{n+1}}  
\decke^i_{n+1}(x) \Bigr\} \} $

$\leq \min \{\ubf(x), \min_{i =1,...,N_n} \decke^i_{n}(x)  \}=  \decke_{n}(x) $. Statement $\boden_{n+1} (x) \geq  \boden_{n}(x)$ follows analogously.

\textit{4 a) Pointwise convergence.} In absence of errors, one could show pointwise convergence by utilising Cor. \ref{cor:monseqfctsencl} --which is applicable due to Lem. \ref{lem:samplefloorceiling} in conjunction with 3). We will now prove the more general statement in the presence of observational errors $\varepsilon$.

Pick an arbitrary $x \in I$ such that the error $\varepsilon(\xi) \leq m_x$ for all $\xi$ in some $\epsilon-$ball $\mathcal U_\epsilon(x) = \{\xi \in I | \metricp(\xi ,x) < \epsilon \}$ around $x$.
It remains to be shown that $\lim_{n\to \infty} \decke_n(x) - \boden_n(x) \leq 2 m_x$ for inputs $x$.
Define $L := \sup_{J \subset I} L[J] $  to be the maximum H\"older constant on the domain.
Let $e>0$ be arbitrary. We show that there exists $N_0 \in \nat$ such that for all $n \geq N_0: \decke_n(x;L) - \boden_n(x;L) \leq e + 2 m_x$ as follows:

Since we assume $G_n$ converges to a dense subset of $I$, Lem. \ref{lem:hoeldermetricconv} applies. Hence, there is $N_0 \in \nat$ such that $\forall n \geq N_0 \exists i \in \{1,...,N_n\}: s_i \in \mathcal U_{e/2L}(x) = \{\xi \in I | \metricp(x,\xi) < \frac{e}{2L}\}$.
 
So, choose $n \geq N_0$. 
Hence, $L \metricp(x,s_j)  < \frac{e}{2}, \,\varepsilon(s_q) \leq m_x \hspace{1cm} \text{ (*)}$ 

where 
$q \in \arg\min_{i \in \{1,...,N_n\} } L \, \metricp(x,s_i) $. 
We have:

 $\decke_n^*(x;L) - \boden_n^*(x;L)$ 

$= \min_{i \in \{1,...,N_n\} } L \, \metricp(x,s_i) + \tilde f(s_i) + \varepsilon(s_i) - \max_{i \in \{1,...,N_n\} }  \tilde f(s_i) - \varepsilon(s_i) - L \metricp(x,s_i) $

$= \min_{i \in \{1,...,N_n\} } \bigl\{L \, \metricp(x,s_i) + \tilde f(s_i) + \varepsilon(s_i) \bigr\}+ \min_{i \in \{1,...,N_n\} }  \bigl\{-\tilde f(s_i) + \varepsilon(s_i)+ L \, \metricp(x,s_i)\bigr\} $

$\leq \min_{i \in \{1,...,N_n\} } \bigl\{L \, \metricp(x,s_i) + \tilde f(s_i) + \varepsilon(s_i)    -\tilde f(s_i) + \varepsilon(s_i)+ L \metricp(x,s_i) \bigr\}$

$=2\min_{i \in \{1,...,N_n\} } L \, \metricp(x,s_i) + \varepsilon(s_i) $
$\leq 2 L \, \metricp(x,s_q)+ 2\varepsilon(s_q) $
$\stackrel{(*)}{<} e + 2 m_x  $.\\
As a special case, in the noise free setting with  $m_x=0$, this result implies that the enclosure shrinks to a single value as $n \to \infty$. That this value is $f(x)$ follows from Lem. \ref{lem:optenclcontainstarget}.  \\

We have shown convergence of $\decke_n^*(x;L) - \boden_n^*(x;L)$. Convergence of $\decke_n(x) - \boden_n(x) = \min\{\ubf(x), \decke_n^*(x)\} - \max\{\lbf(x),\boden_n^*(x)\}$ follows by continuity of the $\max$ and $\min$ operation.


 \textit{4 b) Uniform convergence.}
Let $G_n = \{s_1,\ldots,s_{N_n}\}$ denote the $N_n$-sample input grid which we assume to converge uniformly to a dense set of domain $I$. 


(I) Firstly, we show uniform convergence of $\decke_n^*, \boden_n^*$ to target $f$.

Assuming $m_x =0$, we desire to show that $\forall e >0 \exists N_0 \forall n \geq N_0 , x \in I : \abs{ \decke^*_n(x) - f(x)} \leq e $ and $\forall e >0 \exists N_0 \forall n \geq N_0 , x \in I : \abs{ \boden^*_n(x) - f(x)} \leq e $.
Let $e > 0$.
 %and define $L := \sup_{J \subset I} L[J] $  to be the maximum Lipschitz constant on the domain and $n$ the corresponding normalization constant making the target $L$-Lipschitz. 
Let $G_n$ converge uniformly to a dense subset  $G \subset I$. By Lem. \ref{lem:unifdenseset1}, we know that 
there exists $N_0$ such that for all $n \geq N_0$ and all $x \in I$ there is a $q \in G_n$ such that $\metricp(x,q) < \frac{e}{2  L}$. 
In particular, $ L \, \metricp(s_q ,x ) \leq \frac{e}{2}$ where we define $q \in \arg\min_{i} \metricp(s_i ,x )$. 
Hold such $N_0$ fixed, choose arbitrary $n \geq N_0$ and $x \in I$. 

For starters, we show that each $\decke^*_n$ converges uniformly to $ f$ by showing $\abs{\decke^*_n(x) - f(x) } \leq e$.

We have
$\abs{\decke^*_n(x) - f(x)} \stackrel{2)}{=} \decke^*_n(x) - f(x) $  
$\stackrel{def.}{\leq}\min_{i} \decke^i_n(x) - f(x) $
$\leq   \decke^q_n(x) - f(x) $
$\stackrel{def.}{\leq}  L \, \metricp(x,s_q)+f(s_q) - f(x) $
$\leq  L \, \metricp(x,s_q)+ \abs{f(s_q) - f(x) }$
$\stackrel{f \text{ L-Lip.}}{\leq}  L \, \metricp(x,s_q)+   L \, \metricp(x,s_q) \leq  e$ where in the last step we have leveraged $L \, \metricp(x,s_q) \leq \frac{e}{2}$.

Next, we show the analogous for the floor. 
That is we show  $\abs{\boden^*_n(x) - f(x) }\leq e$:

$\abs{  \boden^*_n(x) - f(x)}\stackrel{2)}{=} f(x) - \boden^*_n(x) $  
$\stackrel{def.}{\leq} f(x) - \max_{i} \boden^i_n(x) $
$\leq   f(x)- \boden^q_n(x)  $
$\stackrel{def.}{\leq} f(x) - (f(s_q) -  L \, \metricp(x,s_q))  $
$\leq  L \, \metricp(x,s_q)+ \abs{f(s_q) - f(x) }$
$\leq  L \, \metricp(x,s_q)+   L\, \metricp(x,s_q) \leq 2 \frac{e}{2}= e$ where, as before, in the last step we have utilised $ L \, \metricp(x,s_q) \leq \frac{e}{2}$.\\

(II) Secondly, we need to show that $\decke_n (\cdot)= \max\{\lbf(\cdot), \decke^*_n(\cdot)\}$ and $\boden_n = \min\{\lbf(\cdot), \boden^*_n(\cdot)\}$ converge uniformly to $f$. However, this presents no difficulty since we know that $f(x) \in [\lbf(x) ,\ubf(x)]$. Let $e\geq0$ be arbitrary. We need to show $\exists \tilde N_0(e) \forall n \geq \tilde N_0(e) , x \in I : \abs{ \decke_n(x) - f(x)} \leq e $. In (I), we already have established $\exists  N_0(e) \forall n \geq \tilde N_0(e) , x \in I : \abs{ \decke^*_n(x) - f(x)} \leq e $. We choose $\tilde N_0(e) := N_0(e)$. Since $f \leq \decke_n = \min\{ \ubf(x), \decke^*_n\} \leq \decke^*_n$ pointwise, for all $x \in I$, we have 
$e \geq \abs{\decke^*_n(x) - f(x) } =  \decke^*_n(x) - f(x) \geq \decke_n(x) - f(x)  = \abs{\decke_n(x) - f(x)} $. 

Uniform convergence of the floor $\boden_n$ follows completely analogously.


\textit{5) Optimality.}  By Lem. \ref{lem:Hoeldarithmetic}.(6) we know that $\decke_n^*,\boden_n^* \in \lipset L \metricp$. Hence, $\decke_n , \boden_n \in \lipset L \metricp \cap \bfset$. 
Thus, if $\lipset L \metricp \cap \bfset \subset \mathcal E^b_a $ then also $\decke_n, \boden_n \in \mathcal E^b_a$. This implies $\decke_n \leq b, \boden_n \geq a$, i.e. $\einschluss \subseteq \mathcal E^b_a$.
\end{proof} 
\end{thm}

%So far, our guarantee of optimality of the enclosure only holds for $p=1$. This is due to the fact that at present, we cannot guarantee that the minimum of two $p-L-$H\"older functions also is $p-L-$ H\"older, unless $p=1$. Intuitively, this might well be true also for $p<1$, but investigating this rigorously has to be deferred to future work.

\subsection{Proof of Thm. \ref{thm:KIdesiderata}}
\label{sec:proofKIdesiderata}
%
%
%\begin{defn}[Desiderata] \label{defn:desiderata}
 %Based on an observed, erroneous data set $D_n$, we desire to define enclosing functions $\decke_n, \boden_n$ that give rise to an enclosure $\einschluss$ with the following properties:
%
%\begin{enumerate} 
%
    %\item \textbf{Sample-Consistency}: The enclosure is sample-consistent, i.e. $\einschluss \subseteq \mathcal K(D_n)$.
		%%The enclosing functions are sample-consistent, i.e. $\decke_n,\boden_n \in \mathcal K(D_n)$.
    %
     %\item \textbf{Exhaustiveness (conservatism)}: Every $\phi, \lbf \leq \phi \leq \ubf$ coinciding with target $f$ on with grid $G_n$ and
%having at most Lipschitz
    %constant $L[J]$ on every subset $J \subset I$ is also contained in the enclosure: $\forall \phi: I \to \Real, \phi \in \mathcal K_{prior} \cap \mathcal K(D_n): \phi \in \einschluss $. That is, $\mathcal K_{prior} \cap \mathcal K(D_n) \subseteq \einschluss$.
    %In particular, the target is always contained in the enclosure: $f \in \einschluss$.
%
%\item \textbf{Monotonicity:} Additional data does not increase uncertainy. That is,
%if $G_n \subseteq G_{n+1} $, we have $\mathcal E^{\decke_{n+1}}_{\boden_{n+1}} \subseteq \einschluss, \forall n \in \nat$.
		   %
%\item \textbf{Convergence} to the target: Let the set of sample inputs $G_n$ in $D_n$ converge to a dense subset of domain $I$ and for each input $x \in I$ let the sample error function $\varepsilon: I \to \Real_{\geq 0}$ be bounded by $m_x \geq 0$ in some neighbourhood of $x$. Then, we have 
%\begin{itemize}
%\item (a) The sequence of enclosures converges point-wise. In particular, 
%
%$\forall x \in I: 0 \leq \lim_{n \to \infty} \decke_n (x) -\boden_n(x) \leq 2 m_x$.
%In particular, the enclosure converges to the target $f(x)$ at inputs $x$ where $m_x=0$.  
		%
		%\item (b) If convergence of $G_n$ is uniform and the target observations are error-free, i.e. $m_x = 0, \forall x \in I$, then the enclosure converges to the target $f$ uniformly.
%\end{itemize}	
   %\item \textbf{Minimality (optimality)}: 
%If an enclosure $\mathcal E^b_a$  satisfies \emph{Desideratum 2} then it is a superset of our enclosure $\einschluss$, i.e. $b \geq \decke_n, a \leq \boden_n$, $\einschluss \subseteq \mathcal E^b_a$.    
%
%\end{enumerate}
%
%\end{defn}
%
%\begin{defn}[Desiderata] \label{def:KIdesiderata} With definitions as above, we desire a machine learning algorithm to implement a mapping $\data_n \mapsto (\predfn,\prederrn)$ such that, for all data sets $\data_n$, the resulting inductive inference satisfies the following \textbf{desiderata}:
%\begin{enumerate}
	%\item \textit{Conservatism:} We can guarantee $\forall x \in \inspace \, \forall \phi \in \mathcal K_{prior} \cap \mathcal K(\data_n): \phi(x) \in \prederrbox_n(x)$. In particular, the ground-truth $f$ is always contained in the posterior set and its function values always are contained in the corresponding uncertainty hyperrectangles.
	%\item \textit{Monotonicity:} Additional data cannot increase the uncertainty. 
	%
	%That is, $\data_n \subseteq \data_{n+1} $ implies 
		%$\prederrbox_n(x) \supseteq \prederrbox_{n+1}(x)$ or equivalently, $\prederr_n(x) \geq \prederr_{n+1}(x), \forall x \in \inspace$ (where the inequality holds for each component).
	%%\item \textbf{Convergence} to the target: Let the set of sample inputs $G_n$ in $D_n$ converge to a dense subset of domain $I \subset \inspace$ and for each input $x \in I$ let the sample error function $\varepsilon: I \to \Real_{\geq 0}$ be bounded by $m_x \geq 0$ in some neighbourhood of $x$. Then, we have 
%%\begin{itemize}
%%\item (a) The uncertainty converges point-wise: $\forall x \in I: 0 \leq \lim_{n \to \infty} \prederrn(x) \leq m_x$.
%%In particular, the enclosure converges to the target $f(x)$ at inputs $x$ where $m_x=0$.  
		%%
		%%\item (b) If convergence of $G_n$ is uniform and the target observations are error-free, i.e. $m_x = 0, \forall x \in I$, then the enclosure converges to the target $f$ uniformly.
%%\end{itemize}	
	%\item \textit{Convergence}: If $(G_n )_{n \in \nat }$ is a sample grid sequence of inputs converging to a dense subset of $\inspace$ (as $n \to \infty$) then  $\prederrn(x) \stackrel{n \to \infty}{\longrightarrow} \varepsilon(x), \forall x \in \inspace$. If convergence of the grid to the dense subset is uniform (cf. Def. \ref{def:uniform_setconvergence}) and the observational error is constant ($\exists c \in \Real: \varepsilon \equiv c $) then the convergence  $\prederrn \stackrel{n \to \infty}{\longrightarrow} \varepsilon$ is uniform. 
	   %\item \textit{Minimality (optimality)}: There is no conservative uncertainty bound that is tighter than $\prederr_n$. That is, if for some hyperrectangle $H$, $x \in \inspace$ we have $H \subsetneq \prederrbox_n(x)$ then we have: $\exists x \in \inspace, \phi \in \mathcal K_{prior} \cap \mathcal K(\data_n) : \phi(x) \notin H$. In particular, it might be possible that the function value of the ground-truth function at $x$ is not contained in $H$.
%%If an enclosure $\mathcal E^b_a$  satisfies \emph{Desideratum 2} then it is a superset of our enclosure $\einschluss$, i.e. $b \geq \decke_n, a \leq \boden_n$, $\einschluss \subseteq \mathcal E^b_a$.    
%\end{enumerate}
%\end{defn}

We are now in a position to conclude the statement of Theorem \ref{thm:KIdesiderata} which is restated here for convenience:
\textbf{Theorem \ref{thm:KIdesiderata}:}

Assuming all (a priori) possible targets $f: \inspace \to \outspace$ are given by the class   
\begin{equation}
	\mathcal K_{prior}= \bigl\{ f : \inspace \to \outspace \subseteq \Real^m |  f \in \hoelset L {\metric_{\inspace}} p \cap \bfset \bigr\}
\end{equation}
where $\hoelset L {\metric_\inspace} p =\{ f: \inspace \to \outspace \subset \Real^m \, |  \forall j \in \{1,\ldots,m\} \forall x,x' \in \inspace: \abs{f_j(x) - f_j(x')}  \leq \, L_j \metric^p_{\inspace}(x,x') \}$ denotes the class of $L-p$- H\"older continuous functions with respect to metric $\metric_\inspace$ and $\bfset :=\{\phi : \inspace \to \outspace \, | \, \forall x \in \inspace, j \in\{1,...,m\}: \lbf_j(x) \leq \phi_j(x) \leq \ubf_j(x)\} $
is the set of all functions bounded component-wise between functions $\lbf,\ubf: \Real^d \to \Real \cup \{- \infty, \infty\}$, where we will always define $\Real_\infty := \Real \cup\{- \infty, \infty\}$. 

Then we have:
%\begin{enumerate}
%\item  
The inference rule as per Def. \ref{def:KIL} is conservative, monotonically convergent (in the limit of dense sample grids) and optimal in the sense of Def. \ref{def:KIdesiderata}. That is, it satisfies Desiderata 1-4 as per Def. \ref{def:KIdesiderata}. 
%\item If in addition, for some $d \in \nat$, $\inspace \subseteq \Real^d$ and $\metric_{\inspace}(x,x') = \norm{x-x'}$ for some norm that is equivalent to the Euclidean norm then the inference mechanism is also optimal (as per Desideratum 4 in Def. \ref{def:KIdesiderata}). That is, there is no other conservative inference mechanism with tighter uncertainty bound function $\prederrn$. 
%\end{enumerate}
%\end{thm}

\begin{proof}
We desire to apply Thm. \ref{thm:enclmain} to each component function.
Inspecting the definitions, this turns out to establish the desired statement for each component function of the predictors and target. 
Since the desiderata as per Def. \ref{def:KIdesiderata} are requirements for each output component, this will conclude the proof. 

In detail:
We prove the claim for each output component $j=1,...,m$. %So, let $j \in \{1,...,m\}$ be fixed. 
By assumption, the target's component function $f_j$ is $L_j-p$ H\"older. Remember from Def. \ref{def:KIL}, 
%\begin{align}
  $ \predfnj(x) := \frac{1}{2} \min\{ \ubf_j(x), \tilde \decke_{n,j}(x)\} + \frac{1}{2} \max\{ \lbf_j, \tilde \boden_{n,j}(x) \}$ and   
$	\prederrnj(x) := \frac{1}{2} \bigl(\min\{ \ubf_j(x), \tilde \decke_{n,j}(x)\} - \max\{ \lbf_j, \tilde \boden_{n,j}(x) \} \bigr)$
	%\end{align}
	with component functions given by
	$\tilde \decke_{n,j}(x) := \min_{i=1,\ldots,N_n}   \tilde f_{i,j} + L_j \metric^p(x,s_i) + \varepsilon_j(x)$ and 
	$\tilde \boden_{n,j}(x) := \max_{i=1,\ldots,N_n}   \tilde f_{i,j} - L_j \metric^p(x,s_i) - \varepsilon_j(x)$, respectively. 
Connecting to Thm. \ref{thm:enclmain}, for $x \in \inspace$, we define $\decke_n (x) := \predfnj(x) + \prederrnj(x) =  \min\{ \ubf_j(x), \tilde \decke_{n,j}(x) \}$ and $\boden_n (x) := \predfnj(x) - \prederrnj(x) =\max\{ \lbf_j, \tilde \boden_{n,j}(x) \} $. Furthermore, we note $\decke_n - \boden_n = 2 \prederrnj(x)$. So, convergence of the enclosure (i.e. convergence of $\decke_n - \boden_n$ ) is equivalent to convergence of $2 \prederrnj$. Finally, by definition, we see that $\decke_n^*(x) = \decke_{n,j}(x)$ and $\decke_n^*(x) = \boden_{n,j}(x)$ where $\decke^*_n, \boden^*_n$ match up the definitions of Def. \ref{def:optenclosingfcts}. 
Hence, Thm. \ref{thm:enclmain} is applicable. Therefore, Desideratum 1 -5 of Def. \ref{defn:desiderata} hold for the $j$th component of the prediction and target. 

Note, the $j$th prediction uncertainty interval $\prederrbox_j(x)$ just coincides with $[\boden_n(x), \decke_n(x)]$ (cf. Eq. \ref{eq:prederrint}). Thus, By Desideratum 2 of Def. \ref{defn:desiderata} we conclude:
%\begin{equation}\label{eq:prederrint}
$\forall \phi_j \in \einschluss : \phi_j(x) \in \prederrbox_{n,j}=[ \predfnj(x) - \prederrnj(x), \predfnj(x) + \prederrnj(x)] $.
%\end{equation}
%is referred to as the $j$th \textit{prediction uncertainty} interval.
In particular, this means $f_j(x)   \in \prederrbox_{n,j}$. Hence, Desideratum 1 of Def. \ref{def:KIdesiderata} (conservatism) holds.
The remaining desiderata as per Def. \ref{thm:KIdesiderata} follow from the validity of the corresponding desiderata as per Thm. \ref{thm:enclmain} on the enclosure for each component $j$. The fact that the desiderata in the former are equivalent to the validity of the desiderata for each component $j$ (and the latter can be shown by the established link 

By Desideratum 2 implies $\boden_n(x) \leq f_j(x) \leq \decke_n(x), \forall x$ which by our definition is equivalent to stating $f_j(x) \in [\boden_n(x), \decke_n(x)] = \prederrbox_j(x)$. Desiderata 3,4 of Def. \ref{defn:desiderata}, establishes the desired properties of monotonocity and convergence, which extend to the corresponding properties to $\prederrbox_j$ and hence, to $\prederrnj$. In turn, this establishes Desiderata 2-3 of Def. \ref{def:KIdesiderata}. 
Owing to the same link, $[\boden_n(x), \decke_n(x)] = \prederrbox_j(x)$, minimality of $\prederrbox_j(x)$ (i.e. of $\prederrnj$) follows from the minimality of the enclosure (Desideratum 5 of Def. \ref{defn:desiderata}). Thus, Desideratum 4 as per Def. \ref{def:KIdesiderata} holds as well.

\end{proof}

\section{Pruning of uninformative sample points}

The remaining derivations of this subsection show how the data can be pruned when new data points arrive the render old ones uninformative. They can be skipped by a reader not interested in the details.


We will focus our exposition on the ceiling functions. The derivations for the floor functions are entirely analogous (where one has to substitute $\leq$ by $\geq$ and $\min$ by $\max$).

\begin{lem}\label{lem:dominatedsamplefct}
Let $\mathcal N := \{1,...,N_n\}$, $q,i \in \mathcal N$ be the indices of a sample ceiling functions $\decke_n^q(\cdot;L_q)$ and $\decke_n^i(\cdot;L_i)$ where $L_q \leq L_i$ everywhere. We have
\[\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i) \Leftrightarrow \forall t \in I: \decke_n^q(t;L_q) \leq \decke_n^i(t;L_i).\]
\begin{proof}
$\underline \Rightarrow:$
$\decke_n^q (t;L_q) = \decke_n^q(s_q;L_q) + L_q \metricp(t, s_q)$
$\leq \decke_n^q(s_q;L_q) +L_q \metricp(s_i, s_q)+ L_q\metricp(t,s_i) $
$=\decke_n^q(s_i;L_q) +  L_q\metricp(t,s_i)$ 
$\leq \decke_n^i(s_i;L_i) + L_q\metricp(t,s_i)  $
$= \overline f(s_i) + L_q\metricp(t,s_i)    $
$\leq \overline f(s_i) + L_i\metricp(t,s_i)    = \decke_n^i(t;L)$.\\
$\underline \Leftarrow:$ Trivial.
\end{proof}
\end{lem}

The lemma implies that we can remove samples that are dominated by other samples' ceiling functions:
\begin{thm} 
\label{thm:removedominatedsamples}
Let $\mathcal N := \{1,...,N_n\}$ and let $i \in \mathcal N$ be the index of sample ceiling function $\decke_n^i(\cdot;L_i): t \mapsto \overline f(s_i) + L_i \abs{t - s_i}$. If there exists a sample ceiling function $u^q(\cdot;L_q), q \in \mathcal N \backslash \{i\}$, $L_q \leq L_i$ everywhere, having a value below $\decke_n^i$ at the $i$th sample, then the $i$th sample plays no role in computing the optimal ceiling. That is:\\  
If there is $q \in \mathcal N \backslash\{ i\}$ such that $\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i)$, then we have: \\
$\decke^*(t;L_1,\ldots,L_n) = \min_{j \in \mathcal N} \decke^j(t;L_j) =  \min_{j \in \mathcal N\backslash \{i\}} \decke^j(t;L_j)$.
\begin{proof}
The theorem is a direct consequence of Lem. \ref{lem:dominatedsamplefct}. 
\end{proof}

\end{thm}

\begin{rem}
Normally, $L_i = L_q\, \forall q,j \in \mathcal N$ where each $L_i$ is a function mapping $t$ to a H\"older constant valid in some neighbourhood of $t$.
\end{rem}

\begin{thm}
\label{thm:dominatedsamples_greatLIPconst}
Let $\mathcal N := \{1,...,N_n\}$ and let $i \in \mathcal N$ be the index of sample ceiling function $\decke_n^i(\cdot;L_i): t \mapsto \overline f(s_i) + L_i \metricp(t,s_i) $. We have: \\if $\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i)$ then 
\[  \decke^*(t;L_1,...,L_n) \geq \min_{j \in \mathcal N} \decke^j(t;L_j) =  \min \bigl\{ \min_{j \in \mathcal N\backslash \{i\}} \decke^j(t;L_j), \decke_n^q(s_i) + L_i \metricp(t,s_i) \bigr\}.\]

\begin{proof} Let $\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i)$ and $L_q > L_i $ everywhere. Since $\decke_n^q(s_i) \leq \decke_n^i(s_i)$ and $L_i < L_q$ we have $\decke_n^i(t;L_i) = \overline f(s_i) + L_i \metricp(t,s_i) $
$= \decke_n^i(s_i;L_i) + L_i \metricp(t,s_i)$
$\geq \decke_n^q(s_i;L_i) + L_i \metricp(t,s_i)$.

\end{proof}

\end{thm}

\begin{rem} \label{rem:assumptionsceil}
The theorems allow us to assume, without loss of generality, that $\decke_n^i(s_i) = \min_j \decke_n^j(s_i)$ (as a preprocessing step, Thm. 
\ref{thm:removedominatedsamples} allows us to remove samples violating this assumption, without changing the optimal ceiling). 
\end{rem}



\section{Special case: one-dimensional inputs, p=1}
\label{sec:onedimlipfloorceil}
For functions on one-dimensional domains and exponent $p=1$, matters simplify. We assume $\metric(x,y) := \abs{x-y}$. This case has been considered in the context of optimisation \cite{Shubert:72} and quadrature \cite{Baran2008} and the results therefore are not new. However, for our kinky inference method, the results rederived below have favourable practical implications (see Rem. \ref{rem:lipencl1d4KI}).
%
%gravity of the results of Thm Lem. \ref{lem:ceiling_maxvalues} and Lem. {lem:floor_minvalues} is that in the one dimensional (Lipschitz) case, the floor and ceiling functions (and hence, the prediction functions $\predfn, \prederrn$ can be evaluated based on the minimisation of two neighbouring 

%From now on, we will assume that $L_1,\ldots, L_n =: L$. 

For ease of notation we will therefore often omit explicit mention of $L$ in the statements of the ceiling and floor functions, unless it becomes necessary. Additionally, we assume, without loss of generality, that the sample inputs are ordered such that $s_1\leq \ldots \leq s_n$. Let $b := \sup I $ and $a := \inf I$.



Under these assumptions, we next show that computing the optimal ceiling function only requires taking into account the up to two most adjacent samples :

\begin{lem}\label{lem:shieldingsamples_1d}
Let the assumptions of Rem. \ref{rem:assumptionsceil} hold.

We have:

\begin{enumerate}
\item $\forall i \in \mathcal N, t \geq s_i: \decke_n^* ( t) =\min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N, j \geq i\}, $	
\item $\forall i \in \mathcal N, t \leq s_i: \decke_n^* ( t) =\min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N,j \leq i\}.$ 
\end{enumerate}

\begin{proof}
1.) Let $t \geq s_i$. 

$\text{Showing} \leq:$ This is trivial since $\decke_n^*(t) = \min_{j \in \mathcal N} \decke_n^j(t) \leq \min_{j \in \mathcal N, j \geq i}\decke_n^j(t)$. 


$\text{Showing} \geq:$ For contradiction, assume $\decke_n^* ( t) < \min_{j\geq i} \decke_n^j(t).$ 
Hence, there is a $q \in \mathcal N, q < i$ such that 

\begin{equation}
\label{eq:lala1}
\forall t \geq s_i: \decke_n^q(t) < \min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N, j \geq i\}.
\end{equation}
%Again, utilizing $s_i \leq t \leq s_{i+1}$ this is equivalent to $\exists q : \decke_n^q(t) < \overline f(s_i) + L \abs{t - s_i} \wedge \decke_n^q(t) < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$
%
%$\stackrel{def.}{\Leftrightarrow} \exists q : \overline f(s_q) + L \abs{t - s_q} < \overline f(s_i) + L \abs{t - s_i} \wedge f(s_q) + L \abs{t - s_q} < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$.
Choose such a $q \in \mathcal N, q < i$.
By assumption, we have $s_q < s_i$. Hence, Condition \ref{eq:lala1} implies in particular $\decke_n^q(t) = \overline f(s_q) + L (t - s_q) < \decke_n^i(t) = \overline f(s_i) + L (t - s_i)$. We have $\overline f(s_q) + L (t - s_q) = \overline f(s_q) + L (s_i - s_q) + L (t - s_i) = \decke_n^q(s_i) + L (t-s_i) \stackrel{!}{ <} \overline f(s_i) + L (t-s_i)=\decke_n^i(s_i) + L (t-s_i) $ which holds, if and only if $\decke_n^q(s_i) < \decke_n^i(s_i)$. However, the last inequality contradicts our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (Rem. \ref{rem:assumptionsceil}).\\

2.) The proof is analogous to 1.):

Let $t \leq s_i$. 

$\text{Showing} \leq:$ This is trivial since $\decke_n^*(t) = \min_{j \in \mathcal N} \decke_n^j(t) \leq \min_{j \in \mathcal N, j \leq i}\decke_n^j(t)$. 


$\text{Showing} \geq:$ For contradiction, assume $\decke_n^* ( t) < \min_{j\leq i} \decke_n^j(t).$ 
Hence, there is a $q \in \mathcal N, q > i$ such that 

\begin{equation}
\label{eq:lala2}
\forall t \leq s_i: \decke_n^q(t) < \min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N, j \leq i\}.
\end{equation}
%Again, utilizing $s_i \leq t \leq s_{i+1}$ this is equivalent to $\exists q : \decke_n^q(t) < \overline f(s_i) + L \abs{t - s_i} \wedge \decke_n^q(t) < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$
%
%$\stackrel{def.}{\Leftrightarrow} \exists q : \overline f(s_q) + L \abs{t - s_q} < \overline f(s_i) + L \abs{t - s_i} \wedge f(s_q) + L \abs{t - s_q} < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$.
Choose such a $q \in \mathcal N , q > i$ (thus, $s_q > s_i$).


The way we ordered the samples, $q>i$ implies $s_q > s_{i}$. Thus, Condition \ref{eq:lala2} implies in particular: $\decke_n^q(t) =\overline f(s_q) + L (s_q -t ) < \decke_n^i(t) = \overline f(s_{i}) + L ( s_{i} -t) = \decke_n^{i}(s_{i}) + L ( s_{i} -t)$. We have $\overline f(s_q) + L (s_q-t) = \overline f(s_q) + L (s_q - s_{i} ) + L (s_{i} - t) = \decke_n^q(s_{i}) + L (s_{i} - t) \stackrel{!}{ <} \decke_n^{i}(s_{i}) + L (s_{i} -t) $. However, the last inequality contradicts our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (made in Rem. \ref{rem:assumptionsceil}).



%By definition of the sample ceilings, it follows 
%$\exists q : \decke_n^q(t) < \decke_n^i(t) \wedge \decke_n^q(t) < \decke_n^{i+1} (t)$.
\end{proof}

\end{lem}


The Lemma allows us to tremendously simplify computation of the optimal ceiling-- it tells us that all samples, except the up to two neighbouring ones, can be discarded when computing the optimal ceiling at a given input:

\begin{thm}\label{thm:lipceil1d}
Let the assumptions of Rem. \ref{rem:assumptionsceil} hold.
Let $a:=s_0: = \inf I, s_{n+1} := b:=\sup I$ and for $i=0,\ldots,N_n$ define $I_i := [s_i,s_{i+1}]$.

%we define line segments via \[\alpha^\decke_n_i: t
%\mapsto \overline f(s_i) + L (t - s_i)\] and \[\beta^\decke_n_i: t \mapsto
%\overline f(s_{i+1}) -L (t - s_{i+1}).\] 

We have:

\[ \forall i, t \in I_i: \decke_n^*(t) = \begin{cases} \decke_n^{i+1}(t) &, i=0\\
															\min\{\decke_n^i(t),\decke_n^{i+1}(t) \}&, i \in \{1,\ldots,N_n-1 \} \\
															\decke_n^{i}(t)&, i=N.	\end{cases} \]


\end{thm}



The analogous statement for the H\"older floor function can be derived completely analogously and will therefore be given at this point without proof:


\begin{thm}\label{thm:lipfloor1d}
Assume the assumptions of Rem. \ref{rem:assumptionsceil} hold.
Let $a:=s_0: = \inf I, s_{n+1} := b:=\sup I$ and for $i=0,\ldots,N_n$ define $I_i := [s_i,s_{i+1}]$.

%we define line segments via \[\alpha^\boden_i: t
%\mapsto \overline f(s_i) + L (t - s_i)\] and \[\beta^\boden_i: t \mapsto
%\overline f(s_{i+1}) -L (t - s_{i+1}).\] 

We have:

\[ \forall i, t \in I_i: \boden_n^*(t) = \begin{cases} \boden_n^{i+1}(t) &, i=0\\
															\max\{\boden_n^i(t),\boden_n^{i+1}(t) \}&, i \in \{1,\ldots,N_n-1 \} \\
															\boden_n^{i}(t)&, i=N.	\end{cases} \]


\end{thm}

In addition to saving computation by discarding irrelevant samples, the the theorems will play an important role when computing a closed-form the integral of the optimal ceiling and floor functions.


%\begin{cor}\label{cor:lipceil}
%Assume the assumptions of Rem. \ref{rem:assumptionsceil} hold.
%On interval $I_i = [s_i,s_{i+1}]$ we define line segments via \[\alpha^\decke_n_i: t
%\mapsto \overline f(s_i) + L (t - s_i)\] and \[\beta^\decke_n_i: t \mapsto
%\overline f(s_{i+1}) -L (t - s_{i+1}).\] 
%
%We have:
%
%\begin{enumerate}
%\item
%For $i \in \mathcal N$ the projection of the optimal H\"older ceiling onto interval $I_i$ can be computed as the point-wise minimum of $\alpha^\decke_n_i$ and $ \beta^\decke_n_i$:
%\[\forall t \in I_i: \decke_n^* ( t) =\min\{ \alpha^\decke_n_i(t), \beta^\decke_n_i(t) \}= \min\{\decke_n^i(t),\decke_n^{i+1}(t) \} .\] 
%
%\item $\forall t \in [a,s_1], \tau \in [s_n,b] : \decke_n^*(t) = \decke_n^1(t) \wedge  \decke_n^*(\tau) = \decke_n^N(\tau)$.
%\end{enumerate}
%\begin{proof}
%1.) Since $s_i \leq t \leq s_{i+1}$, $\alpha^\decke_n_i(t) = \decke_n^i(t)$ and $\beta^\decke_n_i(t) = \decke_n^{i+1}(t)$.
%Let $t \in I_i$.
%
%$\text{Showing} \leq:$ By definition, $\decke_n^*(t) = \min_j \decke_n^j(t) = \min_j \overline f(s_j) + L \abs{t - s_j}  \leq \min\{\overline f(s_i) + L \abs{t - s_i}, \overline f(s_{i+1}) + L \abs{t - s_{i+1}} \} = \min\{\overline f(s_i) + L (t - s_i), \overline f(s_{i+1}) - L  (t-s_{i+1}) \}$ where the last equality holds owing to $s_i \leq t \leq s_{i+1}$.
%
%$\text{Showing} \geq:$ For contradiction, assume $\decke_n^* ( t) <  \min\{\overline f(s_i) + L (t - s_i), \overline f(s_{i+1}) - L  (t-s_{i+1}) \}$. This implies the existence of a $q \in \mathcal N$ such that 
%
%\begin{equation}
%\label{eq:lala1}
%\decke_n^q(t) < \overline f(s_i) + L (t - s_i)
%\end{equation}
%and 
%\begin{equation}
%\label{eq:lala2}
 %\decke_n^q(t) < \overline f(s_{i+1}) - L  (t-s_{i+1}). 
%\end{equation}
%%Again, utilizing $s_i \leq t \leq s_{i+1}$ this is equivalent to $\exists q : \decke_n^q(t) < \overline f(s_i) + L \abs{t - s_i} \wedge \decke_n^q(t) < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$
%%
%%$\stackrel{def.}{\Leftrightarrow} \exists q : \overline f(s_q) + L \abs{t - s_q} < \overline f(s_i) + L \abs{t - s_i} \wedge f(s_q) + L \abs{t - s_q} < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$.
%Choose such a $q \in \mathcal N$.
%
%Case A: Let $s_q < s_i$. Then, Condition \ref{eq:lala1} implies $\decke_n^q(t) = \overline f(s_q) + L (t - s_q) < \overline f(s_i) + L (t - s_i)$. We have $\overline f(s_q) + L (t - s_q) = \overline f(s_q) + L (s_i - s_q) + L (t - s_i) = \decke_n^q(s_i) + L (t-s_i) \stackrel{!}{ <} \overline f(s_i) + L (t-s_i)=\decke_n^i(s_i) + L (t-s_i) $ which holds, if and only if $\decke_n^q(s_i) < \decke_n^i(s_i)$. However, the last inequality contradicts our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (Rem. \ref{rem:assumptionsceil}).
%
%Case B: Let $s_q > s_{i+1}$. Then, Condition \ref{eq:lala2} implies $\overline f(s_q) + L (s_q -t ) < \overline f(s_{i+1}) + L ( s_{i+1} -t) = \decke_n^{i+1}(s_{i+1}) + L ( s_{i+1} -t)$. We have $\overline f(s_q) + L (s_q-t) = \overline f(s_q) + L (s_q - s_{i+1} ) + L (s_{i+1} - t) = \decke_n^q(s_{i+1}) + L (s_{i+1} - t) \stackrel{!}{ <} \decke_n^{i+1}(s_{i+1}) + L (s_{i+1} -t) $. However, the last inequality contradicts our our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (made in Rem. \ref{rem:assumptionsceil}).
%We have proven the first claim.\\
%
%2.) 
%
%%By definition of the sample ceilings, it follows 
%%$\exists q : \decke_n^q(t) < \decke_n^i(t) \wedge \decke_n^q(t) < \decke_n^{i+1} (t)$.
%\end{proof}
%
%\end{cor}



In preparation for the part on quadrature it will prove useful to determine the extrema of the enclosing functions on each subinterval $I_i$.


\begin{lem} \label{lem:Lipbetweensamples}
We have:
\begin{enumerate}
\item If $\decke^i(s_i)  \leq \decke^{i+1}(s_i)$ and $\decke^{i+1}(s_{i+1})  \leq \decke^i(s_{i+1})$ then 
we have 

$ \abs{\overline f(s_{i+1})- \overline f(s_i)} \leq L \abs{s_{i+1} -s_i}$.
\item If $\boden^i(s_i)  \geq \boden^{i+1}(s_i)$ and $\boden^{i+1}(s_{i+1})  \geq \boden^i(s_{i+1})$ then 
we have

$ \abs{\underline f(s_{i+1})- \underline f(s_i)} \leq L \abs{s_{i+1} -s_i}$.
\end{enumerate}

\begin{proof}
1.) 
On the one hand, we have:
$\decke^i(s_i)  \leq \decke^{i+1}(s_i)$ 
$\Leftrightarrow$
 $\decke^i(s_i) - \decke^{i+1}(s_i)  \leq 0$
%
$\Leftrightarrow$ $ \overline f(s_i) + L \abs{s_i-s_i} -\overline f(s_{i+1}) - L \abs{s_i-s_{i+1}}  \leq 0$
%
$\Leftrightarrow$ $ \overline f(s_i) -\overline f(s_{i+1}) - L \abs{s_i-s_{i+1}}  \leq 0$
%
$\Leftrightarrow$ $ \overline f(s_i) -\overline f(s_{i+1})   \leq  L \abs{s_i-s_{i+1}}$

$\Leftrightarrow$ $ \overline f(s_{i+1})-\overline f(s_i)    \geq  -L \abs{s_{i+1} - s_i}$.\\
%
On the other hand:
$\decke^{i+1}(s_{i+1})  \leq \decke^i(s_{i+1})$
%
$\Leftrightarrow$ $\decke^{i+1}(s_{i+1}) - \decke^i(s_{i+1}) \leq 0$
$\Leftrightarrow$ $\overline f(s_{i+1})  - \overline f(s_i) - L \abs{s_{i+1} -s_i} \leq 0$
$\Leftrightarrow$ $\overline f(s_{i+1})  - \overline f(s_i)  \leq  L \abs{s_{i+1} -s_i}$.

2.) The proof is completely analogous to 1.). 
\end{proof}
\end{lem}

\begin{lem} \label{lem:ceiling_maxvalues}
Let $\metric(x,y) := \abs{x-y}$. For $i \in \{1,\ldots,N_n-1\}$ let  $L_i > 0$, $I_i = [s_i,s_{i+1}]$.
Define $\xi^{\mathfrak u}_i :=  \frac{s_i+s_{i+1}}{2}+ \frac{\overline f(s_{i+1}) - \overline f(s_i)}{2 L_i}  $.\\
For $t \in I_i$ we have 
\begin{enumerate}
\item $\xi^{\mathfrak u}_i \in I_i$ and  $\decke^*_n(t) = 
 \begin{cases}  
 \decke^i_n (t), & t \leq \xi^\decke_i \\
 \decke^{i+1}_n(t), & t \geq \xi^\decke_i.
 \end{cases}$
\item $\xi^{\mathfrak u}_i \in \arg\max_{\tau \in I_i} \decke^*_n (\tau)$.
\item  $y^{\mathfrak u}_i := \decke_n^*(\xi^{\mathfrak u}_i) = \frac{\overline f(s_{i+1}) +\overline f(s_i)}{2} + L_i \frac{s_{i+1}-s_i}{2}$ .
\end{enumerate}
\begin{proof} Let $1 \leq i \leq N-1, t \in I_i$. Define $\alpha^\decke_i(t) = \overline f(a_i) + L_i (t-a_i) = \decke_n^i(t), \beta^\decke_i (t) = \overline f(b_i) + L_i (b_i - t) = \decke^{i+1}_n(t), \forall t \in I_i$.

Firstly, $\xi^\decke_i \in I_i$ is a direct consequence of Lem. \ref{lem:Lipbetweensamples}.

Secondly, we show $\decke^*_n(t) = 
 \begin{cases}  
 \decke^i_n (t), & t \leq \xi^\decke_i \\
 \decke^{i+1}_n(t), & t \geq \xi^\decke_i.
 \end{cases}$:

By definition,
$\decke^*_n (t) = \min\{ \decke^{i}_n(t), \decke^{i+1}_n(t)\} = \min\{\alpha^i_n (t),\beta^i_n(t)\}$.
We have $\dot  \alpha^\decke_i(t) = L_i > 0$ and $\dot  \beta^\decke_i(t) = - L_i < 0$. Hence, the functions are strictly monotonous. Let $\xi$ be the input where the lines intersect, i.e. $\alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$. Monotonicity implies $\forall t \leq \xi : \alpha^\decke_i(t) \leq \alpha^\decke_i(\xi) \wedge \beta^\decke_i(t) \geq \beta^\decke_i(\xi) = \alpha^\decke_i(\xi)$. 
Hence,
 \[\forall t \leq \xi: \decke^*_n(t) = \min \{\alpha_i^{\mathfrak u} (t), \beta_i^{\mathfrak u} (t) \}= \alpha_i^{\mathfrak u} (t).\] 
 
Analogously, monotonicity implies $\forall t \geq \xi : \beta^\decke_i(t) \leq \beta^\decke_i(\xi) \wedge \alpha^\decke_i(t) \geq \alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$. 
Thus,
 \[\forall t \geq \xi: \decke^*_n(t) = \min \{\alpha_i^{\mathfrak u} (t), \beta_i^{\mathfrak u} (t) \}= \beta_i^{\mathfrak u} (t).\] 

In conjunction, we have 
 $\decke^*_n(t) = 
 \begin{cases}  
 \alpha_i^{\mathfrak u} (t), & t \leq \xi \\
 \beta_i^{\mathfrak u} (t), & t \geq \xi 
 \end{cases}$.
 Again, using monotonicity of $\alpha_i^{\mathfrak u}$ and $\beta_i^{\mathfrak u}$ we infer that $\decke^*_n$ has a single maximum $y := \decke^*_n(\xi)$ at $\xi$.

Next, we show that $\xi = \xi_i^{\mathfrak u}$: 

$\alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$

$\Leftrightarrow  \overline f(s_i) + L_i (\xi - s_i) = \overline f(s_{i+1}) -L_i (\xi - s_{i+1})$

$\Leftrightarrow  L_i \bigl( 2 \xi - s_{i+1}  - s_i\bigr) = \overline f(s_{i+1}) - \overline f(s_i) $

$\stackrel{L_i > 0}{\Leftrightarrow}   \bigl( 2 \xi - s_{i+1}  - s_i\bigr) = \frac{\overline f(s_{i+1}) - \overline f(s_i)}{L_i} $

$\Leftrightarrow   \xi  = \frac{\overline f(s_{i+1}) - \overline f(s_i)}{2 L_i}  + \frac{s_{i+1}+s_i}{2} = \xi^{\mathfrak u}_i$.



Finally, we need to evaluate $\decke^*_n(\xi^{\mathfrak u}_i)$ to prove the last claim:
We have 

 $\decke^*_n(\xi) = \alpha_i^{\mathfrak u} (\xi) =  \overline f(s_i) + L_i (\xi - s_i) $

$= \overline f(s_i) + L_i \bigl( \frac{\overline f(s_{i+1}) - \overline f(s_i)}{2 L_i}  + \frac{s_{i+1}+s_i}{2} - s_i \bigr) $ 

$=  \frac{\overline f(s_{i+1}) - \overline f(s_i) + 2\overline f(s_i)}{2 }  + L_i \frac{s_{i+1}-s_i}{2}   = y_i^{\mathfrak u}$. 



\end{proof}

\end{lem}


Completely analogously to the the proof of Lem. \ref{lem:ceiling_maxvalues} we can prove the corresponding statement for the H\"older floor:
\begin{lem} \label{lem:floor_minvalues}
Let $\metric(x,y) := \abs{x-y}$.
For $i \in \{1,\ldots,N_n-1\}$ let  $L_i > 0$, $I_i = [s_i,s_{i+1}]$.
Define $\xi^{\boden}_i :=  \frac{s_i+s_{i+1}}{2}- \frac{\underline f(s_{i+1}) - \underline f(s_i)}{2 L_i}  $.\\
For $t \in I_i$ we have 
\begin{enumerate}
\item $\xi^{\boden}_i \in I_i$ and  $\boden^*_n(t) = 
 \begin{cases}  
 \boden^i_n (t), & t \leq \xi^\boden_i \\
 \boden^{i+1}_n(t), & t \geq \xi^\boden_i.
 \end{cases}$
\item $\xi^{\boden}_i \in \arg\min_{\tau \in I_i} \boden^*_n (\tau)$.
\item  $y^{\boden}_i := \boden_n^*(\xi^{\boden}_i) = \frac{\underline f(s_{i+1}) +\underline f(s_i)}{2} - L_i \frac{s_{i+1}-s_i}{2}$ .
\end{enumerate}

\begin{proof} The proof is analogous to the one provided for Lem. \ref{lem:ceiling_maxvalues}.
%
%The case $i = N$ is trivial. Let $1 \leq i \leq N-1$. By definition,
%$\boden^i_n (t) = \min\{ \alpha^\boden_i(t), \beta^\boden_i(t)\}$.
%We have $\dot  \alpha^\boden_i(t) = - L_i < 0, \forall t$ and $\dot  \beta^\boden_i(t) =  L_i > 0, \forall t$. Hence, the functions are strictly monotonous. Let $\xi$ the input where the lines intersect, i.e. $\alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$. Monotonicity implies $\forall t \leq \xi : \alpha^\boden_i(t) \geq \alpha^\boden_i(\xi) \wedge \beta^\boden_i(t) \leq \beta^\boden_i(\xi) = \alpha^\boden_i(\xi)$. 
%Hence,
 %\[\forall t \leq \xi: \boden_n^i(t) = \max \{\alpha_i^{\mathfrak l} (t), \beta_i^{\mathfrak l} (t) \}= \alpha_i^{\mathfrak l} (t).\] 
 %
%Analogously, monotonicity implies $\forall t \geq \xi : \beta^\boden_i(t) \geq \beta^\boden_i(\xi) \wedge \alpha^\boden_i(t) \leq \alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$. 
%Thus,
 %\[\forall t \geq \xi: \boden_n^i(t) = \max \{\alpha_i^{\mathfrak l} (t), \beta_i^{\mathfrak l} (t) \}= \beta_i^{\mathfrak l} (t).\] 
%
%In conjunction, we have 
 %$\boden_n^i(t) = 
 %\begin{cases}  
 %\alpha_i^{\mathfrak l} (t), & t \leq \xi \\
 %\beta_i^{\mathfrak l} (t), & t \geq \xi 
 %\end{cases}$.
 %Again, utilizing monotonicity of $\alpha_i^{\mathfrak l}$ and $\beta_i^{\mathfrak l}$ we infer that $\boden_n^i$ has a single minimum $y := \boden_n^i(\xi)$ at $\xi$.
%It remains  (i) to show that $\xi = \xi_i^{\mathfrak l}$, (ii) we need to evaluate $\boden_n^i(\xi^{\mathfrak l}_i)$ showing $y = y_i^{\mathfrak l}$, and (iii) we need to show that 
%$\xi^{\mathfrak l}_i \in \bar I_i$ .
%
%(i) $\alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$
%
%$\Leftrightarrow  f(a_i) - L_i (\xi - a_i) = f(b_i) +L_i (\xi - b_i)$
%
%$\Leftrightarrow  L_i \bigl( 2 \xi - b_i  - a_i\bigr) = f(a_i) - f(b_i) $
%
%$\stackrel{L_i > 0}{\Leftrightarrow}   \bigl( 2 \xi - b_i  - a_i\bigr) = \frac{f(a_i) - f(b_i)}{L_i} $
%
%$\Leftrightarrow   \xi  = \frac{f(a_i) - f(b_i)}{2 L_i}  + \frac{b_i+a_i}{2} = \xi^{\mathfrak l}_i$.
%
%(ii) $\boden_n^i(\xi) = \alpha_i^{\mathfrak l} (\xi) =  f(a_i) - L_i (\xi - a_i) $
%
%$= f(a_i) - L_i \bigl( \frac{f(a_i) - f(b_i)}{2 L_i}  + \frac{b_i+a_i}{2} - a_i \bigr) $ 
%
%$=  \frac{-f(a_i) + f(b_i) + 2f(a_i)}{2 }  - L_i \frac{b_i-a_i}{2}   = y_i^{\mathfrak l}$. 
%
%(iii) $\xi^{\mathfrak l}_i \in \bar I_i$ if and only if $a_i \leq \xi^{\mathfrak l}_i \leq b_i$. Since $\xi^{\mathfrak l}_i = -\frac{f(b_i) - f(a_i)}{2 L_i}  + \frac{b_i+a_i}{2}$ and $\frac{b_i+a_i}{2}$ is just in the middle value of interval $\bar I_i = [a_i,b_i]$, we have 
%
%$\xi^{\mathfrak l}_i \in \bar I_i$ if $\abs{\frac{f(b_i) - f(a_i)}{2 L_i}} \leq \abs{\frac{b_i-a_i}{2}}$.
%However, the latter is the case due to $L_i$-H\"older continuity of $f$ on $\bar I_i$.  
  
\end{proof}

\end{lem}

\begin{rem}[Reduction of computational effort for KI and collision detection] \label{rem:lipencl1d4KI}
While the results above are not new, their statement has practical benefits in terms of computational effort of the kinky inference rule in one-dimensions when the canonical metric $\metric(x,x') = \abs{x-x'}$ is employed and $p=1$. Then Thm. \ref{thm:lipceil1d} and Thm. \ref{thm:lipfloor1d} tell us that the ceiling and floor functions can be evaluated by only considering the two most adjacent sample ceiling and floor functions. If we maintain a search tree over the grid, we can search for those two entries in $\mathcal O(\log N_n)$. This reduces the computational effort for evaluating the prediction functions $\predfn,\prederrn$ (cf. Def. \ref{def:KIL}) from linear to logarithmic asymptotic complexity. This can make a significant difference in terms of computational speed of the inference in the presence of large data sets.

As a second benefit of our derivations, Lem. \ref{lem:floor_minvalues} and Lem. \ref{lem:ceiling_maxvalues} can be utilised in the collision detection method as presented in Sec. \ref{sec:adaptiveLipshubertstyle} where negative function values need to be proven or ruled out. The Lemmata tell us which finite number of points to check.
\end{rem}

==> content2/Ch_kinkyinf/SIctrl_Hfe.tex <==
\section{Kinky inference and model reference adaptive control}
\label{sec:hfeandcontrol}
\label{sec:ctrlapplications}
In Sec. \ref{sec:KI_core}, we have presented \textit{kinky inference} (KI),  a non-parametric machine learning method that entertains assumptions about H\"older continuity and boundedness and can handle interval-bounded noise. In this section, we illustrate the utility of the approach in the context of model learning of nonlinear dynamical systems and (tracking) control.

As a first test and introduction to the control applications, Sec. \ref{sec:firstorderctrlandKI} considers an application of KI for model learning and control in a first-order system where the control can directly influence the velocity of a continuous-time plant. The bounds afforded by the KI rule are employed to provide a stability guarantee for a controlled uncertain system that meets the prior assumptions of the KI learner. 
In Sec. \ref{sec:KIMRAC}, we translate the controller to a more realistic second-order system. 
Simulations conducted in the context of wingrock tracking control demonstrate that our KI learning method is well suited for learning dynamic system models both offline and online and can outperform established machine learning methods such as Gaussian processes or radial basis function neural networks in model-reference adaptive control. 
%\jcom{If possible include SIIC and inversion model learning}


   

\subsection{A kinky inference velocity controller with stability guarantees }
\label{sec:firstorderctrlandKI}
Consider an agent that desires to control a plant with the first-order dynamics 
$\dot x = f(x) + g(x) u $
where $x \in \statespace \subset \Real^d$ is the state (``position'') and $u \in \Real^d$ a control that can be chosen by the agent. Set $\inspace$ might be some bounded space. For instance, the bounds could be imposed by the confines of a room a robot moves in or, in heating control, might be a range of temperatures. 
For simplicity, we assume that $g(x) \in \Real^{d \times d}$ is invertible and known for all $x \in \statespace$. By contrast, drift vector field $f$ is assumed to be uncertain a priori and will be identified and inverted utilising our kinky inference rule.
%We then combine the learner with a closed-loop inversion procedure quite in lieu to the procedure outlined in Ch. \ref{ch:SPSIIC}. (That is, in place of a random field the belief over $f$ will be inferred by the kinky inference learner introduced above.)


It is our aim to design a controller such that state trajectory $x(\cdot)$ follows \textit{reference} trajectory $\xref(\cdot)$. 
For instance, in the one-dimensional case, if we desire the state to reach setpoint $\xi$ we could set the reference derivative to $\dxref(t) = w (\xi - x )$, i.e. $\xref(t) = x(0) \exp( - w t ) - \xi (1- \exp(1- Kt) )$. That is, if the devised control law were successful in causing the state to follow the reference, the state  would converge to the target $\xi$ as $t \to \infty$. Control with a reference model is also referred to as \textit{tracking}, since the objective is to follow (i.e. track) the reference signal $\xref$. A special case, which we also have encountered in Ch. \ref{ch:SPSIIC}, is the task of \textit{stabilisation}. Here, the reference signal $\xref$ is set to a constant setpoint $\xi \in \statespace$. That is, the only control objective is to reach, and stay close to, the one point $\xi$. Note, in setpoint control we have $\dxref =0$.
%Alternatively, we might choose $\xref =\xi, \dxref=\dot \xi =0$ and need to make sure 

Having chosen a reference, we can utilise feedback linearisation in a model-reference adaptive control fashion \cite{Narendra1989} similar to the approach in Ch. \ref{ch:SPSIIC} and Sec. \ref{sec:KIMRAC}. That is, we define a control law:
\begin{equation}
	u:= g^{-1}(x) ( \nufb - \nu_{ad} + \nuref).
\end{equation}
Here, $\nuref := \dxref(t)$ defines the reference derivative and $\nufb$ is a \textit{feedback element} we will define below. Furthermore, intended to remove the drift $f$,
\textit{adaptive element} $\nu_{ad} := \predfn(x)$ is the output of the kinky inference rule as per Def. \ref{def:KIL} after having observed data set $\data_n=\Bigl\{\bigl(x_j, f(x_j), \varepsilon(x_j) \bigr) \,|\, j=1,...,N_n\Bigr\}$ containing a (noisy) sample of the drift at $N_n$ inputs $x_1,\ldots,x_{N_n}$. 

Closing the control-loop changes the plant dynamics to
%\begin{equation}
$\dot x = F(x) +\nufb + \nuref = F(x) +\nufb + \dxref$
%\end{equation}
where $F_n(x) = f(x) - \predfn(x)$. 
Consequently the \textit{error dynamics} are
\begin{equation}
	\dot e = F_n(x) +\nufb
\end{equation}
where the \textit{state error trajectory} $e (\cdot) = x(\cdot)- \xref(\cdot)$ represents the deviation of the state trajectory from the nominal trajectory given by the reference.

Since the drift $f$ is uncertain, $F(x)$ will generally not be zero. Assuming $f$ satisfies the prior assumptions inserted into the kinky inference learner ($f \in \mathcal K_{prior}$), Thm. \ref{thm:KIdesiderata} guarantees that the prediction bounds $\prederr$ provided by our KI rule (cf. Def. \ref{def:KIL}) hold and $F$ is bounded. In particular, $F_n(x) \in E_n := [-\prederr_{n,1}(x), \prederr_{n,1}(x)] \times [-\prederr_{n,d}(x),...,\prederr_{n,d}(x)]$ where $\prederrn$ is defined as per Def. \ref{def:KIL}.
 
One way of driving the error to zero and to supress the influence of the remaining uncertainty is to set the feedback term to $\nufb = -K e$ with $K := \text{diag}(w_1,...,w_d)$ for some gain weights $w_1,...,w_d \geq 0$.
%
This yields error dynamics given by the differential equation:
 \begin{equation}
	\dot e (t) = F_n(x(t)) - K e(t).
\end{equation}


%If we can bound the error, we can construct a robust tube about the trajectory and harness it for stability analysis and collision avoidance:
%By integration, we see that $x(\tau) = x(0) + \int_0^\tau \dxref(t) \dt + \int_0^\tau F(x(t)) - K x(t) \dt = \xref(\tau) + e(t)$.
We will now analyse the impact of both $K$ and the maximal prediction uncertainty on stability.

Remember, we can restate the differential equation integral form as follows (cf. Lem. \ref{lem:intcurve}):
 %\begin{equation}
	$e (t) = e(0) + \int_{0}^t - K e(\tau) \d \tau+ \int_{0}^t F_n(x(\tau)) \d \tau  .$
%\end{equation}
Since $F_n = f - \predfn$, by Thm. \ref{thm:KIdesiderata}, $\abs{F_n(x)} \leq \maxerrn:= \sup_{x \in \statespace}\norm{\prederrn(x)}_\infty $. Thus, 
$\norm{e (t)}_\infty \leq  \norm{ e(0) + \int_{0}^t - K e(\tau) \d \tau}_{\infty} + \norm{ \int_{0}^t F_n(x(\tau)) \d \tau}_\infty \leq \norm{ e(0) + \int_{0}^t - K e(\tau) \d \tau}_{\infty} +t \, \maxerrn.$ Observe,
 $e(0) + \int_{0}^t - K e(\tau) \d \tau $ is the solution to the ODE $\dot e = - K e$ with initial value $e(0)$. The solution is well-known to be:  $e(0) \exp(-K t)$ (cf. Sec. \ref{sec:OUprocess}). Therefore, the following bound always holds:
%
\begin{equation}\label{eq:errorboundgrowingconttimeKI}
	\norm{e (t)}_\infty \leq \norm{ e(0) \exp(-K t)}_{\infty} +t \, \maxerrn.
\end{equation}
Note, the term $\maxerr$ depends on the learning experience. As we know from Thm. \ref{thm:KIdesiderata}, the uncertainty of the learner (and hence $\maxerrn$ vanishes with increasing data size). Hence, the state  error bound can be reduced if the environment of the agent is uniformly explored.

\subsubsection{An agent exploration scenario} 
\label{sec:agentexploration}
%\textbf{An agent exploration scenario.}  
\begin{figure}\label{fig:explorsingleint}
        \centering
				\subfigure[Path taken by the exploring agent.]{
    \includegraphics[width =5cm, height =4cm]{content/figures/situationexplore1.pdf}
  } %\hspace{2cm}
		%\subfigure[Phase plot prior training.]{
    %\includegraphics[scale =.4]{content/figures/situationexplore.pdf}
  %} %\hspace{2cm}
	%\subfigure[Full history of exploring agent.]{
   %\includegraphics[scale =.35, clip, trim = 3.5cm 9cm 4cm 5cm]{content/figures/animate_hist.pdf}
  %}
       \caption{Path of an agent exploring the map. The agent obtains a new drift training example every 7 seconds. The start position is denoted by $S_1$. The subsequent waypoints (given by the setpoints), denoted by $SP1,...,SP11$, were determined incrementally as the positions of maximum posterior uncertainty. That is, on the basis of data set $\data_n$ the agent chose a new setpoint $\xi$ with components $\xi_j \in \arg\max_{x \in \statespace} \prederr_{n,j}(x)$. Note how the agent became increasingly successful in reaching his waypoints. With increasing learning experience, the trajectories become increasingly straight. This is a result of the adaptive element becoming more successful over time in cancelling the nonlinearity of the uncertain drift.} 
       %
\end{figure}	  
%The bounds we derived provide an insight into a trade-off between uncertainty and tighten with decreasing maximal uncertainty $\maxerr$ as well as with increased feedback gain. The understanding between 
%
%
As an illustration, consider the a situation in which an agent is deployed in a confined state space, say an ``arena'' $\statespace = [0, 10] \times  [0,10]$. The agent's plant adheres to a dynamic model as above with uncertain drift field $f(x) = \begin{cases}  [\sin(x_1); 2 \cos(x_2)], &\,  x \in \statespace\\ [0;0], &\text{otherwise}. \end{cases} $. Initially the agent is uncertain about the drift. However, we assume it can acquire a sample point of the drift at its current location once every $\tinc =7$ seconds at times $n\tinc$ ($n \in \nat_0$). The observations are obtained by taking finite differences with sample rate $0.01$. To account for numerical error we allow for a small observational noise level of $\varepsilon =0.01$.  At the initial learning step $n=0$, we initialise the controller's adaptive element $\nu_{ad} = \predfn$ with a kinky inference predictor (cf. Def. \ref{def:KIL}). The KI learner is given the correct parameters $L=2,p=1$ and we set the upper and lower bound functions $\lbf$ and $\ubf$ to zero outside the arena $\statespace$. This folds in the knowledge about the state of affairs outside of the map. 
The agent aims to explore the state space in a manner suitable to decrease the maximal uncertainty $\maxerrn$ over time. Starting out with an estimated initial maximal uncertainty of $4.8$, the agent is only allowed to stop the exploration process when $\maxerrn < 0.5$. 
For simplicity, we let the agent adopt a heuristic strategy and define a setpoint at the location $\xi_n \in \statespace$ where the current uncertainty is highest. This can be determined by setting $\xi_n \in \arg\max_{x \in \statespace } \prederrn(x)$. This minimizer, as well as the pertaining maximum uncertainty $\maxerrn$, required for computing the stopping criterion of the exploration process, is found by optimising each component uncertainty function $\prederrn$. As we have noted before, Lem. \ref{lem:Hoeldarithmetic} allows us to obtain a H\"older constant and exponent for this function. This renders it amenable to the bounded optimisation approach discussed in Sec. \ref{sec:Hoelder_opt_basic_brief}. In our specific case, this is even easier, since the $\prederrn$ is even Lipschitz. Therefore, it can be optimised (and the optimum be bounded) using Shupert's algorithm \cite{Shubert:72}.  
Starting at position $S_1 = [1;1]$, the agent computes new setpoints with this optimisation procedure every $\tinc = 7$ seconds. The agent then observes a new drift sample, updates the data set, computes a new setpoint and starts over.  A simulation of the path taken by the agent is depicted in Fig. \ref{sec:agentexploration}. Notice how the controller becomes increasingly successful in reaching the waypoints  and in cancelling out the nonlinearity of the dynamics. An excerpt of the inferred beliefs over the drift at three different stages of the online learning process is depicted in Fig. \ref{fig:postbeliefsexplor}. It shows how a new training example is inserted at the point of maximum uncertainty (Fig. \ref{fig:kipredexpl1} vs Fig. \ref{fig:kipredexpl2}), decreasing the overall maximum uncertainty given by the floor and ceiling functions. The last plot (Fig. \ref{fig:kipredexplfin}) shows the inferred model over the drift at the end of the exploration process. 
\begin{rem}
We can see that the maximum uncertainty is mainly due to the belief over the first component $\predf_{n,1}$. This can be attributed to the fact that the maximum slope of the ground truth of this component function is $1$. Therefore, the assumed Lipschitz constant $L=2$ is a conservative choice for this function, which means the bounds are not as tight as possible. By contrast, for the second component function, this constant is tight. We can see this where the slope is steepest, few training examples are needed to shrink the uncertainty down to negligible amounts (that is, down to the level of observational noise). As a way out, it would have been possible to choose a separate constant for both component functions. For the first component function, $L_1=1$ would have been the best choice. 
\end{rem}

\subsubsection{Stability and safety bounds}
The attractive property of the bound of Eq. \ref{eq:errorboundgrowingconttimeKI} is that it holds for all times (not just in the limit) and that $K$ would not even have to be stable (i.e. Hurwitz). The clear disadvantage is that the bound grows with time and hence, does not provide a guarantee of stability of the state trajectory. 
To overcome this limitation, we will now provide a simple stability guarantee for the closed-loop trajectory of the kinky inference controlled plant. Since $F_n$ is bounded (due to the guaranteed conservatism of the KI rule), this is a situation where our learning guarantees can be combined with  standard results from robust control \cite{Kofman2007}. To this end, we remind the reader of the following fact:

\begin{lem}[\cite{Kofman2007}] \label{lem:kofman}
Consider the system $\dot x = A x + v$ where matrix $A$ is stable and has the Jordan canonical form 
$J = V^{-1} A V$. Suppose that $v(t) \leq \bar v, \forall t \in [0,T]$. Finally for a matrix $M$ and vector $x$ let $\abs{M}$ and $\abs{x}$ denote their respective component-wise moduli.
Then, we have:

 (I) $\abs{x(t)} \leq \abs{V} \abs{\text{Re}(J)^{-1}} \abs{V^{-1}} \, \bar v$, provided $\abs{V^{-1} x(0) \leq  \abs{\text{Re}(J)^{-1}} \abs{V^{-1}}}$.  

(II) Furthermore,  $\forall \epsilon >0 \exists \bar t \forall t \geq \bar t:  \abs{x(t)} \leq \abs V |\text{Re}(J)^{-1}| \, \abs{V^{-1}} \, \bar v + \abs V \epsilon $ (regardless of the initial condition). 
\end{lem}


\begin{figure*}
        \centering
				%\subfigure[Post. belief with three data points.]{
    %\includegraphics[scale =.33]{content/figures/driftpred1.pdf}
  %}
	\subfigure[KI predictions after 6 learning steps.]{\label{fig:kipredexpl1}
   \includegraphics[width = 5.3cm, clip, trim = 1cm 9cm 1cm 10cm]{content/figures/driftpred41.pdf}
  }
	\subfigure[KI predictions after one additional learning step.]{\label{fig:kipredexpl2}
    \includegraphics[width = 5.3cm, clip, trim = 1cm 9cm 1cm 10cm]{content/figures/driftpred51.pdf}
  }
	\subfigure[Final prediction.]{\label{fig:kipredexplfin}
   \includegraphics[width = 5.3cm, clip, trim = 1cm 9cm 1cm 9cm]{content/figures/driftpred111.pdf}
  }         %add desired spacing between images, e. g. ~, \quad, \qquad etc. 
          %(or a blank line to force the subfigure onto a new line)
       \caption{Excerpt of the evolution of the posterior beliefs during the exploration phase. The agent starts out with a kinky inference learner that has initial knowledge of the fact that velocity outside the arena $\statespace$ is zero. The agent utilises the uncertainty bounds (floor and ceiling function) to guide exploration. That is, it puts a new setpoint at the position of the maximum uncertainty. The agent 
			stops exploring after the maximal uncertainty threshold $\maxerr$ is below  $0.5$. The top row shows the posteriors over the first output component of the learned drift vector field. The bottom row depicts the posterior beliefs over the second output dimension of the drift vector field. Plots Fig. \ref{fig:kipredexpl1} and Fig. \ref{fig:kipredexpl2} show how the exploration heuristic manages (after some learning) to explore the parts of state space with high uncertainty.} 
       \label{fig:postbeliefsexplor}
\end{figure*}	 

 


%Before proceeding, we remind ourselves of the following well-known facts (adapted from \cite{Haddad2008} ):
%
%
%\begin{thm} [Barbashin-Krasovskii-LaSalle invariance theorem]
%Let $\dot x = f(x(t))$, $x(t_0) = x_0, t \geq t_0$ be a dynamic system where $f$ is differentiable.
%Assume $I \subset \statespace$ is a positively invariant set (that is: $x(t) \in I$ implies $x(t') \in I, \forall t' \geq t$). Assume there exists a continuously differentiable function $V:I \to \Real$ such that $\dot V(x) =(\nabla_x V)(x)  f(x) \leq 0, \forall x \in I$. Let $Z:= \{ x \in I \, | \, (\nabla_x V)  (x)  f(x) =0 \}$ and $M \subset Z$ denote the largest invariant set contained in $Z$.
%We have: If $x(0) \in I $ then $x(t) \stackrel{t \to \infty}{\longrightarrow} M \subset Z$.
%\end{thm}
%
%For our purposes, the point of the theorem is that via construction of a \textit{Lyapunov function} $V$, one can establish stability bounds on the state trajectory, without the need to solve the integral curve. 
%
%Invoking a generalisation \cite{Bhat2009} of La Salle's invariance principle\cite{lasalle1960}, we can provide the following stability guarantee:
%
%\begin{ques}
%\jcom{Does the following argument go through for time-varying reference?}
%\end{ques}

Harnessed with our Thm. \ref{thm:KIdesiderata} about the KI learner, we can immediately apply the lemma to yield the following simple stability guarantee:
\begin{thm}\label{thm:KIvelocagstab}
Assume we are given a sample $\data=\Bigl\{\bigl(x_j, f(x_j), \varepsilon(x_j) \bigr) \,|\, j=1,...,N\Bigr\}$ of uncertain drift $f \in \Kprior$ where $\Kprior$ is defined as in Sec. \ref{sec:KI_core}. For each output dimension $i$ we train a kinky inference learner on the data yielding predictors $\predf_{n,i}$ with error function $\prederr_{n,i}$ (as per Def. \ref{def:KIL}) for components $i=1,...,d$. Define $\maxerr_i := \sup_{ x \in \statespace \subset \Real^d} \prederr_i(x)$ to be the maximum prediction error in any dimension on the state space. 
Desiring to stabilise setpoint $\xi$, we apply the control $u:= g^{-1}(x) ( -K e - \predf + \dxref)$. This causes the plant to follow trajectory $x(t) = \xref(t) + e(t)$ where $\xref = \xi$.
We have:
\begin{enumerate}
	\item  For dimensions $(i=1,...,d)$, define the interval $S_i:= [- \frac{\maxerr_i}{w_i}, \frac{\maxerr_i}{w_i}]$. 
 $S=S_1 \times \ldots \times S_d$ is an invariant set for the error dynamics. That is, $e(t) \in S $ implies $e(t') \in S, \forall t'\geq t$.
	\item For any initial error $e(0)$, $e(t)$ converges to the largest invariant set in $S$.
\end{enumerate}

\end{thm}
\begin{proof}
One approach of showing the result would be to construct a piece-wise Lyapunov type function that is zero on $S$ and assumes values proportional to the distance of the error to the set $S$ otherwise. We can then apply one of the more modern versions of La Salle's invariance theorem \cite{Bhat2009,Haddad2008} to conclude the statement.
However, the statement also follows directly from Lem. \ref{lem:kofman}. To see this, we choose $K =A$, $F_n(x(t)) = v(t)$ where $A$ and $v$ are as defined in the lemma. 


By assumption, $K$ is stable. Since in our simple case, $K$ is diagonal, $J = K$ and $V = I_d$ is the identity matrix. Hence, $\abs{V}=\abs{V^{-1}} =I_d$. Because of the diagonal form of $K$, we have the simple situation of no component interactions. Hence, for each component $i \in \{1,...,d\}$, we have 
$\abs{e_i(t)} \leq \abs{V_{ii}} \abs{M_{ii}^{-1}} \abs{V_{ii}^{-1}} \maxerr_i= \frac{1}{w_i} \maxerr_i$ where we also have utilised $F_{n,i}(x) \leq \maxerr_{n,i}$ which holds by Thm. \ref{thm:KIdesiderata}.
This shows that $S$ is invariant.
The second statement about convergence to $S$ now follows directly from Lemma \ref{lem:kofman} (II).
%
%
%=========== Old proof ==========================
%We show the stability result for each component $i$ in isolation. So, let $i \in \{1,...,d\}$. 
%Define the function $V_i(e_i) = \begin{cases} \text{dist}(e_i,S)^2 & e_i \notin S\\ 0 & e_i \in S. \end{cases}$
%Furthermore, $\dot V_i(e_i) = 2 e_i \dot e_i = 2 e_i \, (F - w e_i)$.
%
%(i) Obviously, $V_i$ is pos. semi-definite. 
%
%(ii) We show $\dot V_i(e_i) \leq 0, \forall e_i$:
%
%
%Two cases: a) $e_i > \frac{\maxerr_i}{w_i} \geq 0$: Since $w_i \geq 0$ this implies $ \maxerr_i - w_i e_i \leq 0$. Since $F \leq \maxerr_i$, we also have $F - w_i e_i \leq 0$. Hence, $\dot V_i(e_i) =  2 e_i (F - w_i e_i) \leq 2 e_i (\maxerr_i - w_i e_i)\leq 0$.
%
%b) Showing $\dot V_i(e_i) \leq 0$ for  $e_i < - \frac{\maxerr_i}{w_i} \leq 0$ is completely analogous.
%In conclusion, we have established $\dot V_i(x) \leq 0, \forall x$.
%
%(iii) Define  $\Omega_i(e_i(0)) = [-r_i,r_i]$ where $r_i = \max\{ \abs{e_i(0)},\frac{\maxerr_i}{w_i}\}$. That is, $\Omega_i(e_i(0)) $ is the smallest ball around $0$ that contains both $e_i(0)$ and $S$. By convexity of $V_i$, $V(r_i) \geq V_i(x), \forall x \in \Omega_i$  and $\Omega_i(e_i(0))$ is an invariant set (which also follows from Thm. 7.1 in \cite{Bhat2009}). 
%Owing to (i) - (iii), we can apply La Salle's invariance principle \cite{lasalle1960} in the form given by \cite{astroembook2008} (or again Thm. 7.1 in \cite{Bhat2009}) to conclude that $\text{dist}(e_i(t), S_i) = \inf\{ \abs{e_i(t) - s } : s \in S_i \} \to 0 \, (t \to \infty)$.
%
%In summary, we have shown that $e_i(t) \in \Omega_i$ and $e_i(t) \to S_i$.
%%In particular, $e(t) \in \tube= \Omega_1(e(0)) \times \ldots \Omega_d(e(0))$ and 
\end{proof} 


 \begin{figure}
        \centering
							%\subfigure[Uncoordinated plans (prior learning).]{
    %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4.5cm 9cm]{content/figures/rsstalkfigs/maspriorlearn3d.pdf}
  %}\label{fig:preplans_uncoord3d}
	%\subfigure[Coordinated plans (prior learning).]{
   %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4.5cm 9cm]{content/figures/rsstalkfigs/maspriorlearn3d_coord.pdf}
  %} \label{fig:preplans_coord3d}
	%\subfigure[Uncoordinated plans  (after learning).]{
    %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4.5cm 9cm]{content/figures/rsstalkfigs/maspostlearn3d_uncoord.pdf}
  %}\label{fig:postplans_uncoord3d} 
	%\subfigure[Coord. plans (after learning).]{
   %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4.5cm 9cm]{content/figures/rsstalkfigs/maspostlearn3d_coord.pdf}
  %} \label{fig:postplans_coord3d}       
				\subfigure[Uncoordinated plans (prior learning).]{\label{fig:preplans_uncoord}
    \includegraphics[width = 3.9cm]{content/figures/prelearninit.pdf}
  }
	\subfigure[Coordinated plans (prior learning).]{\label{fig:preplans_coord}
   \includegraphics[width = 3.9cm]
	{content/figures/coordcoordviaK.pdf}
  } 
	\subfigure[Uncoordinated plans  (after learning).]{\label{fig:postplans_uncoord} 
    \includegraphics[width = 4.0cm]{content/figures/postlearninit.pdf}
  }
	\subfigure[Coord. plans (after learning).]{\label{fig:postplans_coord}  
   \includegraphics[width = 4.0cm]{content/figures/coordcoord_learned.pdf}
  }      
       \caption{The grey boxes represent the agents' safety regions (invariant sets plus a margin taking into account the agent radius of 0.1) for various choices of maximal uncertainties $\maxerr_i$ and feedback gains $w_i$ for dimensions $i \in \{1,2\}$. Fig. \ref{fig:preplans_uncoord}: $w_i=2, \maxerr_i = 4.8$. Fig. \ref{fig:preplans_coord}: $w_i=5.3, \maxerr_i = 4.8$. Fig. \ref{fig:postplans_uncoord}: $w_i=2, \maxerr_i = 0.5$. Fig. \ref{fig:postplans_uncoord}: $w_i=0.55, \maxerr_i = 0.5.$}
\label{fig:coordlearningagentsplansKIvel}
\end{figure}	  

 
The theorem tells us something interesting about the connection between learning success (measured by the $\maxerr_i$) and the magnitude of the feedback gain. That is, in order to stabilise the system up to a desired error bound, we can either increase the gain or reduce the uncertainty by learning. To illustrate this point, assume we have two agents $1$ and $2$ tasked to stabilise their plants at setpoints $S1=[4;5]$ and $S2=[6;5]$, respectively. Having a diameter of $0.2$, and being immersed in an uncertain drift field as considered in the exploration scenario above, the agents desire to find a ``plan'' of how to set their feedback gains such that it is guaranteed that they stabilise their setpoints (up to a certain error) while being guaranteed to avoid a collision with the other agent. Thm. \ref{thm:KIvelocagstab} helps us to achieve this.  That is, the agents can ``coordinate'' their plans gains such that their invariant sets do not overlap and are sufficiently small. 
Consider Fig. \ref{fig:coordlearningagentsplansKIvel}. 
Fig. \ref{fig:preplans_uncoord} depicts a situation the agents would encounter if they were initialised with the configuration the agent in our exploration scenario had prior to learning. That is, their uncertainties were $4.8$ and the feedback gain was set to a diagonal matrix with diagonal entries $w_i =2$. As the figure shows, the safety regions (invariant sets, plus some margin representing the agents' diameter) overlap and hence, a collision cannot be ruled out. As one way out, we can employ Thm. \ref{thm:KIvelocagstab} to adjust the gain such that the regions will be disjoint (Fig. \ref{fig:preplans_coord}). 

In order to improve control success without having to resort to higher feedback gain, the agent can alternatively attempt to bring down the uncertainty by learning. That is, we can incorporate the learning experience gained during the agent exploration phase (see above) to bring down the prediction uncertainties $\maxerr_i$ in each dimension, while leaving the gains unaltered (Fig. \ref{fig:postplans_uncoord}).
As we can see from the plots, the reduced uncertainties ensure that the safety regions are disjoint, without further need to increase the gain.
If all we were interested in was collision avoidance (or if we wanted to save control energy), we now could decrease the gains $w_i$ as much as possible without making the safety regions overlap again (Fig. \ref{fig:postplans_coord}). Once, again Thm. \ref{thm:KIvelocagstab} tells us how to set the gains accordingly. 


Note that so far, we have assumed that the agents are homogenous and have not taken (differing) notions of cost into account. For instance, an agent who experiences a lower loss when expending control energy might be assigned a higher gain than one with a lower notion of control cost. Automating such coordination methods in continuous time is the subject of Ch. \ref{ch:contcoll}. Our bounds for the kinky inference controllers could be combined with the coordination methods developed therein. This would yield a method for autmated coordination with guaranteed continuous time-collision avoidance of the learning agents.
%\subsection{A simple agent exploration scenario}%\label{sec:agentexploration}





  %
%\subsection{Multi-agent collision avoidance taking epistemic uncertainty into account}
  %
%\begin{figure*} 
        %\centering
							%\subfigure[Uncoordinated plans (prior learning).]{
    %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/preplans3d2ag_uncoord.pdf}
  %}\label{fig:preplans_uncoord3d}
	%\subfigure[Coordinated plans (prior learning).]{
   %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/preplans3d2ag_coord.pdf}
  %} \label{fig:preplans_coord3d}
	%\subfigure[Uncoordinated plans  (after learning).]{
    %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/postplans3d2ag_uncoord.pdf}
  %}\label{fig:postplans_uncoord3d} 
	%\subfigure[Coord. plans (after learning).]{
   %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/postplans3d2ag_coord.pdf}
  %} \label{fig:postplans_coord3d}       
				%\subfigure[Uncoordinated plans (prior learning).]{
    %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/preplans2d2ag_uncoord.pdf}
  %}\label{fig:preplans_uncoord}
	%\subfigure[Coordinated plans (prior learning).]{
   %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/preplans2d2ag_coord.pdf}
  %} \label{fig:preplans_coord}
	%\subfigure[Uncoordinated plans  (after learning).]{
    %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/postplans2d2ag_uncoord.pdf}
  %}\label{fig:postplans_uncoord} 
	%\subfigure[Coord. plans (after learning).]{
   %\includegraphics[width = 3.9cm, clip, trim = 3.5cm 9cm 4cm 9cm]{content/figures/postplans2d2ag_coord.pdf}
  %} \label{fig:postplans_coord}       
       %\caption{Multi-agent collision avoidance before and after learning. Top row: Draws from the Ito hulls of the agents' uncertain trajectories. Bottom row: Paths with 50\% error ellipses drawn at regular time intervals. 
			%Before the map is explored, the agents' uncertainties are so large that Agent 2 (blue agent) does not reach his goal location (5,9) without incurring a collision with subjective probability $< 0.05$. Therefore, collision avoidance causes him to wait until Agent 1 has completely passed by to her goal location (10,5) and causes Agent 1 to miss his destination.  }
			%\label{fig:coordlearningagentsplans}
%\end{figure*}	     
           




\input{content/ch_kinkyinf/KIMRAC_wingrock.tex}

\subsection{Boundedness in discrete-time systems}
\label{sec:KIMRACstabbounds}

In the previous subsection, we gave an illustration KI-MRAC -- a combination of a feedback-linearising controller with our KI learning method. The results are encouraging -- our adaptive control law managed to learn a dynamic system online and to track a reference in the presence of wingrock dynamics where other state of the art methods failed. 

However, KI-MRAC is an online learning approach and assumed the training corpus could be updated with the entire history of past observations. This might work for short time horizons. Unfortunately, such assumptions are often unrealistic. Despite being a fast nonparametric method, eventually the size of the training corpus will grow to an extent where the required prediction response time exceeds the desired control refresh frequency. 
%\jcom{Should explain these notions in background section}

Furthermore, the controller in KI-MRAC did not take the uncertainty into account when making decisions on the control action. 


In this section, we assume that predictions are made on the basis of a fixed offline training corpus.
This means that the uncertainty will always be bounded from below. 
For this setting, we are interested in the following questions:
\begin{enumerate}
\item 
Given a linearising adaptive control law in GP-MRAC in offline learning mode, can we quantify a bound on the error dynamics ? That is, folding in the prediction bounds of our KI learner, how do we construct a robust tube around the nominal trajectory that is guaranteed to contain the real trajectory? 
\item 
How can we utilise the tubes for collision avoidance in a multi-agent setting?
\end{enumerate}
The second question will be addressed in Sec. \ref{sec:KIcollavoiddiscretetime} in the context of predictive (open-loop) control. In this section, we will lay some of the ground work and address the first question.
However, this is a question that is also of relevance for collision avoidance since it can be harnessed to bound the trajectory within a safety region or tube. The latter can be converted into collision avoidance constraints or a criterion function (cf.  Ch. \ref{ch:contcoll}, Ch. \ref{ch:discrcoll} as well as references in Sec. \ref{sec:optMPC}).
 %Our exposition will focus on discrete-time systems.




%\section{Boundedness of the discrete-time closed-loop dynamics of an agent utilising Kinky inference learning to identity a H\"older continuous drift vector field}
%\subsubsection{Discrete-time dynamics}
The exposition in this section will focus on KI-MRAC in discrete-time. Here, we assume the dynamics are given as first-order Euler approximations of the second-order control-affine dynamics of Sec. \ref{sec:KIMRAC}.
This means that the error dynamics as per Eq. \ref{eq:errordynmrac} translate to the recurrence relation:
\begin{equation}\label{eq:errordynmrac_KIMRACdiscrete}
	e_{k+1}  = M e_k + \tinc F_k
\end{equation}


where $\tinc \in \Real_+$ is a positive time increment,  $k$ is the time step index. Furthermore,

\begin{equation}
	F_k: = F_k(x) =F_n(x) = f(x) - \predf(x) = B \bigl(\nu_{ad}(x_k) -  \tilde a(x_k)\bigr) 
\end{equation}
is an uncertain increment due to the model error of the learner (cf. Sec. \ref{sec:firstorderctrlandKI} or Eq. \ref{eq:errordynmrac}), 						$B = \left(\begin{array}[h]{c}
				O_m \\ \tinc I_m
						\end{array}\right)$ and 
%\begin{equation}
	%M_k = \left(\begin{array}[h]{cc}
				%I_m &  \, O_{m}\\
				%-\tinc K_1(k) & I_m- \tinc K_2(k) 
						%\end{array}\right) 
%\end{equation}
\begin{equation}
	M = \left(\begin{array}[h]{cc}
				I_m &  \, \tinc I_{m}\\
				-\tinc K_1 & I_m- \tinc K_2 
						\end{array}\right) 
\end{equation}
					is the (error state) transition matrix. 
					%
					%Note, in contrast to Sec. \ref{sec:KIMRAC} we allow for time-varying feedback gains $K_i(k) \,\, (i =1,2)$. 
					
This is completely consistent with the uncertain recurrence considered in Eq. \ref{eq:dynextstatediscrete1}, with the exception, that the uncertainty of increment $F_k$ is not probabilistic but interval-bounded due to Thm. \ref{thm:KIdesiderata}. Employing the same type of argument as in Lem. \ref{lem:origprocdiscrfacts} we see that the solution of the recurrence is given by:
%\begin{equation}
	%\vc e_k = M_{k-1} \vc e_{k-1} + \tinc \vc F_{k-1} = \ldots = P_{k-1,0} \, \vc e_0 + \tinc \sum_{i=0}^{k-1}  P_{k-1,i+1} \, \vc F_i		
%\end{equation}
\begin{equation}
	\vc e_k = M \vc e_{k-1} + \tinc \vc F_{k-1} = \ldots = M^k \, \vc e_0 + \tinc \sum_{i=0}^{k-1} M^{k-1-i} \, \vc F_i	.	
\end{equation}		 

%where as before, we define 
%
%\begin{equation}
	%P_{j,i}  =
	%\begin{cases}
	 %M_j \, M_{j-1} \, \ldots M_i&, i \leq j\\
	%I_d, &,i > j.
	%\end{cases}
%\end{equation}

We desire to bound the  norm of the error. To this end, we leverage that the norms are sub-additive and sub-multiplicative to deduce: 
%\begin{equation}
	%\norm{\vc e_k} \leq   \matnorm{P_{k-1,0}} \, \norm{\vc e_0} + \tinc \sum_{i=0}^{k-1}  \matnorm{P_{k-1,i+1}} \, \norm{\vc F_i}		
%\end{equation}
%
%where $\matnorm{\cdot}$ is a sub-multiplicative matrix norm pertaining to vector norm $\norm{\cdot}$. So, if $\norm{\cdot} = \norm{\cdot}_2$ is the Euclidean norm, then $\matnorm{\cdot}$ is the spectral norm.
%
%For the special case of constant $M:= M_k, \forall k$ we get:
\begin{equation}
	\norm{\vc e_k} \leq   \matnorm{M^{k}} \, \norm{\vc e_0} + \tinc \sum_{i=0}^{k-1}  \matnorm{M^{k-1-i}} \, \norm{\vc F_i}		\leq \matnorm{M^{k}} \, \norm{\vc e_0} + \tinc \maxerrn_k	 \sum_{i=0}^{k-1}  \matnorm{M^{k-1-i}}
\end{equation}
where $\maxerrn_k	= \max_{i=1,...,k-1} \norm{F_i}$.
As in Sec. \ref{sec:firstorderctrlandKI}, we assume there exists a maximum model error norm $\maxerrn$, i.e. $\forall i: F_i \leq \maxerrn$. 
For instance, if we construct the tube for collision avoidance within a confined part of state space (such as an arena), if we know the drift is periodic or bounded, we can set $\maxerrn = \sup_{x} \norm{F(x)}_{\infty}$. 
Then we have: \vspace{-1em}
\begin{equation}
	\norm{\vc e_k} \leq   \matnorm{M^{k}} \, \norm{\vc e_0} + \tinc \maxerrn \sum_{i=0}^{k-1}  \matnorm{M^{k-1-i}}.
\end{equation}

As shown in Sec. \ref{sec:critexpintbnddisturb}, the right hand side is convergent provided the gains $K_1, K_2$ are chosen such that $M$ is stable, i.e. $\specrad(M) <1$, and provided $\maxerrn_k$ is is bounded. 

Whether or not $M$ is stable, in low dimensions, the sums can be computed offline and in advance. This is of great benefit if 
 the controller that is building on the error bounds is utilising optimisation-based control with a finite time-horizon (for a related setup, see cf. Sec. \ref{sec:KIcollavoiddiscretetime}).   

To get a (conservative) closed-form bound on the error norms, Sec. \ref{sec:critexpintbnddisturb}
contains a derivation and discussion of the following result:

\begin{thm}\label{thm:normboundsboundeddisturbmainbody}
Let $(F_k)_{k \in \nat_0}$ be a norm-bounded sequence of vectors with $\maxerrn_k :=\max_{i \in \{0,\ldots,k-1\}} \norm{F_i} \leq \maxerrn \in \Real$. 
For sequence $(x_k)_{k \in \nat_0}$ defined by the linear recurrence 
	$x_{k+1}  = M x_k + \tinc F_k \,\,\,\, (k \in \nat_0)$, we can define the following bounds:
	
	\begin{enumerate}
	\item $\norm{\vc x_k} \leq \matnorm{M^{k}} \, \norm{\vc x_0} + \tinc \maxerrn_{k} \sum_{i=0}^{k-1}  \matnorm{M^{i}}$. If $\specrad(M) <1$ and $\exists \maxerrn$ $:\maxerrn\geq \maxerrn_k \geq 0, \forall k$, the right-hand side converges as $k \to \infty$.
	\item Let $k_0 \in \nat, k_0 >1$ such that $\matnorm{M^k} <1, \forall k \geq k_0$ and let $\varphi := \matnorm{M^{k_0}} <1$ and let $\delta_k := \floor{k/k_0}$. If $r:=\specrad(M) < 1$, for $k > k_0$,  we also have:
	\begin{align} \norm{\vc x_k} &\leq c \, \varphi^{\delta_k} \, \norm{\vc x_0} + \tinc \maxerrn_{k} \Bigl(\sum_{j=0}^{k_0-1} \matnorm{M^j} + c \, k_0 \frac{\varphi-\varphi^{ \floor{\frac{k}{k_0}}+1 }}{1-\varphi} \Bigr) \stackrel{k \to \infty}{\longrightarrow} \tinc \maxerrn_{k} \sum_{j=0}^{k_0-1} \matnorm{M^j} 
	+ \frac{\tinc \maxerrn_{k}\,  c\, k_0 \,\varphi}{1-\varphi} 
	\end{align}
	where possible choices for $c \in \Real$ are: 
(i) $c= \max\{\matnorm{M^i} | i=1,\ldots,k_0-1 \}$ 

or (ii) $c = \frac{1}{(d-1)!} \Bigl(\frac{1 - d}{\log r}\Bigr)^{d-1}	\matnorm{M}^{d-1}\, \, \, r^{\frac{1 - d}{\log r}-d+1}  $.
%
Since $\matnorm{M} \geq 1$, one can also choose (iii) $c:= \matnorm{M}^{k_0}$. %In this case, $\matnorm{M^k} \leq  \, \matnorm{M}^{k_0}^{(k \text{ div } k_0) +1} $.

\item If $\matnorm{M} < 1$, the following holds:
$\norm{\vc x_k} \leq \matnorm{M}^{k} \, \norm{\vc x_0} + \tinc \maxerrn_{k}   \frac{1-\matnorm{M}^k}{1-\matnorm{M}}. $
	\end{enumerate}
\begin{proof}
1) is due to Eq. \ref{eq:9jn44mm4}. 2) follows by Lem. \ref{lem:CMEbndnormofM2k2}  and  Lem. \ref{lem:alphaYtermbnds2}. 3) Is a direct application of the geometric sum formula in conjunction with the condition that $\matnorm{M}<1$ and that the matrix norm is sub-multiplicative. 3) is a consequence of the geometric sum formula (Lem. \ref{lem:geommatseries}). 
\end{proof}	
\end{thm}


In Ch. \ref{ch:critexp}, we derive a fast, conservative algorithm that can calculate a sequence of improving upper bounds on the ``critical matrix exponent'' $k_0$. This is of interest in cases where its naive computation is expensive (e.g. in high-dimensional systems). Furthermore, the chapter contains an illustration of how the error norm bounds decrease with decreasing spectral radius $\specrad(M)$.

Finally, Sec. \ref{sec:KIcollavoiddiscretetime} considers an application of a bound similar to 1) in Thm. \ref{thm:normboundsboundeddisturbmainbody} to the different setting where there is no feedback gain and where the reference control is determined via mixed-integer programming in the context of MPC with collision avoidance constraints. However, we point out that in such a setting, one could also use feedback control in combination with predictive control. For this situation, the bounds of Thm. \ref{thm:normboundsboundeddisturbmainbody} would be of immediate utility.


  

==> content2/Ch_kinkyinf/abstract.tex <==
%\begin{abstract}
%We propose a method for inductive inference that yields error bounds on the accuracy of the drawn conclusions. 
%The approach yields a nonparametric machine learning method with theoretical guarantees. We apply the method to system identification and control and show how the prediction bounds can be utilised in collision avoidance under uncertain dynamics. Here the constituent agents learn to update their dynamics models and take the rest uncertainty into account properly in order to compute plans that are guaranteed to avoid collisions.
%\end{abstract}
%\begin{abstract}
%An approach for inductive inference that yields error bounds on the accuracy of the drawn conclusions is considered. Generalising existing work spread across various communities under headlines such as \emph{Lipschitz Interpolation} or \emph{Nonlinear Set Interpolation (NSI)}, the approach can be understood as a nonparametric machine learning method with theoretical guarantees. In the basic setup, the method can learn any H\"older continuous function with given parameters. In this paper, it is shown how to adapt parameters to the data such that the resulting machine learning approach becomes a universal approximator in a strong sense. That is, the inference rule introduced can learn any continuous function on compact support up to an arbitrarily small error. The second part of the paper, applies the new inference rule to \emph{nonparametric model-reference adaptive control (MRAC)}. For discrete-time systems with uncertain drift stability of the resulting online learning-based controller (\emph{KI-MRAC}) is proven.
%Across a range of simulated aircraft roll-dynamics and performance metrics KI-MRAC outperforms recently proposed alternatives that were based on \emph{Gaussian processes} and \emph{RBF-neural networks}. 
%%We provide a proof of stability for our nonparametric adaptive controller. 
%\end{abstract}


\begin{abstract}
Techniques known as \emph{Nonlinear Set Membership} prediction, \emph{Lipschitz Interpolation} or \emph{Kinky Inference} are  approaches to machine learning that utilise \emph{presupposed} Lipschitz properties to compute inferences over unobserved function values. Provided a bound on the true best Lipschitz constant of the target function is known a priori they offer convergence guarantees as well as bounds around the predictions.
Considering a more general setting that builds on H\"older continuity relative to pseudo-metrics, we propose an online method for estimating the H\"older constant online from function value observations that possibly are corrupted by bounded observational errors. Utilising this to compute  adaptive parameters within a kinky inference rule gives rise to a nonparametric machine learning method, for which we establish strong \emph{universal approximation} guarantees. That is, we show that our prediction rule can learn any continuous function in the limit of increasingly dense data to within a worst-case error bound that depends on the level of observational uncertainty.
%To provide evidence that our method can be beneficial not only in theory but also in practice, 
We apply our method in the context of \emph{nonparametric model-reference adaptive control (MRAC)}. 
Across a range of simulated aircraft roll-dynamics and performance metrics our approach outperforms recently proposed alternatives that were based on \emph{Gaussian processes} and \emph{RBF-neural networks}. For discrete-time systems, we provide stability guarantees for our learning-based controllers both for the batch and the online learning setting. 
\end{abstract}

==> content2/Ch_kinkyinf/cons_est.tex <==


\section{Problem Definition}
\label{sec:prob_def}
In Ex. \ref{ex:topinf_quad}, we provided an example of a topological inference problem for conservative quadrature. Unfortunately, the proof of conservativeness of the trapezoid method relies upon existence and knowledge of second derivatives and is restricted to one-dimensional integrands. Many applications demand coarser knowledge and applicability to a less-restricted class of integrands. 

%As a basic example, consider the ordinary differential equation $\frac{\d x}{\d t} = (\xi - x)$ where $\xi: I \subset \Real \to \Real $ is an absolutely continuous function superimposed by a countable number of steps. Suppose, the ODE describes the trajectory $x: I \to \Real$ of a controlled particle in one-dimensional state space. Based on $N$ time-state observations $D_N=(t_1,x_1 ),..., (t_N,x_N )$ we desire to estimate the total distance travelled $S$ in time interval $I$, $S = \int_I x(t) \d t$. Solving



\textbf{Setting.}
Let $d \in \nat$ and $I=[a_1,b_1] \times \ldots \times [a_d,b_d] \subset \Real^d$ be a bounded hyperrectangle domain. Assume, we have access to a sample set $D_N:= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N \} $ containing $N \in \nat$ samples value $\tilde f_i$ of the target function $f: I \to \Real$ at sample input $s_i \in I$. The samples have interval-bounded error given by $\varepsilon : I \to \Real_{\geq 0}$. That is, all we know is that $f(s_i) \in [\underline f(s_i), \overline f(s_i) ]$ where $\underline f(s_i) := \tilde f_i - \varepsilon(s_i)$ and $\overline f(s_i) := \tilde f_i + \varepsilon(s_i)$.

The interpretation of the errors depends on the given application. For instance, in an experimental setting they could represent measurement errors. Most relevant to this work, the errors might represent approximation errors that arise if the target has to be approximated numerically.

Furthermore, for each sub-hyperrectangle $J \subset I$ we have access to a Lipschitz number $L_J \geq 0$. That is, $L_J$ is a number such that $\forall x,x' \in J: \abs{f(x) - f(x')} \leq L_J \, \norm{ x- x'}$ where $\norm \cdot$ is a fixed norm on $I$.\footnote{Note, due to norm-equivalence in finite-dimensional space, it is of no principal concern which norm is chosen.} \\


 Based on sample set $D_N$, we desire to design algorithms solving the following two
tasks:

\subsection{Task1 -- Computing a conservative \textit{function estimate}}
\label{sec:problemdef_task1}
Compute a function $B: D_N \mapsto (\decke_N,\boden_N)$ estimating the target that satisfies the following \textbf{desiderata}:
\begin{enumerate}
	\item \textit{Conservativeness}. $\decke_N, \boden_N :I \to \Real$ functions that enclose the target conservatively. That is, 
			we can guarantee  $\decke_N(x) \geq f(x) \geq \boden_N(x), \forall x \in I$. (We will refer to $\decke_N, \boden_N$ as (Lipschitz-) ceiling and floor, respectively. 
				\item \textit{Convergence} to the target. If $(D_N)_{N \in \nat }$ is a sample set sequence whose inputs converge to a dense subset of $I$ (as $N \to \infty$), we require $\exists \gamma, \phi \geq 0: \decke_N - f \stackrel{N \to \infty} \longrightarrow \gamma \leq \varepsilon, f- \boden_N \stackrel{N \to \infty} \longrightarrow \phi \leq \varepsilon$ pointwise. In the absence of errors ($\varepsilon \equiv 0$) this means uniform convergence to the target.
				\item \textit{Optimality}. We desire the enclosure to be optimal. That is, to $\decke_N, \boden_N$ should be as tight as possible, without losing conservativeness.
\end{enumerate}

From the perspective of topological inference, the estimator is a data inference method for function estimation:
$B(\cdot) = M_{dinf}(\mathcal K_{prior}, \cdot, \gamma ) $ (for some sufficiently large $\gamma$) mapping sample data into a hypothesis interval of possible functions. 
Here,  our a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L_J$ such that the underlying target $f \in \mathcal F$ is $L_J-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L_J \norm{x-x'}\}$. 
Note, we will not explicitly compute the prior knowledge set. Instead will will fold in the Lipschitzness to define an optimal estimator output defining an enclosure that coincides with $\mathcal K_{post} \subset \mathcal K_{prior}$ and hence, with $T (\mathcal K_{post} \cup \mathcal K_{prior})$. Therefore, the resulting inference mechanism will be optimal. 

Note, how our desiderata are equivalent to the corresponding notions of the inference mechanism that is to be designed.

\subsection{Task2 -- Estimating definite integrals.}
	\label{sec:problemdef_task2}
 Compute an \textit{integral estimator} $E: D_N \mapsto (\underline S_N, \overline S_N)$ of the definite integral $S := \int_I f(x) \, \d x$. The estimator's outputs translate to an estimate $\hat S_N = \frac{\underline S_N+ \overline S_N}{2}$ of $S$ with error $\mathfrak E(D_N) =\overline S_N - \hat S_N = \frac{1}{2} \abs{\overline S_N - \underline S_N}$. Similarly to before, we desire our estimator to exhibit the following properties:
\begin{enumerate}
			\item \textit{Conservativeness}.  Regardless of $D_N$, we can guarantee $\overline S_N \geq S \geq \underline S_N$. 
			
			\item \textit{Convergence} to the ground truth. If $(D_N)_{N \in \nat }$ is a sample set sequence whose inputs converge to a dense subset of $I$ (as $N \to \infty$) and $\varepsilon$ is integrable, we require $\abs{\overline S_N - \underline S_N} \stackrel{N \to \infty} \longrightarrow \int_I  \overline \varepsilon(x) \d x$ where $\overline \varepsilon$ is the smallest upper bound function on $\varepsilon$ that is integrable. In the absence of errors ($\varepsilon \equiv 0$) this implies convergence of estimate $\hat S_N$ to the true integral $S$.
			\item \textit{Optimality}. Finally, we desire the bounds to be optimal, that is, to be as tight as possible, without losing conservativeness.
\end{enumerate}

Viewed from the perspective of our topological inference frame-work, the estimator is a data inference method for quadrature:
$E(\cdot) = M_{dinf}(\mathcal K_{prior}, \cdot, \gamma ) $ (for some sufficiently large $\gamma$) mapping sample data into a hypothesis interval of possible functions. 
Here,  our a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L_J$ such that the underlying target $f \in \mathcal F$ is $L_J-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L_J \norm{x-x'}\}$. 
Note, we will not explicitly compute the prior knowledge set. Instead will will fold in the Lipschitzness to define an optimal estimator output defining an enclosure that coincides with $ T (\mathcal K_{post} \cup \mathcal K_{prior})$ and thus, is optimal.

As for Task1, our desiderata are equivalent to the corresponding notions of the inference mechanism that is to be designed.



==> content2/Ch_kinkyinf/constantadaptation.tex <==

\subsection{An incremental lazy update rule for the H\"older constant}
\label{sec:lazyconstants}
Above our theoretical guarantees are based on the assumption that the parameters $L(n)$ were set to a fixed H\"older constant of the target function. In other words, if we know a H\"older constant $L^*$ of the ground truth $f$ then setting $L(n)=L^*,\forall n$ ensures the desired conservatism and convergence properties of the KI rule. However, in a black-box learning setting, a H\"older constant may not be know a priori. Therefore, the estimation of Lipschitz constants on the basis of a sample is a problem that has been considered by several authors in the past \cite{Wood1996,Beliakov2006}. For instance, Wood and Zhang \cite{Wood1996} reduced the problem of estimating a global Lipschitz constant of a one-dimensional function to fitting a Weibull distribution to random absolute slope estimates between uniformly sampled inputs. Unfortunately, their results are restricted to one-dimensional functions that satisfy the Gnedenko condition and where one has access to a batch of samples drawn i.i.d. uniformly at random and no observational errors. Beliakov \cite{Beliakov2006} used a simple empirical estimator of a Lipschitz constant that did not require distributional assumptions and can be seen as a simple special case of our proposed lazy method. In contrast to his estimator, our approach is designed to receive data incrementally and makes provisions for observational noise in the sample. We do not make any distributional assumptions about the noise or any assumptions about the target other than that it is 
a continuous function from a pseudo-metric space into an additive group endowed with a translation-invariant metric. 
  


%
%\subsection{A Bayesian treatment of probabilistically uncertain H\"older constants}
%\label{sec:bayesupdatelipconst}
%Throughout the previous section we have assumed that the H\"older constants were known to us. 
%However, in many cases, we may be uncertain about the best H\"older constant. We assume the uncertainty is expressed as a distribution. Following the Bayesian point of view, we interpret probability densities over events as subjective degrees of beliefs that these events hold true. 
%In the following subsection, we describe how to utilize the densities over the best H\"older constant $L^* \in \Real_+$ to yield a (once again, conservative) bound on the probability of our functions estimates and integrands not being conservative. After that, we will address the question of how to update our beliefs over $L^*$ in the light of new function evaluations in a Bayesian manner.
%
%For simplicity, we will assume there are no observational errors and that there are no a priori bounds. That is, $\obserr_i = 0, \, \forall i$ and $\lbf = -\infty, \ubf = \infty$. Furthermore, we tacitly assume the H\"older exponent $p$ is known and fixed.
%
%Let $\pi: \Real_+ \to \Real_+$ be a density encoding our belief over best H\"older constant $L^*$ of target function $f$.
%In the absence of bounds and observational error, we define the H\"older enclosure $\einschluss (\ell) =\{ \phi \,| \, \phi(x) \in \prederrbox_n(x)\}$  where $\prederrbox_n$ is the uncertainty hyperrectangle defined above (see Eq. \ref{eq:prederrint}), computed on the basis of H\"older constant $L=\ell$.
%Assume we construct a H\"older enclosure $\einschluss (\ell)$ based on choosing $\ell \in \Real_+$ as a H\"older constant.  How large do we need to choose $\ell$ to guarantee that $f$ is completely contained in the enclosure? Since we are uncertain about the true H\"older constant, this question can only be framed probabilistically. That is, for a given certainty threshold  $\theta \in (0,1)$ we desire to find $\ell > 0$ such that 
%\[ \theta \leq \Pr[ f \in \einschluss (\ell) ]. \]  
%
%\begin{thm} \label{thm:ksjhdkjs} Let $\decke_n,\boden_n$ be a valid ceiling and floor function, respectively.
%Let $P: t \mapsto \int_{x \leq t} \pi(x) \,\d x $ our density's cumulative distribution function (cdf).
%We have, \[P(\ell) \geq \theta \Rightarrow \theta \leq \Pr[ f \in \einschluss (\ell) ].  \] 
%\begin{proof} 
%Let $L^*$ denote the best H\"older constant of function $f$.
%
% $\forall \ell \geq L \geq 0 :   \Pr[ f \in \einschluss (\ell) | L^*=L] = 1$. 
%Hence,
%$
%\Pr\bigl[ f \in \einschluss (\ell) \bigr] 
%= \int_0^\ell \Pr\bigl[ f \in \einschluss (\ell) | L^*=L\bigr] \,\d P(L) 
% + \int_\ell^\infty \Pr\bigl[ f \in \einschluss (\ell) | L^*=L\bigr] \,\d P(L) 
%=  \int_0^\ell \,\d P(L) + \int_\ell^\infty \Pr\bigl[ f \in \einschluss (\ell) | L^*=L\bigr] \,\d P(L)  
%\geq \int_0^\ell \,\d P(L) 
%= P(\ell).$
%\end{proof}
%\end{thm}
%
%That is to say, in order to guarantee conservativeness of our enclosure, all we need to do is to compute it on the basis of 
%a fixed H\"older constant that is just large enough such that $P(\ell) = \int_0^l \pi(L) \,dL \geq \theta$. Notice, if the integral cannot easily be determined in closed-form, but a H\"older constant for density $\pi$ is known, we can employ our H\"older quadrature method described previously (based on a known constant), to evaluate $P(\ell)$ conservatively by finding a lower bound on it. \\
%
%
%%When it comes to the task of quadrature, in the presence of an uncertain H\"older constant, the error bounds of the integral estimates afforded by our method also are valid to a level of probabilistic belief. 
%%
%%Combining Thm. \ref{thm:ksjhdkjs} with our boundedness results for conservative quadrature of Sec. \ref{sec:quadr} immediately yields the following result:
%%\begin{cor}
%%Let $S := \int_I f(t) \, \d t$. 
%%With the definitions introduced above, we have  \[P(\ell) \geq \theta \Rightarrow \theta \leq \Pr\Bigl[ \hat S^\decke_N \geq S \geq \hat S^\boden_N  \Bigr]  \] 
%%where $\hat S^\decke_N , \hat S^\boden_N $ are computed assuming a H\"older constant of $\ell$. 
%%
%%\end{cor}
%%
%%The Corollary asserts that if we check that $P(\ell) \geq \theta$ for some desired threshold $\theta$ then our probabilistic belief in the integral $S$ being within the interval $[S_n^\boden,S_n^\decke]$ also is at least $\theta$.
%
%\subsubsection{A Bayesian update rule}
% Define $\metric_{\outspace}(f_1,f_2) = \abs{f_1-f_2}$ and let $\metric_{\inspace}(x,y)$ be some input space (pseudo-) metric as before. 
%
%%That is a H\"older constant $L$ with respect to the canonical metric $(x,y) \mapsto \norm{x-y}$ is a Lipschitz constant w.r.t $\metric_\inspace$. We will refer to $L$ uniformly as \textit{H\"older} constant.
%
%
%Assume we hold a prior belief over the best H\"older constant $L^*$ encoded as a density $\pi_0 : I \subset \Real_+ \to [0,1]$.
%Assume we are given a sample $D = \{(s_i,f_i)\}_{i=1,...,N}$ of input-function value pairs, $x_i \in \mathcal X$, $f_i = f(s_i) \in \outspace, \forall i$, the question arises of to calculate a posterior in the light of the new data. 
%
%Since we assume $f :\mathcal X \to \mathcal Y \subseteq \Real$ is H\"older we have $ \frac{\metric_\outspace(f_i,f_j)}{\metric_{\inspace}(s_i,s_j)} \leq L^*,  (i,j =1,...,N, x_i \neq x_j)$ where $L^*$ is the best H\"older constant of $f$. So, our observations allow us to infer that the \emph{empirical H\"older constant} 
%\begin{equation}
%	L_D := \max_{i,j,i\neq j} \frac{\metric_\outspace(f_i,f_j)}{\metric^p_{\inspace}(s_i,s_j)}
%	\label{eq:LD}
%\end{equation}
%is a lower bound on the best H\"older constant.\footnote{In the context of a special Lipschitz interpolation rule, Beliakov \cite{Beliakov2006} considered this quantity as an estimate of the Lipschitz constant.} Note, the computation of an update of this quantity can be done with computational effort linear in the number of pre-existing quantities. 
%That is, assuming a pre-existing data set $D$ and that we make an additional observation $s_{N+1},f_{N+1}$ which is incorporated into the updated data set $D' = D \cup \{(s_{N+1},f_{N+1})\}$. Instead of computing $L_{D'}$ from scratch as per Eq. \ref{eq:LD}, we can leverage:
%
%\begin{equation}
%	L_{D'}=\max \{L_D,L'\}, \,\text{ where } L' := \max_{i=1,\ldots,N} \frac{\metric_\outspace(f_{N+1},f_i)}{\metric^p_{\inspace}(s_{N+1},s_i)} 
%	\label{eq:LDupdate}
%\end{equation}
%
%which can be computed in $\mathcal O(d N)$ where as before, $d = \dim \inspace$.
%The remaining question is how to derive a posterior over $L^*$ based on this newly observed lower bound. 
%%
%%\begin{ques}
%%How can we prove that there is no information about the H\"older constant in the data other than $L_D$? That is, in particular, that \[p(L^*|D) \stackrel{!}{=}p(L^* |L_D) ??\]
%%\end{ques}
%%
%%
%%We will discuss two approaches, the Minimum-Relative-Entropy approach and Bayesian inference.
%%
%
%
%%\subsubsection{Bayesian approach}
%
%By Bayes theorem, we can write 
%\[\pi(L|L_{D'}) = \frac{\pi(L_{D'}|L) \, \pi_0(L) }{ \int_I \pi(L_{D'}|L) \, \pi_0(L) \, \d L}.\]
%
%If we are uncertain about which empirical H\"older constant we observe given the real H\"older constant  $L^* = L$ we set the Likelihood function 
%\[ \pi(L_{D'}|L) = \begin{cases} 0, L_{D'} > L\\ \frac{1}{L}, \text{otherwise}. \end{cases}.\]
%
%Of course, if the definite integrals of prior $\pi_0$ are not known in closed form, we need to approximate numerically. Depending on knowledge of smoothness properties we can either employ standard methods such as Gaussian quadrature or, if necessary, utilise our H\"older quadrature methods to that effect.
%%\begin{ques}[@Mike]
%%What is the likelihood function $p(L_D|L)= ... ?$
%%\end{ques}
%
%%\subsubsection{Minimum-Relative-Entropy Approach} 
%%
%%Computing posteriors from priors subject to constraints is the focus of max-ent inference. 
%%
%%Remember, 
%%\begin{defn}[Relative Entropy] For two densities $p,q: I  \to [0,1]$ the \textit{relative entropy} or \textit{Kullback-Leibler divergence} is defined as 
%%\[\KLD {p}{q} = \int_{I} p(x) \log \frac{p(x)}{q(x)} d\mu(x)\] where $\mu$ is a measure appropriate for domain $I$.
%%\end{defn}
%%
%%For example, if $I \subset \Real$ then $\mu$ is normally tacitly assumed to be the standard Lebesgue measure. If $I$ is a discrete set, $\mu$ is noramlly assumed to be the counting measure. In this case \[\KLD {p}{q} = \sum_{x\in I} p(x) \log_2 \frac{p(x)}{q(x)}. \]
%%
%%For our problem, we can pose the desired posterior density as the solution to the variational problem:
%%
%%\begin{align}
%%\argmin_p & \KLD {p}{p_0}\\
%%\text{s.t.:}&\\
%%& p(l) \in [0,1], \forall l \geq 0\\
%%&\SP{p}{e}_{L_2(\Real)} =1\\
%%& \SP{p}{\chi_{[0,L_D]}}_{L_2(\Real)} =0
%%\end{align}
%%
%%where $e: t \mapsto 1$ is the constant mapping to $1$ and $\chi_{[0,L_D]}$ is the indicator function for interval $[0,L_D]$.
%%
%%\begin{ques}
%%Can we solve this variational problem in closed form? How can we solve them numerically. If we have no clue, we can make everything discrete as follows...
%%\end{ques}
%%
%%\emph{Discretization}.
%%For practical purposes, it will be convenient to reduce the problem to a standard convex optimization problem as follows:
%%Let $J_1,...,J_m \subset I$ be a partition of $I\subset \Real_+$.
%%Instead of expressing a belief as a density on a continuous interval we may limit our modelling efforts to defining a belief as a discrete distribution function $\pi_0 : \{ 1,...,m\} \to [0,1], i \mapsto \Pr[ L \in J_i]$.  
%%
%%\begin{rem}
%%Notice, that this belief encoding may be easier to specify than the density on a continuum of points. 
%%For instance, assume $I = [a,b] , 0<a<b \in \Real_+ \cup \{\infty\}$ and let $a=t_0<t_1<...<t_m =b$ such that $J_i = [t_{i-1},t_i], (i=1,...,m)$.
%%Then, knowing the continuous density $p_0$ on $I$ allows us to compute the discrete density via $ \pi_0 (i) = \int_{J_i} p_0(t) \,dt=P_0 (t_i) - P_0(t_{i-1})$. The inverse computation (from discrete to continuous distribution) is not possible without further assumptions.
%%\end{rem}
%%
%%We anticipate our discretization to spawn information loss, since we only encode information about the interval not about the relative location of the H\"older number within the interval. This will be investigated next.
%%
%%%Let $\tau \in (0,1]$ denote this relative interval coordinate. That is to say, H\"older number $L = t_{i-1}+ \tau (t_i -t_{i-1}) $ is completely given by coordinates $(i,\tau) \in \{1,...,m\} \times (0,1]$ . 
%%%
%%%After discretization, our uncertainty about the exact H\"older number (not just the interval) is described by $\tilde p_0(L) =  \pi_0(i) \, p_\tau[\tau | i ]$. Assuming that, after discretization, we are completely oblivious about the location within the interval, we have $p_\tau [\tau | i ] = \frac{1}{| (0,1] |} =1$.
%%%Hence, 
%%%
%%%The magnitude of the information loss due to discretziation could be quantified as 
%%%\begin{align*}
% %%H_{\tilde p_0}-H_{ p_0}  &=\int_I p_0(t) \log p_0(t) \, dt  - \bigl(\sum_{i=1}^m \pi_0(i)   \log \pi_0(i) \bigr) \\
%%%& =  \sum_{i=1}^m \int_{J_i} p_0(t) \log p_0(t) \, dt  \\ 
%%%&- \bigl(\sum_{i=1}^m \int_{J_i} p_0(t) \,dt  \log \int_{J_i} p_0(t) \,dt \bigr)\\
%%%% 
%%%& =  \sum_{i=1}^m \Bigl(\int_{J_i} p_0(t) \log [p_0(t)] \, dt  \\
%%%&-   \int_{J_i} p_0(t) \,dt  \log [\int_{J_i} p_0(t) \,dt] \Bigr)\\
%%%& \stackrel{!?}{\leq} 0
%%%\end{align*}
%%%
%%%
%%%WEIRD !!!  The loss should be greater than 0, not smaller ! 
%%%Mhh... perhaps I should instead try this (?? Makes any difference??)
%%
%%In the discretized situation, our ignorance over $L^*$ can be encoded by the density  $\tilde p_0(L) =  \sum_{i=1}^m \pi_0(i) \, p_L [L| i ]$. Assuming that, after discretization, we are completely oblivious about the location within the interval, we have $p_L [L | i ] = \frac{1}{| J_i |} =\frac{1}{| t_i-t_{i-1} |}$.
%%Hence, $\tilde p_0(L)  =  \sum_{i=1}^m  \frac{\pi_0(i)}{| J_i |} $. 
%%
%%The magnitude of the information loss due to discretziation could be quantified as 
%%\begin{align*}
% %H_{\tilde p_0}-H_{ p_0}  &=\int_I p_0(L) \log p_0(L) \, dL  - \int_I \tilde p_0(L)    \log  \tilde p_0(L) \, dL \\
%%& = \int_I p_0(L) \log p_0(L) \, dL  \\
%%&- \int_I\sum_{i=1}^m \pi_0(i) \, p_L [L| i ]    \log \bigl(\sum_{i=1}^m \pi_0(i) \, p_L [L| i ]\bigr) \, dL \\
%%& = \int_I p_0(L) \log p_0(L) \, dL  \\
%%&- \int_I\sum_{i=1}^m \frac{\pi_0(i)}{|J_i|}     \log \bigl(\sum_{i=1}^m \frac{\pi_0(i)}{|J_i|} \bigr) \, dL \\
%%& = \int_I p_0(L) \log p_0(L) \, dL  \\
%%&- |I|  \log \bigl(\sum_{i=1}^m \frac{\pi_0(i)}{|J_i|} \bigr) \sum_{i=1}^m \frac{\pi_0(i)}{|J_i|}     \\
%%& =  \sum_{i=1}^m \Bigl(\int_{J_i} p_0(t) \log [p_0(t)] \, dt \Bigr)   \\
%%&- |I|  \log \bigl(\sum_{i=1}^m \frac{\int_{J_i} p_0(t) dt}{|J_i|} \bigr) \sum_{i=1}^m \frac{\int_{J_i} p_0(t) dt}{|J_i|}     \\
%%& \stackrel{!?} {\geq }0
%%\end{align*}
%%
% %
%%However, the benefit is that (continuous) extremization problem is reduced to a tractable, discrete optimization problem of dimensionality $m$. In fact, it is a convex program with linear constraints:
%%
%%\begin{align}
%%\argmin_p & \KLD {\pi}{\pi_0}\\
%%\text{s.t.:}&\\
%%& \pi(i) \in [0,1], \forall i \in\{1,...,m\}\\
%%&\SP{p}{e}_{2} =1\\
%%& \SP{p}{n_{L_D}}_{2} =0
%%\end{align}
%%where $e$ is a vector of $m$ ones and $n_{L_D}$ is suitably defined to mimic a discretized version of the indicator function above and whose $i$th component is defined as follows:
%%
%%$n_{L_D} (i) = \begin{cases} 1, t_i \geq L_D\\ 0, \text{otherwise.} \end{cases}$ Of course, if $t_{i-1} < L_D < t_i$ for some $i$, we have once again thrown away information,as the constraint $\SP{p}{n_{L_D}}_{2} =0$ does not capture the knowledge that there must be zero probability mass on $K_i' := [t_{i-1},L_D)$ as well. To cover this, we could consider 
%%introducing an additional component representing the probability on $K_i$  and replace the original meaning of the original $i$th component by representing the probability on  $J_i' = [L_D, t_i] =J_i - K_i$ instead of on $J_i$. In this case, the CP becomes $m+1$-dimensional. Since this is always possible to do, we can assume, without loss of generality, that $L_D $ will always be an element of $t_1,...,t_m$ for some $m$.
%%
%%
%%Note, an $m$-dimensional CP can be solved in worst-time complexity $\mathcal O(m^3)$ (LOOK IT UP!!).
%%
%%
%%\begin{rem}
%%We could investigate how the information loss (which we would expect to grow as a function of $m$) compares to the 
%%the gain in computational complexity. We should then conceive a common exchange rate / currency / trade-off parameter to 
%%find a good cut-off point.
%%\end{rem}
%%
%
%
%\begin{figure}
%        \centering
%				  \subfigure[Inferred model with $L=10$.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.5cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/predL10}
%    \label{fig:Hoelderconstvar1}
%  } 	
%	 \subfigure[Inferred model with $L=0.1$.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.5cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/predLpt1}
%    \label{fig:Hoelderconstvar2}
%  } 	%\hspace{2cm}
%	 \subfigure[Inferred model with $L=1$.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.5cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/predL1}
%    \label{fig:Hoelderconstvar3}
%  } 		
%	\label{fig:Hoelderconstvar}
%   \caption{Example of the predictions of the values of ground-truth function $x \mapsto \sqrt{\abs{\sin(x)}}$ using varying H\"older constants. For all predictions, a standard metric $\metric_\inspace(x,x') = \abs{x-x'}$ and a H\"older exponent of $p= \frac 1 2$ was employed. The global H\"older constant (and hence, the optimal constant) was $L=1$. }
%\end{figure}	 


%\subsection{A lazy update rule} 
\label{sec:lazylipconstupdate}
%We assume there is a global H\"older constant that is uncertain. 
%In the presence of uncertainty it is important to be able to update the H\"older constant $L$ in the light of the data. After all, if chosen too conservatively high, the regularity properties of the actual ground truth will be lost and yield predictions that are too steep and, for large $L$, yield step function predictions (cf. Fig \ref{fig:Hoelderconstvar1}). And, if decision making takes the error bounds provided into account, the unnecessary uncertainty may result in overly cautious behaviour and hence, poor performance. 
%On the other hand, underestimating $L$ may even be worse. If $L$ is chosen too small then the error bounds are off and predictions may be unable to accurately infer the true shape of the function (cf. Fig \ref{fig:Hoelderconstvar2}). 
%
%Above we have outlined a Bayesian treatment in the face of probabilistic uncertainty. This is an adequate choice if one's uncertainty can be specified by a prior and if the necessary integrals can be computed efficiently. 
%
%In practice, both can be difficult and we might resort to a more pragmatic approach which we will outline in this subsection. Furthermore, the Bayesian approach can fall prey to stubbornness and cannot recover from false beliefs of impossibility. That is, if an observed data point provides evidence for the validity of an event that has zero measure under the prior the posterior will be unable to adjust and also ascribe zero-measure to the event, even if most strongly supported by the evidence.  
%
%To avoid underestimating the H\"older constant without resorting to overly conservative choices of $L$ it might be possible to start with a good estimate of $L$ that is not overly conservative and to update 
%this lazily, that is, only if required. 

\subsubsection{A first update rule}
 In this subsection, we present an incremental update law that allows our method to increase the estimate of the H\"older constant if newly available data suggests the previously assumed upper bound on the constant was insufficiently high.
 
Assume we have sequential access to a sequence $\seq{\data_n}{n \in \nat}$ of data sets $\data_n:= \{\bigl( s_i, \tilde f_i \bigr) \vert i=1,\ldots, N_n\} $ with $\data_n \subset \data_{n+1}$ ($n \in \nat$) with observational error bound $\obserr$. For simplicity (of notation), we will for now assume that the input space pseudo-metric is a full metric. That is, that we have $\metric_\inspace(x,x') = 0 \Leftrightarrow x=x'$.
%For notational brievty we introduce the set $$\mathcal U := \{ (x,x') \in \inspace^2 | \metric_\inspace(x,x') >0 \}.$$
  We will consider the task of utilising the data to compute estimates to update a deterministic belief over a H\"older constant. In order to bound the conservatism of our uncertainty bounds derived from the constant in the context of kinky inference, the ability to uncover low H\"older constants or even the \emph{optimal} H\"older constant $L^* = \sup_{x'\neq x } \frac{\metric_\outspace \bigl(f(x) - f(x')\bigr)}{\metric_{\inspace}^p(x,x') }$ of the target function $f$ are of particular interest. 
Remember, $\hoelset p {} {L'}  \subset \hoelset p {} {L''} $ for $L'' \geq L'$. Therefore, in order not to inflate the set of hypothesis functions that could have generated the data more than necessary, one might choose not to rule out any lower global H\"older constant candidates unless the data suggests ones has to. In this approach, after having observed $\data_{N_n+1}$, $L(n+1)$ is chosen to be just large enough such that the H\"older condition is not in conflict with sample-consistency, i.e. such that $\mathcal K(\data_{N_n+1}) \cap \bigl(  \mathcal K_{prior} \cup \hoelset p {} {L(n+1)} \bigr) \neq \emptyset$. This approach gives rise to a \emph{lazy} update rule which only increases the current estimate $L(n)$ by the minimal amount necessary to remove any inconsistency with the new data if such inconsistencies are detected. %if the new data point is otherwise inconsistent with it.

Before introducing our lazy update approach in full generality, we will consider a special case first:
For simplicity, we assume that the target is real-valued with $\outspace \subseteq \Real, \metric_\outspace(y,y') = \abs{y-y'}$ for all $y,y \in \outspace$ and that a uniform observational error bound $\obserr =\obserr(x) \in \Real_{\geq 0}, \forall x$ is given. Furthermore, we assume the bounding functions $\ubf,\lbf$ are inactive, i.e. $\lbf \equiv -\infty, \ubf \equiv \infty$. Therefore, the uncertainty hyperrectangle $\prederrbox_n(x)$ around the prediction $\predfn(x)$ coincides with the interval $[\boden_n\bigl(x; L(n)\bigr) ,\decke_n\bigl(x; L(n)\bigr)]$.


For now, we also assume that at each time $n$ we receive one new data point. In this scenario we have $\data_{n+1} \backslash \data_n=\{(s_{N_n+1},\tilde f_{N_n+1}) \}$ with $N_n = n$. Given that at time $n$ the lazy estimator proposes the optimal H\"older constant $L^*$ to be $L(n) \in \Real_{\geq 0}$, how should the arrival of the new data point $(s_{N_n+1},\tilde f_{N_n+1},\obserr)$ affect the belief in the H\"older constant? %Now assume that a new sample observation $(s_{N_n+1},f_{N_n+1}, \obserr)$ arrives.  
Following our lazy approach, we only make modifications if the previous estimate is unduly low in the light of the new data. Here the new data point $(s_{N_n+1},\tilde f_{N_n+1},\obserr)$ is evidence for constant $L(n)$ to be unduly low if it falls outside of the prediction uncertainty  interval $\prederrbox_n(x)$. This is the case if 
$\tilde f_{N_n+1} +\obserr < \boden_n(s_{{N_n}+1}) \vee \tilde f_{{N_n}+1} - \obserr > \decke_n\bigl(s_{{N_n}+1}; L(n)\bigr)$ or equivalently, if 
$\tilde f_{{N_n}+1} +\obserr < \max_{i=1,\dots,N_n} \tilde f_i - \obserr - L(n) \metric^p_{\inspace}(s_{{N_n}+1},s_i) \vee \tilde f_{{N_n}+1} - \obserr > \min_{i=1,\dots,N_n} \tilde f_i + \obserr + L(n) \metric^p_{\inspace}(s_{{N_n}+1},s_i)$.
Equivalently, this means that 
\begin{equation}
	\abs{\tilde f_{{N_n}+1} -\tilde f_i} > 2 \obserr +  L(n) \metric^p_{\inspace}(s_{N_n+1},s_i) \, \forall i \in \{1,...,N_n\}. 
\label{eq:Lupdatecond}
\end{equation}
This is a condition one could test for in $\mathcal O(d \, N_n)$ steps. If the condition is met, we can change the presupposed H\"older constant  to assume a value such that the condition is no longer met. To this end, we can choose the updated H\"older constant $L({n+1})$ to be 
%
\begin{equation}
	L({n+1}) := \max\left\{ L(n), \max_{i=1,...,N_n} \frac{\abs{\tilde f_{{N_n}+1}-\tilde f_i} -  2 \obserr}{\metric^p_{\inspace}(s_{N_n+1},s_i)} \right\}
\label{eq:Lupdateeq}
\end{equation}
which can be computed in $\mathcal O(M \, N_n)$, assuming the metrics can be evaluated in the order of $\mathcal O(M)$ computational steps. 
%
Note, if we set $L(0) = L(1) := 0$, we are guaranteed that our incremental estimate $L({n+1}) $ coincides with the empirical H\"older constant estimate $$L({\data_{n+1}} ) :=  \max \bigl\{0,\max_{i,j =1,...,N_{n+1}, i\neq j} \frac{\metric_\outspace(\tilde f_i,\tilde f_j) -2 \obserr}{\metric^p_{\inspace}(s_i,s_j)} \bigr\}.$$ As we will see below, this estimate always is a lower bound on the true lowest H\"older constant $L^* = \sup_{x \in \inspace, x' \in \inspace\backslash \{x\}} \frac{\abs{f(x) - f(x')}}{\metric_{\inspace}(x,x') }$.



\subsubsection{Generalisations and properties} 
Next, we will examine our lazy update rule in a generalised setting. Here, we assume the target function is a mapping $f: \inspace \to \outspace$ where the input space $\inspace$ is endowed with a pseudo-metric $\metric_\inspace$ and the output space $\outspace$ is an additive group, endowed with a pseudo-metric $\metric_\outspace$ that is translation-invariant, i.e. $\metric_\outspace(y+\tau,y'+\tau) = \metric_\outspace(y,y'),\forall y,y',\tau \in \outspace$. Throughout the remainder of the article, we will frequently take maxima over sets. 
Now allowing for non-definite pseudo-metrics, we need to ensure none of the denominators can be zero. For notiational convenience, for two sets $S,S' \subset \inspace$ of inputs we define  $$U(S,S') := \{(s,s') \in S \times S' | \metric_\inspace(s,s') >0\}$$ as the set of input pairs that the pseudo-metric can tell apart and define $U_n := U(G_n,G_n) $.
For notational simplicity, we assume $\max(\emptyset) = -\infty$ and $\max(S\cup \{
-\infty\}) = \max (S)$ for any set $S$.

We assume that a priori, that is, before having seen any data, we know a lower bound $\underline L$ on the optimal H\"older constant $L^* \in \Real_{\geq 0}$.
At time $n$ we desire to entertain a deterministic belief $\ell_n \geq 0$ about H\"older constant $L^*$ which is consistent with the data $\data_n$ observed so far.
In this context consistency means that 
$\ell_n $ is at least as large as the empirical estimator $\ell({\data_n};\hestthresh,\underline L)$ of the constant defined as follows:  
%\begin{equation}
%\ell(\data_n;\hestthresh,\underline L)  :=  \begin{cases} \underline L &, \text{ if } N_n =\abs{\data_n} \leq 1\\ 
% \max \Bigl\{ \max_{i,j =1,...,N_n, i\neq j} \frac{\metric_\outspace(\tilde f_i,\tilde f_j) - \hestthresh}{\metric_{\inspace}^p(s_i,s_j)},\underline L \Bigr\}.
% &, \text{ otherwise }. \end{cases}
%\end{equation}
\begin{equation}\label{eq:lazyconstupdaterule_batch}
\ell(\data_n;\hestthresh,\underline L)  := 
 \max \Bigl\{ \underline L, \max_{(s,s') \in U_n} \frac{\metric_\outspace(\tilde f_i,\tilde f_j) - \hestthresh}{\metric_{\inspace}^p(s_i,s_j)}\Bigr\}.
\end{equation}

 Here $\hestthresh \in \Real$ is a parameter which, consistent with our considerations above, by default we set to $\hestthresh = 2 \metric_\outspace(0, \obserr)$. This imposes a tolerance margin that is necessary since the presence of observational error $\obserr$ could cause the \emph{empirical H\"older constant} $\ell(\data_n;0,\underline L)$ to overestimate the actual smallest constant $L$ in an unbounded manner. 
Parameter $\underline L$ is an a priori specifiable lower bound on the true best H\"older constant $L^*$. In the absence of further domain-specific a priori knowledge on this bound we can always set $\underline L=0$ (since negative constants are not meaningful in the definition of H\"older continuity). 
In the absence of observational errors (i.e. in case $\obserr =0$) it should be clear that the sequence of estimates $\seq{\ell(\data_n;\lambda,0)_n;0,\underline L)}{n \in \nat}$ converges to $L^*$ if the sequence of grids $\seq{G_n}{n \in \nat}$ converges to a dense subset of the domain $\inspace$ (and provided that indeed $\underline L \leq L^*$).

However, in the presence of observational errors, $\ell(\data_n;0,\underline L)$ can in general overestimate the H\"older constant with arbitrarily high error. Fortunately, parameter $\hestthresh$ can prevent this:
Provided that $\hestthresh$ is chosen sufficiently large and that the a priori lower bound is a valid lower bound (i.e. $\underline L \leq L^*$), it is easy to show that the empirical estimates of the constant converge and never exceed the true optimal H\"older constant $L^*$. 
This is formalised as follows:

\begin {lem} \label{lem:constadaptation_boundedness} Let $\metric_\outspace: \outspace^2 \to \Real$ be a translation-invariant pseudo-metric on an abelian group $(\outspace,+)$.n Define $L^*$ to be the best H\"older constant of the target $f$.
With the definitions as above, we have:
\begin{itemize}
\item \textbf{(I)} If $D \subset D'$ then $\ell(D;\hestthresh,\underline L) \leq \ell(D';\hestthresh,\underline L)$.
\end{itemize}
If $\hestthresh \geq 2 \metric_\outspace(0,\obserr)$ we have:
\begin{itemize}
\item \textbf{(II)} $\forall n \in \nat: \ell(\data_n; \hestthresh,\underline L) \leq \max\{L^*,\underline L\}$ and  
\item \textbf{(III)} the sequence \seq{\ell(\data_n; \hestthresh,\underline L)}{n \in \nat} of empirical estimators monotonically converges to a number less than or equal to $\max\{L^*,\underline L\}$ provided that $\data_{n} \subset \data_{n+1}, \forall n \in \nat$.
\end{itemize}
\end{lem}
\begin{proof}
\textbf{(I)} This follows trivially from the fact that $\max S \leq \max M$ for two sets $S \subseteq M$. \\
\textbf{(II) }
We know that the $\tilde f_i$ are noisy observations of the ground truth $f(s_i)$ $(i=1,...,N_n$. That is, there exist $\phi$ such that $(i)$ $\tilde f = f + \phi$  and $(ii)$ $\metric_\outspace(0,\phi_i) \leq \metric_\outspace(0,\obserr)$ $(i =1,\ldots, N_n)$. 
Furthermore, note that in general (cf. Lem. \ref{lem:bilinaddtransinvgroup}), in additive groups $(G,+)$ endowed with a translation-invariant pseudo-metric $\metric_G$ one has $(iii)$ $\forall g,g',g'' \in G: \metric_G (g+g',g'') \leq \metric_G (g+g',g)+\metric_G(g,g'') = \metric_G (g',0)+\metric_G (g,g'')$. Finally, we remind ourselves that $(iv)$ $L^* \geq \sup_{x,x' \in \inspace, \metric_\inspace(x,x')>0} \frac{\metric_\outspace\bigl(f(x),f(x') \bigr)}{\metric_{\inspace}^p(x,x')}$ $\geq \ell(S;0,0)$ for any finite subset of input points $S \subset \inspace$.

These facts allow us to reason as follows:
%\begin{tiny}
\begin{align}
&\ell(\data_n;\hestthresh,\underline L)  %& = \max \bigl\{ 0, \max_{i,j =1,...,N_n, i\neq j} \frac{\metric_\outspace(\tilde f_i,\tilde f_j) - \hestthresh}{\metric_{\inspace}^p(s_i,s_j)} \bigr\} \\ 
\\
 &\stackrel{(i)}{=} \max \Bigl\{ \underline L, \max_{(s,s') \in U_n} \frac{\metric_\outspace\bigl( f(s) + \phi(s),f(s')+\phi(s')\bigr) - \hestthresh}{\metric_{\inspace}^p(s,s')} \Bigr\}\\
  &\stackrel{(iii)}{\leq} \max \Bigl\{ \underline L, \max_{(s,s') \in U_n} \frac{\metric_\outspace\bigl( f(s),f(s') \bigr)  + \metric_\outspace(0,\phi(s)) + \metric_\outspace(0,\phi(s')) - \hestthresh}{\metric_{\inspace}^p(s,s')} \Bigr\}\\
    &\stackrel{(ii)}{\leq} \max \Bigl\{ \underline L,  \max_{(s,s') \in U_n} \frac{\metric_\outspace\bigl( f(s),f(s') \bigr)  }{\metric_{\inspace}^p(s,s')} +\frac{2 \metric_\outspace(0,\obserr) - \hestthresh}{\metric_{\inspace}^p(s,s')} \Bigr\}\\
        &\stackrel{(iv)}{\leq}  \max \Bigl\{ \underline L, L^* +\max_{(s,s') \in U_n} \frac{2 \metric_\outspace(0,\obserr) - \hestthresh}{\metric_{\inspace}^p(s,s')} \Bigr\}.
\end{align} 
%\end{tiny}
Hence, for $\ell(\data_n;\hestthresh,\underline L) \leq \max\{L^*,\underline L\}$ to hold it suffices to choose parameter $\hestthresh$ such that \newline
%
$L^* +\max_{(s,s') \in U_n}  \frac{2 \metric_\outspace(0,\obserr) - \hestthresh}{\metric_{\inspace}^p(s,s)} \leq L^*$.
Since the denominators cannot be negative, this holds if the nominator $2 \metric_\outspace(0,\obserr) - \hestthresh$ is not positive, i.e. if $2 \metric_\outspace(0,\obserr) \leq \hestthresh$. \\
\textbf{(III)} is entailed by applying the monotone convergence theorem in conjunction with (I) and (II).
\end{proof}
For time $n$, let $S_{n+1} := G_{n+1} \backslash G_n$ be the set of new sample inputs.
Similarly to above, we can define an incremental update rule recursively as follows: 
\begin{align} \label{eq:Hoelconstlazyupdateincr}
\ell_{n+1} &:= \max\Bigl\{\ell_n, \max_{(s,s') \in U(G_n, S_{n+1})} \frac{\metric_\outspace\bigl(\tilde f(s),\tilde f(s')\bigr) - \hestthresh}{\metric_{\inspace}^p(s,s')},\\
&\max_{(s,s') \in U(S_{n+1}, S_{n+1})} \frac{\metric_\outspace\bigl(\tilde f(s),\tilde f(s')\bigr) - \hestthresh}{\metric_{\inspace}^p(s,s')} \Bigr\},
\end{align} for $n \in \nat$ 
and where 
$\ell_0 := \underline L$. 
The effort for computing $\ell_{n+1}$ is in the order of $\mathcal O\bigl(M (\abs{S_{n+1}} N_n+ \abs{S_{n+1}}^2)\bigr)$ where $M$ denotes the effort for evaluating the pseudo-metrics.
By construction, we have \[\ell_n =\ell(\data_n;\hestthresh,\underline L), \forall n \in \nat.\] Therefore, our convergence and boundedness results about the sequence
 $\seq{\ell(\data_n;\hestthresh,\underline L)}{n \in \nat}$ readily apply to the incrementally computed sequence of estimators $\seq{\ell_n}{n \in \nat}$.

%\begin{rem} Above, we have assumed that the input space pseudo-metric was a full metric. This was done for notational convenience to keep the statements of our maximisations terse. The modifications to these statements to accommodate a non-definite input pseudo-metric is straight-forward: all we need to do is to only consider input pairs $s_i,s_j$ in the maximisation steps that give rise to non-zero denominators $\metric_\inspace(s_i,s_j)$. For example, \end{rem}

==> content2/Ch_kinkyinf/est_enclosingfcts.tex <==
\section{Conservative Lipschitz function estimates via enclosing functions }

Let $a,b \in \Real, a \leq b, I := [a,b] \subset \Real$. Given a
Lipschitz continuous \emph{target function} $f: I \to \Real $ and
let $L \geq 0$ be its Lipschitz constant. That is, $\forall S
\subset I \,\exists L_S \leq L \,\forall x,x' \in S: \abs{f(x) -
f(x')} \leq L_S \, \abs{x-x'}$. Let $a = t_1 < t_2 <...<t_N = b $
and define $G_N = \{ t_1,...,t_N\}$ to be the \emph{sample grid} of
size $N \geq 2$ consisting of the input at which we choose to evaluate the
target $f$.

\subsection{On dense grids}
Remember, a subset $G$ of a topological space $I$ is called \textit{dense} if for every point $x \in I$ we have $x \in G$ or that $x$ is a limit point of $G$: That is, if every neighborhood of $x$ contains at least one point of $I$.
In our case, we will consider the set $I$ to be the compact input interval together with the standard topology. The latter is defined to be the set of all open $\epsilon$ neighborhoods of the form $U_\epsilon (x) := \{t \in I | \norm{t - x} < \epsilon \}$ $(\epsilon \in \Real_+, x \in I)$.

To establish convergence to the ground truth (may it be the target function or its definite integral), we will assume that we constructs grids $G_N$ that become increasingly dense, with increasing grid size. That is to say, we desire that $G_N \to G \subset I$, where $G$ is dense in $I$.
If this is the case, we know the following:

\begin{defn}[Eventually dense partition]
Grid sequence $(G_N)_{N \in \nat}, G_N = \{t_1^N,...,t_N^N \}$ becomes an eventually dense partition of $I$ if the maximum interval radius $\bar r_N = \max\{\frac{t^{N}_{i+1} - t^{N}_{i}}{2} | i=1,...,N-1 \}$
vanishes in the limit of large $N$. That is, $\bar r_N \stackrel{N \to \infty}{\longrightarrow} 0$. 
\end{defn}

The following lemma establishes that a sequence converging to a dense subset of $I$ yields an eventually dense partition:

\begin{lem} \label{lem:densegridmaxdist}
Let $G_N = \{t_1^N,...,t_N^N \} \stackrel{N \to \infty }{\longrightarrow} G$ where $G$ is a dense subset of $I=[a,b]$ and where $a=t_1^N<,\ldots,<t_N^N=b$. 
Eventually, the maximum distance between any two consecutive grid elements is arbitrarily small:
\[ \forall \epsilon >0 \exists N_0 \in \nat \forall N\geq N_0 \forall i <N: \abs{t_{i+1}^N - t_i^N} \leq \epsilon.\]
\begin{proof}
Since $G_N$ converges to a dense set in $I$ as $N \to \infty$, we know
\begin{equation}\label{eq:densegrid}
 \forall \epsilon >0 \forall x \in I \exists N_0 \forall N\geq N_0: G_N \cap U_\epsilon(x) \neq \{\emptyset\} 
\end{equation}
where $U_\epsilon(x)$ denotes an $\epsilon -$ball around $x$.
Choose any $\epsilon >0$. Divide $I$ into $q =  \frac{\abs I}{\epsilon/2}$ compact intervals $U^1_{\epsilon/4},\ldots,U^q_{\epsilon/4}$, i.e. $U^j_{\epsilon/4} = \{x \in I \,|\, \norm{x - \bigl(a+(2j-1)\,\frac{\epsilon}{4}\bigr)  } \leq \frac{\epsilon}{4} \}$.
Due to (\ref{eq:densegrid}) we know that for each $j$ there exists $N_0^j$ such that $G_N \cap U^j_{\epsilon/4} \neq \emptyset, \forall N \geq N_0^j$. Choose $N_0 := \max_{j \in \{1,\ldots,q\}} N^j_0$.
Then, $\forall N \geq N_0,j \in \{1,\ldots,q\}: G_N \cap U^j_{\epsilon/4} \neq \emptyset  $. 
Equivalently, $\forall N \geq N_0,j \in \{1,\ldots,q\}\exists i \in \{1,\ldots, N\}: t^N_i \in U^j_{\epsilon/4}$. That is, all neighborhoods contain at least one grid point in $G_N$ ($N \geq N_0$). Hence, two consecutive grid points are either contained in the same neighborhood or in adjacent ones: 
$\forall i <N \exists j \in \{1,\ldots,q\}:  t^N_i \in U^j_{\epsilon/4} \Rightarrow (t^N_{i+1} \in U^j_{\epsilon/4} \vee t^N_{i+1} \in U^{j+1}_{\epsilon/4})$. 
Since the maximal distance between points of two adjacent $\epsilon/4$ neighborhoods is twice their diameter (and within the neighborhood is once the diameter), we have $ \abs{t_{i+1}^N - t_i^N} \leq \epsilon$.

\end{proof}

\end{lem}


\subsection{Enclosures}
\label{sec:enclosures}

\begin{defn}[Enclosure]
Let $\decke,\boden: I \to \Real$ be two functions, such that $\decke
\geq \boden$ pointwise on $I$. We define their enclosure on $I$ as
the compact interval $\mathcal E^\decke_\boden (I)$ of all functions
between them. That is, \[\mathcal E^\decke_\boden (I) := \{\phi: I
\to \Real \vert \forall t \in I: \decke(t) \geq \phi(t) \geq
\boden(t) \}.\]
\end{defn}
For ease of notation we omit the domain argument whenever we refer
to $I$. That is, we write  $\mathcal E^\decke_\boden :=\mathcal
E^\decke_\boden (I)$.

\begin{defn}[Sample-consistency]
A function is \emph{sample-consistent} (with $f$ on grid $G_N$) if
it coincides with $f$ on values contained in the grid $G_N$.
\end{defn}

\begin{defn}[Sample-consistent enclosure]
A \emph{sample-consistent enclosure} is a set containing all
sample-consistent functions of an enclosure.
\end{defn}



Based on the sample $f(t_1),...,f(t_N)$ we desire to find two
\emph{enclosing functions} $\decke_N: I \to \Real$, $\mathfrak
\boden_N: I \to \Real$ bounding the target from above and below that
are as tight as possible and converge to the target in the limit of
infinite, (equidistant) sample grid size $N$. Formally, we state the
following \textbf{desiderata}:
\begin{enumerate} 
    \item \textbf{Consistency}: The enclosing functions coincide with the target on the sample grid. That is,
    $\forall t \in G_N: \, f(t) = \decke_N(t) = \boden_N(t)$.
     \item \textbf{Exhaustiveness}: Every $\phi$ coinciding with target $f$ on with grid $G_N$ and
having the same Lipschitz
    constant $L$ on $I$ as $f$ is also contained in the enclosure:$\forall \phi: I \to \Real, \phi \notin \einschluss:
       \phi_{\vert G_N} \neq f_{\vert
    G_N} \vee L_I(\phi) > L$.
    
    In particular, the target is contained in the enclosure: $f \in \einschluss$.
\item \textbf{Minimality}: If $\mathcal E$ is an enclosure satisfying \emph{Desideratum 2} then $\einschluss \subseteq \mathcal E$.    
    
\item \textbf{Convergence} to the target: $\lim_{N \to \infty} \decke_N = \lim_{N \to \infty}
    \boden_N = f$ uniformly, if $(G_N)$ converges to a dense subset of $I$ as $N \to \infty$ or, if $(G_N)_{N \in \nat}$ becomes an eventually dense partition of $I$.
   % \item Minimality of the enclosure --the enclosure only contains functions with a minimum Lipschitz number up to
   % the target function's: $\phi \in \einschluss \Rightarrow L_I(\phi) \leq
%    L \wedge \phi_{\vert G_N} = f_{\vert
%    G_N}$ ;

\end{enumerate}

Next, we will define enclosing functions meeting all desiderata.

For $i=1,\ldots,N-1$ we define the \emph{sample intervals} $J_i :=
[t_i,t_{i+1}) \subset I$ and $\bar J_i :=
[t_i,t_{i+1}) \subset I$. In addition, we define $J_N = b$. Furthermore, we define $a_i = t_i, b_i =
t_{i+1}$, i.e. $J_i= [a_i,b_i), \bar J_i= [a_i,b_i], (i=1,\ldots,N-1)$. For $i=N$ we define $a_i=b_i=b$.


Due to Lipschitz continuity, we have

\begin{equation} \forall x,x' \in J_i: \abs{f(x) - f(x')} \leq L_i \,
\abs{x-x'}
\end{equation}
where $L_i := L_{J_i}$.

\begin{defn}[Lipschitz ceiling]\label{def:lipceil}
On interval $J_i$ we define line segments via $\alpha^\decke_i: x
\mapsto f(a_i) + L_i (x - a_i)$ and $\beta^\decke_i: x \mapsto
f(b_i) -L_i (x - b_i)$. We define components of the (Lipschitz)
\emph{ceiling} of function $f$ on interval $J_i$ as the piece-wise
linear function
\[\decke^i_N: t \mapsto \min\{ \alpha^\decke_i(t), \beta^\decke_i(t) \}.\] On
the entire interval $I = \bigcup_i J_i$ the upper enclosing function
is equated to the \emph{ overall (Lipschitz) ceiling} connecting the
local ceilings:
\[ \decke_N (t) :=   \sum_{i=1}^{N}  \chi_{J_i}(t) \,\decke^i_N(t),\,\,  \]
where $\chi_{J_i}: \Real \to \{0,1\}$ denotes the indicator function
for interval $J_i$.
\end{defn}
To complete our definition of our enclosing function we need to
define the lower bound as well, which we will refer to as the
\emph{Lipschitz-floor}.

\begin{defn}[Lipschitz floor]\label{def:lipbot}
On interval $J_i$ we define line segments via $\alpha^\boden_i: t
\mapsto f(a_i) - L_i (t - a_i)$ and $\beta^\boden_i: t \mapsto
f(b_i) +L_i (t - b_i)$. We define components of the (Lipschitz)
\emph{floor} of function $f$ on interval $J_i$ as the piece-wise
linear function
\[\boden^i_N: t \mapsto \max\{ \alpha^\boden_i(t), \beta^\boden_i(t) \}.\] On
the entire interval $I = \bigcup_i J_i$ the upper enclosing function
is equated to the \emph{ overall (Lipschitz) ceiling} connecting the
local ceilings:
\[ \boden_N (t) :=  \sum_{i=1}^{N}  \chi_{J_i}(t) \,\boden^i_N(t),\,\,  \]
where $\chi_{J_i}: \Real \to \{0,1\}$ denotes the indicator function
for interval $J_i$.
\end{defn}


An example for a Lipschitz enclosure is given in Fig. 
\begin{figure*}
	\centering
		\includegraphics[scale = .4]{content/figs/enclosure.pdf}
	\caption{Example of a Lipschitz enclosure for a given sample of function values. The Lipschitz constant was one, uniformly over the entire domain.}
	\label{fig:enclosure}
\end{figure*}


The following lemmata will prove useful:

\begin{lem} \label{lem:ceiling_values}
For $i \in \{1,\ldots,N-1\}$ let  $L_i > 0$, and let $L_N \geq 0$.
Define $\xi^{\mathfrak u}_i :=  \frac{b_i+a_i}{2}+ \frac{f(b_i) - f(a_i)}{2 L_i}  $.\\
We have 
\[\xi^{\mathfrak u}_i \in \arg\max_{t \in I} \decke^i_N (t), \,\,\xi^{\mathfrak u}_i \in \bar J_i\]
and 
 \[y^{\mathfrak u}_i := \decke_N^i(\xi^{\mathfrak u}_i) = \frac{f(b_i) +f(a_i)}{2} + L_i \frac{b_i-a_i}{2} .\]
\begin{proof} The case $i = N$ is trivial. Let $1 \leq i \leq N-1$. By definition,
$\decke^i_N (t) = \min\{ \alpha^\decke_i(t), \beta^\decke_i(t)\}$.
We have $\dot  \alpha^\decke_i(t) = L_i > 0$ and $\dot  \beta^\decke_i(t) = - L_i < 0$. Hence, the functions are strictly monotonous. Let $\xi$ the input where the lines intersect, i.e. $\alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$. Monotonicity implies $\forall t \leq \xi : \alpha^\decke_i(t) \leq \alpha^\decke_i(\xi) \wedge \beta^\decke_i(t) \geq \beta^\decke_i(\xi) = \alpha^\decke_i(\xi)$. 
Hence,
 \[\forall t \leq \xi: \decke_N^i(t) = \min \{\alpha_i^{\mathfrak u} (t), \beta_i^{\mathfrak u} (t) \}= \alpha_i^{\mathfrak u} (t).\] 
 
Analogously, monotonicity implies $\forall t \geq \xi : \beta^\decke_i(t) \leq \beta^\decke_i(\xi) \wedge \alpha^\decke_i(t) \geq \alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$. 
Thus,
 \[\forall t \geq \xi: \decke_N^i(t) = \min \{\alpha_i^{\mathfrak u} (t), \beta_i^{\mathfrak u} (t) \}= \beta_i^{\mathfrak u} (t).\] 

In conjunction, we have 
 $\decke_N^i(t) = 
 \begin{cases}  
 \alpha_i^{\mathfrak u} (t), & t \leq \xi \\
 \beta_i^{\mathfrak u} (t), & t \geq \xi 
 \end{cases}$.
 Again, using monotonicity of $\alpha_i^{\mathfrak u}$ and $\beta_i^{\mathfrak u}$ we infer that $\decke_N^i$ has a single maximum $y := \decke_N^i(\xi)$ at $\xi$.
It remains  (i) to show that $\xi = \xi_i^{\mathfrak u}$, (ii) we need to evaluate $\decke_N^i(\xi^{\mathfrak u}_i)$ and (iii) that $\xi^{\mathfrak u}_i \in \bar J_i$.

(i) $\alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$

$\Leftrightarrow  f(a_i) + L_i (\xi - a_i) = f(b_i) -L_i (\xi - b_i)$

$\Leftrightarrow  L_i \bigl( 2 \xi - b_i  - a_i\bigr) = f(b_i) - f(a_i) $

$\stackrel{L_i > 0}{\Leftrightarrow}   \bigl( 2 \xi - b_i  - a_i\bigr) = \frac{f(b_i) - f(a_i)}{L_i} $

$\Leftrightarrow   \xi  = \frac{f(b_i) - f(a_i)}{2 L_i}  + \frac{b_i+a_i}{2} = \xi^{\mathfrak u}_i$.

(ii) $\decke_N^i(\xi) = \alpha_i^{\mathfrak u} (\xi) =  f(a_i) + L_i (\xi - a_i) $

$= f(a_i) + L_i \bigl( \frac{f(b_i) - f(a_i)}{2 L_i}  + \frac{b_i+a_i}{2} - a_i \bigr) $ 

$=  \frac{f(b_i) - f(a_i) + 2f(a_i)}{2 }  + L_i \frac{b_i-a_i}{2}   = y_i^{\mathfrak u}$. 

(iii) $\xi^{\mathfrak u}_i \in \bar J_i$ if and only if $a_i \leq \xi^{\mathfrak u}_i \leq b_i$. Since $\xi^{\mathfrak u}_i = \frac{f(b_i) - f(a_i)}{2 L_i}  + \frac{b_i+a_i}{2}$ and $\frac{b_i+a_i}{2}$ is just in the middle value of interval $\bar J_i = [a_i,b_i]$, we have 

$\xi^{\mathfrak u}_i \in \bar J_i$ if $\abs{\frac{f(b_i) - f(a_i)}{2 L_i}} \leq \abs{\frac{b_i-a_i}{2}}$.
However, the latter is the case due to $L_i$-Lipschitz continuity of $f$ on $\bar J_i$.  
\end{proof}

\end{lem}


\begin{lem} \label{lem:floor_values}
For $i \in \{1,\ldots,N-1\}$ let  $L_i > 0$, and let $L_N \geq 0$.
Define $\xi^{\mathfrak l}_i := \frac{b_i+a_i}{2} - \frac{f(b_i) - f(a_i)}{2 L_i}  $.\\
We have 
\[\xi^{\mathfrak l}_i \in \arg\min_{t \in I} \boden^i_N (t), \,\,\xi^{\mathfrak l}_i \in \bar J_i\]
and 
 \[y^{\mathfrak l}_i := \boden_N^i(\xi^{\mathfrak l}_i) = \frac{f(b_i) +f(a_i)}{2} - L_i \frac{b_i-a_i}{2} .\]
\begin{proof} The case $i = N$ is trivial. Let $1 \leq i \leq N-1$. By definition,
$\boden^i_N (t) = \min\{ \alpha^\boden_i(t), \beta^\boden_i(t)\}$.
We have $\dot  \alpha^\boden_i(t) = - L_i < 0, \forall t$ and $\dot  \beta^\boden_i(t) =  L_i > 0, \forall t$. Hence, the functions are strictly monotonous. Let $\xi$ the input where the lines intersect, i.e. $\alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$. Monotonicity implies $\forall t \leq \xi : \alpha^\boden_i(t) \geq \alpha^\boden_i(\xi) \wedge \beta^\boden_i(t) \leq \beta^\boden_i(\xi) = \alpha^\boden_i(\xi)$. 
Hence,
 \[\forall t \leq \xi: \boden_N^i(t) = \max \{\alpha_i^{\mathfrak l} (t), \beta_i^{\mathfrak l} (t) \}= \alpha_i^{\mathfrak l} (t).\] 
 
Analogously, monotonicity implies $\forall t \geq \xi : \beta^\boden_i(t) \geq \beta^\boden_i(\xi) \wedge \alpha^\boden_i(t) \leq \alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$. 
Thus,
 \[\forall t \geq \xi: \boden_N^i(t) = \max \{\alpha_i^{\mathfrak l} (t), \beta_i^{\mathfrak l} (t) \}= \beta_i^{\mathfrak l} (t).\] 

In conjunction, we have 
 $\boden_N^i(t) = 
 \begin{cases}  
 \alpha_i^{\mathfrak l} (t), & t \leq \xi \\
 \beta_i^{\mathfrak l} (t), & t \geq \xi 
 \end{cases}$.
 Again, utilizing monotonicity of $\alpha_i^{\mathfrak l}$ and $\beta_i^{\mathfrak l}$ we infer that $\boden_N^i$ has a single minimum $y := \boden_N^i(\xi)$ at $\xi$.
It remains  (i) to show that $\xi = \xi_i^{\mathfrak l}$, (ii) we need to evaluate $\boden_N^i(\xi^{\mathfrak l}_i)$ showing $y = y_i^{\mathfrak l}$, and (iii) we need to show that 
$\xi^{\mathfrak l}_i \in \bar J_i$ .

(i) $\alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$

$\Leftrightarrow  f(a_i) - L_i (\xi - a_i) = f(b_i) +L_i (\xi - b_i)$

$\Leftrightarrow  L_i \bigl( 2 \xi - b_i  - a_i\bigr) = f(a_i) - f(b_i) $

$\stackrel{L_i > 0}{\Leftrightarrow}   \bigl( 2 \xi - b_i  - a_i\bigr) = \frac{f(a_i) - f(b_i)}{L_i} $

$\Leftrightarrow   \xi  = \frac{f(a_i) - f(b_i)}{2 L_i}  + \frac{b_i+a_i}{2} = \xi^{\mathfrak l}_i$.

(ii) $\boden_N^i(\xi) = \alpha_i^{\mathfrak l} (\xi) =  f(a_i) - L_i (\xi - a_i) $

$= f(a_i) - L_i \bigl( \frac{f(a_i) - f(b_i)}{2 L_i}  + \frac{b_i+a_i}{2} - a_i \bigr) $ 

$=  \frac{-f(a_i) + f(b_i) + 2f(a_i)}{2 }  - L_i \frac{b_i-a_i}{2}   = y_i^{\mathfrak l}$. 

(iii) $\xi^{\mathfrak l}_i \in \bar J_i$ if and only if $a_i \leq \xi^{\mathfrak l}_i \leq b_i$. Since $\xi^{\mathfrak l}_i = -\frac{f(b_i) - f(a_i)}{2 L_i}  + \frac{b_i+a_i}{2}$ and $\frac{b_i+a_i}{2}$ is just in the middle value of interval $\bar J_i = [a_i,b_i]$, we have 

$\xi^{\mathfrak l}_i \in \bar J_i$ if $\abs{\frac{f(b_i) - f(a_i)}{2 L_i}} \leq \abs{\frac{b_i-a_i}{2}}$.
However, the latter is the case due to $L_i$-Lipschitz continuity of $f$ on $\bar J_i$.  
  
\end{proof}

\end{lem}


The reason for calling $\mathfrak r$ \emph{ceiling} is that it
constitutes an upper bound on the function. This is formally
established in the following theorem:

\begin{thm} \label{thm:enclosure1d_desiderata}
With enclosing functions $\decke_N, \boden_N$ defined as per Def.
\ref{def:lipceil} and Def. \ref{def:lipceil} the resulting enclosure
$\einschluss$ satisfies \textit{Desiderata 1-4} specified above.
\begin{proof}
We will need the following fact:
\begin{equation} \label{eq:absineq}
\forall r,r': \abs{r -r'} \geq r -r' \wedge \abs{r -r'} \geq r' -r,
\end{equation}
which follows immediately from the definition of the absolute value.
1) We start proving \textit{Desideratum 1} stating that the enclosing functions defined above are consistent: Let $t_i \in G_n$ be a grid input. 

By definition, we have 
For $t_i =b$, trivially $\decke_N (t_i) = f(t_i)$ by definition. 
For $i < N$:
$ \decke_N (t_i) =   \sum_{j=1}^{N}  \chi_{J_j}(t_i) \,\decke^j_N(t_i) = \decke^i_N(t_i)$
$= \min\{f(a_i) + L_i (t_i - a_i), f(b_i) -L_i (t_i - b_i)\}$ 
$= \min\{f(t_i), f(b_i) -L_i (t_i - b_i)\} = f(t_i)$. The last equality can be shown as follows:
$f(t_i)\leq f(b_i) -L_i (t_i - b_i)$
$\Leftrightarrow f(t_i) - f(b_i) \leq  L_i (b_i - t_i)$
$\Leftrightarrow f(t_i) - f(b_i) \leq  L_i \abs{b_i - t_i}$.
But the latter holds true due to Lipschitz continuity and the fact that 
$f(t_i) - f(b_i) \leq \abs{f(t_i) - f(b_i)}$.

Analogously, for $i=1,...,N-1$, we have 
$ \boden_N (t_i) =  \sum_{i=1}^{N}  \chi_{J_i}(t_i) \,\boden^i_N(t_i)$
$= \max\{f(t_i), f(b_i) +L_i (t_i - b_i)\}$ 
 $= \max\{f(t_i), f(b_i) -L_i (b_i -t_i)\}  = f(t_i)$. The last equality can be shown as follows:
$f(t_i)\geq f(b_i) -L_i (b_i -t_i)$
$\Leftrightarrow L_i (b_i -t_i) \geq f(b_i) - f(t_i)$.
This is the case since: $L_i (b_i -t_i) = L_i \abs{b_i-t_i} \stackrel{\text{Lipschitz}}{\geq} \abs{f(b_i) - f(t_i)} \geq f(b_i) - f(t_i)$.\\

2) Next, we prove exhaustiveness of the enclosure.  
Let $N > 1$, $i \in \{1,...,N \}$, $t,t' \in J_i = [a_i,b_i] \subset
I$ be arbitrary.

Let $\Phi$ be the set of all functions agreeing with $f$ on the grid
and having the same Lipschitz properties as $f$. That is, $\Phi = \{
\phi: I \to \Real| \, (\forall i: L_i(f) = L_i(\phi)) \wedge
(\forall x \in G_N: f(x) = \phi(x)) \}$.

By Lipschitz continuity we have $\forall t,t' \in J_i \abs{\phi(t)
-\phi(t')} \leq L_{i} \, \abs{t-t'}$. In particular, $\abs{\phi(t)
-\phi(a_i)} \leq L_{i} \, \abs{t-a_i}$ and $\abs{\phi(b_i) -\phi(t)}
\leq L_{i} \, \abs{b_i -t}$. Hence, $\abs{\phi(t) - \phi(a_i)}
\stackrel{eq. \ref{eq:absineq}}{\geq} \phi(t) - \phi(a_i)
\wedge\abs{\phi(t) - \phi(a_i)} \stackrel{eq.
\ref{eq:absineq}}{\geq} \phi(a_i) - \phi(t)$.

Now, $t\geq a$ and the Lipschitz property imply $\phi(t) - \phi(a_i)
\leq L_{i} (t-a_i) \wedge  \phi(a_i) -\phi(t) \leq L_{i} (t-a_i)$.
This is equivalent to
\begin{equation} \label{eq:lipintungl1}
\phi(t)  \leq  L_{i} (t-a_i) + \phi(a_i) \wedge  \phi(a_i) - L_{i}
(t-a_i) \leq \phi(t).
\end{equation}

Analogously, we can derive
\begin{equation}\label{eq:lipintungl2}
\phi(t)  \leq  L_{i} (b_i-t) + \phi(b_i) \wedge  \phi(b_i) - L_{i}
(b_i -t) \leq \phi(t) .
\end{equation}

By definition of the ceiling (cf. Def. \ref{def:lipceil}) and floor
(cf. Def. \ref{def:lipbot}) functions, statement
(\ref{eq:lipintungl1}) and statement (\ref{eq:lipintungl2})
collectively yield
%
\begin{eqnarray}
% \nonumber to remove numbering (before each equation)
  \phi(t) &\leq& \decke_N^i (t)   \\
  \phi(t) &\geq& \boden_N^i (t).
\end{eqnarray}

This holds true for all $i$ and all grids of size $N$ and hence, on
all parts of the domain $I$. 
Hence, $ \phi \in \einschluss, \forall
\phi \in \Phi$. In particular, $f \in \Phi$. Thus, $f \in \einschluss$.\\

3) We prove minimality of the enclosure. Let $g,h$ be functions such that the enclosure $\mathcal E := \mathcal E_g^h$ is exhaustive, i.e. satisfies Desideratum 2. Now, $\alpha_i^{\mathfrak u},\alpha_i^{\mathfrak l},\beta_i^{\mathfrak u},\beta_i^{\mathfrak l}$ are all $L_i$-Lipschitz continuous. Thus, $\decke_N,\boden_N$ are Lipschitz with the same constants. Owing to our assumption of exhaustiveness we therefore have: $\decke_N,\boden_N \in \mathcal E$. Hence, $g \leq \boden_N \leq \decke_N \leq h$. Hence, $\einschluss \subset \mathcal E$.

4) We show that each $\phi_N \in \einschluss$ converges uniformly to $f$, regardless of the identity of $f$, as long as $G_N$ converges to a dense subset of $I$ (or is an eventually dense partition of $I$). That is, we show $\forall \epsilon >0 \exists N_0 \forall N \geq N_0 \forall t \in I : \abs{\phi_N(t) - f(t)} \leq \epsilon$.

Let $\epsilon > 0$ and define $L := \max_{i=1,...,N-1} L_i$ to be the maximum Lipschitz constant among the intervals $J_1,...,J_N$. By Lem. \ref{lem:densegridmaxdist}, we know that there exists $N_0$ such that for all $N \geq N_0$, the distance between two consecutive points in grid $G_N$ is maximally $\delta:=\frac{\epsilon}{L}$. That is,
$\forall N \geq N_0 \forall i: b_i - a_i = |J_i| \leq \delta$. 

So, let $N \geq N_0$. 
Note, $\sup_{ t \in I} \abs{\phi_N(t) - f(t)} \leq \sup_{ t \in I} \abs{\decke_N(t) - \boden_N (t)} \leq \max_{i} \sup_{ t \in J_i} \abs{\decke_N^i(t) - \boden_N^i (t)}$
$\leq \max_{i}  \abs{\sup_{ t \in J_i}\decke_N^i(t) - \inf_{ t \in J_i} \boden_N^i (t)}$
$\stackrel{Lem. \ref{lem:ceiling_values}, Lem. \ref{lem:floor_values}}{=} \max_i \abs{ \bigl(\frac{f(b_i) +f(a_i)}{2} + L_i \frac{b_i-a_i}{2}  \bigr)- \bigl(\frac{f(b_i) +f(a_i)}{2} - L_i \frac{b_i-a_i}{2} \bigr)}$
$=\max_i \abs{ L_i (b_i-a_i) }$
$\leq \max_i \abs{ L_i \delta } = \delta \max_i L_i = \epsilon$.
Thus, $\forall t \in I: \abs{\phi_N(t) - f(t)} \leq \epsilon$.

\end{proof}

\end{thm}


==> content2/Ch_kinkyinf/est_multidim.tex <==

\section{Task 1 -- Conservative function estimation }
\label{sec:Hfe}
\textbf{Overview.} We desire to solve the conservative estimation problem (Task 1). As described above it can be described as a topological inference problem for which we will now design an optimal inference mechanism.  

In Sec. \ref{sec:targetest_multidim}, we derive computable H\"older ceiling and floor functions and prove that they satisfy the desiderata conservatism, convergence and optimality.  

To this end, we derive a number of upper and lower bound functions and show that these bound each function that is sample-consistent and H\"older continuous (hence, in particular, our target function). This constrains all H\"older continuous candidate functions that are sample-consistent, i.e. all H\"older functions that could have generated the (erroneous) sample set $D_n$. We then show how to convert these bounding constraints into our desired ceiling and floor functions $\decke_n, \boden_n$. Having established conservatism, we then establish optimality by realizing that $\decke_n$ and $\boden_n$ are indeed both H\"older functions that are sample consistent. Therefore, no tighter bounds can be found establishing optimality. Finally, we prove uniform convergence to the ground truth.

\jcom{--- EVTL RAUS:}
The section concludes with a discussion of the one-dimensional case in preparation of our elucidations in Sec. \ref{sec:quadr}. Among other things, we will find that in the one-dimensional case, $\decke_n$ and $\boden_n$ can be evaluated at substantially lower computation.\\

\subsection{Convergence properties}
We will construct function estimates that converge to the ground truth in the limit of large sample sets, provided the samples fulfil certain convergence properties themselves. To establish this in a rigorous manner, we need to review a few core convergence concepts. 
\begin{defn}[Uniform convergence of function sequences] Let $(\inspace, \metric_\inspace), (\outspace,\metric_\outspace)$ be two metric spaces.
For $n \in \nat$, let $f_n : I \to \Real$. $f_n \stackrel{n \to \infty}{\longrightarrow} f$ \emph{uniformly} (with respect to $\metric_\outspace$) if
\[  \forall \epsilon >0  \exists N_0 \in \nat \forall n\geq N_0 \forall x \in I: \metric_\outspace(f_n(x), f(x)) < \epsilon. \] 
\end{defn}

The key distinction between both variants of convergence is that in point-wise convergence, the convergence rate can depend on $x$. By contrast, in uniform convergence the rate is independent of function input $x$.


For our purpose the following definition of a dense set suffices:
\begin{defn}[Dense] Let $(\mathcal X,\metric)$ be a metric space.  
A set $D \subset \mathcal X$ is ($\metric$-) dense in a set $I \subset \mathcal X$ if every  $\metric-$ open subset of $I$ contains at least one point of $D$. That is:
$\forall x \in I, \epsilon > 0 \exists \xi \in D: \metric(\xi,x) < \epsilon$.     
\end{defn}


\begin{defn}[Uniform convergence of sequences of sets]\label{def:uniform_setconvergence}
Let $\bigl(\mathcal X,\metric\bigr)$ be a metric space.  
A sequence of sets $(Q_n)_{n \in \nat}$, $Q_n \subset \mathcal X$, $\abs{Q_n} < \infty$ converges to set $Q \subset \mathcal X$ \textit{uniformly} if we have:
\[\forall \epsilon > 0 \exists N_0 \in \nat \forall n \geq N_0 \forall q \in Q \exists q_n \in Q_n : \metric(q_n,q) < \epsilon. \]

If the sequence consists of finite sets, we can rewrite the condition as 
\[\forall \epsilon > 0 \exists N_0 \in \nat \forall n \geq N_0 \forall q \in Q : \min_{q_n \in Q_n} \metric(q_n,q) < \epsilon. \]

\end{defn}

In preparation for the derivations below, it will be useful to establish that uniform convergence to a dense subset of set $I$ implies uniform convergence to $I$ itself. Formally we express this as follows:

\begin{lem}
\label{lem:unifdenseset1}
Let $Q$ be a dense subset of $I$ and let $Q_n$ be a sequence of sets uniformly converging to $Q$ in the limit of $n \to \infty$. We have \[\forall e > 0 \exists N_0 \forall n \geq N_0 \forall x \in I \exists s \in Q_n: \metric(x,s) \leq e. \]


\begin{proof}
Let $e>0$, $N_0 \in \nat$ such that for all $n \geq N_0$ we have $\forall q \in Q \exists s_n(q) \in Q_n: \metric(s_n(q),q) \leq \frac{e}{2}$. 
Now, choose any $x \in I, n \geq N_0$. Since $Q$ is dense in $I$ we can choose $q \in Q$ such that $\metric(q,x) \leq \frac{e}{2}$. 
Hence, utilising the triangle inequality, we conclude $\metric(x,s_n(q)) \leq \metric(x,q) +\metric(q,s_n(q)) \leq \frac{e}{2} + \frac{e}{2} = e$.
\end{proof}
\end{lem}
An alternative statement of the lemma is that, under the lemma's premise, we have 

\[\forall e > 0 \exists N_0 \forall n \geq N_0 \forall x \in I : \inf_{s \in Q_n} \metric(x,s) \leq e. \]


\begin{defn} [``Eventually dense partition '']
For each $n \in \nat$ let $\mathcal P_n :=\{P_{n,1},...P_{n,n}\}$ be a partition of $I$ into subsets, each being a connected set and having the property that $P_{n,i}$ contains exactly one sample input $s_i$. Furthermore, let $r_{n,i} = \sup_{x,x' \in P_{n,i}} \frac{1}{2} \norm{x-x'}$ be $ P_{n,i}$'s ``radius'' w.r.t norm $\norm{\cdot}$. 
We call $(\mathcal P_n)_{n \in \nat}$ an \emph{eventually dense} partition sequence if the sequence $(r^*_n)$ of maximum radii, $r^*_n : = \max \{ r_{n,i} \}$, converges to zero as $n \to \infty$.

A sequence of inputs $(G_n)_{n \in \nat}$ will be called ``eventually dense'' if it is impossible to define a partition sequence separating the points in $G_n$ for each $n$ such that $G_n$ is not eventually dense.
\end{defn}
It should be clear that a sample grid that converges to a dense subset in $I$ is eventually dense (and vice versa).


It will become useful to remind ourselves of the standard fact that monotone sequences converge if they are bounded:
\begin{thm}[Monotone convergence theorem]
Let $(a_n)_{n \in \nat}$ be a monotone sequence of real numbers. That is, $a_n \geq a_{n+1}, \forall n \in \nat$ or $a_n \leq a_{n+1}, \forall n \in \nat$. The sequence converges to a finite real number if and only if the sequence is bounded. In particular, if the sequence is monotonically increasing then $\lim_{n \to \infty} a_n = \sup a_n$. If it is decreasing, we have $\lim_{n \to \infty} a_n = \inf a_n$.
\end{thm}
This theorem can be directly applied to prove the following result:
\begin{cor}
\label{cor:monseqfctsencl}
Let $(\phi_n)_{n \in \nat}$, $\phi_n : I \to \Real$ be a point-wise monotonically increasing sequence of functions and, let $(\gamma_n)_{n \in \nat}$, $\gamma_n : I \to \Real$ be a point-wise monotonously decreasing sequence of functions. That is, $\forall x \in I \forall n \in \nat: \phi_n(x) \leq \phi_{n+1}(x) \wedge \gamma_n(x) \geq \gamma_{n+1}(x) $. Furthermore, we assume $\forall x \in I \forall n \in \nat: \phi_n(x) \leq \gamma_{n}(x)$. 

Then, both sequences are point-wise convergent with point-wise limits 
$\lim_{n \to \infty} \phi_n (x) = \sup_{n \in \nat} \phi_n \leq \inf_{n \in \nat} = \lim_{n \to \infty} \gamma_n (x) $.
\end{cor}
The corollary will be needed below when we establish convergence of our function estimate bounds.

\subsubsection{Convergence with respect to the exponentiated metric}
\label{sec:unifconvhoeldermetricequivmetricunifconv}
The purpose of the next two results is to show that it does not matter whether one establishes a convergence property with respect to a metric $\metric$ or whether one does so with respect to the exponentiated $\metric^p$.
\begin{lem}\label{lem:hoeldermetricconv}
Let $p \in (0,1]$, $\mathcal X$ be a metric space and $(x_n)_{n \in \nat}$ be a sequence in $\mathcal X$ converging to $x \in \mathcal X$ with respect to metric $\metric$ iff the sequence converges to $x$ with reselect to metric $\metric^p$.

\begin{proof}
$\Rightarrow:$
Define the sequence $d_n :=  \metric(x_n,x) $.
Convergence with respect to $\metric$ means that $d_n \to 0$ as $n \to \infty$. Since $d_n \geq$ mapping $ \psi: \mathfrak x \mapsto \mathfrak x^p$ is well-defined for sequence inputs $d_n$. Furthermore, $\psi$ is a continuous function and thus, 
$\lim_{n \to \infty} \metric^p(x_n,x) = \lim_{n \to \infty} \psi(d_n) =  \psi( \lim_{n \to \infty} d_n) = \psi (0)  =0$.
Hence, $x_n$ converges to $x$ with respect to $\metric^p$ as well.
$\Leftarrow:$ Completely analogous.

\end{proof}  
\end{lem}

\begin{lem}\label{lem:hoeldermetricconv}
Let $p \in  (0,1]$, $\mathcal F$ be a metric space of functions. Sequence of functions $(f_n)_{n \in \nat}$ converges uniformly to $f$ with respect to metric $\metric$ iff the sequence also converges uniformly to $f$ with respect to metric $\metric^p$.


\begin{proof} $\Rightarrow:$
Since $f_n \to f$ uniformly, we have 
$\forall e >0 \exists N_e \geq 0 \forall n \geq N_e, x \in I : \metric(f_n , f) < e$. We show that also $\forall e >0 \exists N_e \geq 0 \forall n \geq N_e, x \in I : \metric(f_n , f)^p < e$.
Mapping $\psi: x \mapsto x^p$ invectively maps positive numbers onto the set of positive real numbers. Hence, $\metric(f_n, f) < e \Leftrightarrow \metric(f_n , f)^p < e^p$.
Let $e >0$ and $ \varepsilon := \sqrt[p]{e}$. Due to uniform convergence, we can choose $ N_\varepsilon$ such that $\forall x \in I, n \geq N_\varepsilon: \metric(f_n , f) <\varepsilon$ which is equivalent to stating $\forall x \in I, n \geq N_\varepsilon: \metric(f_n , f)^p <\varepsilon^p = e$. $\Leftarrow:$ Completely analogous.
\end{proof}  
\end{lem}




\subsection{Theoretical guarantees for kinky inference and learning}
\label{sec:targetest_multidim}

%\jcom{Talks about Lipschitz instead of Hoelder .. needs to be fixed}
%We assume the dimensionality of the target's input domain $I \subseteq \inspace$ is $d \geq 1$. 
 Remember, we defined the set of samples as $D_n= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N_n \} $. To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the grid of sample inputs contained in $D_n$.
Our exposition focusses on the case of one-dimensional output space. That is, $\outspace = \Real$.


In this subsection, we assume $\metric$ to be any suitable metric on the target function domain. For instance, we have seen that  $\metric(x,y) := \normtop{x-y}$ defines a proper metric and (uniform) convergence with respect to this metric is equivalent to (uniform) convergence with respect to metric $ D: (x,y) \mapsto \norm{x-y}$ (see Sec. \ref{sec:unifconvhoeldermetricequivmetricunifconv}). Also note, that Lipschitz continuity with respect to $\metric$ is H\"older continuity with respect to metric $D$. Therefore, we may use the terms Lipschitz continuity and H\"older continuity interchangeably if it is clear which metrics the terms refer to.
Furthermore, remember we are primarily interested in functions restricted to be Lipschitz with respect to $\metric$ and bounded by functions $\lbf,\ubf$. That is, we know the target is contained in $\mathcal K_{prior} = \lipset L \metric  \cap \bfset$ where $\lipset L \metric$ denotes the $L$- Lipschitz functions with respect to metric $\metric$ and $\bfset :=\{\phi : I \to \Real \, | \, \forall x \in I : \lbf(x) \leq \phi(x) \leq \ubf(x)\} $. 

%We will now define a data inference mechanism $M_{dinf}$ that maps the sample $D_n$ into a subset 
%
%\subsubsection{A priori knowledge} We assume, our  a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L[J]$ such that the underlying target $f \in \mathcal F$ is $L[J]-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L[J] \norm{x-x'}\}$.

%\subsubsection{Computing a posteriori knowledge}

\begin{defn}[Sample-consistent functions]
A function $\kappa: I \to \Real$ is called \textit{consistent with sample} $D_n$ (shorthand: \emph{sample-consistent}) if \[ \forall i \in \{1,\ldots,N_n\}: \kappa(s_i) \in [\tilde f_i - \varepsilon(s_i), \tilde f_i + \varepsilon(s_i)  ] =[\underline f(s_i),\overline f(s_i) ].\] The set of all sample-consistent functions on $I$ will be denoted by $\mathcal K(D_n)$.
\end{defn}
Informally speaking, $\mathcal K(D_n)$ contains all functions that could have created the sample set. Conversely, sample $D_n$ rules out all functions that are not sample-consistent as candidates for being the target. 

%In the lingo of our consideration on topological inference, $\mathcal K(D_n)$ embodies part of our posterior knowledge: $\mathcal K_{\text{post}} = \mathcal K(D_n)$. 





\begin{defn}[Enclosure]
Let $\decke,\boden: I \to \Real$ be two functions, such that $\decke
\geq \boden$ pointwise on $I$. We define their enclosure on $I$ as
the compact interval $\mathcal E^\decke_\boden (I)$ of all functions
between them. That is, \[\mathcal E^\decke_\boden (I) := \{\phi: I
\to \Real \vert \forall t \in I: \decke(t) \geq \phi(t) \geq
\boden(t) \}.\]
\end{defn}
For ease of notation we omit the domain argument whenever we refer
to $I$. That is, we write  $\mathcal E^\decke_\boden :=\mathcal
E^\decke_\boden (I)$.


An \emph{enclosure} is sample-consistent if it is contained in the set $\mathcal K(D_n)$ of sample-consistent functions. 

Based on the sample, we desire to find two
\emph{enclosing functions} $\decke_n: I \to \Real$, $\mathfrak
\boden_n: I \to \Real$ bounding the target from above and below that
are as tight as possible and converge to the target in the limit of
infinite, sample set size $N$. 
More formally, we would ideally like it to satisfy the following desiderata:

\begin{defn}[Desiderata] \label{defn:desiderata}
 Based on an observed, erroneous data set $D_n$, we desire to define enclosing functions $\decke_n, \boden_n$ that give rise to an enclosure $\einschluss$ with the following properties:

\begin{enumerate} 

    \item \textbf{Sample-Consistency}: The enclosure is sample-consistent, i.e. $\einschluss \subseteq \mathcal K(D_n)$.
		%The enclosing functions are sample-consistent, i.e. $\decke_n,\boden_n \in \mathcal K(D_n)$.
    
     \item \textbf{Exhaustiveness (conservatism)}: Every $\phi, \lbf \leq \phi \leq \ubf$ coinciding with target $f$ on with grid $G_n$ and
having at most Lipschitz
    constant $L[J]$ on every subset $J \subset I$ is also contained in the enclosure: $\forall \phi: I \to \Real, \phi \in \mathcal K_{prior} \cap \mathcal K(D_n): \phi \in \einschluss $. That is, $\mathcal K_{prior} \cap \mathcal K(D_n) \subseteq \einschluss$.
    In particular, the target is always contained in the enclosure: $f \in \einschluss$.

\item \textbf{Monotonicity:} Additional data does not increase uncertainy. That is,
if $G_n \subseteq G_{n+1} $, we have $\mathcal E^{\decke_{n+1}}_{\boden_{n+1}} \subseteq \einschluss, \forall n \in \nat$.
		   
\item \textbf{Convergence} to the target: Let the set of sample inputs $G_n$ in $D_n$ converge to a dense subset of domain $I$ and for each input $x \in I$ let the sample error function $\varepsilon: I \to \Real_{\geq 0}$ be bounded by $m_x \geq 0$ in some neighbourhood of $x$. Then, we have 
\begin{itemize}
\item (a) The sequence of enclosures converges point-wise. In particular, 

$\forall x \in I: 0 \leq \lim_{n \to \infty} \decke_n (x) -\boden_n(x) \leq 2 m_x$.
In particular, the enclosure converges to the target $f(x)$ at inputs $x$ where $m_x=0$.  
		
		\item (b) If convergence of $G_n$ is uniform and the target observations are error-free, i.e. $m_x = 0, \forall x \in I$, then the enclosure converges to the target $f$ uniformly.
\end{itemize}	
   \item \textbf{Minimality (optimality)}: 
If an enclosure $\mathcal E^b_a$  satisfies \emph{Desideratum 2} then it is a superset of our enclosure $\einschluss$, i.e. $b \geq \decke_n, a \leq \boden_n$, $\einschluss \subseteq \mathcal E^b_a$.    

\end{enumerate}

\end{defn}
 
Next, we will derive enclosing functions that give rise to such an enclosure.

\begin{defn}[Sample point ceiling and floor functions]
\label{def:sampleceilandfloormultidim}
Remember, $\overline f(s_i) = \tilde f_i + \varepsilon(s_i)$ and $\underline f(s_i) = \tilde f_i - \varepsilon(s_i)$.  For the $i$th sample ($i \in \{1,\ldots,N_n\}$, $L \geq 0$, $x \in I$, we define  
\begin{enumerate}
	\item The $i$th \emph{sample point ceiling} function: \[\decke_n^i (x; L) :x \mapsto  \overline f (s_i) +  \,L \, \metric(x, s_i), \]
	\item and the $i$th \emph{sample point floor} function: \[\boden_n^i (x; L) :x \mapsto  \underline f (s_i) -  \,L \, \metric(x, s_i) .\] 
\end{enumerate}
%Here $n_i$ is a norm-dependent constant ensuring that both functions are $L$-Lipschitz with repect to $\norm{\cdot}$. 
If constant $L$ is clear from the context, its explicit mention shall be omitted.
\end{defn}
%Note, for the maximum-norm $\norm{\cdot}_\infty$ it is easy to see that  $n_i =1$ renders both functions $L$-Lipschitz. For the 1-norm, one can either utilize Lipschitz arithmetic to show that for $n_i=1$ the functions would be $d L$-Lipschitz or, one can leverage the well-known inequality~\cite{koenigsberger:2000}   $\norm{\cdot}_1 \leq d \norm{\cdot}_\infty$ to determine $n_i := \frac{1}{d}$.

We show that these functions give rise to enclosures that satisfy the first three Desiderata of Def. \ref{defn:desiderata}:
\begin{lem} 
\label{lem:samplefloorceiling}
Let  $i \in \{1,...,N_n\}$.
Enclosure $\mathcal E^{\decke_n^i}_{\boden_n^i}$ is (i) consistent with the $i$th sample and (ii) conservative. 
More specifically: 

(i)  \[\forall i \in \{1,...,N_n\}, \phi \in \mathcal E^{\decke_n^i}_{\boden_n^i}:  \phi(s_i) \in [\underline f(s_i), \overline f(s_i)].\]

(ii) If target $f: I \to \Real$ is $L$-Lipschitz on $J \subset I$ with respect to metric $\metric$ then the corresponding sample ceilings are upper bounds and the sample floor functions are lower bounds. That is, for $i =1,\ldots, N$, $\forall x \in J$ we have \[\decke_n^i (x; L) \geq f(x)  \geq  \boden_n^i (x; L).\]

\begin{proof}
(i) Follows directly from the definitions.
(ii) We show the first inequality, $\decke_n^i (x; L) \geq f(x)$. (The proof of the second inequality,  $f(x)  \geq  \boden_n^i (x; L)$, is completely analogous.) 

Due to Lipschitz continuity, we have 
$\forall x,x' \in J: \abs{f(x) - f(x')} \leq L \metric(x,x').$
In particular, 
$\forall x \in J: f(x) - f(s_i) \leq\abs{f(x) - f(s_i)} \leq L \, \metric(x, s_i).$
Hence, 
$\forall x \in J: f(x)  \leq f(s_i) + L \, \metric(x, s_i)$ 
$\leq \tilde f(s_i) +\varepsilon(s_i) + L \, \metric(x, s_i) = \decke_n^i (x; L)$.

%Since $\decke_n^i (x; L)  = \tilde f_i + \varepsilon(s_i) + L_i \metric(x, s_i)$, this entails $\decke_n^i (x; L) \geq f(x)$ for all $\varepsilon(s_i) \geq 0$. Therefore, it suffices to focus on the case for $\varepsilon(s_i) =0$.
 %So, let $\varepsilon(s_i) =0$. 

%&\leq f(c_i) + \ell_i \normtop{x-c_i}_{\infty}:= \decke^i_n(x)
%\end{align}
%where $\ell_i = \sqrt d L_i$ is a Lipschitz constant for the max-norm.
%The last inequality is due to the well-known relationship 
%$\normtop{x}_\infty \leq \normtop{x}_2 \leq \sqrt{d} \, \normtop{x}_\infty $.



\end{proof}
\end{lem}



\begin{defn}[Lipschitz enclosure] On  $J \subset I$, define the \emph{optimal ceiling} as
\[\decke^*_n (x; L) : x \mapsto  \min_{i=1,\ldots,N_n} \decke^i_n(x;L)\]
and the \emph{optimal floor function} as
 \[\boden^*_n (x; L) :x \mapsto   \max_{i=1,\ldots,N_n} \boden^i_n(x; L).\]
The enclosure $\einschluss$ with enclosing function choices $\decke_n := \decke_n^*$ and $\boden_n := \boden_n^*$ will be called ``Lipschitz enclosure'' and be denoted by $\opteinschluss$.
If constant $L$ is fixed and clear from the context we may omit its explicit mention from the syntax.
\end{defn}
An example for a Lipschitz enclosure is depicted in Fig. \ref{figlipencl_nonoise_neo}.
\begin{figure*}
%
	\centering
		\includegraphics[scale = .4]{content/content_hoelderquad2/figs/enclosure.pdf}
	\caption{Example of an enclosure (for metric $\metric: (x,y) \mapsto \norm{x-y}$) for a given sample of function values on one-dimensional domain $I = [0,2.5]$. The Lipschitz constant was one, uniformly over the entire domain. The samples were noise-free.}
	\label{figlipencl_nonoise_neo}
\end{figure*}

Before we can prove that the optimal functions are indeed optimal, we need to undergo some derivative preparations.

\begin{lem} \label{lem:optenclcontainstarget}
The Lipschitz enclosure always contains the target. That is, $\decke^*_n(x) \geq f(x) \geq \boden^*_n(x), \forall x \in I, n \in \nat$.
\begin{proof}
This is a direct consequence of Lem. \ref{lem:samplefloorceiling}.
\end{proof}
\end{lem}


\begin{thm}
Choosing $\decke_n := \min\{ \decke_n^*, \ubf\}$ and $\boden_n := \max\{\boden_n^*,\lbf\}$ yields an enclosure $\einschluss$ that satisfies Desiderata 1-5 specified in Def. \ref{defn:desiderata}.
\begin{proof}
We bear in mind that $\einschluss = \bfset \cap \opteinschluss$.

\textit{1) Consistency}. By definition of $\decke_n^*$ and $\boden_n^*$ in conjunction with Lem. \ref{lem:samplefloorceiling}.(i) we see that $\opteinschluss = \cap_i \mathcal E_{\boden_n^i}^{\decke_n^i} \subseteq \mathcal K(D_n)$. Desideratum 1 follows from $\einschluss = \bfset \cap \opteinschluss \subseteq \opteinschluss$.\\

\textit{2) Conservatism}. By definition of $\decke_n^*$ and $\boden_n^*$ in conjunction with Lem. \ref{lem:samplefloorceiling}.(ii) we have $\mathcal K(D_n) \cap \lipset L \metric \subseteq \opteinschluss $. Hence, $\mathcal K_{prior} \cap \mathcal K(D_n) =  \bfset \cap \lipset L \metric \cap \mathcal K(D_n) \subseteq \opteinschluss \cap \bfset = \einschluss$ proving
Desideratum 2.

\textit{3) Monotonicity.} 

This follows directly from the way the ceiling and floor functions are defined. Considering the ceiling:
We have $\decke_n (x) = \min\{\ubf,\min_{i =1,...,N_n} \decke^i_{n}(x) \} $. W.l.o.g., for $i=1,\ldots,N_n$, let $\decke_n^i = \decke_{n+1}^{i}$. 

Then 
$\decke_{n+1} (x) = \min\{\ubf(x),\min\Bigl\{ \min_{i =1,...,N_n} \decke^i_{n}(x), \min_{i= N_n +1,\ldots,N_{n+1}}  
\decke^i_{n+1}(x) \Bigr\} \} $

$\leq \min \{\ubf(x), \min_{i =1,...,N_n} \decke^i_{n}(x)  \}=  \decke_{n}(x) $. Statement $\boden_{n+1} (x) \geq  \boden_{n}(x)$ follows analogously.

\textit{4 a) Pointwise convergence.} In absence of errors, one could show pointwise convergence by utilising Cor. \ref{cor:monseqfctsencl} --which is applicable due to Lem. \ref{lem:samplefloorceiling} in conjunction with 3). We will now prove the more general statement in the presence of observational errors $\varepsilon$.

Pick an arbitrary $x \in I$ such that the error $\varepsilon(\xi) \leq m_x$ for all $\xi$ in some $\epsilon-$ball $\mathcal U_\epsilon(x) = \{\xi \in I | \metric(\xi ,x) < \epsilon \}$ around $x$.
It remains to be shown that $\lim_{n\to \infty} \decke_n(x) - \boden_n(x) \leq 2 m_x$ for inputs $x$.
Define $L := \sup_{J \subset I} L[J] $  to be the maximum Lipschitz constant on the domain.
Let $e>0$ be arbitrary. We show that there exists $N_0 \in \nat$ such that for all $n \geq N_0: \decke_n(x;L) - \boden_n(x;L) \leq e + 2 m_x$ as follows:

Since we assume $G_n$ converges to a dense subset of $I$, Lem. \ref{lem:hoeldermetricconv} applies. Hence, there is $N_0 \in \nat$ such that $\forall n \geq N_0 \exists i \in \{1,...,N_n\}: s_i \in \mathcal U_{e/2L}(x) = \{\xi \in I | \metric(x,\xi) < \frac{e}{2L}\}$.
 
So, choose $n \geq N_0$. 
Hence, $L \metric(x,s_j)  < \frac{e}{2}, \,\varepsilon(s_q) \leq m_x \hspace{1cm} \text{ (*)}$ 

where 
$q \in \arg\min_{i \in \{1,...,N_n\} } L \, \metric(x,s_i) $. 
We have:

 $\decke_n^*(x;L) - \boden_n^*(x;L)$ 

$= \min_{i \in \{1,...,N_n\} } L \, \metric(x,s_i) + \tilde f(s_i) + \varepsilon(s_i) - \max_{i \in \{1,...,N_n\} }  \tilde f(s_i) - \varepsilon(s_i) - L \metric(x,s_i) $

$= \min_{i \in \{1,...,N_n\} } \bigl\{L \, \metric(x,s_i) + \tilde f(s_i) + \varepsilon(s_i) \bigr\}+ \min_{i \in \{1,...,N_n\} }  \bigl\{-\tilde f(s_i) + \varepsilon(s_i)+ L \, \metric(x,s_i)\bigr\} $

$\leq \min_{i \in \{1,...,N_n\} } \bigl\{L \, \metric(x,s_i) + \tilde f(s_i) + \varepsilon(s_i)    -\tilde f(s_i) + \varepsilon(s_i)+ L \metric(x,s_i) \bigr\}$

$=2\min_{i \in \{1,...,N_n\} } L \, \metric(x,s_i) + \varepsilon(s_i) $
$\leq 2 L \, \metric(x,s_q)+ 2\varepsilon(s_q) $
$\stackrel{(*)}{<} e + 2 m_x  $.\\
As a special case, in the noise free setting with  $m_x=0$, this result implies that the enclosure shrinks to a single value as $n \to \infty$. That this value is $f(x)$ follows from Lem. \ref{lem:optenclcontainstarget}.  \\

We have shown convergence of $\decke_n^*(x;L) - \boden_n^*(x;L)$. Convergence of $\decke_n(x) - \boden_n(x) = \min\{\ubf(x), \decke_n^*(x)\} - \max\{\lbf(x),\boden_n^*(x)\}$ follows by continuity of the $\max$ and $\min$ operation.


 \textit{4 b) Uniform convergence.}
Let $G_n = \{s_1,\ldots,s_{N_n}\}$ denote the $N_n$-sample input grid which we assume to converge uniformly to a dense set of domain $I$. 
Assuming $m_x =0$, we desire to show that $\forall e >0 \exists N_0 \forall n \geq N_0 , x \in I : \abs{ \decke_n(x) - f(x)} < e $ and $\forall e >0 \exists N_0 \forall n \geq N_0 , x \in I : \abs{ \boden_n(x) - f(x)} < e $.
Let $e > 0$.
 %and define $L := \sup_{J \subset I} L[J] $  to be the maximum Lipschitz constant on the domain and $n$ the corresponding normalization constant making the target $L$-Lipschitz. 
Let $G_n$ converge uniformly to a dense subset  $G \subset I$. By Lem. \ref{lem:unifdenseset1}, we know that 
there exists $N_0$ such that for all $n \geq N_0$ and all $x \in I$ there is a $q \in G_n$ such that $\metric(x,q) < \frac{e}{2  L}$. 
In particular, $ L \, \metric(s_q ,x ) < \frac{e}{2}$ where we define $q \in \arg\min_{i} \metric(s_i ,x )$. 
Hold such $N_0$ fixed, choose arbitrary $n \geq N_0$ and $x \in I$. 

Firstly, we show that each $\decke_n$ converges uniformly to $ f$ by showing $\abs{\decke_n(x) - f(x) }< e$.

We have
$\abs{\decke_n(x) - f(x)} \stackrel{2)}{=} \decke_n(x) - f(x) $  
$\stackrel{def.}{\leq}\min_{i} \decke^i_n(x) - f(x) $
$\leq   \decke^q_n(x) - f(x) $
$\stackrel{def.}{\leq}  L \, \metric(x,s_q)+f(s_q) - f(x) $
$\leq  L \, \metric(x,s_q)+ \abs{f(s_q) - f(x) }$
$\stackrel{f \text{ L-Lip.}}{\leq}  L \, \metric(x,s_q)+   L \, \metric(x,s_q) <  e$ where in the last step we have leveraged $L \, \metric(x,s_q) < \frac{e}{2}$.

Secondly, we show the analogous for the floor. 
That is we show  $\abs{\boden_n(x) - f(x) }< e$:


$\abs{  \boden_n(x) - f(x)}\stackrel{2)}{=} f(x) - \boden_n(x) $  
$\stackrel{def.}{\leq} f(x) - \max_{i} \boden^i_n(x) $
$\leq   f(x)- \boden^q_n(x)  $
$\stackrel{def.}{\leq} f(x) - (f(s_q) -  L \, \metric(x,s_q))  $
$\leq  L \, \metric(x,s_q)+ \abs{f(s_q) - f(x) }$
$\leq  L \, \metric(x,s_q)+   L\, \metric(x,s_q) < 2 \frac{e}{2}= e$ where, as before, in the last step we have utilised $ L \, \metric(x,s_q) < \frac{e}{2}$.\\

\textit{5) Optimality.}  By Lem. \ref{lem:Hoeldarithmetic}.(6) we know that $\decke_n^*,\boden_n^* \in \lipset L \metric$. Hence, $\decke_n , \boden_n \in \lipset L \metric \cap \bfset$. 
Thus, if $\lipset L \metric \cap \bfset \subset \mathcal E^b_a $ then also $\decke_n, \boden_n \in \mathcal E^b_a$. This implies $\decke_n \leq b, \boden_n \geq a$, i.e. $\einschluss \subseteq \mathcal E^b_a$.
\end{proof} 
\end{thm}

%So far, our guarantee of optimality of the enclosure only holds for $p=1$. This is due to the fact that at present, we cannot guarantee that the minimum of two $p-L-$H\"older functions also is $p-L-$ H\"older, unless $p=1$. Intuitively, this might well be true also for $p<1$, but investigating this rigorously has to be deferred to future work.


\subsubsection{Pruning of uninformative sample points}

The remaining derivations of this subsection show how the data can be pruned when new data points arrive the render old ones uninformative. They can be skipped by a reader not interested in the details.


We will focus our exposition on the ceiling functions. The derivations for the floor functions are entirely analogous (where one has to substitute $\leq$ by $\geq$ and $\min$ by $\max$).

\begin{lem}\label{lem:dominatedsamplefct}
Let $\mathcal N := \{1,...,N_n\}$, $q,i \in \mathcal N$ be the indices of a sample ceiling functions $\decke_n^q(\cdot;L_q)$ and $\decke_n^i(\cdot;L_i)$ where $L_q \leq L_i$ everywhere. We have
\[\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i) \Leftrightarrow \forall t \in I: \decke_n^q(t;L_q) \leq \decke_n^i(t;L_i).\]
\begin{proof}
$\underline \Rightarrow:$
$\decke_n^q (t;L_q) = \decke_n^q(s_q;L_q) + L_q \metric(t, s_q)$
$\leq \decke_n^q(s_q;L_q) +L_q \metric(s_i, s_q)+ L_q\metric(t,s_i) $
$=\decke_n^q(s_i;L_q) +  L_q\metric(t,s_i)$ 
$\leq \decke_n^i(s_i;L_i) + L_q\metric(t,s_i)  $
$= \overline f(s_i) + L_q\metric(t,s_i)    $
$\leq \overline f(s_i) + L_i\metric(t,s_i)    = \decke_n^i(t;L)$.\\
$\underline \Leftarrow:$ Trivial.
\end{proof}
\end{lem}

The lemma implies that we can remove samples that are dominated by other samples' ceiling functions:
\begin{thm} 
\label{thm:removedominatedsamples}
Let $\mathcal N := \{1,...,N_n\}$ and let $i \in \mathcal N$ be the index of sample ceiling function $\decke_n^i(\cdot;L_i): t \mapsto \overline f(s_i) + L_i \abs{t - s_i}$. If there exists a sample ceiling function $u^q(\cdot;L_q), q \in \mathcal N \backslash \{i\}$, $L_q \leq L_i$ everywhere, having a value below $\decke_n^i$ at the $i$th sample, then the $i$th sample plays no role in computing the optimal ceiling. That is:\\  
If there is $q \in \mathcal N \backslash\{ i\}$ such that $\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i)$, then we have: \\
$\decke^*(t;L_1,\ldots,L_n) = \min_{j \in \mathcal N} \decke^j(t;L_j) =  \min_{j \in \mathcal N\backslash \{i\}} \decke^j(t;L_j)$.
\begin{proof}
The theorem is a direct consequence of Lem. \ref{lem:dominatedsamplefct}. 
\end{proof}

\end{thm}

\begin{rem}
Normally, $L_i = L_q\, \forall q,j \in \mathcal N$ where each $L_i$ is a function mapping $t$ to a H\"older constant valid in some neighbourhood of $t$.
\end{rem}

\begin{thm}
\label{thm:dominatedsamples_greatLIPconst}
Let $\mathcal N := \{1,...,N_n\}$ and let $i \in \mathcal N$ be the index of sample ceiling function $\decke_n^i(\cdot;L_i): t \mapsto \overline f(s_i) + L_i \metric(t,s_i) $. We have: \\if $\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i)$ then 
\[  \decke^*(t;L_1,...,L_n) \geq \min_{j \in \mathcal N} \decke^j(t;L_j) =  \min \bigl\{ \min_{j \in \mathcal N\backslash \{i\}} \decke^j(t;L_j), \decke_n^q(s_i) + L_i \metric(t,s_i) \bigr\}.\]

\begin{proof} Let $\decke_n^q(s_i;L_q) \leq \decke_n^i(s_i;L_i)$ and $L_q > L_i $ everywhere. Since $\decke_n^q(s_i) \leq \decke_n^i(s_i)$ and $L_i < L_q$ we have $\decke_n^i(t;L_i) = \overline f(s_i) + L_i \metric(t,s_i) $
$= \decke_n^i(s_i;L_i) + L_i \metric(t,s_i)$
$\geq \decke_n^q(s_i;L_i) + L_i \metric(t,s_i)$.

\end{proof}

\end{thm}

\begin{rem} \label{rem:assumptionsceil}
The theorems allow us to assume, without loss of generality, that $\decke_n^i(s_i) = \min_j \decke_n^j(s_i)$ (as a preprocessing step, Thm. 
\ref{thm:removedominatedsamples} allows us to remove samples violating this assumption, without changing the optimal ceiling). 
\end{rem}



\subsection{Special case: one-dimensional inputs, p=1}
For functions on one-dimensional domains and exponent $p=1$, matters simplify. We assume $\metric(x,y) := \abs{x-y}$. This case has been considered in the context of optimisation \cite{Shubert:72} and quadrature \cite{Baran2008}.

%From now on, we will assume that $L_1,\ldots, L_n =: L$. 

For ease of notation we will therefore often omit explicit mention of $L$ in the statements of the ceiling and floor functions, unless it becomes necessary. Additionally, we assume, without loss of generality, that the sample inputs are ordered such that $s_1\leq \ldots \leq s_n$. Let $b := \sup I $ and $a := \inf I$.



Under these assumptions, we next show that computing the optimal ceiling function only requires taking into account the up to two most adjacent samples :

\begin{lem}\label{lem:shieldingsamples_1d}
Let the assumptions of Rem. \ref{rem:assumptionsceil} hold.

We have:

\begin{enumerate}
\item $\forall i \in \mathcal N, t \geq s_i: \decke_n^* ( t) =\min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N, j \geq i\}, $	
\item $\forall i \in \mathcal N, t \leq s_i: \decke_n^* ( t) =\min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N,j \leq i\}.$ 
\end{enumerate}

\begin{proof}
1.) Let $t \geq s_i$. 

$\text{Showing} \leq:$ This is trivial since $\decke_n^*(t) = \min_{j \in \mathcal N} \decke_n^j(t) \leq \min_{j \in \mathcal N, j \geq i}\decke_n^j(t)$. 


$\text{Showing} \geq:$ For contradiction, assume $\decke_n^* ( t) < \min_{j\geq i} \decke_n^j(t).$ 
Hence, there is a $q \in \mathcal N, q < i$ such that 

\begin{equation}
\label{eq:lala1}
\forall t \geq s_i: \decke_n^q(t) < \min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N, j \geq i\}.
\end{equation}
%Again, utilizing $s_i \leq t \leq s_{i+1}$ this is equivalent to $\exists q : \decke_n^q(t) < \overline f(s_i) + L \abs{t - s_i} \wedge \decke_n^q(t) < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$
%
%$\stackrel{def.}{\Leftrightarrow} \exists q : \overline f(s_q) + L \abs{t - s_q} < \overline f(s_i) + L \abs{t - s_i} \wedge f(s_q) + L \abs{t - s_q} < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$.
Choose such a $q \in \mathcal N, q < i$.
By assumption, we have $s_q < s_i$. Hence, Condition \ref{eq:lala1} implies in particular $\decke_n^q(t) = \overline f(s_q) + L (t - s_q) < \decke_n^i(t) = \overline f(s_i) + L (t - s_i)$. We have $\overline f(s_q) + L (t - s_q) = \overline f(s_q) + L (s_i - s_q) + L (t - s_i) = \decke_n^q(s_i) + L (t-s_i) \stackrel{!}{ <} \overline f(s_i) + L (t-s_i)=\decke_n^i(s_i) + L (t-s_i) $ which holds, if and only if $\decke_n^q(s_i) < \decke_n^i(s_i)$. However, the last inequality contradicts our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (Rem. \ref{rem:assumptionsceil}).\\

2.) The proof is analogous to 1.):

Let $t \leq s_i$. 

$\text{Showing} \leq:$ This is trivial since $\decke_n^*(t) = \min_{j \in \mathcal N} \decke_n^j(t) \leq \min_{j \in \mathcal N, j \leq i}\decke_n^j(t)$. 


$\text{Showing} \geq:$ For contradiction, assume $\decke_n^* ( t) < \min_{j\leq i} \decke_n^j(t).$ 
Hence, there is a $q \in \mathcal N, q > i$ such that 

\begin{equation}
\label{eq:lala2}
\forall t \leq s_i: \decke_n^q(t) < \min\{  \decke_n^j (t) \,\vert \, j \in \mathcal N, j \leq i\}.
\end{equation}
%Again, utilizing $s_i \leq t \leq s_{i+1}$ this is equivalent to $\exists q : \decke_n^q(t) < \overline f(s_i) + L \abs{t - s_i} \wedge \decke_n^q(t) < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$
%
%$\stackrel{def.}{\Leftrightarrow} \exists q : \overline f(s_q) + L \abs{t - s_q} < \overline f(s_i) + L \abs{t - s_i} \wedge f(s_q) + L \abs{t - s_q} < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$.
Choose such a $q \in \mathcal N , q > i$ (thus, $s_q > s_i$).


The way we ordered the samples, $q>i$ implies $s_q > s_{i}$. Thus, Condition \ref{eq:lala2} implies in particular: $\decke_n^q(t) =\overline f(s_q) + L (s_q -t ) < \decke_n^i(t) = \overline f(s_{i}) + L ( s_{i} -t) = \decke_n^{i}(s_{i}) + L ( s_{i} -t)$. We have $\overline f(s_q) + L (s_q-t) = \overline f(s_q) + L (s_q - s_{i} ) + L (s_{i} - t) = \decke_n^q(s_{i}) + L (s_{i} - t) \stackrel{!}{ <} \decke_n^{i}(s_{i}) + L (s_{i} -t) $. However, the last inequality contradicts our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (made in Rem. \ref{rem:assumptionsceil}).



%By definition of the sample ceilings, it follows 
%$\exists q : \decke_n^q(t) < \decke_n^i(t) \wedge \decke_n^q(t) < \decke_n^{i+1} (t)$.
\end{proof}

\end{lem}


The Lemma allows us to tremendously simplify computation of the optimal ceiling-- it tells us that all samples, except the up to two neighbouring ones, can be discarded when computing the optimal ceiling at a given input:

\begin{thm}\label{thm:lipceil1d}
Let the assumptions of Rem. \ref{rem:assumptionsceil} hold.
Let $a:=s_0: = \inf I, s_{n+1} := b:=\sup I$ and for $i=0,\ldots,N_n$ define $I_i := [s_i,s_{i+1}]$.

%we define line segments via \[\alpha^\decke_n_i: t
%\mapsto \overline f(s_i) + L (t - s_i)\] and \[\beta^\decke_n_i: t \mapsto
%\overline f(s_{i+1}) -L (t - s_{i+1}).\] 

We have:

\[ \forall i, t \in I_i: \decke_n^*(t) = \begin{cases} \decke_n^{i+1}(t) &, i=0\\
															\min\{\decke_n^i(t),\decke_n^{i+1}(t) \}&, i \in \{1,\ldots,N_n-1 \} \\
															\decke_n^{i}(t)&, i=N.	\end{cases} \]


\end{thm}



The analogous statement for the H\"older floor function can be derived completely analogously and will therefore be given at this point without proof:


\begin{thm}\label{thm:lipfloor1d}
Assume the assumptions of Rem. \ref{rem:assumptionsceil} hold.
Let $a:=s_0: = \inf I, s_{n+1} := b:=\sup I$ and for $i=0,\ldots,N_n$ define $I_i := [s_i,s_{i+1}]$.

%we define line segments via \[\alpha^\boden_i: t
%\mapsto \overline f(s_i) + L (t - s_i)\] and \[\beta^\boden_i: t \mapsto
%\overline f(s_{i+1}) -L (t - s_{i+1}).\] 

We have:

\[ \forall i, t \in I_i: \boden_n^*(t) = \begin{cases} \boden_n^{i+1}(t) &, i=0\\
															\max\{\boden_n^i(t),\boden_n^{i+1}(t) \}&, i \in \{1,\ldots,N_n-1 \} \\
															\boden_n^{i}(t)&, i=N.	\end{cases} \]


\end{thm}

In addition to saving computation by discarding irrelevant samples, the the theorems will play an important role when computing a closed-form the integral of the optimal ceiling and floor functions.


%\begin{cor}\label{cor:lipceil}
%Assume the assumptions of Rem. \ref{rem:assumptionsceil} hold.
%On interval $I_i = [s_i,s_{i+1}]$ we define line segments via \[\alpha^\decke_n_i: t
%\mapsto \overline f(s_i) + L (t - s_i)\] and \[\beta^\decke_n_i: t \mapsto
%\overline f(s_{i+1}) -L (t - s_{i+1}).\] 
%
%We have:
%
%\begin{enumerate}
%\item
%For $i \in \mathcal N$ the projection of the optimal H\"older ceiling onto interval $I_i$ can be computed as the point-wise minimum of $\alpha^\decke_n_i$ and $ \beta^\decke_n_i$:
%\[\forall t \in I_i: \decke_n^* ( t) =\min\{ \alpha^\decke_n_i(t), \beta^\decke_n_i(t) \}= \min\{\decke_n^i(t),\decke_n^{i+1}(t) \} .\] 
%
%\item $\forall t \in [a,s_1], \tau \in [s_n,b] : \decke_n^*(t) = \decke_n^1(t) \wedge  \decke_n^*(\tau) = \decke_n^N(\tau)$.
%\end{enumerate}
%\begin{proof}
%1.) Since $s_i \leq t \leq s_{i+1}$, $\alpha^\decke_n_i(t) = \decke_n^i(t)$ and $\beta^\decke_n_i(t) = \decke_n^{i+1}(t)$.
%Let $t \in I_i$.
%
%$\text{Showing} \leq:$ By definition, $\decke_n^*(t) = \min_j \decke_n^j(t) = \min_j \overline f(s_j) + L \abs{t - s_j}  \leq \min\{\overline f(s_i) + L \abs{t - s_i}, \overline f(s_{i+1}) + L \abs{t - s_{i+1}} \} = \min\{\overline f(s_i) + L (t - s_i), \overline f(s_{i+1}) - L  (t-s_{i+1}) \}$ where the last equality holds owing to $s_i \leq t \leq s_{i+1}$.
%
%$\text{Showing} \geq:$ For contradiction, assume $\decke_n^* ( t) <  \min\{\overline f(s_i) + L (t - s_i), \overline f(s_{i+1}) - L  (t-s_{i+1}) \}$. This implies the existence of a $q \in \mathcal N$ such that 
%
%\begin{equation}
%\label{eq:lala1}
%\decke_n^q(t) < \overline f(s_i) + L (t - s_i)
%\end{equation}
%and 
%\begin{equation}
%\label{eq:lala2}
 %\decke_n^q(t) < \overline f(s_{i+1}) - L  (t-s_{i+1}). 
%\end{equation}
%%Again, utilizing $s_i \leq t \leq s_{i+1}$ this is equivalent to $\exists q : \decke_n^q(t) < \overline f(s_i) + L \abs{t - s_i} \wedge \decke_n^q(t) < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$
%%
%%$\stackrel{def.}{\Leftrightarrow} \exists q : \overline f(s_q) + L \abs{t - s_q} < \overline f(s_i) + L \abs{t - s_i} \wedge f(s_q) + L \abs{t - s_q} < \overline f(s_{i+1}) + L  \abs{t-s_{i+1}}$.
%Choose such a $q \in \mathcal N$.
%
%Case A: Let $s_q < s_i$. Then, Condition \ref{eq:lala1} implies $\decke_n^q(t) = \overline f(s_q) + L (t - s_q) < \overline f(s_i) + L (t - s_i)$. We have $\overline f(s_q) + L (t - s_q) = \overline f(s_q) + L (s_i - s_q) + L (t - s_i) = \decke_n^q(s_i) + L (t-s_i) \stackrel{!}{ <} \overline f(s_i) + L (t-s_i)=\decke_n^i(s_i) + L (t-s_i) $ which holds, if and only if $\decke_n^q(s_i) < \decke_n^i(s_i)$. However, the last inequality contradicts our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (Rem. \ref{rem:assumptionsceil}).
%
%Case B: Let $s_q > s_{i+1}$. Then, Condition \ref{eq:lala2} implies $\overline f(s_q) + L (s_q -t ) < \overline f(s_{i+1}) + L ( s_{i+1} -t) = \decke_n^{i+1}(s_{i+1}) + L ( s_{i+1} -t)$. We have $\overline f(s_q) + L (s_q-t) = \overline f(s_q) + L (s_q - s_{i+1} ) + L (s_{i+1} - t) = \decke_n^q(s_{i+1}) + L (s_{i+1} - t) \stackrel{!}{ <} \decke_n^{i+1}(s_{i+1}) + L (s_{i+1} -t) $. However, the last inequality contradicts our our assumption of $\min_j \decke_n^j(s_i) =\decke_n^i(s_i)\,\forall i$ (made in Rem. \ref{rem:assumptionsceil}).
%We have proven the first claim.\\
%
%2.) 
%
%%By definition of the sample ceilings, it follows 
%%$\exists q : \decke_n^q(t) < \decke_n^i(t) \wedge \decke_n^q(t) < \decke_n^{i+1} (t)$.
%\end{proof}
%
%\end{cor}



In preparation for the part on quadrature it will prove useful to determine the extrema of the enclosing functions on each subinterval $I_i$.


\begin{lem} \label{lem:Lipbetweensamples}
We have:
\begin{enumerate}
\item If $\decke^i(s_i)  \leq \decke^{i+1}(s_i)$ and $\decke^{i+1}(s_{i+1})  \leq \decke^i(s_{i+1})$ then 
we have 

$ \abs{\overline f(s_{i+1})- \overline f(s_i)} \leq L \abs{s_{i+1} -s_i}$.
\item If $\boden^i(s_i)  \geq \boden^{i+1}(s_i)$ and $\boden^{i+1}(s_{i+1})  \geq \boden^i(s_{i+1})$ then 
we have

$ \abs{\underline f(s_{i+1})- \underline f(s_i)} \leq L \abs{s_{i+1} -s_i}$.
\end{enumerate}

\begin{proof}
1.) 
On the one hand, we have:
$\decke^i(s_i)  \leq \decke^{i+1}(s_i)$ 
$\Leftrightarrow$
 $\decke^i(s_i) - \decke^{i+1}(s_i)  \leq 0$
%
$\Leftrightarrow$ $ \overline f(s_i) + L \abs{s_i-s_i} -\overline f(s_{i+1}) - L \abs{s_i-s_{i+1}}  \leq 0$
%
$\Leftrightarrow$ $ \overline f(s_i) -\overline f(s_{i+1}) - L \abs{s_i-s_{i+1}}  \leq 0$
%
$\Leftrightarrow$ $ \overline f(s_i) -\overline f(s_{i+1})   \leq  L \abs{s_i-s_{i+1}}$

$\Leftrightarrow$ $ \overline f(s_{i+1})-\overline f(s_i)    \geq  -L \abs{s_{i+1} - s_i}$.\\
%
On the other hand:
$\decke^{i+1}(s_{i+1})  \leq \decke^i(s_{i+1})$
%
$\Leftrightarrow$ $\decke^{i+1}(s_{i+1}) - \decke^i(s_{i+1}) \leq 0$
$\Leftrightarrow$ $\overline f(s_{i+1})  - \overline f(s_i) - L \abs{s_{i+1} -s_i} \leq 0$
$\Leftrightarrow$ $\overline f(s_{i+1})  - \overline f(s_i)  \leq  L \abs{s_{i+1} -s_i}$.

2.) The proof is completely analogous to 1.). 
\end{proof}
\end{lem}

\begin{lem} \label{lem:ceiling_maxvalues}
Let $\metric(x,y) := \abs{x-y}$. For $i \in \{1,\ldots,N_n-1\}$ let  $L_i > 0$, $I_i = [s_i,s_{i+1}]$.
Define $\xi^{\mathfrak u}_i :=  \frac{s_i+s_{i+1}}{2}+ \frac{\overline f(s_{i+1}) - \overline f(s_i)}{2 L_i}  $.\\
For $t \in I_i$ we have 
\begin{enumerate}
\item $\xi^{\mathfrak u}_i \in I_i$ and  $\decke^*_n(t) = 
 \begin{cases}  
 \decke^i_n (t), & t \leq \xi^\decke_i \\
 \decke^{i+1}_n(t), & t \geq \xi^\decke_i.
 \end{cases}$
\item $\xi^{\mathfrak u}_i \in \arg\max_{\tau \in I_i} \decke^*_n (\tau)$.
\item  $y^{\mathfrak u}_i := \decke_n^*(\xi^{\mathfrak u}_i) = \frac{\overline f(s_{i+1}) +\overline f(s_i)}{2} + L_i \frac{s_{i+1}-s_i}{2}$ .
\end{enumerate}
\begin{proof} Let $1 \leq i \leq N-1, t \in I_i$. Define $\alpha^\decke_i(t) = \overline f(a_i) + L_i (t-a_i) = \decke_n^i(t), \beta^\decke_i (t) = \overline f(b_i) + L_i (b_i - t) = \decke^{i+1}_n(t), \forall t \in I_i$.

Firstly, $\xi^\decke_i \in I_i$ is a direct consequence of Lem. \ref{lem:Lipbetweensamples}.

Secondly, we show $\decke^*_n(t) = 
 \begin{cases}  
 \decke^i_n (t), & t \leq \xi^\decke_i \\
 \decke^{i+1}_n(t), & t \geq \xi^\decke_i.
 \end{cases}$:

By definition,
$\decke^*_n (t) = \min\{ \decke^{i}_n(t), \decke^{i+1}_n(t)\} = \min\{\alpha^i_n (t),\beta^i_n(t)\}$.
We have $\dot  \alpha^\decke_i(t) = L_i > 0$ and $\dot  \beta^\decke_i(t) = - L_i < 0$. Hence, the functions are strictly monotonous. Let $\xi$ be the input where the lines intersect, i.e. $\alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$. Monotonicity implies $\forall t \leq \xi : \alpha^\decke_i(t) \leq \alpha^\decke_i(\xi) \wedge \beta^\decke_i(t) \geq \beta^\decke_i(\xi) = \alpha^\decke_i(\xi)$. 
Hence,
 \[\forall t \leq \xi: \decke^*_n(t) = \min \{\alpha_i^{\mathfrak u} (t), \beta_i^{\mathfrak u} (t) \}= \alpha_i^{\mathfrak u} (t).\] 
 
Analogously, monotonicity implies $\forall t \geq \xi : \beta^\decke_i(t) \leq \beta^\decke_i(\xi) \wedge \alpha^\decke_i(t) \geq \alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$. 
Thus,
 \[\forall t \geq \xi: \decke^*_n(t) = \min \{\alpha_i^{\mathfrak u} (t), \beta_i^{\mathfrak u} (t) \}= \beta_i^{\mathfrak u} (t).\] 

In conjunction, we have 
 $\decke^*_n(t) = 
 \begin{cases}  
 \alpha_i^{\mathfrak u} (t), & t \leq \xi \\
 \beta_i^{\mathfrak u} (t), & t \geq \xi 
 \end{cases}$.
 Again, using monotonicity of $\alpha_i^{\mathfrak u}$ and $\beta_i^{\mathfrak u}$ we infer that $\decke^*_n$ has a single maximum $y := \decke^*_n(\xi)$ at $\xi$.

Next, we show that $\xi = \xi_i^{\mathfrak u}$: 

$\alpha^\decke_i(\xi) = \beta^\decke_i(\xi)$

$\Leftrightarrow  \overline f(s_i) + L_i (\xi - s_i) = \overline f(s_{i+1}) -L_i (\xi - s_{i+1})$

$\Leftrightarrow  L_i \bigl( 2 \xi - s_{i+1}  - s_i\bigr) = \overline f(s_{i+1}) - \overline f(s_i) $

$\stackrel{L_i > 0}{\Leftrightarrow}   \bigl( 2 \xi - s_{i+1}  - s_i\bigr) = \frac{\overline f(s_{i+1}) - \overline f(s_i)}{L_i} $

$\Leftrightarrow   \xi  = \frac{\overline f(s_{i+1}) - \overline f(s_i)}{2 L_i}  + \frac{s_{i+1}+s_i}{2} = \xi^{\mathfrak u}_i$.



Finally, we need to evaluate $\decke^*_n(\xi^{\mathfrak u}_i)$ to prove the last claim:
We have 

 $\decke^*_n(\xi) = \alpha_i^{\mathfrak u} (\xi) =  \overline f(s_i) + L_i (\xi - s_i) $

$= \overline f(s_i) + L_i \bigl( \frac{\overline f(s_{i+1}) - \overline f(s_i)}{2 L_i}  + \frac{s_{i+1}+s_i}{2} - s_i \bigr) $ 

$=  \frac{\overline f(s_{i+1}) - \overline f(s_i) + 2\overline f(s_i)}{2 }  + L_i \frac{s_{i+1}-s_i}{2}   = y_i^{\mathfrak u}$. 



\end{proof}

\end{lem}


Completely analogously to the the proof of Lem. \ref{lem:ceiling_maxvalues} we can prove the corresponding statement for the H\"older floor:
\begin{lem} \label{lem:floor_minvalues}
Let $\metric(x,y) := \abs{x-y}$.
For $i \in \{1,\ldots,N_n-1\}$ let  $L_i > 0$, $I_i = [s_i,s_{i+1}]$.
Define $\xi^{\boden}_i :=  \frac{s_i+s_{i+1}}{2}- \frac{\underline f(s_{i+1}) - \underline f(s_i)}{2 L_i}  $.\\
For $t \in I_i$ we have 
\begin{enumerate}
\item $\xi^{\boden}_i \in I_i$ and  $\boden^*_n(t) = 
 \begin{cases}  
 \boden^i_n (t), & t \leq \xi^\boden_i \\
 \boden^{i+1}_n(t), & t \geq \xi^\boden_i.
 \end{cases}$
\item $\xi^{\boden}_i \in \arg\min_{\tau \in I_i} \boden^*_n (\tau)$.
\item  $y^{\boden}_i := \boden_n^*(\xi^{\boden}_i) = \frac{\underline f(s_{i+1}) +\underline f(s_i)}{2} - L_i \frac{s_{i+1}-s_i}{2}$ .
\end{enumerate}

\begin{proof} The proof is analogous to the one provided for Lem. \ref{lem:ceiling_maxvalues}.
%
%The case $i = N$ is trivial. Let $1 \leq i \leq N-1$. By definition,
%$\boden^i_n (t) = \min\{ \alpha^\boden_i(t), \beta^\boden_i(t)\}$.
%We have $\dot  \alpha^\boden_i(t) = - L_i < 0, \forall t$ and $\dot  \beta^\boden_i(t) =  L_i > 0, \forall t$. Hence, the functions are strictly monotonous. Let $\xi$ the input where the lines intersect, i.e. $\alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$. Monotonicity implies $\forall t \leq \xi : \alpha^\boden_i(t) \geq \alpha^\boden_i(\xi) \wedge \beta^\boden_i(t) \leq \beta^\boden_i(\xi) = \alpha^\boden_i(\xi)$. 
%Hence,
 %\[\forall t \leq \xi: \boden_n^i(t) = \max \{\alpha_i^{\mathfrak l} (t), \beta_i^{\mathfrak l} (t) \}= \alpha_i^{\mathfrak l} (t).\] 
 %
%Analogously, monotonicity implies $\forall t \geq \xi : \beta^\boden_i(t) \geq \beta^\boden_i(\xi) \wedge \alpha^\boden_i(t) \leq \alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$. 
%Thus,
 %\[\forall t \geq \xi: \boden_n^i(t) = \max \{\alpha_i^{\mathfrak l} (t), \beta_i^{\mathfrak l} (t) \}= \beta_i^{\mathfrak l} (t).\] 
%
%In conjunction, we have 
 %$\boden_n^i(t) = 
 %\begin{cases}  
 %\alpha_i^{\mathfrak l} (t), & t \leq \xi \\
 %\beta_i^{\mathfrak l} (t), & t \geq \xi 
 %\end{cases}$.
 %Again, utilizing monotonicity of $\alpha_i^{\mathfrak l}$ and $\beta_i^{\mathfrak l}$ we infer that $\boden_n^i$ has a single minimum $y := \boden_n^i(\xi)$ at $\xi$.
%It remains  (i) to show that $\xi = \xi_i^{\mathfrak l}$, (ii) we need to evaluate $\boden_n^i(\xi^{\mathfrak l}_i)$ showing $y = y_i^{\mathfrak l}$, and (iii) we need to show that 
%$\xi^{\mathfrak l}_i \in \bar I_i$ .
%
%(i) $\alpha^\boden_i(\xi) = \beta^\boden_i(\xi)$
%
%$\Leftrightarrow  f(a_i) - L_i (\xi - a_i) = f(b_i) +L_i (\xi - b_i)$
%
%$\Leftrightarrow  L_i \bigl( 2 \xi - b_i  - a_i\bigr) = f(a_i) - f(b_i) $
%
%$\stackrel{L_i > 0}{\Leftrightarrow}   \bigl( 2 \xi - b_i  - a_i\bigr) = \frac{f(a_i) - f(b_i)}{L_i} $
%
%$\Leftrightarrow   \xi  = \frac{f(a_i) - f(b_i)}{2 L_i}  + \frac{b_i+a_i}{2} = \xi^{\mathfrak l}_i$.
%
%(ii) $\boden_n^i(\xi) = \alpha_i^{\mathfrak l} (\xi) =  f(a_i) - L_i (\xi - a_i) $
%
%$= f(a_i) - L_i \bigl( \frac{f(a_i) - f(b_i)}{2 L_i}  + \frac{b_i+a_i}{2} - a_i \bigr) $ 
%
%$=  \frac{-f(a_i) + f(b_i) + 2f(a_i)}{2 }  - L_i \frac{b_i-a_i}{2}   = y_i^{\mathfrak l}$. 
%
%(iii) $\xi^{\mathfrak l}_i \in \bar I_i$ if and only if $a_i \leq \xi^{\mathfrak l}_i \leq b_i$. Since $\xi^{\mathfrak l}_i = -\frac{f(b_i) - f(a_i)}{2 L_i}  + \frac{b_i+a_i}{2}$ and $\frac{b_i+a_i}{2}$ is just in the middle value of interval $\bar I_i = [a_i,b_i]$, we have 
%
%$\xi^{\mathfrak l}_i \in \bar I_i$ if $\abs{\frac{f(b_i) - f(a_i)}{2 L_i}} \leq \abs{\frac{b_i-a_i}{2}}$.
%However, the latter is the case due to $L_i$-H\"older continuity of $f$ on $\bar I_i$.  
  
\end{proof}

\end{lem}

\section{Kinky inference over function values - nonparametric machine learning}
%Non-deductive inference is the process of drawing conclusions about the general on the basis of the particular. Machine learning is about the automated construction of a mathematical model that facilitates non-deductive inference. 
%These days, supervised machine learning essentially is function estimation. That is, given a (noisy) sample of a target function, artificial learning is the process of constructing a computable model of a function that generalises beyond the observed sample. 
%While parametric machine learning subsumes all the information contained in the sample in a parameter of fixed size, nonparametric machine learning typically takes the entire sample into account when making inference. That is, it creates models for non-deductive inference whose complexity grows with the sample size. This conceptual difference typically leads to complementary advantages and disadvantages \cite{mitchellbook:97}: Parametric methods typically can take longer to aggregate all information into the finite parameter, have stronger inductive bias, but once a model is learned, inference speed is determined by the size of the parameter, not the size of the data and thus, can be very fast. For instance, in artificial neural networks, the parameter is given by the weights of the network links. Once the weights are determined from the training data, the required computation only depends on the number of weights, not on the size of the training data. 
Supervised machine learning methods are algorithms for inductive inference. On the basis of a sample, they construct (learn) a generative model of a data generating process that facilitates inference over the underlying ground truth function and aims to predict function values at unobserved inputs. If the inferences (i.e. predictions of function values) are utilised in a decision-making process whose outcome involves risk, information about the prediction uncertainty can be vital. For instance, a robot that has a poor model about its dynamics would have to keep greater distance to obstacles than one that has a good model. Having such applications in mind, we are especially interested in learning algorithms that allow for conservative inference. That is, the predictions come with uncertainty quantifications that never underestimate the true uncertainty. 

Since typically there are infinitely many explanations that could explain any finite data set, one needs to impose assumptions a priori in order to be able to generalise beyond the observed data and to establish the desired uncertainty quantifications. 

These assumptions, sometimes referred to as inductive bias \cite{mitchellbook:97}, take different forms and are an essential distinguishing factor between different machine learning algorithms. 
The inductive bias implicitly or explicitly restricts the hypothesis space. That is, the space of target functions that can be learned.
In this work, we devise a learning method for ground truth functions that are assumed to be contained in the a priori hypothesis space $\Kprior$ of H\"older continuous functions that may moreover be known to be contained within certain predefined bounds. 

In case the parameters of the H\"older class the function is contained in are known (or at least an upper bound on the H\"older constant and bounds) we can give robust error estimates that give worst-case guarantees on the predictions.

\subsubsection{Conservative learning and inference in a nutshell \jcom{perhaps an intro candidate}}

The general approach we will consider is as follows. We desire to learn a function $f$ based prior knowledge in the form that $f \in \mathcal K_{prior}$ and some (noisy) function sample $\data$. 
The task of conservative inference over functions (i.e. learning) then is the step of forming a posterior belief of the form $f \in \mathcal K_{post}= \mathcal K_{prior} \cap \mathcal K(\data)$
where data is the set of all functions that could have generated the observed data. 
The conservatism lies in the fact that we have not ruled out any candidate functions that are consistent with our information. 
To perform inference over a function value at input $x$ in a conservative manner, we merely infer that $f \in \prederrbox(x) =[\boden(x), \decke(x)]$ 
where \textit{floor function} $\boden(x) =\inf_{\phi \in \mathcal K_{post}} \phi(x)$ and  \textit{ceiling function } $\decke(x) = \sup_{\phi \in \mathcal K_{post}} \phi(x)$ delimit the values the any function in the posterior class $\mathcal K_{post}$ could give rise to. If a point prediction of a function value is required, we could choose any function value between the values given by the floor and ceiling which also give rise to the bounds on the point prediction. 
Of course, the type of inference we get from this general procedure depends on the chosen prior class $\mathcal K_{prior}$ and the specifics of the data. We will develop \textit{kinky inference} which is a method for considering prior classes of multi-output functions over metric input spaces that are optionally constrained by boundedness and by knowledge of H\"older regularity as well as knowledge on uncertainty bounds on the observations and function inputs. For this class of inference mechanisms we prove conservatism and convergence guarantees to the learning target. What is more, we will consider classes where the imposed regularity assumptions are uncertain or adapted lazily to adjust for overly restrictive prior assumptions that do not fit the observations.

The capability of imposing boundedness assumptions, accommodating for noise and being able to adjust the regularity assumptions will prove of great importance in the 
control applciations we will consider in Sec. \jcom{fill in} 
\subsection{The framework of conservative inference -- definitions, setting and desiderata }
\label{sec:prob_def}

%As a basic example, consider the ordinary differential equation $\frac{\d x}{\d t} = (\xi - x)$ where $\xi: I \subset \Real \to \Real $ is an absolutely continuous function superimposed by a countable number of steps. Suppose, the ODE describes the trajectory $x: I \to \Real$ of a controlled particle in one-dimensional state space. Based on $N$ time-state observations $D_N=(t_1,x_1 ),..., (t_N,x_N )$ we desire to estimate the total distance travelled $S$ in time interval $I$, $S = \int_I x(t) \d t$. Solving


%%\textbf{Setting.}
%Let $(\inspace, \metric_\inspace)$, $(\outspace ,\metric_\outspace)$ be two metric spaces and $f: \inspace \to \outspace$ be a function. Spaces $\inspace, \outspace$ will be referred to as \textit{input space} and \textit{output space}, respectively.
%Assume, we have access to a \textit{sample set} $\data_n:= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N_n \} $ containing $N_n \in \nat$ sample vectors $\tilde f_i \in \outspace$ of function $f$ at sample input $s_i \in \inspace$. To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the \textit{grid} of sample inputs contained in $\data_n$.
%
%
%The sampled function values are allowed to have interval-bounded \textit{observational error} given by $\varepsilon : \inspace \to \Real^m_{\geq 0}$. That is, all we know is that $f(s_i) \in \obserrhyprec_i := [\underline f_1(s_i), \overline f_1(s_i) ] \times \ldots \times [\underline f_d(s_i), \overline f_d(s_i) ]$ where $\underline f_j(s_i) := \tilde f_{i,j} - \varepsilon_j(s_i)$, $\overline f(s_i) := \tilde f_{i,j} + \varepsilon_j(s_i)$ and $\tilde f_{i,j}$ denotes the $j$th component of vector $\tilde f_{i}$.
%
%The interpretation of these errors depends on the given application. For instance, in the context of system identification, the sample might be based on noisy measurements of velocities. The noise may be due to sensor noise or may represent numerical approximation errors. As we will see below, $\varepsilon$ may also quantify \textit{input} uncertainty (that is when predicting $f(x)$, $x$ is uncertain). This is an important case to consider, especially in the context of control applications where the ground truth might represent a vector field or an observer model.
%
%
%It is our aim to learn function $f$ in the sense that, folding in knowledge about $\data_n$, we infer \textit{predictions} $\predf(x)$ of $f(x)$ at unobserved \textit{query inputs} $x \notin G_n$. Being the target of learning, we will refer to $f$ as the \emph{target} or \emph{ground-truth} function. 
%
%In addition to the predictions themselves, we are also interested in \textit{conservative bounds} on the error of the inferred predictions. Depending on the hypothesis space under consideration these bounds can be of a probabilistic or deterministic nature. In this chapter, for the time being, we are interested in the latter.
%
%That is, we desire to provide a computable \textit{prediction uncertainty} function $\prederr: \inspace \to \outspace$ such that we can guarantee that for any query $x$, our prediction $\predf(x)$ is within the cube of error given by $\prederr(x)$ as follows 
%
%
%Being interested in conservative worst-case guarantees, we are mostly interested 
%
%
%
%In order to be able to deduce the error bounds around the predictions $\predf$, it is important to impose a priori restrictions on the class of possible targets (the hypothesis space). 

%\textbf{Definitions.}
Let $f: \inspace \to \outspace$ be a function where $\inspace$, $\outspace$ are two spaces endowed with (semi-) metrics $\metric_{\inspace}: \inspace^2 \to \Real_{\geq 0}, \metric_\outspace:\outspace^2 \to \Real_{\geq 0}$, respectively. Spaces $\inspace, \outspace$ will be referred to as \textit{input space} and \textit{output space}, respectively. 

For simplicity, in this work, we will assume $\outspace \subseteq \Real^m$ and $\metric_{\outspace}(y,y') = \norm{y-y'}$ for some standard norm that is equivalent to the maximum norm.\footnote{Extensions to more general output spaces seem very possible, albeit, instead of learning a function, we would then learn a discrepancy from a nominal reference in output space. We will leave this to future work.}
In contrast, we do not impose restrictions on the input space metric. While our simulations will consider the deterministic case, it would be entirely possible to consider inputs spaces that are index sets of stochastic processes endowed with suitable norm metrics (for further comments, refer to Sec. \ref{sec:kinkyinf_futurework}). Since the output metric is defined via a norm, we will often drop the subscript of the input metric. That is we may write $\metric$ instead of $\metric_\inspace$.


\jcom{probably move remark below where the experiments are and we can show a periodic kernel.}
\begin{rem}[Remarks on relationship to kernels]
Metrics are measures of dissimilarity and will aid our efforts to perform inference.
%For instance, we have seen that  $\metric(x,y) := \normtop{x-y}$ defines a proper metric and (uniform) convergence with respect to this metric is equivalent to (uniform) convergence with respect to metric $ D: (x,y) \mapsto \norm{x-y}$ (see Sec. \ref{sec:unifconvhoeldermetricequivmetricunifconv}). 
In much of the recent machine learning literature, kernel functions are utilised to perform inference.
Note, a kernel function is a measure of similarity often based on quantities inversely related to metrics (which are dissimilarity measures). Therefore, we can draw on the kernel learning literature to draw inspiration about metrics or pseudo-metrics suitable for an application at hand (for a recent overview of kernels, including periodic ones, refer to\cite{duvenaud2014}). 
For instance, we might consider folding in knowledge of periodicity of the underlying function class which we might borrow from the kernel learning literature \cite{duvenaud2014}.
\end{rem}


Assume, we have access to a \textit{sample} or \textit{data set} $\data_n:= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N_n \} $ containing $N_n \in \nat$ sample vectors $\tilde f_i \in \outspace$ of function $f$ at sample input $s_i \in \inspace$. To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the \textit{grid} of sample inputs contained in $\data_n$. Subscript $n$ aides our exposition when we consider sequences of data sets indexed by $n$.

The sampled function values are allowed to have interval-bounded \textit{observational error} given by $\varepsilon : \inspace \to \Real^m_{\geq 0}$. That is, all we know is that $f(s_i) \in \obserrhyprec_i := [\underline f_1(s_i), \overline f_1(s_i) ] \times \ldots \times [\underline f_d(s_i), \overline f_d(s_i) ]$ where $\underline f_j(s_i) := \tilde f_{i,j} - \varepsilon_j(s_i)$, $\overline f(s_i) := \tilde f_{i,j} + \varepsilon_j(s_i)$ and $\tilde f_{i,j}$ denotes the $j$th component of vector $\tilde f_{i}$.

The interpretation of these errors depends on the given application. For instance, in the context of system identification, the sample might be based on noisy measurements of velocities. The noise may be due to sensor noise or may represent numerical approximation errors. As we will see below, $\varepsilon$ may also quantify \textit{input} uncertainty (that is when predicting $f(x)$, $x$ is uncertain). This is an important case to consider, especially in the context of control applications where the ground truth might represent a vector field or an observer model. Finally, the observational error can also model error around the compuation of the metric. This might be of interest if the metric has to be approximated numerically or estimated with statistical methods. 


It is our aim to learn function $f$ in the sense that, combining prior knowledge about $f$ with the observed data $\data_n$, we infer \textit{predictions} $\predfn(x)$ of $f(x)$ at unobserved \textit{query inputs} $x \notin G_n$. Being the target of learning, we will refer to $f$ as the \emph{target} or \emph{ground-truth} function. In our context, the evaluation of $\predf_n$ is what we refer to as \textit{(inductive) inference}. For a discussion of the competing definitions of non-deductive inference in a philosophical context the reader is referred to \cite{Flach2000}. The entire function $\predfn$ that is learned to facilitate predictions is referred to as the \textit{predictor}. Typically,
the predictor lies in the space that coincides or is at least dense in space $\mathcal K_{prior}$ of conceivable target functions. In this case the predictor can be referred to as a \textit{candidate function} or \textit{hypothesis} \cite{mitchellbook:97}.

In addition to the predictions themselves, we are also interested in \textit{conservative bounds} on the error of the inferred predictions. Depending on the hypothesis space under consideration these bounds can be of a probabilistic or deterministic nature. In this chapter, for the time being, we are interested in the latter.

That is, we desire to provide a computable \textit{prediction uncertainty function} $\prederr: \inspace \to \outspace$ such that we \textit{believe} that for any query $x \in \inspace$, the ground truth value $f(x)$ lies somewhere within the \textit{uncertainty hyperrectangle }
\begin{equation}
	\prederrbox_n(x) := \Bigl\{ y \in \outspace \, | \, \forall j \in \{1,...,\dim{\outspace}\} : f_j(x) \in [ \predfnj(x) - \prederrnj(x), \predfnj(x) + \prederrnj(x)] \Bigr\}
\end{equation} around the prediction $\predfn (x)$.
Here, $\predfnj(x)$, $\prederrnj(x)$ denote the $j$th components of vectors $\predfn(x), \prederrn(x)$, respectively.

 %As a word of caution, we remark that using the last statement as a definition still seems very broad. 

%\textbf{Desiderata.}
In this chapter, will understand a \textit{machine learning mechanism} to implement a computable function that maps a data set $\data_n $ to a prediction function $\predf_n$ and an uncertainty estimate function $\prederr_n$ both of which exhibit certain desirable properties, which will be discussed next. 

Mitchell \cite{mitchellbook:97} proposed to call an algorithm to be a machine learning algorithm, if it improves its performance with respect to some specified cost function with increasing data. We are interested in learning a function that \textit{converges} to the ground truth. That is, in the limit of infinite, informative data, the point-wise distance, measured by a norm, between the prediction and the ground-truth should shrink \textit{monotonically}. That is, the cost in Mitchell's definition might be quantified by this distance.

%Note, converse statement would be too general to be useful to capture behaviour that matches the intuition of learning. 

Being interested in \textit{conservative} inference, we desire to give conditions under which the uncertainty beliefs $\prederr_n(x)$ around the predictions $\predf_n(x)$ are never overoptimistic. That is, we desire to give a guarantee that the target cannot assume values outside the uncertainty hyperrectangle $\prederrbox_n$.

In order to conceive an inference mechanism that can generalise beyond the sample and to establish its desired properties, we need to make a priori assumptions.
That is, it is important to impose a priori restrictions on the class of possible targets (the \textit{hypothesis space}). As mentioned above, we will denote this space by $\mathcal K_{prior}$.


%Furthermore, for each sub-hyperrectangle $J \subset I$ we have access to a Lipschitz number $L_J \geq 0$. That is, $L_J$ is a number such that $\forall x,x' \in J: \abs{f(x) - f(x')} \leq L_J \, \norm{ x- x'}$ where $\norm \cdot$ is a fixed norm on $I$.\footnote{Note, due to norm-equivalence in finite-dimensional space, it is of no principal concern which norm is chosen.} 

%We assume $\metric_\inspace: \inspace^2 \to \Real$ to be any suitable metric (or pseudo-metric) on the target function domain that encodes a notion of dissimilarity between inputs. 
%
%%For instance, we have seen that  $\metric(x,y) := \normtop{x-y}$ defines a proper metric and (uniform) convergence with respect to this metric is equivalent to (uniform) convergence with respect to metric $ D: (x,y) \mapsto \norm{x-y}$ (see Sec. \ref{sec:unifconvhoeldermetricequivmetricunifconv}). 
%
%Note, a kernel function is a measure of similarity often based on quantities inversely related to metrics (which are dissimilarity measures). Therefore, we can draw on the kernel learning literature to draw inspiration about metrics or pseudo-metrics suitable for an application at hand (for a recent overview of kernels, including periodic ones, refer to\cite{duvenaud2014}). 
%For instance, we might consider folding in knowledge of periodicity of the underlying function class which we might borrow from the kernel learning literature \cite{duvenaud2014}.

%Also note, Lipschitz continuity with respect to $\metric$ is H\"older continuity with respect to metric $D$ (cf. Thm. \ref{thm:pmetricphoelder}). Therefore, we may use the terms Lipschitz continuity and H\"older continuity interchangeably if it is clear which metrics the terms refer to.

Once sample $\data_n$ is known, we can combine the information contained therein with the prior. At the very least, we can form a \textit{posterior hypothesis space} $\mathcal K_{post}$ by falsification. That is, we eliminate all hypotheses from $\mathcal K_{prior}$ that could not have generated the sample. 

To formalise this, we define 
\begin{equation}
	\Kdat = \Bigl\{ f: \inspace \to \outspace | \, \forall i \in \{1,...,N_n\}: \, f(s_i) \in \obserrhyprec_i  \Bigr\}
\end{equation}
to be the set of \textit{sample-consistent} functions as the set of all functions that might have generated the data.


To perform inference over functions, we construct a posterior hypothesis set $\mathcal K_{post}$. 
Normally, we would expect \textit{monotonicity} of our inference in that the additional information afforded by the data should not make us more uncertain. That is,  $\mathcal K_{post} \subset \mathcal K_{prior}$. In the light of the data, we should 
also require consistency yielding the requirement $\mathcal K_{post} \subset \mathcal K(\data_n)$. In conjunction we then have 
\begin{equation}
	\mathcal K_{post} \subseteq \mathcal K_{prior} \cap \mathcal K(\data_n)
\end{equation} or, conservatively, 
$\mathcal K_{post} = \mathcal K_{prior} \cap \mathcal K(\data_n)$.\footnote{As an aside, note that the latter choice is consistent with conservatism and would be the choice consistent with Popper's approach of falsification to epistemology.}

\begin{rem}[False prior hypotheses, lazy relaxations and search bias]
\label{rem:lazyrelaxationpriorspace}
Furthermore, note that it might happen that $\mathcal K_{prior} \cap \mathcal K_{post} =\emptyset$. Presuming there was no problem with the data set, this might be indicative of $\mathcal K_{prior}$ being too restrictive. One approach to deal with such a situation would be to relax our prior assumptions. If we do so just enough to ensure that $\mathcal K_{post} \neq \emptyset$, we will call this relaxation \emph{lazy}. Below, where we consider prior hypothesis spaces constrained by H\"older regularity under the assumption that the parameters of the H\"older condition are known. Since this is often difficult to achieve in practice, Sec. \ref{sec:uncertainconstants} contains a lazy adaptation rule of the H\"older constant. This is an example of a lazy relaxation of the prior hypothesis space. 
From a wider point of view, one could of course interpret the relaxation procedure as part of the learning algorithm. From this vantage point, the actual prior hypothesis space is the maximally relaxed space on which the algorithm imposes the search bias \cite{mitchellbook:97} preferring hypothesis in more constrained sets over relaxed ones. Since more constrained spaces have lower learning capacity, this search bias imposes a form of regularization found in many machine learning approaches. Interestingly, in the context of the relaxations of the H\"older constant consider in Sec. \ref{sec:lazylipconstupdate}, preferring lower H\"older constants over larger ones seems to establish a strong link to regularisation in kernel methods \cite{wahabarepresenter:1990}. Investigating these links is something we have not done yet, but will be undertaken in future work. \jcom{perhaps last paragraph into discussion and future work. also check wahabas book}
\end{rem}

Having learned, i.e. performed inference over functions, we can use this to predict function values conservatively by considering all the function values within the posterior class which could be assumed at a given query input $x \in \inspace$.

We are now in a position to summarize our desiderata on the joint inference mechanism as follows:

%Based on sample set $\data_n$, we desire to design an inference 
%method that satisfies the following desiderata:

%\subsection{Task 1 -- Computing a conservative \textit{function estimate}}
%\label{sec:problemdef_task1}

\begin{defn}[Desiderata] \label{def:KIdesiderata} With definitions as above, we desire a machine learning algorithm to implement a mapping $\data_n \mapsto (\predfn,\prederrn)$ such that, for all data sets $\data_n$, the resulting inductive inference satisfies the following \textbf{desiderata}:
\begin{enumerate}
	\item \textit{Conservatism:} We can guarantee  $ f(x) \in \prederrbox_n(x),  \forall x \in \inspace, \forall f \in \mathcal K_{prior} \cap \mathcal K(\data_n)$.
	\item \textit{Monotonicity:} Additional data cannot increase the uncertainty. 
	
	That is, $\data_n \subseteq \data_{n+1} $ implies 
		$\prederrbox_n(x) \supseteq \prederrbox_{n+1}(x)$ or equivalently, $\prederr_n(x) \geq \prederr_{n+1}(x), \forall x \in \inspace$ (where the inequality holds for each component).
	%\item \textbf{Convergence} to the target: Let the set of sample inputs $G_n$ in $D_n$ converge to a dense subset of domain $I \subset \inspace$ and for each input $x \in I$ let the sample error function $\varepsilon: I \to \Real_{\geq 0}$ be bounded by $m_x \geq 0$ in some neighbourhood of $x$. Then, we have 
%\begin{itemize}
%\item (a) The uncertainty converges point-wise: $\forall x \in I: 0 \leq \lim_{n \to \infty} \prederrn(x) \leq m_x$.
%In particular, the enclosure converges to the target $f(x)$ at inputs $x$ where $m_x=0$.  
		%
		%\item (b) If convergence of $G_n$ is uniform and the target observations are error-free, i.e. $m_x = 0, \forall x \in I$, then the enclosure converges to the target $f$ uniformly.
%\end{itemize}	
	\item \textit{Convergence}: If $(G_n )_{n \in \nat }$ is a sample grid sequence of inputs converging to a dense subset of $\inspace$ (as $n \to \infty$) then  $\prederrn(x) \stackrel{n \to \infty}{\longrightarrow} \varepsilon(x), \forall x \in \inspace$. If convergence of the grid to the dense subset is uniform (cf. Def. \ref{def:uniform_setconvergence}) and the observational error is constant ($\exists c \in \Real: \varepsilon \equiv c $) then the convergence  $\prederrn \stackrel{n \to \infty}{\longrightarrow} \varepsilon$ is uniform. 
	   \item \textit{Minimality (optimality)}: There is no conservative uncertainty bound that is tighter than $\prederr_n$. That is, if for some hyperrectangle $H$, $x \in \inspace$ we have $H \subsetneq \prederrbox_n(x)$ then we have: $\exists x \in \inspace, f \in \mathcal K_{prior} \cap \mathcal K(\data_n) : f(x) \notin H$. 
%If an enclosure $\mathcal E^b_a$  satisfies \emph{Desideratum 2} then it is a superset of our enclosure $\einschluss$, i.e. $b \geq \decke_n, a \leq \boden_n$, $\einschluss \subseteq \mathcal E^b_a$.    
\end{enumerate}
\end{defn}

%Note, Desiderta 1-3 combined imply that in the absence of observational errors ($\varepsilon \equiv 0$), the prediction $\predfn$ converges monotonically to the target when data sets become increasingly dense.

\subsection{The kinky inference and nonparametric machine learning mechanism}

We are now in a position to define our kinky inference rule:

\begin{defn}[Kinky inference rule (KIR)] \label{def:KIL}
Let  $\Real_\infty := \Real \cup\{- \infty, \infty\}$ and $\inspace$ be some space endowed with a semi-metric $\metric_\inspace$. Let $\lbf,\ubf: \inspace \to \outspace \subseteq \Real_\infty^m$ denote \textit{lower- and upper bound functions}, that can be specified in advance and assume $\lbf(x) \leq \ubf(x), \forall x \in I \subset \inspace$ component-wise. 
Given sample set $\data_n$ we define the predictive functions $\predfn: \inspace \to \outspace, \prederrn: \inspace \to \Real^m_{\geq 0}$ to perform inference over function values.
For $j=1,\ldots,m$, their $j$th output component is given by  
%Furthermore, define
% $\coeff1,\coeff2 \in \Real_{\geq0}$ such that $\coeff1+\coeff2 =1$ (unless explicitly stated otherwise, we assume $\coeff1=\coeff2 =\frac 1 2)$.
	\begin{align}
   \predfnj(x) &:= \frac{1}{2} \min\{ \ubf_j(x), \decke_{n,j}(x)\} + \frac{1}{2} \max\{ \lbf_j, \boden_{n,j}(x) \} \label{eq:KIpred}\\  
	\prederrnj(x) &:= \frac{1}{2} \bigl(\min\{ \ubf_j(x), \decke_{n,j}(x)\} - \max\{ \lbf_j, \boden_{n,j}(x) \} \bigr)   
	\end{align}
	where $\decke_n, \boden_n: \inspace \to \Real^m$ are called ceiling and floor functions, respectively. Their $j$ component functions are given by
	$\decke_{n,j}(x) := \min_{i=1,\ldots,N_n}   \tilde f_{i,j} + L_j \metric^p(x,s_i) + \varepsilon_j(x)$ and 
	$\boden_{n,j}(x) := \max_{i=1,\ldots,N_n}   \tilde f_{i,j} - L_j \metric^p(x,s_i) - \varepsilon_j(x)$, respectively.
  Here $p \in \Real, L \in \Real^m$ and functions $\lbf,\ubf,\varepsilon$ are parameters that have to be specified in advance. To disable restrictions of boundedness, it is allowed to specify the upper and lower bound functions to constant $\infty$ or $-\infty$, respectively.	
	Function $\predfn$ is the predictor that is to be utilised for predicting/inferring function values at unseen inputs. Function $\prederrn(x)$ quantifies the uncertainty of prediction $\predfn(x)$. 
	%Note, if the data set is fixed (i.e. $n$ does not change), we may sometimes drop the subscript $n$ and write $\predf$ instead of $\predf_n$.
\end{defn}

%
%\begin{defn}[Kinky inference rule (KIR)] \label{def:KIL}
%Define $\lbf,\ubf: \inspace \to \Real \cup\{- \infty, \infty\}$ to be the \textit{lower- and upper bound function}, and assume $\lbf(x) \leq \ubf(x), \forall x \in I \subset \inspace$. 
%Given sample set $D_n$ we define the following predictive functions to perform inductive inference:
%%Furthermore, define
%% $\coeff1,\coeff2 \in \Real_{\geq0}$ such that $\coeff1+\coeff2 =1$ (unless explicitly stated otherwise, we assume $\coeff1=\coeff2 =\frac 1 2)$.
	%\begin{align}
   %\predf_n(x) &:= \frac{1}{2} \min\{ \ubf(x), \decke_n(x)\} + \frac{1}{2} \max\{ \lbf, \boden_n(x) \} \\  
	%\prederr_n(x) &:= \frac{1}{2} \bigl(\min\{ \ubf(x), \decke_n(x)\} - \max\{ \lbf, \boden_n(x) \} \bigr) \label{eq:KIprederr}\\  
	%\end{align}
	%where $\decke_n(x) := \min_{i=1,\ldots,N_n}  \tilde f_i + L \metric(x,s_i)+\varepsilon(x)$
	%is called the ceiling 
	%and $\boden_n(x) := \max_{i=1,\ldots,N_n}   \tilde f_i - L \metric(x,s_i) - \varepsilon(x)$
	%is called the floor function.
	%Function $\predf$ is the predictor that is to be utilised for predicting/inferring function values at unseen inputs. Function $\prederr_n(x)$ quantifies the uncertainty of prediction $\predf_n(x)$. Note, if the data set is fixed (i.e. $n$ does not change), we will drop the subscript $n$ and write $\predf$ instead of $\predf_n$.
%\end{defn}
 

\begin{figure}
        \centering
				  \subfigure[KI prediction with two examples.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/ex1Hfe1}
    \label{fig:hfe1}
  } 	
	 \subfigure[Refined prediction.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/ex1Hfe2}
    \label{fig:hfe2}
  } 	%\hspace{2cm}
	  \subfigure[Using a periodic pseudo-metric.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/ex1hfeperiodic}
    \label{fig:hfe3}
  } 	
	\label{fig:exHfe1}
   \caption{Examples of different target functions and kinky inference predictions. \textbf{Fig. \ref{fig:hfe1} and  Fig. \ref{fig:hfe2}} show kinky inference performed for two and ten noisy sample inputs of target function $x\mapsto \sqrt{\abs{\sin(x)}}$ with observational noise level $\varepsilon =0.3$. The floor function folds in knowledge of the non-negativity of the target function ($\lbf = 0$). The predictions were made based on the assumption of $p=\frac 1 2$ and $L = 1$ and employed the standard metric $\metric(x,x') = \abs{x-x'}$. 
	As can be seen from the plots, the function is well interpolated between sample points with small perturbations. Furthermore, the target is within the bounds predicted by the ceiling and floor functions.
		\textbf{Fig. \ref{fig:hfe3}} depicts a prediction folding in knowledge about the periodicity of the target function by choosing a pseudo-metric $\metric = \abs{\sin(\pi \abs{x-x'}}$. The prediction performs well even in unexplored parts of input space taking advantage of the periodicity of the target. This time, there was no observational error and the target function was $x \mapsto \abs{\sin(\pi x)} +1$.   }
\end{figure}	  


\begin{figure}
        \centering
				  \subfigure[Wingrock dynamics.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/hfewingrock_dyn_groundtruth}
    \label{fig:hfe5}
  } 	
	 \subfigure[Inferred model.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/hfewingrock_dyn_learned}
    \label{fig:hfe4}
  } 	%\hspace{2cm}
	 
	\label{fig:exHfe2}
   \caption{Example of a prediction on two-dimensional input space. \textit{Left plot:} the target function being a patch of the wingrock dynamics we will study in Sec. \ref{sec:KIMRAC}. \textit{Right plot:} the predictions inferred on the basis of 100 sample points using metric $\metric(x,x') = \norm{x-x'}_\infty$ and $p=1, L=2.5$.}
\end{figure}	 

To develop a first feel for the kinky inference rule, we have plotted some examples of ground-truth functions and pertaining predictions in Fig. \ref{fig:exHfe1} and Fig. \ref{fig:exHfe2}. Firtsly, we can see that the predictions involve kinks. This is due to the minimisations and maximisations that occur in the computation of the ceiling and floor functions which introduce breakpoints into the prediction signal. This property provided the motivation behind the term ``kinky inference''.

Secondly, we note that in all the examples, the conservative bounds were accurate. That is, the target remained contained in them. An example where we see how the bounds shrink to the ground-truth (up to the observational error tube) will be given in Sec. \ref{sec:agentexploration}, where we consider an agent that utilises kinky inference guide online exploration of a drift vector field it is immersed in. Also, note from Fig. \ref{fig:hfe3} how the choice of distance metric $\metric$ can affect the predictions. In this example, a metric was chosen that took into account an a priori known periodicity of the target function. This allowed predictions to be accurate even in unexplored parts of the input space. 


\subsection{Theoretical guarantees}

The examples depicted in the plots of Fig. Fig. \ref{fig:exHfe1} and Fig. \ref{fig:exHfe2} seem to be consistent with what we would expect from an inference mechanism that is conservative and monotonically convergent and hence, might satisfy the desiderata we stated in Def. \ref{def:KIdesiderata}.
We will now give conditions under which we can guarantee the desiderata to be fulfilled. 

Of course, the validity of our guarantees depends on the a priori hypothesis space $\mathcal K_{prior}$. Inspection of the prediction rules reveals that the minimisation and maximisations eliminate all those function values that do not adhere to boundedness conditions (imposed by $\lbf,\ubf$) and conditions on H\"older continuity up to a margin of error given by $\varepsilon$. 

That this is exactly the right class for which our desiderata hold is asserted by the following theorem:

\begin{thm}
Assuming all (a priori) possible targets $f: \inspace \to \outspace$ are given by the class   
\begin{equation}
	\mathcal K_{prior}= \bigl\{ f : \inspace \to \outspace \subseteq \Real^m |  f \in \hoelset L {\metric_{\inspace}} p \cap \bfset \bigr\}
\end{equation}
where $\hoelset L {\metric_\inspace} p =\{ f: \inspace \to \outspace \subset \Real^m \, |  \forall j \in \{1,\ldots,m\} \forall x,x' \in \inspace: \abs{f_j(x) - f_j(x')}  \leq \, L_j \metric^p_{\inspace}{x,x'} \}$ denotes the class of $L-p$- H\"older continuous functions with respect to metric $\metric_\inspace$ and $\bfset :=\{\phi : \inspace \to \outspace \, | \, \forall x \in \inspace, j \in\{1,...,m\}: \lbf_j(x) \leq \phi_j(x) \leq \ubf_j(x)\} $
is the set of all functions bounded component-wise between functions $\lbf,\ubf: \Real^d \to \Real \cup \{- \infty, \infty\}$, where we will always define $\Real_\infty := \Real \cup\{- \infty, \infty\}$. 

Then we have:
%\begin{enumerate}
%\item  
The inference rule as per Def. \ref{def:KIL} is conservative, monotonically convergent (in the limit of dense sample grids) and optimal in the sense of Def. \ref{def:KIdesiderata}. That is, it satisfies Desiderata 1-4 as per Def. \ref{def:KIdesiderata}. 
%\item If in addition, for some $d \in \nat$, $\inspace \subseteq \Real^d$ and $\metric_{\inspace}(x,x') = \norm{x-x'}$ for some norm that is equivalent to the Euclidean norm then the inference mechanism is also optimal (as per Desideratum 4 in Def. \ref{def:KIdesiderata}). That is, there is no other conservative inference mechanism with tighter uncertainty bound function $\prederrn$. 
%\end{enumerate}
\end{thm}

\jcom{Requirements on the regularity of the bound functions or error ? Can metric be a pseudo-metric?}

   %
%%=================
%
%Let  $\Real_\infty := \Real \cup\{- \infty, \infty\}$.
%In this work, we are primarily interested in functions restricted to be H\"older continuous and bounded component-wise by some known bounding functions $\lbf,\ubf: \inspace \to \Real^m_\infty$. That is, we know the target is contained in 
%the a priori hypothesis space 
%\begin{equation}
	%\mathcal K_{prior}= \bigl\{ f : \inspace \to \Real |  f \in \hoelset L \metric p \cap \bfset \bigr\}
%\end{equation}
%where $\hoelset L \metric p =\{ f: \inspace \to \outspace \subset \Real^m \, |  \norm{}  \leq \, \}$ denotes the class of $L-p$- H\"older continuous functions with respect to metric $\metric$ and $\bfset :=\{\phi : \inspace \to \outspace \, | \, \forall x \in \inspace, j \in\{1,...,m\}: \lbf_j(x) \leq \phi_j(x) \leq \ubf_j(x)\} $
%is the set of all functions bounded component-wise between functions $\lbf,\ubf: \Real^d \to \Real \cup \{- \infty, \infty\}$, where we will always define $\Real_\infty := \Real \cup\{- \infty, \infty\}$. 
%
%For ease of notation, we will follow the convention of dropping the subscripts from inequalities and interpret an inequality component-wise. Similarly, if we omit the argument from an inequality, the inequality is understood to hold point-wise. For example, we interpret write $\lbf \leq \phi$ in place of  $\lbf_j(x) \leq \phi_j(x), \forall j,x$. 

%
%%=======================
%
%
%
%From the perspective of topological inference, the estimator is a data inference method for function estimation:
%$B(\cdot) = M_{dinf}(\mathcal K_{prior}, \cdot, \gamma ) $ (for some sufficiently large $\gamma$) mapping sample data into a hypothesis interval of possible functions. 
%Here,  our a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L_J$ such that the underlying target $f \in \mathcal F$ is $L_J-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L_J \norm{x-x'}\}$. 
%Note, we will not explicitly compute the prior knowledge set. Instead will will fold in the Lipschitz continuity to define an optimal estimator output defining an enclosure that coincides with $\mathcal K_{post} \subset \mathcal K_{prior}$ and hence, with $T (\mathcal K_{post} \cup \mathcal K_{prior})$. Therefore, the resulting inference mechanism will be optimal. 
%
%Note, how our desiderata are equivalent to the corresponding notions of the inference mechanism that is to be designed.


%Our method will 
%
%We 
%
%In this section, we consider hypotheses spaces comprising H\"older continuous functions. This is a very general class of uniformly continuous functions that can exhibit infinitely many non-differentiable points.
%
%
 %In addition to a learned hypothesis, our approach also provides error bounds around each prediction that are conservative and tight. That is, the bounds contain exactly those function within the assumed H\"older class that could have generated the sample. 
%
%The rest of the section is structured as follows: First we 
%
%
%
%Our conservative function estimation procedure constructed upper and lower bound functions that are sample-consistent. The enclosure encompasses all possible candidate functions with an assumed H\"older property that could have generated the sample. Therefore, any H\"older function within the enclosure is a valid hypothesis that could have generated the data and hence, a suitable generalisation model for non-deductive inference. 
%
%
%We assume the dimensionality of the target's input domain $I$ is $d \geq 1$. Remember, we defined the set of function samples as $D_n= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N_n \} $. 
%Let $f$ denote the \textit{ground-truth} or \textit{target function} generating the data. $\tilde f_i$ is a noisy function value such that we know $f(s_i) \in [\tilde f_i - \varepsilon(s_i) , \tilde f_i + \varepsilon(s_i)], \, (i=1,\ldots, N_n)$. To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the grid of sample inputs contained in $D_n$.  
%
%A robust learning rule is a computable mapping $\mathcal R : D_n \mapsto (\predf, \prederr) $.
%Here $\predf$ is a predictor allowing to make inductive inference and $\prederr(x)$ quantifies the uncertainty or error around the prediction $\predf(x)$.
%
 %
%Let $\metric: \inspace^2 \to \Real$ be a metric. We propose the following nonparametric inference rule:

\subsubsection{Computational effort}
We can see from Def. \ref{def:KIL} that the kinky inference method can be classified as supervised nonparametric learnign method. That is, the computational effort for predicting grows with the data set size $N_n$. if the computational effort 
As we observed, our posterior knowledge coincides with the set of sample-consistent functions. Therefore, an exhaustive enclosure is a superset of $\mathcal K_{prior} \cap \mathcal K_{post}$. 
Remembering our discussion of topological inference, we realize that all we need to do to solve Task 1 (as specified in Sec. \ref{sec:problemdef_task1}), is to define our data inference mechanism $M_{\text{dinf}}$ to output the optimal enclosure. A prescription for computing the bounds of this enclosure was given in the definitions above. From these, we see that $M_{dinf}$computes in $\mathcal O(N_n d)$. That is, its computational effort (translating to the necessary inference investment $\gamma_{\text{dinf}})$ is linear in the number of samples and dimensionality of the problem. If we deal with maximum-norms, norm computation can be done with computation that is logarithmic in $d$, reducing the overall evaluation effort to $\mathcal O(N_n \log d)$.   


\subsection{Uncertain inputs}
So far, we have considered output uncertainty but not input uncertainty. That is, we have assumed that the function values $f(s_i)$ at the sample inputs are uncertain but that query inputs $x$ as well as sample 
inputs $s_i$ are known exactly. However, in many applications this assumption typically is not met. For example, in Sec. \ref{sec:hfeandcontrol}, we will employ KI for learning and controlling dynamic systems.
Here the target functions are state-dependent vector fields. Here, the state measurements often are corrupted by noise (e.g. due to sensor noise or delays) which can affect both training data and query inputs. In the latter case, the controller might query the KI method to predict 
a function value $f(x)$ based on the assumption of the plant being in state $x$ while the plant may in fact be in a different state $x+\delta_x$. We would like to guarantee that our inference over the actual function value still is within the predicted bounds provided the input estimation error $\delta_x$ is known or known to be bounded. 
Fortunately, the H\"older property of the target can help to address the problem of quantifying the prediction error due to input uncertainty. For instance, consider $\metric(x,x') = \norm{x-x'}$. By H\"older continuity, the error of the prediction of the $j$th output component of the target function $f$ is bounded by $\abs{f_j(x+\delta_x) - f_j(x)} \leq \norm{\delta_x}^p$. 

Firstly, assume the training inputs $s_i$ were certain but the query inputs $x$ during prediction are uncertain.
Therefore, assuming we know an upper bound $\errinp(x)$ on the input uncertainty, i.e. 
$\norm{\delta_x}^p\leq \errinp(x), \forall x$, we can add this term to the uncertainty estimate $\prederr(x)$ as per Eq. \ref{eq:KIprederr}.
%This means that the additional uncertainty only affects the prediction of this particular query point. 

Secondly, consider the case were both the sample inputs $s_i$ and the query inputs $x$ are uncertain with the uncertainty being quantified by the function $\errinp(\cdot)$. In this case, the uncertainty of the sample inputs
 affects the posterior hypothesis (i.e. the enclosure) over $f$ and hence, the inferences over function values at all inputs. 
By the same argument as for the case of query noise, we accommodate for this fact leveraging the H\"older property. Instead of adjusting just the prediction uncertainty, we simply add $ \errinp(\cdot)$ to the error function $\varepsilon(\cdot)$ (that we have previously used to model observational 
error of the function values). That is, the observational uncertainty model has absorbed the input uncertainty.  Predictions with uncertain query points can then be done as per Def. \ref{def:KIL} (but with $ \errinp(\cdot)+ \varepsilon(\cdot)$ in place of $\varepsilon(\cdot) )$.


\subsection{A smoothed inference rule}
The inferred predictor of kinky inference as per Eq. \ref{eq:KIpred} contains kinks. In certain applications, this can be disadvantageous. For instance, below we will feed the predictor into a control signal. However, in applications such as robotics, smooth controllers are typically preferred over non-smooth ones since the latter give rise to increase wear and tear of the actuators. With this in mind we will consider a modification of the predictor which filters the prediction output through a smoothing filter as known from computer vision \cite{forsyth2002,Baessmann2004}. The idea is to convolve the predictor with a function that implements a low-pass filter and abates high frequencies thereby smoothing out rough transitions in the signal. 
For now, we will restrict the exposition to one-dimensional input and output spaces. However, extensions to multiple output dimensions result from following our steps through for each component function. Extensions to multi-dimensional input spaces follow by taking advantage of the corresponding filters developed for multi-dimensional signal processing. \jcom{citation??}

As an example, for some $n \in \nat, w_i \geq 0 \, (i=1,...,n)$ and (typically small) step size $\sigma \in \Real \geq 0$, consider the modified prediction rule (\textit{smoothed kinky inference (SKI) rule} ):
%
\begin{equation}
f_n^* = \frac{1}{\sum_{i=-q}^N w_i} 
\sum_{i=-q}^q w_i \predfn (x+i \sigma) .
\end{equation}
%
Either $w_0 = 2$ and $w_{-1}=w_2 =1$ or $w_{-2} = w_2 = 7, w_{-1}=w_1 = 26, w_0 = 41$  are common choices for discrete approximations of a Gaussian filter \cite{Baessmann2004}. 

A comparison of the predictions made by the {smoothed kinky inference rule (SKI) } against the prediction function of the standard kinky inference rule is depicted in Fig. \ref{fig:exSKI1}. As can be seen from the plot, in the SKI prediction the kinks have been smoothed out while all the predictions still are contained within the prediction bounds given by the floor and ceiling functions.

\begin{figure}
        \centering
				  %\subfigure[KI on a sine curve.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/sinKI1}
    %\label{fig:KI1}
  %} 	
	 \subfigure[KI on a sine curve.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/sinKI3}
    \label{fig:KI2}
  } 	%\hspace{2cm}
	  %\subfigure[SKI on a sine curve.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/sinSKI1}
    %\label{fig:SKI1}
		%} 	
	  \subfigure[SKI on a sine curve.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/sinSKI3}
    \label{fig:SKI2}
  } 	
	\label{fig:exSKI1}
   \caption{Comparison of the kinky inference rule (left) versus the smoothed kinky inference rule (right) when predicting a sine curve. Note the smoothed out kinks of the SKI rule due to the application of the smoothing filter. Here we chose $\sigma =0.1$. }
\end{figure}	  

The question arises how the smoothing might affect the theoretical properties. Firstly, we note that due to Lem. \ref{lem:Hoeldarithmetic}, the H\"older exponent and constant remain unchanged. For the constant, we apply point 4 and 9 of the lemma to see that $L(f_n^*) = \frac{1}{\sum_{i=-q}^q w_i} 
\sum_{i=-q}^q w_i L(\predfn (x+i \sigma)) = L(\predf_n) \frac{1}{\sum_{i=-q}^q w_i}  \sum_{i=-q}^q w_i = L(\predfn)$.

Secondly, the question arises what the maximal discrepancy between $\predfn$ and $f_n^*$ is. This question is of importance to make sure that the prediction still is within the bounds given by the ceiling and floor functions. To this end, assume $\predfn$ is H\"older with constant $L$ and exponent $p$. For simplicity assume we utilise Gaussian smoothing for the SKI rule with $n=1$, $w_{-1} = w_1 =1, w_0 =2$. The deviation of this resulting smoothed predictor $f_n^* $ from the kinky inference predictor $\predfn$ can be bounded as follows
\begin{align}
\abs{\predfn(x) - f_n^*(x)} &= \abs{\predfn(x) - \frac 1 {w_{-1}+w_0+w_1} (w_{-1} \predfn(x-\sigma) + w_0 \predfn(x)+ w_1 \predfn(x+\sigma)} \\
&= \frac 1 4 \abs{ 2 \predfn(x) -   \predfn(x-\sigma) - \predfn(x+\sigma)} \\
&\leq  \frac 1 4 \abs{  \predfn(x) -   \predfn(x-\sigma)} + \frac 1 4 \abs{ \predfn(x) - \predfn(x+\sigma)}\\
&\leq  \frac L 4  \metric^p(x,x-\sigma) + \frac L 4 \metric^p(x,x+\sigma).
\end{align}
If the metric is induced by a norm $\norm{\cdot}$ the last expression simplifies to $\frac L 2 \norm{\sigma}^p$.
In order to ensure that uncertainty bound takes this error into account, we can add this error to the uncertainty quantification $\prederrn$. This guarantees that the ground truth is contained within the error bounds around predictions $f_n^*$. Furthermore, since the bound is valid for all inputs $x \in \inspace$, the convergence guarantees established for kinky inference also hold for the smoothed version up to supremum norm error of at most $\sup_{x \in \inspace} \frac L 4  \metric^p(x,x-\sigma) + \frac L 4 \metric^p(x,x+\sigma)$ (which in the norm-based metric case equals $\frac L 2 \norm{\sigma}^p$).

%\subsection{Discussion}
%As we observed, our posterior knowledge coincides with the set of sample-consistent functions. Therefore, an exhaustive enclosure is a superset of $\mathcal K_{prior} \cap \mathcal K_{post}$. 
%Remembering our discussion of topological inference, we realize that all we need to do to solve Task 1 (as specified in Sec. \ref{sec:problemdef_task1}), is to define our data inference mechanism $M_{\text{dinf}}$ to output the optimal enclosure. A prescription for computing the bounds of this enclosure was given in the definitions above. From these, we see that $M_{dinf}$computes in $\mathcal O(N_n d)$. That is, its computational effort (translating to the necessary inference investment $\gamma_{\text{dinf}})$ is linear in the number of samples and dimensionality of the problem. If we deal with maximum-norms, norm computation can be done with computation that is logarithmic in $d$, reducing the overall evaluation effort to $\mathcal O(N_n \log d)$.   

==> content2/Ch_kinkyinf/gridrefinements.tex <==
\section{Grid sequence definitions}
For both the 1-dimensional case and the $d$- dimensional case we have derived convergence guarantees that were based on the assumption, that the grid sequence $(G_N)$ was an eventually dense partition of domain $I$. In this section, we will define grid sequences that satisfy this assumption.

\subsection{Multi-dimensional domains}

As before, for $N \in \nat$, let $H_N$ denote the number of grid hyperrectangles partitioning $I$. 
$G_N =: \{\bigl(c_1^N,f(c_1^N), J_1^N\bigr),\ldots,\bigl(c_{H_N}^N,f(c_{H_N}^{N}), J_{H_N}^{N}\bigr)\}$ being a set of triples consisting of centre points $c_i^N$, function values $f(c_i^N)$ and hyperrectangle $J_i^N$ (centred around $c_i^N$). 
Let $\mathcal J^N = \{ J_i^N | i=1,\ldots,H_N \} $ be the set of all hyperrectangles of grid $G_N$ that partition domain $I$.

We defined $\bar r_i^N = \max\{ r_{i,1}^N,\ldots, r_{i,d}^N\}$ denotes the maximum radius of hyperrectangle $J_i^N = c_i + \bigl([-r_{i,1}^N ,r_{i,1}^N ]\times \ldots \times [-r_{i,d}^N ,r_{i,d}^N ] \bigr)$. Furthermore, $\bar r^N := \max_{i \in \{1,...,N\}} \bar r_i^N$ is the maximum radius of any hyperrectangle in the $N$th partition of $I$.


\subsubsection{Method 1-- Doubling} 

Let $i \in \nat$, $c_{i,j}^N$ be the $j$th component of centre point $c_{i}^N$. We define hyperrectangle 
$J_i^N = c_i + [-r_i^N,r_i^N]^d =  [-r_i^N+c_{i,1}^N,r_i^N+c_{i,1}^N],\ldots,[-r_i^N+c_{i,d}^N,r_i^N+c_{i,d}^N] $ as follows:

Assume $I= [a_1,b_1] \times,...,\times [a_d,b_d]$.


$N=1$: we set $J^1_1 = I$ and $\mathcal J = \{J^1_1 \}$. Hence, the centre point is 
$c_1^1 = (c_{1,j}^1)_{j=1,...,d}$ where $c_{1,j}^1 = \frac{b_j-a_j}{2}$.

$N\geq 1$:  For $j=1,...,d:$ We partition the projection $[a_j,b_j]$ of the domain onto the $j$th axis into $2^N-1$ intervals $J_{1,j}^N = [a_j,a_j+ \frac{b_j-a_j}{2^N-1}],\ldots, J_{2^N-1,j}^N = [a_j+(2^N-2) \frac{b_j-a_j}{2^N-1},a_j+ (2^N-1) \frac{b_j-a_j}{2^N-1}] $ of length $l_{j}^N=\frac{b_j-a_j}{2^N-1}$.
That is, $J_{k,j}^N =[a_j + (k-1)\, l_j^N ,a_j+ k \, l_j^N]$ $(k=1,...,2^N-1, j=1,...,d)$.   

We set \[ \mathcal J^N := \bigl\{ J_{k_1,1}^N\times \ldots \times J_{k_d,d}^N \, \vert \, k_1,...,k_d \in \{1,...,2^N-1 \}\,   \bigr\}.\]

Note, we have $H_N = |J^N| = (2^N-1)^d$.

By definition, the intervals on the $j$th axis were of uniform length $l_{j}^N=\frac{b_j-a_j}{2^N-1}$.
With $r_{i,j}^N = \frac{l_j^N}{2} \, (i=1,...,H_N)$ we have   \[\bar r^N = \max_{i,j} r_{i,j}^N =  \max_{j \in \{1,...,d\}} \frac{b_j-a_j}{2^N-1} \stackrel{N \to \infty}{\longrightarrow} 0.\]

Therefore, the resulting grid sequence is an eventually dense partition of $I$ (cf. Def. \ref{defn:eventuallydensepartition}) as desired.  

\subsubsection{Method 2-- Incremental refinement}
Next, we will define a gridding method that incrementally refines the grid. 
This can be be of interest if our computational budget is not allowing us to evaluate a power of two function values, or, 
if a regular grid is not ideal. The latter could be the case, for instance, when the Lipschitz constant is not uniform over $I$. In this case it may be beneficial to refine the grids with a higher resolution in regions of the domain where the Lipschitz constant is large. Or, if we want to use our conservative function estimates to answer the question whether the target function ever drops below a certain threshold (as we will want to do in the context of collision detection), we may not choose to refine the estimate in regions where the Lipschitz floor is positive. 

In order to refine grids we proceed as follows:



%\IncMargin{-1em}
%\begin{algorithm}
%\begin{small}
%\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up} \SetKwData{Constraints}{Constraints} 
 %\SetKwData{Collisions}{Collisions} \SetKwData{flag}{flag} \SetKwData{C}{$\mathfrak C$} \SetKwData{winner}{winner} \SetKwData{tcoll}{$t_{\text{coll}}$}
%\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress} \SetKwFunction{Resolve}{Resolve}
%\SetKwFunction{Broadcast}{Broadcast} \SetKwFunction{Planner}{Planner} \SetKwFunction{Auction}{Auction}
%\SetKwFunction{Receive}{Receive} \SetKwFunction{Avoid}{Avoid}
%\SetKwFunction{DetectCollisions}{CollDetect}
%\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%%
%\Input{Agents $\agi \in \agset$, cost functions $c^\agi$, dynamics, initial start and goal states, initial plans $p^1,...,p^{|\agset|}$ .}
%\Output{collision-free plans $p^1,...,p^{|\agset|}$.}
%\BlankLine
%%\emph{special treatment of the first line}\;
%\Repeat{$\forall \agi \in \agset: \flag^\agi =0 $}
%{
%\For{$\agi \in \agset$}{[
%\flag$^\agi,\C^\agi,\tcoll ]\leftarrow$ \DetectCollisions$^\agi (\agi, \agset-\{\agi\})$\\
%
%\If{$\flag^\agi =1$}
%{
%$\winner \leftarrow \Auction(\C^\agi \cup \{\agi\},\tcoll )$\\
%\ForEach{$\agii \in (\C^\agi \cup \{\agi\})-\{\winner\} $}{
%$p^\agii \leftarrow \Avoid^\agii((\C^\agi \cup \{\agi\})-\{\agii\},\tcoll )$\\
%$\Broadcast^\agii$ ($p^\agii$)
%}
%}
%
%}
%
%}
%\caption{Lazy auction coordination method (AUC) (written in a sequentialized form). Collisions are resolved by choosing new setpoints to enforce collision avoidance. 
%$\mathfrak C^\agi$: set of agents detected to be in conflict with $\agi$. flag$^\agi$: collision detection flag (=0, iff no collision detected). 
%$t_{\text{coll}}$: earliest time where a collision was detected. Avoid: collision resolution method updating the plan by a single new setpoint according to WAIT or FREE ( ref. (II), Sec. \ref{sec:avoidance}).}
%
%\label{alg:lazyauctions}
%\end{small}
%\end{algorithm}

%\IncMargin{-1em}
\begin{algorithm}
\begin{small}
%\SetKwData{flag}{flag}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\SetKwFunction{SelectHyperrectangle}{SelectHyperrectangle}
\SetKwFunction{RefineGrid}{RefineGrid}
\SetKwFunction{SplitRectAlongDim}{SplitRectAlongDim}

%
\Input{Set of hyperrectangles $S=\{J_1,...,J_{H_{N-1}} \}$, $J_i =  c_i +\prod_{j =1}^d \, [-r_{i,j},r_{i,j}] $}
\Output{Refined set of hyperrectangles $S'= J_1,...,J_{H_{N}}$}
\BlankLine
%\emph{special treatment of the first line}\;
%$\flag \leftarrow 0$;\\
$\mathfrak J = c+ \prod_{j =1}^d [-r_j,r_j] \leftarrow \SelectHyperrectangle(S)$;\\ %choose a hyperrectangle to refine
$ m \leftarrow \arg \max_{j \in \{1,....,d\}} r_j$;\\
%$Q := \{\mathfrak J_1, \mathfrak J_2, \mathfrak J_3\} \leftarrow \SplitRectAlongDim(\mathfrak J,m)$;
$\{J',J'',J'''\} \leftarrow \SplitRectAlongDim (\mathfrak J,m);$\\
$S' \leftarrow (S \backslash \{\mathfrak J\}) \cup \{J', J'', J'''\}$;\\
return $S'$;

\caption{Function \texttt{RefineGrid}. Incremental grid refinement.}

\label{alg:incgridrefinement1}
\end{small}
\end{algorithm}


%-------------------------------------------------------------------------
\begin{algorithm}
\begin{small}
%\SetKwData{flag}{flag}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\SetKwFunction{SelectHyperrectangle}{SelectHyperrectangle}
\SetKwFunction{RefineGrid}{RefineGrid}
\SetKwFunction{SplitRectAlongDim}{SplitRectAlongDim}

%
\Input{Hyperrectangle $J =  \vc c +\prod_{j =1}^d \, [-r_{j},r_{j}] $, dimension $m \in \{1,...,d\}$.}
\Output{Three hyperrectangles $J',J'',J'''$ partitioning $J$.}
\BlankLine
%\emph{special treatment of the first line}\;
%$\flag \leftarrow 0$;\\
$\vc c' \leftarrow \vc c - \frac{2 r_m}{3} \vc{e_m}$; $\vc c'' \leftarrow c$;
$\vc c''' \leftarrow \vc c + \frac{2 r_m}{3} \vc{e_m}$;\\
$\mathfrak I \leftarrow   \prod_{j =1}^{m-1} \, [-r_{j},r_{j}] \times [\frac{-1}{3} r_m,\frac{1}{3}r_m]\times \prod_{j =m+1}^d \, [-r_{j},r_{j}] $;\\
$J' \leftarrow \tilde c' + \mathfrak I$; $J'' \leftarrow \tilde c'' + \mathfrak I$; $J''' \leftarrow \tilde c''' + \mathfrak I$;\\

\caption{Function \texttt{SplitRectAlongDim}. Compart an input hyperrectangle into three sub-hyperretangles along the $m$th dimension. Each output hyperrectangle is one third of the volume of the original one. }

\label{alg:incgridrefinement1}
\end{small}
\end{algorithm}


Our approach to incremental grid refinment is similar to DIRECT... blahblah-cite.

The remaining issue is how to choose which hyperrectangle to refine. That is, we need to flesh out function 
\texttt{SelectHyperrectangle}. The answer as to how to make this choice depends on our objective. 

For instance, in the \textit{ estimation problem} we may be interested in making refinements that maximally reduce the maximal error on the domain.
That is we would choose to refine sub-hyperrectangle $J_q$ such that  
\begin{align}
q &= \argmax_{i=1}^{H_N} \sup_{x \in J_i} \decke_N^i (x) - \boden_N^i(x) \\
& \stackrel{Lem. \ref{lem:supinfonJimultidim}}{=} \argmax_{i=1}^{H_N} 2 \ell_i \max_{j=1}^d r_{i,j}^N.
\end{align}

Here, the choice of refinement only depends on the Lipschitz constant and the maximal expansion of the hyperrectangle in any dimension.

By contrast, in the \emph{threshold problem}, where we desire to test the hypothesis that the function drops below a certain threshold $\theta$, our choice of expansion should also depend on the function value in question. For instance, so far, all of our function evaluations $f(c_1),...,f(c_{H_N})$ have not dropped below $\theta$. Faced with the choice which hyperrectangle to split next, we may pick the hyperrectangle $J_i$ where the reduction of integral below $\theta$ after the split is maximal. Of course, here the actual function values may come into play. Unfortunately, this means that if our actual goal is to choose a regions such that the splitting results in a maximal decrease of the area of our conservative estimate under the threshold $\theta$, we would have to sample the target function at all candidate hyperrectangles before making our decision. In cases where obtaining such samples is expensive this may be infeasible. In such cases, practicality might suggest a heuristic approach. That is, we might simply pick the hyperrectangle whose current area under $\theta$minimum value is largest. That is, choose $J_q$ such that
\begin{align}
q &= \argmax_{i=1}^{H_N} \int_{J_i} \abs{\min\{ \theta, \boden_N^i(x)\}} \, dx. \\
\end{align}
Alternatively, we may choose to refine $J_q$ to be the hyperrectangle with the lowest value. That is to say,

\begin{align}
q &= \argmin_{i=1}^{H_N} \inf_{x \in J_i} \boden_N^i(x) \\
 &= \argmin_{i=1}^{H_N}  f(c_i) - \ell_i  \max_{j \in \{1,...,d\}} r_{i,j}^N \\
\end{align}

where the last equality follows from Lem. \ref{lem:supinfonJimultidim}.


....
....

....

Finally, in the conservative integration problem, we may choose to elect our next hyperrect $J_q$ for refinement such that 

\begin{align}
q &= \argmax_{i=1}^{H_N} \int_{J_i} \decke_N^i (x) - \boden_N^i(x) \, \d x \\
& = \argmax_{i=1}^{H_N} 2 \ell_i \int_{J_i}  \norm{x-c_i}_\infty \, \d x.
\end{align}

Fortunately, the definite integrals can be computed in closed-form utilizing Lem. \ref{lem:defint_of_maxnorm}. Furthermore, determination of $q$ is independent of the additional function values to be sampled in $J_i$.


\subsubsection{Method 0 -- Batch grid}
For now, we assume we are given a finite function sample of ${H_N}$ evaluations $\{\bigl(c_1^N,f(c_1^N)\bigr),\ldots,\bigl(c_{H_N}^N,f(c_{H_N}^{N})\bigr)\}$ without access to additional function values. How should we construct a grid $G_N$ for conservative estimation and quadrature?

That is, we need to determine $J_N^1,...,J_N^{H_N}$ with centre points $c_1^N,...,c_{H_N}^N$, respectively, that partition domain hyperrectangle $I$.

To this end, we consider the centre-point projections onto the $j$th axis and define a permutation $\mathfrak p_j \in \text{Perm}(H_N)$ such that $c_{\mathfrak p (1),j}^N \leq \ldots \leq c_{\mathfrak p (H_N),j}^N$.

...Ok...should not use centre points... but instead the framework with flexible samples.
Can solve this with Alg. \ref{alg:recursivequad1}. However, this one scales poorly in the dimensionality of the integrand's domain.

==> content2/Ch_kinkyinf/intersectionsofenclosure.tex <==
\section{Incorporation of additional knowledge}
So far, our knowledge was confined to Lipschitz continuity. This yielded the definition of the Lipschitz enclosure $\einschluss$ for which we proved convergence to the ground truth in the limit of an infinite number of function samples $N$. Often however, we may actually have additional knowledge about our target function $f$. Such information could translate to another set $F_N$ of function for which this additional piece of knowledge holds true. For instance, if our method was to be applied to marginalization in Bayesian inference, we would know that the integrands involved are nonnegative. In this case, we would have $F_N =\{ \phi: I \to \Real | \phi(x) \geq 0, \forall x \in I\}$. 
In such a case, we would consider the somewhat less conservative enclosure 
$F_N \cap \einschluss$ to represent our uncertainty about $f$ (and to base our $ceiling$ and $floor$ functions on).

If we can define $F_N$ by a ceiling and floor function $b_N,a_N$, $F_N = \{\phi : I \to \Real | a_N(x) \leq \phi(x) \leq b_N(x) \}$, then $F_N \cap \einschluss$ is given by the ceiling function $\Gamma_N: x \mapsto \min\{b_N(x), \decke_N(x) \}$ and floor function $\Phi_N:  x \mapsto \max\{a_N(x), \boden_N(x) \}$:
$F_N \cap \einschluss = \{ \psi : I \to \Real | \Phi_N(x) \leq \psi(x) \leq \Gamma_N(x) \}$.
In our example with additional non-negativity constraints, we would have $\Gamma_N (x) = \infty$ and $\Phi_N(x) = 0$ $\forall x \in I$.

Ignoring this information may yield unnecessarily conservative estimates. 
Therefore, we should work with $\Gamma_N$ and $\Phi_N$.

All we need to do is to show that the convergence properties extend.

\begin{thm}\label{thm:trunkunifconv}
Let $(\decke_N)_{N \in \nat}, (\boden_N)_{N \in \nat}$ be two sequences of functions, $\decke_N,\boden_N: I \subset \Real^d \to \Real$, converging to function $f: I \to \Real$ uniformly on $I$ as $N \to \infty$.
Furthermore, let $\mathfrak b, \mathfrak a : I \to \Real$ be two functions such that $\forall x \in I: 
\mathfrak b(x) \geq f(x) \geq \mathfrak a(x)$. For all $N \in \nat$, define $\Phi_N: x \mapsto \max\{\mathfrak a(x),\boden_N(x) \}$ and $\Gamma_N: x \mapsto \min\{\mathfrak b(x),\decke_N(x) \}$.
These function sequences also converge uniformly to $f$: 

$\Gamma_N, \Phi_N \stackrel{N \to \infty}{\longrightarrow} f$ uniformly on $I$.
\begin{proof}
We prove uniform convergence of $(\Phi_N)$. The proof for uniform convergence of $(\Gamma_N)$ is completely analogous and can be omitted.


Uniform convergence of $(\boden_N)$ to $f$  is equivalent to the predicate $\forall \epsilon >0 \exists N_0 \forall N \geq N_0\forall x \in I: \abs{\boden_N(x) - f(x)} < \epsilon$. 

Let $\epsilon > 0$ and choose $N_0$ such that $\forall N \geq N_0, x \in I$ we have 
$\abs{\boden_N(x) - f(x)} < \epsilon$. Choose $N \geq N_0, x\in I$.
Consider $\abs{\Phi_N(x) - f(x)}$. 

Case I: Let $\mathfrak a(x) = f(x)$. Hence, $\abs{\Phi_N(x) - f(x)}
{=} \abs{\max\{\mathfrak a(x),\boden_N(x) \} - f(x)}$
$\stackrel{\boden_N(x) \leq f(x)}{=} \abs{f(x) - f(x)} = 0 < \epsilon$.

Case II: Let $\mathfrak a(x) < f(x)$. Hence, $\mathfrak a(x) = f(x) - \delta_x$, for some $\delta_x >0$.
Due to uniform convergence (and since $\boden_N(x) \leq f(x)$), we have $\exists \tilde N \forall N \geq \tilde N: f(x) - \boden_N(x) < \delta_x$. In particular, for any $N \geq \bar N := \max\{\tilde N, N_0\}$ we have:  $f(x) - \boden_N(x) < \delta_x$. Hence, $\forall N\geq \bar N: a(x) < \boden_N(x)$.
Thus, $\forall N\geq \bar N:  \abs{\Phi_N(x) - f(x)}
{=} \abs{\max\{\mathfrak a(x),\boden_N(x) \} - f(x)}
\stackrel{\bar N \geq N_0}{=} \abs{\boden_N(x) - f(x)} < \epsilon
$.
\end{proof}


\end{thm}
\subsection{Definite integrals}
So far, we have established uniform convergence of the truncated estimates $\Gamma_N$ and $\Phi_N$ to the target. As an immediate consequence Thm. \ref{thm:trunkunifconv}, in conjucntion with Thm. \ref{thm:defintconv_multidim} allow us to conclude that the definite integrals converge to the desired target integral, in the limit of infinite sample points:


\begin{thm}\label{thm:defintconv_multidim_trunkated}
If the grid sequence $G_N$ becomes dense in domain $I$ we have 
\[\forall N \in \nat : \int_I \Gamma_N(x) \, d x \geq \int_I f(x) \, d x \geq  \int_I  \Phi_N \, d x \]

\[ \int_I \Gamma_N(x) \, d x,  \int_I  \Phi_N \, d x  \stackrel{N \to \infty}{\longrightarrow} \int_I f(x) \, d x.  \]
\end{thm} 

It remains to derive closed-form expressions for the estimate integrals $\int_I \Gamma_N(x) \, d x$ and  $\int_I  \Phi_N \, d x $. Of course, this depends on the definitions of the bounding functions $\mathfrak a_N , \mathfrak b_N$. As a special case of particular importance, we consider the case where our additional knowledge is that our target function cannot be nonnegative. That is, $F_N =\{ \phi: I \to \Real | \phi(x) \geq 0, \forall x \in I\}$ and so, $\forall x: \mathfrak a_N(x) = 0, \mathfrak b_N(x) = \infty$. Therefore, $\int_I \Gamma_N(x) \, d x = S^\decke_N$ as above. So, the only integrals we need to be concerned about are the lower bound integrals $\int_I  \Phi_N \, d x$ where in our case, $\Phi_N^i (x) = \max\{0,\boden^i_N(x)\}$.
How to calculate its definite integral is subject to the following theorem:

\begin{thm}
Let $\Phi_N (x) = \max\{0,\boden_N(x)\}, \Phi^i_N (x) = \max\{0,\boden^i_N(x)\}$ and $J_i = c_i +\prod_{j=1}^d [-r_{i,j},r_{i,j}]$. 
Furthermore, let $\underline J_i = c_i + \prod_{j=1}^d [-p_{i,j},p_{i,j}] $ 
where $p_{i,j} := \min\{\frac{f(c_i)}{\ell_i},r_j \}$.
We have $\int_I \Phi_N(x) \, dx = \sum_i\int_{J_i} \Phi^i_N(x) \, dx$ where 
\[\int_{J_i} \Phi^i_N(x) \, dx = \int_{\underline J_i} \boden^i_N(x) \, dx.  \]
\begin{proof}
We show that $\underline J_i \subset J_i$ is the support of $\Phi^i_N$ on $J_i$. (Since $\Phi^i_N(x) = \max\{ 0, \boden^i_N(x) \} \geq 0, \forall x$ this implies 
$\int_{J_i} \Phi^i_N(x) \, dx = \int_{\underline J_i} \boden^i_N(x) \, dx$ as desired.)

$x \in J_i \cap \text{supp } \Phi^i_N \Leftrightarrow x \in J_i \wedge \boden^i_N(x) \geq 0$ 
$\stackrel{def.}{\Leftrightarrow} x \in J_i \wedge \frac{f(c_i)}{\ell_i} \geq \norm{x-c_i}_\infty$ 
${\Leftrightarrow} \forall j \in {1,...,d}: x_j    \in c_{i,j} + [-r_{i,j},r_{i,j}] \wedge \frac{f(c_i)}{\ell_i} \geq \abs{x_j-c_{i,j}}$
${\Leftrightarrow} \forall j \in {1,...,d}: x_j    \in c_{i,j} + [-r_{i,j},r_{i,j}] \wedge \frac{f(c_i)}{\ell_i} + c_{i,j}  \geq x_j \geq -\frac{f(c_i)}{\ell_i} + c_{i,j}$
${\Leftrightarrow} \forall j \in {1,...,d}: x_j    \in c_{i,j} + \bigl([-r_{i,j},r_{i,j}]\cap [-\frac{f(c_i)}{\ell_i}, \frac{f(c_i)}{\ell_i}] \bigr)$
%
$\Leftrightarrow x    \in c_{i} + \prod_j [-\min\{r_{i,j}, \frac{f(c_i)}{\ell_i}\} , \min\{r_{i,j}, \frac{f(c_i)}{\ell_i}\}]$.

\end{proof}
\end{thm}
Note, each term $\int_{\underline J_i} \boden^i_N(x) \, dx$ can be calculated as derived above. Therefore, the theorem is a recipe for closed-form calculation of $\int_I \Phi_N(x) \, dx$.

==> content2/Ch_kinkyinf/intro.tex <==
\section{Introduction} Quadrature is key in a multitude of contexts including
probabilistic inference, numerical solutions to differential equations and their applications to optimal control. In many practically relevant
cases, integrals cannot be calculated in closed-form rendering it
necessary to resort to numerical approximation. 
A large number of numerical quadrature methods exist that allow a quantification of the error of the integrals estimate. This becomes 

While existing
methods guarantee convergence in the limit of infinite integrand
evaluations, the estimate of the integral may be either larger or
smaller than the true value. This renders those methods unsuitable
in situations where we desire a conservative estimate of the
integral in questions; that is, where we desire to guarantee that
our estimate is either always at least as large or at most as large
as the true integral.

In this paper, such a method for conservative integration is
developed. Our method is applicable in all cases where the integrand
is Lipschitz continuous. As an example application, we utilize our
quadrature method to compute conservative estimates of the collision
probability of stochastic trajectories of multiple objects.

\subsection{Problem 1 -- Erroneous samples, uncertain Lipschitz constant}
\textbf{Problem 2:} Let $I=[a_1,b_1] \times \ldots \times [a_d,b_d] \subset \Real^d$ be a hyperrectangle. For an unknown function $f: I \to \Real$ we are given access to an oracle $O_f:  I \subset \Real^d \times \Real_+ \to \Real^2$ that, incurring  an oracle query cost $\Gamma_O(x,\epsilon_x)$, we can query about target function value $f(x)$ up to error $\epsilon_x > 0$. That is, $O_f(x,\epsilon_x) = V_x := [\underline f(x), \overline f(x)] \subset \Real$ such that it is guaranteed that $f(x) \in V(x) $ and $|V(x)| \leq 2 \epsilon_x$. The oracle could be a numerical approximation procedure to compute target $f$ at input $x$ up to error $\epsilon(x)$ and oracle $\Gamma_O(x,\epsilon(x) )$ could be the algorithm's run-time. In quadrature, it becomes useful to have additional knowledge $K_f$ about the underlying target function. In classical quadrature, this often is knowledge about the maximum value of a $k$th - order derivative.  
In contrast, and allowing wider applicability, we assume this knowledge consists of an uncertain Lipschitz constant $L >0$ drawn from a distribution $P_L$.

Let $D_N = \Bigl( (x_1, V_{x_1}),\ldots,(x_N, V_{x_N}) \Bigr)$ be a set of $N$ samples
and define a function of permissible error $\epsilon : I \to \Real_+, x\mapsto \epsilon_x$.

\begin{defn}[Solution method]
A solution method $M_P = (E,Q)$ for problem $P = (I,O_f,\Gamma_O,K_f)$ consists of 
\begin{itemize}
 \item A sequence of incremental query generation functions $Q_N: D_N \mapsto x_{N+1}$; $\tilde Q_N: D_N \mapsto D_N \cup \{x_{N+1}\}$. 
With initial query set $D_0 = \emptyset$, we can the query set generation function $Q: \nat \to 2^{\nat}$, $Q(N; I, O_f) :=  \tilde Q_N \circ \ldots  \tilde Q_0 \circ D_0 $;
 \item An error estimator, i.e. $E: D_N \mapsto  [\underline S (D_N), \overline S (D_N) ] \subset\Real^2$  based on sample $D_N$;
\item An integral estimator $S: D_N \mapsto  \hat S_N$ where $\hat S_N$ is an estimate of target function integral $\mathcal I = \int_I f(x) \d x$ -- e.g. one could set $S(D_N) := \frac{\underline S (D_N) + \overline S(D_N)}{2}$.
 \end{itemize}
\end{defn}

\begin{defn}[Total cost of a method]

We define  \emph{ total horizon cost} $\Gamma_N(M)$ up to horizon $N$ of method $M = (E,P)$)  as   
\[\Gamma_N(E,Q) := \abs{E(D_N)} + \beta\Bigl( \sum_{i=1}^N \Gamma_O \bigl(x_i,\epsilon(x_i)\bigl), \sum_{i=1}^N \Gamma_{Q_i}(D_i), \Gamma_a(E(D_N) \Bigr).\] Here, 
\begin{itemize}
\item $\Gamma_{Q_i}$ is a query generation cost. For instance, it could be the time required to compute $Q_i(D_i)$;
\item $\Gamma_O$ is the oracle cost as defined before. For instance,  
\item $\Gamma_a (E(D_N))$ is a cost for evaluating and returning the algorithm's output.
\item $\beta: \Real \to \Real$ is a term penalizing processing cost. For example, we could set $\beta (\omega,\sigma,\alpha) = \lambda \max(0, \omega + \psi + \alpha - b), \lambda \approx \infty$ penalizing a solution that exceeds spending more than permitted by budget level $b$.
\end{itemize}
\end{defn}

Given problem $P$ we aim to design a method $M$ fulfilling the following \textbf{desiderata}:
\begin{enumerate}
 \item $\lim_{ N \to \infty} \abs{\hat S_N  - \int_I f(x) \d x} = 2 \int_I \epsilon(x) \d x$ (where convergence is uniform) with probability at least $\delta \in (0,1)$ 
 \item The error vanishes uniformly with increasing sample size: $\abs{E (D_N)} = \abs{\overline S(D_N) - \underline S(D_N)} \stackrel{N \to \infty}{\longrightarrow} 2 \int_I \epsilon(x) \d x$ with probability at least $\delta \in (0,1)$. 
\item The error estimator is \textit{anytime conservative.} That is, for all $N \in \nat, D_N$ it is guaranteed that $\mathcal I \in E (D_N)$ with probability at least $\delta \in (0,1)$;
\item The total horizon costs $\Gamma_N (M)$  are as small as possible $(N \in \nat)$. 
 \end{enumerate}

In this paper we will develop solution methods for our given quadrature problem. The total horizon costs give as a criterion with which to compare the performance of different methods subject to our convergence desiderata. ...


\subsection{Problem 2 -- Erroneous samples, known Lipschitz constant}
We now consider a special case of Problem 1:
\textbf{Problem 2:} Let $I=[a_1,b_1] \times \ldots \times [a_d,b_d] \subset \Real^d$ be a hyperrectangle. For an unknown function $f: I \to \Real$ we are given access to an oracle $O_f:  I \subset \Real^d \times \Real_+ \to \Real^2$ that, incurring  an oracle query cost $\Gamma_O(x,\epsilon_x)$, we can query about target function value $f(x)$ up to error $\epsilon_x > 0$. That is, $O_f(x,\epsilon_x) = V_x := [\underline f(x), \overline f(x)] \subset \Real$ such that it is guaranteed that $f(x) \in V(x) $ and $|V(x)| \leq 2 \epsilon_x$. The oracle could be a numerical approximation procedure to compute target $f$ at input $x$ up to error $\epsilon(x)$ and oracle $\Gamma_O(x,\epsilon(x) )$ could be the algorithm's run-time.
In quadrature, it becomes useful to have additional knowledge $K_f$ about the underlying target function. In classical quadrature, this often is knowledge about the maximum value of a $k$th - order derivative.  
In contrast, we base our consideration on the more general assumption that our knowledge consists of a Lipschitz constant $L >0$. Since all differentiable functions are Lipschitz (but not the other way around), our method applies to a wider scope of target functions.

Let $D_N = \Bigl( (x_1, V_{x_1}),\ldots,(x_N, V_{x_N}) \Bigr)$ be a set of $N$ samples
and define a function of permissible error $\epsilon : I \to \Real_+, x\mapsto \epsilon_x$.

\begin{defn}[Solution method]
A solution method $M_P = (E,Q)$ for problem $P = (I,O_f,\Gamma_O,K_f)$ consists of 
\begin{itemize}
 \item A sequence of incremental query generation functions $Q_N: D_N \mapsto x_{N+1}$; $\tilde Q_N: D_N \mapsto D_N \cup \{x_{N+1}\}$. 
With initial query set $D_0 = \emptyset$, we can the query set generation function $Q: \nat \to 2^{\nat}$, $Q(N; I, O_f) :=  \tilde Q_N \circ \ldots  \tilde Q_0 \circ D_0 $;
 \item An error estimator, i.e. $E: D_N \mapsto  [\underline S (D_N), \overline S (D_N) ] \subset\Real^2$  based on sample $D_N$;
\item An integral estimator $S: D_N \mapsto  \hat S_N$ where $\hat S_N$ is an estimate of target function integral $\mathcal I = \int_I f(x) \d x$ -- e.g. one could set $S(D_N) := \frac{\underline S (D_N) + \overline S(D_N)}{2}$.
 \end{itemize}
\end{defn}

\begin{defn}[Total cost of a method]

We define  \emph{ total horizon cost} $\Gamma_N(M)$ up to horizon $N$ of method $M = (E,P)$)  as   
\[\Gamma_N(E,Q) := \abs{E(D_N)} + \beta\Bigl( \sum_{i=1}^N \Gamma_O \bigl(x_i,\epsilon(x_i)\bigl), \sum_{i=1}^N \Gamma_{Q_i}(D_i), \Gamma_a(E(D_N) \Bigr).\] Here, 
\begin{itemize}
\item $\Gamma_{Q_i}$ is a query generation cost. For instance, it could be the time required to compute $Q_i(D_i)$;
\item $\Gamma_O$ is the oracle cost as defined before. For instance,  
\item $\Gamma_a (E(D_N))$ is a cost for evaluating and returning the algorithm's output.
\item $\beta: \Real \to \Real$ is a term penalizing processing cost. For example, we could set $\beta (\omega,\sigma,\alpha) = \lambda \max(0, \omega + \psi + \alpha - b), \lambda \approx \infty$ penalizing a solution that exceeds spending more than permitted by budget level $b$.
\end{itemize}
\end{defn}

Given problem $P$ we aim to design a method $M$ fulfilling the following \textbf{desiderata}:
\begin{enumerate}
 \item $\lim_{ N \to \infty} \abs{\hat S_N  - \int_I f(x) \d x} = 2 \int_I \epsilon(x) \d x$ where convergence is uniform. 
 \item The error vanishes uniformly with increasing sample size: $\abs{E (D_N)} = \abs{\overline S(D_N) - \underline S(D_N)} \stackrel{N \to \infty}{\longrightarrow} 2 \int_I \epsilon(x) \d x$. 
\item The error estimator is \textit{anytime conservative.} That is, for all $N \in \nat, D_N$ it is guaranteed that $\mathcal I \in E (D_N)$;
\item The total horizon costs $\Gamma_N (M)$  are as small as possible $(N \in \nat)$. 

 \end{enumerate}

In this paper we will develop solution methods for our given quadrature problem. The total horizon costs give as a criterion with which to compare the performance of different methods subject to our convergence desiderata. ...




\subsubsection{Idea on the side: Automated Algorithm Generation by solving a Variational Extremization Problem}
Can we just find a solution method as a solution to the variational problem ?:

\[ \min_{E \in \mathcal E,Q \in \mathcal Q} \sum_{N=1}^\infty \alpha_N \Gamma_N(E,Q) \] where the $\alpha_N$ are discount factors and $E,Q$ need to be appropriately constrained...

Some thoughts:
\begin{itemize}
	\item $\mathcal Q$, the space of all possible $Q$ functions, should essentially be isomorph (I hope) to the set of all countably infinite sequences contained in target domain $I$. I believe we could use diminishing returns properties to limit ourselves to $\ell_2(I)$ sequences (which should contain dense sequences in $I$). That means we should be able to recast the optimization problem as a search for $Q \in l_2(I) $. This now is a variational problem as $l_2(I) $ is isomorph to $L_2(I)$ as far as I recall (or some other well-behaved class of functions). Of course I am not sure how to recast the objective. 
	\item If we can do it for $Q$, the analogous statement should be derivable for $E$. 
	\item Assume, $\epsilon(x) = 0$. Perhaps we can set $\alpha_N : = \abs{E(D_N)}$. This makes sure that the series is not convergent unless $E(D_N) \to 0$ as desired. Not sure how to go about anytime conservativeness
	but that could be lifted and still the approach would be awesome.
	
	\item In fact, if we restrict ourselves to horizons up to a certain order, things should become even a bit easier. This should not be a problem, if our computational budget is restricted anyway as in the example above. Then, the problem degenerates to effectively a finite-dimensional optimization problem (I think).
	\item Additional knowledge (such as the Lipschitz constant) could go into the definition of the function spaces (or into the objective function).
	\item Of course, the whole method is not restricted to quadrature!
	 
\end{itemize}

\subsubsection{Other hunch: Dynamical system}
$Q$ describes the dynamics of a symbolic dynamical system...

\subsection{Coming up with examples:}
Solving for a mean in an SDE whose drift parameters were determined by a probabilistic system identification method -- > gives density over Lipschitz constant... work that out!





==> content2/Ch_kinkyinf/kinkyinf_root.tex <==
%\begin{abstract}
%\begin{quote}
%\input{content/content_hoelderquad2/abstract}
%\end{quote}
%\end{abstract}

%\noindent
%In this chapter, we propose a method for inductive inference that yields error bounds on the accuracy of the drawn conclusions. 
%The approach yields a non-parametric machine learning method which is applied to system identification and control. The provided error bounds are an attractive property since they offer guidelines for adjusting the control to take the remaining uncertainty of a partially identified system into account. This is shown to be beneficial in settings where we desire to impose robustness constraints on collision avoidance or stability and helps to guide state space exploration in active learning. Based on our nonparametric inference rule, we construct a variety of learning-based controllers for some of which we provide guarantees of stability and construct robust tubes. In addition to our theoretical guarantees, our simulations suggest that kinky inference is a very flexible and fast learning approach that is well suited for learning and controlling dynamical systems and that it can outperform state-of-the-art methods. 
%
%
%
%
\vspace{-3em}
\section{Introduction}
In order to generalise beyond an observed sample, inductive inference needs to make assumptions about the underlying ground truth function. In this chapter, we will derive non-parametric learning and inference methods that fold in knowledge about boundedness, H\"older continuity and error bounds on the observations and inputs. Since these types of a priori knowledge impose weak forms of regularity, the method will be applicable to non-smooth functions that contain kinks- a property that is reflected in the predictions of the inference method and that gave rise to the catch-phrase \emph{kinky inference}.
While weak enough an assumption to encompass rich function classes, the approach has the advantage of yielding bounds on the inference.

The approach yields a non-parametric machine learning method which is applied to system identification and control. The provided error bounds are an attractive property since they offer information on bounded stability and provide guidelines for adjusting the control to take the remaining uncertainty of a partially identified system into account. This can be beneficial in settings where we desire to impose robustness constraints on collision avoidance (see Sec. \ref{sec:KIMRAC}) or stability and can help to guide state space exploration in active learning. Based on our nonparametric inference rule, we construct a variety of learning-based controllers for some of which we provide guarantees of stability and construct robust tubes. In addition to our theoretical guarantees, our simulations suggest that kinky inference is a very flexible and fast learning approach that is well suited for learning and controlling dynamical systems and that it can outperform state-of-the-art methods. 


%\subsection{Related Work}
%Supervised machine learning algorithms construct models of functions to generalise from a data set of function values. We are interested in developing a method that can quantify the uncertainty around the predictions inferred from the learned model. Few methods seem able to do so, with the exception of Bayesian methods. To the best of our knowledge, Gaussian process regression is the only approach in Bayesian inference that combines the capablity to learn rich function classes with analytic tractability on the other (cf. Sec. \ref{GPbackground}, \cite{GPbook:2006}).
%%
%%By contrast, Gaussian processes learning is an example of a nonparametric machine learning method (cf. Sec. \ref{GPbackground}). 
%
%As is the case with most nonparametric learning methods, the computational complexity for training and prediction of GPs grows with number of training examples. In fact, the computational complexity for training is cubic and the computational complexity for inference (prediction) is quadratic in the number of data points \cite{GPbook:2006} (although the former can be reduced to quadratic either approximately \cite{Gibbs1997} or exactly for specific cases \cite{Storkey1999} and the latter effort can be reduced to linear growth by recent SDE conversion techniques \cite{Reece2010,SimoAISTATS2012}). As in most non-parametric methods, the increased computational complexity is rewarded with a reduced inductive bias. That is, when choosing the right covariance function, Gaussian processes can learn any smooth function. Unfortunately, to date it is not well-understood how to fold in the uncertainty quantifications of GPs into the predictions of state-dependent system dynamics in a conservative (that is uncertainty-preserving) manner. This is important if we desire to give error bounds on the control success of a control law that is based on an uncertain dynamics model identified by a GP.
%
%In this work, we go an alternative route. Instead of placing a prior measure over some probability space of function values, we leverage a priori knowledge about H\"older continuity and boundedness of the ground-truth function.
%%
%%In order to generalise beyond unobserved function values kinky inference utilises assumptions of H\"older regularity and, in so far available, information of boundedness of the ground truth function. 
%
%H\"older continuity is a generalisation of Lipschitz continuity. While not being harnessed much within the artificial intelligence and machine learning communities, Lipschitz properties are widely used in applied mathematics to establish error bounds and, among many other, finds application in optimisation \cite{Shubert:72,direct:93} and quadrature \cite{Baran2008,curbera1998,dereich2006}. Upon submission of this work, we also have become aware of related work in function estimation and interpolation \cite{Cooper2006,Cooper1995,Zabinsky2003}. Zabinsky et. al. \cite{Zabinsky2003} consider the problem of estimating a one-dimensional Lipschitz function using a ceiling and floor function as bounding functions an making predictions by taking the average of these functions. Our inference rule can be seen as a generalisation of their approach. Our method provides extensions to multi-dimensional H\"older continuous functions with erroneous observations and inputs, can fold in additional knowledge about boundedness, learn parameters from data and provides guarantees such as uniform convergence of the error. As part of the analysis of our method we construct bounding functions we call \textit{ceiling} and \textit{floor} functions. The construction of similar functions is a recurring theme that, in the Lipschitz context, can be found in global optimisation \cite{Shubert:72} and quadrature \cite{Baran2008} as well as in the analysis of linear splines for function estimation \cite{Cooper1995,Zabinsky2003}. Cooper \cite{Cooper2006,Cooper1995} utilises such upper and lower bound functions in a multi-dimensional setting to derive probabilistic PAC-type error bounds \cite{Valiant1984} for a linear interpolation rule assuming the data is sampled uniformly at random on a hypercube domain. Our inference rule is different from this and our guarantees do not rely on distributional assumptions, although there is some overlap in the ideas for analysing generalisation performance. In future work, we would be interested in utilising Cooper's statistical analysis techniques to extend our guarantees to stochastic settings.
%
%None of the aforementioned works seems to be able to cope with interval-bounded errors, folds in additional knowledge such as boundedness or considers adaptation of the Lipschitz (H\"older) constant to the data.
%Finally, we are not aware of any work that employs these methods in the context of system identification, control or collision avoidance as we do.
%\subsection{Contributions}
%\input{content/Ch_kinkyinf/preliminaries.tex}
%\input{content/Ch_kinkyinf/topological_inference.tex}
%\input{content/Ch_kinkyinf/problem_def}


%
%\input{content/Ch_kinkyinf/est_multidim}
\input{content/Ch_kinkyinf/KI_core}
%\input{content/Ch_kinkyinf/KI_theory_derivations}

\input{content/Ch_kinkyinf/constantadaptation}


\input{content/Ch_kinkyinf/SIctrl_Hfe}
\input{content/Ch_kinkyinf/KISIICKIIML}
%\input{content/Ch_kinkyinf/quad1d}

%\input{content/Ch_kinkyinf/KIMPCcollavoid.tex}

%\input{content/Ch_kinkyinf/optimisation}


%\subsection{Multi-dimensional domains via Fubini's Theorem}
%\label{sec:quadr_multidim}
%\subsection{Optional: Dumping information to avoid the curse of dimensionality.}




\section{Conclusions}
This chapter has introduced the kinky inference framework as an approach to inductive inference in dynamical systems. Folding in knowledge about boundedness and H\"older continuity (with respect to an arbitrary pseudo-metric) the method has been demonstrated to be able to infer unobserved function values successfully. Assuming any observational or input uncertainties are interval-bounded, the method is capable of providing bounds around its predictions. That is, for any finite sample we have shown that the inferred function value is correct up to lying within a given hyperrectangle. We have shown that this uncertainty vanishes (uniformly) in the limit of data sets that (uniformly) converge to a dense subset of input space. Provided no additional a priori knowledge about the target function is known, our bounds are provably tight. We have discussed several variations of the kinky inference rule, including a smooth version, the capability of handling input uncertainty and we have provided two methods for updating beliefs over the H\"older constant. 


We have discussed applications to system identification and control in uncertain dynamical systems highlighting the benefits (and some of its shortcomings) of kinky inference in this application domain. 
In particular, the benefits are rapid learning and prediction, the error bounds around the predictions as well as the flexibility to learn rich function classes. 

In the design of learning-based controllers, the uncertainty bounds afforded by our KI rule are a particularly useful feature. These allowed us to convert the prediction bounds into bounds on the error dynamics. That is, assuming the prior assumptions are correct (and no H\"older constant updates are necessary),  we have obtained stability bounds for the closed-loop dynamics. 



To highlight the applicability of KI in control, we have provided simulations for the different controllers in the model-reference adaptive control framework, in combination with our SIIC control approach of Ch. \ref{ch:SPSIIC} and in inverse dynamics model learning and control. Apart from simple illustrations in the control of double-pendula, we have also provided simulations of KI-MRAC in tracking control problem of the rudder of an unstable fighter-aircraft in the presence of wingrock. Here, KI-MRAC proved competitive with recent state-of-the art algorithms in the test scenario considered in \cite{Chowdhary2013,ChowdharyCDC2013,chowdharyacc2013}. Furthermore, across the board of a several hundred of randomized problem instances, KI-MRAC largely outperformed all competing controllers. 

In Ch. \ref{ch:discrcoll}, we will present an additional application in the context of multi-agent control. There we will utilise the uncertainty bounds afforded by the kinky inference rule to construct robust tubes. These will be converted into robust collision avoidance constraints that are incorporated into the optimisation problem of a predictive controller. This construction will yield a multi-agent controller for KI learners that folds in the posterior knowledge about an uncertain drift.

\textit{Future work} will be invested in extended tests on realistic, higher-dimensional systems and explore the benefits and weaknesses of the different approaches. To this end, we will employ results on input and observational noise to a greater extent than we had to in our proof-of-concept simulations. 
Other extensions of interest pertain to the H\"older constants. At the moment, these are global estimates. In a spirit similar to localised model learning \cite{lwpr2000,TuongSeegerPeters2009}, it may be beneficial to entertain a number of local KI models, each basing their inferences and constant estimates on local information. This might be beneficial not only from a computational point of view, but also provide improved inferences if there is a large variation of the H\"older constant across state space.

Another avenue would be to address the problem of data scarification. That is, given a sample size budget, which data points are most informative? 

From a theoretical point of view, we believe to be able to prove bounds on the error dynamics of KI-IMLC. As the treatment of \cite{Tuongmodellearningsurvey2011} indicates, this would be the first time a guarantee on an inversion model learning-based controller would be given.



%\subsection{Extensions and Future Work}
%\label{sec:kinkyinf_futurework}
%In this chapter, we have considered kinky inference. Our exposition focussed on the simple case where the output space metric was given by a standard norm on finite-dimensional vector space. Future work will examine 
%taking advantage of the generality of the notion of a norm and will look into application to more general metric spaces. An immediate extension would be to the learning of mean-square integrable stochastic processes. 
 %Here the metric could be the \emph{natural semi-metric} $\metric(X,Y) = \expect{ (X-Y)^2}$ which is known to induce a topology on the index set of the process \cite{Piterbarg1991}. 
%
%Additional work will examine our learning methods when applied to real mechanical systems. 
%
%Moreover, extending  \cite{Baran2008}, we have work under preparation for cubature of H\"older continuous functions. Here the simple idea is to integrate the ceiling and floor functions (which are integrable) in closed form. Since we have proven that both of these bounding functions converge uniformly in the limit of increasing data size $N_n$ (provided the grids converge to a dense set of the domain), convergence of the integral estimate is implied. 
%
%The analysis conducted in the context of cubature error may also become of relevance to study the function approximation error of the kinky inference learner and to give optimal active sampling guarantees. 
%So far, we have only given convergence guarantees to the ground truth in the limit of a dense subset of the input space. While we have given error bounds for each prediction for a given sample, we have not provided error bounds for the entire function approximation error specified, for example, with respect to some norm over functions. Questions of interest include how one might sample optimally in order to decrease the error at a maximal rate. If samples are drawn from a distribution, how does the choice of distribution affect the error convergence rate? How does the choice of input metric affect things? And what are the computational trade-offs? That is, if one is subject to diminishing returns, when should one stop sampling? Here, one might explore in how far the analysis provided by Cooper \cite{Cooper2006} in the context of linear spline interpolation rules might be transferred to our kinky inference situation. As an alternative, we have recently become aware of the field of scattered data approximation \cite{wendlandscattereddata2005}, which seems to share a great many goals with the machine learning community. Studying our problems under the lens of the tools and frameworks developed by this community may be a fruitful direction to consider. \jcom{perhaps this in related work}




%
%\appendix{OLD stuff:}
%
%\input{content/intro}
%\input{content/est_enclosingfcts}
%\input{content/quad_shubertstyle}
%\input{content/multidimdom}
%\input{content/intersectionsofenclosure}
%\input{content/gridrefinements}
%\input{content/uncertainLipconst}
%\input{content/notes}

%\begin{small}
%\bibliographystyle{IEEEtran}
%\bibliography{content/lit}
%\end{small}


==> content2/Ch_kinkyinf/meinzeugs.tex <==
%------------------------Meinzeugs----------------------------------------
\usepackage{graphicx}\usepackage{subfigure}
\usepackage{cite}
\usepackage{amscd,amssymb} % AMS-Pakete fuer Theoreme
\usepackage{graphicx} \usepackage{array} \usepackage{subfigure}
\usepackage{psfrag}
%\usepackage{kpfonts}
\usepackage{xy} 
\usepackage{amsmath} 
%\usepackage{mathabx}
\usepackage{fancyhdr}
\usepackage{setspace} 
\usepackage{rotating,epsfig} \usepackage{epsfig}
\usepackage{verbatim} \usepackage{multicol} \usepackage{longtable}
\usepackage{amsthm}
% THEOREMS -------------------------------------------------------
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{conj}[thm]{Conjecture}
%\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{ques}[thm]{\textbf{QUESTION}}
\newtheorem{ex}[thm]{\textbf{Example}}
% MATH -----------------------------------------------------------
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\normtop}[1]{\left\Vert#1\right\Vert^p}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\abstop}[1]{\left\vert#1\right\vert^p}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\Real}{\mathbb R}
\newcommand{\Complex}{\mathbb C}
\newcommand{\integer}{\mathbb Z}
\newcommand{\nat}{\mathbb N}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\BX}{\mathbf{B}(X)}
\newcommand{\A}{\mathcal{A}}
\newcommand{\aff}[1]{\text{aff } #1}
\newcommand{\dom}[1]{\text{dom } #1}
\newcommand{\epi}[1]{\text{epi } #1}
\newcommand{\ri}[1]{\text{ri } #1}
\newcommand{\cl}[1]{\text{cl } #1}


%-----------------------------------------
\newcommand{\argmin}{\text{argmin}}
\newcommand{\argmax}{\text{argmax}}
\newcommand{\arginf}{\text{arginf}}
\newcommand{\argsup}{\text{argsup}}

\newcommand{\sgn}{\ensuremath{\text{sgn}}}
% fuer skalare:
%\newcommand{\s}[1]{\mathfrak{#1}}
\newcommand{\s}[1]{{#1}}
% fuer vectoren:
%\newcommand{\vc}[1]{\mathbf{#1}}
\newcommand{\vc}[1]{#1}
% scalar product:
\newcommand{\Sp}[1]{\ensuremath{\mathbf{\langle} #1 \mathbf{\rangle}}}
\newcommand{\SP}[2]{\ensuremath{\mathbf{\langle} \vc{#1} \mathbf{,} \vc{#2} \mathbf{\rangle}}}
\newcommand{\SPL}[2]{\ensuremath{\mathbf{\langle} \vc{#1}\mathbf{,} \vc{#2} \mathbf{\rangle}_{L_2}}}
\newcommand{\SPLintI}[2]{\ensuremath{\int_I {#1(t)}\, {\overline{#2}(t)} \, {\mu}}}

\newcommand{\pp}[1]{\langle #1 \rangle}

\newcommand{\metric}{\, \mathfrak{d}} % distance metric

%HS:
\newcommand{\hs}[1]{\ensuremath{\mathcal{#1}}}
%operators:
\newcommand{\op}[1]{\ensuremath{ {#1}}}

\newcommand{\dif}[2]{{\operatorname{d}\over\operatorname{d}#2}#1}
\newcommand{\pdif}[2]{{\operatorname{\partial}\over\operatorname{\partial}#2}#1}
\newcommand{\ppdif}[3]{{\operatorname{\partial^2}\over\operatorname{\partial}#2 \partial#3}#1}
%\renewcommand{\d}[1]{\operatorname{d}#1}
\renewcommand{\d}[1]{\text{ d}#1}


\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}

%Fourier Operator:
\newcommand{\FT}[1]{\mathcal F #1}

%Koerper:
\newcommand{\field}{\mathbb F}
%nullspace:
\newcommand{\ns}{\mathcal{NS}}
\newcommand{\GP}{\mathcal {GP} }
\newcommand{\Gauss}{\mathcal {N} }
\newcommand{\gauss}{p_{\mathcal {N}} }
\newcommand{\expect}[1]{\ensuremath{ \langle#1\rangle } }
\newcommand{\cov}[2]{\ensuremath{ \text{cov}(#1,#2) } }
\newcommand{\var}[1]{\ensuremath{ \text{var}[#1]} }

%parameter:
\newcommand{\pardop}{\ensuremath{\omega}}%parameter for lin. Dif OP

\newcommand{\pardopspace}{\ensuremath{\Omega}}%parameter space for lin. OP

\newcommand{\pardi}{\ensuremath{\mathfrak p}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\pardispace}{\ensuremath{\mathfrak P}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\state}{\ensuremath{ \vc x}} % state of the system... integral curve of the ODE/ signal.
\newcommand{\statespace}{\ensuremath{ \mathcal X}}

\newcommand{\inspace}{\ensuremath{ \mathcal X}}
\newcommand{\outspace}{\ensuremath{ \mathcal Y}}

\newcommand{\di}{\ensuremath{ u}} % driving force / control input

\newcommand{\agi}{\ensuremath{ \mathfrak a}} %an agent index
\newcommand{\agii}{\ensuremath{ \mathfrak r}} %index if another agent
\newcommand{\agiii}{\ensuremath{ \mathfrak q}} %index if another agent

\newcommand{\agset}{\ensuremath{ \mathfrak A}} %set of Agents

\newcommand{\collevent}{\ensuremath{\mathfrak C}}


\newcommand{\decke}{\ensuremath{\mathfrak u}}
\newcommand{\boden}{\ensuremath{\mathfrak l}}
\newcommand{\einschluss}{\ensuremath{\mathcal E^{\decke_n}_{\boden_n}}}

\newcommand{\menge}[2]{\ensuremath{\{#1 \, \vert \, #2 \}}}

%\newcommand{\diag}{\ensuremath{ \text{diag}} %set of

\renewcommand{\Pr}{\mathrm{Pr}}
\newcommand{\KLD}[2]{\text{KLD}(#1||#2) }

\newcommand{\erw}[2][]{
%    \ensuremath{\pmb{\mathcal{M}}^{\operatorfont{#1}}}%
     \ensuremath{\mathbb{E}_{#1} \! \left\lbrace #2 \right\rbrace}%
}
%----------- probability stuff------------------------
\newcommand{\pmeas}[1]{\ensuremath{\mathbb #1}} % probability measure

\newcommand{\embedding}{\ensuremath{\tilde \mu}} % probability measure
\newcommand{\ewx}[1]{\ensuremath{\mathbb E_x[ #1 ] }} % expected value
\newcommand{\ew}{\ensuremath{\mathbb E }} % expected value
\newcommand{\is}{\ensuremath{\mathfrak X }} % input space / index set
\newcommand{\Vol}{\ensuremath{\text{Vol}}}

% --------------------environments--------------------------------------------
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eq}[1]{\begin{equation} #1 \end{equation}}

% ----------------------------------------------------------------
%-------------- Meinzeugs Ende-----------------------------------------


==> content2/Ch_kinkyinf/multidimdom.tex <==
\section{Conservative integration on multi-dimensional domains}
This time, the target function is assumed to be of the form $f: I \subset \Real^d \to \Real$ where $I$ is a $d-$dimensional hyper-rectangle.

Evoking Fubini's theorem, one could in principle apply the one-dimensional method developed above recursively in order to compute conservative estimates of $\int_I f(x) \, \d x$. Unfortunately, the necessity to evaluate $f$ at all corner points of $I$ renders the approach intractable for high-dimensional situations $d>>1$ -- the number of corner points of a $d$-dimensional hyper-rectangle is $2^d$. 
To overcome this limitation, we borrow a trick used in the DIRECT optimisation algorithm (CITE!!!!): instead of sampling at the corner points, we will always sample the centre point of a hyperrectangle. Thereby, we decouple the number of samples from the dimensionality of the problem.

\subsection{Conservative estimates and definite integrals on multi-dimensional domains based on 1-norm integrals}
Assume our grid $G_N$ is given by a sequence of $N$ tuples $\bigl(s_{i}^N, f(s_{i}^N), J_{i}^N\bigr)_{i=1,\ldots,N}$ where the sub-hyperrectangles $J_{1}^N,\ldots, J_{N}^N$ partition $I$ up to a zero-set, $s_i^N \in J^N_i$ is a sample of the function. We assume, each hyperrectangle $J_{i}^N$ is given by a Cartesian product of intervals $[-a_{i,1}^N,b_{i,1}^N] \times \ldots \times [-a_{d,1}^N,b_{d,1}^N]$ where \emph{``radii''} $a_{i,1}^N,b_{i,1}^N,\ldots, a_{i,d}^N,b_{i,d}^N\in \Real_+$ are known we can reconstruct hyperrectangle $J^N_i$ by pointwise addition: $J^N_i= s_i^N + \bigl( [-a_{i,1}^N,b_{i,1}^N] \times \ldots \times [-a_{d,1}^N,b_{d,1}^N] \bigr)$. 


For ease of notation, we will omit superscript $N$ when $N$ is fixed and it is not necessary to distinguish between 
grids of different resolutions. Similarly, when the hyperrectangle is fixed, we will omit subscript $i$. For example, $a_{i,j}^N , b_{i,j}^N$ are the radii of the $i$th hyperrectangle in the $j$th dimension. If we consider a particular hyperrectangle for grid $G_N$ $(N \text{fixed})$ we may write these as $a_j,b_j$.

\begin{figure}[htbp]
			\centering
			\includegraphics[scale =.2]{content/figs/rect2.pdf}
	%
	%
	\caption{A hyperrectangle in two dimensional space given by radii and sample point.}
	\label{fig:rect2}
\end{figure}


\begin{lem} \label{lem:defint_of_1norm}
Let $s \in \Real^d$ the sample point of hyperrectangle $J = \{ x \in \Real^d \vert \,(x-s)\, \in ([-a_1,b_1] \times \ldots \times [-a_d,b_d])\}\subset \Real^d$ where $a_1,b_1,\ldots,a_d,b_d \in \Real_+$ are the ``radii'' of the hyperrectangle.
We have 
\begin{align}
\bar S  &= \int_{J} \norm{x-s}_1 \d x \\
& =  \frac{1}{2} \Bigl( \prod_{j=1}^d a_j + b_j\Bigr)  \sum_{i=1}^d \frac{a_i^2+b_i^2}{a_i + b_i}  .
\end{align}

%(where we adhere to the convention $\prod_{j=1}^0 \rho_j = 1$).


\begin{proof}
Let $\bar J := J - s$.
We have $\bar S= \int_{\bar J} \norm{x}_1 \d x$.
We will proof the claim by induction on dimension $d$. \\
%
\textit{Base case} ($d=1$). $\int_{-a_1}^{b_1} \abs{x_1} dx_1 = \frac{1}{2} (a_1^2+b_1^2)$.\\
%
\textit{Induction hypothesis (I.H.).} For some dimension $d$ we have $ \bar S = \int_{-a_{d}}^{b_{d}}  \ldots \int_{-a_{1}}^{b_{1}}  \sum_{i=1}^{d} \abs{x_i} \d x_1 \ldots \d x_{d} =  \frac{1}{2} \sum_{i=1}^d  \Bigl( (a_i^2+b_i^2) \prod_{j=1,j\neq i}^d (a_j + b_j) \Bigr)$.\\
%
\textit{Induction step ($d \to d+1$).} Assume we are in $d+1$ dimensional space. 
Using Fubini's theorem we get 
$\int_{\bar J \times [-a_{d+1},b_{d+1}]} \norm{x}_1 \d x$
%
$ = \int_{-a_{d+1}}^{b_{d+1}}\ldots \int_{-a_{1}}^{b_{1}} \sum_{i=1}^{d+1} \abs{x_i} \d x_1 \ldots \d x_{d+1}$
%
$ = \int_{-a_{d+1}}^{b_{d+1}}\ldots \int_{-a_{1}}^{b_{1}}  \abs{x_{d+1}} \d x_1 \ldots \d x_{d+1} +  \int_{-a_{d+1}}^{b_{d+1}} \bigl( \int_{-a_{d}}^{b_{d}}  
\ldots \int_{-a_{1}}^{b_{1}}  \sum_{i=1}^{d} \abs{x_i} \d x_1 \ldots \d x_{d} \bigr) \d x_{d+1}$ 
%
$ \stackrel{I.H.}{=}   \frac{1}{2} (a_{d+1}^2 +b_{d+1}^2) \int_{-a_{d}}^{b_{d}}\ldots \int_{-a_{1}}^{b_{1}}  \d x_1 \ldots \d x_{d} +  \int_{-a_{d+1}}^{b_{d+1}} \frac{1}{2} \sum_{i=1}^d  \Bigl( (a_i^2+b_i^2) \prod_{j=1,j\neq i}^d (a_j + b_j) \Bigr) \d x_{d+1} $ 
%
$ =   \frac{1}{2} (a_{d+1}^2 +b_{d+1}^2) \bigl(\prod_{j=1}^d (a_j+b_j)\bigr) + (a_{d+1}+ b_{d+1} ) \frac{1}{2} \sum_{i=1}^d  \Bigl( (a_i^2+b_i^2) \prod_{j=1,j\neq i}^d (a_j + b_j) \Bigr) $ 
%
$  =\frac{1}{2} \sum_{i=1}^{d+1}  \Bigl( (a_i^2+b_i^2) \prod_{j=1,j\neq i}^{d+1} (a_j + b_j) \Bigr) $. 

\end{proof}
\end{lem}


\begin{rem}
Note, by pre-computing the product, the formula can be computed in $\mathcal O(d )$.
\end{rem}

\subsection{Conservative estimates and definite integrals on multi-dimensional domains based on max-norm integrals}

\subsubsection{Grids sampling centre points of hyperrectangles }
 For now, assume our grid $G_N$ consists of $N$ sub-hyperrectangles $J_1^N,\ldots,J_N^N$ that partition $I$. Let $c_i^N$ denote the centre point of $J_i^N$ and, let $r_j^i$ denote half of $J_i$'s edge length in the $j$th dimension $(j=1,...,d)$. 
That, is each grid $G_N$ is given by a sequence of triples $(c_i^N, f(c_i^N), r^N)_{i=1}^N$ where $c_i \in \Real^d$ is a centre point of $i$th hyperrectangle $J_i^N = c_i^N + [-r_{1,1}^N,+r_{1,1}^N] \times \ldots \times  [-r_{i,d}^N,+r_{i,d}^N] $ and $r_i^N$ is the vector of radii.  

For ease of notation, we will omit superscript $N$ when $N$ is fixed and it is not necessary to distinguish between 
grids of different resolutions. Similarly, when the hyperrectangle is fixed, we will omit subscript $i$. For example, $r_{i,j}^N$ is the radius of the $i$th hyperrectangle in the $j$th dimension. If we consider a particular hyperrectangle for grid $G_N$ $(N \text{fixed})$ we may write this as $r_j$.

\begin{figure}[htbp]
			\centering
			\includegraphics[scale =.2]{content/figs/rect1.pdf}
	%
	%
	\caption{A hyperrectangle in two dimensional space given by radii and centre point.}
	\label{fig:rect1}
\end{figure}


\textbf{Lipschitz Ceiling}. For now, let us only be concerned with upper bound estimates. 

Due to Lipschitz continuity on each hyperrectangle, we have 


\[\forall i \forall x,x' \in J_i: \abs{f(x) - f(x')} \leq L_i \norm{x-x'}. \]

In particular, 

\[\forall i \forall x \in J_i: f(x) - f(c_i) \leq\abs{f(x) - f(c_i)} \leq L_i \norm{x-c_i}. \]
Hence, 
\begin{align}
\forall i \forall x \in J_i: f(x)  &\leq f(c_i) + L_i \norm{x-c_i} \\
&\leq f(c_i) + \ell_i \norm{x-c_i}_{\infty}:= \decke^i_N(x)
\end{align}
where $\ell_i = \sqrt d L_i$ is a Lipschitz constant for the max-norm.
The last inequality is due to the well-known relationship 
$\norm{x}_\infty \leq \norm{x}_2 \leq \sqrt{d} \, \norm{x}_\infty $.

Thereby, we can define a new \textit{Lipschitz ceiling} 

\[\decke_N: x \mapsto \sum_{i=1}^N \chi_{J_i} (x) \, \decke^i_N(x)\]
guaranteeing to be an upper bound on $f$:

\[\decke_N( x) \geq f(x), \forall x \in I \subset \Real^d.\]

Therefore, 

\[\hat S_N^\decke:=\int_I \decke_N( x) d\mu(x) \geq \int_I f(x) \d\mu(x) =: S, \forall x \in I \subset \Real^d.\]
If each $\decke^i_N$ are integrable, we have 
\begin{equation}
\sum_{i=1}^N \int_{J_i} \decke^i_N( x) d\mu(x)=\hat S_N^\decke \geq \int_I f(x) \d\mu(x).
\label{eq:defint_ceiling2}
\end{equation}
Fortunately, we can evaluate $\hat S_i :=\int_{J_i} \decke^i_N( x) d\mu(x)$ in closed-form. To this end, we can use the following lemma:



%
%\begin{lem} Let $c \in \Real^d$, $l\in \Real$ be the edge length of hyper-square $J := \menge{x \in \Real^d}{ (x -c) \in [-r,r]^d } \subset \Real^d$ where $r= \frac{1}{2} l$. 
%We have \[
%\bar S = \int_{J} \norm{x-c}_\infty \d x = \frac{d}{2(d+1)}  l^{d+1}.\]
%
%
%\begin{proof}
%The idea of the proof will be to establish that the desired definite integral coincides with the volume of a $d+1$-dimensional hyperrectangle $B$  minus the volume of an inverted $d+1$-dimensional hyper-pyramid $P$ with a $d$-dimensional hyper-square base $J$ and height $r$. 
%It is well known, that such a hyper-pyramid has volume $\frac{1}{ d+1} r l^{d}$. 
%Hyper-rectangle $B$ has edge length $l$ in the first $d$ dimensions and edge length $r$ in the $d+1$th. Therefore, its volume is $r l^{d}$
%
%Before proceeding, we need to introduce the notion of an \textit{inverted hyper-pyramid}. For convenience, we will translate the space. Note, this neither  changes any volumes nor the definite integral we desire to calculate. That is, utilizing the substitution rule for definite integration, we see
%$\bar S = \int_{J} \norm{x-c}_\infty \d x =  \int_{J'} \norm{x}_\infty \d x$ where $J' = J - c = \{\xi \in \Real^d | (\xi_1,...,\xi_d)^T \in J'\} = [-r,r]^d$ is a translated version of hyperrectangle $J$. We will derive the last integral.
%
%A regular \emph{inverted} (half-open) hyper-pyramid (centred at zero) is the set
%$P:=\{ \xi \in \Real^{d+1} \, \vert \,  \xi_{d+1} \in (0,r], \forall j \in \{1,\ldots,d\}:\xi_j \in (-\xi_{d+1}, \xi_{d+1} )  \}.$
%
%For $d=2$, one can imagine the inverted pyramid as one standing on its tip on point $0 \in \Real^{d+1}$.
%An illustration of this case can be found in Fig. \ref{fig:pyramid_sampled_green}.
%\begin{figure}
%	\centering
%		\includegraphics[scale =.5]{content/figs/pyramid_sampled_green.pdf}
%	\caption{Samples drawn from an inverted pyramid centred at the origin and with edge length $l=2$.}
%	\label{fig:pyramid_sampled_green}
%\end{figure}
%
%
%
%
%Now, let $V(S) \in \Real$ denote the volume of a set $S \subset \Real^{d+1}$ and define 
%
%$K =\menge{\xi \in \Real^{d+1}}{ \xi_{d+1} \leq \norm{\xi}_{\infty}, (\xi_1,...,\xi_d)^T \in J', \xi_{d+1} \in [0,r]  }$  
%
%$
%= \menge{\xi \in \Real^{d+1}}{(\xi_1,...,\xi_d)^T \in J, \,  \, 0 \leq \xi_{d+1} \leq \max_{j \in \{1,...,d\}} \abs{\xi_j}\leq r }$.
%
%
%We have $\bar S = V(K)$. (Do I NEED TO JUSTIFY THIS ?????????????????)
%Furthermore, define $B := [-r,r]^{d} \times [0,r] = J' \times [0,r]$. We can show \[ K = B - P \] and hence, \[\bar S= V(K) = V(B) - V(P) = r l^{d} - \frac{1}{d+1} r l^{d} = \frac{d}{2(d+1)} l^{d+1}. \]
%
%It remains to be shown that indeed we have $K = B - P$:  
%To this end, we show that $B$ is partitioned into $K$ and $P$. 
%
%Firstly, we notice that obviously $K \subset B$ and $P \subset B$. 
%
%Secondly, we prove 
%%
%%%- --- beweis dass schnitt leer ist----
%% \underline{$K \cap P \stackrel{!}{=} \{\emptyset\}$}: For contradiction, assume $K \cap P \neq\{\emptyset\}$ and choose any $x \in K \cap P$. Since $x \in K$ we can choose $j \in \{1,...,d\}$ such that 
%%
%%$x_{d+1} \leq |x_j|$. That is, $x_{d+1} \leq x_j$ (i) or $x_{d+1} \leq -x_j$ (ii).
%%
%%1st case: Assume $x_{d+1} \leq x_j$. Since also $x \in P$, we have $x_j < x_{d+1}$. Hence, $x_{d+1} < x_{d+1}$ which is the desired contradiction.
%%
%%2nd case: Assume $x_{d+1} \leq -x_j$. Hence, $-x_{d+1} \geq x_j$. Since $x \in P$, we also have $x_j > -x_{d+1}$. In conjunction, this yields $-x_{d+1} > - x_{d+1}$ and thus, our desired contradiction.\\
%%%------------- beweis des leeren schnittes ende ---------------
%\underline{$x \notin K \wedge x \in B \Leftrightarrow x \in P$}: 
%
%%Note, $x \in K \cup P \Leftrightarrow x \in K \vee x \in P \Leftrightarrow (x \notin K \Rightarrow x \in P) \wedge (x \notin P \Rightarrow x \in K)$.
%
%$ x \in B \wedge x \notin K$  
%
%$\Leftrightarrow ( x \in [-r,r]^d \times [0,r] \wedge \bigl( x_{d+1} \notin [0,r] \vee (\exists j \in \{1,...,d\}: x_j \notin [-r,r]) \vee x_{d+1} > \max_{j \in \{1,...,d\}} \abs{x_j} \bigr) $ 
%
%$\Leftrightarrow (\forall j \in \{1,...,d\}: x_j \in [-r,r]) \wedge  r \geq x_{d+1} > \max_{j \in \{1,...,d\}} \abs{x_j} \geq 0 $
%
%$\Leftrightarrow x_{d+1} \in (0,r] \wedge \forall j \in \{1,...,d\}: (x_j \in [-r,r] \wedge  x_{d+1} > \abs{x_j} ) $
%
%$\Leftrightarrow x \in P$.
%
%\end{proof}
%\end{lem}


%-------------------

\begin{lem} \label{lem:defint_of_maxnorm}
Let $c \in \Real^d$ the centre point of hyperrectangle $J = \{ x \in \Real^d \vert \,(x-c)\, \in ([-r_1,r_1] \times \ldots \times [-r_d,r_d])\}\subset \Real^d$ where $r_1,\ldots,r_d \in \Real_+$ are the ``radii'' of the hyperrectangle. Let $r^* := \max\{r_1,\ldots,r_d \}$ and let $\mathfrak p: \in \text{Perm}(d)$ be a permutation such that $\rho_0 := 0 \leq \rho_1 := r_{\mathfrak p(1)}\leq \ldots \leq \rho_d := r_{\mathfrak p(d)} =r^*$.
We have 
\begin{align}
\bar S  &= \int_{J} \norm{x-c}_\infty \d x \\
& =  2^d r^* (\prod_{q=1}^d r_q) - 2^d \sum_{q=0}^{d-1} \frac{\prod_{j=1}^{q} \rho_j }{d-q+1} (\rho_{q+1}^{d-q+1} - \rho_{q}^{d-q+1} )
\end{align}

(where we adhere to the convention $\prod_{j=1}^0 \rho_j = 1$).


\begin{proof}
Before commencing further, note $\bar S = \int_{J} \norm{x-c}_\infty \d x = \int_{J'} \norm{x}_\infty \d x$ where 
\[J' =[-r_1,r_1] \times \ldots \times [-r_d,r_d] \subset \Real^d \]
 is a $d$-dimensional hyperrectangle. We will derive the value of the latter definite integral. For a set $S \subset \Real^d$ let $\Vol_{d}(S)$ be its volume (measure) in $d$ dimensions. By realizing that $\norm{x}_\infty \geq 0,\forall x \in J'$ we notice that $\int_{J'} \norm{x}_\infty \d x$ equals the volume of the set of points in $d+1$-dimensional space whose first $d$ components form a vector in $J'$ and whose last components are below the maximum norm and above zero. That is, $\int_{J'} \norm{x}_\infty \d x = \text{Vol}_{d+1}(K)$ where 
\[K :=\menge{\xi \in J' \times (0,r^*]}{ \xi_{d+1} \leq \norm{ \pi_{d}(\xi)}_{\infty}} 
 \] 
 where \[r^* := \max\{r_1,\ldots,r_d \}\] is the maximum radius 
 and \[\pi_d: \begin{cases} \Real^{d+1} \to \Real^d\\ (x_1,\ldots,x_d,x_{d+1})^T \mapsto (x_1,\ldots,x_d)^T 
 \end{cases}  \] is the projection onto the first $d$ components.
A key component of our proof is to establish that the desired definite integral coincides with the volume of the $d+1$-dimensional hyperrectangle 
%
\[B:= J' \times (0,r^*] \]  minus the volume of an half-open convex set \\
%
%\begin{small}

\[P:=\bigl\{ \xi \in B \, \vert  \forall  j \in \{1,...,d\} :\abs{\xi_j} < \min\{r_j,\xi_{d+1}\}   \bigr\}\]

%\end{small}
%
whose volume we can determine in closed form (as we will do below). In fact, one can notice that for equal radii $r_1,...,r_d = r^*$, $P$ is an inverted $d+1$-dimensional hyper-pyramid with a $d$-dimensional hyper-square base $J'$ and height $r^*$. 
An illustration of this case for $d=2$ can be found in Fig. \ref{fig:pyramid_samples}.

%\begin{figure*}
%	\centering
%		\includegraphics[scale =.5]{content/figs/maxnorm_fct_regular.pdf}
%	\caption{Surface plot of the maxnorm function on $J' =[-1,1] \times [-1,1]$}
%	\label{fig:maxnorm_fct_regular}
%\end{figure*} & 
%
%
%
%\begin{figure}
%	\centering
%		\includegraphics[scale =.5]{content/figs/pyramid_sampled_green.pdf}
%	\caption{Samples drawn from an inverted pyramid centred at the origin and with uniform radius $r_1=r_2=1$.}
%	\label{fig:pyramid_sampled_green}
%\end{figure}



\begin{figure*}
        \centering
        \begin{subfigure}
                \centering
                \includegraphics[scale =.20]{content/figs/maxnorm_samples.pdf}
               % \caption{Samples from $x \mapsto \norm{x}_{\infty}$ on  $J' =[-1,1] \times [-1,1]$.}
               % \label{fig:gull}
        \end{subfigure}%
         %add desired spacing between images, e. g. ~, \quad, \qquad etc. 
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}
                \centering
                \includegraphics[scale =.20]{content/figs/pyramid_sampled_green.pdf}
                %\caption{Samples from the interior of $P$.}
                %\label{fig:tiger}
        \end{subfigure}
        %
        \begin{subfigure}
                \centering
                \includegraphics[scale =.20]{content/figs/maxnorm_and_pyramid_samples.pdf}
                %\caption{Both merged. Note, }
                %\label{fig:tiger2}
        \end{subfigure}
         %add desired spacing between images, e. g. ~, \quad, \qquad etc. 
          %(or a blank line to force the subfigure onto a new line)
       \caption{Left: Samples from $x \mapsto \norm{x}_{\infty}$ on  $J' =[-1,1] \times [-1,1]$. Centre: Samples drawn from an inverted pyramid $P$ centred at the origin and base $J'$. Right: Note, how the points of $P$ are contained in the intersection of $B =[-1,1]^2 \times (0,1]$ and the epigraph of $x \mapsto \norm{x}_{\infty}$. }
       \label{fig:pyramid_samples}
\end{figure*}	


As explained above, $\bar S = \Vol(K)$. 
Below, we will show \[ K = B \backslash P \] and hence, 
\begin{equation}
\bar S= \Vol(B) - \Vol(P)=  r^* \prod_{i=1}^d (2r_i) - \Vol(P). 
\end{equation}

So, we need to derive two things:\\
 
(I) Firstly, it remains to be shown that indeed we have $K = B - P$.\\
(II) Secondly, we need to find a closed-form formula for $\Vol (P)$.\\
 


Derivation of (I). In order to prove $K = B \backslash P$. We notice that, by definition, $K,P \subset B$. Next, we show that $B$ is partitioned into $K$ and $P$ which we achieve by showing the following equivalence: 

\[\forall x \in B: x \in K \oplus x \in P. \]

where $\oplus$ denotes the \emph{exclusive or}. 

The \textit{exclusive or} statement can be rewritten as 

$x \notin K \wedge x \in B \Leftrightarrow x \in P \wedge x \in B$ which we show as follows: 

%Note, $x \in K \cup P \Leftrightarrow x \in K \vee x \in P \Leftrightarrow (x \notin K \Rightarrow x \in P) \wedge (x \notin P \Rightarrow x \in K)$.

$ x \in B \wedge x \notin K$  

$\Leftrightarrow ( x \in J' \times (0,r^*] \wedge \bigl( x \notin J' \times (0,r^*] \vee x_{d+1} > \max_{j \in \{1,...,d\}} \abs{x_j} \bigr) $ 

$\Leftrightarrow ( x \in J' \times (0,r^*] \wedge   x_{d+1} > \max_{j \in \{1,...,d\}} \abs{x_j} \geq 0 $

$\Leftrightarrow x_{d+1} \in (0,r^*] \wedge \forall j \in \{1,...,d\}: (x_j \in [-r_j,r_j] \wedge  x_{d+1} > \abs{x_j} ) $

$\Leftrightarrow x \in B \wedge \forall j \in \{1,...,d\} : \min \{x_{d+1}, r_j\} > \abs{x_j } \bigr\}$

$\Leftrightarrow x \in P \wedge x \in B$.\\


Derivation of (II). We desire to determine $\Vol_{d+1}(P)$. We have 

\[\Vol_{d+1}(P) = \int_0^{r^*} \Vol_d \bigl(R(h)\bigr) \, dh\]
%\end{equation} 

where $R(h) = \bigl\{(\xi_1,...,\xi_d)^T \vert  \forall  j \in \{1,...,d\} :\abs{\xi_j} < \min\{r_j,h \} \bigr\} = \pi_d(P \cap \{x \in \Real^{d+1} | x_{d+1} =h \})$ is the set of all points of $P$ having ``height'' $h \in (0,r^*]$.
Let $\mathfrak p: \in \text{Perm}(d)$ be a permutation such that $\rho_0 := 0 \leq \rho_1 := r_{\mathfrak p(1)}\leq \ldots \leq \rho_d := r_{\mathfrak p(d)} =r^*$.

So, we can write \[R(h) = \bigl\{(\xi_1,...,\xi_d)^T \vert  \forall  j \in \{1,...,d\} :\abs{\xi_{\mathfrak p (j)}} < \min\{\rho_j,h \} \bigr\}. \]
We have, 
$\Vol_{d+1}(P) = \int_0^{r^*} \Vol_d \bigl(R(h)\bigr) \, dh$ 
\begin{equation}
\label{eq:volgenhyperpyramid}
= \int_0^{\rho_1} \Vol_d \bigl(R(h)\bigr) \, dh + \sum_{i=1}^{d-1} \int_{\rho_i}^{\rho_{i+1}} \Vol_d \bigl(R(h)\bigr) \, dh.
\end{equation}

We note,
$\forall h \in (0, \rho_1):  h < \rho_j, \forall j >1$. Hence, $\forall h \in (0, \rho_1): R(h) = \bigl\{(\xi_1,...,\xi_d)^T \vert  \forall  j \in \{1,...,d\} :\abs{\xi_j} < h \bigr\}$ which is a hyper-square in $R^d$ with edge length $2h$. Hence, \[\Vol_d\bigl(R(h)\bigr) = (2h)^d, \,\,\,\, \forall h \in (0, \rho_1).\] 
Hence, 
\begin{equation}
\int_0^{\rho_1} \Vol_d\bigl(R(h)\bigr) \, dh = \int_0^{\rho_1} (2h)^d \, dh = \frac{2^d \rho_1^{d+1}}{d+1}.
\end{equation}

Analogously, let  $i \in \{1,...,d-1\}$ and  $h \in (\rho_i, \rho_{i+1})$ arbitrary. We have $  \rho_1 \leq ... \leq \rho_i <h < \rho_{i+1} \leq ... \leq \rho_d$. Hence, $R(h) = \bigl\{(\xi_1,...,\xi_d)^T \vert  \forall  j \in \{1,...,d\} :\abs{\xi_{\mathfrak p (j)}} < \min\{\rho_j,h \} \bigr\} = \bigl\{(\xi_1,...,\xi_d)^T \vert  \forall  j \in \{1,...,i\} :\abs{\xi_{\mathfrak p (j)}} < \rho_j,  \forall  j \in \{i+1,...,d\} :\abs{\xi_{\mathfrak p (j)}} < h \bigr\}$ being a hyperrectangle. 
Thus, $\Vol_d\bigl(R(h) \bigr) = (2h)^{d-i} \prod_{j=1}^{i} (2\rho_j), \forall i \in \{1,...,d-1\}, h \in (\rho_i, \rho_{i+1}).$

Hence, 
\begin{eqnarray}
\int_{\rho_i}^{\rho_{i+1}} \Vol_d\bigl(R(h)\bigr) \, dh = \prod_{j=1}^{i} 2\rho_j \int_{\rho_i}^{\rho_{i+1}} (2h)^{d-i}  \, dh \\= 2^d \frac{\prod_{j=1}^{i} \rho_j }{d-i+1} (\rho_{i+1}^{d-i+1} - \rho_{i}^{d-i+1} ).
\end{eqnarray}

Inserting the formulae into Eq. \ref{eq:volgenhyperpyramid} yields the solution:

\[\Vol_{d+1}(P) = 2^d \sum_{i=0}^{d-1} \frac{\prod_{j=1}^{i} \rho_j }{d-i+1} (\rho_{i+1}^{d-i+1} - \rho_{i}^{d-i+1} ). \]

\end{proof}
\end{lem}

As a special case we obtain for hyper-square domains:
\begin{cor} Let $c \in \Real^d$, $l\in \Real$ be the edge length of hyper-square $J := \menge{x \in \Real^d}{ (x -c) \in [-r,r]^d } \subset \Real^d$ where $r= \frac{1}{2} l$. 
We have \[
\bar S = \int_{J} \norm{x-c}_\infty \d x = \frac{d}{2(d+1)}  l^{d+1}.\]
\end{cor}


 Let $J_i = c_i + ([-r_1(i),r_1(i)]\times,\ldots, \times[-r_d(i),r_d(i)])$ ($r_j(i) >0, \forall j$) be a hyperrectangle with centre point $c_i \in \Real^d$. As in Lem. \ref{lem:defint_of_maxnorm},  $r^{*}(i) := \max\{r_1(i),\ldots,r_d(i) \}$ and let $\mathfrak p^i: \in \text{Perm}(d)$ be a permutation such that $\rho_0(i) := 0 \leq \rho_1(i) := r_{\mathfrak p^i(1)}(i)\leq \ldots \leq \rho_d(i) := r_{\mathfrak p^i(d)}(i) =r^{*}(i)$. We can utilize Lem. \ref{lem:defint_of_maxnorm} to calculate our conservative estimate of the integral:

\begin{align*}
%
\hat S_{N,i}^\decke &=\int_{J_i} \decke^i_N( x) \, \d x \\
%
& = \int_{J_i} f(c_i) + \ell_i \norm{x-c_i}_{\infty} \, \d x \\
%
& = \int_{J_i} f(c_i) \, \d x + \ell_i \int_{J_i}  \norm{x-c_i}_{\infty} \, \d x \\
%
& = f(c_i) \Vol(J_i) + \ell_i 2^d r^{*}(i) (\prod_{q=1}^d r_q(i)) \\
&- \ell_i 2^d \sum_{q=0}^{d-1} \frac{\prod_{j=1}^{q} \rho_j(i) }{d-q+1} \bigl(\rho_{q+1}^{d-q+1}(i) - \rho_{q}^{d-q+1}(i) \bigr) \\
%
& = \bigl(f(c_i) + \ell_i r^{*}(i) \bigr) \,2^d (\prod_{q=1}^d r_q(i)) \\
&- \ell_i 2^d \sum_{q=0}^{d-1} \frac{\prod_{j=1}^{q} \rho_j(i) }{d-q+1} \bigl(\rho_{q+1}^{d-q+1}(i) - \rho_{q}^{d-q+1}(i) \bigr) \\
\end{align*}

In conjunction with Eq. \ref{eq:defint_ceiling}, this yields 
\begin{align} \label{eq:quadupper_multidim}
\hat S_N^\decke &= \sum_{i=1}^N \int_{J_i} \decke^i_N( x) \d x \\
&= \sum_{i=1}^N  \Bigl[ \bigl(f(c_i) + \ell_i r^{*}(i) \bigr) \,2^d (\prod_{q=1}^d r_q(i)) \\
&- \ell_i 2^d \sum_{q=0}^{d-1} \frac{\prod_{j=1}^{q} \rho_j(i) }{d-q+1} \bigl(\rho_{q+1}^{d-q+1}(i) - \rho_{q}^{d-q+1}(i) \bigr) \Bigr]\\
& \geq \int_I f(x) \,dx = S.
\end{align}


\textbf{Lipschitz floor.}

The derivation is completely analogous to the derivation of the Lipschitz ceiling provided above. 

Lipschitz continuity gives

\[\forall i \forall x,x' \in J_i: \abs{f(x) - f(x')} \leq L_i \norm{x-x'}. \]

and hence, 

\[\forall i \forall x \in J_i: f(c_i) - f(x) \leq\abs{f(c_i) - f(x)} \leq L_i \norm{x-c_i}. \]
Thus, 
\begin{align}
\forall i \forall x \in J_i: f(x)  &\geq f(c_i) - L_i \norm{x-c_i} \\
&\geq f(c_i) - \ell_i \norm{x-c_i}_{\infty}:= \boden^i_N(x)
\end{align}
where $\ell_i = \sqrt d L_i$ is a Lipschitz constant for the max-norm.

Therefore, we can define a new \textit{Lipschitz floor} 

\[\boden_N: x \mapsto \sum_{i=1}^N \chi_{J_i} (x) \, \boden^i_N(x)\]
guaranteeing to be a \emph{lower} bound on $f$:

\[\boden_N( x) \leq f(x), \forall x \in I \subset \Real^d.\]

Therefore, 

\[\hat S_N^\boden:=\int_I \boden_N( x) \, \d x \leq \int_I f(x) \, \d x  = S, \forall x \in I \subset \Real^d.\]
Each $\boden^i_N$ being integrable, we have 
\begin{equation}
\sum_{i=1}^N \int_{J_i} \boden^i_N( x) d\mu(x)=\hat S_N^\boden \leq \int_I f(x) \, \d x.
\label{eq:defint_ceiling}
\end{equation}
Fortunately, we can evaluate $\hat S_{N,i} :=\int_{J_i} \boden^i_N( x) \, \d x$ in closed-form. To this end, we once again evoke Lem. \ref{lem:defint_of_maxnorm} to deduce:

\begin{align*} 
%
\hat S_{N,i}^\boden &=\int_{J_i} \boden^i_N( x) \, \d x \\
%
& = \int_{J_i} f(c_i) - \ell_i \norm{x-c_i}_{\infty} \, \d x \\
%
& = \int_{J_i} f(c_i) \, \d x - \ell_i \int_{J_i}  \norm{x-c_i}_{\infty} \, \d x \\
%
& = f(c_i) \Vol(J_i) - \ell_i 2^d r^{*}(i) (\prod_{q=1}^d r_q(i)) \\
&+ \ell_i 2^d \sum_{q=0}^{d-1} \frac{\prod_{j=1}^{q} \rho_j(i) }{d-q+1} \bigl(\rho_{q+1}^{d-q+1}(i) - \rho_{q}^{d-q+1}(i) \bigr) \\
%
& = \bigl(f(c_i) -  \ell_i r^{*}(i) \bigr) \,2^d (\prod_{q=1}^d r_q(i)) \\
&+ \ell_i 2^d \sum_{q=0}^{d-1} \frac{\prod_{j=1}^{q} \rho_j(i) }{d-q+1} \bigl(\rho_{q+1}^{d-q+1}(i) - \rho_{q}^{d-q+1}(i) \bigr). 
\end{align*}
%
Therefore,
\begin{align} \label{eq:quadlower_multidim}
\hat S_N^\boden &= \sum_{i=1}^N \int_{J_i} \boden^i_N( x) \d x \\
&= \sum_{i=1}^N  \Bigl[ \bigl(f(c_i) -  \ell_i r^{*}(i) \bigr) \,2^d (\prod_{q=1}^d r_q(i)) \\
&+ \ell_i 2^d \sum_{q=0}^{d-1} \frac{\prod_{j=1}^{q} \rho_j(i) }{d-q+1} \bigl(\rho_{q+1}^{d-q+1}(i) - \rho_{q}^{d-q+1}(i) \bigr) \Bigr]\\
& \geq \int_I f(x) \,dx = S.
\end{align}

\textbf{Convergence.}


We have shown $S$

As before we will have to argue that $\decke_N \to f$ uniformly and hence, $\hat S_N^\decke \to S$ as $N \to \infty$ 
for a dense grid sequence $G_N$.
Let $(G_N)_{N \in \nat}$ be a sequence of grids in $\Real^d$. For each  $N \in \nat$, we denote $G_N =: \{\bigl(c_1^N,f(c_1^N), J_1^N\bigr),\ldots,\bigl(c_N^N,f(c_N^N), J_N^N\bigr)\}$ being a set of triples consisting of centre points $c_i^N$, function values $f(c_i^N)$ and hyperrectangle $J_i^N$ (centred around $c_i^N$). 
Superscript $N$, in $c_i^N$ serves to distinguish between the $i$th domain sample in the grid for different choices of $N \in \nat$. Above, we could afford to omit these superscripts, simply writing $c_i$, tacitly assuming fixed $N$. However, for the following argument the superscripts become necessary.
Also, remember, we assumed the hyperrectangles partition the domain. That is, $\forall N \in \nat \forall 1\leq j< q \leq N:  I = \bigcup_{i=1}^N J_i^N \wedge J_j^N \cap J_q^N = \emptyset$.


For $N \in \nat$, $\bar r_i^N = \max\{ r_{i,1}^N,\ldots, r_{i,d}^N\}$ denotes the maximum radius of hyperrectangle $J_i^N = c_i + \bigl([-r_{i,1}^N ,r_{i,1}^N ]\times \ldots \times [-r_{i,d}^N ,r_{i,d}^N ] \bigr)$. Furthermore, $\bar r^N := \max_{i \in \{1,...,N\}} \bar r_i^N$ is the maximum radius of any hyperrectangle in the $N$th partition of $I$.


\begin{defn}[``Eventually dense partition'']
 We say the grid sequence $G_N$ becomes an ``eventually dense partition'' of $I$ if the hyperrectangles shrink indefinitely while still partitioning the entirety of $I$. That is, \\
 
$G_N$ ``becomes an eventually dense partition '' of $I$ $:\Longleftrightarrow$ 
$\bar r^N \stackrel{N \to \infty}{\longrightarrow} 0$ $ \wedge \forall N \in \nat: \Bigl(I = \bigcup_{i=1}^N J_i^N \wedge \forall 1\leq j< q \leq N : J_j^N \cap J_q^N = \emptyset\Bigr)$.

Here, $\bar r^N \stackrel{N \to \infty}{\longrightarrow} 0$ is equivalent to $\forall \epsilon >0 \exists N_0 \in \nat \forall N > N_0 \forall i \in \{1,...,N\}: 0< \bar r_i^N < \epsilon $.
\label{defn:eventuallydensepartition}
\end{defn}
%
%\begin{lem}
%Let $(G_N)_{N \in \nat}$ be a sequence of grids that becomes dense in $I$.
%
%Eventually, the maximum expansion of each hypersquare in the grid becomes arbitrarily small. More precisely, we have  
%$\forall \epsilon > 0 \exists N_0  \in \nat \, \forall N \geq N_0 \forall i \in \{1,\ldots,N\}: \bar r_i^N  \leq \epsilon$.
%
%\begin{proof}
%Assume the conclusion does not hold. That is, $\exists \epsilon > 0 \forall N_0  \in \nat \, \exists N \geq N_0 \exists i \in \{1,\ldots,N\}: \bar r_i^N  > \epsilon$. So, assume $\bar r_i^N  > \epsilon$ where the negation of the conclusion of the lemma implies that $N$ can be arbitrarily large. Now, choose $x \in J_i$
%\end{proof}
%
%\end{lem}

In preparation for the following theorem, we will establish the following observation:
\begin{lem} \label{lem:supinfonJimultidim}
We have:

(I) $\sup_{x \in J_i} \decke_N^i (x) = f(c_i) + \ell_i \bar r_i^N$,\\


(II) $\inf_{x \in J_i}  \boden^i_N(x) = f(c_i) - \ell_i \bar r_i^N$\\
 
and\\

(III)  $\sup_{x \in J_i} \decke_N^i (x) - \boden_N^i(x) = 2 \ell_i \bar r_i^N$.


\begin{proof}
Referring to the relevant definitions, we see that $\sup_{x \in J_i} \norm{x-c_i}_{\infty} = \bar r_i^N$.
Hence, 

(I): $\sup_{x \in J_i} \decke^i_N(x) = f(c_i) + \ell_i \sup_{x \in J_i} \norm{x-c_i}_{\infty}$
$= f(c_i) + \ell_i \bar r_i^N$.

(II): $\inf_{x \in J_i} \boden^i_N(x) = f(c_i) - \ell_i \sup_{x \in J_i} \norm{x-c_i}_{\infty}$
$= f(c_i) + \ell_i \bar r_i^N$.

(III): $\sup_{x \in J_i} \decke_N^i (x) - \boden_N^i(x) = 2 \ell_i \sup_{x \in J_i} \norm{x-c_i}_{\infty}  =  2 \ell_i \bar r_i^N. $
\end{proof} 
\end{lem}


\begin{thm}
If $G_N$ becomes eventually dense in $I$, we have: $\decke_N, \boden_N$ converge to target function $f: I\subset \Real^d \to \Real$ uniformly on domain $I$.

\begin{proof}

Since $G$ is dense with respect to a canonical metric, it is also dense with respect to the max-norm metric $d: \Real^d \times \Real^d \to \Real, (x,\xi) \mapsto \norm{x-\xi}_{\infty}$.

We show that sequence, $(\phi_N)$, $\phi_N \in \einschluss = \{ \phi: I \to \Real | \forall x \in I : \decke_N(x) \geq \phi(x) \geq \boden_N(x) \}$ converges uniformly to $f$, regardless of the identity of $f$, as long as $G_N$ becomes eventually a dense partition of $I$. 

That is, we show $\forall \epsilon >0 \exists N_0 \forall N \geq N_0 \forall x \in I : \abs{\phi_N(x) - f(x)} \leq \epsilon$:
 

Let $\epsilon > 0$ and define $\ell := \max_{i=1,...,N-1} \ell_i$ to be the maximum Lipschitz constant of the intervals $J_1,...,J_N$. Since $G_N$ becomes eventually dense, we know that $\bar r^N \stackrel{N \to \infty}{\longrightarrow} 0 $. Hence, $\exists N_0 \in \nat \forall N > N_0 \forall i \in \{1,...,N\}: 0< \bar r_i^N \leq \delta:=\frac{\epsilon}{2 \ell} $ for some $N_0 \in \nat$.


So, let $N \geq N_0$. 
Note, $\sup_{ x \in I} \abs{\phi_N(x) - f(x)} \leq \sup_{ x \in I} \abs{\decke_N(x) - \boden_N (x)} \leq \max_{i\in \{1,...,N\}} \sup_{ x \in J_i} \abs{\decke_N^i(x) - \boden_N^i (x)}$
$\leq \max_{i}  \abs{\sup_{ x \in J_i}\decke_N^i(x) - \inf_{ x \in J_i} \boden_N^i (x)}$
$\stackrel{Lem. \ref{lem:supinfonJimultidim}}{=} \max_i \abs{ f(c_i) + \ell_i \bar r_i^N - f(c_i) + \ell_i \bar r_i^N}$
$=\max_i \abs{ 2 \ell_i \bar r_i^N}$
$\stackrel{\bar r_i^N \leq \delta}{\leq} 2 \max_i \abs{ l_i \delta } = 2 \delta \max_i l_i = \epsilon$.
Thus, $\forall x \in I: \abs{\phi_N(x) - f(x)} \leq \epsilon$.

We have shown  $\forall \epsilon >0 \exists N_0 \forall N \geq N_0  \sup_{x \in I} \abs{\phi_N(x) - f(x)} \leq \epsilon$ which is equivalent to uniform convergence to $f$.


\end{proof}

\end{thm}

Having established conditions under which our conservative estimates $\decke_N, \boden_N$ converge uniformly to the ground-truth $f$, we apply this result to establish convergence of the corresponding definite integrals to the definite integral of $f$. Owing to the uniformity of our previous convergence results, this proof goes through in a straight-forward manner. 


\begin{thm}\label{thm:defintconv_multidim}
If the grid sequence $G_N$ becomes an eventually dense partition of domain $I$, our conservative definite integrals converge to the ground truth. That is, we have 
\[\forall N \in \nat : \hat S^\decke_N \geq \int_I f(x) \, \d x \geq  \hat S^\boden_N \]

\[ \hat S^\decke_N, \hat S^\boden_N  \stackrel{N \to \infty}{\longrightarrow} \int_I f(x) \, \d x,  \]
 


where $\hat S^\decke_N$ and $ \hat S^\boden_N$ are defined as in Eq. \ref{eq:quadupper_multidim} and Eq. \ref{eq:quadlower_multidim}, respectively. 

\begin{proof}
The first inequalities, $\forall N \in \nat : \hat S^\decke_N \geq \int_I f(x) \, \d x \geq  \hat S^\boden_N$
are a direct consequence of the conservativeness of our estimates. That is, it follows from  $\decke_N(x) \geq f(x) \geq \boden_N(x),\forall x \in I, \forall N \in \nat $ which was shown above utilizing the Lipschitz properties of $f$.

As for the convergence properties, recall that $G_N$ becoming dense implies uniform convergence of the conservative estimates to $f$. 
Due to uniform convergence, we can exchange integral and limites. That is, we have 

$0 = \int_I f(t) \, dt - \int_I f(t) \, dt$
$=  \int_I \lim_{N \to \infty} \decke_N(t) \, dt  - \int_I \lim_{N \to \infty}  \boden_N (t) \, dt$
$\stackrel{unif. conv.}{=} \lim_{N \to \infty} \int_I \decke_N(t) \, dt  - \lim_{N \to \infty} \int_I \boden_N (t) \, dt$    
$=\lim_{N \to \infty} \hat S^\decke_N - \hat S^\boden_N $. Combining this with $\forall N \in \nat : \hat S^\decke_N \geq \int_I f(x) \, \d x \geq  \hat S^\boden_N $ yields the desired result: $\hat S^\decke_N, \hat S^\boden_N  \stackrel{N \to \infty}{\longrightarrow} \int_I f(x) \, \d x$. 


\end{proof}

\end{thm}

\subsubsection{Grids with function samples at arbitrary points within hyperrectangles}
Above, our conservative estimates were based on the assumption that the grid was constructed such that the $N$ function samples 
where always obtained at centre points of the hyperrectangles partitioning the domain in question. If we have complete control over where to sample the target function, it will always possible to construct a grid where this assumption holds true.

However, in certain scenarios, we may have to lift this assumption. For instance, in cases where the samples of the function values represent observational data from experiments where active sampling is not possible or to costly to ensure. 
While we can still partition our integration domain $I$ into $N$ hyperrectangles $J_i^N$   such that each function sample input $c_i^N \in \Real^d$ lies in hyperrectangle $J_i^N$ $(i=1,...,N)$, it may not necessarily be possible to ensure, that $c_i^N$ is a centre point of $J_i^N$. In this case, we need to alter the definition of a grid $G_N$ to be a sequence of $N$ triples $\bigl(c_i^N,f(c_i^N), [-a_i^N,b_i^N]\bigr)$ where $a_i^N,b_i^N \in  \Real_+^d$  $(i=1,...,N)$. Here, each hyperrectangle $J_i^N$ is defined as the set of points 
$c_i^N + [-a_{i,1}^N,b_{i,1}^N] \times \ldots \times [-a_{i,d}^N,b_{i,d}^N]$. 

It will be the goal of the remainder of this section to extend our results to such grids. While our formulas will be recursive rather than closed-form, the solutions are exact and computational effort can be bounded before run-time.
As before, we will omit indices $i$ and $N$, for ease of notation, wherever possible.

In preparation of the following we need the following lemma:

\begin{lem} \label{lem:intcompeven}
For $i=1,...,d$ let $0 < a_i \leq b_i$, and let 

$f: J= [-a_1,b_1] \times ... \times [-a_d,b_d]\to \Real$ \textit{even} in the $j$th component. That is, $\forall i \in \{1,...,d\}: f\bigl( x_1,...,x_d \bigr) =  f\bigl( x_1,...,x_{j-1},-x_j,x_{j+1},...,x_d \bigr)$. If $f$ is Riemann integrable, we have 

$
\int_{-a_1}^{b_1} \ldots \int_{-a_{d}}^{b_{d}} f(x_1,\ldots,x_d ) \, \,dx_1 \ldots \d x_d \\
 =\int_{-a_1}^{b_1} \ldots\int_{-a_{j-1}}^{b_{j-1}} \int_{-b_j}^{a_j} \int_{-a_{j+1}}^{b_{j+1}} \ldots \int_{-a_{d}}^{b_{d}} f(x_1,\ldots,x_d ) \, \,dx_1 \ldots \d x_d  
$
where $\int $ denotes the Riemann integral.

\begin{proof}
Since $f$ is Riemann integrable, it is continuous almost everywhere. Since the integral does not change if we alter the function on a zero-measure subset, we can, without loss of generality, assume that it is continuous on $J$. Hence, we can apply Fubini's theorem. Therefore, without loss of generality, we can assume $j=d$ (if $j<d$ Fubini's allows us to reorder the components to make the $j$th the last component). That is, we assume that $f$ is even in its last input component.

\begin{align*}
&\int_{-a_1}^{b_1} \ldots \int_{-a_{d}}^{b_{d}} f(x_1,\ldots,x_d ) \, \,dx_1 \ldots \d x_d\\
% 
&=\lim_{N_1 \to \infty} \ldots \lim_{N_d \to \infty} \sum_{i_1=1}^{N_1} \ldots \\ 
&\ldots \sum_{i_{d-1}=1}^{N_{d-1}} \Bigl(\sum_{i_d=1}^{N_d} f(-a_1 + i_1 \frac{b_1+a_1}{N_1},...,-a_d + i_d \frac{b_d+a_d}{N_d})  \Bigr)\\
&\stackrel{(i)}{=}\lim_{N_1 \to \infty} \ldots \lim_{N_d \to \infty} \sum_{i_1=1}^{N_1} \ldots \\ 
&\ldots \sum_{i_{d-1}=1}^{N_{d-1}} \Bigl(\sum_{i_d=1}^{N_d} f(-a_1 + i_1 \frac{b_1+a_1}{N_1},...,a_d - i_d \frac{b_d+a_d}{N_d})  \Bigr)\\
&\stackrel{(ii)}{=}\lim_{N_1 \to \infty} \ldots \lim_{N_d \to \infty} \sum_{i_1=1}^{N_1} \ldots \\ 
&\ldots \sum_{i_{d-1}=1}^{N_{d-1}} \Bigl(\sum_{i_d=1}^{N_d} f(-a_1 + i_1 \frac{b_1+a_1}{N_1},...,-b_d + i_d \frac{b_d+a_d}{N_d})  \Bigr)\\
%
&=\int_{-a_1}^{b_1} \ldots \int_{-a_{d-1}}^{b_{d-1}} \int_{-b_{d}}^{a_{d}}f(x_1,\ldots,x_d ) \, \,dx_1 \ldots \d x_d.
\end{align*}
Equality (i) follows from the assumption that $f$ is $d-$ even.
Equality $(ii)$ can be seen by showing $\Bigl(\sum_{i=1}^{N_d} f(-a_1 + i_1 \frac{b_1+a_1}{N_1},...,p_i)  \Bigr) =\Bigl(\sum_{k=1}^{N_d} f(-a_1 + i_1 \frac{b_1+a_1}{N_1},...,q_k)  \Bigr) $ where $p_i = a_d - i \frac{b_d+a_d}{N_d}$ and $q_k = -b_d + k \frac{b_d+a_d}{N_d}$ for $i,k \in \{1,...,N_d\}$. 
We prove this equality by showing 
$\forall i \in \{1,...,N_d\} \exists !  k \in \{1,...,N_d\}: p_i = q_k $ as follows:

Let $i,j \in \{1,...,N_d\}$.
$p_i = q_j \stackrel{def.}{\Leftrightarrow}  a_d - i \frac{b_d+a_d}{N_d} = -b_d + j \frac{b_d+a_d}{N_d} $
$\Leftrightarrow a_d +b_d  =  (j+i) \frac{b_d+a_d}{N_d} \stackrel{(iii)}{\Leftrightarrow}  1 =  (j+i) \frac{1}{N_d} $
${\Leftrightarrow}  i = N_d -j$.

$(iii):$ Equivalence holds since we can divide by $a_d+b_d >0 $ (remember, $b_d \geq a_d > 0$).  
\end{proof}

\end{lem}

\begin{thm}  For $j \in \{1,...,d\}$ let $0 \leq a_j \leq b_j$ $J^{\neg j} := \prod_{i \in \{1,...,d\} \backslash \{j\}} \, [-a_i,b_i]$ the Cartesian product of all intervals except$ [-a_j,b_j]$. Similarly, $x_{\neg j}$ denotes the vector $(x_1,...,x_{j-1},x_{j+1},...,x_d)$ of all components of $x \in \Real^d$, except the $j$th.  
\\ 

Let $M_j := \int_{-a_j}^{b_j} \int_{J^{\neg j}} \norm{x}_\infty \d x_{\neg j} \d x_j$.\\
Assume, we know how to calculate \\
$S_j = \int_{-a_d}^{a_d} \int_{J^{\neg j}} \norm{x}_\infty  \d x_{\neg j} \d x_j$ and \\
$B_j = \int_{-b_d}^{b_d} \int_{J^{\neg j}} \norm{x}_\infty \d x_{\neg j} \d x_j$. We have,
\[M_j = \frac{B_j + S_j}{2}.\]

\begin{proof}
Define $F_j : x_j \mapsto \int_{J^{\neg j}} \norm{(x_1,...,x_d)}_\infty \d x_{\neg j} $. We have,
 
$M_j =  \int_{-a_j}^{b_j} F_j(x_j) \d x_j $
$= \frac{ 2 \int_{-a_j}^{a_j} F_j(x_j) \d x_j + 2 \int_{a_j}^{b_j} F_j(x_j) \d x_j }{2}$
$\stackrel{(i) }{=} \frac{ 2 \int_{-a_j}^{a_j} F_j(x_j) \d x_j +  \int_{a_j}^{b_j} F_j(x_j) \d x_j 
+ \int_{-b_j}^{-a_j} F_j(x_j) \d x_j }{2}$
${=} \frac{  \int_{-a_j}^{a_j} F_j(x_j) \d x_j +  \int_{-b_j}^{b_j} F_j(x_j) \d x_j}{2}$.
Here, equality (i) follows from application of Lem. \ref{lem:intcompeven} to the term $\int_{a_j}^{b_j} F_j(x_j) \d x_j $.
\end{proof}
\end{thm}

We can utilize this theorem in conjunction with Lem. Lem. \ref{lem:defint_of_maxnorm} to prove correctness of the following recursive algorithm:  

\IncMargin{-1em}
\begin{algorithm}
\begin{small}
%\SetKwData{flag}{flag}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%
\Input{Domain $J =  \prod_{i \in \{1,...,d\}} \, [-a_i,b_i], \forall i: b_i \geq a_i >0$}
\Output{Integral $S \, \, (= \int_J \norm{x}_{\infty} \d x)$}
\BlankLine
%\emph{special treatment of the first line}\;
%$\flag \leftarrow 0$;\\
\For{$i \in \{1,...,d\}$}{

\If{ $a_i \neq b_i$}
{
$S \leftarrow \frac{1}{2} Alg. \ref{alg:recursivequad1} (J^{\neg i} \times [-a_i,a_i])  + \frac{1}{2} Alg. \ref{alg:recursivequad1} (J^{\neg i} \times [-b_i,b_i]) $;
return S;
}

}
Compute $S$ according to Lem. \ref{lem:defint_of_maxnorm};\\
return S;

\caption{Recursive integration method.}

\label{alg:recursivequad1}
\end{small}
\end{algorithm}

PROBLEM: recursion might be evoked for each dimension. So, worst-case complexity is at least of the order of $2^d$!!

\begin{ques}
Surely, we can do better than that! ?
\end{ques}


==> content2/Ch_kinkyinf/notes.tex <==
\section{Diverse Notes}

\subsection{Trapezoid rule} 
Non-uniform grid:
\[ \hat S = \frac{1}{2} \sum_{i=1}^N \bigl(\,(t_{i+1} - t_i) \,(f(t_{i+1}) - f(t_i)\, \bigr).\]

Uniform grid with interval length $h$:
\[ \hat S = \frac{h}{2} \sum_{i=1}^N  f(t_{i+1}) - f(t_i).\].

Error:
\[E(f) \leq \sum_{j=1}^N \frac{h^3}{12} \max_{x \in J_j} \abs{f''(x)}\]
where $J_j = [t_j,t_{j+1}]$.

If $f$ real-valued, then 

\[ \xi_1 \in J_1,...,\xi_N \in J_N: E(f) = \sum_{j=1}^N - \frac{h^3}{12} f''(\xi_j) \] 

\subsection{Numerical error}
Due to finite precision of computers need to add a margin of numerical error to the results to be truly conservative when implemented. Such error bounds can be found with standard numerical analysis.
%
%\subsection{H\"older continuity of the map $x \mapsto \metric(x,s)^p$ for $p \in (0,1], s\in I$}
%
 %
%We endeavor to show that $x \mapsto L \norm{ x -s}^p$ is H\"older continuous with coefficient $L$ and exponent $p$.
%
%To this end, we will show that $(x,y) \mapsto \norm{x-y}^p$, for $p \in (0,1] $, is a metric.  This can be utilized to show that
%$x \mapsto \norm{ x -s}^p$ is a H\"older continuous function.
%
%To establish the metric property, we note that any positive definite function that is subadditive gives rise to a canonical metric. Formally :
%
%
%To prove $(x,y) \mapsto \norm{x-y}^p$ is a metric, we need to establish a few facts. 
%Firstly, we remind ourselves of the following well-known fact:
%\begin{lem} \label{lem:pd_n_concave_subadditive}
 %A nonnegative, concave function $g:\Real_{\geq 0} \to \Real$ with $g(0) = 0$ is subadditive. 
 %That is, $\forall x,y \in \Real_{\geq 0}: g(x+y) \leq g(x) + g(y)$. 
 %
 %\begin{proof}
%If $x = y = 0$ then subadditivity trivally holds:  $0=g(x+y) \leq g(x) + g(y) = 0$.
%So, let $x, y \in \Real_+$ such that $x >0 \vee y >0$.
%We have, $g( x +y) = \frac{x}{x+y} g(x+y) + \frac{y}{x+y} g(x+y) \leq g(\frac{x}{x+y} (x+y) ) +  g(\frac{y}{x+y}(x+y)) = g(x) + g(y)$.
%Taking into account that $\frac{x}{x+y}, \frac{x}{x+y} \in [0,1]$, the last inequality can be seen as follows:
%
 %Since $g$ is concave we have 
%$\forall p \in [0,1], x \in \Real: g(p x) =  g(px + (1-p) 0) \geq p g(x) + (1-p) g(0) \geq p g(x)  $. The last inequality follows from $g(0) \geq 0$.
%\end{proof}
%\end{lem}
%
%\begin{lem} \label{lem:x2p_pdNsubadd}
 %Let $h: \begin{cases} \Real_{\geq 0} \to \Real_{\geq 0},\\ \, x \mapsto x^p\end{cases}$, for $p \in (0,1] $. $h$ is positive definite and subadditive. 
 %That is, (i) $h(0) = 0 $ and  $h(x) > 0, \forall x \neq 0$ and (ii) $\forall x,y \in \Real_{\geq 0}: h(x+y) \leq h(x) + h(y)  $.
 %Moreover, $h$ is concave. If $p \in (0,1)$, h is strictly concave. 
 %
%\begin{proof}
%\textit{Pos. def. :} $h(0) = 0$.  Also $\lim_{x \to 0_+} h(x) =0$. Since $\nabla h (x) = p h^{p-1}(x) >0 $ for $x >0$, $h$ is strictly monotonously increasing on $\Real_+$. Hence, $h(x) > 0, \forall x >0$. 
%
%\textit{Concavity:} If $p =1$, $h$ is linear and hence, concave. If $p \in (0,1)$, $\nabla^2 h(x) = p (p-1) h(x)^{p-2} > 0$ regardless of $x$.
%
%\textit{Subadditivity:} Follows directly with Lem. \ref{lem:pd_n_concave_subadditive} on the basis of established positive definiteness and concavity.
  %
%\end{proof}
%\end{lem}
%
%
%
%\begin{lem}\label{lem:hoeldererror_metric}
%Let $p \in (0,1]$.
%With definitions as in Thm. \ref{thm:subaddmetric1}, we assume that set $G$ is endowed with a quasi- metric $d$. Function
%$\metric: \begin{cases} \inspace \times \inspace \to \Real_{\geq 0} \\ (x,y) \mapsto \Bigl(d(x,y)\Bigr)^p \end{cases}$ is a quasi-metric on $G$.
%If $d$ is a metric then so is $\metric$.
%\begin{proof}
 %By Lem. \ref{lem:x2p_pdNsubadd}, $x\mapsto x^p$ is pos. def. and subadditive. Therefore, positive definiteness and the triangle inequality of $d$ readily extend to $\metric$ as follows: 
%
%\textit{Pos. def.:}
%Let $x=0$. $\metric(x,x) = d(x,x)^p = 0^p = 0$. If $x \neq 0$ then $k :=d(x,x) \neq 0$. Hence   $\metric(x,x) = d(x,x)^p = k^p \neq 0$.
%
%\textit{Triangle inequality:}
%Choose arbitrary $x,y,z \in \inspace $. We have $\metric(x,z) = d(x,z)^p \leq (d(x,y) + d(y,z) \bigr)^p \leq d(x,y)^p + d(y,z)^p = \metric(x,y) + \metric(y,z)$. Here, the first inequality followed from the triangle inequality of quasi-metric $d$ and the second from subadditivity properties established in Lem. \ref{lem:x2p_pdNsubadd}.
%
%\textit{Symmetry:} If $d$ is a metric it is symmetric. Hence, $\metric(x,y) = d(x,y)^p = d(y,x)^p = \metric(y,x), \forall x,y \in \inspace $ in which case $\metric$ also is symmetric.
%\end{proof}
%\end{lem}
%
%Before proceeding we establish a slight generalization of the well-known \textit{reverse triangle inequality}:
%
%\begin{lem}[Reverse Triangle Inequality] \label{thm:revtriangle}
%Let  $\inspace$ be a set and $\metric : \inspace^2 \to \Real$ a symmetric function that fulfills the triangle inequality. 
%That is,  $\forall x,y,z \in \inspace: \metric (x,y) = \metric(y,x) \wedge \metric(x,z) \leq \metric(x,y) + \metric(y,z)$.
%
%Then \[\forall x,y,z \in \inspace: \abs{\metric(x,y) - \metric(z,y)} \leq \metric(x,z).\]
%\begin{proof}
%
%For contradiction, assume 
%$\abs{\metric(x,y) - \metric(z,y)}>\metric(x,z)$ for some $x,y,z \in \inspace$.
%This is implies  
%$
%(i)\,\,\, \metric(x,y) - \metric(z,y)>\metric(x,z) 
%\, \, $  or  $
  %\,\,  (ii) \,\,\,\, \metric(z,y)-\metric(x,y) >\metric(x,z)$.
%Both inequalities contradict the triangle inequality:
%$(i) \Leftrightarrow \metric(x,y)  >\metric(x,z) \metric(z,y) $ and 
%$(ii) \Leftrightarrow  \metric(z,y) > \metric(x,z) + \metric(x,y) =  \metric(z,x) + \metric(x,y)$.
%
%\end{proof}
%\end{lem}
%
%
%\begin{thm}
%Let $\metric$ be a metric on set $G$. For arbitrary $s \in \inspace $ we define $\phi_s: \inspace \to \Real $ as $\phi_s: x \mapsto \metric (x,s) $.
%$\phi_s $ is Lipschitz with respect to metric $\metric$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq \metric (x,y). \]
%\begin{proof}
%$\abs{\phi_s(x) - \phi_s(y)} = \abs{\metric(x,s) - \metric(y,s)} \stackrel{Thm. \ref{thm:revtriangle}} {\leq} \metric(x,y), \forall x,y,s \in \inspace $.
%\end{proof}
%\end{thm}
%Finally, combining this theorem with Lem. \ref{lem:hoeldererror_metric} immediately establishes that mappings of the form $\metric(\cdot,s)^p$ and hence, of the form
%$\norm{\cdot -s}^p$ are H\"older continuous with exponent $p$ ($\in (0,1]$):
%
%\begin{thm}
%Let $\metric$ be a metric on set $G$ and let $p \in (0,1], L \geq 0$. For arbitrary $s \in \inspace $ we define $\phi_s:\begin{cases}  \inspace \to \Real \\ x \mapsto L \, \bigl(\metric (x,s) \bigr)^p\end{cases}$.
%$\phi_s $ is H\"older with exponent $p$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq L \, \metric (x,y)^p. \]
%In particular, for any norm $\norm \cdot$ on $G$ and $s \in \inspace $, mapping $x \mapsto L \norm{x-s}^p$ is H\"older with constant $L$ and exponent $p$.
%\begin{proof}
%By Lem. \ref{lem:hoeldererror_metric}, $\metric(\cdot,\cdot)$ is a metric on $G$. Hence, Lem. \ref{thm:revtriangle} is applicable yielding:
%$\abs{\phi_s(x) - \phi_s(y)} = L \, \abs{\metric(x,s)^p - \metric(y,s)^p} \stackrel{Lem. \ref{thm:revtriangle} } {\leq} \metric(x,y)^p, \forall x,y,s \in \inspace$. The last sentence concerning the norms follows from the fact that a mapping $(x,y) \mapsto \norm{x-y}$ defines a metric.
%\end{proof}
%\end{thm}


\subsection{Nice to know but no longer necessary..}
\begin{lem}
Let $(G,+)$ be an Abelian group with neutral element $0$. Let $A: G \to \Real$ be a mapping such that 
$\forall x,y \in G: $
\begin{enumerate}
\item $A(-x) = A(x)$ (A is even),
	\item $A(x) \geq 0 $ and $A(x) = 0 \Leftrightarrow x =0$ (A is pos. def.),
	\item $ A(x+y) \leq A(x) + A(y)$ (A is subadditive). 
\end{enumerate}
Then $\metric (x,y) := A(x-y)$ is a proper metric on $\inspace$.
\begin{proof}
Let $x,y,z \in G$.
Symmetry and pos. def. properties of $\metric$ follow directly from commutativity of $G$ and the assumption that 
$A$ is positive definite and even: Firstly, in a group, we have $x-y = -(y-x)$. Hence, $\metric(x,y) = A(x-y) = A(-(y-x) ) \stackrel{A \, \text{even}}{=} A(y-x) = \metric(x,y)$. Positive definiteness follows directly from the fact that $A$ is positive defininte.

Next, the triangle inequality of our metric is shown: 
 Leveraging subadditivity of $A$,  we have 
$\metric(x,z) = A(x-z) = A\bigl((x-y) + (y-z)\bigr) \leq A(x-y)+A(y-z) = \metric(x,y) +\metric(y,z)$.
\end{proof}
\end{lem}

\begin{thm} \label{thm:subaddmetric1}
Let $p \in (0,1)$ and $(G,+)$ be an Abelian group and $A: \inspace \to \Real_{\geq 0}$ be an even, pos. def. and subadditive mapping. 
Then $\metric: \begin{cases} \inspace \times \inspace \to \Real_{\geq 0} \\ (x,y) \mapsto \bigl(A(x-y)\bigr)^p \end{cases}$ is a metric between elements of $G$.
\begin{proof} 
Let $x \in G$.
$\metric(x,x) = A(0)^p = 0$ due to pos. def. of $A$ and $x \mapsto x^p$.
If $|G| = 1$ we are done. Otherwise assume the contrary and let $y \in \inspace \backslash \{x\}$.
$\metric(x,y) = A(x-y)^p = A(y-x)^p = \metric(y,x)$ since $ \inspace $ is Abelian. This proves symmetry.

Finally we prove the triangle inequality. This is also straight forward, since we have established that $A$ and $x \mapsto x^p$
are subadditive:
Hence, 
$\forall x,y,z \in  \inspace : \metric(x,z) = A(x-y + y-z)^p \leq (A(x-y)  + A(y-z))^p \leq \bigl(A(x-y)\bigr)^p  + \bigl(A(y-z)\bigr)^p$.
\end{proof}
\end{thm}

\subsection{Background}

\begin{defn}[Convergence of function sequences]
For $N \in \nat$, let $f_N : I \to \Real$. $f_N \stackrel{N \to \infty}{\longrightarrow} f$ \textit{pointwise} if
\[\forall \epsilon >0 \exists N_0 \in \nat \forall N\geq N_0\forall x\in I: \abs{f_N(x) - f(x)} < \epsilon. \] 
 
\end{defn}

\begin{defn}[Uniform convergence of function sequences]
For $N \in \nat$, let $f_N : I \to \Real$. $f_N \stackrel{N \to \infty}{\longrightarrow} f$ \emph{uniformly} if
\[ \forall x \in I \forall \epsilon >0  \exists N_0 \in \nat \forall N\geq N_0: \abs{f_N(x) - f(x)} < \epsilon. \] 
\end{defn}

The key distinction between both variants of convergence is that in pointwise convergence, the convergence rate can depend on $x$. By contrast, in uniform convergence the rate is independent of function input $x$.


For our purpose the following definition of a dense set suffices:
\begin{defn}[Dense] Let $(\mathcal X,\norm{\cdot})$ be a $d$-dimensional vector space endowed with norm $\norm{\cdot}$.  
A set $D \subset \mathcal X$ is ($\norm{\cdot}-$) dense in a set $I \subset \mathcal X$ if every  $\norm{\cdot}-$ open subset of $I$ contains at least one point of $D$. That is:
$\forall x \in I, \epsilon > 0 \exists \xi \in D: \norm{\xi - x} < \epsilon$.     
\end{defn}


\begin{defn}[Convergences of set sequences]
Let $(\mathcal X,\norm{\cdot})$ be a $d$-dimensional vector space endowed with norm $\norm{\cdot}$.  
A sequence of sets $(Q_N)_{N \in \nat}$, $Q_N \subset \mathcal X$, converges to set $I \subset \mathcal X$ if the following two conditions hold:

1. For all $ x \in I$ we can chose a sequence $(q_N)_{N \in \nat}$ (where $q_N \in Q_N, \,\forall N \in \nat$) which converges to $x$: $q_N \stackrel{N \to \infty}{\longrightarrow} x$. That is, $\forall x \in I \exists q_1 \in Q_1, q_2 \in Q_2,... \forall \epsilon > 0 \exists N_0 \forall N \geq N_0:  \norm{q_N - x}  < \epsilon$


2. Every sequence $(q_N)_{N \in \nat}$ with $q_N \in Q_N \, (\forall N \in \nat)$ converges to a subset of points $S \subset I$. The latter is to say, $\forall \epsilon > 0 \exists N_0 \forall N \geq N_0: \sup\{ \norm{q_N - \xi} | \xi \in S\} < \epsilon$.

STIMMT DAS????
\end{defn}


\begin{defn}[Uniform convergence of sequences of sets]
Let $(\mathcal X,\norm{\cdot})$ be a $d$-dimensional vector space endowed with norm $\norm{\cdot}$.  
A sequence of sets $(Q_N)_{N \in \nat}$, $Q_N \subset \mathcal X$, $\abs{Q_N} < \infty$ converges to set $I \subset \mathcal X$ \textit{uniformly} if we have:
\[\forall \epsilon > 0 \exists N_0 \in \nat \forall N \geq N_0 \forall x \in I \exists q \in Q_N : \norm{q-x} < \epsilon. \]

If the sequence consists of finite sets, we can rewrite the condition as 
\[\forall \epsilon > 0 \exists N_0 \in \nat \forall N \geq N_0 \forall x \in I : \min_{q \in Q_N} \norm{q-x} < \epsilon. \]

\end{defn}


\section{Norm equivalences}

\begin{thm}
Let $V$ be a $d$-dimensional vector space, $d < \infty$. 
We have \[\forall p, q \in \nat_+ \cup \infty, v\in V: \norm{v}_p \leq \norm{v}_q \leq d^{\frac{1}{q} - \frac{1}{p}} \norm{v}_p.  \]
\end{thm}
In particular:
\begin{cor}
Let $V$ be a $d$-dimensional vector space, $d < \infty$. 
We have $\forall  v\in V:$ 
\begin{enumerate}
\item $\norm{v}_2 \leq \norm{v}_1 \leq \sqrt d \norm{v}_2$, 
\item $\norm{v}_\infty \leq \norm{v}_2 \leq \sqrt d \norm{v}_\infty$, 
\item $\norm{v}_\infty \leq \norm{v}_1 \leq d \norm{v}_\infty$.
\end{enumerate}
\end{cor}


==> content2/Ch_kinkyinf/optimisation.tex <==
\subsubsection{A note on H\"older continuity for optimisation bounds}
%\jcom{Nat suggests to cite no regret optim paper}
%\subsection{A simple bounded optimisation procedure for Hoelder continuous functions on multi-dimensional domains} 
\label{sec:Hoelder_opt_basic_brief}
In the presence of a known Lipschitz constant, optimisation of a Lipschitz continuous function can be done with Shupert's algorithm \cite{Shubert:72}. Of importance to us at various parts of the thesis is, that it also provides non-asymptotic error bounds.  Unfortunately, it is limited to minimising functions on one-dimensional input domains. 
For multi-dimensional domains DIRECT \cite{direct:93} is a global optimiser that is popular, not least because no Lipschitz constant is required. On the flip side, it does not provide the error bounds afforded by Shupert's methods. Furthermore, we will sometimes be interested in bounds on the maxima and minima for the more general case, where the functions to be optimised are H\"older continuous with respect to normed spaces.  
%This is fine when we attempt to find $\bar v$ for a GP. However, for random fields, i.e. multi-input GPs, we require an optimisation algorithm capable of finding a conservative upper bound on the maximum of the kernels $k(\cdot,x_i)$ even for vector inputs. Fortunately, a naive method one could use, even for H\"older-continuous functions, is as follows:
We are currently working on such a method, as well as on a corresponding cubature algorithm. 
As it is work in progress and its exposition is beyond the scope of this work, we will merely sketch a naive version that provides some desired bounded optimisation for H\"older continuous functions:

Let $f: I \subset \Real^d \to \Real$ be a H\"older continuous function with H\"older constant $L$ and exponent $p$ given with respect to the maximum-norm $\norm{\cdot}_\infty$.\footnote{Due to norm-equivalence relationships we can bound each norm by each other norm by multiplication with a well-known constant (see e.g. \cite{koenigsberger:2000}). Therefore, knowing a H\"older-constant with respect to one norm immediately yields a constant with respect to another, e.g. $\norm{\cdot}_\infty \leq \norm{\cdot}_2 \leq \sqrt{d} \norm{\cdot}_\infty$ where $d$ is the dimension of the input space.}  
$S = \{(s_i, f_i) | i =1,...,N\} $ be a sample of target function $f$ with $f_i = f(s_i)$, $s_i \in I, \forall i$. 

Assume $I$ is a hyper-rectangle and  let  $J_1,...,J_N \subset I$ be a partition of the domain $I$ such that each sub-domain $J_j$ is a hyperrectangle containing $s_j$.
(More generally, to avoid $I$ having to be a hyperrectangle itself, one could alternatively assume that the $J_1,\ldots,J_N$ are a covering of $I$. That is, $I \subset \cup_i J_i$.)
 
By H\"older continuity $\forall x \in J_i: \abs{f_i - f(x)} \leq L \norm{x - s_i}_\infty^p$for some $p \in (0,1], L \geq 0$. 
Let  $a_1,\ldots,a_d >0$, $b_1,\ldots,b_d>0$ be defined such that $J_i =  s_i + ([-a_1,b_1] \times...\times [-a_d,b_d])$ where the addition is defined point-wise. Furthermore, let 
\begin{equation}
	D_j:= \max\{a_1,\ldots,a_d, b_1,\ldots,b_d\}
\end{equation}
 be the maximal distance of $s_i$ to the boundary of $J_j$.

Then, $\forall x \in J_j: f(x)  \leq f_j + L \max_{x \in J_j} \norm{x - s_j}_\infty^p =f_j + L D_j^p =: q_i$. 

Since, the hyperrectangles formed a covering of domain $i$, the desired upper bound on the maximum is $\max_{j=1}^N q_j \geq \max_{x \in I} f(x)$.
By the same argument, a lower bound on the maximum based on the finite sample can be obtained as:
$\min_{j=1}^N f_j - L D_j^p  \leq \min_{x \in I} f(x)$.

In conclusion, we have 
\begin{align}
\underline M := \min_{j=1\,...,N} f_j - L \, D_j^p  \leq \min_{x \in I} f(x) \label{eq:minhoeldineqfinsample}\\
\overline M := \max_{j=1,...,N} f_j + L \, D_j^p  \geq \max_{x \in I} f(x). \label{eq:maxhoeldineqfinsample}
\end{align}
%
A \textit{batch} algorithm would get a sample, construct a partition $J_1,...,J_N$ for that sample and then compute the minimum and maximum bounds $\underline M, \overline M$ given above.


An \textit{adaptive} algorithm for bounded optimisation would be able to incrementally expand the given sample. That is, it would incrementally partition domain $I$ into increasing small sub-hyperrectangles until the computational budget is expended or the bounds on the maxima and minima have shrunk satisfactorily. 

The exploration criterion of where to obtain the next function sample could be tailored to finding $\overline M$ or  $\underline M$, depending on the task at hand.

For instance, in a minimisation problem one might choose to obtain a new sample point in the hyperrectangle $J_{j_*}$ where  $ j_* = \arg\min_{j=1\,...,N} f_j - L \, D_j^p $ is the current rectangle where our present bounds allow for the lowest value to be.


%based on reduction of the error $E=\overline M - \underline M$. That is, we desire to add a sample such that $E$ is minimal after the new sample is inserted. 

%
%As an illustration, consider the following situation: We are given the covariance function
%$k(t,t') := \exp(- \abs{t-t'})$. One a priori upper bound on $\bar v$ would be to choose $k(t,t) = 1$.
%If we have training data $\data$, we can compute $\bar v$ as per  Eq. \ref{eq:barvQ}.
%
%To this end, we notice that $k(\cdot,t') = f \circ g (\cdot)$ with $f(t) = \exp(- t)$ and $g(t) = \abs{t-t'}$. Both functions are Lipschitz. That is, they are H\"older with exponent $p_f=p_g = 1$ and constants $L_f=L_g = 1$.



==> content2/Ch_kinkyinf/preliminaries.tex <==
\section{Preliminaries}

\begin{defn} 
Let $(\inspace ,\metric_\inspace ), (\outspace , \metric_\outspace )$ be two metric spaces
$I \subset \inspace$ be an open set. A function $f: \inspace \to \outspace $ is called \emph{H\"older} 
continuous on $I \subset \inspace$ if there exist a \emph{(H\"older) coefficient} $L[I] \geq 0$ and \emph{(H\"older) 
exponent} $p\geq 0$ such that 
\[\forall x,x' \in I : \metric_\outspace \bigl(f(x),f(x')\bigr) \leq L[I] \, \bigl( \metric_\inspace (x,x') \bigr)^p. \]
 \end{defn}
H\"older functions are known to be uniformly continuous. 
A special case of importance is the class of $L$-Lipschitz functions. These are H\"older continuous 
functions with exponent $p=1$. In this context, coeffient $L$ is referred to as Lipschitz constant or number.

\begin{ex}[Square root function]\label{ex:sqrtfctHoelder}
As an example of a H\"older function that is not Lipschitz we can consider $x \mapsto \sqrt(x)$ on domain $I = [0+\epsilon,c]$ where 
$c >\epsilon \geq 0 $. For $\epsilon >0 $ the function is Lipschitz with $L[I] = \sup_{x \in I} \frac{1} {2 \sqrt{x}}$. We can see that the 
coefficient grows inifinitely large as $\epsilon \to 0$. By contrast, the function is H\"older continuous 
with H\"older coefficient $L[I]=1$ and exponent $p=\frac 1 2 $ for any bounded $I \subset \Real$.
We can see this as follows: Let $x,y \in I$ and, without loss of generality,  $y \geq x$. Let $\xi := \sqrt{x}, \gamma := \sqrt{y}$ and thus, $\gamma \geq \xi$. We have:
$\xi \leq \gamma $ $\Leftrightarrow 2 \xi^2 \leq 2\xi\gamma$ $\Leftrightarrow \gamma^2 - 2 \xi\gamma + \xi^2  \leq \gamma^2 - \xi^2$ $\Leftrightarrow (\gamma-\xi)^2  \leq \gamma^2-\xi^2$ $\Leftrightarrow \abs{\gamma-\xi}^2  \leq \abs{\gamma^2-\xi^2}$
 $\Leftrightarrow \abs{\gamma-\xi}  \leq \sqrt{\abs{\gamma^2-\xi^2}}$  $\Leftrightarrow \abs{\sqrt{x}-\sqrt{y}}  \leq \abs{y-x}^{\frac{1}{2}}$. Since, $x,y$ were chosen arbitrarily, we have shown Hoelder continuity as desired.
\end{ex}
 
 In this paper we will consider the special case  $\inspace = \outspace = \Real$ endowed with metric 
 $\metric(x,x') = \abs{x-x'}$.
 Therefore, the H\"older condition becomes 
 \[\forall x,x' \in I : \abs{f(x)-f(x')} \leq L[I] \, \abs{x-x'}^p. \]

\input{content/Ch_kinkyinf/HoelderNLipcontfacts}

\subsection{H\"older continuity of the metric maps}

 
We endeavor to show that $x \mapsto L \norm{ x -s}^p$ is H\"older continuous with coefficient $L$ and exponent $p$. This will become important since these functions will serve as essential building blocks of our conservative H\"older function estimates. 

To this end, we will show that $(x,y) \mapsto \norm{x-y}^p$, for $p \in (0,1] $, is a metric.  This can be utilized to show that
$x \mapsto \norm{ x -s}^p$ is a H\"older continuous function.

To establish the metric property, we note that any positive definite function that is subadditive gives rise to a canonical metric. Formally :


To prove $(x,y) \mapsto \norm{x-y}^p$ is a metric, we need to establish a few facts. 
Firstly, we remind ourselves of the following well-known fact:
\begin{lem} \label{lem:pd_n_concave_subadditive}
 A nonnegative, concave function $g:\Real_{\geq 0} \to \Real$ with $g(0) = 0$ is subadditive. 
 That is, $\forall x,y \in \Real_{\geq 0}: g(x+y) \leq g(x) + g(y)$. 
 
 \begin{proof}
If $x = y = 0$ then subadditivity trivally holds:  $0=g(x+y) \leq g(x) + g(y) = 0$.
So, let $x, y \in \Real_+$ such that $x >0 \vee y >0$.
We have, $g( x +y) = \frac{x}{x+y} g(x+y) + \frac{y}{x+y} g(x+y) \leq g(\frac{x}{x+y} (x+y) ) +  g(\frac{y}{x+y}(x+y)) = g(x) + g(y)$.
Taking into account that $\frac{x}{x+y}, \frac{x}{x+y} \in [0,1]$, the last inequality can be seen as follows:

 Since $g$ is concave we have 
$\forall p \in [0,1], x \in \Real: g(p x) =  g(px + (1-p) 0) \geq p g(x) + (1-p) g(0) \geq p g(x)  $. The last inequality follows from $g(0) \geq 0$.
\end{proof}
\end{lem}

\begin{lem} \label{lem:x2p_pdNsubadd}
 Let $h: \begin{cases} \Real_{\geq 0} \to \Real_{\geq 0},\\ \, x \mapsto x^p\end{cases}$, for $p \in (0,1] $. $h$ is positive definite and subadditive. 
 That is, (i) $h(0) = 0 $ and  $h(x) > 0, \forall x \neq 0$ and (ii) $\forall x,y \in \Real_{\geq 0}: h(x+y) \leq h(x) + h(y)  $.
 Moreover, $h$ is concave. If $p \in (0,1)$, h is strictly concave. 
 
\begin{proof}
\textit{Pos. def. :} $h(0) = 0$.  Also $\lim_{x \to 0_+} h(x) =0$. Since $\nabla h (x) = p h^{p-1}(x) >0 $ for $x >0$, $h$ is strictly monotonically increasing on $\Real_+$. Hence, $h(x) > 0, \forall x >0$. 

\textit{Concavity:} If $p =1$, $h$ is linear and hence, concave. If $p \in (0,1)$, $\nabla^2 h(x) = p (p-1) h(x)^{p-2} > 0$ regardless of $x$.

\textit{Subadditivity:} Follows directly with Lem. \ref{lem:pd_n_concave_subadditive} on the basis of established positive definiteness and concavity.
  
\end{proof}
\end{lem}



\begin{lem}\label{lem:hoeldererror_metric}
Let $p \in (0,1]$.
With definitions as in Thm. \ref{thm:subaddmetric1}, we assume that set $G$ is endowed with a quasi- metric $d$. Function
$\metric: \begin{cases} \inspace \times \inspace \to \Real_{\geq 0} \\ (x,y) \mapsto \Bigl(d(x,y)\Bigr)^p \end{cases}$ is a quasi-metric on $G$.
If $d$ is a metric then so is $\metric$.
\begin{proof}
 By Lem. \ref{lem:x2p_pdNsubadd}, $x\mapsto x^p$ is pos. def. and subadditive. Therefore, positive definiteness and the triangle inequality of $d$ readily extend to $\metric$ as follows: 

\textit{Pos. def.:}
Let $x=0$. $\metric(x,x) = d(x,x)^p = 0^p = 0$. If $x \neq 0$ then $k :=d(x,x) \neq 0$. Hence   $\metric(x,x) = d(x,x)^p = k^p \neq 0$.

\textit{Triangle inequality:}
Choose arbitrary $x,y,z \in \inspace $. We have $\metric(x,z) = d(x,z)^p \leq (d(x,y) + d(y,z) \bigr)^p \leq d(x,y)^p + d(y,z)^p = \metric(x,y) + \metric(y,z)$. Here, the first inequality followed from the triangle inequality of quasi-metric $d$ and the second from subadditivity properties established in Lem. \ref{lem:x2p_pdNsubadd}.

\textit{Symmetry:} If $d$ is a metric it is symmetric. Hence, $\metric(x,y) = d(x,y)^p = d(y,x)^p = \metric(y,x), \forall x,y \in \inspace $ in which case $\metric$ also is symmetric.
\end{proof}
\end{lem}

Before proceeding we establish a slight generalization of the well-known \textit{reverse triangle inequality}:

\begin{lem}[Reverse Triangle Inequality] \label{thm:revtriangle}
Let  $\inspace$ be a set and $\metric : \inspace^2 \to \Real$ a symmetric function that fulfills the triangle inequality. 
That is,  $\forall x,y,z \in \inspace: \metric (x,y) = \metric(y,x) \wedge \metric(x,z) \leq \metric(x,y) + \metric(y,z)$.

Then \[\forall x,y,z \in \inspace: \abs{\metric(x,y) - \metric(z,y)} \leq \metric(x,z).\]
\begin{proof}

For contradiction, assume 
$\abs{\metric(x,y) - \metric(z,y)}>\metric(x,z)$ for some $x,y,z \in \inspace$.
This is implies  
$
(i)\,\,\, \metric(x,y) - \metric(z,y)>\metric(x,z) 
\, \, $  or  $
  \,\,  (ii) \,\,\,\, \metric(z,y)-\metric(x,y) >\metric(x,z)$.
Both inequalities contradict the triangle inequality:
$(i) \Leftrightarrow \metric(x,y)  >\metric(x,z) \metric(z,y) $ and 
$(ii) \Leftrightarrow  \metric(z,y) > \metric(x,z) + \metric(x,y) =  \metric(z,x) + \metric(x,y)$.

\end{proof}
\end{lem}


\begin{thm}
Let $\metric$ be a metric on set $G$. For arbitrary $s \in \inspace $ we define $\phi_s: \inspace \to \Real $ as $\phi_s: x \mapsto \metric (x,s) $.
$\phi_s $ is Lipschitz with respect to metric $\metric$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq \metric (x,y). \]
\begin{proof}
$\abs{\phi_s(x) - \phi_s(y)} = \abs{\metric(x,s) - \metric(y,s)} \stackrel{Thm. \ref{thm:revtriangle}} {\leq} \metric(x,y), \forall x,y,s \in \inspace $.
\end{proof}
\end{thm}
Finally, combining this theorem with Lem. \ref{lem:hoeldererror_metric} immediately establishes that mappings of the form $\metric(\cdot,s)^p$ and hence, of the form
$\norm{\cdot -s}^p$ are H\"older continuous with exponent $p$ ($\in (0,1]$):

\begin{thm}\label{thm:pmetricphoelder}
Let $\metric$ be a metric on set $G$ and let $p \in (0,1], L \geq 0$. For arbitrary $s \in \inspace $ we define $\phi_s:\begin{cases}  \inspace \to \Real \\ x \mapsto L \, \bigl(\metric (x,s) \bigr)^p\end{cases}$, where 
$\phi_s $ is H\"older with exponent $p$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq L \, \metric (x,y)^p. \]
In particular, for any norm $\norm \cdot$ on $G$ and $s \in \inspace $, mapping $x \mapsto L \norm{x-s}^p$ is H\"older with constant $L$ and exponent $p$.
\begin{proof}
By Lem. \ref{lem:hoeldererror_metric}, $\metric(\cdot,\cdot)$ is a metric on $G$. Hence, Lem. \ref{thm:revtriangle} is applicable yielding:
$\abs{\phi_s(x) - \phi_s(y)} = L \, \abs{\metric(x,s)^p - \metric(y,s)^p} \stackrel{Lem. \ref{thm:revtriangle} } {\leq} \metric(x,y)^p, \forall x,y,s \in \inspace$. The last sentence concerning the norms follows from the fact that a mapping $(x,y) \mapsto \norm{x-y}$ defines a metric.
\end{proof}
\end{thm}



 At first glance, the result may seem intuitive. However, it should be noted that, for $p >1$, $x \mapsto \norm{x -s}^p$ is no longer H\"older with exponent $p$. This is consistent with the well-known fact that H\"older functions with exponent $>1$ are constant functions. 
%We conclude this section by the following theorem stating that any concatenation of Hoelder continuous functions is Hoelder continuous:
%
%\begin{thm} \label{thm:concathoelder}
%Let $(\statespace, \metric)$ be a metric space and $f,g : \statespace \to \statespace$ be two Hoelder continuous mappings with Hoelder constants $L_f, L_g$ and Hoelder exponents $p_f,p_g$, respectively.
%Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also Hoelder continuous with Hoelder constant $L_h:= L_f L_g^{p_f}$ and exponent $p_h:=p_g \, p_f$.
%That is, 
%\[\forall \state,\state' \in \statespace: \metric\bigl(h(\state),h(\state')\bigr) \leq L_h \bigl(\metric(\state,\state')\bigr)^{p_h}.\]
%\begin{proof}
%%\begin{align}
%$\metric\bigl(f \circ g(\state),f\circ g(\state')\bigr) \leq L_f  \Bigl(\metric(g(\state),g(\state'))\Bigr)^{p_f}$
%$\leq L_f  \Bigl(L_g \metric(\state,\state')^{p_g}\Bigr)^{p_f}$ $= L_f L_g^{p_f}   \Bigl(\metric(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using Hoelder continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
%
%\end{proof}
%\end{thm} 
%In conjunction with Hoelder properties of the square root function established in Ex. \ref{ex:sqrtfctHoelder}, Thm. 
%\ref{thm:concathoelder} immediately yields the following result:
%\begin{cor}
%If $f: \statespace \to \statespace $ is Hoelder continuous with constant $L_f$ and exponent $p_f$ then $\sqrt{f}$ also is Hoelder, having  Hoelder constant $\sqrt{L_f}$ and exponent $p_f$.
%\end{cor}



==> content2/Ch_kinkyinf/problem_def.tex <==


\section{Problem Definition}
\label{sec:prob_def}
In Ex. \ref{ex:topinf_quad}, we provided an example of a topological inference problem for conservative quadrature. Unfortunately, the proof of conservativeness of the trapezoid method relies upon existence and knowledge of second derivatives and is restricted to one-dimensional integrands. Many applications demand coarser knowledge and applicability to a less-restricted class of integrands. 

%As a basic example, consider the ordinary differential equation $\frac{\d x}{\d t} = (\xi - x)$ where $\xi: I \subset \Real \to \Real $ is an absolutely continuous function superimposed by a countable number of steps. Suppose, the ODE describes the trajectory $x: I \to \Real$ of a controlled particle in one-dimensional state space. Based on $N$ time-state observations $D_N=(t_1,x_1 ),..., (t_N,x_N )$ we desire to estimate the total distance travelled $S$ in time interval $I$, $S = \int_I x(t) \d t$. Solving

\jcom{REVISE:}

\textbf{Setting.}
Let $d \in \nat$ and $I=[a_1,b_1] \times \ldots \times [a_d,b_d] \subset \Real^d$ be a bounded hyperrectangle domain. Assume, we have access to a sample set $D_N:= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N \} $ containing $N \in \nat$ samples value $\tilde f_i$ of the target function $f: I \to \Real$ at sample input $s_i \in I$. The samples have interval-bounded error given by $\varepsilon : I \to \Real_{\geq 0}$. That is, all we know is that $f(s_i) \in [\underline f(s_i), \overline f(s_i) ]$ where $\underline f(s_i) := \tilde f_i - \varepsilon(s_i)$ and $\overline f(s_i) := \tilde f_i + \varepsilon(s_i)$.

The interpretation of the errors depends on the given application. For instance, in an experimental setting they could represent measurement errors. Most relevant to this work, the errors might represent approximation errors that arise if the target has to be approximated numerically.

Furthermore, for each sub-hyperrectangle $J \subset I$ we have access to a Lipschitz number $L_J \geq 0$. That is, $L_J$ is a number such that $\forall x,x' \in J: \abs{f(x) - f(x')} \leq L_J \, \norm{ x- x'}$ where $\norm \cdot$ is a fixed norm on $I$.\footnote{Note, due to norm-equivalence in finite-dimensional space, it is of no principal concern which norm is chosen.} 

 Based on sample set $D_N$, we desire to design algorithms solving the following two
tasks:

\subsection{Task 1 -- Computing a conservative \textit{function estimate}}
\label{sec:problemdef_task1}
Compute a function $B: D_N \mapsto (\decke_N,\boden_N)$ estimating the target that satisfies the following \textbf{desiderata}:
\begin{enumerate}
	\item \textit{Conservatism}. $\decke_N, \boden_N :I \to \Real$ functions that enclose the target conservatively. That is, 
			we can guarantee  $\decke_N(x) \geq f(x) \geq \boden_N(x), \forall x \in I$. (We will refer to $\decke_N, \boden_N$ as (Lipschitz-) ceiling and floor, respectively. 
				\item \textit{Convergence} to the target. If $(D_N)_{N \in \nat }$ is a sample set sequence whose inputs converge to a dense subset of $I$ (as $N \to \infty$), we require $\exists \gamma, \phi \geq 0: \decke_N - f \stackrel{N \to \infty} \longrightarrow \gamma \leq \varepsilon, f- \boden_N \stackrel{N \to \infty} \longrightarrow \phi \leq \varepsilon$ pointwise. In the absence of errors ($\varepsilon \equiv 0$) this means uniform convergence to the target.
				\item \textit{Optimality}. We desire the enclosure to be optimal. That is, to $\decke_N, \boden_N$ should be as tight as possible, without losing conservativeness.
\end{enumerate}

From the perspective of topological inference, the estimator is a data inference method for function estimation:
$B(\cdot) = M_{dinf}(\mathcal K_{prior}, \cdot, \gamma ) $ (for some sufficiently large $\gamma$) mapping sample data into a hypothesis interval of possible functions. 
Here,  our a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L_J$ such that the underlying target $f \in \mathcal F$ is $L_J-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L_J \norm{x-x'}\}$. 
Note, we will not explicitly compute the prior knowledge set. Instead will will fold in the Lipschitz continuity to define an optimal estimator output defining an enclosure that coincides with $\mathcal K_{post} \subset \mathcal K_{prior}$ and hence, with $T (\mathcal K_{post} \cup \mathcal K_{prior})$. Therefore, the resulting inference mechanism will be optimal. 

Note, how our desiderata are equivalent to the corresponding notions of the inference mechanism that is to be designed.

\subsection{Task 2 -- Estimating definite integrals.}
	\label{sec:problemdef_task2}
 Compute an \textit{integral estimator} $E: D_N \mapsto (\underline S_N, \overline S_N)$ of the definite integral $S := \int_I f(x) \, \d x$. The estimator's outputs translate to an estimate $\hat S_N = \frac{\underline S_N+ \overline S_N}{2}$ of $S$ with error $\mathfrak E(D_N) =\overline S_N - \hat S_N = \frac{1}{2} \abs{\overline S_N - \underline S_N}$. Similarly to before, we desire our estimator to exhibit the following properties:
\begin{enumerate}
			\item \textit{Conservatism}.  Regardless of $D_N$, we can guarantee $\overline S_N \geq S \geq \underline S_N$. 
			
			\item \textit{Convergence} to the ground truth. If $(D_N)_{N \in \nat }$ is a sample set sequence whose inputs converge to a dense subset of $I$ (as $N \to \infty$) and $\varepsilon$ is integrable, we require $\abs{\overline S_N - \underline S_N} \stackrel{N \to \infty} \longrightarrow \int_I  \overline \varepsilon(x) \d x$ where $\overline \varepsilon$ is the smallest upper bound function on $\varepsilon$ that is integrable. In the absence of errors ($\varepsilon \equiv 0$) this implies convergence of estimate $\hat S_N$ to the true integral $S$.
			\item \textit{Optimality}. Finally, we desire the bounds to be optimal, that is, to be as tight as possible, without losing conservativeness.
\end{enumerate}

Viewed from the perspective of our topological inference frame-work, the estimator is a data inference method for quadrature:
$E(\cdot) = M_{dinf}(\mathcal K_{prior}, \cdot, \gamma ) $ (for some sufficiently large $\gamma$) mapping sample data into a hypothesis interval of possible functions. 
Here,  our a priori knowledge is that we know, for each $J \subset I$ a nonnegative number $L_J$ such that the underlying target $f \in \mathcal F$ is $L_J-$Lipschitz on $J$. That is, $\mathcal K_{prior} =\{\phi \in \mathcal F \,|\, \forall J \subset I \forall x,x' \in J: \abs(\phi(x) - \phi(x') \leq L_J \norm{x-x'}\}$. 
Note, we will not explicitly compute the prior knowledge set. Instead will will fold in the Lipschitzness to define an optimal estimator output defining an enclosure that coincides with $ T (\mathcal K_{post} \cup \mathcal K_{prior})$ and thus, is optimal.

As for Task 1, our desiderata are equivalent to the corresponding notions of the inference mechanism that is to be designed.



==> content2/Ch_kinkyinf/quad1d.tex <==
\section{Task 2 -- Quadrature}
\label{sec:quadr}

Many numerical methods and bounds rely on derivatives to drive the algorithm and to provide accuracy bounds. For instance, Newton's method searches for roots on the basis of derivatives but is well-known to diverge when attempting to find the root of $x \mapsto x^{1/3}$ which exhibits unbounded derivatives around the root. Or, Gaussian quadrature provides numerical estimates of a one-dimensional integrand on the basis of polynomial interpolation. However, its error bounds depend on the supremum of higher-order derivatives  within the integration domain and hence are not applicable for functions that are not sufficiently smooth or have derivatives that are unbounded, unknown, unbounded or generally hard to maximise. \jcom{citations}
Therefore, Hoelder continuity has recently be considered for quadrature of one dimensional functions \cite{Baran2008}. In this section, we present an approach that allows for numerical integration of Hoelder continuous integrands. We allow for sample function values that are corrupted by noise of an unknown distribution but have known support.

\subsection{Quadrature on one-dimensional domains}
\label{sec:quadr_1dim} 

We consider the case of integration of $L$-Lipschitz continuous functions on one-dimensional domains with metric $\metric: (x,y) \mapsto \abs{x-y}^p$ for some $p \in (0,1]$. That is, the integrand is H\"older continuous with constant $L$ and H\"older exponent $p$.

Let $a,b \in \Real, a \leq b, I := [a,b] \subset \Real$.
We assume we have access to an erroneous sample of a H\"older function $f: I \to \Real $ on a finite grid $G_{N_n} =\{s_1,\ldots,s_{N_n}\} \subset I$, where $a = s_0 \leq s_1 \leq ...\leq s_{N_n}\leq s_{{N_n}+1} =b$. We define $I_i = [s_i,s_{i+1}]$.

Previously, we assumed $L$ was constant. However, from now on, we assume we are given different constants $L_i := L[I_i] \in \Real$ for each interval $I_i$ $(i = 0,\ldots,{N_n})$.  

Our goal is to compute conservative estimates of the definitive Riemann integral \[S := \int_{I} f(t) \, \d t.\] 

In particular, given a finite budget of ${N_n} \in \nat$ function evaluations, we desire (i) to find two  estimates $S^\decke_n , S^\boden_n$ of the definite integral that are upper and lower conservative, respectively. That is, we desire 
\[S^\boden_n \leq S \leq S^\decke_n. \] Furthermore, we desire (ii) convergence to the true value in the limit of an infinite number of function evaluations. That is, we require
$S^\boden_n, S^\decke_n \stackrel{{N_n} \to \infty}{\longrightarrow} S $.
Finally, we desire (iii) $S^\decke_n,S^\boden_n$ to be expressed in closed-form. 

In the one-dimensional case, one obvious way to achieve this is to use the integrals of the H\"older ceiling and floor. That is, we define $S^\decke_n := \int_I \decke_n^* (t) \,dt $ and $S^\boden_n := \int_I \boden_n^* (t) \,dt $. 

(i) follows directly from the properties of the enclosing functions established by Thm. \ref{thm:enclosure1d_desiderata}.

 (iii) is easily addressed via noticing that both ceiling and floor functions are piece-wise polynomial functions. 
 Hence, their definite integrals can be derived in closed-form.  



 Define the \emph{(sub-domain) partitioning} sequence $\xi:=(\xi_0,\ldots,\xi_{{N_n}+1})$ where
$\xi_1, \ldots, \xi_{{N_n}-1} \in \Real$ are called \emph{sub-domain partition points}. 

\begin{defn}[Admissible partitioning sequence]\label{def:xisandJis_1d}
We call partition sequence $\xi$ \emph{admissible} (with respect to sample grid $s_0,\ldots,s_{{N_n}+1}$) if  \[\xi_{i-1} \leq s_i  \leq \xi_{i} \] for $i=1,\ldots,{N_n}-1\text{ and }\xi_0 = s_0, \xi_{N_n} = s_{{N_n}+1}$.
Admissible partitioning sequence $\xi$ defines a partition of \emph{sub-domain intervals} $J_1,\ldots,J_{N_n}$ where the $i$th \emph{sub-domain} interval is defined as \[J_i := [\xi_{i-1},\xi_{i}]\]  $(i \in \{0,\ldots,{N_n}\})$. 

\end{defn}
\begin{rem}
Let  \[S^\decke_n (\xi) := \sum_{i=1}^{N_n} \int_{J_i} \decke^i_n (t) dt \] and 
\[S^\boden_n (\xi) := \sum_{i=1}^{N_n} \int_{J_i} \boden^i_n (t) dt. \]
Lem. \ref{lem:samplefloorceiling} implies that these two integrals are upper and lower bounds of the ground-truth integral. That is, for any admissible $\xi$ satisfying the constraints given in Def. \ref{def:xisandJis_1d} we have
\[S^\boden_n(\xi) \leq \int_I f(t) dt \leq S^\decke_n(\xi). \]
\end{rem}

In preparation of what is to come, we derive the integrals of the sample ceiling and floor functions on the sub-domains.  
\begin{lem} \label{lem:subdomints_1d}
 Remember, the definitions of the (one-dimensional) sample-ceiling  $\decke_n^i (x; L) :x \mapsto  \overline f (s_i) +L_j \abs{x - s_i}^p $ and sample-floor function  
$\boden_n^i (x; L) :x \mapsto  \underline f (s_i) - L_j \abs{x - s_i}^p $ for $x \in I_j$ where 
$L_j = L[I_j]$ is the H\"older coefficient on interval $I_j = (s_j,s_{j+1})$. As before, $J_i = [\xi_{i-1}, \xi_{i}]$ where we choose the $\xi_i$ to be admissible. 
We have:
\begin{enumerate}
	\item $\int_{J_{i}} \decke^i_n(t) \, dt =\overline f(s_i) (\xi_{i} - \xi_{i-1}) +  \frac{L_{i-1}}{{p+1}}(s_i - \xi_{i-1} )^{p+1} + \frac{L_i}{{p+1}} (\xi_{i}-s_i )^{p+1} $.
	\item $\int_{J_{i}} \boden^i_n(t) \, dt =\underline f(s_i)  (\xi_{i}  -  \xi_{i-1} )- \frac{L_{i-1}}{{p+1}} (s_i- \xi_{i-1} )^{p+1} -
 \frac{L_i}{{p+1}} (\xi_{i}-s_i )^{p+1}$.
\end{enumerate}

\begin{proof}
The proof consists in applying simple integration rules to piece-wise linear function. For the ceiling the calculation is as follows: \\
%
$\int_{\xi_{i-1}}^{\xi_i} \decke^i_n(t) \, dt
= \int_{\xi_{i-1}}^{s_i} \overline f (s_i) +L_{i-1} (s_i - t)^p \, dt + \int_{s_i}^{\xi_i} 
\overline f (s_i) +L_i (t - s_i)^p \, dt \\ 
 = \bigl[t \overline f(s_i) - \frac{L_{i-1} (s_i-t )^{p+1}}{p+1}\bigr]_{\xi_{i-1}}^{s_i} + \bigl[t
 \overline f(s_i) + \frac{L_i (t-s_i )^{p+1}}{p+1}\bigr]_{s_i}^{\xi_{i}} \\
= s_i \overline f(s_i) -  \xi_{i-1} \overline f(s_i) + \frac{L_{i-1} (s_i-\xi_{i-1} )^{p+1}}{{p+1}} + 
\xi_{i} \overline f(s_i) + \frac{L_i (\xi_{i}-s_i )^{p+1}}{{p+1}} - s_i \overline f(s_i) \\
= \overline f(s_i)  (\xi_{i}  -  \xi_{i-1} )+ \frac{L_{i-1} (s_i-\xi_{i-1} )^{p+1}}{{p+1}} + 
 \frac{L_i (\xi_{i}-s_i )^{p+1}}{{p+1}}$.

For the sample floor, the calculations are analogous:\\
%
$\int_{\xi_{i-1}}^{\xi_i} \boden^i_n(t) \, dt  
= \int_{\xi_{i-1}}^{s_i} \underline f (s_i) -L_{i-1} (s_i - t)^p \, dt 
+ \int_{s_i}^{\xi_i} \overline f (s_i) -L_i (t - s_i)^p \, dt \\ 
 = \bigl[t \underline f(s_i) + \frac{L_{i-1} (s_i - t )^{p+1}}{p+1}\bigr]_{\xi_{i-1}}^{s_i} 
 + \bigl[t \underline f(s_i) - \frac{L_i (t-s_i )^{p+1}}{{p+1}}\bigr]_{s_i}^{\xi_{i}} \\
= \underline f(s_i)  (\xi_{i}  -  \xi_{i-1} )- \frac{L_{i-1} (s_i-\xi_{i-1} )^{p+1}}{p+1} -
 \frac{L_i (\xi_{i}-s_i )^{p+1}}{p+1}$.

\end{proof}
\end{lem}

Thereby, we have derived closed-form solutions of the integral bounds $S^\decke_n (\xi),S^\boden_n (\xi)$ for any admissible partition sequence $\xi$:

\begin{thm} \label{thm:ceilfloorintofxi} We have 

\begin{align} S^\decke_n (\xi) &= \sum_{i=1}^{N_n}  \tilde f(s_i) (\xi_{i} - \xi_{i-1}) + E(\xi_{i-1},\xi_i \,; s_i,L_i,\varepsilon_i)
	\end{align} 
	and 
 \begin{align} S^\boden_n (\xi) &= \sum_{i=1}^{N_n}  \tilde f(s_i) (\xi_{i} - \xi_{i-1}) -  E(\xi_{i-1},\xi_i \,; s_i,L_i,\varepsilon_i)
\end{align}
where 

\[E(x,y \,;s,L_{i-1},L,e) :=  (y - x)\, e \,+ \frac{L_i}{{p+1}} (y-s )^{p+1}+  \frac{L_{i-1}}{{p+1}}(s-x)^{p+1}     \] for 
$x,y,s, \in \Real, e, L \geq 0$.


\begin{proof}
\begin{align*} S^\decke_n (\xi) &= \sum_{i=1}^{N_n} \int_{J_i} \decke^i_n (t) dt \\
&\stackrel{Lem. \ref {lem:subdomints_1d}}{=}  \sum_{i=1}^{N_n} \overline f(s_i) (\xi_{i} - \xi_{i-1}) 
+ \frac{L_i}{{p+1}} (\xi_{i}-s_i )^{p+1}+  \frac{L_{i-1}}{{p+1}}(s_i- \xi_{i-1} )^{p+1}  \\
&= \sum_{i=1}^{N_n} (\tilde f(s_i) + \varepsilon_i) (\xi_{i} - \xi_{i-1})+ \frac{L_i}{{p+1}} (\xi_{i}-s_i )^{p+1}+  \frac{L_{i-1}}{{p+1}}(s_i- \xi_{i-1} )^{p+1} \\
&= \sum_{i=1}^{N_n} \tilde f(s_i) (\xi_{i} - \xi_{i-1})  + \Bigl( \varepsilon_i (\xi_{i} - \xi_{i-1}) +  \frac{L_i (\xi_{i}-s_i )^{p+1}+  L_{i-1}(s_i-\xi_{i-1} )^{p+1} }{p+1} \Bigr).
	\end{align*} 
	Similarly, 
	\begin{align*} S^\boden_n (\xi) &= \sum_{i=1}^{N_n} \int_{J_i} \boden^i_n (t) dt \\
&\stackrel{Lem. \ref {lem:subdomints_1d}}{=}  \sum_{i=1}^{N_n} \underline f(s_i) (\xi_{i} - \xi_{i-1}) - \frac{L_i}{p+1} (\xi_{i}-s_i )^{p+1}-  \frac{L_{i-1}}{{p+1}}(s_i-\xi_{i-1} )^{p+1}  \\
&= \sum_{i=1}^{N_n} (\tilde f(s_i) - \varepsilon_i) (\xi_{i} - \xi_{i-1}) -  \frac{ L_i (\xi_{i}-s_i )^{p+1}+  L_{i-1} (s_i-\xi_{i-1} )^{p+1} }{{p+1}} \\
&= \sum_{i=1}^{N_n} \tilde f(s_i) (\xi_{i} - \xi_{i-1})  - \Bigl( \varepsilon_i (\xi_{i} - \xi_{i-1}) + \frac{ L_i (\xi_{i}-s_i )^{p+1}+  L_{i-1} (s_i-\xi_{i-1})^{p+1} }{{p+1}} \Bigr).
	\end{align*} 
\end{proof}
\end{thm}

One can construe summand $ \tilde f(s_i) (\xi_{i} - \xi_{i-1})$ as an estimate of the integral on $J_i$
and $ E(\xi_{i-1},\xi_i \,; s_i,L_i,\varepsilon_i)$ as an error term due to unknown variation up to $L_i$ and measurement error $\varepsilon_i$.
Note, in the absence of measurement errors, as the grid becomes increasingly dense (as ${N_n} \to \infty$), the error due to variation will vanish and the integral estimate $\sum_{i=1}^{N_n} \tilde f(s_i) (\xi_{i} - \xi_{i-1})$ converge to the true integral of $f$.

%
%
%\begin{ques} When we sample  errors (uniformly from a const interval)  and let the grid become dense (but keep pruning) should the sampling error not also vanish since only samples are kept that are informative? Or would the probability of sampling informative values shrink to zero for denser grids? (it might) So what is the stationary uncertainty?
%\end{ques} 

Our next task will be to find $\xi$ such that our integral estimates become as tight as possible. 
Since $\xi_0 = s_0 $ and $\xi_{{N_n}} = s_{{N_n}+1}$ are uniquely predetermined, 
all we are left to do is to find the non-boundary partition points 
$\Xi:=(\xi_1,...,\xi_{{N_n}-1})$. Since we require each $\xi_i$ to be admissible, that is to lie in interval $I_i = [s_{i},s_{i+1}]$, we can reduce the problem of finding $\xi_i$ to determining $\lambda_i \in [0,1]$ where \[\xi_i = s_{i} + \lambda_i (s_{i+1}-s_{i}) = s_{i+1} - (1-\lambda_i) (s_{i+1}-s_{i}) .\]  
That is, we desire to find admissible solutions
\begin{equation}
\Xi^\decke := \argmin_{(\lambda_1,...,\lambda_{{N_n}-1})} \mathfrak S^\decke_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr)
\end{equation} and
 \begin{equation}
\Xi^\boden := \argmax_{(\lambda_1,...,\lambda_{{N_n}-1})} \mathfrak S^\boden_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr)
\end{equation}
where  
\begin{align}
\mathfrak S^\decke_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr) := S^\decke_n\bigl((\xi_0,s_{1} + \lambda_1 (s_{2}-s_{1}),...,s_{{N_n}-1} + \lambda_{{N_n}-1} (s_{{N_n}}-s_{{N_n}-1}),\xi_{{N_n}})\bigr)\\
\mathfrak S^\boden_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr) := S^\boden_n\bigl((\xi_0,s_{1} + \lambda_1 (s_{2}-s_{1}),...,s_{{N_n}-1} + \lambda_{{N_n}-1} (s_{{N_n}}-s_{{N_n}-1}),\xi_{{N_n}})\bigr).
\end{align}

 
Fortunately, this task is simplified by the analytic properties of the objective functions.
For $i \in \{1,\ldots,{N_n}-1\}$ the partial derivatives are 
\begin{align*}
\partial_i \mathfrak S^\decke_n (\lambda_1,\ldots,\lambda_{{N_n}-1}) &= \tilde f(s_i) - \tilde f(s_{i+1})  + \varepsilon_i - \varepsilon_{i+1} 
+ L_i   (s_{i+1}-s_i )^p   (\lambda_i^p- (1-\lambda_i )^p)\\
\partial_i \mathfrak S^\boden_n (\lambda_1,\ldots,\lambda_{{N_n}-1}) &= \tilde f(s_i)  - \tilde f(s_{i+1}) - \varepsilon_i + \varepsilon_{i+1} - L_i   (s_{i+1}-s_i )^p   (\lambda_i^p- (1-\lambda_i )^p).
\end{align*}
%\begin{align*}
%\partial_i \mathfrak S^\decke_n (\xi_1^,...,\xi_n) &= \tilde f(s_i) - \tilde f(s_{i+1})  + \varepsilon_i - \varepsilon_{i+1} + L_i  (\xi_{i}-s_i )^p    - L_{i}  (s_{i+1} - \xi_{i} )^p\\
%\partial_i \mathfrak S^\boden_n (\xi_1,...,\xi_n) &= \tilde f(s_i)  - \tilde f(s_{i+1}) - \varepsilon_i + \varepsilon_{i+1} - L_i  (\xi_{i}-s_i )^p    + L_{i}  (s_{i+1} - \xi_{i})^p
%\end{align*}
%for $i \in \{1,\ldots,{N_n}-1\}$.

Therefore,the second partial derivatives are :
\[
\partial_i \partial_j \mathfrak S^\decke_n (\lambda_1,\ldots,\lambda_{{N_n}-1}) = \begin{cases}  L_i   (s_{i+1}-s_i )^p   (p \, \lambda_i^{p-1}+ p (1-\lambda_i )^{p-1})&, \text{ if } i =j\\ 0 &, \text{ otherwise} \end{cases}
\]
and 
\[
\partial_i \partial_j \mathfrak S^\boden_n (\lambda_1,\ldots,\lambda_{{N_n}-1})= \begin{cases}  - L_i   (s_{i+1}-s_i )^p   (p \lambda_i^{p-1}+ p (1-\lambda_i )^{p-1}) &,  \text{ if }  i =j\\ 0 &, \text{ otherwise.} \end{cases}
\]
Hence, $\nabla^2 \mathfrak S^\boden_n $ and $\nabla^2 \mathfrak S^\decke_n$ are negative definite and positive definite, respectively. Thus, $\mathfrak S^\boden_n, \mathfrak S^\decke_n$ are concave and convex respectively.  Therefore, global extrema exist and, for the optimal ceiling and floor partition, all we need to do is to solve the equations: 
\begin{align}
\nabla \mathfrak S^\decke_n (\lambda_1^\decke,\ldots, \lambda_{N_u-1}^\decke) = 0\\
\nabla \mathfrak S^\boden_n (\lambda_1^\boden,\ldots, \lambda_{N_u-1}^\boden) = 0.
\end{align}





Setting each $i$th partial derivative to zero yields the $N_u-1$ equation pairs :

%%\begin{align*}
%\begin{equation} \label{eq:lambdaceil}
%(\lambda_i^\decke )^p- (1-\lambda_i^\decke )^p = \frac{\tilde f(s_{i+1}) - \tilde f(s_i) + \varepsilon_{i+1} - \varepsilon_i}{ L_i   (s_{i+1}-s_i )^p}  \end{equation}
    %which we need to solve for $\lambda_i \in [0,1]$ to obtain $\xi^\decke_i$ and
%\begin{equation} \label{eq:lambdafloor} \lambda_i^p- (1-\lambda_i )^p =-\frac{\tilde f(s_{i+1}) - \tilde f(s_i) + \varepsilon_{i+1} - \varepsilon_i}{ L_i   (s_{i+1}-s_i )^p}  \end{equation}
%which we need to solve for $\lambda_i \in [0,1]$ to obtain $\xi^\boden_i$.
%%\end{align*}

\begin{align}
g(\lambda_i^\decke) &= \gamma_i \label{eq:g1}\\
   g(\lambda_i^\boden) &= -\gamma_i. \label{eq:g2}
\end{align}
where \[g(\lambda) := \lambda^p- (1-\lambda )^p \] and \[\gamma_i := \frac{\tilde f(s_{i+1}) - \tilde f(s_i) + \varepsilon_{i+1} - \varepsilon_i}{ L_i   (s_{i+1}-s_i )^p}.\]

It is easy to show that both equations can always be solved: Firstly, due to the H\"older properties of the target, we have $\gamma_i \in [-1,1]$. Moreover, $g$ injectively maps $[0,1]$ to $[-1,1]$ (which implies that we can always find a solution by inverting $g$). This is true since $\nabla g (\lambda) = p \lambda^{p-1} + p (1-\lambda)^{p-1} >0 $ and thus, $g$ is strictly monotonously increasing on $[0,1]$. Moreover $g(0) = -1$ and $g(1) = 1$. The rest follows from the Intermediate Value Theorem. Example plots of $g$ for various choices of $p$ are depicted in Fig. \ref{fig:gvonp}. 

Note,
$g(\lambda) = - g(1-\lambda) $ for $\lambda \in [0,1]$. Thus, 
\begin{equation} \lambda_i^\decke = 1 - \lambda_i^\boden,\,\,\forall i. \end{equation} Therefore, solving Eq. \ref{eq:g1} automatically yields a solution to Eq. \ref{eq:g2}.


\begin{figure}[htb] \label{fig:gvonp}
	\centering
		\includegraphics[scale =.4]{content/content_hoelderquad2/figs/gvonp.pdf}
	\caption{Function $g$ as a function of $\lambda$ for varying H\"older exponents $p$.}
\end{figure}


To solve for the $\lambda_i$, and thus, the breakpoints $\xi_i$, for several H\"older exponents $p$, closed -form solutions can be easily derived. For instance, for $p=1$ we have

\begin{align}
 \xi_i^\decke &= \frac{ s_i    + s_{i+1}}{2} + \frac{\varepsilon_{i+1} - \varepsilon_i   +\tilde f(s_{i+1}) - \tilde f(s_i) }{ 2 L_i} \\
&= \frac{ s_i    + s_{i+1}}{2} + \frac{ \overline f(s_{i+1}) - 
\overline f(s_i) }{ 2 L_i} \label{eq:lipxiceil}
\end{align}

and 

\begin{align}
   \xi_{i}^\boden    &=   \frac{ s_i    + s_{i+1}}{2} - \frac{\varepsilon_{i+1} - \varepsilon_i   +\tilde f(s_{i+1}) - \tilde f(s_i) }{ 2 L_i} \\
&= \frac{ s_i    + s_{i+1}}{2} - \frac{ \underline f(s_{i+1}) - 
\underline f(s_i) }{ 2 L_i} \label{eq:lipxifloor}
\end{align}

%\begin{align}
 %\xi_i^\decke &= \frac{\varepsilon_{i+1} - \varepsilon_i   +\tilde f(s_{i+1}) - \tilde f(s_i) +L_i s_i    + 
%L_{i+1}s_{i+1}}{ L_i+ L_{i+1}} \\
%&= \frac{L_i s_i    + L_{i+1}s_{i+1} + \overline f(s_{i+1}) - 
%\overline f(s_i) }{ L_i+ L_{i+1}}
%\end{align}
%
%and 
%
%\begin{align}
   %\xi_{i}^\boden    &=   \frac{ L_{i+1} s_{i+1} + L_i s_i + \tilde f(s_i) - \tilde f(s_{i+1})  - \varepsilon_i  + \varepsilon_{i+1}}{L_i+ L_{i+1}}\\
	%&=   \frac{L_i s_i+ L_{i+1} s_{i+1}  + \underline f(s_i) - \underline f(s_{i+1})  }{L_i+ L_{i+1}}
%\end{align}

for $ i \in \{1,\ldots,{N_n}-1\} $.



Not surprisingly, we have recovered the break-points of the ceiling and floor functions as per  Lem. \ref{lem:ceiling_maxvalues} and Lem. \ref{lem:floor_minvalues}. Both Lemmata also establish admissibility of our solutions (i.e. $\xi^\decke_i, \xi^\boden_i \in I_i)$. 

Consequently, the best partition point sequences  $\Xi^\decke,\Xi^\boden  $ yield integral bounds that coincide with the integrals of the optimal ceiling and floor functions:
$\mathfrak S^\decke_n\bigl(\lambda_1^\decke ,...,\lambda_{{N_n}-1}^\decke \bigr) = \int_I \decke^*_n(t) dt$ and
$\mathfrak S^\boden_n\bigl(\lambda_1^\boden ,...,\lambda_{{N_n}-1}^\boden \bigr) = \int_I \boden^*_n(t) dt.$

In case no closed form solution is known, we can approximate numerically. Due to the simplicity of the problem at hand, this can be achieved rapidly with a robust root finding algorithm such as Ridder's method \cite{ridders1979}. By construction, a suboptimal solution still yields conservative integral estimate bounds so we can stop the root finding method after a few iterations without obtaining overly confident bounds. 

%
%Of course, we could also derive the tightest integral estimate bounds by directly integrating the optimal enclosure:
%
%\begin{thm} \label{thm:quad_ceil} 
%Remember, the sample grid is given by erroneous function samples at inputs $s_1 < \ldots < s_n$. Let  
%$s_0 = \inf I \leq s_1, s_{{N_n}+1} = \sup I \geq s_n$ and  $\xi^{\decke}_i =  \frac{s_i+s_{i+1}}{2}+ \frac{\overline f(s_{i+1}) - \overline f(s_i)}{2 L_i}  $.
%%augmented grid $\tilde G_n = (t_1, \xi_1^\decke, t_2, \xi_2^\decke, t_3,\ldots,t_{{N_n}-1},\xi_{{N_n}-1}^\decke,t_{{N_n}} )$, and let $\tau_j$ denote the $j$th element 
%%of augmented grid $\tilde G_n$.
%We have 
%\begin{align*}
%\int_I \decke_n^* (t) \, \d t  &=s_{{N_n}+1} \overline f(s_n)  - s_0 \overline f(s_{1}) + \frac{L_0 (s_0 -s_{1})^2}{2} + \frac{L_{{N_n}} (s_{{N_n}+1}-s_n )^2}{2}  \\
		 %&+\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( \overline f(s_i) - \overline f(s_{i+1}) \bigr) + \frac{L_i}{2} \bigl( (\xi^\decke_{i}-s_i )^2+ (\xi^\decke_{i} -s_{i+1})^2 \bigr)\\
		%&\Bigl(= \mathfrak S^\decke_n (\Xi^\decke)\Bigr).
%\end{align*}
%
%%\[ S^\decke_n  = \frac{1}{2} \sum_{i=1}^{3{N_n}-1} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\decke_nx^i(\xi^{\decke}_i)(
%%\tau_{i+1}) - \decke_n^i(\xi^{\decke}_i)(
%%\tau_{i})\bigr), \, ({N_n} > 1);\]
%%
%%\[ S^\decke_n  = \frac{1}{2} \sum_{i=1}^{3{N_n}} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\decke_n^i(\xi^{\decke}_i)(
%%\tau_{i+1}) - \decke_n^i(\xi^{\decke}_i)(
%%\tau_{i})\bigr), \, ({N_n} = 1).\]
%
%\begin{proof} With 
%$\alpha^\decke_i: x \mapsto \overline f(a_i) + L_i (x - s_i)$ and $\beta^\decke_i: x \mapsto
%\overline f(b_i) -L_i (x - s_{i+1})$ the H\"older ceiling on $I_i$ coincides with the piecewise-linear function $t \mapsto \min\{ \alpha^\decke_i(t), \beta^\decke_i(t)\}$; as per Lem. \ref{lem:ceiling_maxvalues}, for all $t \in I_i$, we have $\decke_n^*(t) = 
 %\begin{cases}  
 %\overline f(a_i) + L_i (t - s_i), & t \leq \xi^\decke_i \\
 %\overline f(b_i) -L_i (t - s_{i+1}), & t > \xi^\decke_i 
 %\end{cases}$.
%
%Therefore,
%
%%\begin{align*}
%$S^\decke_n = \int_I \decke_n^* (t) \, \d t\\
 %%
 %\stackrel{Thm. \ref{thm:lipceil1d}}{=} \int_{I_0}  \decke^*_1 (t) \, \d t + \int_{I_{N_n}}  \decke^{N_n}_{N_n} (t) \, \d t + \sum_{i=1}^{{N_n}-1} \int_{I_i} \min\{\decke_n^i(t),\decke_n^{i+1}(t) \}\, \d t\\
 %%
 %\stackrel{Lem. \ref{lem:ceiling_maxvalues}} {=} \int_{I_0}  \decke^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \decke^{N_n}_{N_n} (t) \, \d t + \sum_{i=1}^{{N_n}-1} \Bigl(\int_{s_i}^{\xi^\decke_i} \decke_n^i(t) \, \d t + \int_{\xi^\decke_i}^{s_{i+1}} \decke_n^{i+1}(t) \, \d t \Bigl)\\
%%  
  %= \int_{I_0}  \decke^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \decke^{N_n}_{N_n} (t) \, \d t \\
	 %+ \sum_{i=1}^{{N_n}-1} \bigl( \int_{s_i}^{\xi^\decke_{i}}  \overline f(s_i) + L_i (t - s_i) \, \d t + \int_{\xi^\decke_{i}}^{s_{i+1}}   \overline f(s_{i+1}) -L_i (t - s_{i+1})\, \d t \bigr)\\
  %%
  %= \int_{I_0}  \decke^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \decke^{N_n}_{N_n} (t) \, \d t \\
	 %+ \sum_{i=1}^{{N_n}-1} \bigl( \bigl[t \overline f(s_i) + \frac{L_i (t-s_i )^2}{2}\bigr]_{s_i}^{\xi^\decke_{i}}  + \bigl[t \overline f(s_{i+1}) - \frac{L_i (t -s_{i+1})^2}{2}\bigr]^{s_{i+1}}_{\xi^\decke_{i}} \bigr)\\
  %%
  %= \int_{I_0}  \decke^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \decke^{N_n}_{N_n} (t) \, \d t \\
	 %+ \sum_{i=1}^{{N_n}-1} \Bigl( \xi^\decke_{i} \overline f(s_i) + \frac{L_i (\xi^\decke_{i}-s_i )^2}{2} - s_i \overline f(s_i)   
  %- \xi^\decke_{i} \overline f(s_{i+1}) + \frac{L_i (\xi^\decke_{i} -s_{i+1})^2}{2}  + s_{i+1} \overline f(s_{i+1}) \Bigr)\\
  %%
    %=  \int_{s_0}^{s_1}  \decke^1_{N_n} (t) \, \d t + \int_{s_{N_n}}^{s_{{N_n}+1}}  \decke^{N_n}_{N_n} (t) \, \d t \\
	%+ s_{N_n} \overline f(s_{N_n}) - s_1 \overline f(s_1)+\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( \overline f(s_i) - \overline f(s_{i+1}) \bigr) + \frac{L_i}{2} \bigl( (\xi^\decke_{i}-s_i )^2+ (\xi^\decke_{i} -s_{i+1})^2 \bigr)      \\
		%%
    %=  \bigl[t \overline f(s_{1}) - \frac{L_0 (t -s_{1})^2}{2}\bigr]^{s_{1}}_{s_0} +   \bigl[t \overline f(s_{N_n}) + \frac{L_{N_n} (t-s_{N_n} )^2}{2}\bigr]_{s_{N_n}}^{s_{{N_n}+1}}  + s_{N_n} \overline f(s_{N_n}) - s_1 \overline f(s_1) \\
		 %+\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( \overline f(s_i) - \overline f(s_{i+1}) \bigr) + \frac{L_i}{2} \bigl( (\xi^\decke_{i}-s_i )^2+ (\xi^\decke_{i} -s_{i+1})^2 \bigr)     \\ 
				%%
    %=  s_1 \overline f(s_{1})  - s_0 \overline f(s_{1}) + \frac{L_0 (s_0 -s_{1})^2}{2} -   s_{N_n} \overline f(s_{N_n}) + s_{{N_n}+1} \overline f(s_{N_n}) + \frac{L_{N_n} (s_{{N_n}+1}-s_{N_n} )^2}{2}  + s_{N_n} \overline f(s_{N_n}) - s_1 \overline f(s_1) \\
		 %+\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( \overline f(s_i) - \overline f(s_{i+1}) \bigr) + \frac{L_i}{2} \bigl( (\xi^\decke_{i}-s_i )^2+ (\xi^\decke_{i} -s_{i+1})^2 \bigr)     \\ 
						%%
    %= s_{{N_n}+1} \overline f(s_{N_n})  - s_0 \overline f(s_{1}) + \frac{L_0 (s_0 -s_{1})^2}{2} + \frac{L_{N_n} (s_{{N_n}+1}-s_{N_n} )^2}{2}  \\
		 %+\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( \overline f(s_i) - \overline f(s_{i+1}) \bigr) + \frac{L_i}{2} \bigl( (\xi^\decke_{i}-s_i )^2+ (\xi^\decke_{i} -s_{i+1})^2 \bigr).   \\ $
		%%\end{align*}
		%
%\end{proof}
%
%\end{thm}
%
%Of course, we can derive the completely analogous statement for the H\"older floor. 
%
%
%\begin{thm} \label{thm:quad_floor} Remember, the sample grid is given by erroneous function samples at inputs $s_1 < \ldots < s_{N_n}$ and let 
%$s_0 = \inf I \leq s_1, s_{{N_n}+1} = \sup I \geq s_{N_n}$. As before, let $\xi^{\mathfrak l}_i := \frac{s_i+s_{i+1}}{2} - \frac{\underline f(s_{i+1}) - \underline f(s_i)}{2 L_i}  $. 
%%augmented grid $\tilde G_{N_n} = (t_1, \xi_1^\boden, t_2, \xi_2^\boden, t_3,\ldots,t_{{N_n}-1},\xi_{{N_n}-1}^\boden,t_{{N_n}} )$, and let $\tau_j$ denote the $j$th element 
%%of augmented grid $\tilde G_{N_n}$.
%We have \\
%\begin {align*}
%\int_I \boden_n^* (t) \, \d t&=s_{{N_n}+1} \underline f(s_{N_n})-s_0 \underline f(s_1) - \frac{1}{2} L_0 (s_0 - s_1)^2  - \frac{1}{2} L_{N_n} (s_{{N_n}+1} - s_{N_n})^2 \\
%&+  \sum_{i=1}^{{N_n}-1} \Bigl(\xi^\boden_{i} \bigl( \underline f(s_i) - \underline f(s_{i+1})\bigr) - \frac{L_i}{2} \bigl( (\xi^\boden_{i}-s_i )^2 + (\xi^\boden_{i} -s_{i+1})^2 \bigr) 
 %\Bigr)\\
%&\Bigl(= \mathfrak S^\boden_n (\Xi^\boden)\Bigr).
%\end{align*} 
%
%
%%\[ S^\boden_n  = \frac{1}{2} \sum_{i=1}^{3{N_n}-1} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\boden_n^i(\xi^{\boden}_i)(
%%\tau_{i+1}) - \boden_n^i(\xi^{\boden}_i)(
%%\tau_{i})\bigr), \, ({N_n} > 1);\]
%%
%%\[ S^\boden_n  = \frac{1}{2} \sum_{i=1}^{3{N_n}} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\boden_n^i(\xi^{\boden}_i)(
%%\tau_{i+1}) - \boden_n^i(\xi^{\boden}_i)(
%%\tau_{i})\bigr), \, ({N_n} = 1).\]
%
%\begin{proof} By virtue of Lem. \ref{lem:floor_minvalues} we have 
 %$\forall t \in I_i: \,\,\, \boden^*_{N_n}(t) = 
 %\begin{cases}  
 %\alpha_i^{\mathfrak l} (t), & t \leq \xi_i^\boden \\
 %\beta_i^{\mathfrak l} (t), & t \geq \xi_i^\boden
 %\end{cases}$ 
%% 
 %where $\alpha^\boden_i( t) = \underline f(s_i) - L_i (t - s_i)$ and $\beta^\boden_i( t) =
%\underline f(s_{i+1}) +L_i (t - s_{i+1})$.\\
%
%Therefore,
%
%$S^\boden_n = \int_I \boden_n^* (t) \, \d t\\
%\stackrel{Thm\ref{thm:lipfloor1d}}{=} \int_{I_0}  \boden^*_1 (t) \, \d t + \int_{I_{N_n}}  \boden^{N_n}_{N_n} (t) \, \d t + \sum_{i=1}^{{N_n}-1} \int_{I_i} \max\{\boden_n^i(t),\boden_n^{i+1}(t) \}\, \d t\\
%%
 %\stackrel{Lem. \ref{lem:floor_minvalues}} {=} \int_{I_0}  \boden^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \boden^{N_n}_{N_n} (t) \, \d t + \sum_{i=1}^{{N_n}-1} \Bigl(\int_{s_i}^{\xi^\boden_i} \boden_n^i(t) \, \d t + \int_{\xi^\boden_i}^{s_{i+1}} \boden_n^{i+1}(t) \, \d t \Bigl)\\
%%
  %% 
  %= \int_{I_0}  \boden^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \boden^{N_n}_{N_n} (t) \, \d t + \sum_{i=1}^{{N_n}-1} \bigl( \int_{s_i}^{\xi^\boden_{i}}  \underline f(s_i) - L_i (t - s_i) \, \d t + \int_{\xi^\boden_{i}}^{s_{i+1}}   \underline f(s_{i+1}) +L_i (t - s_{i+1})\, \d t \bigr)\\
  %%
  %= \int_{I_0}  \boden^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \boden^{N_n}_{N_n} (t) \, \d t +\sum_{i=1}^{{N_n}-1} \bigl( \bigl[t \underline f(s_i) - \frac{L_i (t-s_i )^2}{2}\bigr]_{s_i}^{\xi^\boden_{i}}  + \bigl[t \underline f(s_{i+1}) + \frac{L_i (t -s_{i+1})^2}{2}\bigr]^{s_{i+1}}_{\xi^\boden_{i}} \bigr)\\
  %%
  %= \int_{I_0}  \boden^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \boden^{N_n}_{N_n} (t) \, \d t +\sum_{i=1}^{{N_n}-1} \Bigl( \xi^\boden_{i} \underline f(s_i) - \frac{L_i (\xi^\boden_{i}-s_i )^2}{2} - s_i \underline f(s_i)   
  %- \xi^\boden_{i} \underline f(s_{i+1}) - \frac{L_i (\xi^\boden_{i} -s_{i+1})^2}{2}  + s_{i+1} \underline f(s_{i+1}) \Bigr)\\
  %%
    %\stackrel{\text{telescope-} \sum}{=}  \int_{I_0}  \boden^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \boden^{N_n}_{N_n} (t) \, \d t + s_{N_n} \underline f(t_{N_n}) - s_1 \underline f(s_1)+\sum_{i=1}^{{N_n}-1} \Bigl(\xi^\boden_{i} \underline f(s_i) - \frac{L_i (\xi^\boden_{i}-s_i )^2}{2}   
  %- \xi^\boden_{i} \underline f(s_{i+1}) - \frac{L_i (\xi^\boden_{i} -s_{i+1})^2}{2}  \Bigr) \\
  %%%
  %%= \int_{I_0}  \boden^1_{N_n} (t) \, \d t + \int_{I_{N_n}}  \boden^{N_n}_{N_n} (t) \, \d t + s_{N_n} \underline f(t_{N_n}) - s_1 \underline f(t_1)+  \sum_{i=1}^{{N_n}-1} \Bigl(\xi^\boden_{i} \bigl( \underline f(s_i) - \underline f(s_{i+1})\bigr) - \frac{L_i}{2} \bigl( (\xi^\boden_{i}-s_i )^2 + (\xi^\boden_{i} -s_{i+1})^2 \bigr) 
 %%\Bigr)  \\
 %%%
  %= [t \underline f(s_1) + \frac{1}{2} L_0 (t - s_1)^2]_{s_0}^{s_1}  + [s \underline f(s_{N_n}) - \frac{1}{2} L_{N_n} (t - s_{N_n})^2]_{s_{N_n}}^{s_{{N_n}+1}}  + s_{N_n} \underline f(t_{N_n}) - s_1 \underline f(s_1)+  \sum_{i=1}^{{N_n}-1} \Bigl(\xi^\boden_{i} \bigl( \underline f(s_i) - \underline f(s_{i+1})\bigr) - \frac{L_i}{2} \bigl( (\xi^\boden_{i}-s_i )^2 + (\xi^\boden_{i} -s_{i+1})^2 \bigr) 
 %\Bigr) \\
%%
  %= s_{{N_n}+1} \underline f(s_{N_n})-s_0 \underline f(s_1) - \frac{1}{2} L_0 (s_0 - s_1)^2  - \frac{1}{2} L_{N_n} (s_{{N_n}+1} - s_{N_n})^2 +  \sum_{i=1}^{{N_n}-1} \Bigl(\xi^\boden_{i} \bigl( \underline f(s_i) - \underline f(s_{i+1})\bigr) - \frac{L_i}{2} \bigl( (\xi^\boden_{i}-s_i )^2 + (\xi^\boden_{i} -s_{i+1})^2 \bigr) 
 %\Bigr) 
%$
 %
 %
 %
%
%\end{proof}
%
%\end{thm}

Note, the definite integrals only require the existing function samples on our grid $G_{N_n}$. 

\subsubsection{Batch quadrature algorithm}
We are now in a position to turn our preparatory derivations into an algorithm implementing a batch quadrature rule. 
The algorithm is provided in 
%\IncMargin{-2em}
\begin{algorithm} 
\label{alg:batchhoelderquad1}
\begin{small}
%\SetKwData{flag}{flag}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%
\Input{H\"older coefficients $L_1,\ldots$, and exponent $p$,00.
erroneous sample $D_n= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N_n \} $.}
\Output{Integral estimate lower and upper bounds $S^\boden_n, S^\decke_n $}
\BlankLine
%\emph{special treatment of the first line}\;
%$\flag \leftarrow 0$;\\
1: // \texttt{Solve for breakpoints: } \\
2: $ (\lambda_1^\decke,...,\lambda_{{N_n}-1}^\decke) \leftarrow \argmin_{(\lambda_1,...,\lambda_{{N_n}-1})} \mathfrak S^\decke_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr)$\\
%3: 
%$ (\lambda_1^\boden,...,\lambda_{{N_n}-1}^\boden) \leftarrow \argmax_{(\lambda_1,...,\lambda_{{N_n}-1})} \mathfrak S^\boden_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr)$

3: 
\ForEach {$i \in \{1,\ldots,N_n-1 \}$}{ 4: $\xi_i^\decke \leftarrow s_{i} + \lambda_i^\decke (s_{i+1}-s_{i})$ ;\\
5: $\xi_i^\boden \leftarrow s_{i} + (1-\lambda_i^\decke) (s_{i+1}-s_{i})$}

5:  \texttt{// Compute integral bounds as per Thm. \ref{thm:ceilfloorintofxi}:}\\
6: $S^\decke_n \leftarrow \sum_{i=1}^{N_n}  \tilde f(s_i) (\xi_{i}^\decke - \xi_{i-1}^\decke) +  (\xi_{i}^\decke - \xi_{i-1}^\decke)\, \varepsilon_i \,+ \frac{L_i}{{p+1}} (\xi_{i}^\decke-s_i )^{p+1}+  \frac{L_{i-1}}{{p+1}}(s_i-\xi_{i-1}^\decke)^{p+1} $\\	 
7: $S^\boden_n \leftarrow \sum_{i=1}^{N_n}  \tilde f(s_i) (\xi_{i}^\boden - \xi_{i-1}^\boden) - (\xi_i^\boden - \xi_{i-1}^\boden)\, \varepsilon_i \,- \frac{L_i}{{p+1}} (\xi_i^\boden-s_i )^{p+1} - \frac{L_{i-1}}{{p+1}}(s_i-\xi_{i-1}^\boden)^{p+1}   $.
\BlankLine
\caption{Batch algorithm yielding a lower and upper bound $S^\decke_n, S^\boden_n $ of the integral to be estimated as per $S^\decke_n \geq \int_I f(x) \d x \geq S^\boden_n $. A point estimate $\hat S_n$ could for instance be obtained as per $\hat S_n := \frac{S^\decke_n + S^\boden_n}{2} $ with error bound $\hat E_n = \frac{S^\decke_n - S^\boden_n}{2}$.}

\end{small}
\end{algorithm}

The statement of the algorithm is fairly general. As stated previously, for special cases the breakpoints $\xi^\decke, \xi^\boden$ can be calculated in closed form (e.g. as per Eq. \ref{eq:lipxifloor} and Eq. \ref{eq:lipxiceil} for the case $p=1$) and directly inserted in lines $5$ and $6$. In all other cases, we have already described how the $\lambda_i^\decke, \lambda_i^\boden$ can be calculated by solving Eq. \ref{eq:lambdaceil} and Eq. \ref{eq:lambdafloor}, respectively. If required, root-finding methods can be employed to solve these equations numerically. For convenience, this approach is epitomised in Alg. \ref{alg:numsolve4lambdahoelderquad}.

%\IncMargin{-2em}
\begin{algorithm} \label{alg:numsolve4lambdahoelderquad}
\begin{small}
%\SetKwData{flag}{flag}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%
\Input{H\"older coefficients $L_i$, and exponent $p$. 

erroneous sample $D_n= \{\bigl( s_i, \tilde f_i, \varepsilon(s_i) \bigr) \vert i=1,\ldots, N_n \} $.}
\Output{Integral estimate lower and upper bounds $S^\boden_n, S^\decke_n $}
\BlankLine
%\emph{special treatment of the first line}\;
%$\flag \leftarrow 0$;\\
1: // \texttt{Solve for breakpoints: } \\
2: $ (\lambda_1^\decke,...,\lambda_{{N_n}-1}^\decke) \leftarrow \argmin_{(\lambda_1,...,\lambda_{{N_n}-1})} \mathfrak S^\decke_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr)$\\
3: 
$ (\lambda_1^\boden,...,\lambda_{{N_n}-1}^\boden) \leftarrow \argmax_{(\lambda_1,...,\lambda_{{N_n}-1})} \mathfrak S^\boden_n\bigl(\lambda_1,...,\lambda_{{N_n}-1}\bigr)$

4: 
\ForEach {$i \in \{1,\ldots,N_n-1 \}$}{ $\xi_i^\decke \leftarrow s_{i} + \lambda_i^\decke (s_{i+1}-s_{i})$ ;
$\xi_i^\boden \leftarrow s_{i} + \lambda_i^\boden (s_{i+1}-s_{i})$}

5:  \texttt{// Compute integral bounds as per Thm. \ref{thm:ceilfloorintofxi}:}\\
6: $S^\decke_n \leftarrow \sum_{i=1}^{N_n}  \tilde f(s_i) (\xi_{i}^\decke - \xi_{i-1}^\decke) +  (\xi_{i}^\decke - \xi_{i-1}^\decke)\, \varepsilon_i \,+ \frac{L_i}{{p+1}} (\xi_{i}^\decke-s_i )^{p+1}+  \frac{L_{i-1}}{{p+1}}(s_i-\xi_{i-1}^\decke)^{p+1} $\\	 
7: $S^\boden_n \leftarrow \sum_{i=1}^{N_n}  \tilde f(s_i) (\xi_{i}^\boden - \xi_{i-1}^\boden) - (\xi_i^\boden - \xi_{i-1}^\boden)\, \varepsilon_i \,- \frac{L_i}{{p+1}} (\xi_i^\boden-s_i )^{p+1} - \frac{L_{i-1}}{{p+1}}(s_i-\xi_{i-1}^\boden)^{p+1}   $.
\BlankLine
\caption{Batch algorithm yielding a lower and upper bound $S^\decke_n, s^\boden_n $ of the integral to be estimated as per $\decke_n \geq \int_I f(x) \d x \geq \boden_n $. A point estimate $\hat S_n$ could for instance be obtained as per $\hat S_n := \frac{S^\decke_n + S^\boden_n}{2} $ with error bound $\hat E_n = \frac{S^\decke_n - S^\boden_n}{2}$.}


\end{small}
\end{algorithm}


\subsubsection{Adaptive quadrature and error convergence -- open} Next, we will investigate . That is, we want to establish convergence of our integrals' estimates to the true definite integral. To this end, we note that $S^\decke_n - S^\boden_n$ quantifies the error or magnitude of our uncertainty about the true integral $S$. 

\begin{thm}
\begin{align*}
		E_n := S^\decke_n - S^\boden_n 
& ...\\
\end{align*}
Furthermore, we have $\lim_{{N_n} \to \infty} S^\decke_n - S^\boden_n =0$, if grid $G_{N_n} \stackrel{{N_n} \to \infty}{\to} G$, where $G$ is dense in domain interval $I$. 

\begin{proof}

Let $e_i = \varepsilon(s_{i+1}) - \varepsilon(s_{i})$ and $d_i = \tilde f(s_{i+1}) - \tilde f(s_i)$.
Note, $\underline f(s_{i+1}) - \underline f(s_i) = d_i - e_i$ and $\overline f(s_{i+1}) - \overline f(s_i) = d_i + e_i$. Furthermore, we define $Q_i := \frac{s_i -s_{i+1}}{2}, P_i:= \frac{d_i + \varepsilon_i}{2 L_i}$ and $M_i := \frac{d_i - \varepsilon_i}{2 L_i}$.
With these definitions, we have \\
$(i)\, \xi^\decke_i - s_i = - Q_i + P_i $\\
%
$(ii) \,\xi^\decke_i - s_{i+1} =  Q_i + P_i $\\
%
$(iii) \,\xi^\boden_i - s_{i} =  -Q_i - M_i $\\
%
$(iv) \, \xi^\boden_i - s_{i+1} =  Q_i - M_i $.

We have:
\begin{align*}
S^\decke_n  - S^\boden_n =& s_{{N_n}+1} (\overline f(s_{N_n}) - \underline f(s_{N_n})) + s_0 ( \underline f(s_1) -  \overline f(s_1))\\ \\ 
&+  L_0 (s_0 - s_1)^2  + L_{N_n} (s_{{N_n}+1} - s_{N_n})^2\\
		 &+\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( \overline f(s_i) - \overline f(s_{i+1}) \bigr) - \xi^\boden_{i} \bigl( \underline f(s_i) - \underline f(s_{i+1})\bigr) \\
		&+ \sum_{i=1}^{{N_n}-1} \frac{L_i}{2} \bigl( (\xi^\decke_{i}-s_i )^2+ (\xi^\decke_{i} -s_{i+1})^2 \bigr) + \frac{L_i}{2} \bigl( (\xi^\boden_{i}-s_i )^2 + (\xi^\boden_{i} -s_{i+1})^2 \bigr) \\
		%
		\stackrel{\text{ }}{=} 
& s_{{N_n}+1} 2 \varepsilon_{N_n} - s_0 2 \varepsilon_1 +  L_0 (s_0 - s_1)^2  + L_{N_n} (s_{{N_n}+1} - s_{N_n})^2\\
		 &-\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( d_i+ e_i \bigr) + \xi^\boden_{i} \bigl(  d_i-e_i \bigr) \\
		&+ \sum_{i=1}^{{N_n}-1} \frac{L_i}{2} \Bigl( (\xi^\decke_{i}-s_i )^2+ (\xi^\decke_{i} -s_{i+1})^2  +  (\xi^\boden_{i}-s_i )^2 + (\xi^\boden_{i} -s_{i+1})^2 \Bigr) \\
\end{align*}
%
\begin{align*}
		\stackrel{\text{(i)-(iv) }}{=} 
& s_{{N_n}+1} 2 \varepsilon_{N_n} - s_0 2 \varepsilon_1 +  L_0 (s_0 - s_1)^2  + L_{N_n} (s_{{N_n}+1} - s_{N_n})^2\\
		 &-\sum_{i=1}^{{N_n}-1} \xi^\decke_{i} \bigl( d_i+ e_i \bigr) + \xi^\boden_{i} \bigl(  d_i-e_i \bigr) \\
		&+  \sum_{i=1}^{{N_n}-1} \frac{L_i}{2} \Bigl( (-Q_i+P_i)^2+ (Q_i+P_i)^2  +  (-Q_i - M_i)^2 + (Q_i - M_i)^2 \Bigr) \\
\end{align*}
%
\begin{align*}
		\stackrel{ }{=} 
& s_{{N_n}+1} 2 \varepsilon_{N_n} - s_0 2 \varepsilon_1 +  L_0 (s_0 - s_1)^2  + L_{N_n} (s_{{N_n}+1} - s_{N_n})^2\\
		&+  \sum_{i=1}^{{N_n}-1} L_i \Bigl( 2 Q_i^2+  P_i^2  +   M_i^2 \Bigr) 
		-\sum_{i=1}^{{N_n}-1} (\xi^\decke_{i} - \xi^\boden_i ) e_i  + (\xi^\boden_{i}+ \xi^\decke_i) d_i
		\\
\end{align*}
%
It can be easily verified that $2 Q_i^2 = \frac{(s_i - s_{i+1})^2}{2}$ and $M_i^2 + P_i^2 = \frac{d_i^2 + e_i^2}{2 L_i^2}$, as well as 
$\xi^\decke_i + \xi^\boden_i = (s_i + s_{i+1}) + \frac{e_i}{L_i}$ and $\xi^\decke_i - \xi^\boden_i = \frac{d_i}{L_i}$.

Substituting these relations into the equation and some simplifying arithmetics yield:
\begin{align*}
		E_n = S^\decke_n - S^\boden_n 
& =s_{{N_n}+1} 2 \varepsilon_{N_n} - s_0 2 \varepsilon_1 +  L_0 (s_0 - s_1)^2  + L_{N_n} (s_{{N_n}+1} - s_{N_n})^2\\
		&+  \sum_{i=1}^{{N_n}-1} L_i \frac{(s_i - s_{i+1})^2}{2} +  \frac{d_i^2 + e_i^2}{2 L_i} \\
		&-\sum_{i=1}^{{N_n}-1} \frac{d_i}{L_i} e_i  + d_i (s_i + s_{i+1}) + d_i \frac{e_i}{L_i} 
		\\
\end{align*}

Resubstitution of the definitions of $e_i$ and $d_i$ yields the desired result.
\end{proof}
\end{thm}

\begin{thm}
\[E_n := S^\decke_n - S^\boden_n = \frac{1}{2} \sum_{i=1}^{{N_n}-1} L_i (s_{i+1} -s_i)^2 - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i} \geq 0.\] 
Furthermore, we have $\lim_{{N_n} \to \infty} S^\decke_n - S^\boden_n =0$, if grid $G_{N_n} \stackrel{{N_n} \to \infty}{\to} G$, where $G$ is dense in domain interval $I$. 

\begin{proof}


Referring to Thm. \ref{thm:quad_ceiling} and Thm. \ref{thm:quad_ceiling}, using the definitions of the $\xi^\decke_i$ and $\xi^\boden_i$, as well as a bit of algebraic manipulation, yields the desired equality 
$S^\decke_n - S^\boden_n = \frac{1}{2} \sum_{i=1}^{{N_n}-1} L_i (s_{i+1} -s_i)^2 - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i}$. 

For each $i$ we have can make the following argument:
Due to H\"older continuity, we have  
$\frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i^2}  \leq (s_{i+1}-s_i)^{2p}$.

Hence,
$a_{N_n}^i:=L_i (s_{i+1} -s_i)^{2p} - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i}$

$=L_i [(s_{i+1} -s_i)^{2p} - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i^2}]$.

$\geq L_i [(s_{i+1} -s_i)^2 - (s_{i+1} -s_i)^2] =0$.
Thus, $S^\decke_n - S^\boden_n = \sum_i a_{N_n}^i \geq 0$. \\

Finally, we prove vanishing error in the limit of a dense grid. 
Let $(G_{N_n})$ a sequence of grids converging to a grid $G$ that is dense in $I$. By Thm. \ref{thm:enclosure1d_desiderata}, we know that $\lim_{{N_n} \to \infty} \decke_n = \lim_{{N_n} \to \infty}
    \boden_n = f$ \textit{uniformly}. Due to uniform convergence, we can exchange integral and limites. That is, we have 

$0 = \int_I f(t) \, \d t - \int_I f(t) \, \d t$
$=  \int_I \lim_{{N_n} \to \infty} \decke_n(t) \, \d t  - \int_I \lim_{{N_n} \to \infty}  \boden_n (t) \, \d t$
$\stackrel{unif. conv.}{=} \lim_{{N_n} \to \infty} \int_I \decke_n(t) \, \d t  - \lim_{{N_n} \to \infty} \int_I \boden_n (t) \, \d t$    
$=\lim_{{N_n} \to \infty} S^\decke_n - S^\boden_n $.






\end{proof}

\end{thm}

\begin{thm}
\[E_n := S^\decke_n - S^\boden_n = \frac{1}{2} \sum_{i=1}^{{N_n}-1} L_i (s_{i+1} -s_i)^2 - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i} \geq 0.\] 
Furthermore, we have $\lim_{{N_n} \to \infty} S^\decke_n - S^\boden_n =0$, if grid $G_{N_n} \stackrel{{N_n} \to \infty}{\to} G$, where $G$ is dense in domain interval $I$. 

\begin{proof}
Referring to Thm. \ref{thm:quad_ceiling} and Thm. \ref{thm:quad_ceiling}, using the definitions of the $\xi^\decke_i$ and $\xi^\boden_i$, as well as a bit of algebraic manipulation, yields the desired equality 
$S^\decke_n - S^\boden_n = \frac{1}{2} \sum_{i=1}^{{N_n}-1} L_i (s_{i+1} -s_i)^2 - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i}$. 

For each $i$ we have can make the following argument:
Due to H\"older continuity, we have  
$\frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i^2}  \leq (s_{i+1}-s_i)^2$.

Hence,
$a_{N_n}^i:=L_i (s_{i+1} -s_i)^2 - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i}$

$=L_i [(s_{i+1} -s_i)^2 - \frac{\bigl(f(s_{i+1}) -f(s_i)\bigr)^2}{L_i^2}]$.

$\geq L_i [(s_{i+1} -s_i)^2 - (s_{i+1} -s_i)^2] =0$.
Thus, $S^\decke_n - S^\boden_n = \sum_i a_{N_n}^i \geq 0$. \\

Finally, we prove vanishing error in the limit of a dense grid. 
Let $(G_{N_n})$ a sequence of grids converging to a grid $G$ that is dense in $I$. By Thm. \ref{thm:enclosure1d_desiderata}, we know that $\lim_{{N_n} \to \infty} \decke_n = \lim_{{N_n} \to \infty}
    \boden_n = f$ \textit{uniformly}. Due to uniform convergence, we can exchange integral and limites. That is, we have 

$0 = \int_I f(t) \, \d t - \int_I f(t) \, \d t$
$=  \int_I \lim_{{N_n} \to \infty} \decke_n(t) \, \d t  - \int_I \lim_{{N_n} \to \infty}  \boden_n (t) \, \d t$
$\stackrel{unif. conv.}{=} \lim_{{N_n} \to \infty} \int_I \decke_n(t) \, \d t  - \lim_{{N_n} \to \infty} \int_I \boden_n (t) \, \d t$    
$=\lim_{{N_n} \to \infty} S^\decke_n - S^\boden_n $.






\end{proof}

\end{thm}

We see from the expression that the error is larger for function samples whose values do not differ much. 


%Thus, $a^i_{N_n} = \abs{a^i_{N_n}}$.
%
%Hence,  sequence $(q_{N_n})_{{N_n} \in \nat}$, $q_{N_n} := S^\decke_n - S^\boden_n = \frac{1}{2} \sum_{i=1}^{{N_n}-1} a_{N_n}^i$ is convergent, iff the series is absolutely convergent.
%
%
%Let $s_{N_n} := \max_i a^i_{N_n} = \max_i \abs{a_{N_n}^i}.$ We show $q_{N_n} \to 0$ by showing $({N_n}-1) s_{N_n} \to 0$ (as ${N_n} \to \infty$).



==> content2/Ch_kinkyinf/quad_shubertstyle.tex <==
\section{Conservative quadrature}

Let $a,b \in \Real, a \leq b, I := [a,b] \subset \Real$.
Given a Lipschitz function $f: I \to \Real $ we aim to compute conservative estimates of the definitive Riemann integral \[S := \int_{I} f(t) \, \d t.\] (Remark: PERHAPS CAN LIFT RIEMANN ASSUMPTION BY
AUGMENTING INTERVAL MEASURE ACCORDING TO AN ALTERNATIVE MEASURE).
In particular, given a finite budget of $N \in \nat$ function evaluations, we desire (i) to find two  estimates $S^\decke_N , S^\boden_N$ of the definite integral that are upper and lower conservative, respectively. That is, we desire 
\[S^\boden_N \leq S \leq S^\decke_N. \] Furthermore, we desire (ii) convergence to the true value in the limit of an infinite number of function evaluations. That is, we require
$S^\boden_N, S^\decke_N \stackrel{N \to \infty}{\longrightarrow} S $.
Finally, we desire (iii) $S^\decke_N,S^\boden_N$ to be closed-form. 

In the one-dimensional case, one obvious way to achieve this is to use the integrals of the Lipschitz ceiling and floor. That is, we define $S^\decke_N := \int_I \decke_N (t) \,dt $ and $S^\boden_N := \int_I \boden_N (t) \,dt $. 

(i) follows directly from the properties of the enclosing functions established by Thm. \ref{thm:enclosure1d_desiderata}.

 (iii) is easily addressed via noticing that both ceiling and floor functions are piece-wise linear functions. Hence, their definite integrals can be determined exactly in closed-form. In particular, the definite integral of the ceiling can be determined as follows:

\begin{thm} \label{thm:quad_floor} As in Sec.\ref{sec:enclosures}, let  $\xi^{\decke}_i =  \frac{t_i+t_{i+1}}{2}+ \frac{f(t_{i+1}) - f(t_i)}{2 L_i}  $. Let $S^\decke_N = \int_I \decke_N (t) \, \d t$ denote the definite integral of the Lipschitz ceiling.
%augmented grid $\tilde G_N = (t_1, \xi_1^\decke, t_2, \xi_2^\decke, t_3,\ldots,t_{N-1},\xi_{N-1}^\decke,t_{N} )$, and let $\tau_j$ denote the $j$th element 
%of augmented grid $\tilde G_N$.
We have 
$S^\decke_N=t_N f(t_N) - t_1 f(t_1)+\sum_{i=1}^{N-1} \xi^\decke_{i} \bigl( f(t_i) - f(t_{i+1}) \bigr) + \frac{L_i}{2} \bigl( (\xi^\decke_{i}-t_i )^2+ (\xi^\decke_{i} -t_{i+1})^2 \bigr) $. 


%\[ S^\decke_N  = \frac{1}{2} \sum_{i=1}^{3N-1} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\decke_N^i(\xi^{\decke}_i)(
%\tau_{i+1}) - \decke_N^i(\xi^{\decke}_i)(
%\tau_{i})\bigr), \, (N > 1);\]
%
%\[ S^\decke_N  = \frac{1}{2} \sum_{i=1}^{3N} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\decke_N^i(\xi^{\decke}_i)(
%\tau_{i+1}) - \decke_N^i(\xi^{\decke}_i)(
%\tau_{i})\bigr), \, (N = 1).\]

\begin{proof} With 
$\alpha^\decke_i: x \mapsto f(a_i) + L_i (x - a_i)$ and $\beta^\decke_i: x \mapsto
f(b_i) -L_i (x - b_i)$ the Lipschitz ceiling is the piecewise-linear function $\decke^i_N: t \mapsto \min\{ \alpha^\decke_i(t), \beta^\decke_i(t)$. As pointed out before, for all $t \in J_i$, we have $\decke_N^i(t) = 
 \begin{cases}  
 f(a_i) + L_i (t - a_i), & t \leq \xi^\decke_i \\
 f(b_i) -L_i (t - b_i), & t > \xi^\decke_i 
 \end{cases}$.

Therefore,
$S^\decke_N = \int_I \decke_N (t) \, \d t$
 
 $= \sum_{i=1}^{N-1} \int_{J_i} \decke_N^i (t) \, \d t$
 
 $= \sum_{i=1}^{N-1} \int_{t_i}^{t_{i+1}} \decke_N^i (t) \, \d t$
  
  $= \sum_{i=1}^{N-1} \bigl( \int_{t_i}^{\xi^\decke_{i}}  f(t_i) + L_i (t - t_i) \, \d t + \int_{\xi^\decke_{i}}^{t_{i+1}}   f(t_{i+1}) -L_i (t - t_{i+1})\, \d t \bigr)$
  
  $= \sum_{i=1}^{N-1} \bigl( \bigl[t f(t_i) + \frac{L_i (t-t_i )^2}{2}\bigr]_{t_i}^{\xi^\decke_{i}}  + \bigl[t f(t_{i+1}) - \frac{L_i (t -t_{i+1})^2}{2}\bigr]^{t_{i+1}}_{\xi^\decke_{i}} \bigr)$
  
  $= \sum_{i=1}^{N-1} \Bigl( \xi^\decke_{i} f(t_i) + \frac{L_i (\xi^\decke_{i}-t_i )^2}{2} - t_i f(t_i)   
  - \xi^\decke_{i} f(t_{i+1}) + \frac{L_i (\xi^\decke_{i} -t_{i+1})^2}{2}  + t_{i+1} f(t_{i+1}) \Bigr)$
  
    $=  t_N f(t_N) - t_1 f(t_1)+\sum_{i=1}^{N-1} \xi^\decke_{i} \bigl( f(t_i) - f(t_{i+1}) \bigr) + \frac{L_i}{2} \bigl( (\xi^\decke_{i}-t_i )^2+ (\xi^\decke_{i} -t_{i+1})^2 \bigr)      $.
\end{proof}

\end{thm}

Of course, we can obtain the completely analogous statement to the Lipschitz floor. 


\begin{thm} \label{thm:quad_ceiling} As in Sec.\ref{sec:enclosures}, let $\xi^{\mathfrak l}_i := \frac{t_i+t_{i+1}}{2} - \frac{f(t_{i+1}) - f(t_i)}{2 L_i}  $. Let $S^\boden_N = \int_I \boden_N (t) \, \d t$ denote the definite integral of the Lipschitz ceiling.
%augmented grid $\tilde G_N = (t_1, \xi_1^\boden, t_2, \xi_2^\boden, t_3,\ldots,t_{N-1},\xi_{N-1}^\boden,t_{N} )$, and let $\tau_j$ denote the $j$th element 
%of augmented grid $\tilde G_N$.
We have 
$S^\boden_N=t_N f(t_N) - t_1 f(t_1)+  \sum_{i=1}^{N-1} \Bigl(\xi^\boden_{i} \bigl( f(t_i) - f(t_{i+1})\bigr) - \frac{L_i}{2} \bigl( (\xi^\boden_{i}-t_i )^2 + (\xi^\boden_{i} -t_{i+1})^2 \bigr) 
 \Bigr) $. 


%\[ S^\boden_N  = \frac{1}{2} \sum_{i=1}^{3N-1} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\boden_N^i(\xi^{\boden}_i)(
%\tau_{i+1}) - \boden_N^i(\xi^{\boden}_i)(
%\tau_{i})\bigr), \, (N > 1);\]
%
%\[ S^\boden_N  = \frac{1}{2} \sum_{i=1}^{3N} \bigl(\,(\tau_{i+1} - \tau_i) \,\bigl(\boden_N^i(\xi^{\boden}_i)(
%\tau_{i+1}) - \boden_N^i(\xi^{\boden}_i)(
%\tau_{i})\bigr), \, (N = 1).\]

\begin{proof} As observed in the proof of Lem. \ref{lem:floor_values}, we have 
 $\boden_N^i(t) = 
 \begin{cases}  
 \alpha_i^{\mathfrak l} (t), & t \leq \xi_i^\boden \\
 \beta_i^{\mathfrak l} (t), & t \geq \xi_i^\boden
 \end{cases}$ 
% 
 where $\alpha^\boden_i( t) = f(t_i) - L_i (t - t_i)$ and $\beta^\boden_i( t) =
f(t_{i+1}) +L_i (t - t_{i+1})$.\\

Therefore,
$S^\boden_N = \int_I \boden_N (t) \, \d t$
 
 $= \sum_{i=1}^{N-1} \int_{J_i} \boden_N^i (t) \, \d t$
  $= \sum_{i=1}^{N-1} \int_{t_i}^{t_{i+1}} \boden_N^i (t) \, \d t$
  
  $= \sum_{i=1}^{N-1} \bigl( \int_{t_i}^{\xi^\boden_{i}}  f(t_i) - L_i (t - t_i) \, \d t + \int_{\xi^\boden_{i}}^{t_{i+1}}   f(t_{i+1}) +L_i (t - t_{i+1})\, \d t \bigr)$
  
  $= \sum_{i=1}^{N-1} \bigl( \bigl[t f(t_i) - \frac{L_i (t-t_i )^2}{2}\bigr]_{t_i}^{\xi^\boden_{i}}  + \bigl[t f(t_{i+1}) + \frac{L_i (t -t_{i+1})^2}{2}\bigr]^{t_{i+1}}_{\xi^\boden_{i}} \bigr)$
  
  $= \sum_{i=1}^{N-1} \Bigl( \xi^\boden_{i} f(t_i) - \frac{L_i (\xi^\boden_{i}-t_i )^2}{2} - t_i f(t_i)   
  - \xi^\boden_{i} f(t_{i+1}) - \frac{L_i (\xi^\boden_{i} -t_{i+1})^2}{2}  + t_{i+1} f(t_{i+1}) \Bigr)$
  
    $\stackrel{telescope \sum}{=}  t_N f(t_N) - t_1 f(t_1)+\sum_{i=1}^{N-1} \Bigl(\xi^\boden_{i} f(t_i) - \frac{L_i (\xi^\boden_{i}-t_i )^2}{2}   
  - \xi^\boden_{i} f(t_{i+1}) - \frac{L_i (\xi^\boden_{i} -t_{i+1})^2}{2}  \Bigr) $
  
  $= t_N f(t_N) - t_1 f(t_1)+  \sum_{i=1}^{N-1} \Bigl(\xi^\boden_{i} \bigl( f(t_i) - f(t_{i+1})\bigr) - \frac{L_i}{2} \bigl( (\xi^\boden_{i}-t_i )^2 + (\xi^\boden_{i} -t_{i+1})^2 \bigr) 
 \Bigr)  $
 
% $\stackrel{def. \,\xi^\boden_{i}} { =} t_N f(t_N) - t_1 f(t_1)+  \sum_{i=1}^{N-1} \Bigl([\frac{t_i+t_{i+1}}{2} - \frac{f(t_{i+1}) - f(t_{i})}{2 L_i}] \bigl( f(t_i) - f(t_{i+1})\bigr) - \frac{L_i}{2} \bigl( (\frac{t_i+t_{i+1}}{2} - \frac{f(t_{i+1}) - f(t_{i})}{2 L_i}-t_i )^2 + (\frac{t_i+t_{i+1}}{2} - \frac{f(t_{i+1}) - f(t_{i})}{2 L_i} -t_{i+1})^2 \bigr) 
% \Bigr)  $
% 
%$= t_N f(t_N) - t_1 f(t_1)+  \sum_{i=1}^{N-1} \Bigl( \bigl[ \frac{t_i f(t_i)}{2}+ \frac{t_{i+1} f(t_i)}{2} - \frac{t_{i} f(t_{i+1})}{2}- \frac{t_{i+1} f(t_{i+1})}{2} - \frac{f(t_{i+1}) f(t_i)}{2 L_i} + \frac{f(t_{i+1})^2}{2 L_i} + \frac{f(t_{i})^2}{2 L_i} - \frac{f(t_{i+1}) f(t_i)}{2 L_i}  \bigr] - \frac{L_i}{2} \bigl[ (\frac{t_{i+1} - t_i}{2} - \frac{f(t_{i+1}) - f(t_{i})}{2 L_i})^2 + (\frac{t_{i+1} -t_i}{2} + \frac{f(t_{i+1}) - f(t_{i})}{2 L_i} )^2 \bigr] 
% \Bigr)  $ 
% 
%$\stackrel{regroup}{=} t_N f(t_N) - t_1 f(t_1)+  \sum_{i=1}^{N-1} \Bigl( \bigl[ \frac{t_i f(t_i)}{2}- \frac{t_{i+1} f(t_{i+1})}{2}+ \frac{t_{i+1} f(t_i)}{2} - \frac{t_{i} f(t_{i+1})}{2} - \frac{f(t_{i+1}) f(t_i)}{ L_i} + \frac{f(t_{i+1})^2}{2 L_i} + \frac{f(t_{i})^2}{2 L_i} \bigr] - L_i \bigl[ (\frac{t_{i+1} - t_i}{2})^2 + (\frac{f(t_{i+1}) - f(t_{i})}{2 L_i} )^2 \bigr] 
% \Bigr)  $  
% 
% $\stackrel{telescope \sum}{=} t_N f(t_N) - t_1 f(t_1)+   \frac{t_1 f(t_1)}{2}- \frac{t_{N} f(t_{N})}{2} + \sum_{i=1}^{N-1} \Bigl( \bigl[  \frac{t_{i+1} f(t_i)}{2} - \frac{t_{i} f(t_{i+1})}{2} - \frac{f(t_{i+1}) f(t_i)}{ L_i} + \frac{f(t_{i+1})^2}{2 L_i} + \frac{f(t_{i})^2}{2 L_i} \bigr] - \bigl[\frac{(f(t_{i+1}) - f(t_{i}))^2 }{4 L_i} \bigr] 
% \Bigr)  - \sum_{i=1}^{N-1} L_i (\frac{t_{i+1} - t_i}{2})^2$  \\
%
% ${=} \frac{t_{N} f(t_{N})}{2} - \frac{t_1 f(t_1)}{2}  + \sum_{i=1}^{N-1} \Bigl( \bigl[  \frac{t_{i+1} f(t_i)}{2} - \frac{t_{i} f(t_{i+1})}{2} - \frac{f(t_{i+1}) f(t_i)}{ L_i} + \frac{f(t_{i+1})^2}{2 L_i} + \frac{f(t_{i})^2}{2 L_i} \bigr] - \frac{f(t_{i+1})^2 - 2f(t_{i+1}) f(t_i)+  f(t_{i})^2 }{4 L_i}
% \Bigr)  - \sum_{i=1}^{N-1} L_i (\frac{t_{i+1} - t_i}{2})^2$   
%
% ${=} \frac{t_{N} f(t_{N})}{2} - \frac{t_1 f(t_1)}{2}  + \sum_{i=1}^{N-1} \Bigl( \bigl[  \frac{t_{i+1} f(t_i)}{2} - \frac{t_{i} f(t_{i+1})}{2} - \frac{f(t_{i+1}) f(t_i)}{ 2L_i} + \frac{f(t_{i+1})^2}{4 L_i} + \frac{f(t_{i})^2}{4 L_i} \bigr] 
% \Bigr)  - \sum_{i=1}^{N-1} L_i (\frac{t_{i+1} - t_i}{2})^2$.    
 

\end{proof}

\end{thm}

Note, the definite integrals only require the existing function samples on our grid $G_N$. 

\subsection{Error Analysis and convergence.} Next, we will investigate (ii). That is, we want to establish convergence of our integrals' estimates to the true definite integral. To this end, we note that $S^\decke_N - S^\boden_N$ quantifies the error or magnitude of our uncertainty about the true integral $S$. 

\begin{thm}
\[E_N := S^\decke_N - S^\boden_N = \frac{1}{2} \sum_{i=1}^{N-1} L_i (t_{i+1} -t_i)^2 - \frac{\bigl(f(t_{i+1}) -f(t_i)\bigr)^2}{L_i} \geq 0.\] 
Furthermore, we have $\lim_{N \to \infty} S^\decke_N - S^\boden_N =0$, if grid $G_N \stackrel{N \to \infty}{\to} G$, where $G$ is dense in domain interval $I$. 

\begin{proof}
Referring to Thm. \ref{thm:quad_ceiling} and Thm. \ref{thm:quad_ceiling}, using the definitions of the $\xi^\decke_i$ and $\xi^\boden_i$, as well as a bit of algebraic manipulation, yields the desired equality 
$S^\decke_N - S^\boden_N = \frac{1}{2} \sum_{i=1}^{N-1} L_i (t_{i+1} -t_i)^2 - \frac{\bigl(f(t_{i+1}) -f(t_i)\bigr)^2}{L_i}$. 

For each $i$ we have can make the following argument:
Due to Lipschitz continuity, we have  
$\frac{\bigl(f(t_{i+1}) -f(t_i)\bigr)^2}{L_i^2}  \leq (t_{i+1}-t_i)^2$.

Hence,
$a_N^i:=L_i (t_{i+1} -t_i)^2 - \frac{\bigl(f(t_{i+1}) -f(t_i)\bigr)^2}{L_i}$

$=L_i [(t_{i+1} -t_i)^2 - \frac{\bigl(f(t_{i+1}) -f(t_i)\bigr)^2}{L_i^2}]$.

$\geq L_i [(t_{i+1} -t_i)^2 - (t_{i+1} -t_i)^2] =0$.
Thus, $S^\decke_N - S^\boden_N = \sum_i a_N^i \geq 0$. \\

Finally, prove vanishing error in the limit of a dense grid. 
Let $(G_N)$ a sequence of grids converging to a grid $G$ that is dense in $I$. By Thm. \ref{thm:enclosure1d_desiderata}, we know that $\lim_{N \to \infty} \decke_N = \lim_{N \to \infty}
    \boden_N = f$ \textit{uniformly}. Due to uniform convergence, we can exchange integral and limites. That is, we have 

$0 = \int_I f(t) \, \d t - \int_I f(t) \, \d t$
$=  \int_I \lim_{N \to \infty} \decke_N(t) \, \d t  - \int_I \lim_{N \to \infty}  \boden_N (t) \, \d t$
$\stackrel{unif. conv.}{=} \lim_{N \to \infty} \int_I \decke_N(t) \, \d t  - \lim_{N \to \infty} \int_I \boden_N (t) \, \d t$    
$=\lim_{N \to \infty} S^\decke_N - S^\boden_N $.






\end{proof}

\end{thm}

We see from the expression that the error is larger for function samples whose values do not differ much. 


%Thus, $a^i_N = \abs{a^i_N}$.
%
%Hence,  sequence $(q_N)_{N \in \nat}$, $q_N := S^\decke_N - S^\boden_N = \frac{1}{2} \sum_{i=1}^{N-1} a_N^i$ is convergent, iff the series is absolutely convergent.
%
%
%Let $s_N := \max_i a^i_N = \max_i \abs{a_N^i}.$ We show $q_N \to 0$ by showing $(N-1) s_N \to 0$ (as $N \to \infty$).






==> content2/Ch_kinkyinf/topological_inference.tex <==
\section{A attempt to formalise inference}
An important part of this work pertains to the problem of inference 

To develop a clearer understanding of our design objectives, we need to formalize our understanding of inference in general. On this basis, the specific configurations of our inference problems and our proposed solutions can be discussed in a general, formalized context that links structurally related problems that could be addressed within the same framework as an inference problem. 

Let $(\mathcal D, \mathcal T_{\mathcal D})$, $(\mathcal F, \mathcal T_{\mathcal F})$ and $(\mathcal F', \mathcal T_{\mathcal F'})$ be three topological spaces with topologies of open sets $\mathcal T_{\mathcal D},\mathcal T_{\mathcal F},\mathcal T_{\mathcal F'}$.
We understand the topologies to encode our notions of uncertainty via inclusion. For instance, we understand $A \in \mathcal T_{\mathcal F} $ to be less uncertain than $B \in \mathcal T_{\mathcal F} $ if $A \subset B$.


In our view, an inference problem can, in general terms, be formalized as a tuple $(\mathcal D, \mathcal F, \mathcal F', E,T, )$ where $E: \mathcal T_{\mathcal D} \to \mathcal T_{\mathcal F}$, $T: \mathcal T_{\mathcal F} \to \mathcal T_{\mathcal F'}$ are maps and $\mathcal D$ is a data space representing some notion of environment. As an intuition, you may think of $\mathcal T_{\mathcal F}$ as a codification of what can be known about objects in $\mathcal F$ and $\mathcal T_{\mathcal F'}$ as encoding what can be known about objects in $\mathcal F'$. $T$ states how these things relate. $\mathcal D$ can be understood as a data space.
$E$ could describe how the data gives information about objects in $\mathcal F$. In a well-behaved setting, $E$ would be expected to be monotonous in the sense that $E(D_1) \subset E(D_2)$ if $D_2 \subset D_1$. That is, informally, the more we observe the more we know. 

\textit{A priori knowledge} can be formalized as a subset $\mathcal K_{\text{prior}} $ and \textit{a posteriori} knowledge as a subset $\mathcal K_{\text{post}}\in \mathcal T_{\mathcal F}$. The difference between the two types of knowledge is that the latter has to be extracted (at a ``data extraction cost'' $\gamma_{\text{dat}}$) from the environment via a data extraction mechanism \[M_{\text{dat}}: (\mathcal D,\gamma_{dat}) \mapsto \mathcal K_{\text{post}}.\] 

We define a \textit{topological inference mechanism} as a mapping \[ M_{\text{inf}}: (\mathcal K_{\text{prior}}, \mathcal K_{\text{post}}, \gamma_{\text{inf}}) \mapsto  \mathcal C \in \mathcal T_{\mathcal F'}\] taking an investment of magnitude $\gamma_{\text{inf}}$ (e.g. a computational/energy cost) to transform the given knowledge into a ``conclusion'' $\mathcal C \in \mathcal T_{\mathcal F'}$.

A \textit{data inference mechanism} \[M_{\text{dinf}} : (\mathcal K_{\text{prior}}, D,\gamma_{\text{dinf}}) \mapsto M_{\text{inf}} \bigl(\mathcal K_{\text{prior}},M_{\text{dat}}(D,\gamma_{\text{dat}}),\gamma_{\text{inf}} \bigr)\] couples a data extraction mechanism with an inductive inference mechanism incurring a cost $\gamma_{\text{dinf}} \geq \gamma_{\text{dat}} + \gamma_{\text{inf}}$.

When a distinction between data inference and inference is not required, we will use both notions interchangeably.

\begin{rem}
Of course, normally, we would expect the costs incurred to increase with the size of the data and the cardinality of the underlying topologies. The topologies define the complexity of the search space (search bias). So, an interesting question will be to investigate the dependence of the cost on the chosen spaces. What properties of the topologies are good measures of the degree of challenge a given inference problem poses in terms of cost?
\end{rem}

The inference is called \textit{deductive} if $M_{\text{inf}} (\mathcal K_{\text{prior}},\cdot,\gamma_{\text{inf}})$ is a constant function. Otherwise, it is called \textit{inductive}.

We call a conclusion $\mathcal C$  \textit{conservative} if $T(\mathcal K_{\text{prior}} \cap \mathcal K_{\text{post}}) \subset  \mathcal C$.
By extension, inference mechanism $M_{\text{inf}}$ is conservative if its outputs are conservative conclusions for all inputs.
The inference is \textit{optimal}, if $T(\mathcal K_{\text{prior}} \cap \mathcal K_{\text{post}}) =  \mathcal C$.
Similarily, the data inference mechanism is optimal if $M_{\text{dinf}} (\mathcal K_{\text{prior}}, E(D),\gamma_{\text{dinf}})$ for all data sets $D \in \mathcal T_{\mathcal D}$ and some sufficient investment $\gamma_{\text{dinf}}$.


It may be desirable that an inference mechanisms becomes increasingly certain when an increasing amount of knowledge becomes available. Furthermore, we may not wish that our inference become worse with increasing investment $\gamma$. We can state such a mechanism property as the following \textit{monotonicity} condition:
For $A,B \in \mathcal T_{\mathcal F}$ with $A \subset \mathcal K_{\text{prior}},B \subset \mathcal K_{\text{post}}, \gamma' \geq \gamma$ we have $M_{\text{inf}} (A,B,\gamma') \subset M_{\text{inf}} (\mathcal K_{\text{prior}},\mathcal K_{\text{post}},\gamma)$.

Given prior knowledge $\mathcal K_{\text{prior}}$ and a sequence of data sets $(D_N)_{N \in \nat}$, $D_N\in \mathcal T_{\mathcal D}$, we say the data inference \textit{converges} to \textit{target} $\mathcal C \in \mathcal T_{\mathcal F'}$ if there is a sequence of investments $\gamma_N$ such that the sequence of conclusions $(\mathcal C_N)$, $\mathcal C_N =  M_{\text{dinf}} : (\mathcal K_{\text{prior}}, D_N,\gamma_N) $, converges to $C$ in the topological sense.

After these abstract definitions we will consider a number of concrete examples.
\subsubsection{Examples}
 \begin{ex} [Function estimation] Function estimation is a core component of machine learning. We see that this is a special case of topological inference by choosing $\mathcal F= \mathcal F'$ to be a space of candidate functions endowed with the topology of all enclosures (compact subintervals) $\mathcal T_{\mathcal F'}=\mathcal T_{\mathcal F}= \{ \mathcal E \subset \mathcal F | \exists u,l \in \mathcal F\forall \phi \in \mathcal E\forall x \in I: u(x) \geq \phi(x) \geq l(x) \} $. We can choose $T$ to be the identity map.
\end{ex}

\begin{ex} [Quadrature] \label{ex:topinf_quad} For instance, we choose $\mathcal F = \mathcal L_1(I)$ to be a space of absolutely integrable functions on domain $I$ and endow the space with the discrete topology ($\mathcal T_{\mathcal F}= \textbf{2}^{\mathcal F} $) or the standard topology induced by the $\mathcal L_1(I)$ -norm metric. 
We can choose $\mathcal F' = \Real$ endowed with the standard topology induced by the distance metric $(x,y) \mapsto \abs{x-y}$ and define $T$ element-wise by the linear functional \cite{wernerfunkana} $T: H=\{\phi_i | i\in Q \} \mapsto \{ \int_I \phi_i(x) \, \d x | i \in Q \}$ where $Q$ is an index set arbitrarily chosen to index the elements of $H \in \mathcal T_{\mathcal F}$. 
The data inference method then is a numerical quadrature algorithm that estimates a target function's integral based on a finite sample. 

By contrast, a large class of quadrature methods provide an error interval of the their estimate. Here, $\mathcal F' = \Real, \mathcal T_{\mathcal F'} := \{ [\underline S, \overline S] | \underline S, \overline S \in \Real, \underline S\leq \overline S \}$. The estimate is found on the basis of a finite data set $D_N= \{ \bigl(s_i,f(s_i)\bigr) | s_i < s_{i+1}, s_{i+1}-s_{i} =: h, i=1,...,N \}$ of an equi-spaced samples of integrand $f \in \mathcal F$ and some additional prior knowledge.
For instance, knowing the target function is twice continuously-differentiable and has a maximum second derivative of $m$ translates to prior knowledge set 
$\mathcal K_{prior}(I) = \{f \in C^2(I) |\max_{t \in I} \abs{  f'' (t)} =m  \}$. Based on this knowledge, and with sufficient computational budget $\gamma$, a classic trapezoid rule 
 could output the error interval $M_{\text{dinf}}(\mathcal K_{prior},\mathcal K_{post}, \gamma) = [\hat S_N- \mathfrak E_N, \hat S_N + \mathfrak E_N]$ where integral estimate $\hat S_N = \frac{1}{2} \sum_{i=1}^N \bigl(\,(s_{i+1} - s_i) \,(f(s_{i+1}) - f(s_i)\, \bigr) $ and error bound $\mathfrak E_N = \frac{h^3}{12 N^2} m$.
 It is standard knowledge that under these conditions the trapezoid rule is conservative. That is, the integrals of all functions in the intersection $\mathcal K_{prior}\cap \mathcal K_{post}$ are guaranteed to fall into $[\hat S_N- \mathfrak E_N, \hat S_N + \mathfrak E_N]$ From the definitions, we see that it suffices to invest (computational) inference cost $ \gamma \in \mathcal O(N)$.
\end{ex}

==> content2/Ch_kinkyinf/uncertainLipconst.tex <==
\section{Uncertain Lipschitz constants}
Throughout the previous section we have assumed that the Lipschitz constants were known to us. 
However, in many cases, we may be uncertain about the best Lipschitz constant. We assume the uncertainty is expressed as a distribution. Adopting an epistemological point of view, we interpret probability densities over events as degrees of beliefs that these events hold true (see Jaynes Book for a discussion). 
In the following subsection, we describe how to utilize the densities over the best Lipschitz constant $L* \in \Real_+$ to yield a (once again, conservative) bound on the probability of our functions estimates and integrands not being conservative. After that, the subsequent subsection will be devoted to the question of how to update our beliefs over $L*$ in the light of new function evaluations.

\subsection{Conservative bounds with uncertain Lipschitz constants}

Let $p: \Real_+ \to \Real_+$ be a density encoding our belief over best Lipschitz constant $L^*$ of target function $f$.
Assume we construct a Lipschitz enclosure $\einschluss (\ell)$ based on choosing $\ell \in \Real_+$ as a Lipschitz constant.  How large do we need to choose $\ell$ to guarantee that $f$ is completely contained in the enclosure ? Since we are uncertain about the true Lipschitz constant, this question can only be framed probabilistically. That is, for a given certainty threshold  $\theta \in (0,1)$ we desire to find $\ell > 0$ such that 
\[ \theta \leq \Pr[ f \in \einschluss (\ell) ]. \]  

\begin{thm}
Let $P: t \mapsto \int_{x \leq t} p(x) \,dx $ our density's cumulative distribution function (cdf).
We have, \[P(\ell) \geq \theta \Rightarrow \theta \leq \Pr[ f \in \einschluss (\ell) ].  \] 
\begin{proof} 
Note, as proven above $\forall \ell \geq L :   \Pr[ f \in \einschluss (\ell) | L^*=L] = 1$. 

Hence,
$
\Pr\bigl[ f \in \einschluss (\ell) \bigr] 
= \int_0^\ell \Pr\bigl[ f \in \einschluss (\ell) | L^*=L\bigr] \,dP(L) 
 + \int_\ell^\infty \Pr\bigl[ f \in \einschluss (\ell) | L^*=L\bigr] \,dP(L) 
=  \int_0^\ell \,dP(L) + \int_\ell^\infty \Pr\bigl[ f \in \einschluss (\ell) | L^*=L\bigr] \,dP(L) \\ 
\geq \int_0^\ell \,dP(L) 
= P(\ell).$

\end{proof}
\end{thm}

That is to say, in order to guarantee conservativeness of our enclosure, all we need to do is to compute it on the basis of 
a fixed Lipschitz constant that is just large enough such that $P(\ell) = \int_0^l p(L) \,dL \geq \theta$. Notice, if the integral cannot easily be determined in closed-form, but a Lipschitz constant for $p$ is known, we can employ our method described previously (based on a known constant), to evaluate $P(\ell)$ conservatively. 

\begin{cor}
Let $S := \int_I f(t) \, \d t$. 
With the definitions introduced above, we have  \[P(\ell) \geq \theta \Rightarrow \theta \leq \Pr\Bigl[ \hat S^\decke_N \geq S \geq \hat S^\boden_N  \Bigr]  \] 
where $\hat S^\decke_N , \hat S^\boden_N $ where computed assuming a Lipschitz constant of $\ell$.

\end{cor}

\subsection{Learning a posterior over the Lipschitz constant from data}

Assume we hold a prior belief over the best Lipschitz constant $L^*$ encoded as a density $p_0 : I \subset \Real_+ \to [0,1]$.
Assume we are given a sample $G = \{x_i,y_i\}_{i=1,...,N}$ of input-function value pairs, $x_i \in \mathcal X$, $y_i = f(x_i) \in \outspace, \forall i$, the question arises of to calculate a posterior in the light of the new data. 

Since we assume $f :\mathcal X \to \mathcal Y$ is Lipschitz we have $ \frac{d_\outspace(y_i,y_j)}{d_{\inspace}(x_i,x_j)} \leq L^*,  (i,j =1,...,N, x_i \neq x_j)$ where $L^*$ is the best Lipschitz number. So, our observations allow us to infer that $L_D := \max_{i,j,i\neq j} \frac{d_\outspace(y_i,y_j)}{d_{\inspace}(x_i,x_j)} $ as a lower bound on the best Lipschitz number. 
The remaining question is how to derive a posterior over $L^*$ based on this newly observed lower bound. 

\begin{ques}
How can we prove that there is no information about the Lipschitz constant in the data other than $L_D$? That is, in particular, that \[p(L^*|D) \stackrel{!}{=}p(L^* |L_D) ??\]
\end{ques}


We will discuss two approaches, the Minimum-Relative-Entropy approach and Bayesian inference.

\subsubsection{Minimum-Relative-Entropy Approach} 

Computing posteriors from priors subject to constraints is the focus of max-ent inference. 

Remember, 
\begin{defn}[Relative Entropy] For two densities $p,q: I  \to [0,1]$ the \textit{relative entropy} or \textit{Kullback-Leibler divergence} is defined as 
\[\KLD {p}{q} = \int_{I} p(x) \log \frac{p(x)}{q(x)} d\mu(x)\] where $\mu$ is a measure appropriate for domain $I$.
\end{defn}

For example, if $I \subset \Real$ then $\mu$ is normally tacitly assumed to be the standard Lebesgue measure. If $I$ is a discrete set, $\mu$ is noramlly assumed to be the counting measure. In this case \[\KLD {p}{q} = \sum_{x\in I} p(x) \log_2 \frac{p(x)}{q(x)}. \]

For our problem, we can pose the desired posterior density as the solution to the variational problem:

\begin{align}
\argmin_p & \KLD {p}{p_0}\\
\text{s.t.:}&\\
& p(l) \in [0,1], \forall l \geq 0\\
&\SP{p}{e}_{L_2(\Real)} =1\\
& \SP{p}{\chi_{[0,L_D]}}_{L_2(\Real)} =0
\end{align}

where $e: t \mapsto 1$ is the constant mapping to $1$ and $\chi_{[0,L_D]}$ is the indicator function for interval $[0,L_D]$.

\begin{ques}
Can we solve this variational problem in closed form? How can we solve them numerically. If we have no clue, we can make everything discrete as follows...
\end{ques}

\emph{Discretization}.
For practical purposes, it will be convenient to reduce the problem to a standard convex optimization problem as follows:
Let $J_1,...,J_m \subset I$ be a partition of $I\subset \Real_+$.
Instead of expressing a belief as a density on a continuous interval we may limit our modelling efforts to defining a belief as a discrete distribution function $\pi_0 : \{ 1,...,m\} \to [0,1], i \mapsto \Pr[ L \in J_i]$.  

\begin{rem}
Notice, that this belief encoding may be easier to specify than the density on a continuum of points. 
For instance, assume $I = [a,b] , 0<a<b \in \Real_+ \cup \{\infty\}$ and let $a=t_0<t_1<...<t_m =b$ such that $J_i = [t_{i-1},t_i], (i=1,...,m)$.
Then, knowing the continuous density $p_0$ on $I$ allows us to compute the discrete density via $ \pi_0 (i) = \int_{J_i} p_0(t) \,dt=P_0 (t_i) - P_0(t_{i-1})$. The inverse computation (from discrete to continuous distribution) is not possible without further assumptions.
\end{rem}

We anticipate our discretization to spawn information loss, since we only encode information about the interval not about the relative location of the Lipschitz number within the interval. This will be investigated next.

%Let $\tau \in (0,1]$ denote this relative interval coordinate. That is to say, Lipschitz number $L = t_{i-1}+ \tau (t_i -t_{i-1}) $ is completely given by coordinates $(i,\tau) \in \{1,...,m\} \times (0,1]$ . 
%
%After discretization, our uncertainty about the exact Lipschitz number (not just the interval) is described by $\tilde p_0(L) =  \pi_0(i) \, p_\tau[\tau | i ]$. Assuming that, after discretization, we are completely oblivious about the location within the interval, we have $p_\tau [\tau | i ] = \frac{1}{| (0,1] |} =1$.
%Hence, 
%
%The magnitude of the information loss due to discretziation could be quantified as 
%\begin{align*}
 %H_{\tilde p_0}-H_{ p_0}  &=\int_I p_0(t) \log p_0(t) \, dt  - \bigl(\sum_{i=1}^m \pi_0(i)   \log \pi_0(i) \bigr) \\
%& =  \sum_{i=1}^m \int_{J_i} p_0(t) \log p_0(t) \, dt  \\ 
%&- \bigl(\sum_{i=1}^m \int_{J_i} p_0(t) \,dt  \log \int_{J_i} p_0(t) \,dt \bigr)\\
%% 
%& =  \sum_{i=1}^m \Bigl(\int_{J_i} p_0(t) \log [p_0(t)] \, dt  \\
%&-   \int_{J_i} p_0(t) \,dt  \log [\int_{J_i} p_0(t) \,dt] \Bigr)\\
%& \stackrel{!?}{\leq} 0
%\end{align*}
%
%
%WEIRD !!!  The loss should be greater than 0, not smaller ! 
%Mhh... perhaps I should instead try this (?? Makes any difference??)

In the discretized situation, our ignorance over $L^*$ can be encoded by the density  $\tilde p_0(L) =  \sum_{i=1}^m \pi_0(i) \, p_L [L| i ]$. Assuming that, after discretization, we are completely oblivious about the location within the interval, we have $p_L [L | i ] = \frac{1}{| J_i |} =\frac{1}{| t_i-t_{i-1} |}$.
Hence, $\tilde p_0(L)  =  \sum_{i=1}^m  \frac{\pi_0(i)}{| J_i |} $. 

The magnitude of the information loss due to discretziation could be quantified as 
\begin{align*}
 H_{\tilde p_0}-H_{ p_0}  &=\int_I p_0(L) \log p_0(L) \, dL  - \int_I \tilde p_0(L)    \log  \tilde p_0(L) \, dL \\
& = \int_I p_0(L) \log p_0(L) \, dL  \\
&- \int_I\sum_{i=1}^m \pi_0(i) \, p_L [L| i ]    \log \bigl(\sum_{i=1}^m \pi_0(i) \, p_L [L| i ]\bigr) \, dL \\
& = \int_I p_0(L) \log p_0(L) \, dL  \\
&- \int_I\sum_{i=1}^m \frac{\pi_0(i)}{|J_i|}     \log \bigl(\sum_{i=1}^m \frac{\pi_0(i)}{|J_i|} \bigr) \, dL \\
& = \int_I p_0(L) \log p_0(L) \, dL  \\
&- |I|  \log \bigl(\sum_{i=1}^m \frac{\pi_0(i)}{|J_i|} \bigr) \sum_{i=1}^m \frac{\pi_0(i)}{|J_i|}     \\
& =  \sum_{i=1}^m \Bigl(\int_{J_i} p_0(t) \log [p_0(t)] \, dt \Bigr)   \\
&- |I|  \log \bigl(\sum_{i=1}^m \frac{\int_{J_i} p_0(t) dt}{|J_i|} \bigr) \sum_{i=1}^m \frac{\int_{J_i} p_0(t) dt}{|J_i|}     \\
& \stackrel{!?} {\geq }0
\end{align*}

 
However, the benefit is that (continuous) extremization problem is reduced to a tractable, discrete optimization problem of dimensionality $m$. In fact, it is a convex program with linear constraints:

\begin{align}
\argmin_p & \KLD {\pi}{\pi_0}\\
\text{s.t.:}&\\
& \pi(i) \in [0,1], \forall i \in\{1,...,m\}\\
&\SP{p}{e}_{2} =1\\
& \SP{p}{n_{L_D}}_{2} =0
\end{align}
where $e$ is a vector of $m$ ones and $n_{L_D}$ is suitably defined to mimic a discretized version of the indicator function above and whose $i$th component is defined as follows:

$n_{L_D} (i) = \begin{cases} 1, t_i \geq L_D\\ 0, \text{otherwise.} \end{cases}$ Of course, if $t_{i-1} < L_D < t_i$ for some $i$, we have once again thrown away information,as the constraint $\SP{p}{n_{L_D}}_{2} =0$ does not capture the knowledge that there must be zero probability mass on $K_i' := [t_{i-1},L_D)$ as well. To cover this, we could consider 
introducing an additional component representing the probability on $K_i$  and replace the original meaning of the original $i$th component by representing the probability on  $J_i' = [L_D, t_i] =J_i - K_i$ instead of on $J_i$. In this case, the CP becomes $m+1$-dimensional. Since this is always possible to do, we can assume, without loss of generality, that $L_D $ will always be an element of $t_1,...,t_m$ for some $m$.


Note, an $m$-dimensional CP can be solved in worst-time complexity $\mathcal O(m^3)$ (LOOK IT UP!!).


\begin{rem}
We could investigate how the information loss (which we would expect to grow as a function of $m$) compares to the 
the gain in computational complexity. We should then conceive a common exchange rate / currency / trade-off parameter to 
find a good cut-off point.
\end{rem}

\subsubsection{Bayesian approach}

By Bayes theorem, we can write 
\[p(L|L_D) = \frac{p(L_D|L) \, p_0(L) }{ \int_I p(L_D|L) \, p_0(L) \, \d L}.\]

If we are uncertain about which empirical Lipschitz constant we observe given the real Lipschitz constant  $L^* = L$ we set the Likelihood function 
\[ p(L_D|L) = \begin{cases} 0, L_D > L\\ \frac{1}{L}, otherwise. \end{cases}.\]

Of course, if the definite integrals of prior $p_0$ are not known in closed form, we need to approximate numerically. This is generally unproblematic, as the 
%\begin{ques}[@Mike]
%What is the likelihood function $p(L_D|L)= ... ?$
%\end{ques}

==> content2/LACKI_main.tex <==


\subsection{Lazily Adapted Constant Kinky Inference (LACKI)}
\label{sec:lacki}
Above we explained the benefits of choosing parameter $L(n)$ to coincide with a H\"older constant of the target. As the uncertainty bounds grow with this constant, choosing a small H\"older constant would be ideal. 
However, if such a constant is unavailable a priori, we desire to set $L(n)$ to an estimate of the H\"older constant. 

For notiational convenience, for two sets $S,S' \subset \inspace$ of inputs we define  $$U(S,S') := \{(s,s') \in S \times S' | \metric_\inspace(s,s') >0\} \text{ and  let } U_n := U(G_n,G_n) $$ be the set of all pairs grid inputs deemed disparate under the pseudo-metric $\metric_\inspace$.

The \emph{best} H\"older constant of a function $f$ is the smallest nonnegative number $L^*$ such that $f$ is contained in the set 
$\hoelset L \inspace p = \{\phi: \inspace \to \outspace \, \vert \, \forall x,x' \in \inspace : \metric_\outspace \bigl(\phi(x),\phi(x')\bigr) \leq L \, \bigl( \metric_\inspace (x,x') \bigr)^p\} $ of $L-p$- H\"older continuous functions. So, this best H\"older constant is given by  
%
$$L^* = \sup_{(x,x') \in U(\inspace,\inspace)} \frac{\metric_\outspace \bigl(f(x) - f(x')\bigr)}{\metric_{\inspace}^p(x,x') }.$$




Given the noisy data $\data_n = \{(s_i,\tilde f_i) | i=1,\ldots,N_n\}$ a natural estimate of the best H\"older constant might be to compute $\hat \ell_n^* := \max_{(s,s') \in U_n} \frac{\metric_\outspace(\tilde f(s),\tilde f(s')) }{\metric_{\inspace}^p(s,s')}$ \cite{Strongin1973}. In the absence of \emph{noise} (may it be stochastic or deterministic), that is, if $\tilde f_i = f(s_i),\forall i$, $\hat \ell_n^*$ never overestimates the true best H\"older constant. That is, $\hat \ell_n^* \leq L^*$. However, in the presence of noise $\nu: \inspace \to \outspace$ (such that $\tilde f = f+ \nu$) this boundedness assumption of the estimates no longer holds true. In particular if the noise is not H\"older continuous, we expect $\hat \ell_n^*$ to grow unbounded with increasingly dense data.
For practical reasons and for the sake of our theoretical arguments presented below, we desire the parameters $L(n)$ to remain bounded both. Thus, without further modifications $\hat \ell_n^*$ is not a suitable candidate for $L(n)$.

Therefore, we will modify the estimates to guarantee they are bounded even in the presence of noise. 
To compensate for the effect of the noise, we instead propose the parameterised estimates 
%
\begin{equation}\label{eq:lazyconstupdaterule_batch_main}
\ell(\data_n;\hestthresh,\underline L)  := 
 \max \Bigl\{ \underline L, \max_{(s,s') \in U_n} \frac{\metric_\outspace(\tilde f(s),\tilde f(s')) - \hestthresh}{\metric_{\inspace}^p(s,s')} \Bigr\}.
\end{equation}
%
Here $\underline L$ is a parameter that can be used to specify a priori knowledge of a lower bound on the best Lipschitz constant. In the absence of particular domain-specific knowledge, one can of course always set $\underline L =0$.
\begin{rem}
As shown in Sec. \ref{sec:lazyconstants}, by setting parameter $\hestthresh$ at least as large as twice the maximum level of observational noise ($\hestthresh \geq 2 \metric_{\outspace}(0,\obserr)$) we can guarantee that the $\ell(\data_n;\hestthresh,0)$ are bounded from above by the best H\"older constant. 
\end{rem}
Next, consider an online learning situation, where the available data increases over time. 
That is, $\data_n \subseteq \data_{n+1}$ for all time steps $n \in \nat$. 
For time step $n \in \nat$, let $S_{n+1} := G_{n+1} \backslash G_n$ be the set of new sample inputs.
Similarly to above, we can define an incremental update rule recursively as follows: 
\begin{align} \label{eq:Hoelconstlazyupdateincr_main}
\ell_{n+1} := \max\Bigl\{ & \ell_n, \max_{(s,s') \in U(G_n, S_{n+1})} \frac{\metric_\outspace\bigl(\tilde f(s),\tilde f(s')\bigr) - \hestthresh}{\metric_{\inspace}^p(s,s')},\\
&\max_{(s,s') \in U(S_{n+1}, S_{n+1})} \frac{\metric_\outspace\bigl(\tilde f(s),\tilde f(s')\bigr) - \hestthresh}{\metric_{\inspace}^p(s,s')} \Bigr\},
\end{align} for $n \in \nat$ 
and where 
$\ell_0 := \underline L$. 
The effort for computing $L(n+1)$ is in the order of $\mathcal O\bigl(M (\abs{S_{n+1}} N_n+ \abs{S_{n+1}}^2)\bigr)$ where $M$ denotes the effort for evaluating the pseudo-metrics.
By construction, we have \[\ell_n =\ell(\mathcal \data_n;\hestthresh,\underline L), \forall n \in \nat.\] 
We can show that the sequence $\seq{\ell_n}{n\in \nat}$ of estimates is not only bounded from above by the true H\"older constant $L^*$ but is also growing monotonically and convergent (cf. Lem. \ref{lem:constadaptation_boundedness}).

So far, we have defined a rule of how to update noise-robust and convergent estimates $\ell_n$ of the H\"older constant. Using these data-dependent estimates in place of $L(n)$ in our kinky inference framework as per Def. \ref{def:KIL} yields an inference rule that shall henceforth be referred to as \textit{Lazily Adapted Constant Kinky Inference (LACKI)}.

\begin{defn}[LACKI rule] \label{def:LACKI} For each output component $j \in \{1,\ldots,\text{dim} \, \outspace \}$ 
define $\predfn(\cdot)_{j}$  as per Def. \ref{def:KIL} but assume we choose the parameters $L_j(n) = \ell(\data_n;\hestthresh,\underline L)$ (according to Eq. \ref{eq:lazyconstupdaterule_batch_main}). We refer to the resulting predictor $\predfn\bigl(\cdot \bigr)$ as a \emph{Lazily Adapted Constant Kinky Inference (LACKI)} rule. Here free parameters are $p \in (0,1], \hestthresh \in \Real_{\geq 0}$ and $\underline L \in \Real_{\geq 0}$.  
\end{defn}

To develop a first feel for our inference rule, refer to Fig. \ref{fig:LACKInoise}. Here, we depicted the predictors for an underlying ground-truth function on the basis of a sample but with different parameter choices $\hestthresh$. When setting this parameter to two times the observational noise level, the predictor accurately smoothes out the noise. In contrast, when the parameter is set to zero, the resulting predictor will perfectly interpolate through the noisy observations, thereby limiting the approximation quality to the level of observational noise. 

Furthermore, we notice that the predictors are H\"older continuous but non-differentiable. Informally speaking, the inference exhibits ``kinks'', motivating the term ``kinky inference''.

%Below, we will provide some essential theoretical underpinnings for our method's properties.
\begin{figure}
        \centering
    \includegraphics[width = 8.8cm,height = 4cm]
								{content/figs/LACKIhestthreshvar}
   \caption{Two LACKI inferences over function values of the target $f: x \mapsto \abs{\cos(2\pi x)}+x$ (dashed line) on the basis of a noisy sample (plotted as dots). The predictors are plotted in grey, the noisy observational function $\tilde f (\cdot) = f(x) + \nu_x$ is plotted in cyan. Here the $\nu_x$ were drawn i.i.d. at random from a uniform distribution on the interval $[-0.5,0.5]$. In both cases we chose the parameters $\ubf \equiv \infty,\lbf \equiv -\infty,\underline L = 0$ and $\hexp=1$.
   The left plot shows the LACKI predictor $\predfn$ (grey line) for parameter choice $\hestthresh =0$, falsely assuming absence of observational noise. As a result, the prediction overfitted to the noise. The right plot depicts the prediction $\predfn$ (grey curve) for correct parameter choice $\hestthresh = 2 \obserrbnd =1$, causing the noise to be smoothed out and resulting in more accurate prediction of the underlying ground truth $f$.  }
			\label{fig:LACKInoise}
\end{figure}

\begin{figure}
        \centering
    \includegraphics[width = 8.8cm,height = 4cm]
								{content/figs/LACKIhestthreshvar_with_bounds}
   \caption{Repetition of the experiment but with $p=0.5$. This time, we also plotted floor and ceiling functions (grey dotted and dashed-dotted curves) delimiting the uncertainty bounds. Note, when setting $\lambda =0$ the estimate $\ell(\mathcal \data_n;\hestthresh,\underline L)$ was found to be 128 resulting in extremely conservative uncertainty estimates (left figure). In contrast, choosing $\lambda =2 \obserrbnd $ gave a parameter estimate $\ell(\mathcal \data_n;\hestthresh,\underline L) = 2.4$ yielding sensible uncertainty bounds (right figure). }
			\label{fig:LACKInoise2}
\end{figure}
%
%
%\begin{figure}
%        \centering
%				  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_trueLinit_7tex.pdf}
%    \label{fig:LACKInoise1}
%  } 	
%	 \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_noe_noalpha_smallLinit_7tex.pdf}
%    \label{fig:LACKInoise2}
%  } 	
%  %
%  %\hspace{2cm}
%	  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_smallLinit_7tex.pdf}
%    \label{fig:LACKInoise3}
%  } 
%  				  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_trueLinit_77tex.pdf}
%    \label{fig:LACKInoise4}
%  } 	
%	 \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_noe_noalpha_smallLinit_77tex.pdf}
%    \label{fig:LACKInoise5}
%  } 	
%  %
%  %\hspace{2cm}
%	  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_smallLinit_77tex.pdf}
%    \label{fig:LACKInoise6}
%  } 	
%   \caption{LACKI inference on the basis of two noisy data sets 
%   $\data_1,\data_2$ with varying parameter settings. Target (blue curve) was $f:x \mapsto 5 \sqrt{\abs x}$ and observational model (magenta curve) $\tilde f: x \mapsto f(x) + \phi_x$ where $\phi_x$ is a uniformly distributed disturbance with $\phi_x \stackrel{i.i.d.}{\sim} \mathcal U(-0.5,0.5),\forall x$. 
%  %
%   \textbf{1st column:} Initial constant L(0) = 5; assumed obs. error bound $\obserrpar= 0.5$; $\hestthresh = 2 \obserr=1$. 
%   %
%   \textbf{2nd column:} Initial constant L(0) = 0.01; assumed obs. error bound $\obserrpar = 0$; $\hestthresh = 2 \obserr =0$.
%   %
%   \textbf{3rd column:} Initial constant L(0) = 0.01; assumed obs. error bound $\obserrpar = 0.5$; $\hestthresh = 2 \obserr =1$.
%   %
%   \textbf{Top row:} Data set $\data_1$ of size 7. 
%   \textbf{Bottom row:} Data set $\data_2$ of size 77.
%   In all cases the exponent parameter was set to $p = 0.5$.}
%			\label{fig:LACKInoise}
%\end{figure}
%
%The figure depicts the inference $\predfn$ (black curve)	 over function values of the target $f$ (blue curve) based on noisy data sets $\data_1$ and $\data_2$. The true observational noise was bounded by level $\obserrbnd = 0.5$ yielding a data-generating function $\tilde f(x) = f(x) +\nu(x)$ (magenta curve) where $\nu(x) \in [-0.5,0.5],\forall x$.
%The first row shows the predictions of our LACKI rule applied to a small sample $\data_1$ with varying parameter settings.
%The second row depicts the pertaining predictions resulting applying the corresponding LACKI rules to an enlarged data set $\data_2 \supset \data_1$.
%
%In plots in the first column and third columns depict situations where LACKI was applied with parameter $\hestthresh=2 \obserrbnd$.  By contrast, the second column depicts a situation where LACKI was parameterised with a parameter $\hestthresh = 0$ and a small initial guess of the H\"older constant of $\underline L = L(0) = 0.01$. As a result, in this case, the LACKI predictor perfectly follows the noisy data. Furthermore, we observe a large uncertainty bound $\prederrn$ with increasing sample size. In the third column the LACKI rule was also initialised with $\underline L =0.01$. However, the larger $\hestthresh = 2 \obserrbnd$ prevents 
%the H\"older constant estimate $L(2)$ to exceed the true constant $L^*=5$. As a result, the prediction ``smoothes out the noise''. The degree of smoothing and approximation error in the limit of infinite data will be theoretically investigated below. 
%At this point we will already mention that all behaviours depicted in the plots seem consistent with our theoretical guarantees we will give in what is to follow.


\subsubsection{Properties}
We will now establish several properties of the LACKI rules including sample-consistency and H\"older continuity. Most importantly however, we will show that the LACKI rules are universal approximators in the sense that they can be set to learn any continuous function with arbitrary worst-case error.

The core idea behind this can be sketched as follows: 
First, we establish H\"older continuity and sample-consistency (cf. Def. \ref{def:sampleconsistency}). This allows us to appeal to Thm. \ref{thm:convergenceifboundedconstandsamplecons} and prove that LACKI can learn any H\"older function.
Note, some universal approximators, such as RBFNs with Gaussian kernels, are provably Lipschitz. Therefore, learning any continuous function can be interpreted as learning some Gaussian RBFN with an observational error level that absorbs the discrepancy between the RBFN and the ground truth. Since a finite RBFN with smooth, bounded-derivative kernel is provably H\"older and since we can learn any H\"older function with LACKI up to the level of observational error, we can learn the continuous ground-truth up to the approximation error of the RBFN. 

Following this outline, we will now proceed to establish the desired properties formally.
 
\begin{lem}[Sample-consistency of LACKI] \label{lem:LACKIsampleconsistency} If for each output dimension $j \in \{1,...,d\}$ and some $\hestthresh \geq 0$ we have $L_j(n)  \geq  \max_{(s,s') \in U_n} \frac{\abs{\tilde f_j(s)- \tilde f_j(s')} -\hestthresh }{\metric_\inspace^p(s,s')}
$ then the LACKI rule is sample-consistent (up to $\frac \hestthresh 2$). 
That is,  \[\forall q \in \{1,\ldots,N_n \}:  \predfn(s_q) \in \ball{\frac \hestthresh 2}{\tilde f_q} \] where $\ball{\frac \hestthresh 2}{\tilde f_q} =\{ x \in \outspace |  \norm{x-\tilde f_q}_\infty \leq \frac \hestthresh 2\}$ denotes the $\frac \hestthresh 2$-ball around the observation $\tilde f_q$.\\
Thus, we also have $\norm{ f(s_q) - \predfn(s_q)}_\infty \leq \frac \hestthresh 2 + \norm{\obserr(s_q)}_\infty$.
\begin{proof}
For ease of notation, we will confine our proof to the case of one-dimensional outputs ($d=1$). The multi-dimensional case follows trivially from the one-dimensional result by applying it to each output component function. 
Let $n \in \nat  $ be fixed and, for ease of notation, write $L := L(n)$. Let $j,k \in   \{1,\ldots,N_n \} $ such that $j \in \argmin_i \tilde f_i + L \metric_\inspace^p(s_i,s_q) $ and 
$k \in \argmax_i \tilde f_i - L \metric_\inspace^p(s_i,s_q) $. 
By definition of $\predfn$ we have:
\begin{align}
\predfn(s_q) 
%&= \frac 1 2 \bigl( \tilde f_j + L \metric_\inspace^p(s_j,s_q)  +\obserrpar(s_q) \bigr) + \frac 1 2 \bigl( \tilde  f_k - L \metric_\inspace^p(s_k,s_q) - \obserrpar(s_q) \bigr)\\
&= \frac 1 2 \bigl(\underbrace{ \tilde f_j + L \metric_\inspace^p(s_j,s_q)}_{:=B}   \bigr) + \frac 1 2 \bigl( \underbrace{\tilde  f_k - L \metric_\inspace^p(s_k,s_q) }_{=:A}\bigr). \label{eq:hru582jsokbbbn}
\end{align}
%
%
(i) Firstly, we show  \underline{$ A \in [\tilde f_q, \tilde f_q +\hestthresh]$}:
If $k = q$, this holds trivially true since then $A= \tilde f_q$. 
So, assume $k \neq q$. 
We have $\tilde f_k \geq \tilde f_k - L \metric_\inspace^p(s_k,s_q)  \geq \tilde f_q - L \metric_\inspace^p(s_q,s_q)  = \tilde f_q$ where the second inequality holds due to $k \in \argmax_i \tilde f_i - L \metric_\inspace^p(s_i,s_q) $. That is,
%\begin{equation} 
%{\tilde f_k - \tilde f_q}  \geq L \metric(s_k,s_q). \label{eq:9p4t37ru8ewihk3hjtu}
%\end{equation} 
\begin{equation} 
A=\tilde f_k - L \metric_\inspace^p(s_k,s_q) \geq \tilde f_q. \label{eq:9p4t37ru8ewihk3hjtu}
\end{equation} 
On the other hand, since $L  \geq  \max_{(s,s') \in U_n} \frac{\abs{\tilde f(s)-\tilde f(s')} - \hestthresh}{\metric_\inspace^p(s,s')}$  we have in particular: $L  \geq  \frac{ \abs{\tilde f_k- \tilde f_q}-\hestthresh }{\metric_\inspace^p(s_k,s_q)}$. Thus,  
 $L \metric_\inspace^p(s_k,s_q) + \hestthresh \geq \abs{\tilde f_k-\tilde f_q} = \tilde f_k - \tilde f_q$. Hence, $\tilde f_q + \hestthresh \geq \tilde f_k - L \metric_\inspace^p(s_k,s_q) = A$. 
 Together with (\ref{eq:9p4t37ru8ewihk3hjtu}) we have shown $A \in [\tilde f_q , \tilde f_q +\hestthresh].$
%  In conjunction with (\ref{eq:9p4t37ru8ewihk3hjtu}) this means that $L \metric(s_k,s_q)  = \abs{\tilde f_k-\tilde f_q} $. Substituting this into the left hand side of Eq. \ref{eq:irndhfkkdnsww} yields the expression 
% $ \tilde f_k - \abs{\tilde  f_k -\tilde  f_q } \stackrel{!}{=}   \tilde f_q $. But since $f_k \geq f_q$, we also have $f_k - \abs{ f_k - f_q }  = f_q$. Therefore, Eq. \ref{eq:irndhfkkdnsww} is equivalent to $f_q = f_q$ which obviously holds. 
% 
%Analogously to the proof of  $f_k - L \metric(s_k,s_q) = f_q$ we can also show $f_j + L \metric(s_j,s_q) = f_q$. Leveraging both equations in Eq. \ref{eq:hru582jsokbbbn} concludes the proof. 

(ii) The proof of \underline{$B \in [ \tilde f_q - \hestthresh, \tilde f_q]$} is completely analogous to that of (i) and hence, is omitted.
%and secondly, that 
%\begin{equation}B \in [ \tilde f_q - \hestthresh, \tilde f_q]. \label{eq:irndhfkkdnswwB}
%\end{equation}

(iii) Together, the statements in (i) and (ii)  entail  $\predfn(s_q) = \frac 1 2 A + \frac 1 2 B  \in [\tilde f_q - \frac \hestthresh 2, \tilde f_q + \frac \hestthresh 2]$.\\
The final statement of the Lemma is a direct consequence of Lem. \ref{lem:groups_sampleconsandobserr}. 
\end{proof}
\end{lem}

Next, we move on to establish that the predictors of the LACKI inference rule are H\"older continuous. More specifically we have:

\begin{lem}[H\"older regularity of LACKI]
With definitions as before, let $(\outspace,\metric_\outspace) = (\Real^m,(x,y) \mapsto \norm{x-y}_\infty)$.
Provided that the bounding functions $\lbf,\ubf$ are H\"older continuous (or set to $-\infty,\infty$, respectively),
the predictors $\predfn$ are H\"older continuous $(n \in \nat)$ with constant $L(n)$ and exponent $p$. That is, $\forall n \in \nat: \predfn \in \Hoelset \bigl(L(n),p\bigr)$.

\begin{proof}
By combining Thm. \ref{thm:d2pmapishoelder} with Lem. \ref{lem:Hoeldarithmetic} it follows that each output component function $\predf_{n,j}$ $(j=1,...,m)$ is $L(n)$-$p$- H\"older. This implies the desired statement. 

\end{proof} 
\label{lem:LACKIpredHoelder}
\end{lem}

In the remainder of this section, we will establish convergence guarantees of our LACKI inference rules. In particular, we shall study the behaviour of the sequence of predictors $\seq{\predfn}{n \in \nat}$ computed on the basis of a sequence of data sets $\seq{\data_n}{n \in \nat}$ that becomes dense on the domain in the limit of increasing sample size. To clarify the latter statement, consider the sequence of grids $\seq{G_n}{n \in \nat}$. We say this sequence \emph{becomes dense in $I \subset \inspace$ in the limit of large $n$ }if it \emph{convergences} to $I$ as $n \to \infty$. That is, if $\forall \epsilon >0,x \in I \exists n_0 \forall n \geq n_0 \exists g \in G_n: \metric_\inspace(x,g) < \epsilon$. If the rate of convergence is independent of $x$ then we say that the grid sequence converges to $I$ \emph{uniformly}. This is the case iff $\forall \epsilon >0 \exists n_0 \forall n \geq n_0, x \in I \exists g \in G_n: \metric_\inspace(x,g) < \epsilon$.

\begin{defn}
Relative to a pseudo-metric $\metric$, a sequence of sets $(\mathcal S_n)_{n \in \nat}$ converges to a set $\mathcal S$ with \emph{rate} $r: \nat \to \Real_+$ iff for all $n \in \nat$ we have $\inf_{s_n \in \mathcal S_n}\inf_{s\in \mathcal S} \metric(s_n,s)\leq r(n)$ and $r(n) \to 0$.
\end{defn}


\begin{thm}[LACKI can learn any H\"older function] \label{thm:convergenceifboundedconstandsamplecons_LACKI}
Let $\seq{\data_n}{n \in \nat}$ be a data set sequence with pertaining grid sequence $\seq{G_n}{n \in \nat}, G_n \subset G_{n+1} \subset \inspace (n \in \nat)$ converging to a dense subset of input domain $\inspace$. 
We assume the observational errors given by $\obserr$ are bounded from above by $\obserrbnd= \sup_x \obserr(x)$.
Furthermore, let the target $f: \inspace \to \outspace$ be H\"older with $f \in \hoelset {L^*}{}  p$ and assume $\lambda$ is set to a value of at least $2 \bar e$.
%
%and let the predictors be sample-consistent up to error $\bar E$ and H\"older continuous, 
%$\predfn \in \hoelset {L(n)}{} p$ with $L(n) \leq \bar L \in \Real_+\, (n \in \nat)$ for some $\bar L \geq 0$.

Then, we have 

%\begin{itemize} \item 
(I) The sequence of predictors $\seq \predfn {n \in \nat}$ converges to the ground truth $f$ pointwise up to error $\frac \hestthresh 2 +\obserrbnd$. That is, $\forall \epsilon \geq 0,  x \in \inspace \exists n_0 \in \nat \forall n \geq n_0: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon + \frac \hestthresh 2 + \obserrbnd$.

%\item 

(II) If the grid sequence $\seq{G_n}{n \in \nat }$ converges to the domain $\inspace$ uniformly then $\seq \predfn {n \in \nat}$ converges to the target $f$ uniformly up to error $ \frac \hestthresh 2 +\obserrbnd$. 

That is, $\forall \epsilon \geq 0 \exists n_0 \in \nat \forall n \geq n_0, x \in \inspace: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon +   \frac \hestthresh 2  +\obserrbnd$.
%\end{itemize}
Convergence occurs with a rate of at most $n \mapsto 2 \max\{\bar L_\lambda, L^* \} r(n)^p$ where $r$ is the rate of convergence of the input data set sequence $(G_n)$ and $\bar L_\lambda =\max_{x,x'} \frac{\metric_\outspace(f(x), f(x')) + 2 \obserrbnd -\hestthresh }{\metric_\inspace^p(x,x')}$ is an upper bound on the maximally attainable empirical estimate of the H\"older constant.

\begin{proof}
We have established that the predictors $\predfn(\cdot)$ of the LACKI rule are $L(n)-p$- H\"older (Lem. \ref{lem:LACKIpredHoelder}) and sample-consistent up to level $\frac \hestthresh 2$ (Lem. \ref{lem:LACKIsampleconsistency}). Furthermore, we can show that the sequence $\seq{L(n)}{n \in \nat}$ is convergent and bounded (Lem. \ref{lem:constadaptation_boundedness}). Furthermore our input and output spaces are additive abelian groups. By assumption, pseudo-metrics $\metric_\inspace,\metric_\outspace$ are translation invariant with respect to addition. Therefore, the predictors meet all assumptions of Thm. \ref{thm:convergenceifboundedconstandsamplecons} which entails the desired convergence statements.
\end{proof}
\end{thm}



Having established that our LACKI rule can learn any H\"older function with any H\"older constant, we will now attend to extend the results to non-H\"older functions. In preparation of the necessary derivations we will first rehearse universality and H\"older properties of radial basis function networks. 

Park and Sandberg derived universal approximation guarantees for radial-basis function networks \cite{Park1991}. In particular, on page 252 in their article the authors make an assertion that translates to our notation as follows: 

\begin{lem}[Expressiveness of RBFNs] \label{lem:RBFNunifapproxcompact} Assume $\inspace \subseteq \Real^d$ is compact. Given parameter  vector $\theta := (w_1,\ldots,w_m,\sigma_1,...,\sigma_m,c_1,\ldots, c_m)$ and kernel function $K: \inspace \to \outspace $ let $\beta(\cdot;\theta ) = \sum_{i=1}^m w_i \, K(\frac{\cdot - c_i}{\sigma_i} )  $ denote a radial basis function network (RBFN). Assume $K: \Real^d \to \Real$ is continuous and has non-vanishing integral, i.e. $\int_{\Real^d} K(x) \d x \neq 0$.
Then, the set $S_K:= \{ \beta(\cdot; \theta) \vert  m \in \nat, \theta \in \Real^{3m}  \}$ of all RBFNs is uniformly dense in the set $C(\inspace)$ of continuous functions on compact domain $\inspace$. That is,  $\forall f \in C(\inspace) \forall \epsilon >0  \exists m, \theta \in \Real^{3m} : \sup_{x \in \inspace}{ \abs{f -\beta(\cdot;\theta)  } } <\epsilon $. 
\end{lem}

\begin{remark} \label{rem:LipconstofRBFN}
We note that, for any finite-dimensional parameter $\theta$, any RBFN $\beta(\cdot;\theta)$ is Lipschitz continuous as long as the kernel $K$ is. This can be seen by applying Lem. \ref{lem:Hoeldarithmetic} which allows us to conclude that the Lipschitz constant of RBFN $\beta(\cdot;\theta ) = \sum_{i=1}^m w_i \, K(\frac{\cdot - c_i}{\sigma_i} ) $ is given by $L_\beta = \sum_{i=1}^m \abs{\frac{w_i}{\sigma_i}} L_{K}$ where $L_K \in \Real_{\geq 0}$ denotes a Lipschitz constant of $K$. By the same Lemma it is easy to see that choosing the Gaussian kernel for $K$ satisfies both the Lipschitz requirement as well as the integrability requirements of Lem. \ref{lem:RBFNunifapproxcompact}. As a by-product this means that on a compact support, any continuous function can be approximated by some Lipschitz function with arbitrarily small, positive worst-case error $\epsilon >0$. Note, it may well be the case that the Lipschitz constant of the approximator grows with decreasing approximation error bound $\epsilon$. We expect this to be inevitable when the approximated function is not Lipschitz.
\end{remark}

Harnessed with these preparatory statements we can move on to give a guarantee of uniform convergence about our LACKI rule: 

\begin{thm}[Universality of LACKI]
\label{thm:LACKIuniversality}
Assume we are given a sequence $\seq{\data_n}{n \in \nat}$ of samples with observational errors bounded by $\obserrbnd \in \Real$. We set the parameters of the LACKI rule to $\lbf =-\infty,\ubf =\infty, \underline L =0$. In this theorem, we assume input space $\inspace$ to be compact.

\textbf{Then, we have:}
The LACKI rule as per Def. \ref{def:LACKI} is a universal approximator in the following sense:
If the sequence of input grids $\seq{G_n}{n \in \nat}$ converges to compact input space $\inspace$ (uniformly) then for any parameter choice $\hestthresh >0, p \in (0,1]$, the sequence of predictors $\seq{\predfn}{n \in \nat}$ computed by the LACKI rule (uniformly) converges to any continuous target $f : \inspace \to \Real$ up to error $\hestthresh+\obserrbnd$.
That is, 
\begin{itemize}
\item (II) $\forall \epsilon >0,x \in \inspace \exists n_0 \geq 0\forall n\geq n_0: \metric_\outspace\bigl(\predfn(x),f(x)\bigr) \leq \epsilon + \hestthresh+\obserrbnd$ if $G_n$ converges to $\inspace$ as $n \to \infty$.
\item (I) If $G_n$ converges to $\inspace$ \textit{uniformly} (as $n \to \infty$) we even have: $\forall \epsilon >0 \exists n_0 \geq 0\forall n\geq n_0, x \in \inspace: \metric_\outspace\bigl(\predfn(x),f(x)\bigr) \leq \epsilon + \hestthresh +\obserrbnd$. 
\end{itemize}
Convergence occurs with a rate of at most $n \mapsto 2 \max\{\bar L_\lambda, \tilde L \} \,r(n)^p$ where $r$ is the rate of convergence of the input data set sequence $(G_n)$, $\bar L_\lambda =\max_{x,x' \in \inspace} \frac{\metric_\outspace(f(x), f(x')) + 2 \obserrbnd -\hestthresh }{\metric_\inspace^p(x,x')}$ is the an upper bound on the maximally attainable empirical estimate of the H\"older constant and $\tilde L \in \Real$ is a constant such that the target $f$ is $\tilde L-p-$ H\"older up to error up to $\frac \lambda 2$.
\end{thm}

\begin{proof}
We choose any parameter $\hestthresh >0$. As observed in Rem. \ref{rem:LipconstofRBFN}, Lem. \ref{lem:RBFNunifapproxcompact} allows us to infer that there exists a Lipschitz function $\beta(\cdot;\theta)$ that approximates the target with worst-case error of at most $\frac \hestthresh 2$. That is, $\sup_{x \in \inspace} \metric_\outspace\bigl(\beta(x,\theta), f(x) \bigr) \stackrel{Lem. \ref{lem:bilinaddtransinvgroup}}{\leq} \sup_{x \in \inspace} \metric_\outspace\bigl(0, \psi(x) \bigr) \leq \frac \hestthresh 2$ where $\psi:\inspace \to \outspace$ is a function such that $f= \beta(\cdot;\theta) + \psi$ pointwise.
Instead of viewing the given sample as being generated by target $f$ (with some observational error) we can view the sample as being generated by the RBFN $\beta(\cdot;\theta)$ (with some larger observational error): 
We can interpret the erroneous sample $\data_n:= \{\bigl( s_i, \tilde f_i\bigr) \vert i=1,\ldots, N_n\} $ with observational error bound $\obserrbnd$ of $f$ as a ``noisy'' sample $\tilde \data_n:= \{\bigl( s_i, \tilde \beta_i \bigr) \vert i=1,\ldots, N_n\}$ of $\beta(\cdot;\theta)$ where $\tilde \beta_i = \tilde f(s_i) = \beta(s_i;\theta)+\nu(s_i) $. Here the new, enlarged observational error $\nu$ assumes the role of the  bounded ``observational error'' with upper bound $\bar \nu := \obserrbnd + \frac \hestthresh 2$. $\nu(\cdot)$ subsumes both the intrinsic observational error in the data $\data_n$, as well as the discrepancy between RBFN $\beta(\cdot;\theta)$ and the target $f$. Using LACKI to learn $f$ on the basis of $\data_n$ therefore is the same as learning $\beta$ with larger observational error bounded by $\bar \nu := \obserrbnd + \frac \hestthresh 2$.


Being a finite sum of smooth functions with bounded Lipschitz constants, $\beta(\cdot;\theta)$ also is Lipschitz with some optimal Lipschitz constant $L_\beta \in \Real_{\geq 0}$ (cf. Rem. \ref{rem:LipconstofRBFN}).
Since Lipschitz continuity implies H\"older continuity (see Lem. \ref{lem:hoeldexpprop2} ), we have $\beta(\cdot,\theta) \in \hoelset {\tilde L}{ }{p}$ for some $(\tilde L \in \Real_{\geq 0}$ and any $p \in (0,1])$.

Since $\beta(\cdot,\theta)$ is H\"older continuous, the desired convergence statements follow immediately by appealing to Thm. \ref{thm:convergenceifboundedconstandsamplecons_LACKI}.
%%OLD PROOF:
%
%By Lem. \ref{lem:constadaptation_boundedness}, the lazily adapted H\"older constant estimates $L(n)$ are bounded from above by $\max\{\underline L, \tilde L\} = \tilde L  < \infty$. In conjunction with Lem. 
%\ref{lem:LACKIsampleconsistency} (which establishes sample consistency up to $\frac \hestthresh 2$) we have established that all preconditions of Thm. \ref{thm:convergenceifboundedconstandsamplecons} are met by the predictors $\predfn$ $ ({n \in \nat})$. Hence, the theorem allows us to conclude that the sequence of predictors $\seq{\predfn}{n \in \nat}$ converges to $\beta(\cdot;\theta)$ up to an error less than or equal to $\sup_x \metric_\outspace(0,\psi(x)) \leq \frac \hestthresh 2$:
%
%
%(I) In the general case this convergence is pointwise. 
%Let $x \in  \inspace$ and $\epsilon > 0$.  Thm. \ref{thm:convergenceifboundedconstandsamplecons}.(I) implies $\exists n_0 \forall n\geq n_0: \metric_\outspace\bigl (\predfn(x), \beta(x,;\theta) \bigr) \leq \epsilon+\frac \hestthresh 2$. Hence, $\metric_\outspace\bigl (\predfn(x), f(x) \bigr) = \metric_\outspace\bigl (\predfn(x), \beta(x,;\theta) + \psi(x) \bigr) \stackrel{Lem. \ref{lem:bilinaddtransinvgroup}}{\leq} \metric_\outspace\bigl(\predfn(x), \beta(x,;\theta)\bigr) +\metric_\outspace\bigl(0, \psi(x) \bigr) \leq \metric_\outspace\bigl(\predfn(x), \beta(x,;\theta)\bigr) +\frac \hestthresh 2\leq \epsilon +\hestthresh$.
%
%(II)  If convergence of the grid to domain $\inspace$ is uniform convergence of the predictors to the RBFN is uniform (by Thm. \ref{thm:convergenceifboundedconstandsamplecons}.II ). The remainder of the proof is completely anaologous to (I), except that $n_0$ can be chosen independently of $x$.
%
%

\end{proof}

\begin{remark}
Note, our universality guarantee of Thm. \ref{thm:LACKIuniversality} is much stronger than the guarantee for RBFNs.
 The universality statement for RBFNs is purely representational. That is, it states that in principle it is possible to find some RBFN with some choice of parameter that approximates any continuous function with arbitrarily small worst-case approximation error. However, it makes no mention of how to find such an RBFN. By contrast, our universality statement is about a concrete learning rule. And, given a desired error level it tells how to set the parameters of the learning rule in order to achieve the desired approximation error in the dense sample limit.
\end{remark}

%\begin{remark}
%Note, the bound on the speed of convergence generally decreases with increasing best Lipschitz constant of the RBFN. Generally, the Lipschitz constant will increase with decreasing $\hestthresh$. Therefore, so far, we have not shown convergence in the case of $\hestthresh=0$. 
%Intuitively, we should still have convergence since in the limit $L^* \to \infty$ the KI rule seems to coincide with a nearest neighbour regression rule. By construction of integrable functions, it should be clear that this rule converges to any function in the set $\mathcal L_q$ of power-$q$ integrable function  with respect to the $\mathcal L_q$ metric and $q \in \nat$.
%Investigating this observation in greater rigour could be subject to future work. Of course, from a practical point of view our current results are sufficient. If we set $\hestthresh >0$ below the machine-epsilon of the computer the algorithm is intended to run on, our results ensure that the algorithm will not be able to distinguish $\predfn(x)$ and the target $f$ for any input value and sufficiently large training data size $N_n \in \nat$.
%\end{remark}


%\subsection{Convergence in probability with uniformly distributed inputs}
%\jcom{Might omit this subsection}
%Above we have given guarantees relative to the deterministic convergence rates of the input sample to the domain.
%In this subsection, we shall study probabilistic convergence rates as a function of the sample size in situations where the sample is obtained by drawing inputs independently from the domain according to the uniform probability distribution.
% 
%We assume the input data sets $G_n=\{s_1,\ldots,s_{n}\}$ are obtained by drawing the sample inputs $s_i$ i.i.d. uniformly at random from the bounded input domain $\inspace$. For ease of notation, we assume $\inspace := [0,1]^d$ is a normalised d-dimensional hypercube and that the input metric is induced by the maximum norm $\norm{\cdot}_\infty$.
%Under these conditions, we can prove that input sequence $\seq{G_n}{n \in \nat}$ converges to a dense subset in probability:
%\begin{lem}
%For all $x \in \inspace = [0,1]^d$ and $\varepsilon \in (0,1)$ we have
%\[ \Pr[\min\{ \norm{x - g_n}_\infty \,| \, g_n \in G_n \} \geq \varepsilon] \leq r(n) \]
%where 
%\[r(n) = \Bigl(1- \varepsilon^d \Bigr)^n \stackrel{n \to \infty}{\longrightarrow} 0.\]
%\begin{proof}
%Let $x \in \inspace$ and $ \varepsilon \in (0,1)$. 
%Let  $\ball{\varepsilon}{x} =\{\xi \in \inspace | \norm{x-\xi}_\infty \leq \varepsilon \}$ denote a $\varepsilon$-ball around $x$. It is easy to see that we have $\Pr[ \ball{\varepsilon}{x} ] = \int_{\xi \in \inspace} \indicator{\ball{\varepsilon}{x}} (\xi) \d \xi \geq \varepsilon^d$. 
%%
%Hence, 
%\begin{align}
%&\Pr[\min\{ \norm{x - g_n}_\infty \,| \, g_n \in G_n \} \geq \varepsilon ]  \\
%&=\Pr[\forall s \in G_n: \norm{x - s}_\infty \geq \varepsilon] \\
%&\stackrel{i.i.d.}{=} \prod_{i=1}^n \Pr[s_i \notin \ball{\varepsilon}{x}] \\
%&= \prod_{i=1}^n 1-\Pr[s_i \in \ball{\varepsilon}{x}] \\
%&\leq \prod_{i=1}^n 1-\varepsilon^d = (1-\varepsilon^d)^n.
%\end{align}
%\end{proof}
%\end{lem}
%\jcom{Next,will tie this to the main theorems..., or porbably leave out}

==> content2/conclusions.tex <==
\section{Conclusions}
In this paper, we have introduced \emph{Lazily Adapted Constant Kinky Inference (LACKI)} as method for nonparametric machine learning. Our method was built on the framework of \emph{Kinky Inference} (which in turn is a generalisation of well-known approaches such as \emph{Lipschitz Interpolation} \cite{Zabinsky2003,Beliakov2006} and \emph{Nonlinear Set Membership (NSM)}  methods \cite{Milanese2004}). 
 Our approach inherits the numerical simplicity of these methods. On top of this, it can deal with bounded additive noise and does not require a priori knowledge about a H\"older constant of the underlying target function but instead estimates the constant online from the data. This of course is of great practical interest since this endows LACKI with superior black-box learning capabilities.
 
To avoid the need to specify the H\"older constant, LACKI adapts the parameter $L(n)$ to reflect a modification of the empirical estimate of the H\"older constant of the underlying target function. 
The adapted parameters were carefully defined to be bounded even if the target function is not H\"older continuous and the data is subject to bounded observational uncertainty.
This allowed us to establish several theoretical guarantees. For instance, we proved that our LACKI rule can learn any H\"older function (up to the level of noise in the data). Moreover, we showed that LACKI can also learn continuous but non-H\"older target functions up to a worst-case approximation error that converges to the level of intrinsic observational  error in the data-generating process, plus a value coinciding with parameter $\hestthresh \geq 0$. Since 
$\hestthresh$ is a free parameter that can be set to arbitrarily small values, convergence can be reduced down to the observational noise-level as much as desired. However, while we have not investigated this theoretically, we would expect that reducing the magnitude of $\hestthresh$ will not only cause the uncertainty bounds to grow (or even grow unbounded if the target is not H\"older or there is noise in the data) but also to slow down the worst-case convergence rate of the LACKI predictors. 
Investigating such convergence rates is a topic we would find interesting to investigate in the context of future work. 

Our theoretical considerations were supplemented by an application of LACKI to 
online learning-based model-reference adaptive control. In a simulated aircraft control problem with nonlinear model uncertainty, we compared our LACKI-based controller against other learning-based methods that were recently proposed in the control literature. Across a range of performance metrics and randomised problem instances, LACKI-MRAC demonstrated consistent and robust performance and outperformed its competitors.
For discrete-time systems with additive nonlinear uncertainty, we provided theoretical guarantees on the tracking success of our LACKI-MRAC controller.

While previous work has utilised NSM methods in control, their methods relied on knowing the true Lipschitz constant a priori - something that is an assumption we would argue is not practically plausible.
Our work addresses this deficiency and provides learning and stability guarantees even in the absence of a priori knowledge of this constant.


In future work, we would like to apply our LACKI learning method to more challenging control tasks that require planning.
To this end, it might be beneficial to link our results to recent work on NSM-based model-predictive control \cite{Canale2014}.

In this work, we have assumed that the observational noise was bounded; we have addressed the issue of unbounded noise in a companion paper \cite{POKIdraft2016} where the H\"older constant parameter $L(n)$ is found as the minimiser of a prediction loss estimator.  We also believe that these estimators could be used to estimate the noise bound if these are unknown a priori.

In this work, our theoretical considerations relied on worst-case analysis. Consequently, our learning guarantees were unable to guarantee the reduction of the approximation error of the predictor to the target below the level of observational noise. However, in Fig. \ref{fig:LACKInoise} and Fig. \ref{fig:LACKInoise2} we observed that our predictors were capable of smoothing out stochastic noise resulting in predictors that exhibited close alignment with the true target. Investigating the extent to which distributional assumptions about the noise can be translated to probabilistic convergence results to the target will also be a subject of future investigation. 



%At this point, we believe that we have found a way to utilise the convergence guarantees derived in this paper to prove that the tracking-error of LACKI-MRAC is guaranteed to vanish as learning is allowed to proceed.

%\section{Conclusions}
%Our paper started by introducing \textit{Kinky Inference (KI)}, a nonparametric machine learning method that can take advantage of knowledge about H\"older regularity and optionally boundedness in order to facilitate inference over function values at unseen (possibly uncertain) inputs on the basis of a (possibly uncertain) sample. When the parameters $L(n)$ are chosen to coincide with a H\"older constant of the target function, the method also provides deterministic prediction uncertainty bounds which we have shown to be tight and (uniformly) convergent to zero in the limit of dense data.
%In contrast to much work in nonparametric regression our theoretical analysis has not made distributional assumptions. This is important in control settings where the collected data might be highly correlated or lie on manifolds of state space. 
%
%To accommodate cases where the target might not be H\"older continuous or the H\"older constant is unknown, we also have presented \textit{Lazily Adapted Constant Kinky Inference (LACKI)}. Here the parameters $L(n)$ are incrementally adapted to the sample $\data_n$ in a manner that allowed us to establish (uniform) universal approximation guarantees. That is, on a compact domain, we can set LACKI up such that its predictors can learn any continuous target up to any arbitrarily small error.
%
%In comparison with other learning methods our approach is not only highly flexible to learn continuous functions but also fast. We have illustrated both properties in the context of model-reference adaptive control where our LACKI method served as the adaptive element of a controller tasked with executing roll commands of a simple aircraft model under wingrock dynamics. In comparison to other recent online-learning methods our LACKI-MRAC controller outperformed its competitors across the board of randomized problem instances. 

==> content2/group_learners.tex <==
\subsection{Learning as inference over group mappings}
\label{sec:group_learners}
Groups provide basic algebraic structures. At this point we will look into several properties that apply to learning of mappings between abelian groups. Since the concept of an abelian group is more general than that of a vector space, all our results readily apply to learning of mappings between vector spaces.


Next, we will consider the following framework for learning mappings $f:\inspace \to \outspace$ between such groups $(\inspace,+), (\outspace,+)$: 

At \emph{stage} or \emph{time} $n \in \nat$, we assume we have access to a \textit{sample} or \textit{data set} $\data_n:= \{\bigl( s_i, \tilde f_i\bigr) \vert i=1,\ldots, N_n \} $ containing $N_n \in \nat$ (possibly erroneous) sample images $\tilde f_i \in \outspace$ of function $f$ at sample input $s_i \in \inspace$. Here the term \emph{erroneous} refers to the situation of bounded additive corruption of the sample images. That is,  $f_i = \tilde f(s_i) = f(s_i) + \phi(s_i)$ where $\phi: \inspace \to \outspace$ is a stochastic or deterministic perturbation we refer to as \emph{(observational) noise} and $\tilde f$ defines the noise-corrupted version of $f$ we can observe. For the purpose of worst-case analysis, we assume the noise to be bounded, i.e. $\metric_\outspace(\phi(x),0) \leq \obserr(x) \leq \obserrbnd <\infty$ for all inputs $x$ of interest.
We refer to $\obserr$ as the \emph{ observational error} and to $\obserrbnd \in \Real_{\geq 0}$ as the \emph{observational error bound}.
To aide our discussion, we define $G_n =\{s_i | i =1,\ldots,N_n\}$ to be the \textit{grid} of sample inputs contained in $\data_n$. Subscript $n$ aides our exposition when we consider sequences $\seq{\data_n}{n \in \nat}$ of data sets indexed by $n$.

Let $I \subseteq \inspace$ be some domain of interest.
The task of learning the \emph{target} $f: I  \to \outspace$ on the basis of data $\data_n$ consists in the generation of a computable \emph{predictor} $\predfn: I \to \outspace$ that somehow approximates the target. Since the predictor is constructed on the basis of the data, we can construe computation of predictions $\predfn(x)$ as \emph{inferences} over function values. Therefore, any algorithm for computing $\predfn(x)$ will be referred to as an \emph{inference rule}. In this lingo, \emph{learning} is the construction of inference rules over function images and machine learning is the discipline of conceiving computatable inference rules.  
That is, a \emph{learner} $\ell$ constitutes a computable mapping $\ell: \data_n \mapsto \predfn$.

For the sake of analysis, the quality of the inference has to be quantifiable. To this end, we will assume the groups $\inspace, \outspace$ are endowed with (pseudo-) metrics $\metric_\inspace,\metric_{\outspace}$, respectively. The output pseudo-metric $\metric_\outspace$ allows us to quantify the error of a prediction as per $\metric_{\outspace} \bigl(\predfn(x),f(x) \bigr) $.
Furthermore, the input pseudo-metric $\metric_\inspace$ allows us to quantify the similarity between a test input $x \in I\subseteq \inspace$ and the learning experience given by the data. Intuitively, a sensible learner might perform well on test inputs $x$ that are similar to the learning experience. That is, we might expect the prediction error  $\metric_{\outspace} \bigl(\predfn(x),f(x) \bigr) $ to decrease with decreasing dissimilarity to the data measured by $\dist(x,\data_n) := \inf_{s \in G_n}  \metric_\inspace(x,s)$. It might not be surprising that we will be able to take advantage of H\"older continuity properties in order to establish such a desirable behaviour of an inference rule. 
In particular, they will prove key in the examination of uniform convergence of the \emph{worst-case prediction error} 
% 
$\sup_{x\in I} \metric_{\outspace} \bigl( \predfn(x), f(x) )$ as $n \to \infty$ in situations where 
the data becomes increasingly dense, i.e. where $\dist(G_n,I):= \sup_{x \in I} \inf_{s \in G_n} \metric_\inspace(x,s)  \stackrel{n \to \infty}{\rightarrow} 0$. In particular, we will construct a class of H\"older continuous inference rules that are universal approximators in the sense that they can guarantee a vanishing worst-case error in the limit of dense grids as long as the target $f$ is continuous (but not necessarily H\"older).
As a preliminary step, we will next provide convergence guarantees for certain H\"older continuous inference rules in situations where the target is indeed H\"older.

\subsubsection{Convergence properties of sample-consistent learners of H\"older continuous group mappings}

It will be convenient to restrict our attention to groups $\inspace$ that are \emph{translation-invariant} with respect to their metric $\metric$. That is, we assume $ \metric(g+g',g''+g') = \metric(g,g''),\forall g,g',g'' \in \inspace$.

In such groups the following holds true:

\begin{lem} Let $\metric : \inspace^2 \to \Real$ be a translation-invariant pseudo-metric on an abelian group $(\inspace,+)$.
We have 
\begin{itemize}
\item \textbf{(I)} $\forall g,g',g'' \in \inspace: \metric(g+g',g'') \leq \metric(g,g'')+\metric(g',0)$.
\item \textbf{(II)} $\forall g \in \inspace: \metric(g,0) = \metric(-g,0)$.
\item \textbf{(III)} If $g'' = g+g'$ and $\metric(g'',g) \leq b$ then $\metric(0,g') \leq b$.
\end{itemize}
\begin{proof}
(I): $\forall g,g',g'' \in \inspace: \metric(g+g',g'') \leq \metric(g+g',g)+\metric(g,g'') = \metric(g',0)+\metric(g,g'').$
(II): $\forall g \in \inspace: \metric(g,0) = \metric(g+(-g),-g) = \metric(0,-g) =\metric(-g,0).$
(III): Follows trivially from translation-invariance.
\end{proof}
\label{lem:bilinaddtransinvgroup}
\end{lem}
 
\begin{defn} [Sample-consistency] A predictor $\predfn : \inspace \to \outspace$ is consistent with sample $\data_n$ (up to error $E: \inspace \to \Real$) iff $\forall (s_i,\tilde f_i,\obserr(s_i) ) \in \data_n: \metric_{\outspace}\bigl(\predfn(s_i),\tilde f(s_i)\bigr) \leq E(s_i) $. An inference is called \emph{sample-consistent} if for every possible sample $\data_n$ the generated predictor $\predfn$ is consistent with $\data_n$. We denote the set of all functions consistent with sample $\data_n$ by $\mathcal K (\data_n)$.
\label{def:sampleconsistency}
\end{defn}

\begin{lem}\label{lem:groups_sampleconsandobserr} As always, let $\obserr(\cdot) $ denote the bound on the observational error.
If $\predf_n$ is sample-consistent up to error $E$ with respect to set data $\data_n$ then, for any sample input $s \in G_n$, we have $\metric_\outspace\bigl(f(s), \predfn(s) \bigr) \leq E(s) + \metric_\outspace(0,\obserr(s))$.  Given an upper bound  $\obserrbnd \in \Real$ on the observational error  such that $\obserrbnd \geq \obserr(x),\forall x$ then sample-consistency up to error $E$ entails that true function is contained in the $E(s) + \obserrbnd$-balls around the predictions of observed inputs. That is, for all $s \in G_n$ we have:
\begin{equation}
 f(s) \in \ball{ E(s) + \obserrbnd}{\predfn(s)} = \{y \in \outspace | \metric_\outspace(\predfn(s),y ) \leq E(s) + \obserrbnd \}.
\end{equation}
\end{lem}
\begin{proof}
Sample consistency up to $E$ implies that for each sample input $s \in G_n$ $\Metrico{\predfn}{\tilde f(s)} \leq E(s)$.
On the other hand, bounded observational errors mean that for $s$ 
there is $\nu_s \in \outspace, \Metrico 0 {\nu_s} \leq \obserrbnd$ such that we have $\Metrico{f(s)}{ \tilde f(s) } = \Metrico{f(s)}{ f(s)+\nu_s } \leq \Metrico{0}{\nu_s } \leq \obserrbnd$.
Since the output pseudo-metric $\Metrico \cdot \cdot$ adheres to the triangle inequality, we have 
$\Metrico{f(s)}{\predfn(s)} \leq \Metrico{f(s)}{ \tilde f(s) } + \Metrico{\predfn(s)}{ \tilde f(s) } \leq E(s) + \obserrbnd $.
\end{proof}

Next, we will establish that sample-consistent and continuous H\"older inference rules can learn any H\"older continuous target.

\begin{defn}
Relative to a pseudo-metric $\metric$, a sequence of sets $(\mathcal S_n)_{n \in \nat}$ converges to a set $\mathcal S$ iff  for all $s \in S$ there is a vanishing function $r_s:\nat \to \Real$, $r(n) \stackrel{n \to \infty} {\to} 0$ such that we have:  $$ \forall n \in \nat: \inf_{s_n \in \mathcal S_n} \metric(s_n,s)\leq r(n).$$
If the same function $r(\cdot)$ can be given for all $s \in \mathcal S$ then the convergence is uniform and we say that $(\mathcal S_n)$ converges to $\mathcal S$ uniformly with rate $r$. In the case of uniform convergence with rate of at most $r$ we have: $$\sup_{s \in \mathcal S} \inf_{s_n \in \mathcal S_n} \metric(s_n,s) \leq r(n) \stackrel{n \to \infty}{\to} 0$$.
\end{defn}


\begin{thm} \label{thm:convergenceifboundedconstandsamplecons}
Let $\seq{\data_n}{n \in \nat}$ be a data set sequence with pertaining grid sequence $\seq{G_n}{n \in \nat}$, \\ with $G_n \subset G_{n+1} \subset \inspace (n \in \nat)$ converging to a dense subset of input domain $\inspace$. Assume all of the following: 
\begin{enumerate} 
\item The data sets $\data_n$ ($n \in \nat$) all have bounded observational error with $\obserrbnd := \sup_x \Metrico{0}{\obserr(x)} \in \Real_{\geq 0}$.
\item The target $f: I \subseteq \inspace \to \outspace$ is H\"older continuous with $f \in \hoelset {L^*}{}  p$.
\item The predictors $\predfn$ $(n \in \nat)$ are sample-consistent up to error $E:\inspace \to \Real$ with $\bar E := \sup_x E(x) \leq \infty$.
\item The predictors are  H\"older continuous with H\"older constants bounded below $\bar L \in \Real_{\geq0}$. That is, 
$\exists \bar L \geq 0 \forall n \in \nat: \predfn \in \hoelset {L(n)}{} p$  $ \wedge$ $ L(n) \leq \bar L$.
\end{enumerate}


Then, we have: 
\begin{itemize}
\item \textbf{(I)}The sequence of predictors $\seq \predfn {n \in \nat}$ converges to the ground truth $f$ pointwise up to error $\bar E$. That is, $\forall \epsilon \geq 0,  x \in \inspace \exists n_0 \in \nat \forall n \geq n_0: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon + \bar E + \obserrbnd$.
%\item 

\item \textbf{(II)} If the grid sequence $\seq{G_n}{n \in \nat }$ converges to the domain $\inspace$ uniformly then $\seq \predfn {n \in \nat}$ converges to the target $f$ uniformly up to error bound $\bar E + \obserrbnd$. 

That is, $\forall \epsilon \geq 0 \exists n_0 \in \nat \forall n \geq n_0, x \in \inspace: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon + \bar E+\obserrbnd$.

\item \textbf{(III)} If the uniform convergence of the grid sequence as per (II) occurs with a rate of at most $r:\nat \to \Real$ then we have:  $$\forall n \in \nat \forall x \in I \subseteq\inspace: \metric_\outspace\bigl(\predfn(x) , f(x)\bigr)\in [0,(\bar L+ L^*) r(n)^p+ \bar E + \obserrbnd].$$ That is, as $n \to \infty$,  convergence (up to error $\bar E +\obserrbnd)$ of the predictors to the target occurs uniformly at a rate of at most $(\bar L+ L^*) r(n)^p$.
\end{itemize}

\begin{proof}
For $x \in I\subseteq \inspace$ let $\xi_n^x$ denote the nearest neighbour of $x$ in grid $G_n$. That is, $\xi_n^x = \arg\inf_{s \in G_n} \metric_\inspace(x,s)$.

\textbf{(I)} 
Since $G_n$ is assumed to converge to a dense subset of the domain $I$, we have$ \metric(x,\xi_n^x )^p
\stackrel{n \to \infty}{\longrightarrow} 0$.
Furthermore, since the the predictors are sample-consistent on grid $G_n$ up to error $E$ and since $\xi_n^x \in G_n$ we can appeal to Lem. \ref{lem:groups_sampleconsandobserr} (as well as to the triangle inequality) to reason as follows:
%there always is some $\phi(\xi_n^x) \in  \ball{\bar E}{0} = \{ y \in \outspace \,| \, \metric_\outspace(y,0 ) \leq \bar E \}$ such that (i) 
$\metric_\outspace\bigl(\predfn(x) , f(\xi_n^x)  \bigr) 
\leq 
\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \metric_\outspace\bigl(\predfn(\xi_n^x) , f(\xi_n^x)  \bigr)
\stackrel{Lem. \ref{lem:groups_sampleconsandobserr}}{\leq} 
\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + E(\xi_n^x) + \obserr(\xi_n^x)$.
Hence,
\begin{equation}
\forall x: \metric_\outspace\bigl(\predfn(x) , f(\xi_n^x)  \bigr) \leq
\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \bar E + \obserrbnd.
\label{ineq:ewlfjhflsape}
\end{equation}
%
Thus, for $x \in \inspace$:
%
$\metric_\outspace\bigl(\predfn(x) , f(x)\bigr) \leq \metric_\outspace\bigl(\predfn(x) ,  f(\xi_n^x)  \bigr) + \metric_\outspace\bigl(f(\xi_n^x) , f(x)\bigr)$
$\leq 
\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \bar E + \obserrbnd+ \metric_\outspace\bigl(f(\xi_n^x) , f(x)\bigr)$
%$\norm{\predfn(x) - f(x)} \leq \norm{\predfn(x) - f(\xi_n)  } + \norm{f(\xi_n) - f(x)} \stackrel{(i)}{=}\norm{\predfn(x) - \predfn(\xi_n)  } + \norm{f(\xi_n) - f(x)}$
$\stackrel{(\dagger)}{\leq} (\bar L+ L^*) \metric_\inspace(x,\xi_n^x )^p + \bar E +\obserrbnd$
$\stackrel{n \to \infty}{\longrightarrow} \bar E +\obserrbnd$.
Here ($\dagger$) leverages the H\"older continuity assumptions. \\

\textbf{(II)} The proof is a trivial extension of (I). Let $\epsilon \geq 0.$ We show $\exists n_0 \in \nat \forall n \geq n_0, x \in \inspace: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon + \bar E +\obserrbnd$.  
Since $G_n$ converges to $I$ uniformly, $\exists n_0 \forall n\geq n_0\forall x \in I: \metric_\inspace(x,\xi_n^x)^p \leq \frac{\epsilon}{2 \max\{\bar L, L^* \}}$. Hold such $n_0$ fixed. Then for all $n \geq n_0, x \in I$ we have 
$\metric_\outspace\bigl(\predfn(x) , f(x)\bigr) \newline \stackrel{(*)}{\leq} (\bar L+ L^*) \metric_\inspace(x,\xi_n^x )^p + \bar E +\obserrbnd \leq \epsilon + \bar E +\obserrbnd$. Here (*) follows from (\ref{ineq:ewlfjhflsape}) and ($\dagger$) in complete analogy to our derivations for case (I) above. 

\textbf{(III)} By assumption of uniform convergence of $\seq{G_n}{n \in \nat}$ with rate $r(n)$, $\sup_{x \in I} \inf_{s_n \in G_n} \metric_{\inspace} (x,s_n) =\sup_{x \in I} \metric_{\inspace} (x,\xi_n^x) \leq r(n)$. The rest follows from (*).
\end{proof}
\end{thm}


%% ============= ONLINE LEARNING CASE IMPORTANT 4 CONTROL


Above theorem considers the case where the data becomes dense in the domain and we are interested in the worst-case prediction error. Relevant to considerations in a setting where online-learning is utilised to control a trajectory $\seq{x_n}{n \in \nat}$ of states is the situation where we are only interested in the error on this specific trajectory in the limit of large time steps $n$. For trajectories on which the prediction error vanishes we will be able to establish convergence of the trajectory to the desired goal state.
In preparation of these considerations, we will establish the following facts:


\begin{lem}
Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs with $x_n \in \inspace$ where input space $\inspace$ can be endowed with a shift-invariant measure. Furthermore, assume the sequence  is bounded, i.e.  
$\metric_\inspace(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
Finally assume the inputs of the available data coincide with the complete history of past inputs, i.e. $G_n = \{ x_i | i \in \nat, i < n\}$.
Then we have: \[ \dist(G_n,x_n) = \min\{\metric_\inspace(g,x_n) | \, g \in G_n\} \stackrel{n \to \infty}{\longrightarrow} 0.\]
\begin{proof}
The intuition behind the following proof is that if the distances were not to converge, there was an infinite number of disjoint balls around the input points that summed up to infinite volume. This however, would be a contradiction to the presupposed boundedness of the sequence.
We formalise this intuition as follows:
We can rephrase the desired convergence statement as 
\begin{equation}
\forall \epsilon > 0 \exists n \in \nat \forall m \geq n : \dist(x_{m}, G_{m}) \leq \epsilon.
\end{equation} 
For contradiction, assume that
\begin{equation}
\exists \epsilon > 0 \forall n \in \nat \exists m(n) \geq n : \dist(x_{m(n)}, G_{m(n)}) > \epsilon.
\end{equation} 
Hold such an $\epsilon >0$ fixed and choose any $n \in \nat$. 
By definition of $G_{m(n)} =\{ x_i | i < m(n)\} $ we have:
\eqn{eq:i34kjjk3}{\forall i < m(n) : \metric_\inspace(x_{m(n)},x_i) > \epsilon.}

Let $C_n := \bigcup_{i < n} \ball{\frac \epsilon 2}{x_i} $ be the union of all $\frac \epsilon 2$-balls around each point in $G_n$ and define $\bar I = \bigcup_{n \in \nat} C_n$.
By definition, each $x_n$ is contained in $\bar I$.
Since sequence $(x_n)_{n \in \nat}$ is bounded, $\bar I $ has a finite volume relative to some positive, shift-invariant measure $\mu$. I.e. $\mu(\bar I) < \infty$ (e.g. choose the Lebesgue measure for $\mu$). Furthermore, $\mu(C_n) \leq \sum_{i <n} \mu(B_i) \leq \mu(\bar I)< \infty$ where $B_i := \ball{\frac \epsilon 2}{x_i}$. Owing to the assumed shift-invariance, we can assign the same measure $M$ each ball, i.e. $M:=\mu(B_1) = \mu(B_n)\forall n \in \nat$. Thus, $\mu(C_n) \leq n M$.
Define $q:= \ceil{\frac{\mu(\bar I)}{M}} \in \nat$. This is an upper bound on the number of disjoint balls of measure $M$  that can be contained in $\bar I$. Intuitively, since this number is finite, there cannot be an infinite number of non-intersecting balls around the elements of the sequence $(x_n)_{n \in \nat}$. More formally our argument proceeds as follows:
Choose $n > q+1$. Statement (\ref{eq:i34kjjk3}) yields:
\eqn{eq:i34kjjk33}{\forall i \in \{1,...,n\} \exists p(i) \geq i \forall j \leq p(i): \metric_\inspace(x_{p(i)},x_j) > \epsilon.}  Define a permutation $\pi$ such that $\pi(p(1)) \leq \ldots \leq \pi(p(n))$. 
With Statement (\ref{eq:i34kjjk33}) it follows that \\
${\metric_\inspace(x_{\pi(p(i))},x_{\pi(p(j))}) > \epsilon}$ , $\forall i,j =1,...,n, i < j$. Thus, we conclude the disjointness conditions $B_{\pi(p(i))} \cap B_{\pi(p(j))} = \emptyset , \forall i,j =1,...,n, i \neq j$. 
Hence,  $\mu(\bar I) \geq \mu(C_{\pi(p(n))}) \geq \mu(C_{\pi(p(1))}) + \sum_{i=1}^n \mu(B_{\pi(p(i))}) \newline = \mu(C_{\pi(p(1))}) +  n M > \mu(C_{\pi(p(1))}) + (q+1) M \geq\mu(C_{\pi(p(1))}) + \mu(\bar I)$, where the last inequality follows from the fact that  $M q= M \ceil{\frac{\mu(\bar I)}{M}} \geq \mu(\bar I)$. Since $\mu(C_{\pi(p(1))}) \geq 0$, we have concluded the false statement $\mu(\bar I) > \mu(\bar I)$.

%Hence, $\mu(\bar I) \geq \mu(C_{\pi(N_n)+1}) = \mu(C_{\pi(N_1)}) + \sum_{i=1}^n \mu(B_{\pi(N_i)}) = \mu(C_{\pi(N_1)}) +  n M > \mu(C_{\pi(N_1)}) + (m+1) M >\mu(C_{\pi(N_1)}) + \mu(\bar I)$ by definition of $m= \ceil{\frac{\mu(\bar I)}{M}}$. But since $\mu(C_{\pi(N_1)}) \geq 0$, we conclude the false statement $\mu(\bar I) > \mu(\bar I)$.
\end{proof}
\label{lem:bndseq_entails_distgridvanish}
\end{lem} 


\begin{lem}
As before, let the observational noise level be bounded by $\obserr$ and assume the output- space pseudo-metric to be translation-invariant. Assume the predictors $\predfn(\cdot)$ all are H\"older with H\"older constants bounded from above by some number $\bar L \in \Real_+$. 
Furthermore, we assume sample-consistency up to error $E$ (cf. Def. \ref{def:sampleconsistency}) where we assume bounded prediction errors $E_s = E + \obserrbnd$ (cf. Lem. \ref{lem:groups_sampleconsandobserr}) at sample inputs with $\sup_x E_s(x) \leq \bar E_s \in \Real$.
For some $L^* \in \Real_+, p \in [0,1]$, let target $f$ be $L^*-p$-H\"older up to error $E_h$. That is, there is an $L^*-p$-H\"older function $\phi \in \hoelset {L^*} { } p$ and a function $\psi$ such that $\forall x: f(x) = \phi(x)+\psi(x), \, \sup_x \metric_\outspace\bigl(0,\psi(x)\bigr) \leq \bar E_h \in \Real$.

Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs that is bounded, i.e. where 
$\metric_\inspace(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
Furthermore, assume $\data_{n+1} = \data_n \cup \{ \bigl(x_n, \tilde f(x_n)\bigr) \}$ and thus, $G_n = \{ x_i | i \in \nat, i < n\}$.
Then the prediction error on the sequence vanishes up to the level of sample-consistency and H\"older continuity in the following sense:
 \[\metric_\outspace\bigl(\predfn(x_n),f(x_n) \bigr) \stackrel{n \to \infty}{\longrightarrow} [0,\bar  E_s + 2 \bar E_h].\]
In particular, in case the observations are error-free ($\tilde f = f$) and assuming the target is H\"older continuous then the prediction error vanishes. That is,
\[\metric_\outspace\bigl(\predfn(x_n),f(x_n) \bigr) \stackrel{n \to \infty}{\longrightarrow}0.\]
\begin{proof}

Let $\xi_n := \argmin_{g \in G_n} \metric_\inspace(x_n,g)$ denote the nearest neighbour of $x_n$ in $G_n = \{x_1,...,x_{n-1}\}$.
We have assumed that $\predfn$ is $L(n)-p$- H\"older with $L(n) \leq \bar L$ for some $\bar L \in \Real_{\geq 0}$.
Since sequence $(x_n)$ is bounded, Lem. \ref{lem:bndseq_entails_distgridvanish} is applicable. 
Hence, $\forall n \in \nat: \metric_\inspace (x_n,\xi_n) \to 0$ as $n \to \infty$.

Let $y \in \outspace$ such that $\predfn(\xi_n) + y = f(\xi_n)$. The sample-consistency assumption renders Lem. \ref{lem:groups_sampleconsandobserr} applicable, allowing us to conclude that 
$\metric_\outspace\bigl(\predfn(\xi_n) ,  f(\xi_n)  \bigr) \leq \obserrbnd + E(\xi_n)$. Hence, by Lem. \ref{lem:bilinaddtransinvgroup}.(III), $\metric_\outspace(0,y) \leq \obserrbnd + E(\xi_n)$. Appealing to Lem. \ref{lem:bilinaddtransinvgroup}.(I), we see that 
$\metric_\outspace\bigl(\predfn(x_n) ,  f(\xi_n)  \bigr) \leq \metric_\outspace\bigl(\predfn(x_n) ,  \predfn(\xi_n)+y  \bigr) \leq 
\metric_\outspace\bigl(\predfn(x_n) ,  \predfn(\xi_n) \bigr) + \metric_\outspace(0,y)$. Thus, 

$(i) \,\,\,\, \metric_\outspace\bigl(\predfn(x_n) ,  f(\xi_n)  \bigr) \leq \metric_\outspace\bigl(\predfn(x_n) ,  \predfn(\xi_n) \bigr) + \obserrbnd + E(\xi_n)$.



Moreover: $(ii)$ There is a maximal constant $\bar L \in \Real$, such that for any $n \in \nat $, the predictor $\predfn$ is $L(n)-p$-H\"older with $L(n) \leq \bar L$. 
  
In conclusion,
$0\leq\metric_\outspace\bigl(\predfn(x_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) ,  f(\xi_n)  \bigr) + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \stackrel{(i)}{\leq}\metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) + \obserrbnd + E(\xi_n) + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) +\obserrbnd + E(\xi_n) + \metric_\outspace\bigl(\phi(\xi_n) , \phi(x_n)\bigr) + 2 \bar E_h 
\newline
\stackrel{(ii)}{\leq} (\bar L+ L^* ) \metric_\inspace(x_n,\xi_n )^p + \obserrbnd + E(\xi_n) + 2 \bar E_h \stackrel{(ii)}{\leq} (\bar L+ L^* ) \metric_\inspace(x_n,\xi_n )^p + \bar E_s + 2 \bar E_h \stackrel{n \to \infty}{\longrightarrow} \bar E_s + 2 \bar E_h $.
\end{proof}
\label{lem:vanisishingseqprederr_groups}
\end{lem} 



==> content2/hoelder_BG.tex <==
\subsection{H\"older and Lipschitz continuity for inference}%\label{sec:HoeldNLipfacts}
\label{sec:Hoelder_brief}
\subsubsection{Introduction and related work}



H\"older continuous functions are uniformly continuous functions that may exhibit infinitely many points of non-differentiability and yet are sufficiently regular to facilitate inference. That is, they have properties that make it possible to make assertions of global properties on the basis of a finite function sample. 

H\"older continuity is a generalisation of Lipschitz continuity.  Lipschitz properties are widely used in applied mathematics to establish error bounds and, among many other, find application in optimisation \cite{Shubert:72,direct:93} and quadrature \cite{Baran2008,curbera1998,dereich2006} and are a key property to establish convergence properties of approximation rules in (stochastic) differential equations \cite{kloedenandplaten1992,Gardiner2009}. 
Furthermore, most machine learning methods for function interpolation seem to impose smoothness (and thereby, H\"older continuity) on the function. For instance, with our Lem. \ref{lem:Hoeldarithmetic} derived below, it would be possible to show that any finite \textit{radial basis function neural network} \cite{Broomhead1988} with a smooth basis function is H\"older continuous on a compact domain. Or, a \textit{Gaussian process} with a smooth covariance function also has a smooth mean function and a.s. smooth sample paths  \cite{GPbook:2006,grimmetbook2001}. Therefore, posterior inference over functions on compact support made with such a Gaussian process on the basis of a finite sample is H\"older continuous. 


Recently, we have become aware of related work published in mathematical and operations research journals \cite{Cooper2006,Cooper1995,Zabinsky2003,Beliakov2006,Beliakovsmoothing2007}. For instance, Zabinsky et. al. \cite{Zabinsky2003} consider the problem of estimating a one-dimensional Lipschitz function (with respect to the canonical norm-induced metric). Similar to the analysis we employ to establish our guarantees, they use a pair of bounding functions and make predictions by taking the average of these functions. While we have developed our kinky inference rule independently, it can be seen as a generalisation of their approach. Our method provides extensions to H\"older continuous multi-output functions over general, multi-dimensional (pseudo-) metric spaces, can cope with with erroneous observations and inputs, can fold in additional knowledge about boundedness, learn parameters from data and provides different guarantees such as (uniform) convergence of the prediction uncertainty. 
As part of the analysis of our method, we construct delimiting functions we refer to as \textit{ceiling} and \textit{floor} functions. The construction of similar functions is a recurring theme that, in the standard Lipschitz context, can be found in global  optimisation \cite{Shubert:72}, quadrature \cite{Baran2008}, interpolation \cite{Beliakov2006,Beliakovsmoothing2007}, as well as in the analysis of linear splines for function estimation \cite{Cooper1995}. Cooper \cite{Cooper2006,Cooper1995} utilises such upper and lower bound functions in a multi-dimensional setting to derive probabilistic PAC-type error bounds \cite{Valiant1984} for a linear interpolation rule. He assumes the data is sampled uniformly at random on a hypercube domain. This precludes the application of his results to much of our control applications where the data normally is collected along continuous trajectories visited by a controlled plant. Our inference rule is different from his and our guarantees do not rely on distributional assumptions. This of course is important in control settings where the common assumption that the input data was drawn independently from a fixed distribution typically is not met.
%As a special case of our kinky inference framework, we consider a case, called \textit{kNN-KI}. Here, the inference over function values is based on up to (approximate) k nearest neighbours aiming to reduce computational prediction effort to log-time. Approaches to this end include maintaining a data structure for fast nearest neighbour search \cite{Bentleykdtree:1975} or utilising locally sensitive hash functions \cite{RusselNorvigbook2009}. 
In this thread of works, perhaps the work that is most closely related to ours is the function interpolation method of Beliakov \cite{Beliakov2006} that is a special case of a kinky inference rule: For a single-output function that is Lipschitz with respect to a special input space norm and where the data is error-free, the authour provides an algorithm that promises logarithmic prediction time. Unfortunately, many of his assumptions are unrealistic in a control setting. And, the improved prediction time is achieved by constructing a data structure from batch data which precludes its use in an online learning setting. However, future work might explore in how far his ideas can be 
converted into an online learning rule. Furthermore, in learning situations where Beliakov's interpolation method is applicable, our theoretical results extend to his work. For instance, our results show how Lipschitz constant estimation can be harnessed to render his approach a universal approximator.

Other work of relevance can be found in analysis. For instance, Miculescu \cite{Miculescu2000} presents work proving that any continuous function on a metric space is a uniform limit of a sequence of \emph{locally} Lipschitz functions and also mentions that the stronger statement, that every function is a limit of a sequence of globally Lipschitz functions, is not true in general. However, he cites earlier work \cite{Georganopoulos1967} that does show that every real-valued continuous function on \emph{compact} domain is a uniform limit of a sequence of Lipschitz functions. In some sense, our work develops a related statement as a by-product. 
From our convergence guarantee of the LACKI rule, we have derived constructive method for showing 
that any continuous function on compact domain is the uniform limit of a sequence of H\"older functions up to an arbitrarily small error.

Finally, in the context of control, Milanese and Novara \cite{Milanese2004} considered NSM methods for interpolation. For a fixed Lipschitz constant, their prediction rule can be
seen as a special case of ours without the $\lbf$ and $\ubf$ parameters and with special choices of metrics. Similar to us, they do consider the problem of estimating the Lipschitz constant from the data and consider bounded noise. However, they obtain the Lipschitz constant estimate via the maximum partial derivative of an arbitrarily chosen fitted parametric model of a bounded input set. And, they give no guarantees on the quality of the resulting estimator that is fitted to the data like this nor do they discuss the impact of the choice of parametric model or the fitting method on the quality of the estimator.
 
%\jcom{Need to read \cite{Georganopoulos1967}}
%\jcom{Need to reassess the following in the light of the newly found control paper:}
%None of the aforementioned works seems to consider interval-bounded input uncertainty and observational errors, fold in additional knowledge such as boundedness or considers inference over multi-output functions as we do. Most importantly the combination with our online constant estimation rule, leading to our LACKI inference rule, as well as our universal approximation guarantees are novel.
%Finally, we are not aware of any work that employs H\"older-based methods in the context of model-reference adaptive control. 


%In particular, we will look into the inference problems of bounded optimisation and quadrature. That is, based on the knowledge of a sample of a H\"older continuous function we will derive upper and lower bounds on its maximum, minimum and definite Riemann integral. In addition we will touch upon adaptive algorithms that can utilise knowledge of the function's H\"older properties to guide exploration. That is, since the regularity of the function allows us to provide interval bounds on the uncertainty of the function, the magnitude of the uncertainty can be a guide to identify regions that are to be sampled next in order to maximise the shrinkage of the provided error bounds. 
%\jcom{The latter is more the 1-dim case, which I may or may not include}\\

\subsubsection{Basic facts and derivations}
In preparation of subsequent parts of the work that take advantage of H\"older properties this section will proceed to establish essential prerequisites.
The remainder of this section is structured as follows: Firstly, we will go over basic definitions and engage in some preliminary derivations that will be of importance throughout this work.
While we do not claim novelty on any of the results we provide proofs for in this section, we had not found them in the literature and hence, had to derive them on our own.

Firstly, we commence with introducing the notions of (pseudo-) metric spaces.

\begin{defn}[(Pseudo-) metrics]
Let $\inspace$ be a set. A mapping $\metric_\inspace: \inspace^2 \to \Real$ is called a \emph{pseudo-metric} if it positive ($\forall x,x' \in \inspace: \metric_\inspace(x,x') \geq 0$) and satisfies the triangle inequality ($\forall x,x',x'' \in \inspace: \metric(x,x') \leq \metric_\inspace(x,x'') + \metric (x'',x')$). If furthermore the pseudo-metric $\metric$ is definite $(i.e. \forall x,x' \in \inspace_\inspace: \metric_\inspace(x,x') =0 \Leftrightarrow x=x')$ then 
the mapping $\metric$ is called a \emph{metric}. The set $\inspace$ endowed with a (pseudo-) metric $\metric_\inspace: \inspace^2 \to \Real$ or the pair $(\inspace, \metric_\inspace)$ are called \emph{(pseudo-) metric space}.
 \end{defn}

\begin{defn} 
Let $(\inspace ,\metric_\inspace ), (\outspace , \metric_\outspace )$ be two (pseudo-) metric spaces and 
$I \subset \inspace$ be an open set. A function $f: \inspace \to \outspace $ is called (L-p-) \emph{H\"older} 
(continuous) on $I \subset \inspace$ if there exists a \emph{(H\"older) constant} $L \geq 0$ and \emph{(H\"older) 
exponent} $p\geq 0$ such that 
\[\forall x,x' \in I : \metric_\outspace \bigl(f(x),f(x')\bigr) \leq L \, \bigl( \metric_\inspace (x,x') \bigr)^p. \]
We denote the space of all L-p- H\"older functions by $\hoelset{L}{}{p}$.
\end{defn}

H\"older functions are known to be uniformly continuous. 
A special case of importance is the class of $L$-\textit{Lipschitz} functions. These are H\"older continuous 
functions with exponent $p=1$. In this context, coefficient $L$ is referred to as\textit{ Lipschitz constant} or \textit{Lipschitz number}.

\begin{ex}[Square root function]\label{ex:sqrtfctHoelder}
As an example of a H\"older function that is not Lipschitz we can consider $x \mapsto \sqrt x$ on domain $I = [0+\epsilon,c]$ where 
$c >\epsilon \geq 0 $. For $\epsilon >0 $ the function is Lipschitz with $L = \sup_{x \in I} \frac{1} {2 \sqrt{x}}$. We can see that the 
coefficient grows infinitely large as $\epsilon \to 0$. By contrast, the function is H\"older continuous 
with H\"older coefficient $L=1$ and exponent $p=\frac 1 2 $ for any bounded $I \subset \Real$.
We can see this as follows: Let $\epsilon =0,$ $x,y \in I$ and, without loss of generality,  $y \geq x$. Let $\xi := \sqrt{x}, \gamma := \sqrt{y}$ and thus, $\gamma \geq \xi$. We have:
$\xi \leq \gamma $ $\Leftrightarrow 2 \xi^2 \leq 2\xi\gamma$ $\Leftrightarrow \gamma^2 - 2 \xi\gamma + \xi^2  \leq \gamma^2 - \xi^2$ $\Leftrightarrow (\gamma-\xi)^2  \leq \gamma^2-\xi^2$ $\Leftrightarrow \abs{\gamma-\xi}^2  \leq \abs{\gamma^2-\xi^2}$
$\Leftrightarrow \abs{\gamma-\xi}  \leq \sqrt{\abs{\gamma^2-\xi^2}}$  $\Leftrightarrow \abs{\sqrt{x}-\sqrt{y}} \leq \abs{y-x}^{\frac{1}{2}}$. Since, $x,y$ were chosen arbitrarily, we have shown H\"older continuity as desired.
\end{ex}

Most commonly, one considers H\"older continuity for the special case of the standard metric induced by a norm, i.e.  $\metric(x,x') = \norm{x-x'}$.
For a function $f: \inspace \to \outspace$, the H\"older condition becomes:
\[\forall x,x' \in I : \norm{f(x)-f(x')}_\outspace \leq L \, \norm{x-x'}_\inspace^p. \]

Similarly, we can consider H\"older continuity for each output component: 

\begin{defn} \label{def:outputwisehoelder}
Let $\outspace \subseteq \Real^m $ and $\inspace$ be a space endowed with a metric (or indeed a semi-metric) $\metric_\inspace$. Then, the function $f: \inspace \to \outspace$ is output-component-wise H\"older continuous with exponent $p$ and constant $L \in \Real^m_{\geq 0}$ if $f \in \hoelset L { } p$ where
$\hoelset L {\metric_\inspace} p:= \bigl\{ \phi: \inspace \to \outspace \,\ | \, \forall j \in \{1,...,m \}, \forall x,x' \in \inspace: \abs{\phi_j(x) - \phi_j(x')} \leq L_j \metric^p_\inspace(x,x') \bigr\}$
is the set of all functions whose component functions are H\"older continuous with respect to input space metric $\metric_\inspace$ and an output space metric that is induced by the canonical norm $\metric_{\outspace} (x,x')= \abs{x-x'}$.  
\end{defn}

\begin{remark}[Best H\"older constant]
Note for $p \in (0,1], 0 \leq L_1 \leq L_2$ we have $\hoelset {L_1} {\metric_\inspace} p \subseteq \hoelset {L_2} { } p$. The smallest $L^* \geq 0$ such that function if is $L^*-p-$ H\"older, $f \in \hoelset {L^*} {\metric_\inspace} p$, is called the \emph{best} H\"older constant of $f$.
\end{remark}

Generally, it is obviously true that $\hoelset{L}{}{p} \subseteq \hoelset{L'}{}{p}$ for $L' \geq L$.
With regard to the H\"older exponent, we will now show that smaller exponents are less restrictive than larger ones. 




\begin{lem} \label{lem:hoeldexpprop2}
Let $\inspace$ be the input space (not necessarily bounded). For some $p \in (0,1], L \geq 0$ assume that  and $f:\inspace \to \outspace$ is locally $L-p$-H\"older continuous.
Then we have: (i) for any $ q \in (0,p]$, f is also locally $L-q$-H\"older. 
(ii) If $f:\inspace \to \outspace$ is bounded with $\sup_{x,x' \in \inspace} \metric_\outspace (f(x),f(x')) \leq B \in \Real$ and globally $L-p$ H\"older then $f$ is globally $L^*-q$-H\"older, where $L^* := \max\{L,B \}$ and $q \in (0,p]$. In particular, on compact support, Lipschitz continuity entails \emph{H\"older} continuity for any H\"older exponent $p \in [0,1)$.
\begin{proof}
(i) Let $p \in (0,1], f \in \hoelset L { } p $ and $p = q+r, r \in [0,1)$. Let $\xi \in \inspace$ and $I$ denote the intersection of the domain with an $\epsilon$-ball around $\xi$ such that $f$ satisfies the H\"older condition on $I$ and such that $\sup_{x,x' \in I} \metric_\inspace(x,x') \leq 1$.  For all $x,x' \in I$ we have $\metric_\outspace (f(x),f(x')) \leq L\metric_\inspace^p (x,x') = L \metric_\inspace^q(x,x') \metric_\inspace^r(x,x') \leq L \metric_\inspace^q(x,x')$ where the last inequality holds since $r \in [0,1)$ and $\sup_{x,x' \in I} \metric_\inspace(x,x') \leq 1$.

(ii) Let $x,x' \in \inspace$. If $\metric_\inspace(x,x') \leq 1$ we can show $\metric_\outspace (f(x),f(x'))  \leq L \metric_\inspace^q(x,x')$ following through the same sequence of inequalities as above in the proof of (i). Now, let $\metric(x',x) >1$. We have $\metric_\outspace (f(x),f(x')) \leq B \leq B  \metric_\inspace(x,x')^q$.
\end{proof}
\end{lem}

%Note for compact domains local H\"older continuity implies global H\"older continuity with the same parameters. Therefore Lem. \ref{lem:hoeldexpprop1} would also be implied 
%by Lem. \ref{lem:hoeldexpprop2}.(i) in cases where $\inspace$ is compact.



%We conclude this section by the following theorem stating that any concatenation of H\"older continuous functions is H\"older continuous:
%
%\begin{thm} \label{thm:concathoelder}
%Let $(\statespace, \metric)$ be a metric space and $f,g : \statespace \to \statespace$ be two H\"older continuous mappings with H\"older constants $L_f, L_g$ and H\"older exponents $p_f,p_g$, respectively.
%Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also H\"older continuous with H\"older constant $L_h:= L_f L_g^{p_f}$ and exponent $p_h:=p_g \, p_f$.
%That is, 
%\[\forall \state,\state' \in \statespace: \metric\bigl(h(\state),h(\state')\bigr) \leq L_h \bigl(\metric(\state,\state')\bigr)^{p_h}.\]
%\begin{proof}
%%\begin{align}
%$\metric\bigl(f \circ g(\state),f\circ g(\state')\bigr) \leq L_f  \Bigl(\metric(g(\state),g(\state'))\Bigr)^{p_f}$
%$\leq L_f  \Bigl(L_g \metric(\state,\state')^{p_g}\Bigr)^{p_f}$ $= L_f L_g^{p_f}   \Bigl(\metric(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using H\"older continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
%
%\end{proof}
%\end{thm} 
%In conjunction with H\"older properties of the square root function established in Ex. \ref{ex:sqrtfctHoelder}, Thm. 
%\ref{thm:concathoelder} immediately yields the following result:
%\begin{cor}
%If $f: \statespace \to \statespace $ is H\"older continuous with constant $L_f$ and exponent $p_f$ then $\sqrt{f}$ also is Hoelder, having  H\"older constant $\sqrt{L_f}$ and exponent $p_f$.
%\end{cor}


\begin{thm} \label{thm:hoelderconcat}
Let $(\statespace, \d)$ be a metric space and $f,g : \statespace \to \statespace$ be two H\"older continuous mappings with H\"older constants $L(f), L(g)$ and H\"older exponents $p_f,p_g$, respectively.
Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also H\"older continuous with H\"older constant $L(h):= L(f) L(g)^{p_f}$ and exponent $p_h:=p_g \, p_f$.
That is, 
\[\forall \state,\state' \in \statespace: \d\bigl(h(\state),h(\state')\bigr) \leq L(h) \, \bigl(\d(\state,\state')\bigr)^{p_h}.\]
\begin{proof}
%\begin{align}
$\d\bigl(f \circ g(\state),f\circ g(\state')\bigr)$ $\leq L(f)\,  \Bigl(\d(g(\state),g(\state'))\Bigr)^{p_f}$
$\leq L(f)\,  \Bigl(L(g)\, \d(\state,\state')^{p_g}\Bigr)^{p_f}$ 

$= L(f)\, L(g)\,^{p_f}   \Bigl(\d(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using H\"older-continuity of $f$ and in the second, we were using H\"older continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
\end{proof}
\end{thm} 






%A special case of H\"older continuity is Lipschitz continuity. A Lipschitz continuous function is H\"older continuous with exponent 1.
%If the metric space is $(\Real,(x,y) \mapsto \abs{x-y})$, $f$ is Lipschitz with constant $L(f)$ if $\forall t,t': \abs{f(t)-f(t')} \leq L(f) \, \abs{t-t'}$. 

Several numerical methods, such as Lipschitz optimisation \cite{Shubert:72}, rely on the knowledge of a Lipschitz constant. In the more general case of H\"older continuous functions this will correspond to the need of knowing a H\"older constant and exponent. To avoid having to derive these for each new function from first principles, we establish the following collection of facts that allows us determine bounds on H\"older constants of combinations of functions with known H\"older parameters.
While we provide proofs for a restatement in the H\"older continuous setting, a number of the following statements have also been proven in \cite{Weaver1999} in the context of Lipschitz algebras.





\begin{lem}[H\"older arithmetic] \label{lem:Hoeldarithmetic}
Let, $I,J \subset \inspace$ where $\inspace$ is a metric space endowed with metric $\metric$. Let $f : \inspace \to \Real$ be H\"older on $I$ with constant $L_I (f) \in \Real_+$ 
and $g :\inspace \to \Real$ be H\"older on $J$ with constant $L_J (g) \in \Real_+$. Assume both functions have the same H\"older exponent $p \in (0,1]$. That is, $\forall x, x' \in \inspace: \abs{f(x)-f(x')} \leq L(f) \metric(x,x')^p$ and  $\forall x, x' \in \inspace: \abs{g(x)-g(x')} \leq L(g)  \metric(x,x')^p$.
We have:

\begin{enumerate}
	\item Mapping $x \mapsto |f(x)|$ is H\"older on $I$ with constant $L_I(f)$ and exponent $p_f$.
	\item If $g$ is H\"older on all of $J=f(I)$ the concatenation $g \circ f: t \mapsto g(f(t))$ is H\"older on $I$ with constant 
	      $L_I(g \circ f) \leq$ $L_J (g) \, L_I^p(f)$ and exponent $p^2$.
	\item Let $r \in \Real$. $r \, f: x \mapsto r \, f(x)$ is H\"older on $I$ having a constant $L_I (r \,f) = |r| \, L_I(f)$.
	\item $f+g: x \mapsto f(x) + g(x)$ has H\"older constant at most $L_I(f) + L_J(g)$.
	\item Let $m_f = \sup_{x\in \inspace } f(x)$ and $m_g = \sup_{x \in \inspace } g(x)$. Product function $f\cdot g: x \mapsto f(x) \, g(x)$ has H\"older exponent $p$ and a H\"older constant on $I$ which is at most $(m_f \, L_J(g)+ m_g \, L_I(f))$.
	%\item Let $\tilde h(x) = \min\{f(x),g(x) \}$, $h(x) = \max\{f(x), g(x) \}, \forall x \in \inspace  \cap J$. We have $L_{I \cap J}(h) \leq \max\{L_I(f),L_J(g)\}$ and $L_{I \cap J}(\tilde h) \leq \max\{L_I(f),L_J(g)\}$.	
	\item For some countable index set $\indsett$, let the sequence of functions $f_i$ be H\"older with exponent $p$ and constant $L(f_i)$ each. Furthermore, let $H(x) =\sup_{i \in \indsett} f_i(x) $ and $h(x) := \inf_{i \in \indsett} f_i(x)$ be finite for all $x$. Then $H,h$ are also H\"older with exponent $p$ and have a H\"older constant which is at most $\sup_{i \in \indsett} L(f_i)$.
	\item Let $b := \inf_{x \in \inspace }| f(x)| > 0$ and let 
	$\phi(x) = \frac{1}{f(x)}, \forall x \in \inspace$ be well-defined.  
	      Then $L_I(\phi) \leq b^{-2} \, L_I(f)$.  
	\item Let $p=1$ (that is we consider the Lipschitz case), let $I$ be convex and $\metric(x,x') = \norm{x-x'}$ where $\norm{\cdot}$ is a norm that induces a sub-multiplicative matrix norm (e.g. all $p-$ norms are valid). $f$ cont. differentiable on I $\Rightarrow$ $L_I(f) \leq \sup_{x \in I } \norm{\nabla f(x)}. $ 
	For one-dimensional input space, $\inspace = \Real$, $L_I(f) = \sup_{x \in I } \abs{\nabla f(x)}$ is the smallest Lipschitz number. 
	 \item Let $c \in \Real$, $f( t) = c, \forall x \in I $. Then $f$ is H\"older continuous with constant $L_I(f) =0$ and for any coefficient $p_f \in \Real$.  
	\item $L_I(f^2) \leq 2 \, L_I(f)\, \sup_{t \in I} f\,$.
	\item With conditions as in 8), and input space dimension one, we have $\forall q \in \mathbb Q : L_I(f^q) = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $.
\end{enumerate}
\begin{proof}

\textbf{1)}  We show $|f|$ has the same constant and exponent as $f$. Let $X,X' \in \inspace $ arbitrary. 
We enter a case differentiation:

\textit{1st case: $f(x), f(x') \geq 0$}. 

Hence, $\bigl| \abs{f(x)}- \abs{f(x')} \bigr| = \bigl| f(x) - f(x') \bigr|  \stackrel{f \,Hoelder}{\leq} L_I(f) \metric(x,x')^{p}$.\\

\textit{2nd case: $f(x) \geq 0, f(x') \leq 0$.} 

Note, $|y| = - y$, iff $y \leq 0$. Hence,  $\bigl| |f(x)| - |f(x')| \bigr| \leq \bigl| |f(x)| + |f(x')| \bigr| $
$= \bigl| |f(x)| - f(x') \bigr|  =  \bigl| f(x) - f(x') \bigr| \leq L_I(f) \, \metric(x,x')^{p}$.\\

\textit{3rd case: $f(x) \leq 0, f(x') \geq 0$.} Completely analogous to the second case.\\

\textit{4th case: $f(x), f(x') \leq 0$}. 

$\bigl| |f(x)| - |f(x')| \bigr| = \bigl| f(x') - f(x) \bigr|= \bigl| f(x) - f(x') \bigr|  \stackrel{f \, Hoelder}{\leq} L_I(f) \metric(x,x')^{p}$.\\

The remaining points are also proven in \cite{Weaver1999} in the context of Lipschitz functions.

\textbf{2)} Special case of Thm. \ref{thm:hoelderconcat}.
% For arbitrary $t,t' \in \indset $ we have:
%
%$\bigl| g(f(t)) - g(f(t'))| \bigr| \leq L_J(g) \, |f(t) - f(t') | \leq L_J(g) \, L_I(f)\, |t-t'|$ 
%where the two inequalities are due to the Lipschitz properties of $g$ and $f$, respectively.\\

\textbf{3)}  For arbitrary $x,x' \in \inspace , r \in \Real$ we have:

$\bigl| r \, f(x) - r \, f(x')| \bigr| = |r|\, |f(x) - f(x')| \leq |r| \,L_I(f)\,  \metric(x,x')^{p}$.\\ 

\textbf{4)}  For arbitrary $x,x' \in \inspace , r \in \Real$ we have:

$\bigl| g(x) + f(x) - (g(x') + f(x'))| \bigr| = \bigl| g(x)  - g(x') + f(x)- f(x')| \bigr|$ 
$\leq \bigl| g(x)  - g(x')\bigr|  + \bigl| f(x)- f(x')| \bigr|$ $\leq (L_J(g)+L_I(f))\,  \metric(x,x')^{p}$.\\

\textbf{5)}  Let  $x,x' \in \inspace $, $d := f(t) - f(t')$.

$\bigl| g(x) f(x) - g(x')  f(x') \bigr| = \bigl| g(x) (f(x') +d) - g(x') f(x') \bigr|$ 
$= \bigl|\bigl( g(x) - g(x') \bigl)  f(x')+ g(x)  d \bigr|  $

$\leq \bigl| g(x) - g(x') \bigr|  |f(x')|   + \bigl|g(x)\bigr| \,  |d|  $
$\leq L_I(g) \metric(x,x')^p  |f(x')|   + \bigl|g(x)\bigr| \,  L_I(f) \metric(x,x')^p  $

$\leq L_I(g) \metric(x,x')^p  \sup_{x' \in \inspace } \{|f(x')|\}  \\ + \sup_{x \in \inspace }\{\bigl|g(x)\bigr|\} \,  L_I(f) \metric(x,x')^p  $

$= \Bigl(L_I(g)  \sup_{x' \in \inspace } \{|f(x')|\}   \\+ \sup_{x \in \inspace }\{\bigl|g(x)\bigr|\} \,  L_I(f)\Bigl) \metric(x,x')^p  $.\\

\textbf{6)}  The proof of Proposition 1.5.5 in \cite{Weaver1999} proves our statement if one replaces their 
metric $\rho$ by $\metric^p$.

\textbf{7)}  Let  $x,x' \in \inspace $.
$\bigl| \frac{1}{f(x)} - \frac{1}{f(x')} \bigr|$ 
$=\bigl| \frac{f(x')}{f(x') f(x)} -\frac{f(x)}{f(x') f(x)} \bigr|$ 
$= \frac{\bigl|f(x')-f(x) \bigr|}{\bigl|f(x')\bigr| \bigr| f(x)\bigr|}$ 
$\leq \frac{L_I(f) \metric(x,x')^p}{\inf_{x \in \inspace } |f(x)|^2}$.\\

\textbf{8)} Let $p=1$ and $\metric(x,x') = \norm{x-x'}$ be a norm that induces a sub-multiplicative matrix norm. Define $\ell := \sup_{x \in I } \norm{ \nabla f(x) } = L_I(f)$. 
Firstly, we show that it is a Lipschitz constant: Let $x,x' \in I $ and 
$\overline{xx'} := \{tx + (1-t) x' \, | \, t \in [0,1]\}$. 
%$\overline{xx'} := \{y | \exists t \in [0,1] : y = tx + (1-t) x'\}$. 
Owing to convexity of I, $\overline{xx'} \subset I$. Due to the mean value theorem $\exists \xi \in \overline{xx'} \subset I: |f(x) - f(x')|=  T_\xi (x-x')$. where $T_\xi (x) = \SP{\nabla f(\xi)}{ x}$ is a linear OP. Assuming the derivative of $f$ is bounded, $T_\xi$ is a bounded OP and we have $\abs{T_\xi (x-x') } \leq \matnorm{T_\xi} \norm{x-x'}$ where 
$\matnorm{T_\xi} = \sup_{\norm{x} = 1} \abs{\SP{\nabla f(\xi)}{x}} \leq \norm{\nabla f(\xi)}$. In conjunction,
$|f(x) - f(x')| \leq \norm{\nabla f(\xi)} \norm{x-x'}$. 

Secondly, we show that $\ell$ is the smallest Lipschitz constant in the one-dimensional case: Let $\bar \ell$ be another Lipschitz constant on $I$ such that $\bar \ell \leq \ell$. Of course, here $\norm{\cdot} = \abs{\cdot}$. Since $I$ is compact and $\norm{\nabla f(\cdot) }$ is continuous, there is some $\xi \in I$ such that $\norm{\nabla f(\xi)} = \sup_{x \in I} \norm{\nabla f(\xi)} = \ell$. Pick any sequence $(y_k)_{k=1}^\infty$ contained in $I$ such that $y_k \stackrel{k \to \infty}{\longrightarrow} \xi$ and $y_k \neq \xi$.
$\forall k: y_k \in I $ and $\bar \ell$ is a Lipschitz constant on $I$. Hence, $ \bar \ell \geq \frac{|f(y_k) - f(\xi)|}{\norm{y_k-\xi}}\stackrel{k \to \infty}{\longrightarrow} \norm{ \nabla f(\xi)} = \ell$. Thus, $\bar \ell = \ell$.

\textbf{9)} Trivial. 

\textbf{10)} Special case of property 5).

\textbf{11)} $L(f^q) \stackrel{8)}{=} \sup_{\tau \in \indset } |\dif{}{t} f^q(\tau)| = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $. 
\end{proof}
\end{lem} 

As a simple illustration, assume we desire to establish that $f(t) = \max\{ 1- 3 \sin(t), \exp\bigl(- \sin(t) \bigr)\}$ is Lipschitz and to find a Lipschitz number on $\Real$. Application of 8. shows that $t \mapsto \sin(t)$ and $t \mapsto \exp(- t)$ have a Lipschitz number of $1$. Application, of 2., 9. 1. and 6. then show that $L(f) =3$ is a Lipschitz number of $f$.


%As another example we consider the standard deviation of the Ornstein-Uhlenbeck process:
%\begin{ex} \label{ex:hoelderOUstd}
%Consider the function $h(t) = f \circ g(t)$ where $f(\cdot) = \sqrt \cdot$ is the square root function and $g(t) = \frac{B^2}{2 K} (1- \fexp{-2Kt}) $, $K >0$. $g$ is the non-stationary factor of the variance trajectory of an Ornstein-Uhlenbeck process (cf. Sec. \ref{sec:OUprocess}). We show that $h$ is H\"older and has constant $L(h)= \sqrt{2K}$ and H\"older exponent $p_h = \frac 1 2$. This can be easily done by applying Lem. \ref{lem:Hoeldarithmetic}.8 to show that $L(g)$ is Lipschitz with constant $L(g) = B^2 $ and then combining the H\"older constant and exponent derived in Ex. \ref{ex:sqrtfctHoelder} with Thm. \ref{thm:hoelderconcat} to yield the H\"older exponent $p_h = p_g p_f = \frac 1 2$ and constant $L(h) = 1 \sqrt{L(g)}  = \abs B$.  
%\end{ex}

%An example important to our considerations above is the establishment of Lipschitz bounds of an RBFN:
%\begin{ex} \label{ex:hoelderRBFN}

%\end{ex}

\subsection{H\"older continuity of the exponentiated map }

 %
The main objective of this subsection is to show that, for each $s \in \inspace$, the function $\phi_s: x \mapsto L \metric(x,s)^p$ is H\"older continuous with coefficient $L$ and exponent $p$ with respect to (pseudo-) metric $\metric: \inspace^2 \to \Real$. This is important in our derivations since these maps are essential building blocks of the kinky inference procedure. Therefore it is easy to employ Lem. \ref{lem:Hoeldarithmetic} to show that the full kinky inference rule is H\"older continuous.

To establish the H\"older regularity result, we will first show that $(x,y) \mapsto \metric(x,y)^p$, for $p \in (0,1] $, is a metric.  This can be utilised to show that
$\phi_s \in \hoelset L \metric p$.




Before proceeding we need to establish a few facts. 
Firstly, we remind ourselves of the following well-known fact:
\begin{lem} \label{lem:pd_n_concave_subadditive}
A nonnegative, concave function $g:\Real_{\geq 0} \to \Real$ with $g(0) = 0$ is subadditive. 
That is, $\forall x,y \in \Real_{\geq 0}: g(x+y) \leq g(x) + g(y)$. 
 \begin{proof}
If $x = y = 0$ then subadditivity trivally holds:  $0=g(x+y) \leq g(x) + g(y) = 0$.
So, let $x, y \in \Real_+$ such that $x >0 \vee y >0$.
We have, $g( x +y) = \frac{x}{x+y} g(x+y) + \frac{y}{x+y} g(x+y) \leq g(\frac{x}{x+y} (x+y) ) +  g(\frac{y}{x+y}(x+y)) = g(x) + g(y)$.
Taking into account that $\frac{x}{x+y}, \frac{x}{x+y} \in [0,1]$, the last inequality can be seen as follows:

 Since $g$ is concave we have 
$\forall p \in [0,1], x \in \Real: g(p x) =  g(px + (1-p) 0) \geq p g(x) + (1-p) g(0) \geq p g(x)  $. The last inequality follows from $g(0) \geq 0$.
\end{proof}
\end{lem}

\begin{lem} \label{lem:x2p_pdNsubadd}
 Let $h: \begin{cases} \Real_{\geq 0} \to \Real_{\geq 0},\\ \, x \mapsto x^p\end{cases}$, for $p \in (0,1] $. $h$ is positive definite and subadditive. 
 That is, (i) $h(0) = 0 $ and  $h(x) > 0, \forall x \neq 0$ and (ii) $\forall x,y \in \Real_{\geq 0}: h(x+y) \leq h(x) + h(y)  $.
 Moreover, $h$ is concave. If $p \in (0,1)$, h is strictly concave. 
 
\begin{proof}
\textit{Pos. def. :} $h(0) = 0$.  Also $\lim_{x \to 0_+} h(x) =0$. Since $\nabla h (x) = p h^{p-1}(x) >0 $ for $x >0$, $h$ is strictly monotonically increasing on $\Real_+$. Hence, $h(x) > 0, \forall x >0$. 

\textit{Concavity:} If $p =1$, $h$ is linear and hence, concave. If $p \in (0,1)$, $\nabla^2 h(x) = p (p-1) h(x)^{p-2} > 0$ regardless of $x$.

\textit{Subadditivity:} Follows directly with Lem. \ref{lem:pd_n_concave_subadditive} on the basis of established positive definiteness and concavity.
  %
\end{proof}
\end{lem}



\begin{lem}\label{lem:hoeldererror_metric}
Let $p \in (0,1]$.
With definitions as above, we assume that set $\inspace$ is endowed with a pseudo- metric $\metric$. Function
$\metricp: \begin{cases} \inspace \times \inspace \to \Real_{\geq 0} \\ (x,y) \mapsto \Bigl(\metric(x,y)\Bigr)^p \end{cases}$ is a pseudo-metric on $\inspace$.
If $\metric$ is a metric then so is $\metricp$.
\begin{proof}
 By Lem. \ref{lem:x2p_pdNsubadd}, $x\mapsto x^p$ is pos. def. and sub-additive. Therefore, positive definiteness and the triangle inequality of $\metric$ readily extend to $\metricp$ as follows: 

\textit{Pos. def.:}
Let $x=0$. $\metricp(x,x) = \metric(x,x)^p = 0^p = 0$. If $x \neq 0$ then $k :=\metric(x,x) \neq 0$. Hence   $\metricp(x,x) = d(x,x)^p = k^p \neq 0$.

\textit{Triangle inequality:}
Choose arbitrary $x,y,z \in \inspace $. We have $\metricp(x,z) = \metric(x,z)^p \leq (\metric(x,y) + \metric(y,z) \bigr)^p \leq \metric(x,y)^p + \metric(y,z)^p = \metricp(x,y) + \metricp(y,z)$. Here, the first inequality followed from the triangle inequality of pseudo-metric $\metric$ and the second from subadditivity properties established in Lem. \ref{lem:x2p_pdNsubadd}.

\textit{Symmetry:} If $\metric$ is a metric it is symmetric. Hence, $\metricp(x,y) = \metric(x,y)^p = \metric(y,x)^p = \metricp(y,x), \forall x,y \in \inspace $ in which case $\metric$ also is symmetric.
\end{proof}
\end{lem}

Before proceeding we establish a slight generalisation of the well-known \textit{reverse triangle inequality}:

\begin{lem}[Reverse Triangle Inequality] \label{thm:revtriangle}
Let  $\inspace$ be a set and $\metric : \inspace^2 \to \Real$ a symmetric function that satisfies the triangle inequality. 
That is,  $\forall x,y,z \in \inspace: \metric (x,y) = \metric(y,x) \wedge \metric(x,z) \leq \metric(x,y) + \metric(y,z)$.

Then \[\forall x,y,z \in \inspace: \abs{\metric(x,y) - \metric(z,y)} \leq \metric(x,z).\]
\begin{proof}
For contradiction, assume 
$\abs{\metric(x,y) - \metric(z,y)}>\metric(x,z)$ for some $x,y,z \in \inspace$.
This is implies  
$
(i)\,\,\, \metric(x,y) - \metric(z,y)>\metric(x,z) 
\, \, $  or  $
\,\,  (ii) \,\,\,\, \metric(z,y)-\metric(x,y) >\metric(x,z)$.
Both inequalities contradict the triangle inequality:
$(i) \Leftrightarrow \metric(x,y)  >\metric(x,z) +\metric(z,y) $ and 
$(ii) \Leftrightarrow  \metric(z,y) > \metric(x,z) + \metric(x,y) =  \metric(z,x) + \metric(x,y)$.

\end{proof}
\end{lem}


\begin{lem}
Let $\metric$ be a (pseudo-) metric on $\inspace$. For arbitrary $s \in \inspace $ we define $\phi_s: \inspace \to \Real $ as $\phi_s: x \mapsto \metric (x,s) $.
$\phi_s $ is Lipschitz with respect to metric $\metric$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq \metric (x,y). \]
\begin{proof}
$\abs{\phi_s(x) - \phi_s(y)} = \abs{\metric(x,s) - \metric(y,s)} \stackrel{Thm. \ref{thm:revtriangle}} {\leq} \metric(x,y), \forall x,y,s \in \inspace $.
\end{proof}
\end{lem}
Finally, combining this lemma with Lem. \ref{lem:hoeldererror_metric} immediately establishes that mappings of the form $\metric(\cdot,s)^p$ are H\"older continuous with exponent $p$ ($\in (0,1]$):

\begin{thm} \label{thm:d2pmapishoelder}
Let $\metric$ be a (pseudo-) metric on set $\inspace$ and let $p \in (0,1], L \geq 0$. For arbitrary $s \in \inspace $ we define $\phi_s:\begin{cases}  \inspace \to \Real \\ x \mapsto L \, \bigl(\metric (x,s) \bigr)^p\end{cases}$.
$\phi_s $ is H\"older with exponent $p$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq L \, \metric (x,y)^p. \]
In particular, for any norm $\norm \cdot$ on $G$ and $s \in \inspace $, mapping $x \mapsto L \norm{x-s}^p$ is H\"older with constant $L$ and exponent $p$.

\begin{proof}
By Lem. \ref{lem:hoeldererror_metric}, $\metric^p(\cdot,\cdot)$ is a (pseudo-) metric on $\inspace$. Hence, Lem. \ref{thm:revtriangle} is applicable yielding:
$\abs{\phi_s(x) - \phi_s(y)} = L \, \abs{\metric(x,s)^p - \metric(y,s)^p} \stackrel{Lem. \ref{thm:revtriangle} } {\leq} \metric(x,y)^p, \forall x,y,s \in \inspace$. The last sentence concerning the norms follows from the fact that a mapping $(x,y) \mapsto \norm{x-y}$ defines a metric.
\end{proof}
\end{thm}



 %At first glance, the result may seem intuitive. However, it should be noted that, for $p >1$, $x \mapsto \norm{x -s}^p$ no longer is H\"older with exponent $p$. This is consistent with the well-known fact that H\"older functions with exponent $>1$ are constant functions.
%
%We conclude this section by the following theorem stating that any concatenation of H\"older continuous functions is H\"older continuous:
%
%\begin{thm} \label{thm:concathoelder}
%Let $(\statespace, \metric)$ be a metric space and $f,g : \statespace \to \statespace$ be two H\"older continuous mappings with  H\"older  constants $L_f, L_g$ and H\"older exponents $p_f,p_g$, respectively.
%Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also H\"older continuous with H\"older constant $L_h:= L_f L_g^{p_f}$ and exponent $p_h:=p_g \, p_f$.
%That is, 
%\[\forall \state,\state' \in \statespace: \metric\bigl(h(\state),h(\state')\bigr) \leq L_h \bigl(\metric(\state,\state')\bigr)^{p_h}.\]
%\begin{proof}
%%\begin{align}
%$\metric\bigl(f \circ g(\state),f\circ g(\state')\bigr) \leq L_f  \Bigl(\metric(g(\state),g(\state'))\Bigr)^{p_f}$
%$\leq L_f  \Bigl(L_g \metric(\state,\state')^{p_g}\Bigr)^{p_f}$ $= L_f L_g^{p_f}   \Bigl(\metric(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using H\"older continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
%
%\end{proof}
%\end{thm} 
%In conjunction with H\"older properties of the square root function established in Ex. \ref{ex:sqrtfctHoelder}, Thm. 
%\ref{thm:concathoelder} immediately yields the following result:
%\begin{cor}
%If $f: \statespace \to \statespace $ is H\"older continuous with constant $L_f$ and exponent $p_f$ then $\sqrt{f}$ also is Hoelder, having  H\"older constant $\sqrt{L_f}$ and exponent $p_f$.
%\end{cor}


==> content2/meinzeugs.tex <==
%\documentclass[10pt]{article}
%\usepackage[usenames]{color} %used for font color
%\usepackage[utf8]{inputenc} %useful to type directly diacritic characters
%\usepackage[pdftex]{graphicx}
%\usepackage[top=2cm, bottom=2cm, left=2.2cm, right=2.1cm]{geometry}
%\usepackage[top=1.9cm, bottom=1.9cm, left=1.9cm, right=1.9cm]{geometry}
%\usepackage{setspace}
%\usepackage{floatflt}
%\usepackage{amsfonts}
%\usepackage{times}
%\usepackage[toc]{appendix}
\usepackage{subfigure}
%\usepackage{epsfig,epstopdf}
%\usepackage{url}
%\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
%\usepackage{latexsym}
%\usepackage{pstricks,pst-node,pst-grad,pst-xkey}
%\usepackage{float}
%\usepackage{multirow}
%\usepackage{cite}
%\usepackage{algorithm,algorithmic}
%\usepackage{psfrag}
%\usepackage{xy} 
%\usepackage{fancyhdr}
%\usepackage{setspace} 
%\usepackage{rotating} 
%\usepackage{citesort}
%\usepackage{cite} 
%\usepackage{verbatim} 
%\usepackage{multicol} 
%\usepackage{longtable}
%\usepackage{booktabs}
%\usepackage{pdfsync} 
%\usepackage{pstricks,pst-node,pst-grad,pst-xkey}
%\usepackage{epigraph}
\usepackage{tikz}
%\usepackage{gantt}
%\usepackage[lined,boxed,commentsnumbered]{algorithm2e}
%\usepackage{algorithm2e}
%\usepackage{color}
%\usepackage{algorithmicx}
%\usepackage[noend]{algpseudocode}


\newcommand{\stevecom}[1]{\textcolor{red} {\emph{Steve says: #1}}}
\newcommand{\jcom}[1]{\textcolor{cyan} {\emph{Jan says: #1}}}
\newcommand{\mikecom}[1]{\textcolor{yellow} {\emph{Mike says: #1}}}
% THEOREMS -------------------------------------------------------
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{conj}[thm]{Conjecture}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{ques}[thm]{\textbf{QUESTION}}
\newtheorem{ex}[thm]{\textbf{Example}}
\newtheorem{ass}[thm]{\textbf{Assumption}}
%\newenvironment{proof}{\textbf{Proof:}}{\hfill$\square$}
% MATH -----------------------------------------------------------
\newcommand{\matnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}		
\newcommand{\specnorm}[1]{\matnorm{#1}_2}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\normtop}[1]{\left\Vert#1\right\Vert^p}
\newcommand{\Ltwonorm}[1]{\left\Vert#1\right\Vert_{\Ltwo}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\abstop}[1]{\left\vert#1\right\vert^p}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\Real}{\mathbb R}
\newcommand{\Complex}{\mathbb C}
\newcommand{\integer}{\mathbb Z}
\newcommand{\nat}{\mathbb N}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\BX}{\mathbf{B}(X)}
\newcommand{\A}{\mathcal{A}}
\newcommand{\aff}[1]{\text{aff } #1}
\newcommand{\dom}[1]{\text{dom } #1}
\newcommand{\epi}[1]{\text{epi } #1}
\newcommand{\ri}[1]{\text{ri } #1}
\newcommand{\cl}[1]{\text{cl } #1}

\newcommand{\QM}[1]{\ensuremath{\mathcal{QM}(#1)} }

\newcommand{\proj}{\Pi_{\text{proj} \,}}
%-----------------------------------------
\newcommand{\argmin}{\text{argmin}}
\newcommand{\argmax}{\text{argmax}}
\newcommand{\arginf}{\text{arginf}}
\newcommand{\argsup}{\text{argsup}}

\newcommand{\sgn}{\ensuremath{\text{sgn}}}
% fuer skalare:
%\newcommand{\s}[1]{\mathfrak{#1}}
\newcommand{\s}[1]{{#1}}
% fuer vectoren:
%\newcommand{\vc}[1]{\mathbf{#1}}
\newcommand{\vc}[1]{#1}
% scalar product:
\newcommand{\Sp}[1]{\ensuremath{\mathbf{\langle} #1 \mathbf{\rangle}}}
\newcommand{\SP}[2]{\ensuremath{\mathbf{\langle} \vc{#1} \mathbf{,} \vc{#2} \mathbf{\rangle}}}
\newcommand{\SPL}[2]{\ensuremath{\mathbf{\langle} \vc{#1}\mathbf{,} \vc{#2} \mathbf{\rangle}_{L_2}}}
\newcommand{\SPLintI}[2]{\ensuremath{\int_I {#1(t)}\, {\overline{#2}(t)} \, {d\mu(t)}}}
\newcommand{\SPLtwo}[2]{\ensuremath{\mathbf{\langle} \vc{#1}\mathbf{,} \vc{#2} \mathbf{\rangle}_{\Ltwo}}}

\newcommand{\normLtwo}[1]{\ensuremath{\norm{ #1}_{\Ltwo}}}

\newcommand{\ball}[2]{\ensuremath{\mathfrak B_{\vc{#1}} \bigl( #2\bigr) }}

\newcommand{\pp}[1]{\langle #1 \rangle}

%HS:
\newcommand{\hs}[1]{\ensuremath{\mathcal{#1}}}
%operators:
\newcommand{\op}[1]{\ensuremath{ {#1}}}

\newcommand{\postmean}{\mathfrak m}

\newcommand{\dif}[2]{{\operatorname{d}\over\operatorname{d}#2}#1}
\newcommand{\pdif}[2]{{\operatorname{\partial}\over\operatorname{\partial}#2}#1}
\newcommand{\ppdif}[3]{{\operatorname{\partial^2}\over\operatorname{\partial}#2 \partial#3}#1}
%\renewcommand{\d}[1]{\operatorname{d}#1}
\renewcommand{\d}[1]{\text{ d}#1}

\newcommand{\floor}[1]{ \left\lfloor #1 \right\rfloor }
\newcommand{\ceil}[1]{ \left\lceil #1 \right\rceil }
\newcommand{\fexp}[1]{\ensuremath{\exp\bigl( #1 \bigr)}}

\newcommand{\errinp}{\varepsilon_{\text{inp}}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}

%Fourier Operator:
\newcommand{\FT}[1]{\mathcal F #1}

\newcommand{\spec}{\sigma }
\newcommand{\specrad}{\rho}

\newcommand{\radfct}{\ensuremath{\mathfrak r}}
%Koerper:
\newcommand{\field}{\mathbb F}
%nullspace:
\newcommand{\ns}{\mathcal{NS}}
\newcommand{\GP}{\mathcal {GP} }
\newcommand{\Gauss}{\mathcal {N} }
\newcommand{\gauss}{p_{\mathcal {N}} }
\newcommand{\expect}[1]{\ensuremath{ \langle#1\rangle } }
\newcommand{\cexpect}[2]{\ensuremath{ \langle#1 \, \vert \, #2\rangle } }
\newcommand{\cov}[2]{\ensuremath{ \text{cov}(#1,#2) } }
\newcommand{\covmat}[2]{\ensuremath{ \text{Cov}(#1,#2) } }
\newcommand{\var}[1]{\ensuremath{ \text{var}[#1]} }
\newcommand{\varmat}[1]{\ensuremath{ \text{Var}[#1]} }
\newcommand{\data}{\ensuremath{ \mathcal D} }

\newcommand{\varmatnormbnd}{\ensuremath{ V}}

\newcommand{\rank}{\ensuremath{ \text{ rank }}}
%parameter:
\newcommand{\pardop}{\ensuremath{\omega}}%parameter for lin. Dif OP


\newcommand{\param}{\ensuremath{\Xi}}%parameter for lin. Dif OP


\newcommand{\pardopspace}{\ensuremath{\Omega}}%parameter space for lin. OP

\newcommand{\pardi}{\ensuremath{\mathfrak p}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\pardispace}{\ensuremath{\mathfrak P}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\state}{\ensuremath{ \vc x}} % state of the system... integral curve of the ODE/ signal.
\newcommand{\isv}{\ensuremath{ \vc s}} % interaction space vector

\newcommand{\statespace}{\ensuremath{ \mathcal X}}
\newcommand{\configspace}{\ensuremath{ \mathcal Q}}
\newcommand{\inspace}{\ensuremath{ \mathcal X}}
\newcommand{\outspace}{\ensuremath{ \mathcal Y}}
\newcommand{\taskspace}{\ensuremath{ \mathcal }}
\newcommand{\ctrlspace}{\ensuremath{ \mathcal U}}
\newcommand{\fctspace}{\ensuremath{ \mathcal F}}
\newcommand{\hilspace}{\ensuremath{ \mathcal H}}
\newcommand{\HS}{\ensuremath{ \mathcal H}}
\newcommand{\samplespace}{\ensuremath{\Omega}}
\newcommand{\freespace}{\ensuremath{ \mathfrak F}}
\newcommand{\iaspace}{\ensuremath{ \mathcal S}} %interaction space
\newcommand{\policyspace}{\ensuremath{ \mathcal P_u}} %policy space


\newcommand{\grid}{\ensuremath{  G}}

\newcommand{\tube}{\ensuremath{ \mathbb T}}

\newcommand{\Ltwo}{\ensuremath{\mathcal L_2 \,}}

\newcommand{\dW}{\ensuremath{\, \text{d}W}}

\newcommand{\linopspace}{\ensuremath{ \mathcal L}}

\newcommand{\rvc}{\ensuremath{ \vc{X}}}
\newcommand{\rv}{\ensuremath{ {X}}}

\newcommand{\indset}{\ensuremath{ \mathcal I}}
\newcommand{\indsett}{\ensuremath{ {\mathcal I_{t}}}}

\newcommand{\di}{\ensuremath{ u}} % driving force / control input

\newcommand{\agi}{\ensuremath{ \mathfrak a}} %an agent index
\newcommand{\agii}{\ensuremath{ \mathfrak r}} %index if another agent
\newcommand{\agiii}{\ensuremath{ \mathfrak q}} %index if another agent

\newcommand{\agdiam}{\ensuremath{ {\Lambda^{\agi,\agii}}} }
\newcommand{\nagi}{\ensuremath{ {\neg \agi}} }
\newcommand{\nagii}{\ensuremath{ {\neg \agii}} }
\newcommand{\nagiii}{\ensuremath{ {\neg \agiii}}} 

\newcommand{\collcritfct}{\gamma^{\agi,\agii}}

\newcommand{\nuref}{\nu_{\text{ref}}}
\newcommand{\nufb}{\nu_{\text{fb}}}

\newcommand{\xref}{x_{\text{ref}}}
\newcommand{\dxref}{\dot x_{\text{ref}}}
\newcommand{\coupleset}{\mathcal C}
\newcommand{\confl}{\text{confl}}
\newcommand{\tailrad}{\ensuremath{ {\varrho}} }

\newcommand{\maxerr}{\bar{\mathfrak v}} %max error in Hfe
\newcommand{\maxerrn}{\bar{\mathfrak N}} %maximum error norm

\newcommand{\metric}{\, \mathfrak{d}} % distance metric
\newcommand{\metricp}{\,  \tilde {d}} % distance metric
\newcommand{\Metric}[2]{\metric\bigl(#1,#2\bigr) }
\newcommand{\Metrici}[2]{\metric\bigl(#1,#2\bigr) }
\newcommand{\Metrico}[2]{\metric_\outspace\bigl(#1,#2\bigr) }
\newcommand{\Metrictop}[2]{\metric^p\bigl(#1,#2\bigr) }
\newcommand{\Metrictopi}[2]{\metric^p_\inspace\bigl(#1,#2\bigr) }
\newcommand{\Metrictopo}[2]{\metric^p_\outspace\bigl(#1,#2\bigr) }
\newcommand{\dist}{\ensuremath{ \text{dist}}} % driving force / control input

\newcommand{\predf}{\, \mathfrak{  \hat f}} % hypothesis
\newcommand{\predfn}{\, \mathfrak{  \hat f_n}} % hypothesis
\newcommand{\predfnj}{\, \mathfrak{  \hat f_{n,j}}} % hypothesis
\newcommand{\prederr}{\, \mathfrak{\hat v}} % error around hyp
\newcommand{\prederrn}{\, \mathfrak{\hat v_n}} % error around hyp
\newcommand{\prederrnj}{\, \mathfrak{\hat v_{n,j}}} % error around hyp
\newcommand{\prederrbox}{\, {\hat H}} % error around hyp

\newcommand{\noise}{{\nu}} % error around hyp


\newcommand{\hexp}{{ \alpha }}%hoelder exponent
\newcommand{\hconst}{\ensuremath{ L }}%hoelder const
\newcommand{\hestthresh}{\ensuremath{ \lambda}}
\newcommand{\ubf}{\, {\bar B}} % upper bound function
\newcommand{\lbf}{\, {\underline{B}}} % lower bound function
\newcommand{\bfset}{\mathcal B}

\newcommand{\lipset}[2]{\text{Lip}_{#2}(#1)}
\newcommand{\hoelset}[3]{\mathfrak{H}_{#2}(#1,#3)}
\newcommand{\Hoelset}{\mathfrak{H}}
%\newcommand{\coeff1}{ \underline{c}} % 
%\newcommand{\coeff2}{ \overline{c}} %

\newcommand{\errhyprec}{\mathbf  E} % upper bound function
\newcommand{\obserrhyprec}{\mathbf  O} % upper bound function

\newcommand{\obserrpar}{e} % parameter of presupposed obserr
\newcommand{\obserr}{\mathfrak e} % upper bound function on observational noise
\newcommand{\obserrbnd}{\bar{\mathfrak e}}

\newcommand{\agset}{\ensuremath{ \mathfrak A}} %set of Agents
\newcommand{\agsubset}{\ensuremath{ \mathfrak S}} %set of Agents

\newcommand{\indicator}[1]{\ensuremath{\textbf{1}_{#1}}} % indicator function

\newcommand{\collevent}{\ensuremath{\mathfrak C}}
\newcommand{\colleventtwoA}{\ensuremath{\mathfrak C^{\agi,\agii}}}
%\newcommand{\hull}{\ensuremath{\mathfrak C}}

\newcommand{\decke}{\ensuremath{\mathfrak u}}
\newcommand{\boden}{\ensuremath{\mathfrak l}}
\newcommand{\einschluss}{\ensuremath{\mathcal E^{\decke_{n}}_{\boden_{n}}}}
\newcommand{\opteinschluss}{\ensuremath{\mathcal E^*_n}}
\newcommand{\Kprior}{\mathcal K_{\text{prior}} }
\newcommand{\Kdat}{\mathcal K(D_n)}

\newcommand{\menge}[2]{\ensuremath{\{#1 \, \vert \, #2 \}}}

\newcommand{\seq}[2]{\ensuremath{\bigl(#1\bigr)_{#2}}}

%\newcommand{\diag}{\ensuremath{ \text{diag}} %set of

%\newcommand{\e}[1]{\ensuremath{\exp \Bigl(#1\Bigr) }}
\newcommand{\card}[1]{\ensuremath{\left\vert #1 \right\vert }}

\renewcommand{\Pr}{\mathrm{Pr}}
\newcommand{\sqmats}{\mathcal{M}} %set of square matrices


\renewcommand{\d}{\ensuremath{\text{ d}}}
\newcommand{\KLD}[2]{\text{KLD}(#1||#2) }

\newcommand{\erw}[2][]{
%    \ensuremath{\pmb{\mathcal{M}}^{\operatorfont{#1}}}%
     \ensuremath{\mathbb{E}_{#1} \! \left\lbrace #2 \right\rbrace}%
}


%----------- probability stuff------------------------
\newcommand{\pmeas}{\ensuremath{\mathbb P}} % probability measure


\newcommand{\embedding}{\ensuremath{\tilde \mu}} % probability measure
\newcommand{\ewx}[1]{\ensuremath{\mathbb E_x[ #1 ] }} % expected value
\newcommand{\ew}{\ensuremath{\mathbb E }} % expected value
\newcommand{\is}{\ensuremath{\mathfrak X }} % input space / index set
\newcommand{\Vol}{\ensuremath{\text{Vol}}}
\newcommand{\mslim}{\ensuremath{\text{m.s.-lim}}}
\newcommand{\msto}{\ensuremath{\stackrel{ \text{2}}{\longrightarrow}}}

% --------------------environments--------------------------------------------
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eq}[1]{\begin{equation} #1 \end{equation}}
\newcommand{\eqn}[2]{\begin{equation} #2 \label{#1}\end{equation}}
\newcommand{\dt}{\ensuremath{ \, dt \,}}
%\newcommand{\dW}{\ensuremath{ \, dW \,}}
\newcommand{\tinc}{\ensuremath{ \Delta}}

\newcommand{\tr}{\ensuremath{ \text{ tr}}}

\newcommand{\rlem}[1]{Lem. \ref {#1}} % indicator function
\newcommand{\rthm}[1]{Thm. \ref {#1}} % indicator function
%\newcommand{\rch}[1]{Ch. \ref {#1}} % indicator function
% ----------------------------------------------------------------
\newcommand{\convton}{\stackrel{n \to \infty}\longrightarrow}
\newcommand{\convto}{\longrightarrow}
\newcommand{\setconvto}{\longrightarrow}
\newcommand{\setconvtounif}{\stackrel{\text{unif}}{\longrightarrow}}
\newcommand{\bd}{\leadsto} %becomes dense relative to 
\newcommand{\bdu}{\twoheadrightarrow} %becomes dense relative to uniformly

\newcommand{\errmetric}{\mathcal E} %becomes dense relative to uniformly
\newcommand{\queryset}{I} %becomes dense relative to uniformly

%-------------- Meinzeugs Ende-----------------------------------------

==> content2/meinzeugs_automatica.tex <==
%\documentclass[10pt]{article}
%\usepackage[usenames]{color} %used for font color
%\usepackage[utf8]{inputenc} %useful to type directly diacritic characters
%\usepackage[pdftex]{graphicx}
%\usepackage[top=2cm, bottom=2cm, left=2.2cm, right=2.1cm]{geometry}
%\usepackage[top=1.9cm, bottom=1.9cm, left=1.9cm, right=1.9cm]{geometry}
%\usepackage{setspace}
%\usepackage{floatflt}
%\usepackage{amsfonts}
%\usepackage{times}
%\usepackage[toc]{appendix}
\usepackage{subfigure}
%\usepackage{epsfig,epstopdf}
%\usepackage{url}
%\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
%\usepackage{latexsym}
%\usepackage{pstricks,pst-node,pst-grad,pst-xkey}
%\usepackage{float}
%\usepackage{multirow}
%\usepackage{cite}
%\usepackage{algorithm,algorithmic}
%\usepackage{psfrag}
%\usepackage{xy} 
%\usepackage{fancyhdr}
%\usepackage{setspace} 
%\usepackage{rotating} 
%\usepackage{citesort}
%\usepackage{cite} 
%\usepackage{verbatim} 
%\usepackage{multicol} 
%\usepackage{longtable}
%\usepackage{booktabs}
%\usepackage{pdfsync} 
%\usepackage{pstricks,pst-node,pst-grad,pst-xkey}
%\usepackage{epigraph}
\usepackage{tikz}
%\usepackage{gantt}
%\usepackage[lined,boxed,commentsnumbered]{algorithm2e}
%\usepackage{algorithm2e}
%\usepackage{color}
%\usepackage{algorithmicx}
%\usepackage[noend]{algpseudocode}


\newcommand{\stevecom}[1]{\textcolor{red} {\emph{Steve says: #1}}}
\newcommand{\jcom}[1]{\textcolor{cyan} {\emph{Jan says: #1}}}
\newcommand{\mikecom}[1]{\textcolor{yellow} {\emph{Mike says: #1}}}
% THEOREMS -------------------------------------------------------
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{alg}[thm]{Algorithm}
%\newtheorem{conj}[thm]{Conjecture}
%\theoremstyle{definition}
%\newtheorem{defn}[thm]{Definition}
\theoremstyle{remark}
%\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{ques}[thm]{\textbf{QUESTION}}
\newtheorem{ex}[thm]{\textbf{Example}}
\newtheorem{ass}[thm]{\textbf{Assumption}}
\newenvironment{proof}{\textbf{Proof:}}{\hfill$\square$}
% MATH -----------------------------------------------------------
\newcommand{\matnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}		
\newcommand{\specnorm}[1]{\matnorm{#1}_2}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\normtop}[1]{\left\Vert#1\right\Vert^p}
\newcommand{\Ltwonorm}[1]{\left\Vert#1\right\Vert_{\Ltwo}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\abstop}[1]{\left\vert#1\right\vert^p}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\Real}{\mathbb R}
\newcommand{\Complex}{\mathbb C}
\newcommand{\integer}{\mathbb Z}
\newcommand{\nat}{\mathbb N}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\BX}{\mathbf{B}(X)}
\newcommand{\A}{\mathcal{A}}
\newcommand{\aff}[1]{\text{aff } #1}
\newcommand{\dom}[1]{\text{dom } #1}
\newcommand{\epi}[1]{\text{epi } #1}
\newcommand{\ri}[1]{\text{ri } #1}
\newcommand{\cl}[1]{\text{cl } #1}

\newcommand{\QM}[1]{\ensuremath{\mathcal{QM}(#1)} }

\newcommand{\proj}{\Pi_{\text{proj} \,}}
%-----------------------------------------
\newcommand{\argmin}{\text{argmin}}
\newcommand{\argmax}{\text{argmax}}
\newcommand{\arginf}{\text{arginf}}
\newcommand{\argsup}{\text{argsup}}

\newcommand{\sgn}{\ensuremath{\text{sgn}}}
% fuer skalare:
%\newcommand{\s}[1]{\mathfrak{#1}}
\newcommand{\s}[1]{{#1}}
% fuer vectoren:
%\newcommand{\vc}[1]{\mathbf{#1}}
\newcommand{\vc}[1]{#1}
% scalar product:
\newcommand{\Sp}[1]{\ensuremath{\mathbf{\langle} #1 \mathbf{\rangle}}}
\newcommand{\SP}[2]{\ensuremath{\mathbf{\langle} \vc{#1} \mathbf{,} \vc{#2} \mathbf{\rangle}}}
\newcommand{\SPL}[2]{\ensuremath{\mathbf{\langle} \vc{#1}\mathbf{,} \vc{#2} \mathbf{\rangle}_{L_2}}}
\newcommand{\SPLintI}[2]{\ensuremath{\int_I {#1(t)}\, {\overline{#2}(t)} \, {d\mu(t)}}}
\newcommand{\SPLtwo}[2]{\ensuremath{\mathbf{\langle} \vc{#1}\mathbf{,} \vc{#2} \mathbf{\rangle}_{\Ltwo}}}

\newcommand{\normLtwo}[1]{\ensuremath{\norm{ #1}_{\Ltwo}}}

\newcommand{\ball}[2]{\ensuremath{\mathfrak B_{\vc{#1}} \bigl( #2\bigr) }}

\newcommand{\pp}[1]{\langle #1 \rangle}

%HS:
\newcommand{\hs}[1]{\ensuremath{\mathcal{#1}}}
%operators:
\newcommand{\op}[1]{\ensuremath{ {#1}}}

\newcommand{\postmean}{\mathfrak m}

\newcommand{\dif}[2]{{\operatorname{d}\over\operatorname{d}#2}#1}
\newcommand{\pdif}[2]{{\operatorname{\partial}\over\operatorname{\partial}#2}#1}
\newcommand{\ppdif}[3]{{\operatorname{\partial^2}\over\operatorname{\partial}#2 \partial#3}#1}
%\renewcommand{\d}[1]{\operatorname{d}#1}
\renewcommand{\d}[1]{\text{ d}#1}

\newcommand{\floor}[1]{ \left\lfloor #1 \right\rfloor }
\newcommand{\ceil}[1]{ \left\lceil #1 \right\rceil }
\newcommand{\fexp}[1]{\ensuremath{\exp\bigl( #1 \bigr)}}

\newcommand{\errinp}{\varepsilon_{\text{inp}}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}

%Fourier Operator:
\newcommand{\FT}[1]{\mathcal F #1}

\newcommand{\spec}{\sigma }
\newcommand{\specrad}{\rho}

\newcommand{\radfct}{\ensuremath{\mathfrak r}}
%Koerper:
\newcommand{\field}{\mathbb F}
%nullspace:
\newcommand{\ns}{\mathcal{NS}}
\newcommand{\GP}{\mathcal {GP} }
\newcommand{\Gauss}{\mathcal {N} }
\newcommand{\gauss}{p_{\mathcal {N}} }
\newcommand{\expect}[1]{\ensuremath{ \langle#1\rangle } }
\newcommand{\cexpect}[2]{\ensuremath{ \langle#1 \, \vert \, #2\rangle } }
\newcommand{\cov}[2]{\ensuremath{ \text{cov}(#1,#2) } }
\newcommand{\covmat}[2]{\ensuremath{ \text{Cov}(#1,#2) } }
\newcommand{\var}[1]{\ensuremath{ \text{var}[#1]} }
\newcommand{\varmat}[1]{\ensuremath{ \text{Var}[#1]} }
\newcommand{\data}{\ensuremath{ \mathcal D} }

\newcommand{\varmatnormbnd}{\ensuremath{ V}}

\newcommand{\rank}{\ensuremath{ \text{ rank }}}
%parameter:
\newcommand{\pardop}{\ensuremath{\omega}}%parameter for lin. Dif OP


\newcommand{\param}{\ensuremath{\Xi}}%parameter for lin. Dif OP


\newcommand{\pardopspace}{\ensuremath{\Omega}}%parameter space for lin. OP

\newcommand{\pardi}{\ensuremath{\mathfrak p}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\pardispace}{\ensuremath{\mathfrak P}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\state}{\ensuremath{ \vc x}} % state of the system... integral curve of the ODE/ signal.
\newcommand{\isv}{\ensuremath{ \vc s}} % interaction space vector

\newcommand{\statespace}{\ensuremath{ \mathcal X}}
\newcommand{\configspace}{\ensuremath{ \mathcal Q}}
\newcommand{\inspace}{\ensuremath{ \mathcal X}}
\newcommand{\outspace}{\ensuremath{ \mathcal Y}}
\newcommand{\taskspace}{\ensuremath{ \mathcal }}
\newcommand{\ctrlspace}{\ensuremath{ \mathcal U}}
\newcommand{\fctspace}{\ensuremath{ \mathcal F}}
\newcommand{\hilspace}{\ensuremath{ \mathcal H}}
\newcommand{\HS}{\ensuremath{ \mathcal H}}
\newcommand{\samplespace}{\ensuremath{\Omega}}
\newcommand{\freespace}{\ensuremath{ \mathfrak F}}
\newcommand{\iaspace}{\ensuremath{ \mathcal S}} %interaction space
\newcommand{\policyspace}{\ensuremath{ \mathcal P_u}} %policy space




\newcommand{\tube}{\ensuremath{ \mathbb T}}

\newcommand{\Ltwo}{\ensuremath{\mathcal L_2 \,}}

\newcommand{\dW}{\ensuremath{\, \text{d}W}}

\newcommand{\linopspace}{\ensuremath{ \mathcal L}}

\newcommand{\rvc}{\ensuremath{ \vc{X}}}
\newcommand{\rv}{\ensuremath{ {X}}}

\newcommand{\indset}{\ensuremath{ \mathcal I}}
\newcommand{\indsett}{\ensuremath{ {\mathcal I_{t}}}}

\newcommand{\di}{\ensuremath{ u}} % driving force / control input

\newcommand{\agi}{\ensuremath{ \mathfrak a}} %an agent index
\newcommand{\agii}{\ensuremath{ \mathfrak r}} %index if another agent
\newcommand{\agiii}{\ensuremath{ \mathfrak q}} %index if another agent

\newcommand{\agdiam}{\ensuremath{ {\Lambda^{\agi,\agii}}} }
\newcommand{\nagi}{\ensuremath{ {\neg \agi}} }
\newcommand{\nagii}{\ensuremath{ {\neg \agii}} }
\newcommand{\nagiii}{\ensuremath{ {\neg \agiii}}} 

\newcommand{\collcritfct}{\gamma^{\agi,\agii}}

\newcommand{\nuref}{\nu_{\text{ref}}}
\newcommand{\nufb}{\nu_{\text{fb}}}

\newcommand{\xref}{x_{\text{ref}}}
\newcommand{\dxref}{\dot x_{\text{ref}}}
\newcommand{\coupleset}{\mathcal C}
\newcommand{\confl}{\text{confl}}
\newcommand{\tailrad}{\ensuremath{ {\varrho}} }

\newcommand{\maxerr}{\bar{\mathfrak v}} %max error in Hfe
\newcommand{\maxerrn}{\bar{\mathfrak N}} %maximum error norm

\newcommand{\metric}{\, \mathfrak{d}} % distance metric
\newcommand{\metricp}{\,  \tilde {d}} % distance metric
\newcommand{\Metric}[2]{\metric\bigl(#1,#2\bigr) }
\newcommand{\Metrici}[2]{\metric_\inspace\bigl(#1,#2\bigr) }
\newcommand{\Metrico}[2]{\metric_\outspace\bigl(#1,#2\bigr) }
\newcommand{\Metrictop}[2]{\metric^p\bigl(#1,#2\bigr) }
\newcommand{\Metrictopi}[2]{\metric^p_\inspace\bigl(#1,#2\bigr) }
\newcommand{\Metrictopo}[2]{\metric^p_\outspace\bigl(#1,#2\bigr) }
\newcommand{\dist}{\ensuremath{ \text{dist}}} % driving force / control input

\newcommand{\predf}{\, \mathfrak{  \hat f}} % hypothesis
\newcommand{\predfn}{\, \mathfrak{  \hat f_n}} % hypothesis
\newcommand{\predfnj}{\, \mathfrak{  \hat f_{n,j}}} % hypothesis
\newcommand{\prederr}{\, \mathfrak{\hat v}} % error around hyp
\newcommand{\prederrn}{\, \mathfrak{\hat v_n}} % error around hyp
\newcommand{\prederrnj}{\, \mathfrak{\hat v_{n,j}}} % error around hyp
\newcommand{\prederrbox}{\, {\hat H}} % error around hyp

\newcommand{\hexp}{{ p }}%hoelder exponent
\newcommand{\hconst}{\ensuremath{ L }}%hoelder const
\newcommand{\hestthresh}{\ensuremath{ \lambda}}
\newcommand{\ubf}{\, {\bar B}} % upper bound function
\newcommand{\lbf}{\, {\underline{B}}} % lower bound function
\newcommand{\bfset}{\mathcal B}

\newcommand{\lipset}[2]{\text{Lip}_{#2}(#1)}
\newcommand{\hoelset}[3]{\mathfrak{H}_{#2}(#1,#3)}
\newcommand{\Hoelset}{\mathfrak{H}}
%\newcommand{\coeff1}{ \underline{c}} % 
%\newcommand{\coeff2}{ \overline{c}} %

\newcommand{\errhyprec}{\mathbf  E} % upper bound function
\newcommand{\obserrhyprec}{\mathbf  O} % upper bound function

\newcommand{\obserrpar}{e} % parameter of presupposed obserr
\newcommand{\obserr}{\mathfrak e} % upper bound function on observational noise
\newcommand{\obserrbnd}{\bar{\mathfrak e}}

\newcommand{\agset}{\ensuremath{ \mathfrak A}} %set of Agents
\newcommand{\agsubset}{\ensuremath{ \mathfrak S}} %set of Agents

\newcommand{\indicator}[1]{\ensuremath{\textbf{1}_{#1}}} % indicator function

\newcommand{\collevent}{\ensuremath{\mathfrak C}}
\newcommand{\colleventtwoA}{\ensuremath{\mathfrak C^{\agi,\agii}}}
%\newcommand{\hull}{\ensuremath{\mathfrak C}}

\newcommand{\decke}{\ensuremath{\mathfrak u}}
\newcommand{\boden}{\ensuremath{\mathfrak l}}
\newcommand{\einschluss}{\ensuremath{\mathcal E^{\decke_{n}}_{\boden_{n}}}}
\newcommand{\opteinschluss}{\ensuremath{\mathcal E^*_n}}
\newcommand{\Kprior}{\mathcal K_{\text{prior}} }
\newcommand{\Kdat}{\mathcal K(D_n)}

\newcommand{\menge}[2]{\ensuremath{\{#1 \, \vert \, #2 \}}}

\newcommand{\seq}[2]{\ensuremath{\Bigl(#1\Bigr)_{#2}}}

%\newcommand{\diag}{\ensuremath{ \text{diag}} %set of

%\newcommand{\e}[1]{\ensuremath{\exp \Bigl(#1\Bigr) }}
\newcommand{\card}[1]{\ensuremath{\left\vert #1 \right\vert }}

\renewcommand{\Pr}{\mathrm{Pr}}
\newcommand{\sqmats}{\mathcal{M}} %set of square matrices


\renewcommand{\d}{\ensuremath{\text{ d}}}
\newcommand{\KLD}[2]{\text{KLD}(#1||#2) }

\newcommand{\erw}[2][]{
%    \ensuremath{\pmb{\mathcal{M}}^{\operatorfont{#1}}}%
     \ensuremath{\mathbb{E}_{#1} \! \left\lbrace #2 \right\rbrace}%
}


%----------- probability stuff------------------------
\newcommand{\pmeas}{\ensuremath{\mathbb P}} % probability measure


\newcommand{\embedding}{\ensuremath{\tilde \mu}} % probability measure
\newcommand{\ewx}[1]{\ensuremath{\mathbb E_x[ #1 ] }} % expected value
\newcommand{\ew}{\ensuremath{\mathbb E }} % expected value
\newcommand{\is}{\ensuremath{\mathfrak X }} % input space / index set
\newcommand{\Vol}{\ensuremath{\text{Vol}}}
\newcommand{\mslim}{\ensuremath{\text{m.s.-lim}}}
\newcommand{\msto}{\ensuremath{\stackrel{ \text{2}}{\longrightarrow}}}

% --------------------environments--------------------------------------------
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eq}[1]{\begin{equation} #1 \end{equation}}
\newcommand{\eqn}[2]{\begin{equation} #2 \label{#1}\end{equation}}
\newcommand{\dt}{\ensuremath{ \, dt \,}}
%\newcommand{\dW}{\ensuremath{ \, dW \,}}
\newcommand{\tinc}{\ensuremath{ \Delta}}

\newcommand{\tr}{\ensuremath{ \text{ tr}}}

\newcommand{\rlem}[1]{Lem. \ref {#1}} % indicator function
\newcommand{\rthm}[1]{Thm. \ref {#1}} % indicator function
%\newcommand{\rch}[1]{Ch. \ref {#1}} % indicator function
% ----------------------------------------------------------------
%-------------- Meinzeugs Ende-----------------------------------------

==> content2/root.tex <==
\input{content/Ch_kinkyinf/abstract}


\section{Introduction}

Typically, a controller is designed on the basis of a dynamical model of the system. When little is known about these dynamics a priori or, if the dynamics may be subject to unexpected change, machine learning methods can be employed to learn such a model online on the basis of measurements. 

Supervised machine learning methods are algorithms for inductive inference. On the basis of a sample, they construct (learn) a computable model of a data generating process that facilitates inference over the underlying ground truth function and aims to predict its function values at unobserved inputs.
%
Among supervised learning methods, nonparametric algorithms tend to offer greater flexibility to learn rich 
function classes (e.g. rich classes of nonlinear dynamics). 
 
Perhaps the most popular nonparametric machine learning method is Bayesian inference with \textit{Gaussian processes (GPs)} \cite{GPbook:2006}. GPs offer a flexible and principled probabilistic method for nonparametric regression and have evolved into one of the primary work-horses for learning dynamic systems \cite{Deisenroth2009,Deisenroth2011,Deisenroth2015,Tuongmodellearningsurvey2011,deisenrothsurvey2013,McHutchonthesis2014} in the research communities related to artificial intelligence. 
However, they suffer from several limitations, including scalability to large data sets, a lack of understanding of how to bound the closed-loop dynamics resulting from controlling on the basis of a GP state-space model and the question of how to choose a good prior in a principled yet computable manner. To alleviate the last problem, it is common practice to tune hyper-parameters of a chosen (typically universal) kernel to explain the data via the marginal log-likelihood. While often successful on many data sets, the result can be highly sensitive to the choice of optimiser, initialisations, data sets and computational budget. Unfortunately, little theoretical understanding of the important interplay between these components in the resulting inference mechanism seems to exist.
%
%Apart from the confinement to Gaussian a priori knowledge, the GP approach suffers from a few additional limitations. Firstly, the computational complexity for learning grows cubically and for computing the prediction variances quadratically with the training data size. This either renders the approach intractable in data rich control applications or necessitates approximations. These turn the Bayesian nonparametric method into a parametric method with somewhat limited flexibility and whose uncertainty quantifications may be hard to compute. 
%Secondly, it seems to be an open problem of how to conservatively quantify the uncertainty of the solution trajectory of the resulting uncertain dynamic system. Therefore, current methods rely on approximations whose effects on the uncertainty are not well understood (see \cite{McHutchonthesis2014} for a discussion of some of the most recent approaches). The latter deficiency is a serious shortcoming in decision making in the presence of state constraints. For instance, if it is hard to quantify or bound the probability of a trajectory being within an obstacle-free region then it will be hard to compute controls that guarantee collision-free state trajectories. 
%Finally, the uncertainties and prediction performance depend on parameter choices of the assumed prior. Since in practice, it is often hard to conceive a good prior a priori, most authors working with GPs seem to adopt a pragmatic approach and choose a prior with a maximally flexible covariance function whose parameters are (a posteriori) computed maximise the marginal log-likelihood of the data (cf. e.g. \cite{GPbook:2006,Deisenroth2015}). Apart from being a departure from Bayesian orthodoxy, this approach has a number of downsides. Firstly, the performance is sensitive to the choice of optimisation algorithm and relies on finding a good (local) maximum. Secondly, the optimisation approach introduces substantial computational overhead that currently can be prohibitive in online learning scenarios where the data needs to be updated incrementally under real-time constraints.
%Furthermore, we are not aware of any theoretical guarantees on the learning success of the inference algorithm resulting from combining the GP with a hyper-parameter optimiser. 

In contrast to such Bayesian methods this work considers an extension of ideas existing in applied mathematics  (e.g. \cite{Shubert:72,Zabinsky2003,Cooper1995,Cooper2006,Baran2008,Beliakov2006}) as well as in control \cite{Milanese2004,Canale2014} that harnesses Lipschitz regularity of the target function to provide bounds on the predictions of the target function at unobserved inputs. Applied to machine learning, the basic idea is that Lipschitz continuity constrains the set of possible function values of a target function at a query input as a function of the distance between the query and the previously observed training examples. A prediction is then made by choosing a function value in the middle of the set of possible function values. This idea, which at least goes back to \cite{Sukharev1978}, has been leveraged in different fields under different headlines including \emph{Lipschitz Interpolation} \cite{Zabinsky2003,Beliakov2006} and \emph{Nonlinear Set Membership (NSM)}  methods \cite{Milanese2004}. If the Lipschitz constant is known, Lipschitz interpolation provides uncertainties around the predictions of function values at unobserved inputs. The uncertainties are maximally tight if no other knowledge is known other than the presupposed Lipschitz regularity \cite{Sukharev1978,calliess2014_thesis}.
The presupposed Lipschitz constant is a crucial parameter of the inference rule, quite similar to the choice of a prior (e.g. via kernel and hyperparameters)  in Bayesian inference.

We would argue that one of the advantages of these methods is their computational simplicity. That is, they are numerically robust and only involve basic computational steps that could be more efficiently computed even on a simple embedded RISC micro-controller.
A practical concern is that the predictions and bounds of these methods hinge on the a priori knowledge of the presupposed Lipschitz parameter of the underlying target function. Some previous works remark that, in the absence of such knowledge the constants might in practice be estimated from the data (e.g. via estimators discussed in  \cite{Strongin1973,Wood1996,Beliakovsmoothing2007,Milanese2004,Beliakov2006}). In fact, \cite{Milanese2004} suggest fitting a parametric regressor to the data first and utilise the Lipschitz constant of the fitted model for the NSM approach. Unfortunately, there is no theoretical analysis given anywhere what the impact of that estimate is to the predictive performance of the regression method. (And, consequently control methods that rely on the resulting predictions would be unable to assert closed-loop stability or robustness guarantees).

Our work addresses this deficiency by proposing an that allows us to provide learning and stability guarantees even in the absence of a priori knowledge of this constant.

 As a first step, we rehearse \emph{Kinky Inference (KI)} \cite{calliess2014_thesis} which generalises the Lipschitz interpolation and NSM frameworks in several ways.
%
%In its basic setup, \cite{calliess2014_thesis}, our generalisations yield 
%a nonparametric machine learning method that facilitates the conversion of assumptions about H\"older continuity (and possibly boundedness) into a set-based a posteriori inference rule over multi-output functions on pseudo-metric spaces. Its prediction time grows at most linearly with the training data size. Learning merely requires the computational effort for storing the training data in memory. Furthermore, it allows us to provide worst-case bounds on the norm of the error around the inferred vector-valued predictions. Since the prediction surface of the inference rule will generally exhibit kinks, we refer to it as \textit{kinky inference (KI)}.
We then combine the KI machine learning approach with a simple online parameter estimator that allows us to incrementally compute an estimate of the H\"older constant on the basis of incrementally arriving (noisy) data. This merger yields a new inference rule we refer to as \emph{Lazily Adapted Constant Kinky Inference (LACKI)}. We prove that this rule is sample-consistent (up to the level observational error in the data) and that the LACKI predictors themselves are H\"older continuous. This allows us to establish strong universal approximation properties: That is, in the limit of infinite data, the LACKI rule is capable of approximating not only any H\"older continuous target function but also any non-H\"older continuous function with arbitrarily low error (up to a bound dependent on the level of observational error in the training data). Since our LACKI rule can be seen as an extension of Lipschitz interpolation with empirical Lipschitz constant estimation as considered in \cite{Beliakov2006}, our results also provide new theoretical guarantees for this previously proposed interpolation rule where the Lipschitz parameters are estimated online from the noisy training data with our proposed modified constant estimation method.

In addition to these learning-theoretic considerations, we apply our LACKI approach to online-learning based model-reference adaptive control.

 As a testbed, we replicate simulations of  the roll dynamics of an F-4 fighter aircraft under uncertain wing rock previously considered by other authors in model-reference adaptive control \cite{Chowdhary2013,Monahemi1996,chowdharyacc2013} and compare our controller against their methods. Here our LACKI-based controller outperforms its competitors across a range of metrics including computational speed, prediction accuracy and tracking success. 

For discrete-time feedback-linearisable systems with uncertain nonlinear drift, we provide theoretical guarantees on the tracking success of our LACKI- model-reference adaptive controller both in the batch and in the online learning setting. 

In contrast to much of the standard literature of probabilistic nonparametric regression (e.g. \cite{Gyoerfi2002,Tsybakov2009}), our analysis focusses on the derivation of deterministic  worst-case error bounds. While possibly being more conservative, we would argue that this type of analysis has the benefit of being more meaningful in a control setting where the learner receives training examples and queries that will typically violate statistical assumptions typically presupposed  in the probabilistic literature.

The remainder of the paper is structured as follows: 

Sec. \ref{sec:LACKI_all} contains the core of the LACKI regression methods. Following a rehearsal of the kinky inference (KI) framework for nonparametric learning, Sec. \ref{sec:lacki} describes the our LACKI approach for setting the KI parameters. Sec. \ref{sec:properties_lacki} is dedicated the derivation of several properties of the resulting LACKI approach, including our consistency guarantees.

Sec. \ref{sec:MRAC_lacki} contains the control part of the paper. We first introduce the framework of model-reference adaptive control in which we propose a controller based on our LACKI learning method.  For illustration purposes, we closely follow the setting of wing-rock control considered in \cite{Chowdhary2013,ChowdharyCDC2013} and compare our LACKI-based controller to other MRAC controllers consdered and proposed by previous work. The section concludes by giving stability guarantees for LACKI-MRAC in discrete-time systems.

The paper concludes with Sec. \ref{sec:concl}, summarising our findings and containing various suggestions for future work. The appendix contains a variety of background material on 
H\"older continuity and various supplementary derivations referred to at various points of the main body of the paper. 

%\jcom{Can we now combine the remaining dynamics with an MPC controller on top that also gets rid of the observational error?}


%In Sec. \ref{sec:KI_core} we will present the inference rule and establish theoretical guarantees. In Sec. \ref{sec:KIcollavoiddiscretetime} we illustrate how the KI approach can be employed in the context of multiagent collision avoidance under uncertain agent dynamics. Linking to work in robust and stochastic predictive control \cite{Kuwata2005,Kuwata2006,Trodden2006,LyonsACC2012}, we state the planning problem as optimisation with constraint tightening to enforce collision avoidance. In the presented example, an initially unmodelled nonlinear drift causes a collision among the agents during plan execution. Introduction of our KI method yields robustness bounds that constrain the planning problem sufficiently to prevent the collision. And, the conservatism of the joint plans can be reduced with increasing training data. We believe the combination of KI learning and multi-agent control is the first work that achieves\textit{ guaranteed }collision avoidance by taking the epistemic uncertainty of a nonparametric machine learning method into account. 
 
 
 %The paper concludes with a summary and hints at some of the manifold future directions this work facilitates. 

%
%
%Typically there are infinitely many explanations that could explain any finite data set. Therefore, one needs to impose assumptions a priori in order to be able to generalise beyond the observed data and to establish the desired uncertainty quantifications. 
%
%These assumptions, sometimes referred to as inductive bias \cite{mitchellbook:97}, take different forms and are an essential distinguishing factor between different machine learning algorithms. 
%The inductive bias implicitly or explicitly restricts the hypothesis space. That is, the space of target functions that can be learned.
%
%
%
%In this work, we devise a learning method for ground truth functions that are assumed to be contained in the a priori hypothesis space $\Kprior$ of H\"older continuous functions. Moreover, these may be known to be contained within certain predefined bounds. 
%
%In the case in which the parameters of the H\"older class the function is contained in are known (or at least an upper bound on the H\"older constant and bounds) we can give robust error estimates that give worst-case guarantees on the predictions. In the event the presumed parameters turn out to be wrong, Sec. \ref{sec:uncertainconstants} contains proposals on how to update the belief over the constants in the light of new data.


\section{Kinky Inference with lazily adapted constants}


\label{sec:LACKI_all}

\subsection{Kinky Inference}
\label{sec:KI_core}
In this section, we will introduce the class of learning rules we refer to as \emph{Kinky Inference}. They encompass a host of other methods such as Lipschitz Interpolation and Nonlinear Set Interpolation.  
%
%We will then establish some theoretical guarantees for certain parameter settings, in particular of the sequence of Lipschitz parameters $L(n)$. In subsequent parts of this section we will then consider a method for adapting these parameters to the data yielding a rule we will refer to as \emph{Lazily Adapted Constant Kinky Inference (LACKI)}. The section culminates in establishing universal approximation guarantees for our LACKI rule.

The rules possess a parameter $L(n)$ that needs to be specified by any KI algorithm. In this paper, we are most concerned with studying LACKI, a KI rule algorithm where $L(n)$ coincides with a noise-robust and multi-variate generalisation of Strongin's estimate \cite{Strongin1973} of a H\"older constant computed from the data set $\data_n$ available at time step $n$. 

%We will consider the special case $\inspace = \Real^d, \outspace \subseteq \Real^m$ with pseudo-metric $\metric$ on the input space and output-space metric defined by $\metric_\outspace(x,x') := \norm{x-x'}_\infty , \forall x,x' \in \inspace$. 

%\subsubsection{Conservative learning and inference in a nutshell}
%
%The general approach we will consider is as follows. We desire to learn a function $f$ based prior knowledge of the form that $f \in \mathcal K_{prior}$ and some (noisy) function sample $\data$. 
%The task of conservative inference over functions (i.e. learning) then is the step of forming a posterior belief of the form $f \in \mathcal K_{post}= \mathcal K_{prior} \cap \mathcal K(\data)$. Here,
%$\mathcal K (\data)$ is the set of all functions that could have generated the observed data. 
%The conservatism lies in the fact that we have not ruled out any candidate functions that are consistent with our information. 
%To perform inference over a function value at input $x$ in a conservative manner, we merely infer that $f \in \prederrbox(x) =[\boden(x), \decke(x)]$ 
%where \textit{floor function} $\boden(x) =\inf_{\phi \in \mathcal K_{post}} \phi(x)$ and  \textit{ceiling function } $\decke(x) = \sup_{\phi \in \mathcal K_{post}} \phi(x)$ delimit the values that any function in the posterior class $\mathcal K_{post}$ could give rise to. If a point prediction of a function value is required, we could choose any function value between the values given by the floor and ceiling which also give rise to the bounds on the point prediction. 
%Of course, the type of inference we get from this general procedure depends on the chosen prior class $\mathcal K_{prior}$ and the specifics of the data. We will develop \textit{kinky inference} which is a method for considering prior classes of multi-output functions over metric input spaces that are optionally constrained by boundedness and by knowledge of H\"older regularity as well as knowledge on uncertainty bounds on the observations and function inputs. For this class of inference mechanisms we prove conservatism and convergence guarantees to the learning target. What is more, we will consider classes where the imposed regularity assumptions are uncertain or adapted lazily to adjust for overly restrictive prior assumptions that do not fit the observations.
%
%
%
%This capability of imposing boundedness assumptions, accommodating for noise and being able to adjust the regularity assumptions will prove of great importance in the 
%control applications of our method.
%
%\subsection{The framework of conservative inference -- definitions, setting and desiderata }
%\label{sec:prob_def}

%As a basic example, consider the ordinary differential equation $\frac{\d x}{\d t} = (\xi - x)$ where $\xi: I \subset \Real \to \Real $ is an absolutely continuous function superimposed by a countable number of steps. Suppose, the ODE describes the trajectory $x: I \to \Real$ of a controlled particle in one-dimensional state space. Based on $N$ time-state observations $D_N=(t_1,x_1 ),..., (t_N,x_N )$ we desire to estimate the total distance travelled $S$ in time interval $I$, $S = \int_I x(t) \d t$. Solving


%%\textbf{Setting.}
%Let $(\inspace, \metric)$, $(\outspace ,\metric_\outspace)$ be two metric spaces and $f: \inspace \to \outspace$ be a function. Spaces $\inspace, \outspace$ will be referred to as \textit{input space} and \textit{output space}, respectively.
%Assume, we have access to a \textit{sample set} $\data_n:= \{\bigl( s_i, \tilde f_i, \obserr(s_i) \bigr) \vert i=1,\ldots, N_n \} $ containing $N_n \in \nat$ sample vectors $\tilde f_i \in \outspace$ of function $f$ at sample input $s_i \in \inspace$. To aide our discussion, we define $\grid_n =\{s_i | i =1,\ldots,N_n\}$ to be the \textit{grid} of sample inputs contained in $\data_n$.
%
%
%The sampled function values are allowed to have interval-bounded \textit{observational error} given by $\obserr : \inspace \to \Real^m_{\geq 0}$. That is, all we know is that $f(s_i) \in \obserrhyprec_i := [\underline f_1(s_i), \overline f_1(s_i) ] \times \ldots \times [\underline f_d(s_i), \overline f_d(s_i) ]$ where $\underline f_j(s_i) := \tilde f_{i,j} - \obserr_j(s_i)$, $\overline f(s_i) := \tilde f_{i,j} + \obserr_j(s_i)$ and $\tilde f_{i,j}$ denotes the $j$th component of vector $\tilde f_{i}$.
%
%The interpretation of these errors depends on the given application. For instance, in the context of system identification, the sample might be based on noisy measurements of velocities. The noise may be due to sensor noise or may represent numerical approximation errors. As we will see below, $\obserr$ may also quantify \textit{input} uncertainty (that is when predicting $f(x)$, $x$ is uncertain). This is an important case to consider, especially in the context of control applications where the ground truth might represent a vector field or an observer model.
%
%
%It is our aim to learn function $f$ in the sense that, folding in knowledge about $\data_n$, we infer \textit{predictions} $\predf(x)$ of $f(x)$ at unobserved \textit{query inputs} $x \notin \grid_n$. Being the target of learning, we will refer to $f$ as the \emph{target} or \emph{ground-truth} function. 
%
%In addition to the predictions themselves, we are also interested in \textit{conservative bounds} on the error of the inferred predictions. Depending on the hypothesis space under consideration these bounds can be of a probabilistic or deterministic nature. In this chapter, for the time being, we are interested in the latter.
%
%That is, we desire to provide a computable \textit{prediction uncertainty} function $\prederr: \inspace \to \outspace$ such that we can guarantee that for any query $x$, our prediction $\predf(x)$ is within the cube of error given by $\prederr(x)$ as follows 
%
%
%Being interested in conservative worst-case guarantees, we are mostly interested 
%
%
%
%In order to be able to deduce the error bounds around the predictions $\predf$, it is important to impose a priori restrictions on the class of possible targets (the hypothesis space). 

%\textbf{Definitions.}
%
\textbf{Setting.}  Let $\inspace$, $\outspace$ be two spaces endowed with (pseudo-) metrics $\metric: \inspace^2 \to \Real_{\geq 0}, \metric_\outspace:\outspace^2 \to \Real_{\geq 0}$, respectively. Spaces $\inspace, \outspace$ will be referred to as \textit{input space} and \textit{output space}, respectively. 
It will be convenient to restrict our attention to input and output spaces that are additive abelian groups and which are \emph{translation-invariant} with respect to their (pseudo-) metrics. That is, for the input space $\inspace$, we assume $ \metric(x+x',x''+x') = \metric(x,x''),\forall x,x',x'' \in \inspace$. 

For simplicity, throughout the remainder of this work, we will assume the output space is the canonical Hilbert space $\outspace = \Real^m$ $(m \in \nat)$ endowed with the $\metric_{\outspace}(y,y') = \norm{y-y'}_\infty, \forall y,y' \in \outspace$. 

Let $f: \inspace \to \outspace$ be a \emph{target} or \emph{ground-truth} function we desire to learn. For our purposes, learning means regression. That is, we utilise the data to construct a computable function that allows us predict values of the target function at any given input.

%\footnote{Extensions to more general output spaces seem very possible, albeit, instead of learning a function, we would then learn a discrepancy from a nominal reference in output space. We will leave this to future work.}
%In contrast, we do not impose restrictions on the input space (pseudo-) metric. 
%While our simulations will consider the deterministic case, it would be entirely possible to consider input spaces that are index sets of stochastic processes endowed with suitable norm metrics. Since the output metric is defined via a norm, we will often drop the subscript of the input metric. That is we may on occasion write $\metric$ instead of $\metric$.





Assume that, at time step $n$, we have access to a \textit{sample} or \textit{data set} $\data_n:= \{\bigl( s_i, \tilde f_i \bigr) \, \vert \, i=1,\ldots, N_n \} $ containing $N_n \in \nat$ sample vectors $\tilde f_i = \tilde f(s_i) \in \outspace$ of an \emph{observable}   function $\tilde f$ at sample input $s_i \in \inspace$. Here, the observable $\tilde f : \inspace \to \outspace$ is a ``noise-corrupted'' version of the true \emph{target function} $f: \inspace \to \outspace$ we would like to make inferences about on the basis of the available sample. In this work, we will typically assume that the observable $\tilde f$ coincides with the target $f$ up to a level of interval-bounded observational noise: $\forall x \in \inspace: \metric_\outspace(\tilde f(x),f(x) ) \leq \obserr(x) $ where $\obserr : \inspace \to \Real_{\geq 0}$ is the error bound function whose values we assume to be bounded by some (known or unknown) bound $\obserrbnd \in \Real_{\geq 0}$. We can model the situation by the presence of a bounded additive observational error (or ``noise'') function $\noise:\inspace \to \outspace$ with $\tilde f = f + \noise$.
%That is, all we know is that $\tilde f_i = \tilde f(s_i) \in \obserrhyprec_i := [\underline f_1(s_i), \overline f_1(s_i) ] \times \ldots \times [\underline f_d(s_i), \overline f_d(s_i) ]$ where $\underline f_j(s_i) := \tilde f_{i,j} - \obserr_j(s_i)$, $\overline f(s_i) := \tilde f_{i,j} + \obserr_j(s_i)$ and $\tilde f_{i,j}$ denotes the $j$th component of vector $\tilde f_{i}$. 
The interpretation of these errors depends on the given application and this ``noise'' may be deterministic or stochastic. For instance, in the context of system identification, the sample might be based on noisy measurements of velocities and it may be due to sensor noise or, the noise might model systematic error such as numerical approximation errors. 

Furthermore, $\obserr$ may also accommodate \textit{input} uncertainty (that is when predicting $f(x)$, $x$ is uncertain) (for details refer to \cite{calliess2014_thesis}). In the course of our theoretical considerations below the error will also serve to absorb the discrepancy between a H\"older and a non-H\"older function.
%
%This is an important case to consider, especially in the context of control applications where the ground truth might represent a vector field or an observer model. Finally, the observational error can also model error around the computation of the metric. This might be of interest if the metric has to be approximated numerically or estimated with statistical methods that provide confidence intervals (in the latter case our predictions also only hold within pertaining confidence bounds). 

\textbf{Learning.}
It is our aim to learn target function $f$ in the sense that, combining prior knowledge about $f$ with the observed data $\data_n$, we infer \textit{predictions} $\predfn(x)$ of $f(x)$ at unobserved \textit{query inputs} $x \notin \grid_n$. Here, $\grid_n =\{s_i | i =1\ldots,N_n\} \subset \inspace$ refers to the (not necessarily regular) \emph{grid} of sample inputs. The entire function $\predfn$ that is learned to facilitate predictions is referred to as the \textit{predictor}. Since the computation of the predictor is based on the available data and utilised to make inferences over unobserved inputs, we can view the learning process as an instance of (inductive) inference. Therefore, the formula to compute the predictor $\predfn$ will also be referred to as an inference rule.
%
%For a discussion of the competing definitions of non-deductive inference in a philosophical context, the reader is referred to \cite{Flach2000}. 
%
In our context, we will understand a \textit{machine learning algorithm} to implement a such an inference rule. That is, it is a computable function that maps a data set $\data_n $ to a 
 predictor $\predf_n$ (and possibly an uncertainty estimate function $\prederr_n$). 
A typical \textit{desideratum} of a good predictor is that it is \textit{efficiently computable}. Its learning performance is measured in terms of the degree and rapidity it  \textit{converges to the target} (up to the observational error given by $\obserr$) in the limit of increasingly dense data. Of course there are many different metrics with respect to which one can assess convergence. Perhaps, the most convenient one is mean-square convergence. However, inspired by our control applications, we desire to investigate worst-case convergence rates which hold independently from distributional assumptions and will yield performance guarantees even in zero-measure events.
%Typically,
%the predictor lies in the space that coincides with (or is at least dense in) the a priori hypothesis space $\mathcal K_{prior}$ of conceivable target functions. In this case the predictor can be referred to as a \textit{candidate function} or \textit{hypothesis} \cite{mitchellbook:97}.

%In addition to the predictions themselves, we are also interested in \textit{uncertainty bounds} on the error of the inferred predictions. 
%%Depending on the hypothesis space under consideration, these bounds can be of a probabilistic or deterministic nature. In this chapter, we  restrict ourselves to the latter.
%
%That is, we desire to provide a computable \textit{prediction uncertainty function} $\prederr: \inspace \to \outspace$ such that we \textit{believe} that for any query $x \in \inspace$, the ground truth value $f(x)$ lies somewhere within the \textit{uncertainty hyperrectangle }
%\begin{equation}
%	\prederrbox_n(x) := \Bigl\{ y \in \outspace \, | \, \forall j \in \{1,...,\dim{\outspace}\} : y_j \in \prederrbox_{n,j}(x)\Bigr\}
%\end{equation} around the prediction $\predfn (x)$ where 
%\begin{equation}\label{eq:prederrint}
%	\prederrbox_{n,j}(x) : = [ \predfnj(x) - \prederrnj(x), \predfnj(x) + \prederrnj(x)] 
%\end{equation}
%is referred to as the $j$th \textit{prediction uncertainty} interval.
%Here, $\predfnj(x)$, $\prederrnj(x)$ denote the $j$th components of vectors $\predfn(x), \prederrn(x)$, respectively.

 %As a word of caution, we remark that using the last statement as a definition still seems very broad. 

%\textbf{Desiderata.}


%The resulting learning or inference rule is called \textit{conservative} if the uncertainty quantifications never underestimate the error. That is, based on the an a priori assumption $f \in \mathcal K_{prior}$, we can guarantee $f(x) \in \prederrbox_n(x), \forall x$, regardless of the observed data set $\data_n$.
\textbf{The Kinky Inference Learning rules.}
In this work we will expand on the basis of the following class of predictors to perform learning as inference over unobserved function values:

\begin{defn}[Kinky Inference (KI) rule ] \label{def:KIL}
Let  $\Real_\infty := \Real \cup\{- \infty, \infty\}$ and $\inspace$ be some space endowed with a pseudo-metric $\metric$. Let $\lbf,\ubf: \inspace \to \outspace \subseteq \Real_\infty^m$ denote \textit{lower- and upper bound functions}, that can be specified in advance and assume $\lbf(x) \leq \ubf(x), \forall x \in I \subset \inspace$ component-wise. 
Furthermore, let $\obserrpar$ denote a parameter that specifies a deterministic belief about the true observational error bound $\obserr$.
Given sample set $\data_n$, we define the predictive functions $\predfn: \inspace \to \outspace, \prederrn: \inspace \to \Real^m_{\geq 0}$ to perform inference over function values.
For $j=1,\ldots,m$, their $j$th output components are given by:
%Furthermore, define
% $\coeff1,\coeff2 \in \Real_{\geq0}$ such that $\coeff1+\coeff2 =1$ (unless explicitly stated otherwise, we assume $\coeff1=\coeff2 =\frac 1 2)$.
	\begin{align*}
   \predfnj(x; \param(n)) :=& \frac{1}{2} \min\{ \ubf_j(x), \decke_{n,j}(x;\param(n)\bigr)\} \\
    &+ \frac{1}{2} \max\{ \lbf_j(x), \boden_{n,j}(x;\param(n)\bigr) \},\\
	\prederrnj(x; \param(n)) :=& \frac{1}{2} \min\{ \ubf_j(x), \decke_{n,j}\bigl(x;\param(n)\bigr)\} \\
	&- \frac{1}{2} \max\{ \lbf_j, \boden_{n,j}\bigl(x;\param(n)\bigr) \}.
	\end{align*}
	Here, $\decke_n\bigl(\cdot;\param(n)\bigr), \boden_n\bigl(\cdot;\param(n)\bigr): \inspace \to \Real^m$ are called ceiling and floor functions, respectively. Their $j$th component functions are given by
	\[\decke_{n,j}\bigl(x; \param(n)\bigr) := \min_{i=1,\ldots,N_n}   \tilde f_{i,j} +  \tilde \metric(x,s_i;\param(n)) \] and 
	\[\boden_{n,j}\bigl(x; \param(n)\bigr) := \max_{i=1,\ldots,N_n}   \tilde f_{i,j} -  \tilde  \metric(x,s_i;\param(n)),\] respectively.
  Here, $\tilde \metric (\cdot,\cdot;\param(n))$ is a mapping parameterised by $ \param(n)$. While there are many conceivable parameterisations, we restrict our attention to the case where, for some pseudo-metric $\metric$ on the input space $\inspace$, we have $\param(n) = (L(n), \hexp,\obserrpar)$ with $$\tilde \metric(\cdot,\cdot; \param(n)) = L(n) \metric^\hexp(\cdot,\cdot) + \obserrpar(x).$$
  As will be seen below,  parameter $L(n)$ has the interpretation of a H\"older constant of the predictor relative to pseudo-metric $\metric$ while $\hexp \in (0,1]$ can be interpreted as a H\"older exponent (cf. Thm. \ref{lem:LACKIpredHoelder}). That is, we will show that $\predfn(\cdot;\param(n))$ belongs to the class $$\Hoelset \bigl(L(n),\hexp\bigr) = \{ \phi: \inspace \to \outspace | \forall x,x' \in \inspace : \metric_\outspace(\phi(x),\phi(x') ) \leq L(n) \metric(x,x')^\hexp\}$$ of $L(n)-\hexp$- H\"older continuous functions. Note, we could alternatively re-express this H\"older class as a generalised class of Lipschitz functions $\text{Lip}(L(n))= \{ \phi: \forall x,x' \in \inspace: \Metrico{\phi(x)}{\phi(x')} \leq L(n) \tilde \metric (x,x')\} $ where, for any $\hexp \in (0,1]$, $\tilde \metric = \metric^\alpha$ is a pseudo-metric provided  $\metric$ is (refer to Lem. \ref{lem:hoeldererror_metric}). However, as it is often customary to define Lipschitz and H\"older continuity in a more restricted sense relative to standard norm-induced metrics (in which case the H\"older class is strictly more general than the Lipschitz class) we chose to refer to H\"older continuity rather than Lipschitz continuity to highlight that such H\"older functions can be learned as well.
  
  As insinuated by our notation, we consider parameter $L(n)$ to be adaptive, i.e.  data-dependent while the other parameters are assumed to be set in advance.
 Function $\obserrpar$ can be utilised to accommodate observational noise. 
That is, if the noise level in the data is assumed to be contained in $[-\obserrbnd, \obserrbnd]$ then one would choose $\obserrpar(x) = \obserrbnd,\forall x$.
 % 
In addition,  functions $\lbf,\ubf:  \inspace \to \Real_\infty^m$ are parameters that have to be specified in advance and can impose a priori knowledge of bounds on the target function. For example, if we know the target function to exclusively map to nonnegative values, then one can set $\lbf(x) = 0,\forall x$.
To disable restrictions of boundedness, it is allowed to specify the upper and lower bound functions to constants $\infty$ or $-\infty$, respectively.	

  
Function $\predfn$ is the predictor that is to be utilised for predicting/inferring function values at unseen inputs. Function $\prederrn(x;\param(n))$ is meant to quantify the uncertainty of prediction $\predfn(x;\param(n))$. 
For ease of notation, we shall often omit explicit mention of the parameter, e.g. we may write $\predfn(x)$ instead of $\predfn(x;\param(n))$.
	%Note, if the data set is fixed (i.e. $n$ does not change), we may sometimes drop the subscript $n$ and write $\predf$ instead of $\predf_n$.
\end{defn}


To provide an intuition of the inference rule, consider the following special case where we have access to a noise-free sample $\data_n$ and suppose 
the target $f$ is a real-valued $L^*-\hexp$ H\"older continuous function. Observing the noise-free sample point $(s_i,f_i)$ constrains the set of function values $f(x)$ to the set $\mathbb S_i(x) =\{ \phi \in \outspace | \metric_\outspace(\phi, f_i) \leq L^* \metric(s_i,x) \}$. Considering a set of sample points $\data_n$, target value $f(x)$ is constrained to lie in the intersection $\mathbb S(x)=\cap_{i=1}^{N_n} \mathbb S_i(x)$. It is easy to see that the floor and ceiling functions are tight lower and upper bounds of $\mathbb S(x)$ with $\mathbb S(x) := \{ \phi \in \outspace | \boden_n(x; L^*) \leq \phi \leq \decke_n(x;L^*)\}$. In other words, setting parameter $L(n)$ to the best H\"older constant $L^*$ and bounds $\lbf =-\infty,\ubf=+\infty$ yields a predictor $\predfn(x)$ that for every query $x$ chooses the mid-point of the set $\mathbb S(x)$ of those function values that can possibly be assumed by a H\"older continuous function that interpolates the observed sample. Prediction error $\prederrn(x)$ simply is the radius of the set.

For the case of $\hexp=1$, this approach is known as \emph{Lipschitz interpolation} \cite{Beliakov2006,Zabinsky2003}. Since a set is utilised for interpolation, the approach is also known as \emph{Nonlinear Set Interpolation} \cite{Milanese2004,Canale2014} in control. Specification of $\ubf,\lbf$ allows us to incorporate additional knowledge and constrain our set $\mathbb S(x)$ further. 
For instance, when estimating densities we might incorporate the knowledge of dealing with nonnegative functions. In this case, it makes sense to set $\lbf$ to a constant value of zero yielding $\mathbb S(x) = \{\phi | \phi \geq 0 \} \cap_{i=1}^{N_n} \mathbb S_i(x) $.

%\begin{figure*}
        %\centering
				  %\subfigure[Initial prediction $\predf_1$.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/akt2learneddrift}
    %\label{fig:KIcollavoidopenlooppredmodels1}
  %} 	 
					  %\subfigure[Improved prediction $\predf_2$.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/akt3learneddrift}
    %\label{fig:KIcollavoidopenlooppredmodels2}
  %} 	
							  %\subfigure[Social cost after each experiment.]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm, clip, trim = 3.1cm 9.5cm 4.5cm 9cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/soccost}
    %\label{fig:KIsoccost}
  %} 
	%\label{fig:KIcollavoidopenlooppredmodels}
   %\caption{Belief over drift models based on $\data_1$ and $\data_2 \supset \data_1$ with $\abs{\data_1} = 2, \abs{\data_2} = 100$. Here, the top figures show the predictions of $\predf_{n,3}(s)$ and the bottom plots depict the predictions of $\predf_{n,4}(s)$ for $n =1$ and $n=2$, respectively. The ground-truth drift model was $f(x) = \bigl(0,0, - \sin(0.5 \, x_1), - \sin( 0.5 \, x_2) \bigr)^\top$. Rightmost plot: Social cost after each experiment. Note how the reduced uncertainty translated to reduced social cost of the last experiment (bar plot 3) vs the cost in the second (bar plot 2). While the first experiment (bar plot 1) also accumulated low social cost, a collision occurred.}
%\end{figure*}	 
%
%\begin{figure}
%        \centering
%				  \subfigure[KI prediction with two examples.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.1cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/ex1hfe1.pdf}
%    \label{fig:hfe1}
%  } 	
%	 \subfigure[Refined prediction.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.1cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/ex1hfe2.pdf}
%    \label{fig:hfe2}
%  } 	%\hspace{2cm}
%	  \subfigure[Using a periodic pseudo-metric.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.1cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/ex1hfeperiodic.pdf}
%    \label{fig:hfe3}
%  } 	
%   \caption{Examples of different target functions and full kinky inference predictions. \textbf{Fig. \ref{fig:hfe1} and  Fig. \ref{fig:hfe2}} show kinky inference performed for two and ten noisy sample inputs of target function $x\mapsto \sqrt{\abs{\sin(x)}}$ with observational noise level $\varepsilon =0.3$. The floor function folds in knowledge of the non-negativity of the target function ($\lbf = 0$). The predictions were made based on the assumption of $p=\frac 1 2$ and $L = 1$ and employed the standard metric $\metric(x,x') = \abs{x-x'}$. 
%	As can be seen from the plots, the function is well interpolated between sample points with small perturbations. Furthermore, the target is within the bounds predicted by the ceiling and floor functions.
%		\textbf{Fig. \ref{fig:hfe3}} depicts a prediction folding in knowledge about the periodicity of the target function by choosing a pseudo-metric $\metric = \Bigl|\sin(\pi \abs{x-x'}\Bigr|$. The prediction performs well even in unexplored parts of input space taking advantage of the periodicity of the target. This time, there was no observational error and the target function was $x \mapsto \abs{\sin(\pi x)} +1$.   }
%			\label{fig:exHfe1}
%\end{figure}	  

%
%\begin{figure}
%        \centering
%							  %\subfigure[Wingrock dynamics.]{
%    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    %\includegraphics[width = 5.5cm]
%								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								%{content/Ch_kinkyinf/figs/hfewingrock_dyn_groundtruth}
%    %\label{fig:KIvs2NN}
%  %} 	
%				  \subfigure[Wingrock dynamics.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 5.5cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/hfewingrock_dyn_groundtruth}
%    \label{fig:hfe5}
%  } 	
%	 \subfigure[Inferred model.]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 5.5cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/Ch_kinkyinf/figs/hfewingrock_dyn_learned}
%    \label{fig:hfe4}
%  } 	%\hspace{2cm}
%	 
%%
%   \caption{Example of a prediction of the KI rule on two-dimensional input space. \textit{Left plot:} the target function being a patch of the wingrock dynamics we will study in Sec. \ref{sec:KIMRAC}. \textit{Right plot:} the predictions inferred on the basis of 100 sample points using metric $\metric(x,x') = \norm{x-x'}_\infty$ and $p=1, L=2.5$.}
%		\label{fig:exHfe2}
%\end{figure}	 

%Note the inference rule is nonparametric in that, that its complexity grows with the sample size. However, as any inference method one has to a priori specify prior knowledge, some of which is encoded in hyper-parmeters. In the KI rule, these parameters include the choice of pseudo-metric (or its parameters), parameter $\hexp$, the sequence of constants $\seq{L(n)}{n \in \nat}$ as well as the presupposed level of observational error $\obserr$.

%To develop a first feel for this kinky inference rule, we plotted some examples of target functions and pertaining predictions in Fig. \ref{fig:exHfe1}. %and Fig. \ref{fig:exHfe2}.
%Firstly, we can see that the predictions involve kinks. This is due to the minimisations and maximisations that occur in the computation of the ceiling and floor functions which introduce kinks into the prediction signal. This property provided the motivation behind the term ``kinky inference'' \cite{calliess2014_thesis}.

When choosing $L(n)$ to coincide with the best H\"older constant, one can give strong guarantees of convergence to the target as on the tightness of the prediction bounds  \cite{Sukharev1978,calliess2014_thesis} showing that bounds are as tight as possible without imposing additional assumptions and that the predictor minimises the worst-case risk.

Unfortunately, this requires us to know at least an upper bound of $L^*$ and therefore, several authors have proposed different approaches of how to estimate the constant from the data (e.g. \cite{Strongin1973,Wood1996}). However, it appears to be largely unknown how to do so in the presence of bounded observational noise $\obserr >0$ in a principled manner. Furthermore, when we replace $L(n)$ by the empirical estimates, nothing seems to be known about the convergence properties of the resulting kinky inference rule that is based on such  estimates.  

In the remainder of the paper, we shall address this gap. Firstly, we propose an estimator to be utilised in place of $L(n)$ that can be set to be robust to noise (i.e. does not grow unbounded). Referring to the resulting KI rule as LACKI, we then prove universal approximation properties of the LACKI rule before considering its performance in a control application.


\subsection{Lazily Adapted Constant Kinky Inference (LACKI)}
\label{sec:lacki}
Above we explained the benefits of choosing parameter $L(n)$ to coincide with a H\"older constant of the target. 
However, if such a constant is unavailable a priori, we desire to compute $L(n)$ as a data-dependent estimate of the H\"older constant. Our proposal for such an estimator will be introduced next. 

For notational convenience, for two sets $S,S' \subset \inspace$ of inputs we define  $$U(S,S') := \{(s,s') \in S \times S' | \metric(s,s') >0\} \text{ and  let } U_n := U(\grid_n,\grid_n) $$ be the set of all pairs grid inputs deemed disparate under the pseudo-metric $\metric$.

The \emph{best} H\"older constant of a function $f$ is the smallest nonnegative number $L^*$ such that $f$ is contained in the set 
$\hoelset {L^*}{}{p} = \{\phi: \inspace \to \outspace \, \vert \, \forall x,x' \in \inspace : \metric_\outspace \bigl(\phi(x),\phi(x')\bigr) \leq L^* \, \bigl( \metric (x,x') \bigr)^\hexp\} $ of $L^*-\hexp$- H\"older continuous functions. So, this best H\"older constant is given by  
%
$$L^* = \sup_{(x,x') \in U(\inspace,\inspace)} \frac{\metric_\outspace \bigl(f(x) - f(x')\bigr)}{\metric^\hexp(x,x') }.$$




Given the noisy data $\data_n = \{(s_i,\tilde f_i) | i=1,\ldots,N_n\}$ a natural estimate of the best H\"older constant might be to compute $\hat \ell_n^* := \max_{(s,s') \in U_n} \frac{\metric_\outspace(\tilde f(s),\tilde f(s')) }{\metric^\hexp(s,s')}$ \cite{Strongin1973}. In the absence of \emph{noise} (may it be stochastic or deterministic), that is, if $\tilde f_i = f(s_i),\forall i$, $\hat \ell_n^*$ never overestimates the true best H\"older constant. That is, $\hat \ell_n^* \leq L^*$. However, in the presence of noise $\noise: \inspace \to \outspace$ (such that $\tilde f = f+ \noise$) this boundedness assumption of the estimates no longer holds true. In particular if the noise is not H\"older continuous, we expect $\hat \ell_n^*$ to grow unbounded with increasingly dense data.
For practical reasons and for the sake of our theoretical arguments presented below, we desire the parameters $L(n)$ to remain bounded. Thus, without further modifications $\hat \ell_n^*$ is not a suitable candidate for $L(n)$.

To ensure bounded estimates even in the presence of noise, we propose the following estimator : %
\begin{equation}\label{eq:lazyconstupdaterule_batch_main}
\ell(\data_n;\hestthresh,\underline L)  := 
 \max \Bigl\{ \underline L, \max_{(s,s') \in U_n} \frac{\metric_\outspace(\tilde f(s),\tilde f(s')) - \hestthresh}{\metric^\hexp(s,s')} \Bigr\}.
\end{equation}
\begin{figure}
        \centering
    \includegraphics[width = 8.8cm,height = 4cm]
								{content/figs/LACKIhestthreshvar}
   \caption{Two LACKI inferences over function values of the target $f: x \mapsto \abs{\cos(2\pi x)}+x$ (dashed line) on the basis of a noisy sample (plotted as dots). The predictors are plotted in grey, the noisy observational function $\tilde f (\cdot) = f(x) + \nu_x$ is plotted in cyan. Here the $\nu_x$ were drawn i.i.d. at random from a uniform distribution on the interval $[-0.5,0.5]$. In both cases we chose the parameters $\ubf \equiv \infty,\lbf \equiv -\infty,\underline L = 0$ and $\hexp=1$.
   The left plot shows the LACKI predictor $\predfn$ (grey line) for parameter choice $\hestthresh =0$, falsely assuming absence of observational noise. As a result, the prediction overfitted to the noise. The right plot depicts the prediction $\predfn$ (grey curve) for correct parameter choice $\hestthresh = 2 \obserrbnd =1$, causing the noise to be smoothed out and resulting in more accurate prediction of the underlying ground truth $f$.  }
			\label{fig:LACKInoise}
\end{figure}

%
Here $\underline L$ is a parameter that can be used to specify a priori knowledge of a lower bound on the best Lipschitz constant. In the absence of particular domain-specific knowledge, one can of course always set $\underline L =0$.
%
\begin{rem} \label{rem:bndedlipconstestimates}
By setting parameter $\hestthresh$ at least as large as twice the maximum level of observational noise, i.e. $\hestthresh = 2 \obserrbnd + q$ for some $q\geq0$, it is easy to see that the $\ell(\data_n;\hestthresh,0)$ are bounded from above by $\bar L  =\sup_{x,x', \metric(x,x') >0} \frac{\metric_\outspace(f(x), f(x'))   -q}{\metric^\hexp(x,x')} \leq L^* $ ( and,  $L^* < \infty$ if the target is H\"older continuous). 
\end{rem}
%
Next, consider an online learning situation where the available data increases over time. 
That is, $\data_n \subseteq \data_{n+1}$ for all time steps $n \in \nat$. 
For time step $n \in \nat$, let $S_{n+1} := G_{n+1} \backslash \grid_n$ be the set of new sample inputs.
We can define an incremental update rule recursively as follows: 
\begin{align} \label{eq:Hoelconstlazyupdateincr_main}
\ell_{n+1} := \max\Bigl\{ & \ell_n, \max_{(s,s') \in U(\grid_n, S_{n+1})} \frac{\metric_\outspace\bigl(\tilde f(s),\tilde f(s')\bigr) - \hestthresh}{\metric^\hexp(s,s')},\\
&\max_{(s,s') \in U(S_{n+1}, S_{n+1})} \frac{\metric_\outspace\bigl(\tilde f(s),\tilde f(s')\bigr) - \hestthresh}{\metric^\hexp(s,s')} \Bigr\},
\end{align} for $n \in \nat$ 
and where 
$\ell_0 := \underline L$. 
The effort of computing $\ell_{n+1}$ is in the order of $\mathcal O\bigl(M (\abs{S_{n+1}} N_n+ \abs{S_{n+1}}^2)\bigr)$ where $M$ denotes the effort for evaluating the pseudo-metrics.
By construction, we have $\ell_n =\ell(\mathcal \data_n;\hestthresh,\underline L), \forall n \in \nat.$ 

\begin{rem}\label{rem:convlipconstestimates}
Remember that $\seq{\ell_n}{n\in \nat}$ is bounded. Since it is also growing monotonically we can appeal to the monotone convergence theorem to show that the sequence is convergent to some number $\bar L \leq \max\{L^*,\underline L\}$.
\end{rem}

So far, we have defined a rule of how to update noise-robust and convergent estimates $\ell_n$ of the H\"older constant. Using these data-dependent estimates in place of $L(n)$ in our kinky inference framework as per Def. \ref{def:KIL} yields an inference rule that shall henceforth be referred to as \textit{Lazily Adapted Constant Kinky Inference (LACKI)}.

\begin{defn}[LACKI rule] \label{def:LACKI} For each output component $j \in \{1,\ldots,\text{dim} \, \outspace \}$ 
define $\predfn(\cdot)_{j}$  as per Def. \ref{def:KIL} but assume we choose the parameters $L(n) := \ell(\data_n;\hestthresh,\underline L)$ (according to Eq. \ref{eq:lazyconstupdaterule_batch_main}). We refer to the resulting predictor $\predfn\bigl(\cdot \bigr)$ as a \emph{Lazily Adapted Constant Kinky Inference (LACKI)} rule. Here, the free parameters are $\hexp \in (0,1], \hestthresh \in \Real_{\geq 0}$ and $\underline L \in \Real_{\geq 0}$.  
\end{defn}

To develop a first feel for our inference rule, refer to Fig. \ref{fig:LACKInoise}. Here, we depicted the predictors for an underlying ground-truth function on the basis of a sample but with different parameter choices $\hestthresh$. When setting this parameter to two times the observational noise level, the predictor accurately smoothes out the noise. In contrast, when the parameter is set to zero, the resulting predictor will perfectly interpolate through the noisy observations, thereby limiting the approximation quality to the level of observational noise. 

Furthermore, we notice that the predictors are H\"older continuous but non-differentiable. Informally speaking, the inference exhibits ``kinks'', motivating the term ``kinky inference''.

Finally note, the estimator $\ell_n$ determining  parameter $L(n)$ is ``lazy'' in the sense that it only increases the estimate of the H\"older constant just enough to be consistent with the observed data. That is, it chooses $L(n)$ to coincide with the smallest H\"older constant of a conceivable target function $f$ that could have generated the data under the given noise assumption. Below, we will see that the predictor $\predfn$ has H\"older constant $L(n)$. Therefore, the ``laziness'' of the estimator of $L(n)$ implements \emph{Occam's razor}: it \emph{regularises} the hypothesis space of continuous functions to prefer simple explanations of the data (i.e. functions with low H\"older constants) over complex ones (i.e. functions with higher H\"older constants). Here, $\hestthresh$ can serve as a parameter that can be utilised to regularise the predictor further in order to compensate for (bounded) noise in the data. 



\begin{figure}
        \centering
    \includegraphics[width = 8.8cm,height = 4cm]
								{content/figs/LACKIhestthreshvar_with_bounds}
   \caption{Repetition of the experiment but with $p=0.5$. This time, we also plotted floor and ceiling functions (grey dotted and dashed-dotted curves) delimiting the uncertainty bounds. Note, when setting $\lambda =0$ the estimate $\ell(\mathcal \data_n;\hestthresh,\underline L)$ was found to be 128 resulting in extremely conservative uncertainty estimates (left figure). In contrast, choosing $\lambda =2 \obserrbnd $ gave a parameter estimate $\ell(\mathcal \data_n;\hestthresh,\underline L) = 2.4$ yielding sensible uncertainty bounds (right figure). }
			\label{fig:LACKInoise2}
\end{figure}
%
%
%\begin{figure}
%        \centering
%				  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_trueLinit_7tex.pdf}
%    \label{fig:LACKInoise1}
%  } 	
%	 \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_noe_noalpha_smallLinit_7tex.pdf}
%    \label{fig:LACKInoise2}
%  } 	
%  %
%  %\hspace{2cm}
%	  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_smallLinit_7tex.pdf}
%    \label{fig:LACKInoise3}
%  } 
%  				  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_trueLinit_77tex.pdf}
%    \label{fig:LACKInoise4}
%  } 	
%	 \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_noe_noalpha_smallLinit_77tex.pdf}
%    \label{fig:LACKInoise5}
%  } 	
%  %
%  %\hspace{2cm}
%	  \subfigure[ ]{
%    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
%    \includegraphics[width = 4.8cm]
%								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
%								{content/figs/LACKInoise_e_alpha_smallLinit_77tex.pdf}
%    \label{fig:LACKInoise6}
%  } 	
%   \caption{LACKI inference on the basis of two noisy data sets 
%   $\data_1,\data_2$ with varying parameter settings. Target (blue curve) was $f:x \mapsto 5 \sqrt{\abs x}$ and observational model (magenta curve) $\tilde f: x \mapsto f(x) + \phi_x$ where $\phi_x$ is a uniformly distributed disturbance with $\phi_x \stackrel{i.i.d.}{\sim} \mathcal U(-0.5,0.5),\forall x$. 
%  %
%   \textbf{1st column:} Initial constant L(0) = 5; assumed obs. error bound $\obserrpar= 0.5$; $\hestthresh = 2 \obserr=1$. 
%   %
%   \textbf{2nd column:} Initial constant L(0) = 0.01; assumed obs. error bound $\obserrpar = 0$; $\hestthresh = 2 \obserr =0$.
%   %
%   \textbf{3rd column:} Initial constant L(0) = 0.01; assumed obs. error bound $\obserrpar = 0.5$; $\hestthresh = 2 \obserr =1$.
%   %
%   \textbf{Top row:} Data set $\data_1$ of size 7. 
%   \textbf{Bottom row:} Data set $\data_2$ of size 77.
%   In all cases the exponent parameter was set to $p = 0.5$.}
%			\label{fig:LACKInoise}
%\end{figure}
%
%The figure depicts the inference $\predfn$ (black curve)	 over function values of the target $f$ (blue curve) based on noisy data sets $\data_1$ and $\data_2$. The true observational noise was bounded by level $\obserrbnd = 0.5$ yielding a data-generating function $\tilde f(x) = f(x) +\nu(x)$ (magenta curve) where $\nu(x) \in [-0.5,0.5],\forall x$.
%The first row shows the predictions of our LACKI rule applied to a small sample $\data_1$ with varying parameter settings.
%The second row depicts the pertaining predictions resulting applying the corresponding LACKI rules to an enlarged data set $\data_2 \supset \data_1$.
%
%In plots in the first column and third columns depict situations where LACKI was applied with parameter $\hestthresh=2 \obserrbnd$.  By contrast, the second column depicts a situation where LACKI was parameterised with a parameter $\hestthresh = 0$ and a small initial guess of the H\"older constant of $\underline L = L(0) = 0.01$. As a result, in this case, the LACKI predictor perfectly follows the noisy data. Furthermore, we observe a large uncertainty bound $\prederrn$ with increasing sample size. In the third column the LACKI rule was also initialised with $\underline L =0.01$. However, the larger $\hestthresh = 2 \obserrbnd$ prevents 
%the H\"older constant estimate $L(2)$ to exceed the true constant $L^*=5$. As a result, the prediction ``smoothes out the noise''. The degree of smoothing and approximation error in the limit of infinite data will be theoretically investigated below. 
%At this point we will already mention that all behaviours depicted in the plots seem consistent with our theoretical guarantees we will give in what is to follow.


\subsection{Properties}
\label{sec:properties_lacki}
We will now establish several properties of the LACKI rules including boundedness of the predictors, sample-consistency and H\"older continuity. Most importantly however, we will show that the LACKI rules are universal approximators, in the sense that they can be set to learn any continuous function with arbitrary worst-case error.

The core idea behind this can be sketched as follows: 
First, we establish H\"older continuity and sample-consistency. This allows us to prove that LACKI can learn any H\"older function.
Note, some universal approximators, such as RBFNs with Gaussian kernels, are provably Lipschitz. Therefore, learning any continuous function can be interpreted as learning some Gaussian RBFN with an observational error level that absorbs the discrepancy between the RBFN and the ground truth. Since a finite RBFN with smooth, bounded-derivative kernel is provably H\"older and since we can learn any H\"older function with LACKI up to the level of observational error, we can learn the continuous ground-truth up to the approximation error of the RBFN. 

Following this outline, we will now proceed to establish the desired properties formally.

\begin{lem}[Boundedness of the predictor]
Irrespective of the boundedness of input space $\inspace$ and assuming finite sample size  $N_n=\abs{\data_n} < \infty$, the predictor $\predfn:\inspace \to \outspace$ is bounded. In particular,
for $\hexp =1$, we have  
$\forall x \in \inspace: \norm{\predfn(x)}_\infty \leq \max_{i=1,...,N_n} \norm{\tilde f_i}_\infty + \frac{L(n)}{2}  \max_{i,j = 1,...,N_n} \metric^\alpha(s_i,s_j) <\infty$.
\begin{proof}
Let $D = \max_{i,j = 1,...,N_n} \metric^\hexp(s_i,s_j)$ and for the $k$th output dimension let  $F_k= \max_{i=1,...,N_n} \abs{\tilde f_{i,k}}$. As shown in Sec. \ref{sec:Hoelder_brief}, $\metric^\hexp$ is a pseudo-metric too and hence, adheres to the triangle inequality. Utilising the definition of the predictor and the triangle inequality we see that, for any  $x \in \inspace$ and any output dimension $k$, there are some $i,j \in \{1,...,N_n\}$ such that we have: 
$\predf_{n,k}(x) =\frac{\tilde f_{j,k} + \tilde f_{i,k}}{2} + \frac{L(n)}{2} \bigl( \metric^\hexp(x,s_i) - \metric^\hexp(x,s_j) \bigr) \leq \frac{\tilde f_{j,k} + \tilde f_{i,k}}{2} +  \frac{L(n)}{2} \metric^\hexp(s_j,s_i) \leq F_k + \frac{L(n)}{2}  D < \infty$.
% We can represent $\predfn$ as a function of the form 
%$g(h_1,...,h_{N_n})$ with $h_i(x) = \metric(x,s_i)$. Now, assume $\hexp \neq 1$. Defining $p: x \mapsto = x^\alpha$. Since 
\end{proof}
\label{lem:LACKIpredbounded}
\end{lem}

As promised, we establish that the predictors of the LACKI inference rule are H\"older continuous:
\begin{lem}[H\"older regularity of LACKI]
With definitions as before, let $(\outspace,\metric_\outspace) = (\Real^m,(x,y) \mapsto \norm{x-y}_\infty)$.
Provided that the bounding functions $\lbf,\ubf$ are H\"older continuous (or set to $-\infty,\infty$, respectively),
the predictors $\predfn$ are H\"older continuous $(n \in \nat)$ with constant $L(n)$ and exponent $\hexp$. That is, $\forall n \in \nat: \predfn \in \Hoelset \bigl(L(n),\hexp\bigr)$.

\begin{proof}
It is easy to show that the one-dimensional mappings of the form $x \mapsto \ell \Metrici{x}{x'}^\hexp$ are $\ell-\hexp-$ H\"older continuous for any choices of $\ell,\hexp$ and inputs $x'$. Furthermore, taking point-wise $\max$, $\min$ as well as averages of H\"older continuous functions is known to not change their H\"older properties (e.g. cf. \cite{calliess2014_thesis}). Therefore, the output-component predictors  $\predf_{n,j}$ $(j=1,...,m)$ are $L(n)$-$\hexp$- H\"older. 
Hence, $\forall x,x': \Metrico{\predfn(x)}{\predfn(x')} = \norm{\predfn(x) - \predfn(x')}_\infty = \max_{j=1,...,m} \abs{\predf_{n,j}(x) - \predf_{n,j}(x')} \leq \max_{j=1,...,m} L(n) \metric(x,x')^\hexp = L(n) \metric(x,x')^\hexp$.
\end{proof} 
\label{lem:LACKIpredHoelder}
\end{lem} 

We now establish how well our LACKI rule can interpolate the training data as function of the noise bound and regularisation parameter $\hestthresh$: 
\begin{lem}[Sample-consistency of LACKI] \label{lem:LACKIsampleconsistency} If for each output dimension $j \in \{1,...,d\}$ and some $\hestthresh \geq 0$ we have $L(n)  \geq  \max_{(s,s') \in U_n} \frac{\abs{\tilde f_j(s)- \tilde f_j(s')} -\hestthresh }{\metric^\hexp(s,s')}
$ then the LACKI rule is sample-consistent (up to $\frac \hestthresh 2$). 
That is,  \[\forall q \in \{1,\ldots,N_n \}:  \predfn(s_q) \in \ball{\frac \hestthresh 2}{\tilde f_q} \] where $\ball{\frac \hestthresh 2}{\tilde f_q} =\{ x \in \outspace |  \norm{x-\tilde f_q}_\infty \leq \frac \hestthresh 2\}$ denotes the $\frac \hestthresh 2$-ball around the observation $\tilde f_q$.\\
Thus, we also have $\norm{ f(s_q) - \predfn(s_q)}_\infty \leq \frac \hestthresh 2 + \norm{\obserr(s_q)}_\infty \leq \frac \hestthresh 2 + \obserrbnd$.
\begin{proof}
Remember, our output-space metric is given by $\Metrico{y}{y'} = \norm{y-y'}_\infty$.
For ease of notation, we will confine our proof to the case of one-dimensional outputs ($d=1$). The multi-dimensional case follows trivially from the one-dimensional result by applying it to each output component function. 
Let $n \in \nat  $ be fixed and, for ease of notation, write $L := L(n)$. Let $j,k \in   \{1,\ldots,N_n \} $ such that $j \in \argmin_i \tilde f_i + L \metric^\hexp(s_i,s_q) $ and 
$k \in \argmax_i \tilde f_i - L \metric^\hexp(s_i,s_q) $. 
By definition of $\predfn$ we have:
\begin{align}
\predfn(s_q) 
%&= \frac 1 2 \bigl( \tilde f_j + L \metric^\hexp(s_j,s_q)  +\obserrpar(s_q) \bigr) + \frac 1 2 \bigl( \tilde  f_k - L \metric^\hexp(s_k,s_q) - \obserrpar(s_q) \bigr)\\
&= \frac 1 2 \bigl(\underbrace{ \tilde f_j + L \metric^\hexp(s_j,s_q)}_{:=B}   \bigr) + \frac 1 2 \bigl( \underbrace{\tilde  f_k - L \metric^\hexp(s_k,s_q) }_{=:A}\bigr). \label{eq:hru582jsokbbbn}
\end{align}
%
%
(i) Firstly, we show  \underline{$ A \in [\tilde f_q, \tilde f_q +\hestthresh]$}:
If $k = q$, this holds trivially true since then $A= \tilde f_q$. 
So, assume $k \neq q$. 
We have $\tilde f_k \geq \tilde f_k - L \metric^\hexp(s_k,s_q)  \geq \tilde f_q - L \metric^\hexp(s_q,s_q)  = \tilde f_q$ where the second inequality holds due to $k \in \argmax_i \tilde f_i - L \metric^\hexp(s_i,s_q) $. That is,
%\begin{equation} 
%{\tilde f_k - \tilde f_q}  \geq L \metric(s_k,s_q). \label{eq:9p4t37ru8ewihk3hjtu}
%\end{equation} 
\begin{equation} 
A=\tilde f_k - L \metric^\hexp(s_k,s_q) \geq \tilde f_q. \label{eq:9p4t37ru8ewihk3hjtu}
\end{equation} 
On the other hand, since $L  \geq  \max_{(s,s') \in U_n} \frac{\abs{\tilde f(s)-\tilde f(s')} - \hestthresh}{\metric^\hexp(s,s')}$  we have in particular: $L  \geq  \frac{ \abs{\tilde f_k- \tilde f_q}-\hestthresh }{\metric^\hexp(s_k,s_q)}$. Thus,  
 $L \metric^\hexp(s_k,s_q) + \hestthresh \geq \abs{\tilde f_k-\tilde f_q} = \tilde f_k - \tilde f_q$. Hence, $\tilde f_q + \hestthresh \geq \tilde f_k - L \metric^\hexp(s_k,s_q) = A$. 
 Together with (\ref{eq:9p4t37ru8ewihk3hjtu}) we have shown $A \in [\tilde f_q , \tilde f_q +\hestthresh].$
%  In conjunction with (\ref{eq:9p4t37ru8ewihk3hjtu}) this means that $L \metric(s_k,s_q)  = \abs{\tilde f_k-\tilde f_q} $. Substituting this into the left hand side of Eq. \ref{eq:irndhfkkdnsww} yields the expression 
% $ \tilde f_k - \abs{\tilde  f_k -\tilde  f_q } \stackrel{!}{=}   \tilde f_q $. But since $f_k \geq f_q$, we also have $f_k - \abs{ f_k - f_q }  = f_q$. Therefore, Eq. \ref{eq:irndhfkkdnsww} is equivalent to $f_q = f_q$ which obviously holds. 
% 
%Analogously to the proof of  $f_k - L \metric(s_k,s_q) = f_q$ we can also show $f_j + L \metric(s_j,s_q) = f_q$. Leveraging both equations in Eq. \ref{eq:hru582jsokbbbn} concludes the proof. 

(ii) The proof of \underline{$B \in [ \tilde f_q - \hestthresh, \tilde f_q]$} is completely analogous to that of (i) and hence, is omitted.
%and secondly, that 
%\begin{equation}B \in [ \tilde f_q - \hestthresh, \tilde f_q]. \label{eq:irndhfkkdnswwB}
%\end{equation}

(iii) Together, the statements in (i) and (ii)  entail  $\predfn(s_q) = \frac 1 2 A + \frac 1 2 B  \in [\tilde f_q - \frac \hestthresh 2, \tilde f_q + \frac \hestthresh 2]$.

Hence, $\Metrico{\predfn(s_q)}{\tilde f(s_q)} \leq \frac \hestthresh 2$.

Moreover, for any sample input $s_q$ we have $\predfn(s_q) = f(s_q) + \phi_q + \psi_q$ with $\metric_{\outspace}(0,\psi_q) \leq \frac \hestthresh 2,  \metric_{\outspace}(0,\phi_q) \leq \Metrico 0 {\obserr(s_q)} \leq \obserrbnd$. 
Our output-space metric is translation-invariant and hence, $\Metrico{f(s_q)}{\predfn(s_q)} = \Metrico{0}{\predfn(s_q)- f(s_q)} = \Metrico{0}{  \phi_q + \psi_q} \leq \frac \hestthresh 2 +\Metrico 0 {\obserr(s_q)} \leq \frac \hestthresh 2 + \obserrbnd$.
\end{proof}
\end{lem}
%
%\begin{lem}\label{lem:groups_sampleconsandobserr} As always, let $\obserr(\cdot) $ denote the bound on the observational error.
%If $\predf_n$ is sample-consistent up to error $E$ with respect to set data $\data_n$ then, for any sample input $s \in \grid_n$, we have $\metric_\outspace\bigl(f(s), \predfn(s) \bigr) \leq E(s) + \metric_\outspace(0,\obserr(s))$.  Given an upper bound  $\obserrbnd \in \Real$ on the observational error  such that $\obserrbnd \geq \obserr(x),\forall x$ then sample-consistency up to error $E$ entails that true function is contained in the $E(s) + \obserrbnd$-balls around the predictions of observed inputs. That is, for all $s \in \grid_n$ we have:
%\begin{equation}
% f(s) \in \ball{ E(s) + \obserrbnd}{\predfn(s)} = \{y \in \outspace | \metric_\outspace(\predfn(s),y ) \leq E(s) + \obserrbnd \}.
%\end{equation}
%\end{lem}
%\begin{proof}
%Sample consistency up to $E$ implies that for each sample input $s \in \grid_n$ $\Metrico{\predfn}{\tilde f(s)} \leq E(s)$.
%On the other hand, bounded observational errors mean that for $s$ 
%there is $\nu_s \in \outspace, \Metrico 0 {\nu_s} \leq \obserrbnd$ such that we have $\Metrico{f(s)}{ \tilde f(s) } = \Metrico{f(s)}{ f(s)+\nu_s } \leq \Metrico{0}{\nu_s } \leq \obserrbnd$.
%Since the output pseudo-metric $\Metrico \cdot \cdot$ adheres to the triangle inequality, we have 
%$\Metrico{f(s)}{\predfn(s)} \leq \Metrico{f(s)}{ \tilde f(s) } + \Metrico{\predfn(s)}{ \tilde f(s) } \leq E(s) + \obserrbnd $.
%\end{proof}




\subsubsection{Prediction error bounds and consistency}

To asses our learning rule, we might be interested the discrepancy $\metric_\fctspace(\predfn,f)$ between the predictor $\predfn$ and the target function $f$ relative to some metric $\metric_{\fctspace}$ between functions in the space $\fctspace$ of continuous functions. In statistics, a typical choice is the mean-square error metric assessed with respect to some distribution over inputs, the function space and the noise. However, in many safety-critical applications, often arising in control, worst-case error considerations are of greater value, leading to a worst-case metric 
$\metric_\fctspace(f,g) = \sup_{x \in I} \Metrico{ f(x)}{g(x)} $ for some subset $I \subseteq \inspace$ of queries on finds interesting to take into consideration. 

Therefore, we will now establish worst-case consistency guarantees of our LACKI inference rules. That is, we shall study the worst-case error  
sequence $\errmetric^\infty :=\seq{\errmetric^\infty_n}{n \in \nat}$, 
\begin{equation}
\errmetric^\infty_n := \sup_{x \in \queryset } \metric_\outspace\bigl(\predfn(x), f(x)\bigr)\end{equation}
for data $\data_n$ that becomes increasingly dense over time relative to a set of query inputs $\queryset \subseteq \inspace$. 
To clarify the latter concept, 
consider the sequence of grids $\seq{\grid_n}{n \in \nat}$. 
We say this sequence converges to a set that \emph{becomes dense relative to a set $I$ in the limit of large $n$ } if we can use points in the sequence to approximate any points in $I$ with increasing accuracy. That is, if $\forall \epsilon >0,x \in I \exists n_0 \forall n \geq n_0 \exists g \in \grid_n: \metric(x,g) < \epsilon$. If the rate at which this happens is independent of $x$ then we say that the grid sequence becomes dense \emph{uniformly}. This is the case iff $\forall \epsilon >0 \exists n_0 \forall n \geq n_0, x \in I \exists g \in \grid_n: \metric(x,g) < \epsilon$.

To make the rates explicit in our notation, we list the following general definitions: 

%\begin{defn} [Becoming dense]
%Let $\inspace$ be a space endowed with a pseudo-metric $\metric$. 
%\begin{itemize}
%\item 
%We say the sequence of sets $(S_n)$, with $S_n \subset \inspace$, \emph{becomes dense} to $S' \subset \inspace$ \emph{pointwise} (written as $(S_n) \convto S'$), iff $$ \forall s \in S' \exists r_s: \nat \to \Real : \bigl(r_s(n) \stackrel{n \to \infty}{\to} 0 \wedge \forall n \in \nat: \inf_{s_n \in S_n} \metric(s_n,s) \leq r_s(n)\bigr).$$
%\item The sequence becomes dense to $S$ \emph{uniformly} (written as (S_n) \to S') if there is a vanishing rate that is independent of the point $s \in S'$ with which $S_n$ becomes dense to $S'$ at all points. That is, if there exists a uniformly applicable rate $r: \nat \to \Real$ with  $r(n)  \stackrel{n \to \infty}{\to} 0$ and  
%$  \forall n \in \nat : \sup_{s \in S} \inf_{s_n \in S_n} \metric(s_n,s) \leq r(n) . $
%%\item Finally, a sequence of points $\seq{s_n}{n \in \nat}$ in $ \inspace$ is said to converge to the set $S \subset \inspace$ iff $\inf_{s \in S} \metric(s_n,s) \to 0$ as $n \to \infty$.
%\end{itemize}
%\end{defn}

\begin{defn} [Becoming dense, rates, $\stackrel{r}{\convto}, \stackrel{r}{\bd}, \stackrel{r}{\bdu}$]
Let $\inspace$ be a space endowed with a pseudo-metric $\metric$. 
Let $r:\nat \to \Real$ be a ``rate'' function. 
that vanishes, that is, with $\lim_{n \to \infty} r(n) = 0$ (i.e. $r \in o(1)$).
\begin{itemize}
\item The sequence $s =\seq{s_n}{n \in \nat}$ of points in $\inspace$ is said to converge to a point $x \in \inspace$ \emph{with rate} $r$ (denoted by $s \stackrel{r} \convto x$) iff  $\forall n \in \nat : \metric(x,s_n) \leq r(n)$ and $r(n) \convton 0$. 
\begin{itemize}
\item The sequence $s $ is said to converge to a set $\mathbb S \subset \inspace$  with rate $r:\nat \to \Real$ (denoted by $s \stackrel{r} \setconvto \mathbb S$) iff $\forall n\in \nat : \inf_{x \in \mathbb S}\metric(x,s_n) \leq r(n)$ and $r(n) \convton 0$. 
\end{itemize}
\item A sequence of sets $S = \seq{S_n}{n \in \nat}$ is said to \emph{become dense} relative to $x \in \inspace$  \emph{with rate} $r$ (denoted by $S \stackrel{r}{\bd} x$) iff $S$ contains a point sequence that converges to $x$ with that rate. That is, iff $\exists s= \seq{s_n}{n\in \nat}: s \stackrel{r}\convto x \wedge \forall n: s_n \in S_n$. 
\begin{itemize}
\item Similarly, the sequence of sets $S$ is said to become dense relative to a \emph{set}  of points $\mathbb S \subset \inspace $ (denoted by $S \bd \mathbb S$) iff it becomes dense relative to all points of $\mathbb S$, i.e. iff $\forall x \in \mathbb S : S \stackrel{r_x}{\bd} x$ for some vanishing rate $r_x : \nat \to \Real$. 
\item The sequence is becoming dense relative to $\mathbb S$ \emph{uniformly} (denoted by $S \bdu \mathbb S$) iff there is a single vanishing rate for all $x \in \mathbb S$. That is, if $\exists r:\nat \to \Real:$ $\lim_{n\to \infty} r(n) =0 \wedge \sup_{x \in \mathbb S} \inf{s_n \in S_n} \metric(s_n,x) \leq r(n), \forall n$. Function $r$ is referred to as the convergence rate and we write $S \stackrel{r}{\bdu}\mathbb S$ to denote that $S$ becomes dense relative to $\mathbb S$ with uniform rate $r$.
\end{itemize}
\end{itemize}
\end{defn}

\begin{thm}[LACKI can learn any H\"older function] \label{thm:convergenceifboundedconstandsamplecons_LACKI}
Assume the following holds true:
\begin{enumerate}
%\item The grid sequence $\seq{\grid_n}{n \in \nat}$ becomes dense in the input domain $\inspace$. 
\item The observational errors given by $\obserr$ are bounded from above by $\obserrbnd= \sup_x \metric_\outspace\bigl(0,\obserr(x)\bigr) \in \Real_{\geq 0}$.
\item  The target $f: \inspace \to \outspace$ is H\"older continuous, i.e. $\exists L^* \in \Real: f \in \hoelset {L^*}{}  p$.
\end{enumerate}
%
%and let the predictors be sample-consistent up to error $\bar E$ and H\"older continuous, 
%$\predfn \in \hoelset {L(n)}{} p$ with $L(n) \leq \bar L \in \Real_+\, (n \in \nat)$ for some $\bar L \geq 0$.

Under these assumptions we can give the following guarantees: 
%\begin{itemize} \item 

\textbf{(A)} If the grid becomes dense (pointwise), the point-wise worst-case error vanishes up to $\frac \hestthresh 2 + \obserr$:
$$
\text{If }\forall x \in I \subset \inspace \exists r_x \in o(1) : L(\cdot) r_x^\hexp(\cdot) \in o(1) \wedge \seq{G_n}{n \in \nat} \stackrel{r_x}{\bd} x  \text{ then }\forall x \in I : \seq{\Metrico{\predfn(x)}{f(x)}}{n \in \nat} \stackrel{\varrho_x} \convto [0,\frac \hestthresh 2 + \obserr]$$
where for the error convergence rate $\varrho_x$ we have $\varrho_x(n) \leq (L(n)+ L^*) r_x^\hexp(n) , \forall n \in \nat$. 

\textbf{(B)} If the grid becomes dense in $I \subset \inspace$ uniformly, then the worst-case prediction error vanishes uniformly (up to $\frac \lambda 2 + \obserrbnd$):
$$\text{If } \exists r \in o(1) :  L(\cdot) r_x^\hexp(\cdot) \in o(1) \wedge (G_n) \stackrel{r}{\bdu} I  \text{ then }  \errmetric^\infty \stackrel{\varrho}{\convto} [0,\frac \hestthresh 2 + \obserrbnd]$$
where for the uniform error convergence rate $\varrho$ we have $\varrho(n) \leq (L(n)+ L^*) r^\hexp(n) , \forall n \in \nat$. 

%
%
%(A) If, the grid becomes dense in $\inspace$ with rates $r_x$ (for $x \in \inspace$) and if the $L(n)$ satisfy $L(\cdot) r_x(\cdot) \in o(1)$  then the sequence of predictors $\seq \predfn {n \in \nat}$ converges to the ground truth $f$ pointwise up to error $\frac \hestthresh 2 +\obserrbnd$. That is, $\forall \epsilon > 0,  x \in \inspace \exists n_0 \in \nat \forall n \geq n_0: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \in \bigl[0, \epsilon + \frac \hestthresh 2 + \obserrbnd\bigr]$.
%
%In particular,  $\sup_{} \mathcal O\bigl(\,  (L(n)+L^*) r_x(n)^\hexp \, \bigr)$. 


%\textbf{(B)} If the grid sequence $\seq{\grid_n}{n \in \nat }$ becomes dense in $\inspace$ uniformly with rate of at most $n \mapsto r(n) \in o(1)$ and if we have $L(\cdot) r(\cdot) \in o(1)$ then $\seq \predfn {n \in \nat}$ converges to the target $f$ uniformly up to error $ \frac \hestthresh 2 +\obserrbnd$. 
%That is, $\forall \epsilon > 0 \exists n_0 \in \nat \forall n \geq n_0, x \in \inspace: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \in \bigl[0, \epsilon + \frac \hestthresh 2 + \obserrbnd\bigr]$. Convergence occurs with a rate of at most $\mathcal O\bigl( \, (L(n)+L^*) r(n)^\hexp \, \bigr)$.


\begin{proof}
We have established that the predictors $\predfn(\cdot)$ of the LACKI rule are $L(n)$-$\hexp$- H\"older (Lem. \ref{lem:LACKIpredHoelder}) and sample-consistent up to level $\frac \hestthresh 2$ (Lem. \ref{lem:LACKIsampleconsistency}). 
%Moreover, the sequence $\seq{L(n)}{n \in \nat}$ is convergent and bounded by some number $\bar L \leq \max\{L^*,\underline L\}$ (cf. Rem. \ref{rem:convlipconstestimates}).
 %Furthermore our input and output spaces are additive abelian groups. By assumption, pseudo-metrics $\metric,\metric_\outspace$ are translation invariant with respect to addition. Therefore, the predictors meet all assumptions of Thm. \ref{thm:convergenceifboundedconstandsamplecons} which entails the desired convergence statements.


For any input $x \in \inspace$ let $\xi_n^x$ denote a nearest neighbour of $x$ in grid $\grid_n$. That is, $\xi_n^x \in \arg\inf_{s \in \grid_n} \metric(x,s)$.
Since $\grid_n$ is assumed to become dense in the input domain $\inspace$, for any input $x$ there is a rate function $r_x : \nat \to \Real_{\geq 0}$ such that $r_x(n) \stackrel{n \to \infty}{\longrightarrow} 0$ and $ \metric(x,\xi_n^x )^\hexp \leq r_x(n) 
, \forall n \in \nat$. In the case of uniform convergence a rate function can be chosen independently of $x$ and will be denoted by $r$ rather than $r_x$.

\textbf{(A)} 
For all $n \in \nat$ and $x \in \inspace$ we have:
%there always is some $\phi(\xi_n^x) \in  \ball{\bar E}{0} = \{ y \in \outspace \,| \, \metric_\outspace(y,0 ) \leq \bar E \}$ such that (i) 
\begin{align} \metric_\outspace\bigl(\predfn(x) , f(\xi_n^x)  \bigr)
&\stackrel{(i)}{\leq} 
\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \metric_\outspace\bigl(\predfn(\xi_n^x) , f(\xi_n^x)  \bigr)\\
&\stackrel{(ii)}{\leq} 
\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \frac \lambda 2 + \metric_\outspace\bigl(0, \obserr(\xi_n^x) \bigr)
\stackrel{ }{=} 
\norm{\predfn(x) - \predfn(\xi_n^x) }_\infty + \frac \lambda 2 + \obserrbnd\\
&\stackrel{(iii) }{\leq} L(n)
\Metrici{x}{\xi_n^x }^\hexp + \frac \lambda 2 + \obserrbnd \label{ineq:kjshkhd8e}
%&\stackrel{(iv) }{\leq} \bar L\,
%r_x(n) + \frac \lambda 2 + \obserrbnd \stackrel{n \to \infty}{\longrightarrow} \frac \lambda 2 + \obserrbnd.
\end{align}
Here, (i) follows from the triangle inequality, (ii) leverages Lem. \ref{lem:LACKIsampleconsistency} and (iii) follows by H\"older continuity of the predictors (Lem. \ref{lem:LACKIpredHoelder}).

%
Thus, for $x \in \inspace, n \in \nat$:
%
\begin{align}
0 \leq \metric_\outspace\bigl(\predfn(x) , f(x)\bigr) &\leq \metric_\outspace\bigl(\predfn(x) ,  f(\xi_n^x)  \bigr) + \metric_\outspace\bigl(f(\xi_n^x) , f(x)\bigr)\\
%$\norm{\predfn(x) - f(x)} \leq \norm{\predfn(x) - f(\xi_n)  } + \norm{f(\xi_n) - f(x)} \stackrel{(i)}{=}\norm{\predfn(x) - \predfn(\xi_n)  } + \norm{f(\xi_n) - f(x)}$
&\stackrel{(\dagger)}{\leq} (L(n)+ L^*) \metric(x,\xi_n^x )^\hexp +  \frac \lambda 2 +\obserrbnd
\end{align}
where ($\dagger$) follows from (\ref{ineq:kjshkhd8e}) and the presupposed H\"older continuity of $f$. \\

Since by assumption, $ \metric(x,\xi_n^x )^\hexp \leq r_x(n) 
, \forall n$ this implies:
\begin{equation}
\metric_\outspace\bigl(\predfn(x) , f(x)\bigr)  \in \bigl[0, (L(n)+ L^*) r_x(n)^\hexp +  \frac \lambda 2 +\obserrbnd \bigr], \forall n. \end{equation} 
By assumption $ r_x(n), L(n) r_x^\hexp(n) \stackrel{n \to \infty}{\to} 0, \forall x$ and hence, $\metric_\outspace\bigl(\predfn(x) , f(x)\bigr)$ converges to $  [0,\frac \lambda 2 +\obserrbnd], \forall x$ with rate $\varrho_x \leq(L(n)+ L^*) r_x(n)^\hexp $.
%
%
%
%By assumption,  $\lim_{n \to \infty}  L(n) r_x (n)^\hexp = 0$ and hence, $\bigl[0, (L(n)+ L^*) r(n)^\hexp +  \frac \lambda 2 +\obserrbnd \bigr] \to \bigl[0,  \frac \lambda 2 +\obserrbnd \bigr]$ and $\bigl[0, (L(n)+ L^*) r_x(n)^\hexp +  \frac \lambda 2 +\obserrbnd \bigr] \to \bigl[0,  \frac \lambda 2 +\obserrbnd \bigr], \forall x$.

\textbf{(B)} Proceeding analogously as before, but utilising uniform convergence with rate $r$, we obtain:  \begin{equation} 
\metric_\outspace\bigl(\predfn(x) , f(x)\bigr)  \in \bigl[0, (L(n)+ L^*) r(n)^\hexp +  \frac \lambda 2 +\obserrbnd \bigr], \forall x \forall n. \end{equation} 
By assumption,  $L(n) r^\hexp(n) \in o(1)$ and thus, $\lim_{n \to \infty} L(n) r(n)^\hexp = 0$. Hence,  $$\errmetric^\infty = \seq{\sup_{x \in I} \metric_\outspace\bigl(\predfn(x) , f(x)\bigr) }{n \in \nat} \stackrel{\varrho}{\convto} [0, \frac \lambda 2 +\obserrbnd] $$ with rate $\varrho $ such that $\varrho(n) \leq (L(n)+ L^*) r(n)^\hexp, \forall n$.

\end{proof}
\end{thm}

Note a necessary condition was that the product of $L(n)$ and the rate was in $o(1)$, that is, vanishing in the limit of $n \to \infty$. A sufficient condition for this to hold is if $L(n)$ is guaranteed to be bounded (assuming the rate is vanishing). Above, we have established a sufficent condition for this (cf. Rem. \ref{rem:convlipconstestimates}): $L(n)$ is bounded as long as parameter $\hestthresh \geq 2 \obserrbnd + q$ for any $q \geq 0$. This yields the following result:

\begin{cor}
With definitions and assumption as in Thm. \ref{rem:convlipconstestimates}, if parameter $\hestthresh $ is chosen to be $2 \obserrbnd + q $ for any $q \geq 0$ then convergence to the ground truth is guaranteed (up to an twice the observational error and a term dependent on $q$). In particular, if the data becomes dense uniformly in $I \subseteq \inspace$ with a rate of $r(n)$  then, for some $\bar L \in [0,L^*]$ and any $n \in \nat$, we have 
\begin{equation}
\sup_{x \in I} \metric_\outspace\bigl(\predfn(x) , f(x)\bigr) \leq (\bar L+ L^*) r(n)^\hexp +  \frac { q} 2 +2 \obserrbnd  \stackrel{n \to \infty}{\convto}  \frac q 2 + 2  \obserrbnd . \end{equation} 
\label{cor:worstcaseconvhoeldertarget}
\end{cor}

%%%% ==== allgem. Bew. --------
%\begin{thm} \label{thm:convergenceifboundedconstandsamplecons}
%Let $\seq{\data_n}{n \in \nat}$ be a data set sequence with pertaining grid sequence $\seq{\grid_n}{n \in \nat}$, \\ with $\grid_n \subset G_{n+1} \subset \inspace (n \in \nat)$ converging to a dense subset of input domain $\inspace$. Assume all of the following: 
%\begin{enumerate} 
%\item The data sets $\data_n$ ($n \in \nat$) all have bounded observational error with $\obserrbnd := \sup_x \Metrico{0}{\obserr(x)} \in \Real_{\geq 0}$.
%\item The target $f: I \subseteq \inspace \to \outspace$ is H\"older continuous with $f \in \hoelset {L^*}{}  p$.
%\item The predictors $\predfn$ $(n \in \nat)$ are sample-consistent up to error $E:\inspace \to \Real$ with $\bar E := \sup_x E(x) \leq \infty$.
%\item The predictors are  H\"older continuous with H\"older constants bounded below $\bar L \in \Real_{\geq0}$. That is, 
%$\exists \bar L \geq 0 \forall n \in \nat: \predfn \in \hoelset {L(n)}{} p$  $ \wedge$ $ L(n) \leq \bar L$.
%\end{enumerate}
%
%
%Then, we have: 
%\begin{itemize}
%\item \textbf{(I)}The sequence of predictors $\seq \predfn {n \in \nat}$ converges to the ground truth $f$ pointwise up to error $\bar E$. That is, $\forall \epsilon \geq 0,  x \in \inspace \exists n_0 \in \nat \forall n \geq n_0: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon + \bar E + \obserrbnd$.
%%\item 
%
%\item \textbf{(II)} If the grid sequence $\seq{\grid_n}{n \in \nat }$ converges to the domain $\inspace$ uniformly then $\seq \predfn {n \in \nat}$ converges to the target $f$ uniformly up to error bound $\bar E + \obserrbnd$. 
%
%That is, $\forall \epsilon \geq 0 \exists n_0 \in \nat \forall n \geq n_0, x \in \inspace: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon + \bar E+\obserrbnd$.
%
%\item \textbf{(III)} If the uniform convergence of the grid sequence as per (II) occurs with a rate of at most $r:\nat \to \Real$ then we have:  $$\forall n \in \nat \forall x \in I \subseteq\inspace: \metric_\outspace\bigl(\predfn(x) , f(x)\bigr)\in [0,(\bar L+ L^*) r(n)^\hexp+ \bar E + \obserrbnd].$$ That is, as $n \to \infty$,  convergence (up to error $\bar E +\obserrbnd)$ of the predictors to the target occurs uniformly at a rate of at most $(\bar L+ L^*) r(n)^\hexp$
%\end{itemize}
%
%\begin{proof}
%For $x \in I\subseteq \inspace$ let $\xi_n^x$ denote the nearest neighbour of $x$ in grid $\grid_n$. That is, $\xi_n^x = \arg\inf_{s \in \grid_n} \metric(x,s)$.
%
%\textbf{(I)} 
%Since $\grid_n$ is assumed to converge to a dense subset of the domain $I$, we have$ \metric(x,\xi_n^x )^\hexp
%\stackrel{n \to \infty}{\longrightarrow} 0$.
%Furthermore, since the the predictors are sample-consistent on grid $\grid_n$ up to error $E$ and since $\xi_n^x \in \grid_n$ we can appeal to Lem. \ref{lem:groups_sampleconsandobserr} (as well as to the triangle inequality) to reason as follows:
%%there always is some $\phi(\xi_n^x) \in  \ball{\bar E}{0} = \{ y \in \outspace \,| \, \metric_\outspace(y,0 ) \leq \bar E \}$ such that (i) 
%$\metric_\outspace\bigl(\predfn(x) , f(\xi_n^x)  \bigr) 
%\leq 
%\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \metric_\outspace\bigl(\predfn(\xi_n^x) , f(\xi_n^x)  \bigr)
%\stackrel{Lem. \ref{lem:groups_sampleconsandobserr}}{\leq} 
%\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + E(\xi_n^x) + \obserr(\xi_n^x)$.
%Hence,
%\begin{equation}
%\forall x: \metric_\outspace\bigl(\predfn(x) , f(\xi_n^x)  \bigr) \leq
%\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \bar E + \obserrbnd.
%\label{ineq:ewlfjhflsape}
%\end{equation}
%%
%Thus, for $x \in \inspace$:
%%
%$\metric_\outspace\bigl(\predfn(x) , f(x)\bigr) \leq \metric_\outspace\bigl(\predfn(x) ,  f(\xi_n^x)  \bigr) + \metric_\outspace\bigl(f(\xi_n^x) , f(x)\bigr)$
%$\leq 
%\metric_\outspace\bigl(\predfn(x) , \predfn(\xi_n^x)  \bigr) + \bar E + \obserrbnd+ \metric_\outspace\bigl(f(\xi_n^x) , f(x)\bigr)$
%%$\norm{\predfn(x) - f(x)} \leq \norm{\predfn(x) - f(\xi_n)  } + \norm{f(\xi_n) - f(x)} \stackrel{(i)}{=}\norm{\predfn(x) - \predfn(\xi_n)  } + \norm{f(\xi_n) - f(x)}$
%$\stackrel{(\dagger)}{\leq} (\bar L+ L^*) \metric(x,\xi_n^x )^\hexp + \bar E +\obserrbnd$
%$\stackrel{n \to \infty}{\longrightarrow} \bar E +\obserrbnd$.
%Here ($\dagger$) leverages the H\"older continuity assumptions. \\
%
%\textbf{(II)} The proof is a trivial extension of (I). Let $\epsilon \geq 0.$ We show $\exists n_0 \in \nat \forall n \geq n_0, x \in \inspace: \metric_{\outspace}\bigl(\predfn(x), f(x) \bigr) \leq \epsilon + \bar E +\obserrbnd$.  
%Since $\grid_n$ converges to $I$ uniformly, $\exists n_0 \forall n\geq n_0\forall x \in I: \metric(x,\xi_n^x)^\hexp \leq \frac{\epsilon}{2 \max\{\bar L, L^* \}}$. Hold such $n_0$ fixed. Then for all $n \geq n_0, x \in I$ we have 
%$\metric_\outspace\bigl(\predfn(x) , f(x)\bigr) \newline \stackrel{(*)}{\leq} (\bar L+ L^*) \metric(x,\xi_n^x )^\hexp + \bar E +\obserrbnd \leq \epsilon + \bar E +\obserrbnd$. Here (*) follows from (\ref{ineq:ewlfjhflsape}) and ($\dagger$) in complete analogy to our derivations for case (I) above. 
%
%\textbf{(III)} By assumption of uniform convergence of $\seq{\grid_n}{n \in \nat}$ with rate $r(n)$, $\sup_{x \in I} \inf_{s_n \in \grid_n} \metric (x,s_n) =\sup_{x \in I} \metric (x,\xi_n^x) \leq r(n)$. The rest follows from (*).
%\end{proof}
%\end{thm}
%
%
%% ==== allgem. bew. ende=====

Of course in the absence of observational errors, one can choose $\hestthresh = 0$. In this case, the corollary implies that LACKI will learn the ground-truth arbitrarily well in the limit of infinitely dense data.
%Note, when $\hestthresh \geq 2 \obserr$, the worst-case error bound in the corollary involves a term of twice the observational error bound. In general, this is unavoidable without making further assumptions.

\begin{remark} [Curse of dimensionality]
Our bounds rely on the proximity (expressed by the rate functions) of the query input to the previously observed data.
Refer to Thm. \ref{thm:convergenceifboundedconstandsamplecons_LACKI}.
Roughly speaking, for a particular query input $x$, our guarantee in (A) asserts that the closer the query is to the previously seen data, the better the confidence in prediction accuracy. In (B) this is extended to a worst-case statement implying that the smaller the worst-case proximity of the data to any query in $I$, the smaller the worst-case prediction error can be. 
Unfortunately, this worst-case proximity and therefore, the prediction error bound, is subject to the \emph{curse of dimensionality}. That is, the number of samples necessary to guarantee a desired reduction in worst-case prediction uncertainty will inevitably have to scale exponentionally with the dimensionality of the space. A manifestation of this fact can be seen in Sec. \ref{sec:probconv_LACKI} where we give a sample complexity bound for uniformly distributed input samples. 
\end{remark}


Having established that our LACKI rule can learn any H\"older function with any H\"older constant, we will now attend to extend the results to non-H\"older functions. In preparation of the necessary derivations we will first rehearse universality and H\"older properties of radial basis function networks. 

Park and Sandberg derived universal approximation guarantees for radial-basis function networks \cite{Park1991}. In particular, on page 252 in their article the authors make an assertion that translates to our notation as follows: 

\begin{lem}[Expressiveness of RBFNs] \label{lem:RBFNunifapproxcompact} Assume $\inspace \subseteq \Real^d$ is compact. Given parameter  vector $\theta := (w_1,\ldots,w_m,\sigma_1,...,\sigma_m,c_1,\ldots, c_m)$ and kernel function $K: \inspace \to \outspace $ let $\beta(\cdot;\theta ) = \sum_{i=1}^m w_i \, K(\frac{\cdot - c_i}{\sigma_i} )  $ denote a radial basis function network (RBFN). Assume $K: \Real^d \to \Real$ is continuous and has non-vanishing integral, i.e. $\int_{\Real^d} K(x) \d x \neq 0$.
Then, the set $S_K:= \{ \beta(\cdot; \theta) \vert  m \in \nat, \theta \in \Real^{3m}  \}$ of all RBFNs is uniformly dense in the set $C(\inspace)$ of continuous functions on compact domain $\inspace$. That is,  $\forall f \in C(\inspace) \forall \epsilon >0  \exists m, \theta \in \Real^{3m} : \sup_{x \in \inspace}{ \abs{f(\cdot) -\beta(\cdot;\theta)  } } <\epsilon $. 
\end{lem}

\begin{remark} \label{rem:LipconstofRBFN}
We note that, for any finite-dimensional parameter $\theta$, any RBFN $\beta(\cdot;\theta)$ is Lipschitz continuous as long as the kernel $K$ is. This can be seen by applying Lem. \ref{lem:Hoeldarithmetic} which allows us to conclude that the Lipschitz constant of RBFN $\beta(\cdot;\theta ) = \sum_{i=1}^m w_i \, K(\frac{\cdot - c_i}{\sigma_i} ) $ is given by $L_\beta = \sum_{i=1}^m \abs{\frac{w_i}{\sigma_i}} L_{K}$ where $L_K \in \Real_{\geq 0}$ denotes a Lipschitz constant of $K$. By the same Lemma it is easy to see that choosing the Gaussian kernel for $K$ satisfies both the Lipschitz requirement as well as the integrability requirements of Lem. \ref{lem:RBFNunifapproxcompact}. As a by-product this means that on a compact support, any continuous function can be approximated by some Lipschitz function with arbitrarily small, positive worst-case error $\epsilon >0$. Note, it may well be the case that the Lipschitz constant of the approximator grows with decreasing approximation error bound $\epsilon$. We consider this to be inevitable when the approximated function is not Lipschitz.
\end{remark}

Harnessed with these preparatory statements we can move on to show that the LACKI rule can be set up to learn any continuous function up to arbitrary low error.
\begin{thm}[Universality of LACKI]
\label{thm:LACKIuniversality}
Assume we are given a sequence $\seq{\data_n}{n \in \nat}$ of samples with observational errors bounded by $\obserrbnd \in \Real_{\geq 0}$. We set the parameters of the LACKI rule to $\lbf =-\infty,\ubf =\infty, \underline L =0$ and $\hestthresh := 2 \bar e +q $ for some $q >0$. In this theorem, we assume that the set of interest $I \subseteq\inspace$ is compact.
\textbf{Then, we have:}

The LACKI rule as per Def. \ref{def:LACKI} is a universal approximator in the following sense:
If the sequence of input grids $\seq{\grid_n}{n \in \nat}$ relative to $I$ (uniformly) then the sequence of predictors $\seq{\predfn}{n \in \nat}$ computed by the LACKI rule (uniformly) converges to any continuous target $f : \inspace \to \Real$ up to error $2 \obserrbnd + \frac{3q}{2}$.
That is, the following holds true:



\begin{itemize}
\item (I) Let $x \in I$. If $\exists r_x \in o(1): (\grid_n) \stackrel{ r_x}{\bd} x$ then $\exists C \in \Real : \seq{\Metrico{\predfn(x)}{f(x)}}{ } \stackrel{C r_x^\hexp}{\convto}[2\obserrbnd + \frac{3q}{2}]$.
\item (II) If $\exists r \in o(1): (\grid_n) \stackrel{ r}{\bdu} I$ then $\exists C \in \Real : {\errmetric^\infty}{ } \stackrel{C r^\hexp}{\convto}[2\obserrbnd + \frac{3q}{2}]$.
%$\forall \epsilon >0,x \in I \exists n_0 \geq 0\forall n\geq n_0: \metric_\outspace\bigl(\predfn(x),f(x)\bigr) \leq \epsilon + 2 \obserrbnd + \frac{3q}{2}$.
%\item (II) If $(\grid_n)$  $\bdu \inspace$  then we have: $$\forall \epsilon >0 \exists n_0 \geq 0\forall n\geq n_0, x \in \inspace: \metric_\outspace\bigl(\predfn(x),f(x)\bigr) \leq \epsilon + 2 \obserrbnd + \frac{3q}{2}.$$ 
\end{itemize}
\end{thm}
\begin{proof}
We choose any parameter $\hestthresh =  2 \obserrbnd + q$ with $q >0$. As observed in Rem. \ref{rem:LipconstofRBFN}, Lem. \ref{lem:RBFNunifapproxcompact} allows us to infer that there exists a Lipschitz function $h$ that approximates the target with worst-case error of at most $\frac q 2$. That is, $\sup_{x \in \inspace} \metric_\outspace\bigl(h(x), f(x) \bigr) \leq \frac q 2$. (Also, note Lipschitz continuity implies H\"older continuity for any H\"older exponent $\hexp \in (0,1]$, and hence, $h \in \hoelset {L_h}{ }{\hexp}$ for some $ L_h \in \Real_{\geq 0}$.)

Consequently, there exists a function $\phi':\inspace \to \outspace$ with $\sup_x \Metrico{ 0}{\phi'(x) } \leq \frac q 2$ accounting for the discrepancy between the H\"older function $h$ and the target $f$: $f = h+ \phi'$. 

Furthermore,we define $\phi$ to be the bounded observational noise. Hence, we have $\tilde f = f+ \phi$ and $\sup_x \Metrico{0}{\phi(x)} \leq \obserrbnd$.
Combining both functions into $\psi := \phi+\phi'$, we can write $\tilde f = h + \psi$ with $\sup_x \Metrico{0}{\psi(x)}\leq \frac q 2 + \obserrbnd =: \bar \nu$.

This can be interpreted as follows:
Instead of viewing the given sample as being generated by target $f$ (with some observational error $\phi$) we can view the sample as being generated by the H\"older function $h$ corrupted by the extended ``observational noise'' $\psi$ accounting for both the original observational error and the discrepancy between the target and H\"older function $h$.
This gives us a reduction to the case of learning H\"older functions with observational error bounded by $\bar \nu$. Firstly, we note that $\hestthresh = 2 \obserrbnd +q =2 \bar \nu$ (which entails that the sequence $\seq{L(n)}{n \in \nat}$ is bounded by some constant $\bar L  =\sup_{x,x', \metric(x,x') >0} \frac{\metric_\outspace(h(x), h(x'))   -q}{\metric^\hexp(x,x')} \leq L_h$). 
Linking to Thm. \ref{thm:convergenceifboundedconstandsamplecons_LACKI}, we get all the desired statements with regard to learning $h$. These can easily be converted into statements about learning $f$ by adding the worst-case difference $\frac q 2$ between $f$ and $h$ to all error bounds. 
For example, leveraging $\sup_x \Metrico{ 0}{\phi'(x) } \leq \frac q 2$ and $\lambda = 2 \obserrbnd + q$ and going through analogous steps as in the previous theorem we obtain:   
%$\metric_\outspace\bigl(\predfn(x) , h(x)\bigr) \leq $\leq (\bar L+ L_h) \metric(x,\xi_n^x )^\hexp + \bar E +\obserrbnd$ 
\begin{align}
\metric_\outspace(\predfn(x), f(x) ) &= \metric_\outspace(\predfn(x), h+\phi' (x) ) 
\leq   \metric_\outspace\bigl(\predfn(x) , h(x)\bigr) + \metric_\outspace(0,\phi'(x) ) \\
&\leq (\bar L+ L_h) \metric(x,\xi_n^x )^\hexp + \frac \lambda 2 +\bar \nu + \frac q 2 \\
&\leq (\bar L+ L_h) \metric(x,\xi_n^x )^\hexp  +2 \obserrbnd + \frac {3q}{2} \label{ineq:euyiweeh}
\end{align}
where  $\xi^x_n := \arg\inf_{s \in \grid_n} \metric(x,s)$ denotes a nearest neighbour of $x$ in the input sample $\grid_n$.

So, convergence (pointwise or uniform) of the grid to the input space with a rate of at most $r(n)$ implies that the right-hand side of (\ref{ineq:euyiweeh}) and hence, the prediction error,  
converges (pointwise or uniformly) to the interval $[0,2 \obserrbnd + \frac {3q}{2}] $ with a rate of at most $(\bar L + L_h) r^\hexp(n)$ as $n \to  \infty$.



%%OLD PROOF:
%
%By Lem. \ref{lem:constadaptation_boundedness}, the lazily adapted H\"older constant estimates $L(n)$ are bounded from above by $\max\{\underline L, \tilde L\} = \tilde L  < \infty$. In conjunction with Lem. 
%\ref{lem:LACKIsampleconsistency} (which establishes sample consistency up to $\frac \hestthresh 2$) we have established that all preconditions of Thm. \ref{thm:convergenceifboundedconstandsamplecons} are met by the predictors $\predfn$ $ ({n \in \nat})$. Hence, the theorem allows us to conclude that the sequence of predictors $\seq{\predfn}{n \in \nat}$ converges to $\beta(\cdot;\theta)$ up to an error less than or equal to $\sup_x \metric_\outspace(0,\psi(x)) \leq \frac \hestthresh 2$:
%
%
%(I) In the general case this convergence is pointwise. 
%Let $x \in  \inspace$ and $\epsilon > 0$.  Thm. \ref{thm:convergenceifboundedconstandsamplecons}.(I) implies $\exists n_0 \forall n\geq n_0: \metric_\outspace\bigl (\predfn(x), \beta(x,;\theta) \bigr) \leq \epsilon+\frac \hestthresh 2$. Hence, $\metric_\outspace\bigl (\predfn(x), f(x) \bigr) = \metric_\outspace\bigl (\predfn(x), \beta(x,;\theta) + \psi(x) \bigr) \stackrel{Lem. \ref{lem:bilinaddtransinvgroup}}{\leq} \metric_\outspace\bigl(\predfn(x), \beta(x,;\theta)\bigr) +\metric_\outspace\bigl(0, \psi(x) \bigr) \leq \metric_\outspace\bigl(\predfn(x), \beta(x,;\theta)\bigr) +\frac \hestthresh 2\leq \epsilon +\hestthresh$.
%
%(II)  If convergence of the grid to domain $\inspace$ is uniform convergence of the predictors to the RBFN is uniform (by Thm. \ref{thm:convergenceifboundedconstandsamplecons}.II ). The remainder of the proof is completely anaologous to (I), except that $n_0$ can be chosen independently of $x$.
%
%

\end{proof}

%\begin{remark}
%Note, our universality guarantee of Thm. \ref{thm:LACKIuniversality} is much stronger than the guarantee for RBFNs.
% The universality statement for RBFNs is purely representational. That is, it states that in principle it is possible to find some RBFN with some choice of parameter that approximates any continuous function with arbitrarily small worst-case approximation error. However, it makes no mention of how to find such an RBFN. By contrast, our universality statement is about a concrete learning rule. And, given a desired error level it tells how to set the parameters of the learning rule in order to achieve the desired approximation error in the dense sample limit.
%\end{remark}






\subsubsection{Convergence in probability with uniformly distributed inputs}
\label{sec:probconv_LACKI}
Above we have given guarantees relative to the deterministic convergence rates of the input sample to the domain.
In this subsection, we shall study probabilistic convergence rates as a function of the sample size in situations where the sample is obtained by drawing inputs independently from a uniform probability distribution on $I=\inspace := [0,1]^d$. 

We can show that the worst-case prediction error given by $\sup_{x \in \inspace}\Metrico{\predfn(x)}{ f(x)}$ vanishes (up to the usual worst-case bounds in the presence of observational errors) in probability for canonical input-space metrics:  

%
%
%Under these conditions, we can prove that input sequence $\seq{\grid_n}{n \in \nat}$ becomes dense in probability:
%\begin{lem}
%For  $x \in \inspace = [0,1]^d$ let $\varepsilon \in (0,1)$ such that $\ball{\varepsilon}{x} =\{\xi \in \inspace | \norm{x-\xi}_\infty \leq \varepsilon \} \subset \inspace$. We have 
%\[ \Pr[\min\{ \norm{x - s}_\infty \,| \, s \in \grid_n \} \geq \varepsilon] \leq r(n) \]
%where 
%\[r(n) = \Bigl(1- \varepsilon^d \Bigr)^n \stackrel{n \to \infty}{\longrightarrow} 0.\]
%\begin{proof}
% It is easy to see that we have $\Pr[ \ball{\varepsilon}{x} ] = \int_{\xi \in \inspace} \indicator{\ball{\varepsilon}{x}} (\xi) \d \xi \geq \varepsilon^d$. 
%%
%Hence, 
%\begin{align}
%&\Pr[\min\{ \norm{x - s}_\infty \,| \, s \in \grid_n \} \geq \varepsilon ]  \\
%&=\Pr[\forall s \in \grid_n: \norm{x - s}_\infty \geq \varepsilon] \\
%&\stackrel{i.i.d.}{=} \prod_{i=1}^n \Pr[s_i \notin \ball{\varepsilon}{x}] \\
%&= \prod_{i=1}^n 1-\Pr[s_i \in \ball{\varepsilon}{x}] \\
%&\leq \prod_{i=1}^n 1-\varepsilon^d = (1-\varepsilon^d)^n.
%\end{align}
%\end{proof}
%\end{lem}

\begin{thm} Let $\inspace = [0,1]^d $ be the domain of target function $f \in \hoelset {L^*} { } \hexp $. Assume the input data $\grid_n = \{s_1,\dots,s_n\}$ contains $n$ data sample inputs which are drawn independently at random from a uniform distribution over $\inspace$. Furthermore, assume there are no observational errors, i.e. $\obserrbnd =0$, and, that $\metric(x,x') = \norm{x-x'}_\infty, \forall x,x' \in \inspace$. The worst-case error of our LACKI predictor vanishes in probability. 

That is, 
$$\forall \epsilon >0 \forall \delta \in (0,1) \exists N \in \nat \forall n \geq N : \Pr[ \sup_{x \in \inspace} \Metrico{\predfn(x)}{f(x)} >\epsilon] \leq \delta.$$
In particular, for all $\delta \in (0,1)$ we have 
$\Pr[ \sup_{x \in \inspace} \Metrico{\predfn(x)}{f(x)} >\epsilon] \leq \delta$
\begin{enumerate}
\item  for any $\epsilon \geq 2 L^*$, provided that $n \geq 1$;
\item for any $\epsilon < 2 L^*$, provided that $n \geq N := \ceil{\frac{ \log(\delta \, 2^{-kd}  )}{\log(1- 2^{-kd})} }$ with $k= \ceil{\frac{\log(\epsilon^{-1}2 L^*)}{\log 2}}$.
\end{enumerate}
\begin{proof}
Let $r_n := \sup_{x \in \inspace} \min_{s \in \grid_n} \metric(x,s) = \sup_{x \in \inspace} \min_{s \in \grid_n} \norm{x-s}_\infty \leq 1$ and let 

$P_n^\epsilon := \Pr[ \sup_{x \in \inspace} \Metrico{\predfn(x)}{f(x)} >\epsilon]$ which we intend to bound from above.
Remember, from Cor. \ref{cor:worstcaseconvhoeldertarget} $\sup_x \Metrico{\predfn(x)}{f(x)} \leq 2 L^*  r_n $. Hence, for $\epsilon \geq 2 L^*$, $P_n^\epsilon \leq 0, \forall n \in \nat$.

So, it suffices to focus on the case where $\epsilon < 2 L^*$. Now, $\sup_x \Metrico{\predfn(x)}{f(x)} \leq \epsilon  $ is implied by $\sup_x \Metrico{\predfn(x)}{f(x)} \leq 2 L^* r_n $ provided that $  r_n  \leq \frac {\epsilon}{2 L^*}$. So, we define an event $E_n$ that ensures $r_n$ satisfies the latter inequality with a probability that grows as $n$ increases.
To this end, we introduce a partition of the domain into $m$ hyper-rectangles $H_1,...,H_m$ of equal size, each having edge length $l_k=\frac 1 {2^k}$ where $k$ is a natural number such that $l_k \leq  \frac {\epsilon}{2 L^*} $. As a valid choice, we set $k:= \ceil{\frac{\log(\epsilon^{-1}2 L^*)}{\log 2}}$. Note, $\Pr[s_i \in H_j] = l_k^d = \frac{1}{2^{dk}}$.  By construction, in the event that each hyper-rectangle ends up containing at least one sample input of $\grid_n$, we have  $r_n \leq \frac {\epsilon}{2 L^*}$. 
We define the complement of this event as $\bar E_n := \{(s_1,...,s_n)  \in \inspace^n | \exists j \in \{1,...,m\} \forall i \in \{1,...,n\}: s_i \notin H_j  \}$. Let  $W:= \{ s=(s_1,...,s_n)  | \sup_x \Metrico{\predfn(x)}{f(x)} > \epsilon \}$ be the event that the sample inputs are located in such a fashion that they give rise to a worst-case error larger than $\epsilon$.  We have: $s \notin \bar E$ implies that $r(n) \leq \frac {\epsilon}{2 L^*} $ which in turn implies $\sup_x \Metrico{\predfn(x)}{f(x)} \leq \epsilon $, i.e. that $s \notin W$. Hence, $W \subseteq \bar E_n$ and thus, $ P_n^\epsilon =\Pr[W] \leq \Pr[\bar E_n]$.
So, to bound $P_n^\epsilon$ from above it suffices to bound $\Pr[\bar E_n]$ from above which we will do next: We can employ the union bound, utilise that $m = 2^{kd}$ and the fact that the $s_i$ are drawn i.i.d. from a uniform to see that $\Pr[\bar E_n] \leq \sum_{j=1}^m \prod_{i=1}^n \Pr[s_i \notin H_j] = 2^{kd}  (1-\frac{1}{2^{dk}})^n \stackrel{n \to \infty}{\convto} 0$ which shows the main statement of the theorem. To find an $n$ sufficently large to ensure $\Pr[W] \leq \delta$ we consider the inequality $2^{kd}  (1-\frac{1}{2^{dk}})^n \leq \delta$. Taking the $\log$ on both sides and rearranging yields the sufficient condition: $n \geq \frac{ \log(\delta \, 2^{-kd}  )}{\log(1- 2^{-kd})}$. 
\end{proof}
\end{thm}



\subsubsection{Some guarantees for online learning}


In the theorems above, we considered the worst-case asymptotics for the case where the data becomes dense in the domain. Here the error was evaluated on the entire input domain. By contrast, we will now consider an online learning setting where we incrementally get to observe samples along the trajectory of inputs $\seq{x_n}{n \in \nat }$ and are interested in the long-term one-step-lookahead prediction errors on this trajectory.
That is, we are interested in the evolution of prediction errors $\Metrico{\predfn(x_n)}{f(x_n) }$
where the predictor $\predf_{n}(\cdot)$ is based on $\data_{n} = \data_{n-1} \cup \{ \bigl(\state_{n-1}, \tilde f(\state_{n-1}) \bigr)\}, \forall n >1 $. 

We will show that this error trajectory vanishes (up to observational errors), provided that the input sequence $\seq{x_n}{n \in \nat}$ is bounded.

In preparation of these considerations, we will establish the following facts:

\begin{lem}
Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs with $x_n \in \inspace$ where input space $\inspace$ can be endowed with a shift-invariant measure. Furthermore, assume the sequence  is bounded, i.e.  
$\metric_\inspace(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
Finally assume the inputs of the available data coincide with the complete history of past inputs, i.e. $G_n = \{ x_i | i \in \nat, i < n\}$.
Then we have: \[ \dist(G_n,x_n) = \min\{\metric_\inspace(g,x_n) | \, g \in G_n\} \stackrel{n \to \infty}{\longrightarrow} 0.\]
\begin{proof}
The intuition behind the following proof is that if the distances were not to converge, there was an infinite number of disjoint balls around the input points that summed up to infinite volume. This however, would be a contradiction to the presupposed boundedness of the sequence.
We formalise this intuition as follows:
We can rephrase the desired convergence statement as 
\begin{equation}
\forall \epsilon > 0 \exists n \in \nat \forall m \geq n : \dist(x_{m}, G_{m}) \leq \epsilon.
\end{equation} 
For contradiction, assume that
\begin{equation}
\exists \epsilon > 0 \forall n \in \nat \exists m(n) \geq n : \dist(x_{m(n)}, G_{m(n)}) > \epsilon.
\end{equation} 
Hold such an $\epsilon >0$ fixed and choose any $n \in \nat$. 
By definition of $G_{m(n)} =\{ x_i | i < m(n)\} $ we have:
\eqn{eq:i34kjjk3}{\forall i < m(n) : \metric_\inspace(x_{m(n)},x_i) > \epsilon.}

Let $C_n := \bigcup_{i < n} \ball{\frac \epsilon 2}{x_i} $ be the union of all $\frac \epsilon 2$-balls around each point in $G_n$ and define $\bar I = \bigcup_{n \in \nat} C_n$.
By definition, each $x_n$ is contained in $\bar I$.
Since sequence $(x_n)_{n \in \nat}$ is bounded, $\bar I $ has a finite volume relative to some positive, shift-invariant measure $\mu$. I.e. $\mu(\bar I) < \infty$ (e.g. choose the Lebesgue measure for $\mu$). Furthermore, $\mu(C_n) \leq \sum_{i <n} \mu(B_i) \leq \mu(\bar I)< \infty$ where $B_i := \ball{\frac \epsilon 2}{x_i}$. Owing to the assumed shift-invariance, we can assign the same measure $M$ each ball, i.e. $M:=\mu(B_1) = \mu(B_n)\forall n \in \nat$. Thus, $\mu(C_n) \leq n M$.
Define $q:= \ceil{\frac{\mu(\bar I)}{M}} \in \nat$. This is an upper bound on the number of disjoint balls of measure $M$  that can be contained in $\bar I$. Intuitively, since this number is finite, there cannot be an infinite number of non-intersecting balls around the elements of the sequence $(x_n)_{n \in \nat}$. More formally our argument proceeds as follows:
Choose $n > q+1$. Statement (\ref{eq:i34kjjk3}) yields:
\eqn{eq:i34kjjk33}{\forall i \in \{1,...,n\} \exists p(i) \geq i \forall j \leq p(i): \metric_\inspace(x_{p(i)},x_j) > \epsilon.}  Define a permutation $\pi$ such that $\pi(p(1)) \leq \ldots \leq \pi(p(n))$. 
With Statement (\ref{eq:i34kjjk33}) it follows that \\
${\metric_\inspace(x_{\pi(p(i))},x_{\pi(p(j))}) > \epsilon}$ , $\forall i,j =1,...,n, i < j$. Thus, we conclude the disjointness conditions $B_{\pi(p(i))} \cap B_{\pi(p(j))} = \emptyset , \forall i,j =1,...,n, i \neq j$. 
Hence,  $\mu(\bar I) \geq \mu(C_{\pi(p(n))}) \geq \mu(C_{\pi(p(1))}) + \sum_{i=1}^n \mu(B_{\pi(p(i))}) \newline = \mu(C_{\pi(p(1))}) +  n M > \mu(C_{\pi(p(1))}) + (q+1) M \geq\mu(C_{\pi(p(1))}) + \mu(\bar I)$, where the last inequality follows from the fact that  $M q= M \ceil{\frac{\mu(\bar I)}{M}} \geq \mu(\bar I)$. Since $\mu(C_{\pi(p(1))}) \geq 0$, we have concluded the false statement $\mu(\bar I) > \mu(\bar I)$.

%Hence, $\mu(\bar I) \geq \mu(C_{\pi(N_n)+1}) = \mu(C_{\pi(N_1)}) + \sum_{i=1}^n \mu(B_{\pi(N_i)}) = \mu(C_{\pi(N_1)}) +  n M > \mu(C_{\pi(N_1)}) + (m+1) M >\mu(C_{\pi(N_1)}) + \mu(\bar I)$ by definition of $m= \ceil{\frac{\mu(\bar I)}{M}}$. But since $\mu(C_{\pi(N_1)}) \geq 0$, we conclude the false statement $\mu(\bar I) > \mu(\bar I)$.
\end{proof}
\label{lem:bndseq_entails_distgridvanish}
\end{lem}  

\begin{thm}
Assume that, for some $q\geq0$, we chose $\hestthresh = 2 \obserrbnd + q$ in our LACKI prediction rule. And, assume that the target $f$ is H\"older continuous up to some error level $\bar E_h$. That is, $f = \phi + \psi$ with $\phi \in \hoelset {L^*} { } \hexp$ and a function $\psi$ such that $\sup_x \metric_\outspace\bigl(0,\psi(x)\bigr) \leq \bar E_h \in \Real$.

Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs that is bounded, i.e. where 
$\metric(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
Furthermore, assume $\data_{n+1} = \data_n \cup \{ \bigl(x_n, \tilde f(x_n)\bigr) \}$ and thus, $\grid_n = \{ x_i | i \in \nat, i < n\}$.
Then the prediction error on the sequence vanishes up to the level of sample-consistency and H\"older continuity in the following sense:
 \[\metric_\outspace\bigl(\predfn(x_n),f(x_n) \bigr) \stackrel{n \to \infty}{\longrightarrow} [0,\frac q 2 + 2  \obserrbnd  + 2 \bar E_h].\]
In particular, in case the observations are error-free ($\tilde f = f$) and assuming the target is H\"older continuous then, when choosing $\hestthresh = 0$, the prediction error is guaranteed to vanish. That is,
\[\metric_\outspace\bigl(\predfn(x_n),f(x_n) \bigr) \stackrel{n \to \infty}{\longrightarrow}0.\]

\begin{proof}

Let $\xi_n  \in \argmin_{g \in \grid_n} \metric(x_n,g)$ denote the nearest neighbour of $x_n$ in $\grid_n = \{x_1,...,x_{n-1}\}$.

Since sequence $(x_n)$ is bounded, Lem. \ref{lem:bndseq_entails_distgridvanish} is applicable and hence: (i) $\lim_{n \to \infty} \metric (x_n,\xi_n) = 0$.

From Lem. \ref{lem:LACKIsampleconsistency} we conclude 
$\metric_\outspace\bigl(\predfn(\xi_n) ,  f(\xi_n)  \bigr) \leq 2\obserrbnd +  \frac q 2$. Hence, appealing to the triangle inequality, we see that 
(ii) $\metric_\outspace\bigl(\predfn(x_n) ,  f(\xi_n)  \bigr) \leq \metric_\outspace\bigl(\predfn(x_n) ,  \predfn(\xi_n) \bigr) + 2 \obserrbnd + \frac q 2$.



Moreover we note that the predictors $\predfn$ have H\"older constants $L(n)$ and that the $L(n)$ are bounded from above by some $\bar L \in \Real$. Thus,  $(iii)$ $\exists \bar L \in \Real\forall n \in \nat : \predfn \in \hoelset {\bar L} { } \hexp$. 
  
In conclusion,
$0\leq\metric_\outspace\bigl(\predfn(x_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) ,  f(\xi_n)  \bigr) + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \stackrel{(ii)}{\leq} \metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) + 2 \obserrbnd + \frac q 2 + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) +2 \obserrbnd + \frac q 2 + \metric_\outspace\bigl(\phi(\xi_n) , \phi(x_n)\bigr) + 2 \bar E_h 
\newline
\stackrel{(iii)}{\leq} (\bar L+ L^* ) \metric(x_n,\xi_n )^\hexp + 2 \obserrbnd + \frac q 2 + 2 \bar E_h  \stackrel{n \to \infty}{\longrightarrow} 2 \obserrbnd + \frac q 2 + 2 \bar E_h $.
\end{proof}
\label{thm:vanisishingseqprederr_LACKI}
\end{thm} 
%
%\subsubsection{misc}
%We make the following assumptions:
%\begin{enumerate}
%\item Target function $f: \inspace \to \outspace = \Real^m$ has H\"older constant $L^* < \infty$ and exponent $\hexp$. 
%\item Parameter $\hestthresh$ is chosen to at least twice the level of observational error, i.e. $\hestthresh \geq 2 \obserrbnd$.
%\end{enumerate}
%
%\begin{lem}
%Define $E^\infty_n:= \sup_{x \in \inspace} \metric(\predfn(x),f(x))$ to be the worst-case error between the predictor and the target. Under the above assumptions this error is bounded as follows:  $$E^\infty_n \leq \mu_n =  2 L^* r_x(n)^\hexp +  \frac \hestthresh 2 +\obserrbnd$$
%where 
%$r_x(n) := \sup_{x \in \inspace} \inf_{s \in \grid_n} \metric(s,x)$ is the worst-case distance of any query input from the input data.
%
%
%\begin{proof}
%
%In the LACKI paper it was shown that 
%\begin{equation}
%\metric_\outspace\bigl(\predfn(x) , f(x)\bigr)  \in \bigl[0, (L(n)+ L^*) r_x(n)^\hexp +  \frac \hestthresh 2 +\obserrbnd \bigr] \end{equation} for any  $ x \in \inspace, n \in \nat$ and  any choice of parameter $\hestthresh \geq 0$.
%And, if $\hestthresh$ was chosen to be at least as large as $2 \obserrbnd$ then $L(n)$ is bounded by some number $\bar L \leq L^*$. Hence, we have 
%\begin{equation}
%\metric_\outspace\bigl(\predfn(x) , f(x)\bigr) \leq (\bar L+ L^*) r_x(n)^\hexp +  \frac \hestthresh 2 +\obserrbnd  \leq \mu_n < \infty,  \forall x \in \inspace, n \in \nat \end{equation}
%\end{proof}
%
%\end{lem}
%
%An immediate consequence is that if that data is sufificently representative then the worst-case prediction error is bounded. 
%In particular, for bounded input space of interest, we obtain boundedness of the worst case error (cf. Assumption 1 in the MPC part of this paper):
%
%\begin{cor}
%If  $\inspace$ is bounded, i.e. $\sup_{x \in \inspace} \metric(0,x) < \infty$ then $r_x(n) = \sup_{x \in \inspace} \inf_{s \in \grid_n} \metric(s,x) < \infty, \forall n \in \nat$ and thus, $\mu_n < \infty$.
%In this case, the the worst-case prediction error is bounded:
%$$E^\infty_n \leq \mu_n =  2 L^* r_x(n)^\hexp +  \frac \hestthresh 2 +\obserrbnd < \infty.$$
%\end{cor}
%
%
%Note, that by definition of the bounds $\mu_n$ on the worst-case prediction error that these bounds are not increasing with incrementallygrowing data size. Furthermore, if the sequence $\seq{\grid_n}{n \in \nat}$ of input data converges to the input space $\inspace$ uniformly, the prediction error sequence $E^\infty_n$ vanishes as $n \to \infty$ Formally, we can write this as follows:
%
%\begin{lem}
%\begin{enumerate}
%\item If $\data_n \subset \data_{n+1}, \forall n $
%then $\mu_m \geq \mu_n \forall m \leq n$.
%\item If  $\grid_n \stackrel{unif}{\to} \inspace$ then $E^\infty_n \to [0,\frac \hestthresh 2 +\obserrbnd] $  as $n \to \infty$.
%\end{enumerate}
%\begin{proof}
%\begin{enumerate}
%\item  $\data_n \subset \data_{n+1}$ implies $r_x(n) \geq r_x(n+1)$. The rest follows by induction appealing to the definition of $\mu_n$.
%\item $\grid_n \stackrel{unif}{\to} \inspace$ implies that $r_x(n) \to 0$ as $n \to \infty$. The rest follows from $0 \leq E^\infty_n \leq \mu_n = 2 L^* r_x(n)^\hexp +  \frac \hestthresh 2 +\obserrbnd \stackrel{n \to \infty}{ \to} \frac \hestthresh 2 +\obserrbnd $.
%\end{enumerate}
%\end{proof} 
%\end{lem}
%
%\begin{lem}
%Assume growing data, i.e. $\forall n: \data_n \subset \data_{n+1}$.
%The worst-case distance between two predictions is bounded by twice the bound on the worst-case error of the predictor that was based on the least amount of data.
%That is,  
%$$ \forall m,n \text{ with } m \leq n: \metric(\predfn(x),\predf_m(x) ) \leq 2 \mu_m, \forall  x \in \inspace.$$
%In particular, is the worst-case discrepancy between predictors bounded, i.e. 
%$$ \forall m,n, x \in \inspace: \metric(\predfn(x),\predf_m(x) ) \leq 2 \mu_1.$$
%\begin{proof}
%This follows trivally by appealing to the previous lemma and the triangle-inequality of pseudometrics:
%For any $m \leq n$ we have $\mu_m \geq \mu_n$. Hence, $\forall x: \metric(\predfn(x),\predf_m(x) ) \leq  \metric(\predfn(x),f ) +  \metric(f,\predf_m(x) ) \leq \mu_n+ \mu_m \leq 2 \mu_m$.
%\end{proof} 
%\end{lem}



%\begin{remark}
%Note, the bound on the speed of convergence generally decreases with increasing best Lipschitz constant of the RBFN. Generally, the Lipschitz constant will increase with decreasing $\hestthresh$. Therefore, so far, we have not shown convergence in the case of $\hestthresh=0$. 
%Intuitively, we should still have convergence since in the limit $L^* \to \infty$ the KI rule seems to coincide with a nearest neighbour regression rule. By construction of integrable functions, it should be clear that this rule converges to any function in the set $\mathcal L_q$ of power-$q$ integrable function  with respect to the $\mathcal L_q$ metric and $q \in \nat$.
%Investigating this observation in greater rigour could be subject to future work. Of course, from a practical point of view our current results are sufficient. If we set $\hestthresh >0$ below the machine-epsilon of the computer the algorithm is intended to run on, our results ensure that the algorithm will not be able to distinguish $\predfn(x)$ and the target $f$ for any input value and sufficiently large training data size $N_n \in \nat$.
%\end{remark}

\subsubsection{Computational complexity}
The computational complexity for computing the parameter update $L(n+1)$ based on $L(n)$, the pre-existing data $\data_n$ of size $N_n$ and a newly arriving sample input is in $\mathcal O(N_n m) $ where $m$ is the effort for evaluating the pseudo-metric. Typically, $m$ will scale linearly with the dimensionality of the input space. Therefore, online updates cost training time that will be linear in the number of existing training data and input dimensionality. In batch training, for a batch of $N$ samples, computation of the estimate will require an effort in $\mathcal O(N^2 D)$. 
Once the parameter $L(n)$ is computed, the effort for evaluating $\predfn(x)$ is linear in the number of samples and, again, typically linear in the input and output space dimensionality. 

However, it should be noted though that generalised nearest neighbor techniques can be utilised to reduce the prediction effort to expected logarithmic effort in the sample size (see \cite{Beliakov2006}). Devised for standard Lipschitz interpolation, this approach could be readily applied to our LACKI inference rule.

%\input{content/Ch_kinkyinf/KIMRAC_wingrock_old}
%============== WINROCK ===========================================
\section{Lazily Adaptive Constant Kinky inference and model reference adaptive control}
\label{sec:MRAC_lacki}
So far, we have established some learning guarantees for LACKI as a method for supervised learning. In this section, we utilise our results and discuss the use of LACKI in the context of model-reference adaptive control. We introduce the control framework with a simple example of controlling the simulated roll dynamics of an aircraft under wing rock. In the second half of the remainder of the paper, we use our theoretical guarantees established in the first half in order to provide global asymptotic convergence guarantees of the closed-loop trajectory to the reference. 
Throughout the entire section we simplify our analysis by assuming the pseudo-metrics $\metric$ and $\metric_\outspace$ are in fact canonical norm-induced metrics. For instance, we assume that $\inspace = \Real^d$ is a finite-dimensional vector space and we have $\metric(x,x') =\norm{x-x'}$ for some norm $\norm{\cdot}$ equivalent to the maximum norm $\norm{\cdot}_\infty$.

\subsection{Online learning and tracking control in the presence of wing rock dynamics }
\label{sec:KIMRAC}
As pointed out in \cite{chowdharyacc2013}, modern fighter aircraft designs are susceptible to lightly damped oscillations in roll known as ``wing rock''. Commonly occurring during landing \cite{Saad2000}, removing wing rock from the dynamics is crucial for precision control of such aircraft.
Precision tracking control in the presence of wing rock is a nonlinear problem of practical importance and has served as a test bed for a number nonlinear adaptive control methods \cite{Chowdhary2013,Monahemi1996,chowdharyacc2013}.

For comparison, we replicate the experiments of the recent work of Chowdhary et. al. \cite{Chowdhary2013,ChowdharyCDC2013}.\footnote{We are grateful to the authors for kindly providing the code.}
Here the authors have compared their Gaussian process based approach, called \textit{GP-MRAC}, to the more established adaptive model-reference control approach based on RBF networks \cite{Sanner1992,Kim1998}, referred to as \textit{RBFN-MRAC}. Replacing the Gaussian process learner by our kinky inference learner, we readily obtain an analogous approach which we will refer to as \textit{LACKI-MRAC}. As an additional baseline, we also examine the performance of a simple P-controller.

While with the exact same parameters settings of the experiments in \cite{Chowdhary2013}, performance of our LACKI-MRAC method comes second to GP-MRAC, we also evaluate the performance of all controllers over a range of 555 random parameter settings and initial conditions. As we will see, across this range of problem instances and parameter settings, LACKI-MRAC markedly outperforms all other methods.

\subsubsection{Model reference adaptive control}\label{sec:mrac}
Before proceeding with the wing rock application we will commence with (i) outlining model reference adaptive control (MRAC) \cite{astroemadaptivectrlbook2013} as considered in \cite{Chowdhary2013} and (ii) describe the deployment of kinky inference to this framework. 
We will now rehearse the description of MRAC for second-order systems following \cite{Chowdhary2013}. 

Assume $m \in \nat$ to be the dimensionality of a configuration of the system in question and define $d = 2m$ to be the dimensionality of the pertaining state space $\statespace$.

Let $x = [x_1;x_2] \in \statespace$ denote the state of the plant to be controlled.
Given the control-affine system 
 
\begin{align}
\dot x_1 &= x_2 \\
\dot x_2 &= a(x) + b(x) \, u(x) \label{eq:secorddynctrlaff}
\end{align}

it is desired to find a control law $u(x)$ such that the closed-loop dynamics exhibit a desired reference behaviour:

\begin{align}
\dot \xi_1 &= \xi_2 \\
\dot \xi_2 &= f_{r}(\xi,r)
\end{align}
where $r$ is a reference command, $f_r$ some desired response and $t \mapsto \xi (t)$ is the reference trajectory.

If a priori $a$ and $b$ are believed to coincide with $\hat a_0, \hat b_0$ respectively, the inversion control 
$u = \hat b_0^{-1} (- \hat a_0 +u')$ is applied. This reduces the closed-loop dynamics to 
$\dot x_1 = x_2, \dot x_2 = u' + \tilde a(x,u) $
where $\tilde a(x,u)$ captures the modelling error of the dynamics: 
\begin{equation}
	\tilde a (x,u ) = a(x) - \hat a_0(x) + \bigl(b(x) - \hat b_0(x)\bigr) u.
\end{equation}
 Let $I_d \in \Real^{d \times d}$ denote the identity matrix.  If $b$ is perfectly known, then $b - \hat b_0^{-1} = 0$ and the model error can be written as $\tilde a (x)= a(x) - \hat a_0(x)$. In particular, $\tilde a$ has lost its dependence on the control input. 



In this situation \cite{Chowdhary2013,ChowdharyCDC2013} propose to set 
the pseudo control as follows: $u'(x) :=  \nu_{r} + \nu_{pd} - \nu_{ad}$ where $\nu_{r} = f_{r}(\xi,r)$ is a feed-forward reference term,  $\nu_{ad}$ is a yet to be defined output of a learning module \emph{adaptive element} and $\nu_{pd} = [K_1 K_2] e$ is a feedback error term designed to decrease the \textit{tracking error} $e(t) = \xi(t) - x(t)$ by defining $K_1,K_2 \in \Real^{m \times m}$ as described in what is to follow.

Inserting these components, we see that the resulting \textit{error dynamics} are:


\begin{equation}\label{eq:errordynmrac}
	\dot e = \dot \xi - [x_2; \nu_r + \nu_{pd}+ \tilde a(x) ] = M e + B \bigl(\nu_{ad}(x) -  \tilde a(x)\bigr)
\end{equation}


where $M = \left(\begin{array}[h]{cc}
			O_m &  \, I_{m}\\
			-K_1 & -K_2 
					\end{array}\right)$ and $B = \left(\begin{array}[h]{c}
			O_m \\ I_m
					\end{array}\right)$.
If the feedback gain matrices $K_1,K_2$ parametrising $\nu_{pd}$ are chosen such that $M$ is stable then the error dynamics converge to zero as desired, provided the learning error $E_\lambda$ vanishes: $E_\lambda (x(t)) = \norm{\nu_{ad}(x(t)) -  a(x(t))} \stackrel{t \to \infty} {\longrightarrow} 0$. 

It is assumed that the adaptive element is the output of a learning algorithm that is tasked to learn $\tilde a$ online. This is done by continuously feeding it training examples of the form $\bigl(x(t_i), \tilde a(x(t_i)) + \varepsilon_i\bigr)$ where $\varepsilon_i$ is observational noise.  

Intuitively, assuming the learning algorithm is suitable to learn target $\tilde a$ (i.e. $\tilde a$ is close to some element in the hypothesis space \cite{mitchellbook:97} of the learner) and that the controller manages to keep the visited state space bounded, the learning error (as a function of time $t$) should vanish.

Substituting different learning algorithms yields different adaptive controllers. \textit{RBFN-MRAC} \cite{Kim1998} utilises radial basis function neural networks for this purpose whereas \textit{GP-MRAC} 
employs Gaussian process learning \cite{GPbook:2006} to learn $\tilde a$ \cite{Chowdhary2013,ChowdharyCDC2013}. 

%\jcom{possibly the following paragraph will go into a related work section:}
%Note, this setting of GP-MRAC is a special case of the SP-SIIC approach we introduced in Ch. \ref{ch:SPSIIC}. Here $\hat a_0$ is the prior mean function of the s.p. we place over the drift. Our exposition in Sec. \ref{ch:SPSIIC} is more general in that it allows for uncertain $b$ that is learned from data, considers under-actuated systems and makes no distributional restrictions. As an additional feature, GP-MRAC assumes that the data sets can be updated continuously. While of course this is not tractable the authors maintain a data corpus of a fixed size by a range of methods including simple FIFO queues as well as sparsification methods \cite{Kingravi2014,Csato2002}. In contrast, we utilise learning criteria to only include informative data points. In addition, we employ hyper-parameter optimisation which we show to be highly beneficial. While hyper-parameter training cannot be done at high frequency, it would be possible to run it in the background on a separate CPU (in parallel to the CPU on which the controller runs). 

In what is to follow, we utilise our LACKI method as the adaptive element. Following the nomenclature of the previous methods we name the resulting adaptive controller \textit{LACKI-MRAC}.

\subsubsection{The wing rock control problem}
The wing rock dynamics control problem considers an aircraft in flight. Denoting $x_1$ to be the roll attitude (angle of the aircraft wings) and $x_2$ the roll rate (measured in angles per second), the controller can set the aileron control input $u$ to influence the state $x := [x_1;x_2]$.

Based on \cite{Monahemi1996}, Chowdhary et. al. \cite{Chowdhary2013,ChowdharyCDC2013} consider the following model of the wing rock dynamics: 

\begin{align}
\dot x_1 &= x_2 \\
\dot x_2 &= a(x) + b \, u 
\end{align}
where $b =3$ is a known constant and 
$a(x) = W_0^* + W_1^* x_1 + W_2^* x_2 + W_3^* \abs{x_1} x_2 + W_4^* \abs{x_2} x_2 + W^*_5 x_2^3$ is an priori unknown nonlinear drift. 



Note, the drift is non-smooth but it would be easy to derive a Lipschitz constant on any bounded subset of state space if the parameters $W := (W_0^*,\ldots, W_5^*)$ were known.

To control the system we employ LACKI as the adaptive element $\nu_{ad}$.
In the absence of the knowledge of a Lipschitz constant, we start with a guess of $\underline L=1$ (which will turn out to be too low) and update it following the procedure described in Sec. \ref{sec:lacki}.

In a first instance, we replicated the experiments conducted in \cite{Chowdhary2013,chowdharyacc2013} with the exact same parameter settings. That is, we chose $W_0^* = 0.8, W_1^* = 0.2314, W_2^* = 0.6918, W_3^* = -0.6245, W_4^* = 0.0095, W_5^* = 0.0214$. 



The simulation initialised with start state $x = (3,6)^\top$ and simulated forward with a first-order Euler approximation with time increment $\tinc = 0.005 [s]$ over a time interval $\indsett = [t_0,t_f]$ with $t_0 = 0[s]$ and $t_f = 50[s]$. Training examples and control signal were continuously updated every $\Delta_u= \Delta_o = \tinc [s]$. The RBF and GP learning algorithms were initialised with fixed length scales of 0.3 units. The GP was given a training example budget of a maximum of 100 training data points to condition the posterior model on. Our LACKI learner was initialised with $\underline L =\hexp= 1$ and updated online following our lazy update method described above.

The test runs also exemplify the working of the lazy update rule.
The initial guess $\underline L=1$ was too low. However, our lazy update rule successfully picked up on this and had ended up increasing constant to $L=2.6014$ by the end of the online learning process.



%
%
\begin{figure*}
        \centering
				  \subfigure[Tracking error (RBF-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[ width=.3\textwidth, clip, trim = 2.5cm 8cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr2RBF}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Tracking error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 2.5cm 8cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr2GP}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Tracking error (KI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 2.5cm 8cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr2}
   % \label{fig:wingrockresultsbp}
  }
   \caption{Tracking error comparison of first example.}
	 \label{fig:wrtrackerrorsex1}
\end{figure*}	   

The results are plotted in Fig. \ref{fig:wrtrackerrorsex1}. 
We can see that in terms of tracking error of the reference our LACKI-MRAC outperformed RBF-MRAC and was a close runner-up to GP-MRAC which had the lowest tracking errors.  

%
To obtain an impression of the learning performance of the three learning algorithms we also recorded the prediction error histories for this example problem. The results are depicted in Fig. \ref{fig:wrprederrorsex1}. We can see that our kinky inference method and the GP method both succeeded in predicting the drift quite accurately while the RBFN method was somewhat lagging behind.
This is consistent with the observations made in \cite{Chowdhary2013,ChowdharyCDC2013}. The authors explain the relatively poor performance of the radial basis function network method by the fact that the reference trajectory on occasion led outside the region of state space where the centres of the basis function were placed in advance. By contrast, due to the non-parametric nature of the GP, GP-MRAC does not suffer from such a priori limitations. In fact, it can be seen as an RBF method that flexibly places basis functions around all observed data points \cite{GPbook:2006}. We would add that, as a non-parametric method, LACKI-MRAC shares this kind of flexibility, which might explain the fairly similar performance. 

However, being an online method, the authors of GP-MRAC explicitly avoided hyperparameter training via optimising the marginal log-likelihood. The latter is commonly done in GP learning \cite{GPbook:2006} to avoid the impact of an unadjusted prior but is often a computational bottle neck. Therefore, avoiding such hyperparameter optimisation greatly enhances learning and prediction speed in an online setting. However, we would expect the performance of the prediction to be dependent upon the hyperparameter settings. As we have noted above, the Lipschitz constant depends on the part of state space visited at runtime. Similarly, we might expect length scale changes depending on the part of state space the trajectory is in. Unfortunately, \cite{Chowdhary2013,ChowdharyCDC2013,chowdharyacc2013} provide no discussion of the length scale parameter setting and also called the choice of the maximum training corpus size ``arbitrary''. 

Since the point of learning-based and adaptive control is to be able to adapt to various settings, we test the controllers across a range of randomised problem settings, initial conditions and parameter settings.

We created 555 randomised test runs of the wingrock tracking problems and tested each algorithm on each one of them. The initial state $x(t_0)$ was drawn uniformly at random from $[0,7] \times [0,7]$, the initial kernel length scales were drawn uniformly at random from $[0.05,2]$, and used both for RBF-MRAC and GP-MRAC. The initial H\"older constant $\underline L$ for LACKI-MRAC was initialised at random from the same interval but was allowed to be adapted as part of the online learning process. Furthermore, we chose $\hestthresh =0$. The parameter weights $W$ of the system dynamics specified above were multiplied by a constant drawn uniformly at random from the interval $[0,2]$. To allow for better predictive performance of GP-MRAC we doubled the maximal budget to 200 training examples. 
The feedback gains were chosen to be $K_1=K_2=1$. 

In addition to the three adaptive controllers we also tested the performance of a simple $\hexp$ controller with just these feedback gains (i.e. we executed x-MRAC with adaptive element $\nu_{ad}=0$). This served as a baseline comparison to highlight the benefits of the adaptive element over simple feedback control.

The performance of all controllers across these randomised trials is depicted in Fig. \ref{fig:wingrockresultsbp}. Each data point of each boxplot represent a performance measurement for one particular trial.

\begin{figure*}
        \centering
				  \subfigure[Prediction v.s. ground truth  (RBF-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .3\textwidth, clip, trim = 3cm 9cm 3cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr4RBF}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Prediction v.s. ground truth  (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 3cm 9cm 3cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr4GP}
   % \label{fig:wingrockresultsbp}
  } 
					  \subfigure[Prediction v.s. ground truth  (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width=.3\textwidth, clip, trim = 3cm 9cm 3cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wr4}
   % \label{fig:wingrockresultsbp}
  } 
   \caption{Prediction vs ground truth comparisons for the first example. Both nonparametric methods accurately predict the true drift and clearly outperform the RBFN learner.}
	\label{fig:wrprederrorsex1}
\end{figure*}	   


\begin{figure}
        \centering
				  \subfigure[Results over 555 randomised examples.]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .5\textwidth, clip, trim = 1.5cm 8cm 1cm 7cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/wingrockbp}
   % \label{fig:wingrockresultsbp}
  } 
   \caption{Performance of the different online controllers over a range of 555 trials with randomised parameter settings and initial conditions. 1: RBF-MRAC, 2: GP-MRAC, 3:LACKI-MRAC, 4: P-Controller. LACKI-MRAC outperforms all other methods with respect to all performance measures, except for prediction runtime (where the parametric learner RBF-MRAC performs best).} 
       \label{fig:wingrockresultsbp}
\end{figure}	   
  
	
	For each method, the figures show the boxplots of the following recorded quantities: 
	\begin{itemize}
		\item \textit{log-XERR}: cummulative angular position error (log-deg), i.e. $\log(\int_{t_0}^{t_f} \norm{\xi_1(t) - x_1 (t)} \dt )$.
		\item \textit{log-XDOTERR}:  cummulative roll rate error (log-deg/sec.), i.e. $\log(\int_{t_0}^{t_f} \norm{\xi_2(t) - x_2 (t)} \dt )$.
		\item \textit{log-PREDERR}: log-prediction error, i.e. 
		
		$\log(\int_{t_0}^{t_f} \norm{\nu_{ad}(x(t)) - \tilde a(x(t))} \dt )$.
		\item \textit{log-CMD}: cummulative control magnitude (log-scale), i.e. $\log(\int_{t_0}^{t_f} \norm{u(t)} \dt )$.
		\item \textit{log-max. RT (predictions)}: the log of the maximal runtime (within time span $[t_0,t_f]$) each method took to generate a prediction $\nu_{ad}$ within the time span.
		\item \textit{log-max. RT (learning)}: the log of the maximal runtime (within time span $[t_0,t_f]$) it took each method to incorporate a new training example of the drift $\tilde a$.
	\end{itemize}
	
	As can be seen from Fig. \ref{fig:wingrockresultsbp}, all three adaptive methods outperformed the simple $\hexp$ controller in terms of tracking error. 
	
	In terms of prediction runtime, the RBF-MRAC outperformed both GP-MRAC and LACKI-MRAC. This is hardly surprising. After all, RBF-MRAC is a parametric method with constant prediction time. By contrast, both non-parametric methods will have prediction times growing with the number of training examples.
That is, it would be the case if GP-MRAC were given an infinite training size budget. Indeed one might argue whether GP-MRAC, if operated with a finite budget, actually is a parametric approximation where the parameter consists of the hyperparameters along with the fixed-size training data matrix. When comparing the (maximum) prediction and learning runtimes one should also bear in mind that GP-MRAC predicted with up to 200 examples in the training data set. By contrast, LACKI-MRAC undiscerningly had incorporated all 10001 training points by the end of each trial.

Across the remaining metrics, LACKI-MRAC markedly outperformed all other methods.

Note, we have also attempted to test all methods across a greater range of problem settings, including larger initial states, more varied hyper-parameter settings, lower feedback gains and more varied choices of dynamics coefficients $W$. However, this resulted in GP-MRAC to often run into conditioning problems. This is a common issue in GP learning due to the necessity of matrix inversion or Cholesky decompositions of the covariance matrix (it seems to be common practice to address this by hand-tuning the observational noise parameters). Similar behaviour ensued when setting the training size budget to large values. All these changes often resulted in long learning runtimes, spiky control outputs and thus, poor overall performance. Similarly, code execution of our RBF-MRAC implementation was frequently interrupted with error messages when the state was initialised to positions outside of the rectangle $[0,7] \times [0,7]$.

We have not investigated the root cause of these issues in greater detail yet. However, it might be worth exploring whether the great robustness of LACKI might be an additional selling point that sets it apart from other recent adaptive control methods. Such robustness is of course important in control settings such as flight control where failure or erratic behaviour of the adaptive element may result in critical incidents. 

An example where GP-MRAC failed to track the reference occurred when repeating our first experiment  with the following modifications: The initial state was chosen to be $x(t_0) = (-90,40)^\top$ corresponding to a rapidly rotating aircraft. Furthermore, the wing rock coefficients $W$ were multiplied by a factor of $5$, amplifying the non-linearities of the drift field. 

When initialised with a length scale parameter of 0.3, the GP ran into conditioning problems and caused the output of the adaptive element in GP-MRAC to produce spikes of very large magnitude and thus, further destabilised the system. We tried the problem with various kernel length scale settings ranging from $0.3$ to $20$. Increasing the length scale parameter to length scale of at least 1 seemed to fix the conditioning problem. Nonetheless, GP-MRAC still did not manage to learn and stabilise the system in any of these settings. A record of GP-MRAC's performance in this example (for length scale of 1) is depicted in Fig.  \ref{fig:gpfailGPWR1} -  \ref{fig:gpfailGPWR3}. As the plots show, GP-MRAC starts with relatively high tracking and prediction error from which it could not recover. At about 26 seconds into the simulation the state rapidly diverged.

 
\begin{figure*}
        \centering
				  \subfigure[Position (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 4cm 9cm 4cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail1}
   \label{fig:gpfailGPWR1}
  } 
					  \subfigure[Tracking error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 4cm 9cm 4cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail2}
   \label{fig:gpfailGPWR2}
  } 
							  \subfigure[Log - prediction error (GP-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[scale =.35]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_gpprederr}
    \label{fig:gpfailGPWR3}
  } 
					  \subfigure[Position (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 3.5cm 9cm 4cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail1_hfe}
    \label{fig:gpfailKIWR1}
  } 
					  \subfigure[Tracking error (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = 5.5cm, clip, trim = 3.5cm 9cm 4cm 10cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail2_hfe}
    \label{fig:gpfailKIWR2}
  } 
%
					  \subfigure[Log - prediction error (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[scale =.35,clip, trim = 0cm 0cm 0cm .1cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_hfeprederr}
    \label{fig:gpfailKIWR3}
  } 
						  %\subfigure[State path (KI-MRAC).]{
    %%\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    %\includegraphics[width = 5cm, clip, trim = 2cm 9cm 1cm 7cm]
								%%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								%{content/Ch_kinkyinf/figs/gpfail_statepathHfe}
   %% \label{fig:wingrockresultsbp}
  %} 	
	%
   \caption{Example where GP-MRAC fails. By contrast, LACKI-MRAC manages to adapt and direct the system back to the desired trajectory.}
	\label{fig:gpfail}
\end{figure*}	 


For comparison, we also tried LACKI-MRAC on the same problem, starting with initial $L=1$ as before. Starting out with a relatively large tracking and prediction error, LACKI-MRAC nonetheless managed to recover and successfully track the system (see  Fig.  \ref{fig:gpfailKIWR1} -  \ref{fig:gpfailKIWR3}). The state path and learned drift model obtained by LACKI-MRAC are depicted in Fig. \ref{fig:gpfail2}.
%
\begin{figure*}
        \centering
				  \subfigure[State path (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .4\textwidth, clip, trim = 3cm 9cm 3cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_statepathHfe}
   % \label{fig:wingrockresultsbp}
  } 	
	  \subfigure[Learned drift model (LACKI-MRAC).]{
    %\includegraphics[width = 3.7cm, height = 3cm]{content/figures/graph1_klein.eps}
    \includegraphics[width = .4\textwidth, clip, trim = 4.3cm 9cm 4cm 9cm]
								%{content/Ch_kinkyinf/figs/resultswingrock_555trials}
								{content/Ch_kinkyinf/figs/gpfail_hfelearnedmodel}
   % \label{fig:wingrockresultsbp}
  } 	
	%
   \caption{Depicted are the state path and the drift model learned online by LACKI-MRAC.}
	\label{fig:gpfail2}
\end{figure*}	 
%=============== WINGROCK END ===================================


%================ STABILITY DISCRETE TIME =================
\subsection{Stability guarantees in discrete-time systems}
\label{sec:KIMRACstabbounds}

In the previous section, we gave an illustration LACKI-MRAC -- a combination of a feedback-linearising controller with our KI learning method. The results are encouraging -- our adaptive control law managed to learn a dynamic system online and to track a reference in the presence of wing-rock dynamics where other methods failed. 
To simulate the dynamics we relied on a first-order Euler approximation resulting in a discrete-time dynamical system.

In this section, we study the convergence of LACKI-MRAC in such discrete-time systems.
In these we will consider both the offline and the online learning setting. In the former, the LACKI-learner receives a sample set once and builds a controller that remains unaltered during execution time.
For this case, we will provide robustness bounds on the control success (as quantified by a bound on the norm of the error dynamics) as a function of the remaining uncertainty of the trained LACKI model. 

In the online learning setting, which we considered in the wing-rock control simulations, the LACKI-learner gets updated with the most recent observation after each time step. Provided the initial uncertainty is bounded on the given state space, we will be able to guarantee that LACKI-MRAC leads to a closed-loop system that is globally asymptotically stable. 

\subsubsection{Tracking error bounds for the offline learning setting} 
In the offline learning setting, the predictor sequence $\seq{\predfn}{n \in \nat}$ of adaptive elements is based on only one fixed data set $\data_0$ at time $0$ which is not updated subsequently.
That is $\data_n = \data_0, \forall n \in \nat$.

Given some data set $\data_n =\data_0$ at time $n$ and the resulting predictor $\predfn(\cdot)$, the model error is given by $F_n(\cdot) := f(\cdot) - \predfn(\cdot)$. Since we assume constant data, the error does not change either. That is, we have $F_n(x) = \ldots = F_0(x) = F(x), \forall n,\forall x$.
 
In our analysis, we consider discrete-time dynamical systems. For example the dynamics might be first-order Euler approximations of the control-affine dynamics of Sec. \ref{sec:KIMRAC}.
Consequently, the error dynamics as per Eq. \ref{eq:errordynmrac} translate to the recurrence relation:
\begin{equation}\label{eq:errordynmrac_nIMRACdiscrete}
	e_{n+1}  = M e_n + \tinc F(x_n)
\end{equation}
where $\tinc \in \Real_+$ is a positive time increment and  $n$ is the time step index. Furthermore,
%
\begin{equation}
	F(x_n) = f(x_n) - \predfn(x_n) = B \bigl(\nu_{ad}(x_n) -  \tilde a(x_n)\bigr) 
\end{equation}
is an uncertain increment due to the model error of the learner (cf. Eq. \ref{eq:errordynmrac}), 						$B = \left(\begin{array}[h]{c}
				O_m \\ \tinc I_m
						\end{array}\right)$ and 

\begin{equation}
	M = \left(\begin{array}[h]{cc}
				I_m &  \, \tinc I_{m}\\
				-\tinc K_1 & I_m- \tinc K_2 
						\end{array}\right) 
\end{equation}
					is the (error state) transition matrix. 	
Here, $m = \frac d 2$ is half the dimensionality of the state space, $I_m$ denotes the $m \times m$ identity matrix and $K_1,K_2$ are gain matrices that can be freely chosen by the designer of the linear pseudo controller.		
%This is completely consistent with the uncertain recurrence considered in Eq. \ref{eq:dynextstatediscrete1}, with the exception, that the uncertainty of increment $F_n$ is not probabilistic. Instead it is an uncertain quantity reflecting the prediction error of the trained KI learner. Assuming its assumptions are met, Thm. \ref{thm:KIdesiderata} tells us that $F_n$ is interval-bounded. Employing the same type of argument as in Lem. \ref{lem:origprocdiscrfacts} we see that the solution of the recurrence is given by:
By induction, it is easy to show that the recurrence can be converted into the closed-form expression:
\begin{align*}
	\vc e_n &= M \vc e_{n-1} + \tinc \vc F(x_{n+1})  \\ 
	&= \dots= M^k \, \vc e_0 + \tinc \sum_{i=0}^{n-1} M^{n-1-i} \, \vc F(x_i)	.	
\end{align*}	
For vector norm $\norm{\cdot}$, let $\matnorm{\cdot}$ denote a matrix norm such that $\norm{Mv} \leq \matnorm{M} \norm{v}$ for all suitable matrices $M$ and vectors $v$. For instance, for the Euclidean norm $\norm{\cdot} =\norm{\cdot}_2$, we can choose the spectral norm $\matnorm{\cdot}= \specnorm{\cdot}$ as a matrix norm. Or, for  $\norm{\cdot} =\norm{\cdot}_\infty$, if the vector space is $d$-dimensional, we can choose the matrix norm $\matnorm{\cdot}= \sqrt{d} \specnorm{\cdot}$. We desire to bound the  norm of the error. To this end, we leverage that the norms are sub-additive and sub-multiplicative to deduce: 
\begin{align}
	\norm{\vc e_n} &\leq   \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \sum_{i=0}^{n-1}  \matnorm{M^{n-1-i}} \, \norm{\vc F(x_i)}		\\
	&\leq \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \maxerrn_n	 \sum_{i=0}^{n-1}  \matnorm{M^{n-1-i}} =: \varrho[n]
	\label{ineq:errnormbasic}
\end{align}
where  $\maxerrn_n$ is chosen such that we can guarantee that $\maxerrn_n	\geq \max_{i=1,...,n-1} \norm{F(x_i)}$.
For instance, we could choose $\maxerrn_n := \sup_{s \in \iaspace_n} \norm{F(s)} $
	where $\iaspace_n = \bigcup_{t< k} \{x \in \iaspace | \norm{x - \xi[t]} \leq \varrho[t] \}$ is the union of the possible states around the reference trajectory $\xi[\cdot]$ at previous time steps.
\begin{remark}	[Bounded error innovations] 
We assume there exists a maximum model error norm $\maxerrn$, i.e. $\forall i: \norm{F_i(x_i)} \leq \maxerrn$ for some bound $\maxerrn \in \Real$.
This is a realistic assumption in any physically plausible systems where the drift forces $a(x)$ are inevitably bounded. Since also, for any finite data, our LACKI learner has a bounded prediction function (cf. Lem. \ref{lem:LACKIpredbounded}), the discrepancy given by $F$ is bounded as well. 
\label{rem:bnd_err_innovations}
\end{remark}

Given the boundedness of $F$ we have: \vspace{-1em}
\begin{equation}
	\norm{\vc e_n} \leq   \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \maxerrn \sum_{i=0}^{n-1}  \matnorm{M^{n-1-i}}.
\end{equation}

The right-hand side is convergent provided the gains $K_1, K_2$ are chosen such that $M$ is stable, i.e. $\specrad(M) <1$, and provided $\maxerrn_n$ is bounded (see e.g. \cite{calliess2014_thesis}). 

Whether or not $M$ is stable, in low dimensions, the sums can be computed offline and in advance. This is of great benefit if 
 the controller that is building on the error bounds is utilising optimisation-based control with a finite time-horizon.   

To obtain a (conservative) closed-form bound on the error norms \cite{calliess2014_thesis}
contains a derivation and discussion of the following result:

\begin{thm}\label{thm:normboundsboundeddisturbmainbody}
Let $(F_n)_{n \in \nat_0}$ be a norm-bounded sequence of vectors with $\maxerrn_n :=\max_{i \in \{0,\ldots,n-1\}} \norm{F_i(x_i)} \leq \maxerrn \in \Real$. 
For error sequence $(e_n)_{n \in \nat_0}$ defined by the linear recurrence 
	$e_{n+1}  = M e_n + \tinc F_n(x_n) \,\,\,\, (n \in \nat_0)$, we can define the following bounds:
	
	\begin{enumerate}
	\item $\norm{\vc e_n} \leq \matnorm{M^{n}} \, \norm{\vc e_0} + \tinc \maxerrn_{n} \sum_{i=0}^{n-1}  \matnorm{M^{i}}$. If $\specrad(M) <1$ and $\exists \maxerrn$ $:\maxerrn\geq \maxerrn_{n-1} \geq 0, \forall n$, the right-hand side converges as $n \to \infty$.
	\item Let $k_0 \in \nat, k_0 >1$ such that $\matnorm{M^n} <1, \forall n \geq k_0$, let $\varphi := \matnorm{M^{k_0}} <1$ and let $\delta_n := \floor{n/k_0}$. If $r:=\specrad(M) < 1$, for $n > k_0$,  we also have:
	\begin{align*} \norm{\vc e_n} &\leq c \, \varphi^{\delta_n} \, \norm{\vc e_0} + \tinc \maxerrn_{n} \Bigl(\sum_{j=0}^{n_0-1} \matnorm{M^j} + c \, k_0 \frac{\varphi-\varphi^{ \floor{\frac{n}{k_0}}+1 }}{1-\varphi} \Bigr)\\
	& \stackrel{n \to \infty}{\longrightarrow} C \leq \tinc \maxerrn \sum_{j=0}^{n_0-1} \matnorm{M^j} 
	+ \frac{\tinc \maxerrn\,  c\, k_0 \,\varphi}{1-\varphi} 
	\end{align*} 
	for some constants $C,c \in \Real$.
	Here, possible choices for $c \in \Real$ are: 
	
(i) $c= \max\{\matnorm{M^i} | i=1,\ldots,k_0-1 \}$ 

or (ii) $c = \frac{1}{(d-1)!} \Bigl(\frac{1 - d}{\log r}\Bigr)^{d-1}	\matnorm{M}^{d-1}\, \, \, r^{\frac{1 - d}{\log r}-d+1}  $.
%
Since $\matnorm{M} \neq 1$, one can also choose (iii) $c:= \matnorm{M}^{n_0}$. %In this case, $\matnorm{M^k} \leq  \, \matnorm{M}^{n_0}^{(k \text{ div } k_0) +1} $.

\item If $\matnorm{M} \neq 1$, we have: \newline
$\norm{\vc e_n} \leq \matnorm{M}^{n} \, \norm{\vc e_0} + \tinc \maxerrn_{n}   \frac{1-\matnorm{M}^n}{1-\matnorm{M}}. $
	\end{enumerate}
%\begin{proof}
%The theorem is proven in \cite{calliess2014_thesis}.
%
%\end{proof}	
\end{thm}


\subsubsection{Global asymptotic stability in the online learning setting}
In this subsection, we lift the assumption that the available sample is static. Instead we assume that at time step $n+1$ we get to see an additional sample of the uncertain drift at the state visited in the previous time step $n$. 
That is, the predictor $\predf_{n+1}(\cdot)$ is based on $\data_{n+1} = \data_n \cup \{ \bigl(\state_n, \tilde f(\state_n) \bigr)\}, \forall n $.
Therefore, we also need to index the innovations vector field by time. That is, $F_n := f - \predfn$ denotes the prediction error function (or innovation) due to the data available at time $n \in \nat$. 
As pointed out in Rem. \ref{rem:bnd_err_innovations}, the error innovations $F_n$ are assumed to be bounded for all finite sample sets $\data_n$. 




Above, we have seen that any continuous function can be approximated by some H\"older continuous LACKI predictor up to an arbitrarily small error. 
For convenience, we will establish the following definition:

\begin{defn}
We say that a continuous function $f$ is $L^*-p$-H\"older \emph{up to} error $\bar E_h \in \Real$ on domain $\inspace$ iff there is an $L^*-p$-H\"older function $\phi \in \hoelset {L^*} { } p$ and a function $\psi$ such that $\forall x: f(x) = \phi(x)+\psi(x), \, \sup_{x \in \inspace} \metric_\outspace\bigl(0,\psi(x)\bigr) \leq \bar E_h$.
\end{defn}


%%\begin{lem} Assume the target $f$ is bounded on sub-domain $I \subseteq \inspace$ and that the data increases between time steps, i.e. $\data_n \subseteq \data_{n+1}, \forall n \in \nat_0$. Then we have:
%%\[\forall x \in I \subset \inspace : \norm{F_n (x)}_\infty \geq \norm{F_{n+1}(x)}_\infty.\]
%%\jcom{true? perhaps not needed anyway..}
%%\end{lem}
% 
%%Above theorems consider the case where the data becomes dense in the domain and we are interested in the worst-case prediction error. Relevant to our online-learning and control setting below is the situation where we are only interested in the error on a specific trajectory of inputs. If the prediction error on such a trajectory vanishes then we will be able to establish stability of the trajectory.
%%In preparation of these considerations, we will establish the following facts:
%
%%
%%\begin{lem}
%%Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs that is bounded, i.e. where 
%%$\metric(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
%%Define $\grid_n = \{ x_i | i \in \nat, i < n\}$.
%%
%%Then we have \[ \dist(\grid_n,x_n) = \min\{\metric(g,x_n) | \, g \in \grid_n\} \stackrel{n \to \infty}{\longrightarrow} 0.\]
%%\begin{proof}
%%The intuition of the following proof is that if the distances were not to converge there would be an infinite number of disjoint balls around the input points that summed up to infinite volume. This however, would be a contradiction to the presupposed boundedness of the sequence.
%%We formalise this intuition as follows:
%%For contradiction assume there is an $\epsilon >0$ such that for all $n \in \nat$ there exists an $N_n \geq n $ such that 
%%\begin{equation}
%%\dist(x_{N_n}, G_{N_n}) > \epsilon.
%%\end{equation} 
%%Hence, by definition of $G_{N_n} =\{ x_i | i < N_n\} $,
%%\eqn{eq:i34kjjk3}{\forall i < N_n : \metric(x_{N_n},x_i) > \epsilon.}
%%
%%Let $C_n := \bigcup_{i < n} \ball{\frac \epsilon 2}{x_i} $ be the union of all $\frac \epsilon 2$-balls around each point in $\grid_n$ and define $\bar I = \bigcup_{n \in \nat} C_n$.
%%By definition, each $x_n$ is contained in $\bar I$.
%%Since sequence $(x_n)_{n \in \nat}$ is bounded, $\bar I $ has a finite volume relative to some positive, shift-invariant measure $\mu$. I.e. $\mu(\bar I) < \infty$. Furthermore, $\mu(C_n) \leq \sum_{i <n} \mu(B_i) \leq \mu(\bar I)< \infty$ where $B_i := \ball{\frac \epsilon 2}{x_i}$. Since $M:=\mu(B_1) = \mu(B_n)\forall n \in \nat$ we have $\mu(C_n) \leq (n-1) M$.
%%Define $m:= \ceil{\frac{\mu(\bar I)}{M}}$.
%%Now, choose $n > m+1$. For $i=1,...,n$ $\exists N_i \geq i \forall j \leq N_i: \metric(x_{N_i},x_j) > \epsilon$.  Define a permutation $\pi$ such that $\pi(N_1) \leq \ldots \leq \pi(N_n)$. Hence, we have $\metric(x_{\pi(N_i)},x_{\pi(N_j)}) > \epsilon , \forall i,j =1,...,n, i < j$. Thus, $B_{\pi(N_i)} \cap B_{\pi(N_j)} = \emptyset , \forall i,j =1,...,n, i \neq j$. Hence, $\mu(\bar I) \geq \mu(C_{\pi(N_n)+1}) = \mu(C_{\pi(N_1)}) + \sum_{i=1}^n \mu(B_{\pi(N_i)}) = \mu(C_{\pi(N_1)}) +  n M > \mu(C_{\pi(N_1)}) + (m+1) M >\mu(C_{\pi(N_1)}) + \mu(\bar I)$ by definition of $m= \ceil{\frac{\mu(\bar I)}{M}}$. But since $\mu(C_{\pi(N_1)}) \geq 0$, we conclude the false statement $\mu(\bar I) > \mu(\bar I)$.
%%\end{proof}
%%\label{lem:bndseq_entails_distgridvanish}
%%\end{lem} 
%%
%%
%\begin{lem}
%As before, let the observational noise level be bounded by $\obserr$ and assume the output- space pseudo-metric to be translation-invariant.
%Let target $f$ be $L^*-p$-H\"older up to error $E$. That is, there is an $L^*-p$-H\"older function $\psi$ and a function $\phi$ such that $\forall x: f(x) = \phi(x)+\psi(x), \, \metric_\outspace\bigl(0,\psi(x)\bigr) \leq E $.
%
%Assume we are given a trajectory $\seq{x_n}{n \in \nat}$ of inputs that is bounded, i.e. where 
%$\metric(x_n,0) \leq \beta$ for some $\beta \in \Real_+$ and all $n \in \nat$.
%Furthermore, assume $\data_{n+1} = \data_n \cup \{ \bigl(x_n, \tilde f(x_n)\bigr) \}$ and thus, $\grid_n = \{ x_i | i \in \nat, i < n\}$.
%Then the prediction error on the sequence vanishes, i.e. \[\metric_\outspace\bigl(\predfn(x_n),f(x_n) \bigr) \stackrel{n \to \infty}{\longrightarrow} \metric_\outspace(0,\obserr) + 2E.\]
%\begin{proof}
%We have established that $\predfn$ is $L(n)-p$- H\"older with $L(n) \leq \bar L$ for some $\bar L \in \Real_{\geq 0}$.
%
%Since sequence $(x_n)$ is bounded, Lem. \ref{lem:bndseq_entails_distgridvanish} is applicable. 
%Let $\xi_n := \argmin_{g \in \grid_n} \metric(x_n,g)$ denote the nearest neighbour of $x_n$ in $\grid_n = \{x_1,...,x_{n-1}\}$.
%Hence, $\forall n \in \nat: \metric (x_n,\xi_n) \to 0$ as $n \to \infty$.
%
%We have:
%$\metric_\outspace\bigl(\predfn(x_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) ,  f(\xi_n)  \bigr) + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \stackrel{(i)}{=}\metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) +\metric_\outspace\bigl(0 , \obserr\bigr) + \metric_\outspace\bigl(f(\xi_n) , f(x_n)\bigr) \leq \metric_\outspace\bigl(\predfn(x_n) , \predfn(\xi_n) \bigr) +\metric_\outspace\bigl(0 , \obserr\bigr) + \metric_\outspace\bigl(\phi(\xi_n) , \phi(x_n)\bigr) + 2E \stackrel{(ii)}{\leq} 2 \max\{\bar L, L^* \} \metric(x,\xi_n^x )^\hexp + \metric_\outspace(0,\obserr) + 2E \longrightarrow \metric_\outspace(0,\obserr) + 2E$.
%where steps denoted by (i) follow from Lem. \ref{lem:bilinaddtransinvgroup} and (ii) follows from the assumed H\"older properties.
%\end{proof}
%\label{lem:vanisishingseqprederr_groups}
%\end{lem} 
% 
% 
%\begin{lem} For some constant $L^*$ let the target $f$ be $L^*-p$-H\"older continuous up to level $\bar E_h$. 
%%Furthermore, 
%%assume that the observational error is zero, i.e. $\obserrbnd =0$.
%
%If $F_n(x_n) = f(x_n) - \predfn(x_n)$ as well as the reference $\xi_n$ are bounded for all $ n \in \nat_0$ then we have: 
%\[\forall k \in \nat_0: \norm{F_n(\state_{n+k})}_\infty \stackrel{n \to \infty}{\longrightarrow} [0, \frac \hestthresh 2 +  \obserrbnd +2\bar E_h]. \] 
%
%
%\begin{proof} Assume that, for some $q\geq0$, we choose $\hestthresh = 2 \obserrbnd + q$ in our LACKI prediction rule.
%If sequence $\seq{F_n(x_n)}{n\in \nat} $ is bounded then by Thm. \ref{thm:normboundsboundeddisturbmainbody} the error sequence \seq{e_n}{n\in \nat} is bounded. If in addition, the reference is bounded this implies that the sequence $(x_n)$ is bounded, too.
%Furthermore,
%by Lem. \ref{lem:LACKIsampleconsistency}, we know that our predictors $\predfn(\cdot)$ are sample-consistent up to $\frac \lambda 2$ and hence, $\norm{ F_n(x)}_\infty \leq \frac \hestthresh 2 +  \obserrbnd= 2 \obserrbnd + \frac q 2  ,\forall x \in \data_n=\{x_1,...,x_{n-1}\}$.
%The rest follows directly from Thm. \ref{thm:vanisishingseqprederr_LACKI} assuming $\metric_\outspace (f,f') = \norm{f-f'}_\infty$.
%\end{proof}
%\label{lem:innovnorm_convergence}
%\end{lem}

%
%\begin{remark}
%In particular, in case the target is H\"older continuous $(\bar E_h =0)$ and there is no observational error ($\obserrbnd =0$), parameterising our LACKI rule with $\hestthresh =0$ yields vanishing innovations, i.e. 
%\[\forall k \in \nat_0: \norm{F_n(\state_{n+k})}_\infty \stackrel{n \to \infty}{\longrightarrow} 0. \]
%\end{remark}
%
%The next theorem gives a stability guarantee for the tracking error of our LACKI-MRAC controller:

\begin{thm}[Tracking error convergence]
Assume that, for some $q\geq0$, we choose $\hestthresh = 2 \obserrbnd + q$ in our LACKI prediction rule and that the sequence of innovations $\seq{F_n(x_n)}{n\in \nat} $ as well as the reference $\seq{\xi_n}{n \in \nat}$ are bounded. 
If the initial error innovation function is bounded, i.e. if $\exists b \in \Real \forall x: \norm{F_0(x)}_\infty \leq b $, and, if $M$ is a stable matrix, i.e. if $\specrad(M) <1$, then the tracking error converges to the interval $[0,\frac q 2 + 2  \obserrbnd  + 2 \bar E_h]$. That is,
\[\norm{e_n}_\infty \stackrel{n \to \infty}{\longrightarrow} [0,\frac q 2 + 2  \obserrbnd  + 2 \bar E_h]. \]

\end{thm}
\begin{proof} Let $\norm{\cdot} := \norm{\cdot}_\infty$ with accociated matrix norm $\matnorm{\cdot} := \sqrt{d} \specnorm{\cdot}$. 


Let $\epsilon >0$. We desire to show: 
\begin{equation}\label{}
\exists N \in \nat \forall n\geq N: \norm{e_n} \leq \epsilon+\frac q 2 + 2  \obserrbnd  +2 \bar E_h.
\end{equation}

If sequence $\seq{F_n(x_n)}{n\in \nat} $ is bounded then, by Thm. \ref{thm:normboundsboundeddisturbmainbody}, the error sequence \seq{e_n}{n\in \nat} is bounded.  That is, $\exists b \in \Real \forall n: \norm{e_n} \leq \beta$.
Knowing that the error dynamics are bounded by some $\beta \geq 0$ we see that $\matnorm{M^{k}} \, \norm{\vc e_n} \leq \matnorm{M^{k}} \beta \stackrel{k \to \infty}{\longrightarrow} 0$. Here, the convergence to zero follows from the assumption that $M$ is a stable matrix. Hence,
we have:

$$(I)  \, \, \forall n \exists k_0(n) \in \nat \forall k \geq k_0(n): \matnorm{M^{k}} \, \norm{\vc e_n} \leq \frac\epsilon 2. $$


If in addition, the reference is bounded this implies that the sequence $(x_n)$ is bounded, too. Thm. \ref{thm:vanisishingseqprederr_LACKI} implies convergence of the innovations and hence, assuming $\metric_\outspace (f,f') = \norm{f-f'}$, we have:
\begin{equation}\label{eq:Fnconv}
\forall \varepsilon >0 \exists n_0 \forall n \geq n_0 : \norm{F_n(x_n)}\leq  \varepsilon +\frac q 2 + 2  \obserrbnd  +2 \bar E_h.
\end{equation} 


Referring to (i) in Thm. \ref{thm:normboundsboundeddisturbmainbody}, With a change of variables we can follow analogous steps to convert Ineq. (\ref{ineq:errnormbasic}) to state that for all $k \in \nat, n \in \nat_0$ we have: 
\begin{align}
	\norm{\vc e_{n+k}} 	&\leq \matnorm{M^{k}} \, \norm{\vc e_n} + \tinc Q_{n:n+k}	 \sum_{i=0}^{k-1}  \matnorm{M^{k-1-i}} 	\label{ineq:errnormgeneral}
\end{align}
$Q_{n:n+k}:=\max\{\norm{F_n(x_n)},\ldots,\norm{F_{k+n-1}(x_{k+n-1})} \}$. 
With Gelfand's formula and the standard root test for series it is easy to establish convergence of the series: That is, there exists $\sigma \in \Real$ with $\lim_{k \to \infty} \tinc \sum_{i=0}^{k-1}  \matnorm{M^{k-1-i}} = \sigma$. And, we have $\tinc \sum_{i=0}^{k-1}  \matnorm{M^{k-1-i}} \leq \sigma, \forall k$.
Hence,
\begin{equation}
\norm{\vc e_{n+k}} \leq \matnorm{M^{k}} \, \norm{\vc e_n} + \sigma \, Q_{k:n+k}, \forall n \in \nat_0, k \in \nat.
\label{eq:errdyn320894}
\end{equation}


With (\ref{eq:Fnconv}) follows that there exists $n_0 \in \nat_0$ such that we have: $$ (II) \,\,  \forall k \in \nat : Q_{n_0:n_0+k}\leq  \frac{\epsilon}{2 \sigma} +\frac q 2 + 2  \obserrbnd  +2 \bar E_h.
 $$


%

Combining (I) and (II) with Eq. \ref{eq:errdyn320894} allows us to conclude that for any $n \geq N:= n_0 +k_0(n_0)$  we have 
\begin{equation*}
\norm{\vc e_{n}} \leq \frac \epsilon 2 + \sigma \,\frac{\epsilon}{2  \sigma} +\frac q 2 + 2  \obserrbnd  +2 \bar E_h= \epsilon +\frac q 2 + 2  \obserrbnd  +2 \bar E_h. 
\label{eq:errdyn3208942}
\end{equation*}
\end{proof}
Note, since the error converges to a bounded set the state will converge to the target trajectory. So, if the target trajectory is bounded, the continuity of the control law (as a function of state) implies that the control is bounded as well.

%
%
\begin{cor}
In the special case of error-free observations of a H\"older continuous target function, choosing a parameter $\hestthresh =0$ implies:
\[\norm{e_n}_\infty \stackrel{n \to \infty}{\longrightarrow} 0. \]
That is, the error dynamics are globally asymptotically stable with equilibrium point 0.
Furthermore, the control action sequence $\seq{u(x_n)}{n \in \nat}$ converges, provided the reference trajectory $\seq{\xi_n}{n \in \nat}$ is bounded.
\end{cor}

\begin{proof} The stability statement is an immediate consequence of the preceding theorem. 
Remember from Sec. \ref{sec:mrac} that the control action at time $n$ is of the form $u_n := u(x_n) = -\predfn(x_n) - K e_n +c $ for some constant $c$. We show that $(u_n)$ is a Cauchy sequence, provided that the reference sequence $\xi_n$ is. Due to the fact that $\inspace$ is a Hilbert space assumption, this implies the desired convergence result.

So, let $\epsilon >0$. Since $(e_n),(\xi_n)$ converge, also the state sequence $(x_n)$ converges. Hence, all three are convergent Cauchy sequences. In particular, there is $N$ such that for all $n,m >N$: $\norm{e_n-e_m}< \frac{\epsilon} {2 \matnorm{K}}$ and $\norm{x_n-x_m}< \frac{\epsilon} {2\bar L}$. 
Hence, utilising the definition of the control law and the fact that all predictors are H\"older continuous with H\"older constant $\bar L$, for all $m,n >N:$ $\norm{u_n-u_m} \leq \matnorm{K} \norm{e_n -e_m} + \norm{\predfn(x_n) - \predf_m(x_m) } \leq \frac{\epsilon}{2} + \bar L \norm{x_n -x_m} \leq \epsilon $. Therefore, $(u_n)$ is a Cauchy sequence and hence, convergent.

\end{proof}



%================= STABILITY DISCRETE TIME END ============
%\input{content/Ch_kinkyinf/KI_stability_discrtime}

%======================= CONCLUSIONS ===================
\section{Conclusions}
\label{sec:concl}
In this paper, we have introduced \emph{Lazily Adapted Constant Kinky Inference (LACKI)} as method for nonparametric machine learning. Our method was built on the framework of \emph{Kinky Inference} (which in turn is a generalisation of well-known approaches such as \emph{Lipschitz Interpolation} \cite{Sukharev1978,Zabinsky2003,Beliakov2006} and \emph{Nonlinear Set Membership (NSM)}  methods \cite{Milanese2004}). 
 Our approach inherits the numerical simplicity of these methods. On top of this, it can deal with bounded additive observational errors and does not require a priori knowledge about a H\"older constant of the underlying target function--  instead it estimates the constant online from the data. This of course is of great practical interest since this endows LACKI with superior black-box learning capabilities while still allowing us to give theoretical guarantees on learning and control success.
 
To avoid the need to specify the H\"older constant, LACKI adapts the parameter $L(n)$ to reflect a modification of the empirical estimate of the H\"older constant of the underlying target function. 
The adapted parameters were carefully defined to be bounded even if the target function is not H\"older continuous and the data is subject to bounded observational uncertainty.
This allowed us to establish several theoretical guarantees of worst-case consistency. That is, we provided asymptotic guarantees on the ability to learn any H\"older (and non-H\"older) continuous target function as well as convergence rates. Our derivations focussed on worst-case prediction error bounds.

Future work will investigate in how far the bounds can be tightened further, albeit we do not expect that worst-case guarantees could be given that avoid the curse of dimensionality without imposing more confining assumptions on the target functions and the nature of the observational uncertainties. 
However, if we were to shift our attention away from worst-case error analysis under general (possibly systematic) observational uncertainties towards standard mean-square risk analysis and assumptions prevalent in probability theory, we believe less conservative consistency results could be established. 
To this end, we believe it is possible to modify our proofs to translate mean-square consistency derivations for nearest-neighbor regression methods (e.g. as discussed in \cite{Gyoerfi2002}) to our LACKI approach. This might provide a theoretical underpinning for the smoothing properties of our approach observed in the presence of i.i.d. stochastic noise (refer to Fig. \ref{fig:LACKInoise} and Fig. \ref{fig:LACKInoise2}). 

%For instance, we proved that our LACKI rule can learn any H\"older function (up to an error proportional to the noise in the data). Moreover, we showed that LACKI can also learn continuous but non-H\"older target functions up to a worst-case approximation error that converges to the level of intrinsic observational  error in the data-generating process, plus a value coinciding with parameter $\hestthresh \geq 0$. Since 
%$\hestthresh$ is a free parameter that can be set to arbitrarily small values, convergence can be reduced down to the observational noise-level as much as desired. However, while we have not investigated this theoretically, we would expect that reducing the magnitude of $\hestthresh$ will not only cause the uncertainty bounds to grow (or even grow unbounded if the target is not H\"older or there is noise in the data) but also to slow down the worst-case convergence rate of the LACKI predictors. 
%Investigating such convergence rates is a topic we would find interesting to investigate in the context of future work. 


Our learning-theoretic considerations were supplemented by an application of LACKI to 
online learning-based model-reference adaptive control. In a simulated aircraft control problem with nonlinear model uncertainty, we compared our LACKI-based controller against other learning-based methods that were recently proposed in the control literature. Across a range of performance metrics and randomised problem instances, LACKI-MRAC demonstrated consistent and robust performance and outperformed its competitors on the majority of randomised test cases.

For discrete-time systems with additive, bounded, nonlinear uncertainty, we provided theoretical guarantees on the tracking success of our LACKI-MRAC controller. For the online learning case where the LACKI learner was assumed to be continuously updated with the most recently visited state, we proved tracking success up to a term dependent on the observational error. 


In future work, we would like to apply our LACKI learning method to more challenging control tasks that require planning.
To this end, it might be beneficial to link our results to recent work on NSM-based model-predictive control (e.g. \cite{Canale2014}). We believe that the worst-case analysis we focus on in this work is key to establish the necessary links to results in robust MPC.

In this work, we have assumed that the observational noise was bounded; we have addressed the issue of unbounded noise in a companion paper \cite{POKIdraft2016} where the H\"older constant parameter $L(n)$ is found as the minimiser of a prediction loss estimator.  We also believe that these estimators could be used to estimate the noise bound if these are unknown a priori.

A final suggestion for future work pertains to the question of speeding up prediction time. In the context of Lipschitz interpolation, Beliakov \cite{Beliakov2006} proposed a way to organise the sample in a tree-structure (in lieu to KD-trees utilised in nearest-neighbor search) in order to reduce the linear prediction time to be logarithmic in the sample size (albeit we would think this would hold in expectation only). While applicable to our LACKI approach in the batch learning setting, it is not clear to us how this tree structure could be efficiently updated in an online learning setting. Future work could explore avenues of connecting his idea of appealing to notions of generalised nearest-neighbor search to existing efficient approaches of \emph{online} nearest neighbor search.

%In the present paper, our theoretical considerations relied on worst-case analysis. On the one hand this is more appropriate than traditional stochastic risk analysis of nonparametric regression if the learning method is to be used in robust control tasks where common 
%distributional assumptions will not hold and guarantees have to be valid even in extreme events of zero measure. 
%
%On the other hand, our learning guarantees are unable to guarantee the reduction of the approximation error of the predictor to the target below the level of observational noise. In the presence of systematic observational errors this is unavoidable. However, things might change if the observational errors are stochastic.
%For example, in Fig. \ref{fig:LACKInoise} and Fig. \ref{fig:LACKInoise2} we observed that our predictors were capable of smoothing out stochastic noise resulting in predictors that exhibited close alignment with the true target. Investigating the extent to which distributional assumptions about the noise can be translated to probabilistic convergence results to the target will also be a subject of future investigation. 
%
%======================= CONCLUSIONS END ===============
%\input{content/conclusions}

\section{Acknowldegements}
I am grateful for useful feedback from Jan Maciejowski, Carl Rasmussen and Stephen Roberts. I would also like to thank Girish Chowdhary and Hassan Kingravi who generously supplied me with their code that allowed me to most closely reproduce their work and use it for my comparisons in Sec. \ref{sec:KIMRAC}. I also gratefully acknowledge funding via the AIS project, NMZR/031 RG64733.
%\newpage
\bibliographystyle{plain}
\bibliography{content/lit}
\appendix 
\section{Supplementaries}
%\section{Preliminaries}
\input{content/hoelder_BG}
%\input{content/Ch_kinkyinf/constantadaptation}
%\input{content/group_learners}




==> hoelder_BG.tex <==
\subsection{H\"older and Lipschitz continuity for inference}%\label{sec:HoeldNLipfacts}
\label{sec:Hoelder_brief}
\subsubsection{Introduction and related work}



H\"older continuous functions are uniformly continuous functions that may exhibit infinitely many points of non-differentiability and yet are sufficiently regular to facilitate inference. That is, they have properties that make it possible to make assertions of global properties on the basis of a finite function sample. 

H\"older continuity is a generalisation of Lipschitz continuity.  Lipschitz properties are widely used in applied mathematics to establish error bounds and, among many other, find application in optimisation \cite{Shubert:72,direct:93} and quadrature \cite{Baran2008,curbera1998,dereich2006} and are a key property to establish convergence properties of approximation rules in (stochastic) differential equations \cite{kloedenandplaten1992,Gardiner2009}. 
Furthermore, most machine learning methods for function interpolation seem to impose smoothness (and thereby, H\"older continuity) on the function. For instance, with our Lem. \ref{lem:Hoeldarithmetic} derived below, it would be possible to show that any finite \textit{radial basis function neural network} \cite{Broomhead1988} with a smooth basis function is H\"older continuous on a compact domain. Or, a \textit{Gaussian process} with a smooth covariance function also has a smooth mean function and a.s. smooth sample paths  \cite{GPbook:2006,grimmetbook2001}. Therefore, posterior inference over functions on compact support made with such a Gaussian process on the basis of a finite sample is H\"older continuous. 


Recently, we have become aware of related work published in mathematical and operations research journals \cite{Cooper2006,Cooper1995,Zabinsky2003,Beliakov2006,Beliakovsmoothing2007}. For instance, Zabinsky et. al. \cite{Zabinsky2003} consider the problem of estimating a one-dimensional Lipschitz function (with respect to the canonical norm-induced metric). Similar to the analysis we employ to establish our guarantees, they use a pair of bounding functions and make predictions by taking the average of these functions. While we have developed our kinky inference rule independently, it can be seen as a generalisation of their approach. Our method provides extensions to H\"older continuous multi-output functions over general, multi-dimensional (pseudo-) metric spaces, can cope with with erroneous observations and inputs, can fold in additional knowledge about boundedness, learn parameters from data and provides different guarantees such as (uniform) convergence of the prediction uncertainty. 
As part of the analysis of our method, we construct delimiting functions we refer to as \textit{ceiling} and \textit{floor} functions. The construction of similar functions is a recurring theme that, in the standard Lipschitz context, can be found in global  optimisation \cite{Shubert:72}, quadrature \cite{Baran2008}, interpolation \cite{Beliakov2006,Beliakovsmoothing2007}, as well as in the analysis of linear splines for function estimation \cite{Cooper1995}. Cooper \cite{Cooper2006,Cooper1995} utilises such upper and lower bound functions in a multi-dimensional setting to derive probabilistic PAC-type error bounds \cite{Valiant1984} for a linear interpolation rule. He assumes the data is sampled uniformly at random on a hypercube domain. This precludes the application of his results to much of our control applications where the data normally is collected along continuous trajectories visited by a controlled plant. Our inference rule is different from his and our guarantees do not rely on distributional assumptions. This of course is important in control settings where the common assumption that the input data was drawn independently from a fixed distribution typically is not met.
%As a special case of our kinky inference framework, we consider a case, called \textit{kNN-KI}. Here, the inference over function values is based on up to (approximate) k nearest neighbours aiming to reduce computational prediction effort to log-time. Approaches to this end include maintaining a data structure for fast nearest neighbour search \cite{Bentleykdtree:1975} or utilising locally sensitive hash functions \cite{RusselNorvigbook2009}. 
In this thread of works, perhaps the work that is most closely related to ours is the function interpolation method of Beliakov \cite{Beliakov2006} that is a special case of a kinky inference rule: For a single-output function that is Lipschitz with respect to a special input space norm and where the data is error-free, the authour provides an algorithm that promises logarithmic prediction time. Unfortunately, many of his assumptions are unrealistic in a control setting. And, the improved prediction time is achieved by constructing a data structure from batch data which precludes its use in an online learning setting. However, future work might explore in how far his ideas can be 
converted into an online learning rule. Furthermore, in learning situations where Beliakov's interpolation method is applicable, our theoretical results extend to his work. For instance, our results show how Lipschitz constant estimation can be harnessed to render his approach a universal approximator.

Other work of relevance can be found in analysis. For instance, Miculescu \cite{Miculescu2000} presents work proving that any continuous function on a metric space is a uniform limit of a sequence of \emph{locally} Lipschitz functions and also mentions that the stronger statement, that every function is a limit of a sequence of globally Lipschitz functions, is not true in general. However, he cites earlier work \cite{Georganopoulos1967} that does show that every real-valued continuous function on \emph{compact} domain is a uniform limit of a sequence of Lipschitz functions. In some sense, our work develops a related statement as a by-product. 
From our convergence guarantee of the LACKI rule, we have derived constructive method for showing 
that any continuous function on compact domain is the uniform limit of a sequence of H\"older functions up to an arbitrarily small error.

Finally, in the context of control, Milanese and Novara \cite{Milanese2004} considered NSM methods for interpolation. For a fixed Lipschitz constant, their prediction rule can be
seen as a special case of ours without the $\lbf$ and $\ubf$ parameters and with special choices of metrics. Similar to us, they do consider the problem of estimating the Lipschitz constant from the data and consider bounded noise. However, they obtain the Lipschitz constant estimate via the maximum partial derivative of an arbitrarily chosen fitted parametric model of a bounded input set. And, they give no guarantees on the quality of the resulting estimator that is fitted to the data like this nor do they discuss the impact of the choice of parametric model or the fitting method on the quality of the estimator.
 
%\jcom{Need to read \cite{Georganopoulos1967}}
%\jcom{Need to reassess the following in the light of the newly found control paper:}
%None of the aforementioned works seems to consider interval-bounded input uncertainty and observational errors, fold in additional knowledge such as boundedness or considers inference over multi-output functions as we do. Most importantly the combination with our online constant estimation rule, leading to our LACKI inference rule, as well as our universal approximation guarantees are novel.
%Finally, we are not aware of any work that employs H\"older-based methods in the context of model-reference adaptive control. 


%In particular, we will look into the inference problems of bounded optimisation and quadrature. That is, based on the knowledge of a sample of a H\"older continuous function we will derive upper and lower bounds on its maximum, minimum and definite Riemann integral. In addition we will touch upon adaptive algorithms that can utilise knowledge of the function's H\"older properties to guide exploration. That is, since the regularity of the function allows us to provide interval bounds on the uncertainty of the function, the magnitude of the uncertainty can be a guide to identify regions that are to be sampled next in order to maximise the shrinkage of the provided error bounds. 
%\jcom{The latter is more the 1-dim case, which I may or may not include}\\

\subsubsection{Basic facts and derivations}
In preparation of subsequent parts of the work that take advantage of H\"older properties this section will proceed to establish essential prerequisites.
The remainder of this section is structured as follows: Firstly, we will go over basic definitions and engage in some preliminary derivations that will be of importance throughout this work.
While we do not claim novelty on any of the results we provide proofs for in this section, we had not found them in the literature and hence, had to derive them on our own.

Firstly, we commence with introducing the notions of (pseudo-) metric spaces.

\begin{defn}[(Pseudo-) metrics]
Let $\inspace$ be a set. A mapping $\metric_\inspace: \inspace^2 \to \Real$ is called a \emph{pseudo-metric} if it positive ($\forall x,x' \in \inspace: \metric_\inspace(x,x') \geq 0$) and satisfies the triangle inequality ($\forall x,x',x'' \in \inspace: \metric(x,x') \leq \metric_\inspace(x,x'') + \metric (x'',x')$). If furthermore the pseudo-metric $\metric$ is definite $(i.e. \forall x,x' \in \inspace_\inspace: \metric_\inspace(x,x') =0 \Leftrightarrow x=x')$ then 
the mapping $\metric$ is called a \emph{metric}. The set $\inspace$ endowed with a (pseudo-) metric $\metric_\inspace: \inspace^2 \to \Real$ or the pair $(\inspace, \metric_\inspace)$ are called \emph{(pseudo-) metric space}.
 \end{defn}

\begin{defn} 
Let $(\inspace ,\metric_\inspace ), (\outspace , \metric_\outspace )$ be two (pseudo-) metric spaces and 
$I \subset \inspace$ be an open set. A function $f: \inspace \to \outspace $ is called (L-p-) \emph{H\"older} 
(continuous) on $I \subset \inspace$ if there exists a \emph{(H\"older) constant} $L \geq 0$ and \emph{(H\"older) 
exponent} $p\geq 0$ such that 
\[\forall x,x' \in I : \metric_\outspace \bigl(f(x),f(x')\bigr) \leq L \, \bigl( \metric_\inspace (x,x') \bigr)^p. \]
We denote the space of all L-p- H\"older functions by $\hoelset{L}{}{p}$.
\end{defn}

H\"older functions are known to be uniformly continuous. 
A special case of importance is the class of $L$-\textit{Lipschitz} functions. These are H\"older continuous 
functions with exponent $p=1$. In this context, coefficient $L$ is referred to as\textit{ Lipschitz constant} or \textit{Lipschitz number}.

\begin{ex}[Square root function]\label{ex:sqrtfctHoelder}
As an example of a H\"older function that is not Lipschitz we can consider $x \mapsto \sqrt x$ on domain $I = [0+\epsilon,c]$ where 
$c >\epsilon \geq 0 $. For $\epsilon >0 $ the function is Lipschitz with $L = \sup_{x \in I} \frac{1} {2 \sqrt{x}}$. We can see that the 
coefficient grows infinitely large as $\epsilon \to 0$. By contrast, the function is H\"older continuous 
with H\"older coefficient $L=1$ and exponent $p=\frac 1 2 $ for any bounded $I \subset \Real$.
We can see this as follows: Let $\epsilon =0,$ $x,y \in I$ and, without loss of generality,  $y \geq x$. Let $\xi := \sqrt{x}, \gamma := \sqrt{y}$ and thus, $\gamma \geq \xi$. We have:
$\xi \leq \gamma $ $\Leftrightarrow 2 \xi^2 \leq 2\xi\gamma$ $\Leftrightarrow \gamma^2 - 2 \xi\gamma + \xi^2  \leq \gamma^2 - \xi^2$ $\Leftrightarrow (\gamma-\xi)^2  \leq \gamma^2-\xi^2$ $\Leftrightarrow \abs{\gamma-\xi}^2  \leq \abs{\gamma^2-\xi^2}$
$\Leftrightarrow \abs{\gamma-\xi}  \leq \sqrt{\abs{\gamma^2-\xi^2}}$  $\Leftrightarrow \abs{\sqrt{x}-\sqrt{y}} \leq \abs{y-x}^{\frac{1}{2}}$. Since, $x,y$ were chosen arbitrarily, we have shown H\"older continuity as desired.
\end{ex}

Most commonly, one considers H\"older continuity for the special case of the standard metric induced by a norm, i.e.  $\metric(x,x') = \norm{x-x'}$.
For a function $f: \inspace \to \outspace$, the H\"older condition becomes:
\[\forall x,x' \in I : \norm{f(x)-f(x')}_\outspace \leq L \, \norm{x-x'}_\inspace^p. \]

Similarly, we can consider H\"older continuity for each output component: 

\begin{defn} \label{def:outputwisehoelder}
Let $\outspace \subseteq \Real^m $ and $\inspace$ be a space endowed with a metric (or indeed a semi-metric) $\metric_\inspace$. Then, the function $f: \inspace \to \outspace$ is output-component-wise H\"older continuous with exponent $p$ and constant $L \in \Real^m_{\geq 0}$ if $f \in \hoelset L { } p$ where
$\hoelset L {\metric_\inspace} p:= \bigl\{ \phi: \inspace \to \outspace \,\ | \, \forall j \in \{1,...,m \}, \forall x,x' \in \inspace: \abs{\phi_j(x) - \phi_j(x')} \leq L_j \metric^p_\inspace(x,x') \bigr\}$
is the set of all functions whose component functions are H\"older continuous with respect to input space metric $\metric_\inspace$ and an output space metric that is induced by the canonical norm $\metric_{\outspace} (x,x')= \abs{x-x'}$.  
\end{defn}

\begin{remark}[Best H\"older constant]
Note for $p \in (0,1], 0 \leq L_1 \leq L_2$ we have $\hoelset {L_1} {\metric_\inspace} p \subseteq \hoelset {L_2} { } p$. The smallest $L^* \geq 0$ such that function if is $L^*-p-$ H\"older, $f \in \hoelset {L^*} {\metric_\inspace} p$, is called the \emph{best} H\"older constant of $f$.
\end{remark}

Generally, it is obviously true that $\hoelset{L}{}{p} \subseteq \hoelset{L'}{}{p}$ for $L' \geq L$.
With regard to the H\"older exponent, we will now show that smaller exponents are less restrictive than larger ones. 




\begin{lem} \label{lem:hoeldexpprop2}
Let $\inspace$ be the input space (not necessarily bounded). For some $p \in (0,1], L \geq 0$ assume that  and $f:\inspace \to \outspace$ is locally $L-p$-H\"older continuous.
Then we have: (i) for any $ q \in (0,p]$, f is also locally $L-q$-H\"older. 
(ii) If $f:\inspace \to \outspace$ is bounded with $\sup_{x,x' \in \inspace} \metric_\outspace (f(x),f(x')) \leq B \in \Real$ and globally $L-p$ H\"older then $f$ is globally $L^*-q$-H\"older, where $L^* := \max\{L,B \}$ and $q \in (0,p]$. In particular, on compact support, Lipschitz continuity entails \emph{H\"older} continuity for any H\"older exponent $p \in [0,1)$.
\begin{proof}
(i) Let $p \in (0,1], f \in \hoelset L { } p $ and $p = q+r, r \in [0,1)$. Let $\xi \in \inspace$ and $I$ denote the intersection of the domain with an $\epsilon$-ball around $\xi$ such that $f$ satisfies the H\"older condition on $I$ and such that $\sup_{x,x' \in I} \metric_\inspace(x,x') \leq 1$.  For all $x,x' \in I$ we have $\metric_\outspace (f(x),f(x')) \leq L\metric_\inspace^p (x,x') = L \metric_\inspace^q(x,x') \metric_\inspace^r(x,x') \leq L \metric_\inspace^q(x,x')$ where the last inequality holds since $r \in [0,1)$ and $\sup_{x,x' \in I} \metric_\inspace(x,x') \leq 1$.

(ii) Let $x,x' \in \inspace$. If $\metric_\inspace(x,x') \leq 1$ we can show $\metric_\outspace (f(x),f(x'))  \leq L \metric_\inspace^q(x,x')$ following through the same sequence of inequalities as above in the proof of (i). Now, let $\metric(x',x) >1$. We have $\metric_\outspace (f(x),f(x')) \leq B \leq B  \metric_\inspace(x,x')^q$.
\end{proof}
\end{lem}

%Note for compact domains local H\"older continuity implies global H\"older continuity with the same parameters. Therefore Lem. \ref{lem:hoeldexpprop1} would also be implied 
%by Lem. \ref{lem:hoeldexpprop2}.(i) in cases where $\inspace$ is compact.



%We conclude this section by the following theorem stating that any concatenation of H\"older continuous functions is H\"older continuous:
%
%\begin{thm} \label{thm:concathoelder}
%Let $(\statespace, \metric)$ be a metric space and $f,g : \statespace \to \statespace$ be two H\"older continuous mappings with H\"older constants $L_f, L_g$ and H\"older exponents $p_f,p_g$, respectively.
%Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also H\"older continuous with H\"older constant $L_h:= L_f L_g^{p_f}$ and exponent $p_h:=p_g \, p_f$.
%That is, 
%\[\forall \state,\state' \in \statespace: \metric\bigl(h(\state),h(\state')\bigr) \leq L_h \bigl(\metric(\state,\state')\bigr)^{p_h}.\]
%\begin{proof}
%%\begin{align}
%$\metric\bigl(f \circ g(\state),f\circ g(\state')\bigr) \leq L_f  \Bigl(\metric(g(\state),g(\state'))\Bigr)^{p_f}$
%$\leq L_f  \Bigl(L_g \metric(\state,\state')^{p_g}\Bigr)^{p_f}$ $= L_f L_g^{p_f}   \Bigl(\metric(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using H\"older continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
%
%\end{proof}
%\end{thm} 
%In conjunction with H\"older properties of the square root function established in Ex. \ref{ex:sqrtfctHoelder}, Thm. 
%\ref{thm:concathoelder} immediately yields the following result:
%\begin{cor}
%If $f: \statespace \to \statespace $ is H\"older continuous with constant $L_f$ and exponent $p_f$ then $\sqrt{f}$ also is Hoelder, having  H\"older constant $\sqrt{L_f}$ and exponent $p_f$.
%\end{cor}


\begin{thm} \label{thm:hoelderconcat}
Let $(\statespace, \d)$ be a metric space and $f,g : \statespace \to \statespace$ be two H\"older continuous mappings with H\"older constants $L(f), L(g)$ and H\"older exponents $p_f,p_g$, respectively.
Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also H\"older continuous with H\"older constant $L(h):= L(f) L(g)^{p_f}$ and exponent $p_h:=p_g \, p_f$.
That is, 
\[\forall \state,\state' \in \statespace: \d\bigl(h(\state),h(\state')\bigr) \leq L(h) \, \bigl(\d(\state,\state')\bigr)^{p_h}.\]
\begin{proof}
%\begin{align}
$\d\bigl(f \circ g(\state),f\circ g(\state')\bigr)$ $\leq L(f)\,  \Bigl(\d(g(\state),g(\state'))\Bigr)^{p_f}$
$\leq L(f)\,  \Bigl(L(g)\, \d(\state,\state')^{p_g}\Bigr)^{p_f}$ 

$= L(f)\, L(g)\,^{p_f}   \Bigl(\d(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using H\"older-continuity of $f$ and in the second, we were using H\"older continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
\end{proof}
\end{thm} 






%A special case of H\"older continuity is Lipschitz continuity. A Lipschitz continuous function is H\"older continuous with exponent 1.
%If the metric space is $(\Real,(x,y) \mapsto \abs{x-y})$, $f$ is Lipschitz with constant $L(f)$ if $\forall t,t': \abs{f(t)-f(t')} \leq L(f) \, \abs{t-t'}$. 

Several numerical methods, such as Lipschitz optimisation \cite{Shubert:72}, rely on the knowledge of a Lipschitz constant. In the more general case of H\"older continuous functions this will correspond to the need of knowing a H\"older constant and exponent. To avoid having to derive these for each new function from first principles, we establish the following collection of facts that allows us determine bounds on H\"older constants of combinations of functions with known H\"older parameters.
While we provide proofs for a restatement in the H\"older continuous setting, a number of the following statements have also been proven in \cite{Weaver1999} in the context of Lipschitz algebras.





\begin{lem}[H\"older arithmetic] \label{lem:Hoeldarithmetic}
Let, $I,J \subset \inspace$ where $\inspace$ is a metric space endowed with metric $\metric$. Let $f : \inspace \to \Real$ be H\"older on $I$ with constant $L_I (f) \in \Real_+$ 
and $g :\inspace \to \Real$ be H\"older on $J$ with constant $L_J (g) \in \Real_+$. Assume both functions have the same H\"older exponent $p \in (0,1]$. That is, $\forall x, x' \in \inspace: \abs{f(x)-f(x')} \leq L(f) \metric(x,x')^p$ and  $\forall x, x' \in \inspace: \abs{g(x)-g(x')} \leq L(g)  \metric(x,x')^p$.
We have:

\begin{enumerate}
	\item Mapping $x \mapsto |f(x)|$ is H\"older on $I$ with constant $L_I(f)$ and exponent $p_f$.
	\item If $g$ is H\"older on all of $J=f(I)$ the concatenation $g \circ f: t \mapsto g(f(t))$ is H\"older on $I$ with constant 
	      $L_I(g \circ f) \leq$ $L_J (g) \, L_I^p(f)$ and exponent $p^2$.
	\item Let $r \in \Real$. $r \, f: x \mapsto r \, f(x)$ is H\"older on $I$ having a constant $L_I (r \,f) = |r| \, L_I(f)$.
	\item $f+g: x \mapsto f(x) + g(x)$ has H\"older constant at most $L_I(f) + L_J(g)$.
	\item Let $m_f = \sup_{x\in \inspace } f(x)$ and $m_g = \sup_{x \in \inspace } g(x)$. Product function $f\cdot g: x \mapsto f(x) \, g(x)$ has H\"older exponent $p$ and a H\"older constant on $I$ which is at most $(m_f \, L_J(g)+ m_g \, L_I(f))$.
	%\item Let $\tilde h(x) = \min\{f(x),g(x) \}$, $h(x) = \max\{f(x), g(x) \}, \forall x \in \inspace  \cap J$. We have $L_{I \cap J}(h) \leq \max\{L_I(f),L_J(g)\}$ and $L_{I \cap J}(\tilde h) \leq \max\{L_I(f),L_J(g)\}$.	
	\item For some countable index set $\indsett$, let the sequence of functions $f_i$ be H\"older with exponent $p$ and constant $L(f_i)$ each. Furthermore, let $H(x) =\sup_{i \in \indsett} f_i(x) $ and $h(x) := \inf_{i \in \indsett} f_i(x)$ be finite for all $x$. Then $H,h$ are also H\"older with exponent $p$ and have a H\"older constant which is at most $\sup_{i \in \indsett} L(f_i)$.
	\item Let $b := \inf_{x \in \inspace }| f(x)| > 0$ and let 
	$\phi(x) = \frac{1}{f(x)}, \forall x \in \inspace$ be well-defined.  
	      Then $L_I(\phi) \leq b^{-2} \, L_I(f)$.  
	\item Let $p=1$ (that is we consider the Lipschitz case), let $I$ be convex and $\metric(x,x') = \norm{x-x'}$ where $\norm{\cdot}$ is a norm that induces a sub-multiplicative matrix norm (e.g. all $p-$ norms are valid). $f$ cont. differentiable on I $\Rightarrow$ $L_I(f) \leq \sup_{x \in I } \norm{\nabla f(x)}. $ 
	For one-dimensional input space, $\inspace = \Real$, $L_I(f) = \sup_{x \in I } \abs{\nabla f(x)}$ is the smallest Lipschitz number. 
	 \item Let $c \in \Real$, $f( t) = c, \forall x \in I $. Then $f$ is H\"older continuous with constant $L_I(f) =0$ and for any coefficient $p_f \in \Real$.  
	\item $L_I(f^2) \leq 2 \, L_I(f)\, \sup_{t \in I} f\,$.
	\item With conditions as in 8), and input space dimension one, we have $\forall q \in \mathbb Q : L_I(f^q) = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $.
\end{enumerate}
\begin{proof}

\textbf{1)}  We show $|f|$ has the same constant and exponent as $f$. Let $X,X' \in \inspace $ arbitrary. 
We enter a case differentiation:

\textit{1st case: $f(x), f(x') \geq 0$}. 

Hence, $\bigl| \abs{f(x)}- \abs{f(x')} \bigr| = \bigl| f(x) - f(x') \bigr|  \stackrel{f \,Hoelder}{\leq} L_I(f) \metric(x,x')^{p}$.\\

\textit{2nd case: $f(x) \geq 0, f(x') \leq 0$.} 

Note, $|y| = - y$, iff $y \leq 0$. Hence,  $\bigl| |f(x)| - |f(x')| \bigr| \leq \bigl| |f(x)| + |f(x')| \bigr| $
$= \bigl| |f(x)| - f(x') \bigr|  =  \bigl| f(x) - f(x') \bigr| \leq L_I(f) \, \metric(x,x')^{p}$.\\

\textit{3rd case: $f(x) \leq 0, f(x') \geq 0$.} Completely analogous to the second case.\\

\textit{4th case: $f(x), f(x') \leq 0$}. 

$\bigl| |f(x)| - |f(x')| \bigr| = \bigl| f(x') - f(x) \bigr|= \bigl| f(x) - f(x') \bigr|  \stackrel{f \, Hoelder}{\leq} L_I(f) \metric(x,x')^{p}$.\\

The remaining points are also proven in \cite{Weaver1999} in the context of Lipschitz functions.

\textbf{2)} Special case of Thm. \ref{thm:hoelderconcat}.
% For arbitrary $t,t' \in \indset $ we have:
%
%$\bigl| g(f(t)) - g(f(t'))| \bigr| \leq L_J(g) \, |f(t) - f(t') | \leq L_J(g) \, L_I(f)\, |t-t'|$ 
%where the two inequalities are due to the Lipschitz properties of $g$ and $f$, respectively.\\

\textbf{3)}  For arbitrary $x,x' \in \inspace , r \in \Real$ we have:

$\bigl| r \, f(x) - r \, f(x')| \bigr| = |r|\, |f(x) - f(x')| \leq |r| \,L_I(f)\,  \metric(x,x')^{p}$.\\ 

\textbf{4)}  For arbitrary $x,x' \in \inspace , r \in \Real$ we have:

$\bigl| g(x) + f(x) - (g(x') + f(x'))| \bigr| = \bigl| g(x)  - g(x') + f(x)- f(x')| \bigr|$ 
$\leq \bigl| g(x)  - g(x')\bigr|  + \bigl| f(x)- f(x')| \bigr|$ $\leq (L_J(g)+L_I(f))\,  \metric(x,x')^{p}$.\\

\textbf{5)}  Let  $x,x' \in \inspace $, $d := f(t) - f(t')$.

$\bigl| g(x) f(x) - g(x')  f(x') \bigr| = \bigl| g(x) (f(x') +d) - g(x') f(x') \bigr|$ 
$= \bigl|\bigl( g(x) - g(x') \bigl)  f(x')+ g(x)  d \bigr|  $

$\leq \bigl| g(x) - g(x') \bigr|  |f(x')|   + \bigl|g(x)\bigr| \,  |d|  $
$\leq L_I(g) \metric(x,x')^p  |f(x')|   + \bigl|g(x)\bigr| \,  L_I(f) \metric(x,x')^p  $

$\leq L_I(g) \metric(x,x')^p  \sup_{x' \in \inspace } \{|f(x')|\}  \\ + \sup_{x \in \inspace }\{\bigl|g(x)\bigr|\} \,  L_I(f) \metric(x,x')^p  $

$= \Bigl(L_I(g)  \sup_{x' \in \inspace } \{|f(x')|\}   \\+ \sup_{x \in \inspace }\{\bigl|g(x)\bigr|\} \,  L_I(f)\Bigl) \metric(x,x')^p  $.\\

\textbf{6)}  The proof of Proposition 1.5.5 in \cite{Weaver1999} proves our statement if one replaces their 
metric $\rho$ by $\metric^p$.

\textbf{7)}  Let  $x,x' \in \inspace $.
$\bigl| \frac{1}{f(x)} - \frac{1}{f(x')} \bigr|$ 
$=\bigl| \frac{f(x')}{f(x') f(x)} -\frac{f(x)}{f(x') f(x)} \bigr|$ 
$= \frac{\bigl|f(x')-f(x) \bigr|}{\bigl|f(x')\bigr| \bigr| f(x)\bigr|}$ 
$\leq \frac{L_I(f) \metric(x,x')^p}{\inf_{x \in \inspace } |f(x)|^2}$.\\

\textbf{8)} Let $p=1$ and $\metric(x,x') = \norm{x-x'}$ be a norm that induces a sub-multiplicative matrix norm. Define $\ell := \sup_{x \in I } \norm{ \nabla f(x) } = L_I(f)$. 
Firstly, we show that it is a Lipschitz constant: Let $x,x' \in I $ and 
$\overline{xx'} := \{tx + (1-t) x' \, | \, t \in [0,1]\}$. 
%$\overline{xx'} := \{y | \exists t \in [0,1] : y = tx + (1-t) x'\}$. 
Owing to convexity of I, $\overline{xx'} \subset I$. Due to the mean value theorem $\exists \xi \in \overline{xx'} \subset I: |f(x) - f(x')|=  T_\xi (x-x')$. where $T_\xi (x) = \SP{\nabla f(\xi)}{ x}$ is a linear OP. Assuming the derivative of $f$ is bounded, $T_\xi$ is a bounded OP and we have $\abs{T_\xi (x-x') } \leq \matnorm{T_\xi} \norm{x-x'}$ where 
$\matnorm{T_\xi} = \sup_{\norm{x} = 1} \abs{\SP{\nabla f(\xi)}{x}} \leq \norm{\nabla f(\xi)}$. In conjunction,
$|f(x) - f(x')| \leq \norm{\nabla f(\xi)} \norm{x-x'}$. 

Secondly, we show that $\ell$ is the smallest Lipschitz constant in the one-dimensional case: Let $\bar \ell$ be another Lipschitz constant on $I$ such that $\bar \ell \leq \ell$. Of course, here $\norm{\cdot} = \abs{\cdot}$. Since $I$ is compact and $\norm{\nabla f(\cdot) }$ is continuous, there is some $\xi \in I$ such that $\norm{\nabla f(\xi)} = \sup_{x \in I} \norm{\nabla f(\xi)} = \ell$. Pick any sequence $(y_k)_{k=1}^\infty$ contained in $I$ such that $y_k \stackrel{k \to \infty}{\longrightarrow} \xi$ and $y_k \neq \xi$.
$\forall k: y_k \in I $ and $\bar \ell$ is a Lipschitz constant on $I$. Hence, $ \bar \ell \geq \frac{|f(y_k) - f(\xi)|}{\norm{y_k-\xi}}\stackrel{k \to \infty}{\longrightarrow} \norm{ \nabla f(\xi)} = \ell$. Thus, $\bar \ell = \ell$.

\textbf{9)} Trivial. 

\textbf{10)} Special case of property 5).

\textbf{11)} $L(f^q) \stackrel{8)}{=} \sup_{\tau \in \indset } |\dif{}{t} f^q(\tau)| = |q| \,\sup_{\tau \in \indset } |f^{q-1}(\tau) \, \dot f(\tau)| $. 
\end{proof}
\end{lem} 

As a simple illustration, assume we desire to establish that $f(t) = \max\{ 1- 3 \sin(t), \exp\bigl(- \sin(t) \bigr)\}$ is Lipschitz and to find a Lipschitz number on $\Real$. Application of 8. shows that $t \mapsto \sin(t)$ and $t \mapsto \exp(- t)$ have a Lipschitz number of $1$. Application, of 2., 9. 1. and 6. then show that $L(f) =3$ is a Lipschitz number of $f$.


%As another example we consider the standard deviation of the Ornstein-Uhlenbeck process:
%\begin{ex} \label{ex:hoelderOUstd}
%Consider the function $h(t) = f \circ g(t)$ where $f(\cdot) = \sqrt \cdot$ is the square root function and $g(t) = \frac{B^2}{2 K} (1- \fexp{-2Kt}) $, $K >0$. $g$ is the non-stationary factor of the variance trajectory of an Ornstein-Uhlenbeck process (cf. Sec. \ref{sec:OUprocess}). We show that $h$ is H\"older and has constant $L(h)= \sqrt{2K}$ and H\"older exponent $p_h = \frac 1 2$. This can be easily done by applying Lem. \ref{lem:Hoeldarithmetic}.8 to show that $L(g)$ is Lipschitz with constant $L(g) = B^2 $ and then combining the H\"older constant and exponent derived in Ex. \ref{ex:sqrtfctHoelder} with Thm. \ref{thm:hoelderconcat} to yield the H\"older exponent $p_h = p_g p_f = \frac 1 2$ and constant $L(h) = 1 \sqrt{L(g)}  = \abs B$.  
%\end{ex}

%An example important to our considerations above is the establishment of Lipschitz bounds of an RBFN:
%\begin{ex} \label{ex:hoelderRBFN}

%\end{ex}

\subsection{H\"older continuity of the exponentiated map }

 %
The main objective of this subsection is to show that, for each $s \in \inspace$, the function $\phi_s: x \mapsto L \metric(x,s)^p$ is H\"older continuous with coefficient $L$ and exponent $p$ with respect to (pseudo-) metric $\metric: \inspace^2 \to \Real$. This is important in our derivations since these maps are essential building blocks of the kinky inference procedure. Therefore it is easy to employ Lem. \ref{lem:Hoeldarithmetic} to show that the full kinky inference rule is H\"older continuous.

To establish the H\"older regularity result, we will first show that $(x,y) \mapsto \metric(x,y)^p$, for $p \in (0,1] $, is a metric.  This can be utilised to show that
$\phi_s \in \hoelset L \metric p$.




Before proceeding we need to establish a few facts. 
Firstly, we remind ourselves of the following well-known fact:
\begin{lem} \label{lem:pd_n_concave_subadditive}
A nonnegative, concave function $g:\Real_{\geq 0} \to \Real$ with $g(0) = 0$ is subadditive. 
That is, $\forall x,y \in \Real_{\geq 0}: g(x+y) \leq g(x) + g(y)$. 
 \begin{proof}
If $x = y = 0$ then subadditivity trivally holds:  $0=g(x+y) \leq g(x) + g(y) = 0$.
So, let $x, y \in \Real_+$ such that $x >0 \vee y >0$.
We have, $g( x +y) = \frac{x}{x+y} g(x+y) + \frac{y}{x+y} g(x+y) \leq g(\frac{x}{x+y} (x+y) ) +  g(\frac{y}{x+y}(x+y)) = g(x) + g(y)$.
Taking into account that $\frac{x}{x+y}, \frac{x}{x+y} \in [0,1]$, the last inequality can be seen as follows:

 Since $g$ is concave we have 
$\forall p \in [0,1], x \in \Real: g(p x) =  g(px + (1-p) 0) \geq p g(x) + (1-p) g(0) \geq p g(x)  $. The last inequality follows from $g(0) \geq 0$.
\end{proof}
\end{lem}

\begin{lem} \label{lem:x2p_pdNsubadd}
 Let $h: \begin{cases} \Real_{\geq 0} \to \Real_{\geq 0},\\ \, x \mapsto x^p\end{cases}$, for $p \in (0,1] $. $h$ is positive definite and subadditive. 
 That is, (i) $h(0) = 0 $ and  $h(x) > 0, \forall x \neq 0$ and (ii) $\forall x,y \in \Real_{\geq 0}: h(x+y) \leq h(x) + h(y)  $.
 Moreover, $h$ is concave. If $p \in (0,1)$, h is strictly concave. 
 
\begin{proof}
\textit{Pos. def. :} $h(0) = 0$.  Also $\lim_{x \to 0_+} h(x) =0$. Since $\nabla h (x) = p h^{p-1}(x) >0 $ for $x >0$, $h$ is strictly monotonically increasing on $\Real_+$. Hence, $h(x) > 0, \forall x >0$. 

\textit{Concavity:} If $p =1$, $h$ is linear and hence, concave. If $p \in (0,1)$, $\nabla^2 h(x) = p (p-1) h(x)^{p-2} > 0$ regardless of $x$.

\textit{Subadditivity:} Follows directly with Lem. \ref{lem:pd_n_concave_subadditive} on the basis of established positive definiteness and concavity.
  %
\end{proof}
\end{lem}



\begin{lem}\label{lem:hoeldererror_metric}
Let $p \in (0,1]$.
With definitions as above, we assume that set $\inspace$ is endowed with a pseudo- metric $\metric$. Function
$\metricp: \begin{cases} \inspace \times \inspace \to \Real_{\geq 0} \\ (x,y) \mapsto \Bigl(\metric(x,y)\Bigr)^p \end{cases}$ is a pseudo-metric on $\inspace$.
If $\metric$ is a metric then so is $\metricp$.
\begin{proof}
 By Lem. \ref{lem:x2p_pdNsubadd}, $x\mapsto x^p$ is pos. def. and sub-additive. Therefore, positive definiteness and the triangle inequality of $\metric$ readily extend to $\metricp$ as follows: 

\textit{Pos. def.:}
Let $x=0$. $\metricp(x,x) = \metric(x,x)^p = 0^p = 0$. If $x \neq 0$ then $k :=\metric(x,x) \neq 0$. Hence   $\metricp(x,x) = d(x,x)^p = k^p \neq 0$.

\textit{Triangle inequality:}
Choose arbitrary $x,y,z \in \inspace $. We have $\metricp(x,z) = \metric(x,z)^p \leq (\metric(x,y) + \metric(y,z) \bigr)^p \leq \metric(x,y)^p + \metric(y,z)^p = \metricp(x,y) + \metricp(y,z)$. Here, the first inequality followed from the triangle inequality of pseudo-metric $\metric$ and the second from subadditivity properties established in Lem. \ref{lem:x2p_pdNsubadd}.

\textit{Symmetry:} If $\metric$ is a metric it is symmetric. Hence, $\metricp(x,y) = \metric(x,y)^p = \metric(y,x)^p = \metricp(y,x), \forall x,y \in \inspace $ in which case $\metric$ also is symmetric.
\end{proof}
\end{lem}

Before proceeding we establish a slight generalisation of the well-known \textit{reverse triangle inequality}:

\begin{lem}[Reverse Triangle Inequality] \label{thm:revtriangle}
Let  $\inspace$ be a set and $\metric : \inspace^2 \to \Real$ a symmetric function that satisfies the triangle inequality. 
That is,  $\forall x,y,z \in \inspace: \metric (x,y) = \metric(y,x) \wedge \metric(x,z) \leq \metric(x,y) + \metric(y,z)$.

Then \[\forall x,y,z \in \inspace: \abs{\metric(x,y) - \metric(z,y)} \leq \metric(x,z).\]
\begin{proof}
For contradiction, assume 
$\abs{\metric(x,y) - \metric(z,y)}>\metric(x,z)$ for some $x,y,z \in \inspace$.
This is implies  
$
(i)\,\,\, \metric(x,y) - \metric(z,y)>\metric(x,z) 
\, \, $  or  $
\,\,  (ii) \,\,\,\, \metric(z,y)-\metric(x,y) >\metric(x,z)$.
Both inequalities contradict the triangle inequality:
$(i) \Leftrightarrow \metric(x,y)  >\metric(x,z) +\metric(z,y) $ and 
$(ii) \Leftrightarrow  \metric(z,y) > \metric(x,z) + \metric(x,y) =  \metric(z,x) + \metric(x,y)$.

\end{proof}
\end{lem}


\begin{lem}
Let $\metric$ be a (pseudo-) metric on $\inspace$. For arbitrary $s \in \inspace $ we define $\phi_s: \inspace \to \Real $ as $\phi_s: x \mapsto \metric (x,s) $.
$\phi_s $ is Lipschitz with respect to metric $\metric$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq \metric (x,y). \]
\begin{proof}
$\abs{\phi_s(x) - \phi_s(y)} = \abs{\metric(x,s) - \metric(y,s)} \stackrel{Thm. \ref{thm:revtriangle}} {\leq} \metric(x,y), \forall x,y,s \in \inspace $.
\end{proof}
\end{lem}
Finally, combining this lemma with Lem. \ref{lem:hoeldererror_metric} immediately establishes that mappings of the form $\metric(\cdot,s)^p$ are H\"older continuous with exponent $p$ ($\in (0,1]$):

\begin{thm} \label{thm:d2pmapishoelder}
Let $\metric$ be a (pseudo-) metric on set $\inspace$ and let $p \in (0,1], L \geq 0$. For arbitrary $s \in \inspace $ we define $\phi_s:\begin{cases}  \inspace \to \Real \\ x \mapsto L \, \bigl(\metric (x,s) \bigr)^p\end{cases}$.
$\phi_s $ is H\"older with exponent $p$. That is, \[\forall x,y \in \inspace : \abs{\phi_s(x) - \phi_s(y) } \leq L \, \metric (x,y)^p. \]
In particular, for any norm $\norm \cdot$ on $G$ and $s \in \inspace $, mapping $x \mapsto L \norm{x-s}^p$ is H\"older with constant $L$ and exponent $p$.

\begin{proof}
By Lem. \ref{lem:hoeldererror_metric}, $\metric^p(\cdot,\cdot)$ is a (pseudo-) metric on $\inspace$. Hence, Lem. \ref{thm:revtriangle} is applicable yielding:
$\abs{\phi_s(x) - \phi_s(y)} = L \, \abs{\metric(x,s)^p - \metric(y,s)^p} \stackrel{Lem. \ref{thm:revtriangle} } {\leq} \metric(x,y)^p, \forall x,y,s \in \inspace$. The last sentence concerning the norms follows from the fact that a mapping $(x,y) \mapsto \norm{x-y}$ defines a metric.
\end{proof}
\end{thm}



 %At first glance, the result may seem intuitive. However, it should be noted that, for $p >1$, $x \mapsto \norm{x -s}^p$ no longer is H\"older with exponent $p$. This is consistent with the well-known fact that H\"older functions with exponent $>1$ are constant functions.
%
%We conclude this section by the following theorem stating that any concatenation of H\"older continuous functions is H\"older continuous:
%
%\begin{thm} \label{thm:concathoelder}
%Let $(\statespace, \metric)$ be a metric space and $f,g : \statespace \to \statespace$ be two H\"older continuous mappings with  H\"older  constants $L_f, L_g$ and H\"older exponents $p_f,p_g$, respectively.
%Then, the concatenation $h=f \circ g: \statespace \to \statespace $ is also H\"older continuous with H\"older constant $L_h:= L_f L_g^{p_f}$ and exponent $p_h:=p_g \, p_f$.
%That is, 
%\[\forall \state,\state' \in \statespace: \metric\bigl(h(\state),h(\state')\bigr) \leq L_h \bigl(\metric(\state,\state')\bigr)^{p_h}.\]
%\begin{proof}
%%\begin{align}
%$\metric\bigl(f \circ g(\state),f\circ g(\state')\bigr) \leq L_f  \Bigl(\metric(g(\state),g(\state'))\Bigr)^{p_f}$
%$\leq L_f  \Bigl(L_g \metric(\state,\state')^{p_g}\Bigr)^{p_f}$ $= L_f L_g^{p_f}   \Bigl(\metric(\state,\state')\Bigr)^{p_g\, p_f} $ where in the first step we were using Hoelder-continuity of $f$ and in the second, we were using H\"older continuity of $g$ combined with the fact that $(\cdot)^{p_f}$ is a monotonically increasing  function. 
%
%\end{proof}
%\end{thm} 
%In conjunction with H\"older properties of the square root function established in Ex. \ref{ex:sqrtfctHoelder}, Thm. 
%\ref{thm:concathoelder} immediately yields the following result:
%\begin{cor}
%If $f: \statespace \to \statespace $ is H\"older continuous with constant $L_f$ and exponent $p_f$ then $\sqrt{f}$ also is Hoelder, having  H\"older constant $\sqrt{L_f}$ and exponent $p_f$.
%\end{cor}


==> meinzeugs.tex <==
%\documentclass[10pt]{article}
%\usepackage[usenames]{color} %used for font color
%\usepackage[utf8]{inputenc} %useful to type directly diacritic characters
%\usepackage[pdftex]{graphicx}
%\usepackage[top=2cm, bottom=2cm, left=2.2cm, right=2.1cm]{geometry}
%\usepackage[top=1.9cm, bottom=1.9cm, left=1.9cm, right=1.9cm]{geometry}
%\usepackage{setspace}
%\usepackage{floatflt}
%\usepackage{amsfonts}
%\usepackage{times}
%\usepackage[toc]{appendix}
\usepackage{subfigure}
%\usepackage{epsfig,epstopdf}
%\usepackage{url}
%\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
%\usepackage{latexsym}
%\usepackage{pstricks,pst-node,pst-grad,pst-xkey}
%\usepackage{float}
%\usepackage{multirow}
%\usepackage{cite}
%\usepackage{algorithm,algorithmic}
%\usepackage{psfrag}
%\usepackage{xy} 
%\usepackage{fancyhdr}
%\usepackage{setspace} 
%\usepackage{rotating} 
%\usepackage{citesort}
%\usepackage{cite} 
%\usepackage{verbatim} 
%\usepackage{multicol} 
%\usepackage{longtable}
%\usepackage{booktabs}
%\usepackage{pdfsync} 
%\usepackage{pstricks,pst-node,pst-grad,pst-xkey}
%\usepackage{epigraph}
\usepackage{tikz}
%\usepackage{gantt}
%\usepackage[lined,boxed,commentsnumbered]{algorithm2e}
%\usepackage{algorithm2e}
%\usepackage{color}
%\usepackage{algorithmicx}
%\usepackage[noend]{algpseudocode}


\newcommand{\stevecom}[1]{\textcolor{red} {\emph{Steve says: #1}}}
\newcommand{\jcom}[1]{\textcolor{cyan} {\emph{Jan says: #1}}}
\newcommand{\mikecom}[1]{\textcolor{yellow} {\emph{Mike says: #1}}}
% THEOREMS -------------------------------------------------------
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{conj}[thm]{Conjecture}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{ques}[thm]{\textbf{QUESTION}}
\newtheorem{ex}[thm]{\textbf{Example}}
\newtheorem{ass}[thm]{\textbf{Assumption}}
%\newenvironment{proof}{\textbf{Proof:}}{\hfill$\square$}
% MATH -----------------------------------------------------------
\newcommand{\matnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}		
\newcommand{\specnorm}[1]{\matnorm{#1}_2}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\normtop}[1]{\left\Vert#1\right\Vert^p}
\newcommand{\Ltwonorm}[1]{\left\Vert#1\right\Vert_{\Ltwo}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\abstop}[1]{\left\vert#1\right\vert^p}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\Real}{\mathbb R}
\newcommand{\Complex}{\mathbb C}
\newcommand{\integer}{\mathbb Z}
\newcommand{\nat}{\mathbb N}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\BX}{\mathbf{B}(X)}
\newcommand{\A}{\mathcal{A}}
\newcommand{\aff}[1]{\text{aff } #1}
\newcommand{\dom}[1]{\text{dom } #1}
\newcommand{\epi}[1]{\text{epi } #1}
\newcommand{\ri}[1]{\text{ri } #1}
\newcommand{\cl}[1]{\text{cl } #1}

\newcommand{\QM}[1]{\ensuremath{\mathcal{QM}(#1)} }

\newcommand{\proj}{\Pi_{\text{proj} \,}}
%-----------------------------------------
\newcommand{\argmin}{\text{argmin}}
\newcommand{\argmax}{\text{argmax}}
\newcommand{\arginf}{\text{arginf}}
\newcommand{\argsup}{\text{argsup}}

\newcommand{\sgn}{\ensuremath{\text{sgn}}}
% fuer skalare:
%\newcommand{\s}[1]{\mathfrak{#1}}
\newcommand{\s}[1]{{#1}}
% fuer vectoren:
%\newcommand{\vc}[1]{\mathbf{#1}}
\newcommand{\vc}[1]{#1}
% scalar product:
\newcommand{\Sp}[1]{\ensuremath{\mathbf{\langle} #1 \mathbf{\rangle}}}
\newcommand{\SP}[2]{\ensuremath{\mathbf{\langle} \vc{#1} \mathbf{,} \vc{#2} \mathbf{\rangle}}}
\newcommand{\SPL}[2]{\ensuremath{\mathbf{\langle} \vc{#1}\mathbf{,} \vc{#2} \mathbf{\rangle}_{L_2}}}
\newcommand{\SPLintI}[2]{\ensuremath{\int_I {#1(t)}\, {\overline{#2}(t)} \, {d\mu(t)}}}
\newcommand{\SPLtwo}[2]{\ensuremath{\mathbf{\langle} \vc{#1}\mathbf{,} \vc{#2} \mathbf{\rangle}_{\Ltwo}}}

\newcommand{\normLtwo}[1]{\ensuremath{\norm{ #1}_{\Ltwo}}}

\newcommand{\ball}[2]{\ensuremath{\mathfrak B_{\vc{#1}} \bigl( #2\bigr) }}

\newcommand{\pp}[1]{\langle #1 \rangle}

%HS:
\newcommand{\hs}[1]{\ensuremath{\mathcal{#1}}}
%operators:
\newcommand{\op}[1]{\ensuremath{ {#1}}}

\newcommand{\postmean}{\mathfrak m}

\newcommand{\dif}[2]{{\operatorname{d}\over\operatorname{d}#2}#1}
\newcommand{\pdif}[2]{{\operatorname{\partial}\over\operatorname{\partial}#2}#1}
\newcommand{\ppdif}[3]{{\operatorname{\partial^2}\over\operatorname{\partial}#2 \partial#3}#1}
%\renewcommand{\d}[1]{\operatorname{d}#1}
\renewcommand{\d}[1]{\text{ d}#1}

\newcommand{\floor}[1]{ \left\lfloor #1 \right\rfloor }
\newcommand{\ceil}[1]{ \left\lceil #1 \right\rceil }
\newcommand{\fexp}[1]{\ensuremath{\exp\bigl( #1 \bigr)}}

\newcommand{\errinp}{\varepsilon_{\text{inp}}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}

%Fourier Operator:
\newcommand{\FT}[1]{\mathcal F #1}

\newcommand{\spec}{\sigma }
\newcommand{\specrad}{\rho}

\newcommand{\radfct}{\ensuremath{\mathfrak r}}
%Koerper:
\newcommand{\field}{\mathbb F}
%nullspace:
\newcommand{\ns}{\mathcal{NS}}
\newcommand{\GP}{\mathcal {GP} }
\newcommand{\Gauss}{\mathcal {N} }
\newcommand{\gauss}{p_{\mathcal {N}} }
\newcommand{\expect}[1]{\ensuremath{ \langle#1\rangle } }
\newcommand{\cexpect}[2]{\ensuremath{ \langle#1 \, \vert \, #2\rangle } }
\newcommand{\cov}[2]{\ensuremath{ \text{cov}(#1,#2) } }
\newcommand{\covmat}[2]{\ensuremath{ \text{Cov}(#1,#2) } }
\newcommand{\var}[1]{\ensuremath{ \text{var}[#1]} }
\newcommand{\varmat}[1]{\ensuremath{ \text{Var}[#1]} }
\newcommand{\data}{\ensuremath{ \mathcal D} }

\newcommand{\varmatnormbnd}{\ensuremath{ V}}

\newcommand{\rank}{\ensuremath{ \text{ rank }}}
%parameter:
\newcommand{\pardop}{\ensuremath{\omega}}%parameter for lin. Dif OP


\newcommand{\param}{\ensuremath{\Xi}}%parameter for lin. Dif OP


\newcommand{\pardopspace}{\ensuremath{\Omega}}%parameter space for lin. OP

\newcommand{\pardi}{\ensuremath{\mathfrak p}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\pardispace}{\ensuremath{\mathfrak P}}%parameter for %inhomogeneous ODE-part / driving force

\newcommand{\state}{\ensuremath{ \vc x}} % state of the system... integral curve of the ODE/ signal.
\newcommand{\isv}{\ensuremath{ \vc s}} % interaction space vector

\newcommand{\statespace}{\ensuremath{ \mathcal X}}
\newcommand{\configspace}{\ensuremath{ \mathcal Q}}
\newcommand{\inspace}{\ensuremath{ \mathcal X}}
\newcommand{\outspace}{\ensuremath{ \mathcal Y}}
\newcommand{\taskspace}{\ensuremath{ \mathcal }}
\newcommand{\ctrlspace}{\ensuremath{ \mathcal U}}
\newcommand{\fctspace}{\ensuremath{ \mathcal F}}
\newcommand{\hilspace}{\ensuremath{ \mathcal H}}
\newcommand{\HS}{\ensuremath{ \mathcal H}}
\newcommand{\samplespace}{\ensuremath{\Omega}}
\newcommand{\freespace}{\ensuremath{ \mathfrak F}}
\newcommand{\iaspace}{\ensuremath{ \mathcal S}} %interaction space
\newcommand{\policyspace}{\ensuremath{ \mathcal P_u}} %policy space


\newcommand{\grid}{\ensuremath{  G}}

\newcommand{\tube}{\ensuremath{ \mathbb T}}

\newcommand{\Ltwo}{\ensuremath{\mathcal L_2 \,}}

\newcommand{\dW}{\ensuremath{\, \text{d}W}}

\newcommand{\linopspace}{\ensuremath{ \mathcal L}}

\newcommand{\rvc}{\ensuremath{ \vc{X}}}
\newcommand{\rv}{\ensuremath{ {X}}}

\newcommand{\indset}{\ensuremath{ \mathcal I}}
\newcommand{\indsett}{\ensuremath{ {\mathcal I_{t}}}}

\newcommand{\di}{\ensuremath{ u}} % driving force / control input

\newcommand{\agi}{\ensuremath{ \mathfrak a}} %an agent index
\newcommand{\agii}{\ensuremath{ \mathfrak r}} %index if another agent
\newcommand{\agiii}{\ensuremath{ \mathfrak q}} %index if another agent

\newcommand{\agdiam}{\ensuremath{ {\Lambda^{\agi,\agii}}} }
\newcommand{\nagi}{\ensuremath{ {\neg \agi}} }
\newcommand{\nagii}{\ensuremath{ {\neg \agii}} }
\newcommand{\nagiii}{\ensuremath{ {\neg \agiii}}} 

\newcommand{\collcritfct}{\gamma^{\agi,\agii}}

\newcommand{\nuref}{\nu_{\text{ref}}}
\newcommand{\nufb}{\nu_{\text{fb}}}

\newcommand{\xref}{x_{\text{ref}}}
\newcommand{\dxref}{\dot x_{\text{ref}}}
\newcommand{\coupleset}{\mathcal C}
\newcommand{\confl}{\text{confl}}
\newcommand{\tailrad}{\ensuremath{ {\varrho}} }

\newcommand{\maxerr}{\bar{\mathfrak v}} %max error in Hfe
\newcommand{\maxerrn}{\bar{\mathfrak N}} %maximum error norm

\newcommand{\metric}{\, \mathfrak{d}} % distance metric
\newcommand{\metricp}{\,  \tilde {d}} % distance metric
\newcommand{\Metric}[2]{\metric\bigl(#1,#2\bigr) }
\newcommand{\Metrici}[2]{\metric\bigl(#1,#2\bigr) }
\newcommand{\Metrico}[2]{\metric_\outspace\bigl(#1,#2\bigr) }
\newcommand{\Metrictop}[2]{\metric^p\bigl(#1,#2\bigr) }
\newcommand{\Metrictopi}[2]{\metric^p_\inspace\bigl(#1,#2\bigr) }
\newcommand{\Metrictopo}[2]{\metric^p_\outspace\bigl(#1,#2\bigr) }
\newcommand{\dist}{\ensuremath{ \text{dist}}} % driving force / control input

\newcommand{\predf}{\, \mathfrak{  \hat f}} % hypothesis
\newcommand{\predfn}{\, \mathfrak{  \hat f_n}} % hypothesis
\newcommand{\predfnj}{\, \mathfrak{  \hat f_{n,j}}} % hypothesis
\newcommand{\prederr}{\, \mathfrak{\hat v}} % error around hyp
\newcommand{\prederrn}{\, \mathfrak{\hat v_n}} % error around hyp
\newcommand{\prederrnj}{\, \mathfrak{\hat v_{n,j}}} % error around hyp
\newcommand{\prederrbox}{\, {\hat H}} % error around hyp

\newcommand{\noise}{{\nu}} % error around hyp


\newcommand{\hexp}{{ \alpha }}%hoelder exponent
\newcommand{\hconst}{\ensuremath{ L }}%hoelder const
\newcommand{\hestthresh}{\ensuremath{ \lambda}}
\newcommand{\ubf}{\, {\bar B}} % upper bound function
\newcommand{\lbf}{\, {\underline{B}}} % lower bound function
\newcommand{\bfset}{\mathcal B}

\newcommand{\lipset}[2]{\text{Lip}_{#2}(#1)}
\newcommand{\hoelset}[3]{\mathfrak{H}_{#2}(#1,#3)}
\newcommand{\Hoelset}{\mathfrak{H}}
%\newcommand{\coeff1}{ \underline{c}} % 
%\newcommand{\coeff2}{ \overline{c}} %

\newcommand{\errhyprec}{\mathbf  E} % upper bound function
\newcommand{\obserrhyprec}{\mathbf  O} % upper bound function

\newcommand{\obserrpar}{e} % parameter of presupposed obserr
\newcommand{\obserr}{\mathfrak e} % upper bound function on observational noise
\newcommand{\obserrbnd}{\bar{\mathfrak e}}

\newcommand{\agset}{\ensuremath{ \mathfrak A}} %set of Agents
\newcommand{\agsubset}{\ensuremath{ \mathfrak S}} %set of Agents

\newcommand{\indicator}[1]{\ensuremath{\textbf{1}_{#1}}} % indicator function

\newcommand{\collevent}{\ensuremath{\mathfrak C}}
\newcommand{\colleventtwoA}{\ensuremath{\mathfrak C^{\agi,\agii}}}
%\newcommand{\hull}{\ensuremath{\mathfrak C}}

\newcommand{\decke}{\ensuremath{\mathfrak u}}
\newcommand{\boden}{\ensuremath{\mathfrak l}}
\newcommand{\einschluss}{\ensuremath{\mathcal E^{\decke_{n}}_{\boden_{n}}}}
\newcommand{\opteinschluss}{\ensuremath{\mathcal E^*_n}}
\newcommand{\Kprior}{\mathcal K_{\text{prior}} }
\newcommand{\Kdat}{\mathcal K(D_n)}

\newcommand{\menge}[2]{\ensuremath{\{#1 \, \vert \, #2 \}}}

\newcommand{\seq}[2]{\ensuremath{\bigl(#1\bigr)_{#2}}}

%\newcommand{\diag}{\ensuremath{ \text{diag}} %set of

%\newcommand{\e}[1]{\ensuremath{\exp \Bigl(#1\Bigr) }}
\newcommand{\card}[1]{\ensuremath{\left\vert #1 \right\vert }}

\renewcommand{\Pr}{\mathrm{Pr}}
\newcommand{\sqmats}{\mathcal{M}} %set of square matrices


\renewcommand{\d}{\ensuremath{\text{ d}}}
\newcommand{\KLD}[2]{\text{KLD}(#1||#2) }

\newcommand{\erw}[2][]{
%    \ensuremath{\pmb{\mathcal{M}}^{\operatorfont{#1}}}%
     \ensuremath{\mathbb{E}_{#1} \! \left\lbrace #2 \right\rbrace}%
}


%----------- probability stuff------------------------
\newcommand{\pmeas}{\ensuremath{\mathbb P}} % probability measure


\newcommand{\embedding}{\ensuremath{\tilde \mu}} % probability measure
\newcommand{\ewx}[1]{\ensuremath{\mathbb E_x[ #1 ] }} % expected value
\newcommand{\ew}{\ensuremath{\mathbb E }} % expected value
\newcommand{\is}{\ensuremath{\mathfrak X }} % input space / index set
\newcommand{\Vol}{\ensuremath{\text{Vol}}}
\newcommand{\mslim}{\ensuremath{\text{m.s.-lim}}}
\newcommand{\msto}{\ensuremath{\stackrel{ \text{2}}{\longrightarrow}}}

% --------------------environments--------------------------------------------
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eq}[1]{\begin{equation} #1 \end{equation}}
\newcommand{\eqn}[2]{\begin{equation} #2 \label{#1}\end{equation}}
\newcommand{\dt}{\ensuremath{ \, dt \,}}
%\newcommand{\dW}{\ensuremath{ \, dW \,}}
\newcommand{\tinc}{\ensuremath{ \Delta}}

\newcommand{\tr}{\ensuremath{ \text{ tr}}}

\newcommand{\rlem}[1]{Lem. \ref {#1}} % indicator function
\newcommand{\rthm}[1]{Thm. \ref {#1}} % indicator function
%\newcommand{\rch}[1]{Ch. \ref {#1}} % indicator function
% ----------------------------------------------------------------
\newcommand{\convton}{\stackrel{n \to \infty}\longrightarrow}
\newcommand{\convto}{\longrightarrow}
\newcommand{\setconvto}{\longrightarrow}
\newcommand{\setconvtounif}{\stackrel{\text{unif}}{\longrightarrow}}
\newcommand{\bd}{\leadsto} %becomes dense relative to 
\newcommand{\bdu}{\twoheadrightarrow} %becomes dense relative to uniformly

\newcommand{\errmetric}{\mathcal E} %becomes dense relative to uniformly
\newcommand{\queryset}{I} %becomes dense relative to uniformly

%-------------- Meinzeugs Ende-----------------------------------------
